Designing, Modeling, and Optimizing Data-Intensive Computing Systems

The cost of moving data between the memory units and the compute units is a major contributor to the execution time and energy consumption of modern workloads in computing systems. At the same time, we are witnessing an enormous amount of data being generated across multiple application domains. These trends suggest a need for a paradigm shift towards a data-centric approach where computation is performed close to where the data resides. Further, a data-centric approach can enable a data-driven view where we take advantage of vast amounts of available data to improve architectural decisions. As a step towards modern architectures, this dissertation contributes to various aspects of the data-centric approach and proposes several data-driven mechanisms. First, we design NERO, a data-centric accelerator for a real-world weather prediction application. Second, we explore the applicability of different number formats, including fixed-point, floating-point, and posit, for different stencil kernels. Third, we propose NAPEL, an ML-based application performance and energy prediction framework for data-centric architectures. Fourth, we present LEAPER, the first use of few-shot learning to transfer FPGA-based computing models across different hardware platforms and applications. Fifth, we propose Sibyl, the first reinforcement learning-based mechanism for data placement in hybrid storage systems. Overall, this thesis provides two key conclusions: (1) hardware acceleration on an FPGA+HBM fabric is a promising solution to overcome the data movement bottleneck of our current computing systems; (2) data should drive system and design decisions by leveraging inherent data characteristics to make our computing systems more efficient.

==> NAPEL/sections/abstract.tex <==
 With the emergence of three-dimensional stacking, the decade-old concept of placing compute units close to the memory has become more viable. Essentially, processing right at the ``home" of data to eliminate unnecessary data movement is referred to as near-memory computing (NMC). 

To harness the power of these architectures, having a high-level performance model can offer fast turnaround times in early design stages. This paper proposes an NMC model that combines technology parameters and application specific characteristics to evaluate the performance of a workload. A statistical design of experiment (DoE) methodology is first employed to select a set of representative design points for simulation. These sampled points well represent the whole space of possible input configurations. Then, ensemble learning is leveraged to develop a model that can predict performance metrics for new unseen applications on these novel architectures. Further, this model can act as a classifier to predict whether or not should an application be offloaded to NMC cores.  The experimental results demonstrate that, by using DoE, we can extract more informative training data with a minimal number of experimental runs. Thus, we save a significant amount of simulation overhead with respect to a traditional exhaustive brute-force approach of random data selection. Besides minimizing the number of experiments, our inexpensive performance model can provide, on average, an additional 10$\times$ reduction in performance evaluation time with an error rate lower than 15\% compared to a computationally-intensive state-of-the-art NMC simulator.



==> NAPEL/sections/abstractDAC.tex <==
% Processing right at the "heart" of data to eliminate unnecessary data movement is referred to as near-memory computing (NMC). To harness the power of these architectures, having a high-level performance model can offer fast turnaround times in performance and energy estimation of an application. To this end, we propose an NMC model that combines technology parameters and application specific characteristics. A statistical design of experiment (DoE) methodology is first employed to select a set of representative design points for simulation which saves a significant amount of simulation overhead. Then, ensemble learning is leveraged to develop a model that can predict performance metrics and identify potential offload candidates on these novel architectures. Our NMC performance model can provide rapid exploration with an error rate lower than 15\% compared to a state-of-the-art NMC simulator.
\vspace{-0.1cm}

The cost of moving data between the memory/storage units and the compute units is a major contributor to the execution {time} and energy consumption of modern workloads in computing systems.
{A promising paradigm} to alleviate {this} \emph{data movement bottleneck} is near-memory computing (NMC), which consists of placing compute units close to the memory/storage units.
There is substantial {research} effort that proposes NMC {architectures and} identifies workloads that can benefit from NMC. System architects typically use simulation techniques to evaluate the performance and energy consumption of their designs. However, simulation is extremely slow, imposing long times for design space exploration.
In order to enable fast {early-stage} design space exploration of NMC {architectures}, {we need} high-level performance and energy models.

We present NAPEL, a high-level performance and energy estimation framework for NMC architectures. NAPEL leverages ensemble learning to develop a model that is based on microarchitectural parameters and application characteristics.
NAPEL training uses a statistical technique, called design of experiments, to collect representative training data efficiently. 
NAPEL provides early design space exploration $220\times$ faster than a state-of-the-art NMC simulator, {on average,} with error rates \juan{of} to 8.5\% and 11.6\% for performance and energy estimations, respectively, compared to {the} NMC simulator.
{NAPEL is also capable of making accurate predictions for previously-unseen applications.}

%A major trend to alleviate the \emph{data movement bottleneck} (i.e., the performance and energy cost of moving data between memory/storage and compute units) consists of placing compute units close to the memory/storage units, which is referred to as \emph{near-memory computing} (NMC). 
%In order to be able to carry out preliminary evaluations of NMC designs in a fast way, a high-level model for NMC is desirable. 
%%To harness the power of near-memory computing (NMC), having a high-level model can offer short turnaround times in performance estimation of applications. 
%%To this end, 
%In this work, we propose an NMC model that combines %hardware 
%microarchitectural parameters with application-specific characteristics to provide accurate performance and energy estimations. 
%An statistical design-of-experiment technique is used to select a set of design-points for simulation, which saves a significant simulation overhead. Then, ensemble learning is leveraged to develop a model that can identify potential offloading candidates. Our framework can provide rapid exploration with an error rate, on average, less than 8.5\% and 12\% for performance and energy estimation respectively compared to a state-of-the-art NMC simulator. 


% To harness the power of near-memory computing (NMC), having a high-level model can offer short turnaround times in performance estimation of applications. To this end, we propose an NMC application performance prediction framework using ensemble learning that combines hardware parameters and application-specific characteristics. A statistical design-of-experiment technique is used to select a set of design-points for simulation, which saves a significant simulation overhead. Our framework can identify potential offloading candidates and provide rapid exploration with an error-rate, on average, less than 8.5\% and 12\% for performance and energy estimation respectively compared to a state-of-the-art NMC simulator. 

==> NAPEL/sections/analyticModel.tex <==


\begin{comment}
The near-memory processing time ($\Pi_{NMC}$) is divided into time spent in executing memory ($\Pi_{memory}$) and non memory ($\Pi_{non-memory}$) instructions.  This time corresponds to the memory model and compute-model respectively in Figure~\ref{fig:model}.
\begin{align}
\Pi_{NMC}=\Pi_{memory}+\Pi_{non-memory}\label{eq:1}
\end{align}
The performance model takes  into  account  the  time to process the instructions and latency due to memory access at  different memory  levels.
\end{comment}
% \sander{You should first explain why this model is needed. It now appears out of the blue.}
A near-memory processing system is modeled similar to a 3D stacked memory (JEDEC's High Bandwidth
Memory~\cite{6757501} or Micron's Hybrid Memory Cube~\cite{7477494}). These 3D-stacked memories are composed of a logic die upon which multiple DRAM layers are stacked. Each
memory chip consists of multiple vertical
DRAM partitions, called vaults, each with its DRAM
controller in the logic layer.
% These memories utilize a packet-based protocol by means of high-speed serializer/deserializer  (SerDes)  I/O  link. The external interface supports two or four links each with different configuration speeds depending upon bus width.
% Packets are partitioned into 16-byte elements, called flits. Supported packet sizes for data payloads range from one flit (16 B) to eight flits (128 B). Each packet also carries an eight-byte header and an eight-byte tail; therefore, each request/response has an overhead of one flit~\cite{hadidi2017demystifying}.

\begin{comment}


 We assume the number of reads and writes are evenly distributed across $n_{vaults}$ vaults. 
 \begin{align}
 n_{load}=n_r/n_{vaults}\label{eq:2}\\
 n_{store}=n_w/n_{vaults}\label{eq:3}\\
 m_{total}= n_{load}+n_{store}
 \end{align}
 
  The model estimates the memory instruction time as the ratio between the number of memory access required in order to move the block of data to and from a DRAM bank and the available I/O bandwidth inside each vault ($BW_{int}$).  We assume a close-page policy, and entire block from the row-buffer of size $b_{rb}$ is consumed by the processing element \textit{pe} in its vault. The total memory access time ($\Pi_{memory}$), when all the \textit{pe}'s $(n_{pe})$ make request to their own vault is given by
  
 \begin{align}
 \Pi_{memory}=\frac{1}{n_{pe}} \displaystyle \sum_{}^{N_{vaults}}\frac{m_{total}*b_{rb}}{BW_{int}}
  \end{align}


\jgl{In Eq. 2 and 3, you divide by the number of vaults. In Eq. 5, you add the contribution of all vaults. Because you don't have n\_r and n\_w per vault, dividing and then adding is a little bit dummy.}
\end{comment}
We embed the 3D memory with processing elements (PE) which are modeled as in-order single issue cores as in other works~\cite{7284059,7429299,DBLP:journals/corr/PicorelJF16} taking into account the limited thermal and area budget in the logic layer. We assume every vault has its own PEs and operates on the data mapped onto its vaults. 

These systems are evaluated in terms of total instructions executed per cycle, $IPC(\xi)$ . The total execution time $(\Pi_{NMC})$ is calculated from core performance as
 \begin{align}
\Pi_{NMC}=\frac{I_{Total}}{IPC(\xi).f_{core}}\label{eq:1}
 \end{align}
where $f_{core}$ is the frequency of in-order cores in the logic layer and $I_{Total}$ is the total offloaded instructions. The IPC ($\xi$) of processing elements in a near-memory processing system is obtained using the approach as described in Section \ref{subsec:machine learning}.


The host system is modeled as a traditional multi-core system with a cache hierarchy. In the host system, each core has its private L1 \& L2 cache and a shared L3 cache. 3D stacked near-memory system, with embedded compute units, is connected with a host system through a serializer/deserializer (SerDes) I/O link.

\begin{comment}

To fully utilize the high bandwidth provided, coalescing of the memory access are also taken into account. 

\section{Discussion}
Given the target computational element c an the SW memtrick vector vk, the system generates the following metrics:
\bold{(i) Number of trees voting for the suggested component}
(ii) Number of trees voting for target component c
iii Influences for each SW metric

In this work,, we are interested in verifying if the model is capable to predict efficiently accelerate a kernel k with respect to its software execution.

\subsection{Black box to white box Analysis}
\end{comment}

==> NAPEL/tables/doeBACKUP.tex <==
{\footnotesize
\begin{table*}[h]
\centering

\caption{Evaluated applications. We show the input datasets, random forest (RF) tuned hyper-parameters, NAPEL training time, including simulation of the selected DoE points, tuning of RF model, and NAPEL prediction time}
\label{tab:results}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\vspace{-0.3cm}
\begin{tabular}{p{1.4cm}p{2.2cm}p{1.8cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}|llll|lllll}
\hline
\multicolumn{3}{c}{\textbf{Application}}  & \multicolumn{6}{c|}{\textbf{DoE Parameter Levels}} &\multicolumn{4}{c}{\textbf{RF Hyper-Parameters}} & \multicolumn{4}{c}{\textbf{Training/Prediction Time}}  \\ 

\rot{ Name}&\rot{ Description}&\rot{ DoE Parameters}&\rot{ Min}&\rot{ Low}&\rot{ Central}&\rot{ High}&\rot{ Max}&\rot{ Test}&\rot{$n_{estimators}$}&\rot{$min_{sample  split}$}&\rot{$min_{sample leaf}$}&\rot{$max_{depth}$} &\rot{DoE simulated}&\rot{DoE run (mins)}&\rot{Tuning (mins)} &\rot{Prediction (mins)}\\ \hline




atax    & Matrix Transpose \newline and Vector \newline Multiplication   & Dimensions    \newline Threads               &500\newline4&1250 \newline8&1500\newline16&2000\newline32&2300\newline64  &8000 \newline 32&200&10&2&30 & 9& 360 &34.9 &0.49  \\

bfs      & Breadth-first \newline Search                        &  Nodes\newline Weights    \newline Threads             &400k \newline1 \newline1 &   800k \newline2\newline9&   900k \newline4 \newline16   &1.2m \newline25   \newline32  &1.4m\newline49 \newline64   &1.0m \newline 4\newline32&600&10&1&None  & 21&320 & 34.2&0.48 \\

bp    & Back-propagation                & Layer Size  \newline Seed   \newline Threads    \newline Iterations                                   &800k \newline 2 \newline 4 \newline 1&1m \newline 4 \newline 8 \newline 3&2m \newline 5 \newline 16\newline 9 &3.5m  \newline10\newline 32\newline 16 &4m \newline 12 \newline 64 \newline 25 &1.1m \newline 5\newline 32\newline 9&1800&5&4&30   & 36&420 &43.8 &0.47\\

chol   & Cholesky \newline Decomposition                  & Dimensions             \newline Threads      &  64 \newline 4&  384 \newline 8&128 \newline 16&320 \newline 32&512 \newline 64 &2000 \newline 32&  1000 &2&1&None & 15&230 &34.9&0.49   \\

gemv &Vector Multiply \newline and Matrix\newline Addition  & Dimensions        \newline Threads                  &    500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64    &8000 \newline 32&1000&2&1&None  &15&260  &24.4 & 0.51  \\

gesu  & Scalar, Vector, and \newline Matrix Multiplication  & Dimensions       \newline Threads                  &          500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64  &8000 \newline 32&1800&10&1&40&15& 310 &36.1 &0.51   \\


gram   & Gram-Schmidt \newline Process                    & Dimension$_i$ \newline Dimension$_j$    \newline Threads                                     &  64 \newline64 \newline 4&  384 \newline384 \newline 8&128 \newline128 \newline 16&320 \newline320 \newline 32&512 \newline512 \newline 64        &2000 \newline 2000 \newline32&400 &10&1&100 &21& 300  &36.5 & 0.52  \\

kme     & K-Means \newline Clustering          & Data Size     \newline Clusters  \newline Threads                                  & 100k \newline3\newline1&300k \newline 5\newline9&700k \newline 6\newline16&    900k \newline 7\newline32&  1.2m  \newline8\newline64 & 819k  \newline 5\newline32&1400&5&2&None & 21&360    &36.9&0.55\\


lu     & LU Decomposition                          & Dimensions      \newline Threads                &196 \newline 4 &256 \newline 8&320 \newline 16&420 \newline 32 &512 \newline 64  &2000 \newline 32& 200&2&4&20    &15& 360 &37.9 & 0.51  \\


mvt     & Matrix Vector \newline Product     &Dimensions          \newline Threads            &     500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64 &2000 \newline 32& 1000&10&1&50& 15&520 &38.0 &0.54     \\
syrk     & Symmetric rank-k \newline operations              & Dimension$_i$     \newline Dimension$_j$ \newline  Threads                               & 64 \newline64 \newline4&128 \newline 128 \newline8&320 \newline 320 \newline16&    512 \newline 512 \newline 32&  640  \newline640  \newline 64      &2000 \newline 2000 \newline32&1000&10&1&50   & 21&480 &35.7 &0.51    \\


trmm      & Triangular matrix \newline multiply       & Dimension$_i$\newline Dimension$_j$              \newline Threads           &196 \newline196 \newline 4 &256 \newline256 \newline 8&320 \newline320 \newline 16&420 \newline 420 \newline32 &512 \newline512 \newline 64 &2000 \newline 2000 \newline32&200&2&4&20  &21& 300 &37.6 & 0.48  \\ 
\bottomrule

\end{tabular}

\vspace{-0.6cm}

\end{table*}
}

==> NAPEL/tables/doe_old.tex <==
\tiny{
\begin{table*}[]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{lp{2cm}p{0.7cm}p{1.1cm}llllllllllp{1cm}l}
\hline
\textbf{Name}     & \textbf{Description}   & \textbf{Variable}&\textbf{Range} & \multicolumn{5}{c}{\textbf{DoE}} &\multicolumn{4}{c}{Random Forest} & \multicolumn{2}{c}{\textbf{Simulation Cost (hours)}}  \\ 
&&&&Min&Low&Central&High&Max& n_{estimators}&min_{sample split}&min_{samples leaf}&max_{depth}& All Configuration &DoE \\ \hline

3MM      & 3 Matrix \newline Multiplication                   & NI \newline NJ \newline NK \newline NL \newline NM                 & 128-1024 \newline 128-1024 \newline 128-1024 \newline 128-1024 \newline    128-1024                             &64&128&448&768&1024    &   400+ & 26 \\
ATAX     & Matrix Transpose \newline and Vector              & NX \newline NY              &     500-4000 \newline 500-4000  &500&1250&1500&2000&2300  & 600+ & 6  \\

CHOLESKY & Cholesky \newline Decomposition                   & N                  &      128-1024 &   -                      &-&-&-& & 400+ & 3  \\
GEMM     & Matrix Multiply                          &  NI \newline NJ \newline NK                 &        128-640 \newline 128-640 \newline 128-640     &64&128&448&768&1024     & 100+ & 2   \\
GESUMMV  & Scalar, Vector, and \newline Matrix Multiplication & N                  &    500-4000              &              &-&-&-&-    & 600+ & 2     \\
GRAMSCHM & Gram-Schmidt \newline Process                     & NI \newline NJ                 & 128-512 \newline 128-512                            &  64&  384&128&320&512        & 150+ & 5    \\
LU       & LU Decomposition                         & N                & 128-1024                               &-&-&-&-&-   & 400+ & 3    \\
MVT      & Matrix Vector \newline Product and                & N                  &      500-400           &               &&-&-& & 600+ & 2.5     \\
SYR2K    & Symmetric rank -2k \newline operations            & NI \newline NJ                  &  128-1024 \newline 128-1024                               & &&&    &     &   400+ & 5    \\
SYRK     & Symmetric rank -k \newline operations             & NI \newline NJ                   &         128-1024 \newline 128-1024                      &    &&&&         & 400+ & 8     \\
TRMM     & Triangular matrix \newline multiply               & NI                  &  128-1024            &                  &-&-&-&  & 150+ & 3   \\ \hline

\end{tabular}
\caption{PolyBench workload description with parameters for DoE,possible input range, possible input configurations and configurations using DoE }
\label{tab:results}
\end{table*}
}

==> NAPEL/tables/doe_old2.tex <==

\begin{table*}[]
\centering

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{p{1.5cm}p{0.9cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}llllll}
\hline
\textbf{Name}      & \textbf{Variable} & \multicolumn{5}{c}{\textbf{Application Input}} &\multicolumn{4}{c}{Random Forest Parameters} & \multicolumn{2}{c}{\textbf{Simulation Cost (hours)}}  \\ 

&&\rot{Min}&\rot{Low}&\rot{Central}&\rot{High}&\rot{Max}&\rot{$n_{estimators}$}&\rot{$min_{sample  split}$}&\rot{$min_{sample leaf}$}&\rot{$max_{depth}$}&\rot{Total} &\rot{DoE} \\ \hline

3MM                        & NI \newline NJ \newline NK \newline NL \newline NM  \newline Threads                                       &64 \newline 64 \newline 64 \newline 64 \newline 64 \newline 4 &128 \newline 128 \newline 128  \newline 128 \newline 128 \newline 8  &448 \newline 448 \newline 448 \newline 448 \newline 448 \newline 16  &768 \newline 768 \newline 768 \newline 768 \newline768 \newline32 &1024 \newline 1024 \newline 1024 \newline 1024 \newline 1024 \newline 64  &1800&5&4&30   &   400+ & 26 \\


ATAX      & NX \newline NY     \newline Threads               &500\newline500\newline4&1250 \newline1250\newline8&1500\newline1500\newline16&2000\newline2000\newline32&2300\newline2300\newline64  &200&10&2&30 & 600+ & 6  \\


CHOLESKY                    & N             \newline Threads     &         -                      &-&-&-& &1000 &2&1&None&  400+ & 3  \\


GEMM                            &  NI \newline NJ \newline NK         \newline Threads                 &64\newline64\newline64\newline4&128\newline128\newline128\newline8&448\newline448\newline448\newline16&768\newline768\newline768\newline32&1024\newline1024\newline1024\newline64    &600&10&1&None &   100+ & 2   \\
GEMVER   & N         \newline Threads                  &              &-&-&-&-    &1000&2&1&None  & 600+ & 2     \\

GESUMMV   & N         \newline Threads                  &              &-&-&-&-    &1800&10&1&40  & 600+ & 2     \\


GRAMSCHM                      & NI \newline NJ     \newline Threads                                     &  64&  384&128&320&512        &400 &10&1&100&  150+ & 5    \\


LU                              & N      \newline Threads                &-&-&-&-&-  &200&2&4&20   & 400+ & 3    \\


MVT         & N           \newline Threads            &               &&-&-& & 1000&10&1&50&  600+ & 2.5     \\


SYR2K              & NI \newline NJ      \newline Threads                                    & &&&    &      &1400&5&2&None &   400+ & 5    \\


SYRK                  & NI \newline NJ    \newline Threads                                &    &&&&        &1000&10&1&50   & 400+ & 8     \\


TRMM           & NI             \newline Threads           &-&-&-& & &200&2&4&20  & 150+ & 3   \\ \hline

\end{tabular}
\caption{PolyBench workload description with parameters for DoE,possible input range, possible input configurations and configurations using DoE }
\label{tab:results}
\end{table*}


==> NAPEL/tables/results.tex <==


\begin{table*}[!t]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{llllp{0.15\linewidth}ll}
\hline
Name                             & Performance Estimation Error\% & Simulation Cost & Model Cost \\ \hline
2MM          &                                &           &       \\
3MM           &                                &           &       \\
ATAX          &                                &           &       \\
BICG          &                                &           &       \\
Cholesky        &                                &           &       \\
GEMM           &                                &           &       \\
GESUMMV         &                                &           &       \\
GRAMSCHM       &                                &           &       \\
LU            &                                &           &       \\
MVT           &                                &           &       \\
SYR2K         &                                &           &       \\
SYRK             &                                &           &       \\
TRMM           &                                &           &       \\ \hline
\end{tabular}
\caption{List of workloads evaluated with estimated error and  run time (cost) compared to the simulator }
\label{tab:napel/results}
\end{table*}

==> NAPEL/tables/results_old.tex <==


\begin{table*}[ht]
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{llllp{0.15\linewidth}ll}
\hline
Name     & Description                              & Variable Parameters & DoE Runs & Performance Estimation Error\% & Simulation Cost & Model Cost \\ \hline
2MM      & 2 Matrix Multiplication                  & 4           & 25       &                                &           &       \\
3MM      & 3 Matrix Multiplication                  & 5           & 43       &                                &           &       \\
ATAX     & Matrix Transpose and Vector              & 2           & 9        &                                &           &       \\
BICG     & BiCG Sub Kernel of Linear Solver         & 2           & 9        &                                &           &       \\
Cholesky & Cholesky Decomposition                   & 1           & 6        &                                &           &       \\
GEMM     & Matrix Multiply                          & 3           & 15       &                                &           &       \\
GESUMMV  & Scalar, Vector and Matrix Multiplication & 1           & 6        &                                &           &       \\
GRAMSCHM & Gram-Schmidt Process                     & 2           & 9        &                                &           &       \\
LU       & LU Decomposition                         & 1           & 6        &                                &           &       \\
MVT      & Matrix Vector Product and                & 1           & 6        &                                &           &       \\
SYR2K    & Symmetric rank -2k operations            & 2           & 9        &                                &           &       \\
SYRK     & Symmetric rank -k operations             & 2           & 9        &                                &           &       \\
TRMM     & Triangular matrix multiply               & 1           & 6        &                                &           &       \\ \hline
\end{tabular}
\caption{List of workloads evaluated, parameters for DoE, resulting experimental run, estimated error and  run time (cost) compared to the simulator }
\label{tab:napel/results}
\end{table*}

==> NERO/algorithms/scaling.tex <==
\begin{algorithm}
 \caption{AFU scaling prediction model}
 \label{algo:fpgaFamily}
\SetAlgoLined\DontPrintSemicolon
 \SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
       
\KwResult{Pareto optimal $(\omega,\mu)$ }
initialization\;
\While{$FPGA_{device}$}{
    \textbf{Step 1: Empirical characterization per AFU}\;
    \Input{ $\omega=\omega_{min},\mu=\mu_{min}$}
    \Output{$\overrightarrow{\eta_{AFU}}$, $\rho_{AFU}$}
   High-level-synthesis with Vivado HLS \&\;
   FPGA implementation with Vivado\;
    \textbf{Step 2: Performance Modeling}\;
    \Input{$\overrightarrow{\eta_{AFU}},\rho_{AFU}$}
    \Output{Pareto optimal $(\omega,\mu)$}
    \For{$\omega=\omega_{min}:\omega_{max}$}{
     \While{$\eta_{\{BRAM or DSP or FF or LUT\}}$ != $\eta_{max \{BRAM or DSP or FF or LUT\}}$  }{
        % \While{$\eta_{max,BRAM}\;\eta_{max,DSP}\;\eta_{max,FF}\;\eta_{max,LUT}\;\eta_{max,URAM}$ }{
        {\footnotesize $\hat \rho=a_{n}\times\mu^{n}(\omega)+a_{n-1}\times\mu^{n-1}(\omega)+...+a_{1}\times\mu(\omega)+a_{0}$\;} \label{line:polyEquation}
        %   $\hat \rho=a\times\mu^{2}(\omega)+b\times\mu(\omega)+c$ \; \label{line:polyEquation}
            % $\hat \rho(\omega,\mu)=a\times\rho^{2}(\omega,\mu)+b\times\rho(\omega,\mu)+c$ \; \label{line:polyEquation}
           {\footnotesize  $\mu \gets \mu + 1 $}
            }
        maximize ($ \hat\rho$)\;
    }
}
\end{algorithm}

==> NERO/tables/fpgaFamily.tex <==
\begin{table*}[h]
  \caption{Prediction results for different CAPI 2.0 enabled boards across FPGA families. }
    \label{tab:nero/fpgaFamily}
   \vspace{-0.2cm}
    \begin{threeparttable}
     \begin{center}
\scalebox{1}{
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{FPGA Board} & \multirow{2}{*}{FPGA Device} & \multicolumn{5}{c|}{Utilization\%} & \multirow{2}{*}{Window} & \multirow{2}{*}{AFU} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Performance\\ (GFLOP/s)\end{tabular}} & \multirow{2}{*}{Energy Impr.}  \\ \cline{3-7}
                             &                              & BRAM  & DSP  & FF  & LUT  & URAM &                         &                      &                                                                                 &                                                                            \\ \hline
                             
ADM-PCIE-9V3\tnote{*} & XCVU3P-2 &  71 &  66 &  49&79 & 58  &$8\times8\times8$ & 16 &  120.1 &  18.1$\times$       \\ \hline

ADM-PCIE-KU3\tnote{*} & XCKU3P-2   & 70      &    33  & 61    & 96     & 70     &  $16\times16\times16$  & 4  &    48.9    &9.3$\times$      \\ \hline
Semptian NSA121B  & XCKU060    &   55    & 49     &   73  &  79    &  -    &$8\times8\times8$   & 8    & 83.5     &20.6$\times$     \\ \hline
ADM-PCIE-8K5  & XCKU115   &    59   &  58    & 81    & 77     &   -   &   $8\times8\times8$ & 16      &  162.7     &   19.2$\times$        \\ \hline


% ADM-PCIE-9V3\tnote{*} \tnote{+} & XCVU3P-2 &  71 &  66 &  49&79 & 58  &$8\times8\times8$ & 16 &  120.1 &  18.1$\times$       \\ \hline

% ADM-PCIE-KU3\tnote{*} \tnote{+} & XCKU3P-2   & 70      &    33  & 61    & 96     & 70     &  $16\times16\times16$  & 4  &    48.9    &9.3$\times$      \\ \hline
% Semptian NSA121B\tnote{$\dagger$}  & XCKU060    &   55    & 49     &   73  &  79    &  -    &$8\times8\times8$   & 8    & 83.5     &20.6$\times$     \\ \hline
% ADM-PCIE-8K5\tnote{+}  & XCKU115   &    59   &  58    & 81    & 77     &   -   &   $8\times8\times8$ & 16      &  162.7     &   19.2$\times$        \\ \hline


\end{tabular}}
\end{center}
% \begin{tablenotes}[para,flushleft]\footnotesize
%  \qquad \qquad \qquad  *URAM memory is available only in  Ultrascale\tnote{+} families \qquad  \tnote{+} Implemented and estimated  \qquad \tnote{$\dagger$} Estimated (not currently \newline \tab \tab   \qquad\qquad\qquad\qquad\qquad\qquad\qquad \qquad available at our nodes)
\begin{tablenotes}[para,flushleft]\footnotesize
 \qquad \qquad \qquad  *URAM memory is available only in  Ultrascale\tnote{+} families 
%  \qquad  \tnote{+} Implemented and estimated  \qquad \tnote{$\dagger$} Estimated (not currently \newline \tab \tab   \qquad\qquad\qquad\qquad\qquad\qquad\qquad \qquad available at our nodes)
 \end{tablenotes}
\end{threeparttable}
\vspace{-0.4cm}
\end{table*}


%KU3 belongs from US+ but has half the amount of resoursce as 9v3


==> NMC_review/sections/future.tex <==
\section{Open Issues and Future Directions}
\label{sec:futuredirections}
Based on our analysis of many existing NMC architectures, we identify the following key
topics for future research that we regard as essential to unlock the full potential of processing close to memory:
\begin{itemize}
   
\item It is unclear which emerging memory technology best supports near-memory architectures; for example, much research is going into new 3D stacked DRAM and non-volatile memories such as PCM, ReRAM, and MRAM. The future of these new technologies relies heavily on advancements in endurance, reliability, cost, and density.

\item 3D stacking also needs unique power and thermal solutions, as traditional heat sink technology would not suffice if we want to add more computation close to the memory. Most of the proposed architectures do not take into account the strict power budget of 3D stacked memories, which limits the architecture's practicality.

\item DRAM and NVM have different memory attributes. A hybrid design can revolutionize our current systems. Huang et al.~\cite{qian2015study} evaluated a 3D heterogeneous storage structure that tightly integrates CPU, DRAM, and a flash-based NVM to meet the memory needs of big data applications, i.e., larger capacity, smaller delay, and wider bandwidth. Processing near heterogeneous memories is a new research topic with high potential (could provide the best of both worlds), and in the future, we expect much interest in this direction.

\item Most of the evaluated architectures focus on the compute aspect. Few architectures focus on providing coherency and virtual memory support. As highlighted in Section~\ref{sec:interondpcachevirtual}, lack of coherency and virtual support makes programming difficult and obstructs the adoption of this paradigm. 

\item More quantitative exploration is required for interconnect networks between the near-memory compute units and also between the host and near-memory compute system. The interplay of NMC units with the emerging interconnect standards like GenZ~\cite{genZdram}, CXL~\cite{cxlwhitepaper}, CCIX~\cite{ccixwhitepaper} and OpenCAPI~\cite{stuecheli2018ibm} could be vital in improving the performance and energy efficiency of big data workloads running on NMC enabled servers.

\item At the application level, algorithms need to provide code and data co-location for energy efficient processing. For example, in case of HMC algorithms should avoid excessive movement of data between vaults and across different memory modules. Whenever it is not possible to avoid an inter-vault data transfer, lightweight mechanisms for data migration should be provided.

\item The field requires a generic set of open-source tools and techniques for these novel systems, as often researchers have to spend a significant amount of time and effort in building the needed simulation environment. Application characterization tools should add support for static and dynamic decision support for offloading processing and data to near-memory systems. To assist in the offloading decision, new metrics are required that could assess whether an application is suitable for these architectures. These tools could provide region-of-interest (or hotspots) in an application that should be offloaded to an NMC system. Besides, a standard benchmark set is missing to gauge different architectural proposals in this domain.


\end{itemize}

==> NMC_review/sections/introduction.tex <==
Over the years, memory technology has not been able to keep up with advancements in processor technology in terms of latency and energy consumption, which is referred to as the \textit{memory wall}~\cite{Wulf1995}. Earlier, system architects tried to bridge this gap by introducing memory hierarchies that mitigated some of the disadvantages of off-chip DRAMs. However, the limited number of pins on the memory package is not able to meet today's bandwidth demands of multicore processors. Furthermore, with the demise of Dennard scaling~\cite{1050511}, slowing of Moore's law, and dark silicon computer performance has reached a plateau~\cite{6175879}. 

At the same time, we are witnessing an enormous amount of data being generated across multiple areas like radio astronomy, material science, chemistry, health sciences etc~\cite{nair2015active}. In radio astronomy, for example, the first phase of the Square Kilometre Array (SKA) aims at processing over 100 terabytes of raw data samples per second, yielding of the order of 300 petabytes of SKA data products annually~\cite{6898703}. The SKA currently is in the design phase with anticipated construction in South Africa and Australia in the first half of the coming decade. These radio-astronomy applications usually exhibit massive data parallelism and low operational intensity with a limited locality. On traditional systems, these applications cause frequent data movement between the memory subsystem and the processor that has a severe impact on performance and energy efficiency. Likewise, cluster computing frameworks like Apache Spark that enable distributed in-memory processing of batch and streaming data also exhibit those mentioned above behaviour~\cite{awan2016micro,javed2015performance,awan2016node}. Therefore, a lot of current research is being focused on coming up with innovative manufacturing technologies and architectures to overcome these problems. 

Today's memory hierarchy usually consists of multiple levels of cache, the main memory, and storage. The traditional approach is to move data up to caches from the storage and then process it. In contrast, near-memory computing (NMC) aims at processing close to where the data resides. This data-centric approach couples compute units close to the data and seek to minimize the expensive data movements. Notably, three-dimensional stacking is touted as the true enabler of processing close to the memory. It allows the stacking of logic and memory together using through-silicon via's (TSVs) that helps in reducing memory access latency, power consumption and provides much higher bandwidth~\cite{6242474}. Micron's Hybrid Memory Cube (HMC)~\cite{7477494}, High Bandwidth Memory (HBM)~\cite{6757501} from AMD and Hynix, and Samsung's Wide I/O~\cite{6025219} are the competing products in the 3D memory arena. 

\begin{figure*}[t]
\centering
\includegraphics[bb=1 6 730 238,width=1\textwidth]{NMC_review/img/allsystems_final.pdf}
\caption{Classification of computing systems based on working set location, which is referred to as a working set~\cite{7092668}. Prior systems were based on a CPU-centric approach where data is moved to the core for processing (Figure 1 (a)-(c)), whereas now with near-memory processing (Figure 1 (d)) the processing cores are brought to the place where data resides. Computation-in-memory (Figure 1 (e)) further reduces data movement by using memories with compute capability (e.g. memristors, phase change memory).
\label{fig:nmc_review/allsystems}}
\end{figure*}


\begin{figure}[!hb]
\centering
\includegraphics[width=0.6\linewidth]{NMC_review/img/NMCtaxonomy_final.pdf}
\caption{Processing options in the memory hierarchy highlighting the conventional compute-centric and the modern data-centric approach
\label{fig:nmc_review/taxonomy}}
\end{figure}

Figure~\ref{fig:nmc_review/allsystems} depicts the system evolution based on the information referenced by a program during execution, which is referred to as a working set~\cite{7092668}. Prior systems were based on a CPU-centric approach where data is moved to the core for processing (Figure 1 (a)-(c)), whereas now with near-memory processing (Figure 1 (d)) the processing cores are brought to the place where data resides. Computation-in-memory (Figure 1 (e)) paradigm aims at reducing data movement completely by using memories with compute capability (e.g. memristors, phase-change memory (PCM)).

The paper aims to analyze and organize the extensive body of literature related to the novel area of near-memory computing. Figure~\ref{fig:nmc_review/taxonomy} shows a high-level view of our classification that is based on the level in the memory hierarchy and further split into the type of compute implementation (programmable, fixed-function, or reconfigurable). Conceptually the approach  of near-memory computing can be applied to any level or type of memory to improve the overall system performance. In our taxonomy, we do not include magnetic disk-based systems as they can no longer offer timely response due to the high access latency and a high failure rate of disks~\cite{7097722}. Nevertheless, there have been research efforts towards providing processing capabilities in the disk. However, it was not adopted widely by the industry due to the marginal performance improvement that could not justify the associated cost~\cite{Keeton:1998:CID:290593.290602,Riedel:1998:ASL:645924.671345}. Instead, we include emerging non-volatile memories termed as storage-class memories (SCM)~\cite{7151782} which are trying to fill the latency gap between DRAMs and disks. Building upon similar efforts~\cite{siegl2016data, ghose2018enabling}, we make the following contributions:


\begin{itemize}
    \item We analyze and organize the body of literature on near-memory computing under various dimensions.
    \item We provide guidelines for design space exploration.
    \item We present our near-memory system outlining application characterization and compiler framework. Also, we include an analytic model to illustrate the potential of near-memory computing for memory intensive application with a comparison to the current CPU-centric approach.
    \item We outline the directions for future research and highlight current challenges.
\end{itemize}

This work extends our previous work~\cite{629e227db47e4e89b539b0e072ecce08} by including our approach to near-memory computing (Section~\ref{sec:nmc_review/system}).  This outlines our application characterization and compilation framework. 
Furthermore, we evaluate more recent work in the NMC domain and provide new insights and research directions. The remainder of this article is structured as follows: Section~\ref{sec:nmc_review/background} provides a historical overview of near-memory computing and related work. Section~\ref{sec:nmc_review/classificationmodel} outlines the evaluation and classification scheme for NMC at main memory (Section~\ref{sec:nmc_review/procmainmem}) and storage class memory (Section~\ref{sec:nmc_review/procstorage}).  Section~\ref{sec:nmc_review/interondpcachevirtual} highlights the challenges with cache coherence, virtual memory, the lack of programming models, and data mapping schemes for NMC. In Section~\ref{sec:nmc_review/modelingmethod}, we look into the tools and techniques used to perform the design space exploration for these systems. This section also illustrates the importance of application characterization. Section~\ref{sec:nmc_review/system} presents our approach to near-memory computing. Additionally, we include a high-level analytic approach with a comparison to a traditional CPU-centric approach. Finally, Section~\ref{sec:nmc_review/futuredirections} highlights the lessons learned and future research directions.


\input{NMC_review/tables/classification.tex}

==> NMC_review/sections/system.tex <==
\section{Practicalities of Near-Memory Computing}
\label{sec:system}
In this section, we describe our approach
to solve some of the issues related to NMC. Besides the design of the near-memory computing platform itself, we are focusing on how such a hybrid system can be effectively programmed to maximize performance and minimize power consumption. Additionally, we are extensively analyzing applications to assess essential application metrics for these devices. The various components of our framework are outlined below.

\subsection{NMC Architecture}
Figure~\ref{fig:targetplatform} depicts an abstract view of our reference computing platform that we consider. We modeled a multi-core host system interconnected to an external stacked near-memory system via high speed interconnect. In this model, the near-memory compute units are modeled as low power cores (Table~\ref{tab:systemparameters}), which are placed in the logic layer of the 3D stacked DRAM. For the 3D stacked memory, we consider a 4-GB HMC like design, with 8 DRAM layers. Each DRAM layer is split into 16 dual banked partitions with four vertical partitions forming a vault. Each vault has its vault controller. 


\begin{figure}[h]
\centering
\includegraphics[width=21pc]{NMC_review/img/systemNMC53_final.pdf}
\caption{Overview of a system with NMC capability~\cite{NAPEL}. On the right, an abstract view of application code with kernels {that are} offloaded to NMC
\label{fig:targetplatform}}
\end{figure}

%}
% \subsection{Platform Agnostic Application Characterization for NMC}
% \label{subsec:platform-agnostic-NMC}

% We define the following microarchitecture independent metrics to characterize the applications from NMC perspective and identify the kernels that can potentially benefit from NMC. 

% \begin{itemize}
%     \item \textbf{Memory Entropy:} It measures the randomness of the memory accesses. Yen~et~al.~\cite{yen2008notary} devise the formula by applying Shannon's definition to the memory addresses. The higher the memory entropy, the higher the miss ratio. Hence, an application with higher entropy can benefit from NMC.  
%     \item \textbf{Spatial Locality:} It measures the probability of accessing nearby memory locations. Spatial Locality is derived from data temporal reuse, which is the number of unique addresses accessed since the last reference of the requested data. We use the formula proposed by Gu~et~al.~\cite{gu2009component} to calculate spatial locality score.     
%     \item \textbf{Data-Level Parallelism:} It measures the average possible vector length and is relevant for NMC when employing specific SIMD processing units as near-memory computation units. It is derived from instruction-level parallelism (ILP) score per opcode such as load, store, etc. This metric represents the number of instructions with the same opcode that could run in parallel, thus expressing the DLP per opcode. We compute the average value of DLP using the weighted sum over all opcodes of the DLP per code. 
%     \item \textbf{Basic-block level Parallelism:} A basic block is the smallest component in the LLVM intermediate representation (IR) that can be parallelized. If an application has high basic-block level parallelism, it can benefit from multiple processing units.

% \end{itemize}

% We extend an open-source platform-independent software analysis tool (PISA)~\cite{anghel2016instrumentation} with the above-listed metrics and use it to analyze multi-thread applications from NMC perspective. As an example, we show in Figure~\ref{fig:pisa-nmc} the analysis result of two applications from PolyBench/C 4.1~\cite{pouchet2012polybench}, which is a collection of standard kernels. Each kernel is a single file that can be tuned at compile time. In Figure~\ref{fig:pisa-nmc} we show the characterization of two applications having opposite memory behavior: \texttt{Gramschmidt} and \texttt{Jacobi-1d}.
% Figure~\ref{fig:spatial} presents the spatial locality values for different pairs of cache line sizes. For instance, 8-16B means spatial locality doubling the cache line size from 8B to 16B. In the figure, the total spatial locality is the weighted sum of all the values (see \cite{corda2019scopes}). Figure~\ref{fig:spatial} shows, for different cache size configurations, how \texttt{Gramschmidt} has significantly lower spatial locality than \texttt{Jacobi-1d}. This lower locality can be attributed to non-regular memory accesses (e.g., diagonal accesses in a matrix). Figure~\ref{fig:entropy} presents memory entropy for different address granularity. The bit reductions mean reduction in the number of bits of the addresses considered to compute the entropy. The bit reduction reflects as using bigger cache line sizes and could be used to perform further spatial locality analysis (see \cite{corda2019scopes,corda2019DSD}). Figure~\ref{fig:entropy} highlights the lower memory entropy of \texttt{Jacobi-1d} compared to \texttt{Gramschmidt} due to localized memory accesses.
% A detailed study on workload characterization from NMC perspective using above mentioned architecture-independent metrics and representative benchmarks are presented in \cite{corda2019scopes,corda2019DSD}.


% \begin{figure}[] 
%     \centering
%     \subfloat[Spatial Locality]{%
%         \includegraphics[width=8.5cm,trim={2.1cm 2cm 4.4cm 1.8cm},clip]{NMC_review/img/spat_jr_final.eps}%
%         \label{fig:spatial}%
%         }%
%     \hfill%
%     \subfloat[Memory Entropy]{%
%         \includegraphics[width=8.5cm,trim={2.1cm 2cm 4.4cm 1.8cm},clip]{NMC_review/img/entr_jr_final.eps}%
%         \label{fig:entropy}%
%         }%
%     \caption{Spatial Locality and Memory Entropy characterization for two applications from PolyBench 
%     \label{fig:pisa-nmc}}
% \end{figure}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.85\linewidth]{NMC_review/img/JournalPaper_final.pdf}
%     \caption{Proposed compilation flow for the system with NMC capabilities depicted in Figure~\ref{fig:targetplatform}. 
%     }
%     \label{fig:my_label}
% \end{figure*}

% \subsection{Compilation and Programming Model}
% The compiler support has been built on top of our previous work~\cite{zinenko:hal-01965599} and is completely integrated into a state-of-the-art loop optimizer~\cite{grosser2012polly}. Similar to previous works~\cite{akin2015data, 7856642}, we assume our near-memory accelerators expose a library of memory-bound kernels via an application programming interface (API). We provide compiler support to automatically, and transparently for the application,  detect such kernels and call the proper accelerator routine. The compilation flow (Figure~\ref{fig:my_label}) follows a classical compiler design with a front-end, a mid-level optimizer, and target-specific back-ends. We extend this design embedding a state-of-the-art pattern matching framework in the mid-level optimizer. 

% Briefly, the compilation flow is as follow: We start from an application written in C/C++; the front-end is responsible for lowering the application code to an intermediate representation. For our work, we use the LLVM compiler infrastructure and exploit its intermediate representation (LLVM-IR). At IR level, we rely on a state-of-the-art polyhedral optimizer~\cite{grosser2012polly} to extract compute kernels and obtain for each of them a mathematical description based on Presburger\cite{10.1007/978-3-642-15582-6_49} sets. On top of this mathematical model, our pattern matching framework is used to match and swap kernels with accelerator-specific run-time calls. Once the run-time calls have been introduced, we rely again on the polyhedral optimizer to lower the mathematical abstraction back to LLVM-IR. During the latest stages of compilation, the run-time accelerator specific libraries are linked with the application binary. With our approach, legacy code can exploit, in a completely transparent way for the user, near-memory acceleration without any change on the application side. 



% \subsection{Early Design Stage Modeling}
% We make use of a first-order analytic model to evaluate the benefit of using near-memory processing in our system in the early design stage. As mentioned in Section~\ref{subsec:performanceevaluation}, a high-level analytic model abstract the detailed micro-architecture. Hence, this approach makes our analytical model more generic and provides quick insights.



% Our analytic model incorporates evaluation methodology as described in Figure~\ref{fig:methodology}. To see the potential of computing close to the memory and when it is useful to follow a data-centric approach, we make a comparison of a CPU-centric approach consisting of a multi-core system and compare it to a data-centric approach which has near-memory processing units in the logic layer of HMC like 3D stacked. In the multi-core system, each core has its L1 cache and a shared L2 cache.  In the near-memory system, we assume certain parts of the computation called NMC-kernels would be offloaded to the near-memory compute units, and the other parts will be executed in the host system. The number of vaults inside the HMC and external interconnects links are kept as varying parameters which have an impact on internal and the external bandwidth of the 3D memory respectively.

% \begin{comment}

% \begin{figure*}
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.5]{img/results/delay.png}
%   \caption{Normalized Delay}
%   \label{fig:delay}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.5]{img/results/energy.png}
%   \caption{Normalized Energy}
%   \label{fig:energy}
% \end{subfigure}
% \caption{Performance and Energy Comparison between multi-core and NMC with a host system using high-level analytic model}
% \label{fig:results}
% \end{figure*}


% \end{comment}



% \begin{figure*}[h]
% \centering
% \subfloat[Normalized Delay]{\includegraphics[width=9cm]{NMC_review/img/delay3_final.png}%img/results/delay.png}
% \label{fig:delay}}
% \subfloat[Normalized Energy]{\includegraphics[width=9cm]{NMC_review/img/energy3_final.png}%img/results/energy.png}
% \label{fig:energy}}
% \caption{Performance and energy comparison between multi-core and an NMC system, which is attached to a host system, using high-level analytic model}
% \label{fig:results}
% \end{figure*}



% \textit{Performance Calculation:} The model estimates the execution time as the ratio between the number of memory accesses required to move the block of data to and from the I/O system and the available I/O bandwidth of each memory subsystem. The execution time takes into account the time to process the instructions $\Pi_{non-memory}$ and latency due to memory access $\Pi_{memory}$ (Table~\ref{tab:systemparameters}).

% \begin{comment}

% \begin{equation}
% \label{eq:1}
% \begin{split}
% n_{load}=n_r/n_{vaults}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:2}
% \begin{split}
% n_{store}=n_w/n_{vaults}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:3}
% \begin{split}
% m_{total}= n_{load}+n_{store}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:4}
% \begin{split}
% \Pi_{memory}=\frac{1}{n_{pe}} \displaystyle \sum_{}^{N_{vaults}}\frac{m_{total}*b_{rb}}{BW_{int}}
% \end{split}    
% \end{equation}

% \end{comment}


% %\todo[author=Gagan, inline]{Add performance model equations here}


% \textit{Energy Calculation:} We build a power model for both CPU-centric and a near-memory system by taking into account dynamic as well as static energy. Dynamic energy is the product of the energy per memory access and the number of memory accesses at each level of the memory hierarchy.  It is assumed to scale linearly with utilization. Static energy is estimated as the product of time and static power for each component. It is scaled based on the number of cores and the cache size. 
    
% For modeling the HMC, we refer to~\cite{6242474} and~\cite{6844483}. We consider energy per bit of 3.7 pJ/b for accessing the DRAM layers and 1.5 pJ/b for the operations and data movements in the HMC logic layer. A static power of 0.96 W is assumed~\cite{6844483} to model the additional components in the logic layer.

% %\todo[author=Gagan, inline]{Add energy model equations here}


% \textit{Performance and Energy Exploration:} 
% We vary the cache miss rate, which encapsulates application characteristics, both at L1 and L2 level to see the impact it has on the performance of the entire system. In case of a near-memory system, we consider the scenario when all accesses are done to the different vaults inside the HMC memory, which can exploit the inherent parallelism offered by the 3D memory. In Figure~\ref{fig:results}, the x and y-axis represent the miss rate at L1 and L2, respectively. Results in Figure~\ref{fig:results} are normalized to NMC+host system. 

% Based on our evaluation, we make the following three observations. First, in case of performance and energy, we can see a similar trend, i.e., if the miss rate (L1 and L2) increases the multi-core system performance degrades compared to the NMC systems. This degradation is because of the increase in data movement. The data has to be fetched from the off-chip DRAM. Second, if the CPU does not reuse the data brought into the caches, the use of caching becomes inefficient. Third, the application (or function) with low locality can take advantage of the near-memory approach, whereas the other application (or function) with high locality would benefit more from the traditional approach. 
 


==> PhD_Thesis_Updated_arxiv (1)/CV.tex <==
\thispagestyle{plain}

\chapter*{Curriculum Vitae}
% \renewcommand{\chaptername}{Biography}
\addcontentsline{toc}{chapter}{Curriculum Vitae}

Gagandeep was born in Chandigarh, India, in 1992. He received a joint M.Sc. degree with distinction in Integrated Circuit Design from Technische Universität München (TUM), Germany, and Nanyang Technological University (NTU), Singapore in 2017. He joined Eindhoven University of Technology, Netherlands, in 2017 to pursue a Ph.D. degree as a part of the Marie Sklodowska-Curie EID (Ph.D.) Program under the supervision of Prof. Henk Corporaal. % for  the project ``Near-Memory Computing''  (Project ID: 676240).  
From June 2018 to January 2020, he was a Predoctoral Researcher at IBM Research Zurich, Switzerland, in the group of Dr. Christoph Hagleitner. Since January 2020, he has been an Academic Guest in Prof. Onur Mutlu's group at ETH Zurich, Switzerland.  He is passionate about FPGA design, computer architecture, and applied machine learning with skills in both hardware and software design. 


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/algorithms/transfer_algorithm.tex <==
\begin{figure}[h]
  \centering
\begin{minipage}{\linewidth}
\centering
{%\fontsize{9}{10}\selectfont
\footnotesize
\begin{algorithm}[H]
 \caption{\namePaper's~transfer learning}
%  \caption{\namePaper's~adaptive transfer learning}
 \label{algo:LEAPER_SIGMETRICS/transfer}
  \begin{algorithmic}[1]
   \State \textbf{Input:}{(1) Base learner ($f_s$) i.e., trained low-end edge FPGA prediction model,\\  \hskip3em (2) Sub-sampled {\emph{few-shot learning} dataset $c_{tl}\subset c_{lhs}$ from the\\\hskip3embase and the target model}}   %$c_{tl}\subset c_{lhs}$
  \State \textbf{Output:}{ Target {cloud FPGA} model $\hat{f}_t:\mathcal{X}_t \to \mathcal{Y}_t$}
\State \textbf{Initialization:} {Maximum number of iterations M}
\While{$M\not=0$}
    \State Normalize the feature vector
    \State Train ensemble transfer learners (TL) with $c_{tl}$
   \State Find the candidate TL ($\hat{f}_t$):
   \State \hskip1em  $\hat{h}_t:\mathcal{X}_{tl} \to \mathcal{Y}_{tl}$ that minimizes the error over the $c_{lhs}-c_{tl}$ \label{algo:LEAPER_SIGMETRICS/line:findTL}
    \State Compute the mean relative error: 
   \State \hskip1em $\epsilon_{mre}=\frac{1}{c_{lhs}-c_{tl}} \displaystyle\sum_{i=1}^{c_{lhs}-c_{tl}} \frac{|y_{t}^{acc} -y_{t}^{pred}|}{y_{t}^{acc}}$
   
    \State {Use identified $\hat{h}_t$ to transform predictions of $f_s$:}
   \State \hskip1em$\hat{f}_t$=$\hat{h}_t(f_s)$ \hskip7em where $f_s: \mathcal{X}_s \to \mathcal{Y}_s$
    \State$M \leftarrow M - 1$
\EndWhile
\textbf{return}  $\hat{f}_t$
\end{algorithmic}
\end{algorithm}
}
\end{minipage}
\end{figure}

==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/images/LHS.tex <==
\begin{SCfigure}[][h]
\vspace{0.8cm}
\centering
    \resizebox{0.3\textwidth}{!}{
    
    
    \begin{tikzpicture}
    %[rotate=90,transform shape]

\draw[step=0.25cm,gray,very thin] (0,0) grid (2,2);

\draw[thick,->] (0,0) -- (2.4,0);
\draw[thick,->] (0,0) -- (0,2.2);
%  \node at (0,0) [circle,fill=black] {};
%  \filldraw [gray] (0,0.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (2,2) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.25,1.5) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.75,0) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1,1.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.75,0.25) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.5,0.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (1.25,1.75) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0,1) circle (2pt);
\filldraw [color=gray!60, fill=gray!5,very thick] (0.5,0.5) circle (2pt);


 
 
\node at (0,2.4)[ rotate=0] {\small \textit{x1}};
\node at (2.6,0)[ rotate=0] {\small \textit{x2}};
\end{tikzpicture}
}
\vspace{-1cm}
\caption{LHS with 2 parameters where the input space is divided into equal intervals and 9 non-overlapping sample points are chosen.
\label{fig:LEAPER_SIGMETRICS/LHS}}
\end{SCfigure}


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/abstract.tex <==
Machine-learning-based models have recently gained traction as a way to overcome the slow downstream implementation process of FPGAs by building models that provide fast and accurate performance predictions. However, these models suffer from two main limitations: (1) a model trained for a specific environment cannot predict for a new, unknown environment; (2) training requires large amounts of data (features extracted from FPGA synthesis and implementation reports), which is cost-inefficient because of the time-consuming FPGA design cycle. In a cloud system, where getting access to platforms is typically costly, error-prone, and sometimes infeasible, collecting enough data is even more difficult. FPGA-based cloud environments are usually $2\times$ more expensive than CPU-only cloud environments. Therefore, before deploying a cloud instance, a user cares whether the attained performance while using an FPGA would justify the incurred cost (both in terms of designing an accelerator and deploying in the cloud). To overcome these limitations, in this chapter,  we propose \namePaper, a \textit{transfer learning}-based approach for FPGA-based systems that adapts an existing ML-based model to a new, {unknown} environment. %Experimental results show that our approach delivers, on average, 85\% accuracy  {when we use our transferred model for prediction in a cloud environment} with \textit{5-shot learning}, and reduces {design-space exploration} time by 10$\times$, from days to {only} a few hours. 


% Machine learning-based models have recently gained traction to overcome the notoriously slow downstream implementation process of FPGAs. However, an ML-based model trained for a specific environment cannot predict for a new environment. Moreover, traditional ML approaches require large amounts of training data, which is cost-inefficient owing to the time-consuming FPGA design cycle. We propose \namePaper, a transfer learning-based approach for heterogeneous systems augmented with intelligent statistical techniques. It overcomes the inefficiency of ML-based approaches by adapting an existing ML-based model for a new environment by retraining with only a few samples.
% Experimental results show that our approach
% delivers 80-90\% accuracy on average with few-shots, and it expedites DSE by 14$\times$, reducing from several days to a few hours. 

% Once transferred, the model can quickly provide accurate results across different environments. Experimental results show that our approach
% delivers 80\% accuracy on average with few-shots, and it expedites DSE by 14$\times$. 
% \gaganCheck{*Need to reduce the abstract, RIGHT now 123 words, shouldn't be more than 100 words}

% Modern CPU-FPGA based heterogeneous systems provide developers with increasingly large
% design options \jgl{Why is that?}. However, FPGA development has low productivity and tool run-times are cost-prohibitive for effective
% design space exploration \juan{DSE}, preventing designers from making approapriate decisions without expert guidance. 
% Several machine learning based models have been proposed to overcome this issue \jgl{What do this models provide?}. 
% However, these traditional approaches are data hungry that are trained for specific platform and hence these models become useless when deployed to new hardware targets.  Naturally, this does not scale when relying on real measurements in the changing environments, i.e., they are highly cost-inefficient. 
% \jgl{State the problems clearly: 1) An ML-based model trained for a specific platform is incapable of estimating performance for a new platform; 2) Training for a new platform requires a large amount of training data.}

% To this end \jgl{What is the end? You are not really stating your goal.} we propose RECOIL, a transfer-learning-based approach for heterogeneous systems that can overcome this inefficiency of traditional ML-based approaches by %adapting the old ML model to a new task by using a few samples only. 
% \juan{adapting an existing ML-based performance estimation model for a new system by retraining with only a few samples.} 
% Once transferred, the model can %be used to 
% quickly provide \juan{accurate} performance results across different configurations. 
% In order to minimize the data collection overhead for DSE, this paper proposes an efficient DSE method which combines Latin hypercube sampling and an adaptive ensemble transfer learning technique. Our experiments show we are able to develop cheaper, faster and accurate performance models for performance prediction in changing environments. Experimental results show that our approach
% delivers 80 to 90\% accuracy with few-shots (5 samples) and is able to explore 14$\times$ faster the entire design space across various platforms.



==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/conclusion.tex <==
\section{Conclusion}
% \vspace{-0.1cm}
% Modern CPU-FPGA %based 
% heterogeneous systems provide developers with extensive design options to optimize an application. However, FPGA development has low productivity, and tool run-times are cost-prohibitive for practical design space exploration (DSE). %Thus, preventing designers from making 
% {This makes difficult for designers to make} appropriate decisions without expert guidance. 

%To this end, 
% {To avoid these shortcomings,} 
We introduce \namePaper, {the first} \textit{transfer learning}-based approach for FPGA-based systems.  \namePaper combines statistical techniques and transfer learning to minimize the ML training data collection overhead.  It overcomes the inefficiency of traditional ML-based methods by accurately \textit{transferring} an existing ML model built on an {inexpensive}, low-end FPGA platform to a new, {unknown}, high-end environment.

% Traditional ML-based approaches have the following two shortcomings: 1) an ML-based model trained for a specific environment (application or hardware) is incapable of estimating {the} performance for a new {unknown} environment, and 2) training for a new environment requires a large amount of training data.
 
 \dd{The experimental results} show that we can develop cheaper (with \textit{5-shot}), faster (up to $10\times$), and highly accurate (on average 85\%) models to predict performance and resource consumption in a new, {unknown} target {cloud} environment. 
%  LHS reduces training samples from 500+ to 50, while  \textit{5-shot} learning further reduces this space to 5, so we achieve $100\times$ effective speedup compared to a conventional brute-force approach. %In the future, we would extend 
 We believe that \namePaper~would open up new avenues for research on FPGA-based systems from edge to cloud computing, and hopefully, inspires the development of other alternatives to traditional ML-based models.

% Another exciting direction would be to evaluate the applicability of transfer learning to a virtualized environment.

% Moreover, we show that with limited time budget, our methods are more suitbale than state-of-the-art supervised learning methods. We are able to generalize from a few examples.

% FPGA ML

% Predicting parallel application performance via machine learning approaches





% "The analytical
% models require a-priori knowledge of performance indicators as a precursor to model construction.
% Predictive models, in contrast, do not require this information, although do require the usage of a
% golden reference values during training"

% One of the key advantages of using a model to learn patterns
% that generalize (as opposed to lookup tables) is that the
% model can then be introspected in order to gain insights into
% the data


% As k gets larger, the difference in size between the training set and the resampling subsets gets smaller. As this difference decreases, the bias of the technique becomes smaller


% the behavior of one program can differ wildly from that of another.2. (In fact, the behavior of a single program can behave wildly different from one input
% to another. For example, consider how the behavior of gcc differs when compiling, say,
% matrix multiplication as opposed to an OS)



% We extract information from the source
% model that guides the sampling in the target environment, to gather
% fewer but more informative samples, and therefore, to gain a better
% understanding of the system performance with less cost.



==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/introduction.tex <==
\section{Introduction}


% The need for energy-efficiency from {edge} to cloud computing has boosted the widespread adoption~of~FPGAs~\cite{diamantopoulos2018ectalk,kara2018columnml, dai2017foregraph}. {An FPGA is highly configurable as its circuitry can be tailored to perform any task. The massive configuration space and complex interactions among configuration options lead many 
% {developers} to explore individual optimization options in an ad-hoc manner.  Therefore, developing an efficient FPGA accelerator %and finding the right system configuration for it (e.g., IBM CAPI offers three versions of cache-coherent interconnects) 
% requires tremendous engineering effort. Moreover, FPGAs have infamously low productivity due to the time-consuming FPGA {implementation} process.
% Exploring the high-dimensional design space can take hours or even days.   
% A common challenge that past works {face} is how to evaluate the performance of an FPGA implementation in a reasonable amount of time~\cite{mutlu2019}. }
%-------------------------------------------------------------------------------
%Power consumption has become one of the significant bottlenecks for our current computer systems. To overcome this issue, complementing general-purpose cores with specialized FPGA accelerators is a promising approach to enhance overall system performance without a significant increase in power consumption. 
The need for energy-efficiency from {edge} to cloud computing has boosted the widespread adoption~of~FPGAs. %Past works~\cite{diamantopoulos2018ectalk,kara2018columnml, dai2017foregraph} show that FPGAs can be employed {effectively} for a wide range of applications, {including graph processing, databases, neural networks, {and} weather forecasting}. 
{In cloud computing~\cite{arefmicrosoft,choi2019depth,aws,alibaba,pourhabibi2020optimus,byma2014fpgas}, %era, 
FPGA's flexibility is not just about being able to make use of reconfigurable hardware for a diverse set of workloads~\cite{10.5555/3294624}. {Its flexibility can also be attributed to the}  {cloud} deployment model that spans from on-premises clusters to compute, storage, and networking capacity in public clouds and even out to the edge where AI and analytics are being increasingly deployed because of latency and data movement issues~\cite{mutlu2019}.} 
% that combine CPUs with specialized accelerators, GPUs, and/or FPGAs. 
% Complementing general-purpose CPU cores with FPGAs~is a successful approach because of the reconfigurability and energy efficiency of FPGAs. 

%  However, taking full advantage of an FPGA for accelerating a workload is not a trivial task.
% First, FPGAs run at extremely low frequencies compared to the state-of-the-art CPU. Therefore, to match the CPU's performance, an FPGA must exploit at least one order of magnitude more parallelism in a target workload. Second, efficient FPGA designing requires comprehensive knowledge of the FPGA micro-architecture with sufficient FPGA programming skills, which often leads to a significant design effort. Third, CPU and FPGA are connected via low-bandwidth I/O links, which cause significant data movement overhead. 


An FPGA is highly configurable as its circuitry can be tailored to perform any task~\cite{umuroglu2017finn,umuroglu2020logicnets,kara2018columnml, dai2017foregraph}. % However, an efficient {implementation of a workload on an} FPGA requires comprehensive knowledge of the FPGA {microarchitecture} combined with sufficient FPGA programming skills. 
%  From a systems perspective, the design choices {are made more complex} by various interconnect options, such as upcoming %high-bandwidth} 
%  interconnect technologies from IBM CAPI~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators
% (CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{sharma2019compute}.
%This often leads to a significant design effort. 
The large configuration space of FPGA and {the} complex interactions among configuration options lead many 
developers to explore individual optimization options in an ad-hoc manner. 
Moreover, FPGAs have infamously low productivity due to the time-consuming FPGA {implementation} process~\cite{o2018predictive}.
%Exploring the high-dimensional design space can take hours or even days.   
 A common challenge that past works {have faced} is how to evaluate the performance of an FPGA implementation in a reasonable amount~of~time~\cite{o2018hlspredict}.  Thus, the development of efficient FPGA accelerators has required tremendous engineering effort due to the complexity of the FPGA configuration space and difficulties in evaluating performance.
 %Therefore, developing an efficient FPGA accelerator %and finding the right system configuration for it (e.g., IBM CAPI offers three versions of cache-coherent interconnects) 
%requires tremendous engineering effort.
To overcome this problem, researchers have {recently} employed machine learning (ML)-based models~\cite{o2018hlspredict,wang2020lutnet,xppe_asp_dac,dai2018fast} to {estimate}  the performance of an FPGA-based system quickly. {These models are} based, in turn, on traditional ML {approaches}. 

Traditional ML models have four fundamental issues {that can reduce the usability for assessing FPGA performance, especially in a cloud environment}. First, they are trained for specific workloads, fixed hardware, and/or a set of inputs. {Therefore,} when presented with a different feature-space distribution {because of a new workload or hardware}, {an ML model must} 
be retrained from scratch. Otherwise, {the model} will perform poorly because the trained model does not have a notion of the new, {unknown} environment.\footnote{{In this chapter, we consider an application or hardware platform as an environment.}} Therefore, traditional ML-based models have limited \textit{re-usability}.

Second, learning-based approaches, { such as neural networks}, require a considerable {number} of samples to construct a useful prediction model. {Collecting such a large number of samples is} often slow and time-consuming {due to the very long FPGA implementation cycle}. 
Similarly, in {settings} such as cloud computing, where getting access to platforms is typically \textit{costly}, \textit{error-prone}, and sometimes \textit{infeasible}, the data collection process {is even more difficult}. 

{Third, traditional machine learning with limited samples {is} prone to serious \emph{overfitting} problems {(i.e., when a model matches too closely to the training data)}~\cite{dai2007boosting}, limiting model generalization.}
Fourth, it is impossible to {construct} one model for all different scenarios as the interpretation of data changes over time. Thus, ML models are prone to \emph{concept drift}, where the accuracy of an ML-based model could degrade due to a change in the statistical properties of a target variable {(e.g., using a different dataset for an application than the one used during the training of an ML-model)}~\cite{model_drift}.\\


%This 
% Our research aims to answer the following question: for an FPGA-based system, can we leverage and transfer our ML-based performance models trained on a low-end local system to a new, unknown, high-end FPGA-based system, thereby avoiding the limitations of traditional ML-based approaches
\textbf{Our research aims to answer the following question: for an FPGA-based system, can we leverage an ML-based performance model trained on a low-end local system to predict the performance in a new, unknown, high-end FPGA-based system?}%. 
% \jgl{There is repeated text in this paragraph.}
% \jgl{We haven't talk about transfer learning yet. It is better to just ask something like: "Is there a way to leverage an ML-model trained for a specific low-end environment to predict the performance in an unknown high-end environment?" Then, we can talk about transfer learning in the introduction to Leaper.} 
%To this end, 

{{As an} answer to this question,} we present \namePaper\footnote{We call our mechanism \namePaper~because it allows us to hop or ``leap'' between machine learning models.}, a transfer learning-based model that predicts the performance of a new, unknown high-end FPGA-based system. We train \namePaper~ on a low-end local system. % \jgl{Leaper is not that. Leaper is a model that can predict the performance in an unknown high-end environment of applications that you have developed for a known low-end environment. After that, you can say what Leaper uses to be such model.}. 
\namePaper~ uses predictive modeling to train an ML-based model % \jgl{How? For what?} 
and statistical techniques to collect representative training data set efficiently. %using which we built 
%The goal of transfer learning is 
\namePaper uses \emph{transfer learning}~\cite{pan2009survey} to leverage a trained \textit{base model} (for a low-end system) and adapt it efficiently to an unknown \emph{{target}} environment {(i.e., a high-end system)} with a few samples from the target environment as possible. 

% {\textit{Transfer learning~\cite{pan2009survey}} \jgl{Cannot start like that. First, say what is Leaper, then say that Leaper uses transfer learning.} allows us} to leverage a trained \textit{base model} {(for a low-end system)} and adapt it efficiently to an unknown, \emph{{target}} environment {(i.e., a high-end system)} with as few samples from the target environment as possible. 



{ Figure~\ref{fig:transfer_intro} demonstrates the traditional approach of building models and the LEAPER transfer learning-based approach. Using the traditional approach, we would %have 
{need} to create two separate prediction models, {one} for the {low-end} edge {environment} and {another for the high-end} cloud environment, each {one} requiring a large number of samples. In contrast, \namePaper~provides the ability to reuse the prediction model  built on an {\emph{inexpensive}} edge FPGA for {performance prediction on a target} cloud environment~\footnote{Note: LEAPER is not limited to a cloud environment.} using only a few samples {from the target environment}. {This allows {developers} to avoid the slow downstream implementation process of FPGAs %to develop
{by generating} cheaper and faster performance models} using transfer learning.  }
This paradigm is also referred to as \textit{few-shot learning}~\cite{fsl}. The idea behind {few-shot learning} is that, similar to humans, algorithms can learn from past experiences and transfer the knowledge to accomplish previously-{unknown} tasks more efficiently. The transferred models usually have high generality~\cite{fsl} and can overcome {concept drift}~\cite{concept_drift}.

 \begin{figure}[h]
  \centering
  \includegraphics[bb=4 14 1147 485,width=1\linewidth,trim={0.2cm 0.9cm 0.4cm 0.3cm},clip]{LEAPER_SIGMETRICS/images/Transfer_intro_7.pdf}
    % \caption{Transfer learning from low-cost edge FPGA to a high-cost cloud FPGA environment}
     \vspace{-0.3cm}
  \caption{Comparison of traditional learning approach and LEAPER. {Traditional learning methods are costly because they build models only for a specific environment. } LEAPER allows transfer of models from a low-cost edge FPGA, where data collection is easier, to a high-cost cloud FPGA environment to build cheaper and faster models.}
  \label{fig:transfer_intro}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {\namePaper~builds} ML models that predict %the
% performance %/
% and resource usage for an application {on an FPGA}. With \textit{few-shot learning}, it adapts these models to a new, unknown environment, %{(i.e., a new FPGA or a new application)} %for 
% {from} which only a few labeled samples are %available.
% {needed}. {\namePaper~uses a statistical} technique called \textit{design-of-experiments} to collect the training data. This technique aims to cover the entire design space effectively in a limited {number of} experimental runs~\cite{singh2019napel}. We use \textit{Latin hypercube sampling} (LHS)~\cite{LHS} to sample FPGA's high-dimensional configuration
% space judiciously. The conventional brute-force approach to run every single input configuration on all the chosen platforms quickly becomes impractical. This is due to the large design space, combined with {the} long FPGA runtime (1-12 hours for a single point), which may take months or years~\cite{liu2013learning}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {Works, such as~\cite{singh2019napel,li2018processor,liu2013learning} show the effective use of these approaches.} 
% in this paper, we apply a 

% Howerver, to collect training data for all these scenarios will lead to massive space. The FPGA allows us to have plethora of optimization options. Moreover, if you want to make your ML model cross platform you execute all these combinations on different FPGA devices. 

% In traditional {ML} approaches, researchers exhaustively run every single input configuration on all the chosen platforms to collect the training data~\cite{tulikaML}. 
% The considerable design space, combined with {the} long FPGA runtime (1-12 hours for a single point), may take months or years~\cite{liu2013learning}, which makes the traditional exhaustive approach impractical. 
% %This calls for 
% {To overcome this issue, we use} %some 
% statistical techniques {to} effectively cover the entire design-space in a limited {number of} experimental runs~\cite{singh2019napel}. 
% % {Works, such as~\cite{singh2019napel,li2018processor,liu2013learning} show the effective use of these approaches.} 
% % in this paper, we apply a 
% {\namePaper~applies a statistical} technique called \textit{design-of-experiment} (DoE).  Specifically, we use \textit{latin hypercube sampling} (LHS)~\cite{LHS} to sample the high-dimensional configuration
% space wisely.
% To address this issue, we need to derive a robust
% prediction model by sampling which motivated us to propose a novel transfer learning based model and a weighted LHS sampling method.


% To find the right applicaiton input we need to perform input sensitivity analysis~\cite{Autotuning algorithmic choice for input sensitivity}. This entails extracting domain-specific algorithmic choices that influence the FPGA design, which inturn affect the overall performance. The large number of inputs, comined with long FPGA run-time (4-8hours for a single point) may take months or years, which makes the traditional exhuastive approach impratical.



% In this paper, we make the following contributions:

% %\vspace{-0.1cm}
% \begin{enumerate}
% \item We present the first use of \textit{few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications (Section~\ref{sec:LEAPER_SIGMETRICS/methodology}). This approach dramatically reduces (up to $10\times$) the training overhead by adapting a \textit{base model}, trained on a low-end {edge} {FPGA} platform to a {new}, unknown high-end environment ({a cloud environment in our case}) rather than building a new model from scratch (Section~\ref{subsection:LEAPER_SIGMETRICS/timing}).




% % \item We design an \emph{ensemble transfer learning model} based on the \textit{boosting} and \textit{Bayesian process} that transfers accurate models to a new target environment with few learning samples (Section~\ref{subsec:ensemble_transfer}). 
% %\jgl{Isn't this the same as 1) with different words? {I was thinking more like that we have ensemble of learners (two learners)}}

% \item We reduce the time needed to gather
% data for {model training} by employing a \textit{design-of-experiments} technique (Section~\ref{subsec:LEAPER_SIGMETRICS/lhs}), which
% selects a small number of input configurations
% that represents the entire space of input configurations.
% \item We create an {ensemble of transfer learning models} to transfer learning from multiple base learners accurately to avoid a negative transfer, i.e., a severe degradation of the predictive power of the transferred model (Section~\ref{subsec:LEAPER_SIGMETRICS/ensemble_transfer}). % The use of {multiple} base learners lets us avoid severe degradation of the \textit{transferred} model's predictive power, i.e., avoid a \textit{negative transfer} \jgl{What is a negative transfer? If you want to include this term, then flip the sentence: "...to avoid a negative transfer, i.e., a severe degradation of the predictive power of the transferred model.}.  
% \item We demonstrate our approach across \textit{five} {state-of-the-art,} high-end, {on-premise cloud} FPGA-based platforms with \textit{three} different {interconnect} technologies on \textit{six} real-world applications (Section~\ref{sec:LEAPER_SIGMETRICS/evaluation}). %{The kernels are specified in C/C++ and compiled to the FPGA target using Vivado HLS for the target and Xilinx SDSoC for the base model.}
% For \textit{5-shot} learning, we achieve an average performance and area prediction accuracy of 80--90\%. 
% \end{enumerate}


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/methodology.tex <==
\section{\namePaper}
\label{sec:LEAPER_SIGMETRICS/methodology}

\namePaper~is a performance %/
{and} resource estimation %approach 
{approach} to \textit{transfer} ML-based models across different FPGA-based platforms. First, we give an overview of \namePaper~(Section~\ref{subsec:LEAPER_SIGMETRICS/overview}). Second, we describe the two %most important 
 components of \namePaper~that are used to generate training datasets: (1) FPGA-based accelerator configuration options and application features used for training our base model (Section~\ref{subsec:LEAPER_SIGMETRICS/fpga_deploy}), and (2) the \textit{design of experiments} (DoE)~\cite{montgomery2017design} methodology (Section~\ref{subsec:LEAPER_SIGMETRICS/lhs}). Third, we briefly describe the {base} model training (Section~\ref{subsec:LEAPER_SIGMETRICS/base_model}).  Fourth, we explain the %important 
 \juan{key} component of \namePaper:
 the transfer learning technique (Section~\ref{subsec:LEAPER_SIGMETRICS/ensemble_transfer}). 

\subsection{Overview}
\label{subsec:LEAPER_SIGMETRICS/overview}
% \namePaper~is based on transfer learning.  It~transfers a base model, trained on an \gaganT{inexpensive}, low-end source environment, to a new, {unknown}, high-end {cloud} environment through {few-shot learning}. 
%Similar to humans, \namePaper~learns from previous models rather than running every single application and FPGA design configuration on a new, {unknown} environment.
Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew} depicts the key components of \namePaper. \juan{The upper part of the figure describes the construction of the base model, while the lower part shows the phases for the target model.}
% We considered random forest and gradient boosting as our base statistical model, which has proven to be a robust feature-based model in past problems. 

 \begin{figure*}[h]
  \centering
  \includegraphics[bb=44 60 2325 1016,width=0.9\linewidth,trim={0.8cm 0.8cm 0.4cm 1cm},clip]{LEAPER_SIGMETRICS/images/model_big_5.pdf}
     \vspace{-0.1cm}
  \caption{Overview of %our approach
  {\namePaper}. Base Model Building: {\namePaper~builds} ML models that predict %the
performance %/
and resource usage for an application {on an FPGA}. Target Model Building: with \textit{few-shot learning}, \namePaper~adapts base models to a new, unknown environment, %{(i.e., a new FPGA or a new application)} %for 
{from} which only a few labeled samples are %available.
{needed}.
}
  \label{fig:LEAPER_SIGMETRICS/transfer_overiew}
 \end{figure*}
 
\noindent \textbf{Base Model Building.} \namePaper~base model building consists of three phases. In the first phase (\circled{1} in Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew}), 
{we employ} 
\textit{Latin hypercube sampling} (LHS)~\cite{li2018processor} %is first employed 
to select a small set of input configurations that well represent the entire space of input configurations ($c_{lhs}$) to build a highly accurate \textit{base learner}. We use LHS to minimize the number of experiments needed to gather training data for \namePaper~while ensuring {good} quality training data (Section~\ref{subsec:LEAPER_SIGMETRICS/lhs}). In the second phase~\circled{2}, FPGA implementations are made with a software-hardware co-design process. Once the FPGA design has been implemented, the \juan{resulting FPGA-based} accelerator is deployed \juan{in a system} with a host CPU. %system. %Following which 
{Then,} we %use 
\juan{run} {the} $c_{lhs}$ configurations on %an FPGA-based platform 
\juan{this FPGA-based system} to gather responses for training our base model. The generated responses, along with \juan{the} applied configuration options {(\textit{ref}. Table~~\ref{tab:LEAPER_SIGMETRICS/pragma})}, form the input to our base ML algorithm. 
In the third phase~\circled{3}, we train our ML algorithm (Section~\ref{subsec:LEAPER_SIGMETRICS/base_model}) using ensemble learning~\cite{opitz1999popular}. %that uses both \textit{boosting} and \textit{bagging}-based ML techniques to create a robust ensemble model. 
We divide our dataset into 10 equal subsamples during cross-validation, of which 1 set is used for validation.  % \jgl{What is a 10-fold cross-validation?}.
Once trained, the framework can predict the performance and resource usage \juan{on the base system (with a low-end FPGA)} of %all 
{previously-unseen} configurations, %that 
\juan{which} are not part \juan{of the} $c_{lhs}$ \juan{configurations used during training.} %{on the base system, i.e., the low-end FPGA}.


\noindent \textbf{Target Model Building.} {To transfer the base model, which we built in the previous stage, to a target cloud environment, we introduce the \emph{few-shot learning} target model stage.} In the first phase (\circled{A} {in Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew}}) of {the} target model building, {we repeat the accelerator generation step to get a few samples.} %} is the same accelerator \jgl{Is it the same accelerator? Need to say that this is repeating the phase on the high-end FPGA to get the few samples.} generation and deployment phase as in the base model building stage
We perform this step to create our \textit{few-shot} transfer learning dataset ($c_{tl}$), % and transfer learning test set ($c_{lhs}$-$c_{tl}$). 
{ which is used to adapt the base model to the target cloud environment.}
% To create $c_{tl}$, in the second phase \circled{B}, we perform subsampling of $c_{lhs}$ \jgl{For what?}. 
In the final phase \circled{B}, we train our transfer learners (see Section~\ref{subsec:LEAPER_SIGMETRICS/ensemble_transfer}) to leverage the base model to perform predictions for a new, {unknown} target environment (new application or hardware).  %to leverage the base model to perform predictions of a new target environment (new application or hardware). 
% We show by empirical experiments, rather than running every single application and FPGA design configuration on a new platform, we can leverage the previously built model through transfer learning.  
\subsection{FPGA Configuration Options and Application Features}
\label{subsec:LEAPER_SIGMETRICS/fpga_deploy}
The ML feature vector used for training an ML model is composed of FPGA configuration options (Table~\ref{tab:LEAPER_SIGMETRICS/pragma}) and application features (Table~\ref{tab:LEAPER_SIGMETRICS/application_features}).
Table~\ref{tab:LEAPER_SIGMETRICS/pragma} describes commonly used HLS pragmas that belong to {our} FPGA configuration {options} for both the base and the target environment and constitute part of our ML feature vector. \juan{We select these HLS pragmas because they are used to optimize and tune the performance of FPGA implementations~\cite{xilinx_hls}.}
\input{LEAPER_SIGMETRICS/tables/pragma_configuration.tex}

Both \textit{loop pipelining} \juan{(PL)} and \textit{loop unrolling} \juan{(U)} can improve application performance significantly. %Memory operations are often the performance bottleneck in real applications. 
To enable simultaneous memory accesses, \textit{array partitioning} \juan{(PR)} \juan{divides arrays} into smaller memory units of arbitrary dimensions %by carefully deciding how 
to map \juan{them} %arrays 
to %memories has a significant influence on the overall implementation
\juan{different memory banks.} This optimization produces considerable speedups but consumes more resources. \textit{Inlining} \juan{(I)} ensures that a function is instantiated as dedicated hardware. \textit{Dataflow} \juan{(D)} allows parallel execution of tasks, which is similar to multi-threading in CPUs. 
%In addition, we take advantage of the large FPGA area to \textit{replicate} accelerators. 
In addition, \textit{burst read} \juan{(R)} and \textit{write}  \juan{(W)} access to/from the host guarantee that the accelerator is not stalled for data. Moreover, \textit{FPGA frequency} \juan{(F)} affects \juan{not only} performance %and 
\juan{but also} resource consumption. For instance, to meet the FPGA timing requirements, the FPGA tool tries to insert registers between the flip-flops, \juan{which increases the resource consumption}. 



In total, our configuration options \juan{for a particular application} consist of \juan{up to} 4,608 configurations. %{Note:  Table~\ref{tab:pragma} describes the configuration options used to train our ML-models.} 
The actual configuration space of an application depends %indirectly 
on the specific application characteristics (see Table~\ref{tab:LEAPER_SIGMETRICS/app_details}). %, e.g., 
\juan{For example, we include} loop unrolling \juan{in the configuration space when an application contains loops that can be unrolled.} %is effective only when an application’s loop can benefit from it.




%The {application} profile \textit{p(k, d)} is obtained by executing the application kernel \textit{k} while processing a dataset \textit{d}. 
\juan{For each application kernel \textit{k} processing a dataset \textit{d}, we obtain an application profile \textit{p(k, d)}.} 
\textit{p(k, d)} is a vector where each parameter is a statistic about an application feature. 
Table~\ref{tab:LEAPER_SIGMETRICS/application_features} lists the main application features {we extract} {by using the LLVM-based PISA analysis tool~\cite{Anghel2016}}. 
{We select} these features to analyze the behavior of an application (data reuse distance, memory traffic, memory footprint, etc.). 
Ultimately, the application profile \textit{p} has 395 features, which includes all the sub-features {of each metric we consider}.% \jgl{At this point, if the reader is paying attention, he/she will understand that the ML feature vector used for training is composed of values for the features in Table 1 and Table 2. The problem is that we are not saying this anywhere. This should be the first thing to say in the beginning of 2.3.}

\input{LEAPER_SIGMETRICS/tables/metrics.tex}

% \jgl{The organization is not good. We talk about LHS in 2.2. before talking about the FPGA configuration options in 2.3. Better organization is: 1) Section 2.2 talks about FPGA configuration options, including LHS; 2) Section 2.3 talks about application features.}
\pagebreak
\subsection{Latin Hypercube Statistical Sampling}
\label{subsec:LEAPER_SIGMETRICS/lhs}
%It would be imprudent to exhaustively run for all the available optimization options, which is often done in research to collect training data. 
{Running experiments to collect training data for all available optimization options can be an extremely time-consuming process. For example,} 
the configuration options ($\mathbb{CO}$) of %just 
{only} eight parameters {with two possible values each} %, even with binary options, would lead to
{entails} $2^8=256$ different configuration inputs. 
If we spend 6 hours (e.g., FPGA downstream implementation process on an ADM-PCIE-KU3 {FPGA board}~\cite{adku3}) to collect one training point, it would take {us} %$\approx$
$\sim$64 days to collect data for all configurations %options 
for just \textit{one} application on a \textit{single} platform. 
{This ``brute-force'' approach to collecting training data is too time-consuming: the sheer number of experiments renders \juan{a} detailed implementation intractable}.

To create a %cost-aware 
{cost-effective} model, we use the \juan{\emph{design of experiments} (DoE) methodology}~\cite{montgomery2017design} %method
to minimize the number of experiments needed %to train
{for training data collection} without sacrificing the amount and quality of the information gathered %by 
\juan{from} the experiments. 
DoE is a set of statistical techniques meant to locate a small set of points in  parameter space to represent the entire parameter space.
%The traditional brute-force approach to collecting training data is {too} time-consuming: the sheer number of experiments renders detailed simulations intractable. 
%Thus, the DoE strategy to gather a training dataset is a critical component of our model. 
{In particular, we make use of \juan{a type of DoE called}  \textit{Latin hypercube sampling} (LHS)~\cite{li2018processor} because it allows each of the critical parameters to be represented in a fully stratified manner (i.e., dividing the configuration space into subgroup before further sampling), which provides a better coverage~\cite{fang2002centered}.}

LHS divides each parameter range into \textit{k} intervals and takes only one sample from each interval with equal probability, which is more efficient than a random approach and more cost-effective than a ``brute-force'' approach. % \jgl{I would say it "is more efficient than a random approach and more cost-effective than a brute-force approach".}.
To apply %Latin Hypercube sampling, one must
{LHS, we} %first 
choose \textit{m} sample points, each from a specific interval,  which together we refer to as \textit{c$_{lhs}$}. % \jgl{Not clear: \textit{c$_{lhs}$} is a configuration point, which considers multiple parameters; but when we talk about intervals above, we talk about each parameter.}. %; hence 
{Thus,} LHS guarantees effective space-filling, i.e.,  LHS spreads out points with the aim of encouraging a diversity of data~\cite{li2018processor}. %\jgl{One can guess what "space-filling" is, but it is just a fancy term for free... Let's explain fancy terms if we use them.}.  
Figure~\ref{fig:LEAPER_SIGMETRICS/LHS} illustrates LHS with two parameters \juan{\textit{x1} and \textit{x2}}, %where the 
\juan{which create an} input space \juan{that} is divided into equal-area intervals. %{To select the amount of samples to build a precise performance prediction model we follow the approach from Valov~\etal~\cite{valov2015empirical} \jgl{And this approach consists of what?}.}   %We use T\textit{$\times\mathbb{CO}$} samples, where T=5 allows to build highly accurate prediction models.

\input{LEAPER_SIGMETRICS/images/LHS.tex}



\subsection{Base Model {Building}}
\label{subsec:LEAPER_SIGMETRICS/base_model}

The third phase of \namePaper~is the base learner training phase. Formally, { in a learning task, $\mathcal{X}$ represents feature space with label $\mathcal{Y}$, where a machine learning model is responsible for estimating a function $f: \mathcal{X} \to \mathcal{Y}$.} %we predict time
{\namePaper~predicts the execution time (resource consumption) $\mathcal{Y}$ for a tuple} $(p,~k,~c)$ {that belongs to the ML feature space $\mathcal{X}$}, where \textit{p} is an {FPGA-based} {configuration option (see Section~\ref{subsec:LEAPER_SIGMETRICS/fpga_deploy})} %running
{that runs an} application characteristics \textit{k}, with %\textit{c} configuration for optimization 
{an optimization configuration vector \textit{c}}. 

We use two base learners.  Our base learners are non-linear algorithms that {can} capture the intricacies of FPGA architectures by predicting the execution time %or 
or resource consumption. %of a {heterogeneous} CPU-FPGA platform.  
Our first algorithm is the \emph{random forest} (RF)~\cite{breiman2001random}. RF consists of an ensemble of learners where it aggregates the predictions of the weak learners to select the best prediction. This technique is called \textit{bagging}. We use RF to avoid a complex feature-selection scheme % and moreover it} 
\juan{since RF} embeds automatic procedures \juan{that are able} to screen many input features~\cite{mariani2017predicting}, \juan{like the ones we selected in the previous section}. 
Starting from a root node, RF constructs a tree and iteratively grows the tree by associating %it 
\juan{a node} with a splitting value for an input %variable 
\juan{feature} to generate two child nodes. 
Each node is associated with a prediction of the target metric, equal to the observed \juan{mean} value in the training dataset for the input subspace that the node represents. 
Our second learner is \emph{gradient boosting}~\cite{gradientboosting}, which consists of an ensemble of learners. Gradient boosting aims to \textit{boost} \juan{the accuracy of a weak learner}  %'s 
by using other learners to correct its predictions. {Bagging reduces model variance and boosting decreases errors~\cite{kotsiantis2004combining}. {Therefore, we use random forest and gradient boosting together to increase the predictive power of our final base model.}}

 %, that forms a part of the ML feature space $\mathcal{X}$. 
% \jgl{If you want to use the formal definition, which is probably not necessary, start the section with it. Then, talk about the two learners. Then, talk about execution time and resource consumption. It seems there are different models for these two, but it is no clear from the text.}

%The input data gathered to train our base model 
{The training dataset for our base model} has two parts: (1) an optimization configuration vector \textit{c}, whose representation remains invariant across different environments, and (2) {the} {responses corresponding to each %pair 
{tuple} $(p,~k,~c)$}. 
To gather the architectural responses, {we run each} application \textit{k} belonging to {the} training set $\mathbb{T}$ with {an} input dataset \textit{d} %is executed 
on an FPGA-based platform \textit{p}, {deploying} a configuration \textit{c}. 
%This produces time\textit{(p,~a,~d)} for that configuration and is used 
{This way, we obtain the execution time for the tuple \textit{(p,~k,~d)}, which we can use} 
as a \textit{label} ($\mathcal{Y}$) for training our base learner {for performance prediction}. 
%Similarly, we build another model 
{We build a similar model} to predict resource consumption, where we use {the} resource consumption ($\eta_{\{BRAM, FF, LUT,  DSP\}}$) {of the tuple \textit{(p,~k,~d)}} as a \textit{label} when we train our base learner {for resource consumption}. 
After training our base learners, %algorithm, 
we can predict the {execution} time (resource usage) ($\hat{f_s}:\mathcal{X}_s \to \mathcal{Y}_s$) of %configurations 
{tuples \textit{(p,~k,~d)}} that are \emph{not} in the training set. We use 10-fold cross-validation to validate our base learner's performance, {whereby the data is divided into ten validation sets.} % This, in turn, produces...
% We improve our framework training by tuning the algorithm's hyper-parameters~\cite{scikit-learn}. Hyper-parameter tuning can provide better performance estimates for some applications. 
% {First, we perform as many iterations of the cross-validation process as hyper-parameter combinations}. %, each time using a different model setting. 
% {Second, we compare all the generated models by evaluating them on the testing set, and select the best one}. 
% The best-tuned configuration is listed in Table~\ref{tab:results} for each application. %\jgl{Do we really need to show the hyper-parameters in the table?}
% After training our RF algorithm, we can predict the time of a configurations that are \emph{not} in the training set.  Similarly, we build another model for area prediction where we use resource utilization as a \textit{label} when we train our RF algorithm.
% Choose m design points with k factors.
% Each factor divided into m equally spaced values
%  Figure  illustrates two sets of LHS samples with
% five intervals in a 2D dimension, one denoted by dots and the other
% by triangles.
\subsection{{{Cloud} Model Building via Transfer Learner}}
\label{subsec:LEAPER_SIGMETRICS/ensemble_transfer}
{The real strength of %the 
LEAPER %framework 
comes from its ability to transfer trained FPGA models.}
{\namePaper~defines} a target environment $\tau_{t}$ as an environment for which we wish to build a prediction model {$\hat{f}_t$ where, however, data collection is expensive}, and %we define 
a source environment $\tau_{s}$ as an environment %one 
for which we can \textit{cheaply} collect many samples to build an ML model ${f}_s$. {In our case, $\tau_{s}$ is a low-cost edge FPGA, while $\tau_{t}$ is a high-cost cloud FPGA. } {\namePaper~then transfers the ML model for $\tau_{s}$ to $\tau_{t}$.}


% For a given prediction task, individual ML-based models provide varying degrees of accuracy. This trend is common across prediction tasks and is referred to as model disagreement~\cite{xapp}. Therefore, we need an adaptive technique that selects the best performing model for each {configuration that we would like to transfer}. %We automatically detect the {strong} models and drop the weak models. 
Algorithm~\ref{algo:LEAPER_SIGMETRICS/transfer} presents \namePaper's transfer learning approach. %{We reuse previously built base learner ($f_s$)} by leveraging transfer learning.   Our  
\juan{\namePaper~ trains transfer learners (TL) that} 
transform the source performance and utilization model $f_{s}$ to \juan{the target model} $f_{t}$ by using {a few} sample observations from {both} the source and the target environments, which we refer to as \textit{c$_{tl}$}. This helps us to avoid measuring all c$_{lhs}$ from a cost-prohibitive target cloud environment. We select \textit{c$_{tl}$} from \textit{c$_{lhs}$} by applying {a} probability-based sampling {technique} called \textit{reservoir sampling}~\cite{vitter1985random}. %We apply a 
\juan{Reservoir sampling} %because it 
assigns an equal probability of being selected to every element of %the 
\juan{a} population \juan{(i.e., \textit{c$_{lhs}$})}. 
 %The intuition behind %choosing this reservoir sampling is to assign an equal probability to every element in the alreadyssampled space.
%{Using 
\juan{By using the selected} \textit{c$_{tl}$}, we generate a transfer model $\hat{h}_t$. Finally, to build $\hat{f}_t$ from ${f}_s$ we use $\hat{h}_t$ that performs a non-linear transformation of the predictions of ${f}_s$. We use non-linear transfer learners because, based on our analysis (\juan{Section}~\ref{subsection:LEAPER_SIGMETRICS/relatedness_analysis}), non-linear models can capture the nonlinearity present in the FPGA performance and configuration options.
% \jgl{In reality, this paragraph should explain the algorithm and refer to the line numbers.}

\input{LEAPER_SIGMETRICS/algorithms/transfer_algorithm.tex}

{In transfer learning, a weak relationship between the base and the target environment can decrease the predictive power for the target environment model. This degradation is referred to as a \textit{negative transfer}~\cite{jamshidi2017transfer}. To avoid this,} we use an ensemble %of \textit{boosting} and \textit{Bayesian probability}-based 
model trained on the transfer set (i.e., {the} \textit{few-shot learning} dataset in Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew}) as our transfer learners (TLs). Our first TL is based on TrAdaBoost~\cite{dai2007boosting}, a boosting algorithm, which is a learning framework that fuses many weak learners into one strong predictor by adjusting the weights of training instances. {The motivation behind such an approach is that by fusing many weak learners boosting can improve the overall predictions
in areas where the previously grown learners did not perform well.} We use Gaussian process regression~\cite{Gaussian} as our second TL. It is a Bayesian non-parametric algorithm that calculates the probability distribution over all the appropriate functions that fit the data.  To transfer a trained model, we train TrAdaBoost and Gaussian progression, which are our candidate TLs. We choose the one that has minimum transfer error (see Line~\ref{algo:LEAPER_SIGMETRICS/line:findTL}). 
 

% To understand the notion of relatedness of the performance models in source and target environments we perform correlation analysis. The correction between the target system and the source system.


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/relatedWork.tex <==
\section{Related Work}
% \vspace{-0.1cm}
\noindent\textbf{Transfer Learning.} Recently, transfer learning~\cite{chen2010experience,pan2009survey,baumann2018classifying} has gained traction to decrease the cost of learning by transferring knowledge. Valov~\etal~\cite{valov2017transferring} investigated the transfer of application models across different CPU-based environments using linear transformations. Jamshidi~\etal~\cite{jamshidi2017transfer} demonstrated the applicability of using nonlinear models to transfer CPU-based  performance models. {The works above influenced the design of~\namePaper}. In contrast, we focus on FPGA-based systems, where we tailor the hardware circuitry to an application by leveraging the large high-dimensional optimization
space and has very low productivity due to the time-consuming downstream implementation process. Moreover, we use an ensemble of transfer learners that transfers accurate models to a target environment via \textit{few-shot learning}. \\

\noindent\textbf{ML-based FPGA Modeling.} Recent works propose ML-based methods to overcome the issue of low productivity with FPGAs. O'Neal~\etal~\cite{o2018hlspredict} use CPU performance counters to train several ML-based models to predict FPGA performance and power consumption. Makrani~\etal~\cite{xppe_asp_dac} trained an ANN to predict application speedup across different FPGAs. Dai~\etal~\cite{dai2018fast} use ML to predict post-implementation resource utilization from pre-implementation results. However, these solutions become largely impractical once the platform, the application, or even the size of the workload changes. \namePaper~proposes to reuse previously built models on a low-end source environment to accelerate the learning of ML models on a high-end target environment through transfer learning. Unlike \namePaper, past works~\cite{tulikaML} apply traditional, time-consuming brute-force techniques to collect training dataset. These techniques quickly become intractable when the number of optimization parameters increases due to the curse of dimensionality~\cite{bellman1966dynamic}.\\
% Moreover, FPGAs are deployed with a host system, and often past works ignore the overhead of data transfer between the host and the FPGA, which makes their model incompetent for the heterogeneous systems. In our work, we consider end-to-end system performance and leverage transfer learning to build models for different platforms and different applications. 
% Moreover, past works~\cite{tulikaML} apply traditional, time-consuming brute-force techniques to collect training dataset. These techniques quickly become intractable when the number of optimization parameters increases due to the curse of dimensionality~\cite{bellman1966dynamic}. 
% In this work, we leverage \textit{design of experiment} techniques to reduce the training overhead dramatically and still build accurate models. 

\noindent\textbf{Analytical FPGA Modeling.} {Analytic models abstract low-level system details and
provide quick performance estimates at the cost of accuracy. These approaches~\cite{linAnalyzer,zhao2017comba,hls_scope} analyze dataflow graphs and apply mathematical equations to approximate resource usage or performance after the HLS pre-implementation phase. These approaches enable {quick early-stage design studies, however, analytical models} cannot model the intricacies of the complete FPGA implementation process~\cite{dai2018fast}. Therefore, these approaches provide crude estimates of the actual performance. Moreover, these models require expert knowledge to form mathematical equations.  In contrast,~\namePaper~does not require expert knowledge to construct equations. \namePaper~learns from the data, taking into account the complete downstream implementation process, and provides the capability to transfer models from an edge-FPGA to a high-end cloud FPGA environment.}

 LEAPER is the first method to deal with transfer learning on FPGAs, which are infamous for low productivity due to the time-consuming mapping process. \namePaper~not only allows us to predict performance for different configurations (Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew} ``Base model building'' stage) but also provides the ability to transfer the models (Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew} ``Target model building - Few-shot learning'' stage). \namePaper~is orthogonal to previous approaches (ML and non-ML) as it also provides the ability to ``transfer'' models in milli-seconds (\textit{ref}. Table~\ref{tab:LEAPER_SIGMETRICS/timing}).   Additionally, in this chapter, we leverage the \textit{design of experiment} techniques to reduce the training overhead dramatically and still build accurate models. 
 %We believe LEAPER can open up new avenues for research on the cloud FPGA-based systems 


% Some works have proposed the use of white-box model techniques for quick performance prediction. However, these techniques have two main limitations. First, it relies on analytical or design models derived from mathematical
% theories or software architecture abstraction, which are often imprecise~\cite{chen2016generating}. Second, coarse analytical models abstract detailed phenomena  that influence the overall application behaviour.
% Our approach  is orthogonal to these approaches and proposes a new way to EDA by reusing previously built model on cheaper sources to accelerate the learning of models on other target platform or applications through transfer learning.





% For a given data parallel application, achieving the best performance on a hetergogneous platform not oonly depends on the performance xplpoitation of eath single processing unit, but also on the perfromance aggregarion of the entire system. That is to say progrormmers have to partition the applicaiton workload such that all the processing units are best utilized and combined to achieve the best aggregate performance.  fingind such a wokrload paritioning remains a challenge~\cite{shen2015workload}. First, the heterogeneity of the platform requires the partitioning ot fully consider the the processing units' difference in processing capabiliyt, hardware archiecture, memory model, external bus. Secondly, the diversity of platforms, applicaitons, and datasets increases the partitioning complexity. Finally, from the programmer's viewpoint, it is challenging to obtain with limited time and effort the optimal partitioning that leads to the best performance for a given heterogenous platform, application, and dataset.


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/sections/results.tex <==
%\section{Evaluation and Results}


\section{{Evaluation}}
\label{sec:LEAPER_SIGMETRICS/evaluation}

% We aim to minimize the prediction error and the model training cost under FPGA area constraint. So it is a multi objective optimization problem
%We consider different
{We evaluate \namePaper~using six} 
 benchmarks (see~Table~\ref{tab:LEAPER_SIGMETRICS/app_details}), which are hand-tuned for FPGA execution %, that 
covering %a wide range of 
{several application} domains, i.e., \textbf{(1) image processing}:  histogram {calculation (\textit{hist})~\cite{gomez2017chai}, and canny edge detection (\textit{cedd})~\cite{gomez2017chai}}; \textbf{(2) machine learning}: binary long short term memory (\textit{blstm})~\cite{diamantopoulos2018ectalk}, digit recognition (\textit{digit})~\cite{zhou2018rosetta}; %and canny edge detection (\textit{cedd})~\cite{gomez2017chai}; 
%and 
\textbf{(3) databases}: relational operation (\textit{select})~\cite{ds-gomezluna-2015}; 
and \textbf{(4) {data reorganization}}: stream compaction (\textit{sc})~\cite{gomez2017chai}. These kernels are specified in C/C++ code that is compiled to the FPGA target. 
% %LHS is applied to these workloads to select a small set of optimizations $c_{lhs}$ that represent the entire space of possible optimizations. Next, we implement and deploy %the
% FPGA accelerators using {Xilinx} SDSoC for %the
% $\tau_{s}$ and Vivado HLS with IBM CAPI-SNAP framework\footnote{https://github.com/open-power/snap} for $\tau_{t}$. Finally, we train our base learner and leverage it to {perform predictions for a new, unseen cloud target environment}. 

\subsection{Hardware Platform and Tools}
With high adoption of FPGAs in the cloud, various emerging CPU-FPGA platforms with competing cache-coherent interconnect standards are being developed, such as  %high-bandwidth} 
 the IBM Coherent Accelerator Processor Interface (CAPI)~\cite{openCAPI}, the Cache Coherent Interconnect for Accelerators
(CCIX)~\cite{benton2017ccix}, the Ultra Path Interconnect (UPI)~\cite{UPI}, and the Compute Express Link (CXL)~\cite{cxlwhitepaper}.  

{The benefits of employing such cache-coherent interconnect links for attaching FPGAs to CPUs, as opposed to the traditional DMA-like communication protocols (e.g., PCIe), are not only the ultra lower-latency and the higher bandwidth of the communication, but most importantly, the ability of the accelerator to access the entire memory space of the CPU coherently, without consuming excessive CPU cycles. Traditionally, the host processor has a shared memory space across its cores with coherent caches. Attached devices such as FPGAs, GPUs, network and storage controllers are memory-mapped because of which they use a DMA to transfer data between local and system memory across an interconnect such as PCIe. The attached devices can not see the entire system memory but only a part of it. Communication between the host processor and attached devices requires an inefficient software stack, including user-space software, drivers, and kernel-space modules, in comparison to the communication scheme between CPU cores using shared memory. Especially when DRAM memory bandwidth becomes a constraint, requiring extra memory-to-memory copies to move data from one address space to another is cumbersome~\cite{Fang2020}. This is the driving force of the industry to push for coherency and shared memory across CPU cores and attached devices, like FPGAs. This way, the accelerators act as peers to the processor cores. %For example, one of the earliest industry-adopted paradigms of cache coherency for accelerators was the Cell Broadband Engine architecture~\cite{5388817}, which introduced coherent shared system memory access for its Synergistic Processor Element accelerators.

Based on this upcoming trend, in this thesis, we adopt cache-coherent FPGA accelerators, both for the low-end and the high-end systems. Specifically, we select a \textit{low-end} edge PYNQ-Z1~\cite{zynq} as the source platform to build base learners. We use the Accelerator Coherency Port (ACP) port~\cite{ACP} for attaching accelerators to the ARM Cortex A9 CPU of PYNQ-Z1. In addition, we select a CAPI-based system as the target platform } that provides the most mature coherent accelerator-based ecosystem with a production-ready cloud offering through Nimbix Cloud~\cite{nimbix}. 
% {Figure~\ref{fig:LEAPER_SIGMETRICS/system} shows the target cloud environment platform and execution timeline from a host system to an FPGA board.} As shown in {Fig.~\ref{fig:LEAPER_SIGMETRICS/system}(b), 

We make use of CAPI in a coarse-grained way since we offload the entire application to the FPGA. In this case, CAPI ensures that the FPGA accelerators access the entire CPU memory with the minimum number of memory copies between the host and the FPGA, e.g., avoiding the intermediate buffer copies that a traditional PCIe-based DMA invokes~\cite{10.1145/2897937.2897972}. However, depending on the application, the CAPI protocol can be employed in finer-grained algorithm-hardware co-design, like \textit{ExtraV} \cite{Lee:2017:EBG:3137765.3137776}, where the authors aggressively utilize the fine-grained communication capability of CAPI to boost graph analytics performance.  Table~\ref{tab:LEAPER_SIGMETRICS/systemparameters} summarizes the system details of the source and our {on-premise research cloud} environment as our target platform.

For accelerator implementation and deployment, we leverage CAPI-compatible tools offered by Xilinx. In particular, we use the {Xilinx} SDSoC~\cite{sdsoc} design tool for implementing the low-end system
$\tau_{s}$ and the Vivado HLS~\cite{hls} with IBM CAPI-SNAP framework\footnote{https://github.com/open-power/snap} for the high-end system $\tau_{t}$. The SNAP framework provides seamless integration of an accelerator~\cite{10.1007/978-3-030-34356-9_25} and allows to exchange of control signals between the host and the FPGA processing elements over the
AXI lite interface~\cite{axilite}. On task completion, the processing element notifies
the host system via the AXI lite interface and transfers back
the results via CAPI-supported DMA transactions. 

As derived from the indicative prices listed at the right column of Table~\ref{tab:LEAPER_SIGMETRICS/systemparameters}, the total cost of ownership (TCO) of a high-end system can be more than 100x of that of the low-end one; thus, it can be prohibitive for a bare-metal deployment for many users. Complementary, moving a workload to a cloud FPGA instance should offer such a speedup that it compensates for the extra design time, effort, and cost of this decision by the end-user. LEAPER helps a user to rapidly quantify such a decision by experimenting with low-cost and broadly available FPGAs, like the PYNQ-Z1.
%, model, which is transferred to different platforms/applications using our ensemble transfer learners.
\input{LEAPER_SIGMETRICS/tables/application}
%  \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{.5\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{LEAPER_SIGMETRICS/images/System4.pdf}
%   \vspace{-0.5cm}
%   \caption{
% %   \label{fig:LEAPER_SIGMETRICS/system}
%   }
% \end{subfigure}%
% \begin{subfigure}[t]{.5\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/Execution_timeline_5.pdf}
%   \vspace{-0.5cm}
%   \caption{
%   \label{fig:LEAPER_SIGMETRICS/execution}}
% \end{subfigure}
%  \vspace{-0.2cm}
% \caption[Two numerical solutions]{(a) Target Cloud Platform: CAPI-based high-end on-prem cloud FPGA platform with IBM\textsuperscript{\textregistered} POWER9  CPU\footnotemark. FPGA acts as a peer to the  CPU by accessing the main-memory~through a high-performance CAPI link, enabled by Power Service Layer (PSL). {A processing element (PE) is composed of basic~FPGA~components i.e., CLB, BRAM, and DSP.} (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard  FPGA  memory. A software-defined API handles %offloading jobs 
% {job-offloading} to PEs with an interrupt-based queuing mechanism. \label{fig:LEAPER_SIGMETRICS/system}}
% % \vspace{-1cm}
% \end{figure*}

 \begin{figure*}[t]
 % \hspace{0.9cm}
  \begin{subfigure}{0.495\textwidth}
   %\vspace{-0.1cm} 
   \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-blstm2.pdf}
   %  \vspace{-0.8cm}
    %  \caption{}
    \label{fig:LEAPER_SIGMETRICS/board_blstm}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
  %\hspace{-0.1cm}  
  \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-cedd2.pdf}
  %  \vspace{-0.3cm}
   % \caption{ \hspace*{1.5cm}}
   % \caption{}
    \label{fig:LEAPER_SIGMETRICS/board_cedd}
  \end{subfigure}
   \begin{subfigure}{0.495\textwidth}
%\hspace*{0.9cm}
\includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-digit2.pdf}    %\vspace{-0.8cm}
   % \caption{\hspace*{-1.8cm}}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/board_digit}
  \end{subfigure}
  %\hspace{1.1cm}
   \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-hist2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/board_hist}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-sc2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/board_sc}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-board-select2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/board_select}
  \end{subfigure}
    \vspace{-0.3cm}
  \caption{\namePaper's accuracy for %transferred
  {transferring} base models across CAPI-enabled {cloud} FPGA-based systems. {The legends indicate the target platforms}. The base model was trained on a low-end PYNQ-Z1 board and, for each application, we \textit{transfer} this model to different high-end cloud FPGA-based %HPC 
  platforms using different samples {(horizontal axis)} from the target platform. Once trained using \textit{few shot}, the transferred model makes predictions for all other configurations in the target platform.}
   \label{fig:LEAPER_SIGMETRICS/acros_board}
\end{figure*}

 \begin{figure*}[t]
 % \hspace{0.9cm}
  \begin{subfigure}{0.495\textwidth}
   %\vspace{-0.1cm} 
   \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-blstm2.pdf}
   %  \vspace{-0.8cm}
    %  \caption{}
    \label{fig:LEAPER_SIGMETRICS/app_blstm}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
  %\hspace{-0.1cm}  
  \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-cedd2.pdf}
  %  \vspace{-0.3cm}
   % \caption{ \hspace*{1.5cm}}
   % \caption{}
    \label{fig:LEAPER_SIGMETRICS/app_cedd}
  \end{subfigure}
   \begin{subfigure}{0.495\textwidth}
%\hspace*{0.9cm}
\includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-digit2.pdf}    %\vspace{-0.8cm}
   % \caption{\hspace*{-1.8cm}}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/app_digit}
    %\vspace{-1.5cm}
  \end{subfigure}
  %\hspace{1.1cm}
   \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-hist2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/app_hist}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-sc2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/app_sc}
  \end{subfigure}
     \begin{subfigure}{0.495\textwidth}
  %   \includegraphics[width=\textwidth,trim={2.7cm 10cm 2cm 10cm},clip]{LEAPER_SIGMETRICS/images/gagan_across-app-select.pdf}
     \includegraphics[width=\textwidth,trim={0cm 0cm 0cm 0cm},clip]{LEAPER_SIGMETRICS/images/across-app-select2.pdf}
   % \vspace{-0.8cm}
    %\caption{}
    \label{fig:LEAPER_SIGMETRICS/app_select}
  \end{subfigure}
\vspace{-0.3cm}
  \caption{\namePaper's accuracy for %transferred 
  {transferring} base models across various applications. {The legends indicate the number of samples}. Each plot represents a different application as a base learner. We \textit{transfer} these base learners, trained on the PYNQ-Z1 platform, by using invariant configuration features to build a target application model.}
   \label{fig:LEAPER_SIGMETRICS/across_app}
\end{figure*}
\subsection{{Target Model }Accuracy Analysis}
\namePaper~is used to transfer a trained model using \textit{few-shot learning} to the $\tau_{t}$'s {optimization} space. We then analyze the accuracy of the newly-built target model to predict the performance and resource utilization of all the other configurations in %the 
$\tau_{t}$. %optimization space.
We evaluate the accuracy of the %the proposed 
{transferred} model in terms of the relative error $\epsilon_i$ to indicate the proximity of the predicted value $y_{i}^\prime$ to the actual value $y_{i}$ across \textit{N} test samples. The mean relative error (MRE) is calculated with Equation~\ref{eq:LEAPER_SIGMETRICS/2}.
\vspace{-0.08cm}
\begin{align}
 MRE= \frac{1}{N} \displaystyle \sum_{i=1}^{N} \epsilon_i=\frac{1}{N} \displaystyle \sum_{i=1}^{N}\frac{|y_{i}^\prime -y_{i}|}{y_{i}}.
\label{eq:LEAPER_SIGMETRICS/2}
\end{align}
\vspace{-0.05cm}

% \subsection*{Transfer Across Platforms and Applications}
\noindent {\textbf{Performance Model Transfer.}}
Figure~\ref{fig:LEAPER_SIGMETRICS/acros_board} shows \namePaper's accuracy for transferring \textit{across different {cloud} platforms}. We make the following four observations.

First, as we increase the number of labeled samples, the target model accuracy increases. However, the accuracy saturates and,  with 5-10 \textit{shots}, we can achieve an accuracy as high as 80 to 90\%. 

Second, compared to applications with multiple complex kernels (\textit{blstm}, \textit{cedd}, \textit{digit}), simpler kernels (\textit{hist}, \textit{sc}, \textit{select}) can be {more} easily transferred using fewer samples. Applications with multiple kernels have a larger optimization space. The large optimization space leads to more complex interactions that have compounding effects with other optimization options because we are %trying to optimize 
{modeling for} multiple kernels rather than just a single~kernel. 
Additionally, simple kernels such as \textit{sc} and \textit{select} have been implemented using \textit{hls stream} interfaces. Here rather than storing intermediate data in local FPGA memories, we read streams of data, and hence certain complex optimizations (like array partitioning) cannot be applied. This leads to a change in the feature space of different environments.
%\jgl{I don't see how this sentence is relevant for the observations}.  

Third, less severe changes are more amenable to transfer as the source, and target models are more closely related, e.g., %change 
{transferring} to CAPI1 {(PCIe Gen3 with $\sim$~3.3 GB/s bandwidth)} %is 
{from low-end PYNQ with PCIe Gen2 $\sim$~1.2 GB/s bandwidth }
{entails} a smaller increment in bandwidth %technology 
than moving to CAPI2, which offers R/W bandwidth of $\sim$~12.3 GB/s. 

Fourth, %change 
 change in {the} technology node from one FPGA to another has a lower impact than changing the external bandwidth to a new {interconnect} standard on the {transferring} process.

Figure~\ref{fig:LEAPER_SIGMETRICS/across_app} shows \namePaper's accuracy for transferring ML models \emph{across different applications}. We make the following three observations.
First, we make a similar observation in the case of transferring models across different platforms: as we increase the number of training samples, the mean relative error for most applications decreases. 
{Second, we notice} that the most considerable improvement %happened
{in accuracy occurs} when our sample size $(c_{tl})$ %was
{is} between 2 to 10. In most cases, {the accuracy} saturates after 20 samples. 
{Third}, in some cases, we see a decrease in accuracy {when increasing the number of samples}. This result could be attributed to training with a small amount of data, which can sometimes lead to overfitting~\cite{dai2007boosting}. 
%Further, in 

We %provide explainability of 
{further explain} our results by measuring the divergence of performance distributions to quantify the statistical distance between the source and target models, see Section~\ref{subsection:LEAPER_SIGMETRICS/relatedness_analysis}. We also compare the average accuracy of predicting performance across boards and applications using different TLs (see Table~\ref{tab:LEAPER_SIGMETRICS/compare}).
\\
\input{LEAPER_SIGMETRICS/tables/hardware.tex}
% \footnotetext{IBM and POWER9 are registered trademarks or common law marks of International Business Machines Corp., registered in many jurisdictions worldwide. Other product and service names might be trademarks of IBM or other companies.}
\noindent \textbf{Resource Model Transfer.} By using \namePaper, %~approach, 
we can also train a resource consumption model on a \textit{low-end} source environment and transfer it to a high-end cloud target environment.  Figure~\ref{fig:LEAPER_SIGMETRICS/area_transfer} shows the accuracy of a target model trained by \textit{5-shot} {transfer} learning for predicting %configuration 
{a} resource utilization vector $\eta_{\{BRAM, FF, LUT, DSP\}}$. Note:~the reported accuracy is for the transferred model, i.e., using a base model (low-end FPGA) to predict a target model (high-end {cloud} FPGA) after few-shot learning. 

In Figure~\ref{fig:LEAPER_SIGMETRICS/area_board}, the horizontal axis depicts the target platform, while the base learner is trained on a PYNQ-Z1 board. In the case of an application model transfer (Figure~\ref{fig:LEAPER_SIGMETRICS/area_app}), the platform remains unchanged (PYNQ-Z1), while the base learner application changes (horizontal axis).
We make %two 
{three} observations. First, the resource model shows low error rates for predicting BRAM and DSP. This is attributed to the fact that the technological configuration of these resources remains relatively unchanged across platforms (e.g., BRAM is implemented as 18 Kbits in both the source and target platforms). Second, flip-flops and look-up-tables have %a 
comparably higher error rates %that is 
because the configuration of CLB\footnote{A configurable logic block (CLB) is the fundamental component of an FPGA, made up of look-up-tables (LUTs) and flip-flops (FF).} slices varies with %change in 
{the} transistor technology and FPGA family. {Third}, Figure~\ref{fig:LEAPER_SIGMETRICS/area_app} shows the mean accuracy for transferring different application-based models on a fixed FPGA board. %In this figure, we see a
{We observe} relatively low accuracy for DSP consumption while transferring a base model trained on \textit{hist}. This low accuracy is because the \textit{hist} FPGA implementation does not make use of DSP units. However, all other applications utilize DSPs. Therefore, the ML model trained on \textit{hist} is not able to perform well in other \textit{transferred} environments.


\begin{figure}[h]
\begin{subfigure}[b]{\textwidth}
\centering
   %\includegraphics[width=1\linewidth,trim={2.2cm 8cm 0cm 7cm},clip]{LEAPER_SIGMETRICS/images/area_board.pdf}
   \includegraphics[width=0.6\linewidth]{LEAPER_SIGMETRICS/images/area-board-2.pdf}
         \phantomcaption
    \label{fig:LEAPER_SIGMETRICS/area_board} 
    \vspace{0.1cm}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\centering
   %\includegraphics[width=1\linewidth,trim={1.8cm 12cm 0.5cm 12cm},clip]{LEAPER_SIGMETRICS/images/area_app.pdf}
   \includegraphics[width=0.6\linewidth]{LEAPER_SIGMETRICS/images/area-app-2.pdf}
      \phantomcaption
    \label{fig:LEAPER_SIGMETRICS/area_app}
%   \caption{\label{fig:area_app}}

\end{subfigure}
\vspace{-0.3cm}
\caption[Two numerical solutions]{\namePaper's average accuracy for transferring FPGA resource usage models through \textit{5-shot} using (a) a base learner trained on a low-end PYNQ-Z1 to different high-end target FPGA boards (horizontal axis), and  (b) different applications as base learners (horizontal axis) to all the target applications, on low-end PYNQ-Z1 board.
% \gaganCheck{Could we change x-axix from target model to target FPGA/platform}
}
\label{fig:LEAPER_SIGMETRICS/area_transfer} 
\end{figure}
\input{LEAPER_SIGMETRICS/tables/compare.tex}
\subsection{Target {Cloud FPGA }Model Building Cost}
\label{subsection:LEAPER_SIGMETRICS/timing}
Table~\ref{tab:LEAPER_SIGMETRICS/timing} shows the time for collecting (see ``DoE run %(mins)
{(hours)}'') {the 50 sampled DoE configurations ($c_{lhs}$) {that we use} to gather training data. {Please note that while the process of synthesis and P\&R of the high-end system's FPGA, which is needed to obtain the maximum operating clock frequency and the resources' utilization, can be carried out offline, most of the cloud providers are offering VMs with all the appropriate software, IPs and licenses needed to generate an FPGA image ready to be deployed at their cloud infrastructure (e.g., the Vivado AMI of AWS~\cite{AMI}). This justifies the argument of the cost of the cloud environment for DoE runs. Specifically, we use a Linux image with FPGA and SoC development tools, IPs, and licenses to generate bitstreams for the selected Xilinx devices of Table~\ref{tab:LEAPER_SIGMETRICS/systemparameters} on the Nimbix cloud.}

Table~\ref{tab:LEAPER_SIGMETRICS/timing} also includes the {execution} time %for execution 
on the ADM-PCIE-KU3 {cloud} platform (``Exec (msec)'') and the transfer time (``Transfer (msec)'') for each model}. By using transfer learning, the DoE runtime is amortized and, by using a few labeled samples $c_{tl}$ (``5-shot (hours)'') from the target platform, we can transfer a previously trained model and make predictions for all the other configurations for the target platform. %Thus, 
{As a result}, quick exploration and {significant} time savings {(at least 10.2$\times$) are possible when transferring a model (i.e., ``5-shot (hours)'' + ``Transfer (msec)'') as compared to building a new model from scratch (i.e., ``DoE run (hours)'') + ``Exec (msec)'')}. Note, LHS reduces training samples from 500+ to 50, while  \textit{5-shot} transfer learning further reduces this space to 5, so we achieve $100\times$ effective~speedup compared to a traditional ``brute-force'' approach.

\input{LEAPER_SIGMETRICS/tables/timing.tex}


Table~\ref{tab:LEAPER_SIGMETRICS/low_high_end} mentions the performance and resource utilization for our considered applications both on a low-end system and a high-end cloud system. We use \namePaper to obtain the performance and resource utilization for the high-end cloud configuration.
\input{LEAPER_SIGMETRICS/tables/values}

\subsection{Base Model Accuracy Analysis}
We also evaluate the accuracy of our base model. The base model (Section~\ref{subsec:LEAPER_SIGMETRICS/base_model}) is trained on our low-end edge PYNQ board using $c_{lhs}$ configurations sampled using LHS. The base can predict performance (resource utilization) outside the base learner dataset (DoE configurations) $c_{lhs}$ (see Figure~\ref{fig:LEAPER_SIGMETRICS/transfer_overiew}). To assess our base model, we use 30 previously unseen configurations that are not part of $c_{lhs}$ on the base system, and we evaluate the mean relative error for all 30 unseen configurations on all six applications.  Figure~\ref{fig:LEAPER_SIGMETRICS/base_mode} shows \namePaper's base model accuracy results. 

We compare \namePaper~to three other ML algorithms
that are also trained using $c_{lhs}$ configurations to predict performance and resource consumption: XG-Boost (XGB) based on  Dai~\etal~\cite{dai2018fast},
an artificial neural network (ANN) used by Makrani~\etal~\cite{xppe_asp_dac} and a traditional
decision tree (DT). We make three observations. First, on average, \namePaper~is more accurate in terms of performance (resource utilization) prediction than the other ML models. Second, XGBoost is more data-efficient than ANNs~\cite{dai2018fast} and can perform better than decision trees~\cite{NAPEL}. Third, ANN is more accurate than the decision tree, but it is less accurate
than \namePaper. This is because ANN requires a much larger
training dataset to reach LEAPER’s accuracy~\cite{li2018processor}. 


 \begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth,trim={0.2cm 0.1cm 0.1cm 0.1cm},clip]{LEAPER_SIGMETRICS/images/BASE_MODEL_FPGAS.pdf}
  
  \caption{Mean accuracy for performance and resource utilization predictions using \namePaper's base model~vs. other methods: XGB (XGBoost), an artificial neural network (ANN), and a decision tree (DT).   }
  \label{fig:LEAPER_SIGMETRICS/base_mode}
  %\vspace{-0.5cm}
 \end{figure}
 
\subsection{{Why Does \namePaper~Work?}}
 \label{subsection:LEAPER_SIGMETRICS/relatedness_analysis}
{To explain our transfer learning results}, we analyze the degree of \textit{relatedness} between the source and target environments. 
We perform a correlation analysis followed by a divergence analysis of the performance distributions of the environments.

{Using the correlation analysis,} we make the following four observations. First, we see a high correlation of 0.76 to 0.97 {between the source and target  execution time for different target hardware platforms}, which indicates that the target model's performance behavior can easily be learned using the source environment.  
%
As the linear correlation is not 1 for all platforms, the use of a nonlinear transfer model is substantiated. Second, as we increase the external bandwidth {of the target platform (i.e., CAPI1 to CAPI2)}, 
the correlation becomes lower because the hardware change is much more \textit{severe}, coming from a low-end FPGA with limited external bandwidth. 
Third, compared to using a single transfer learner, an ensemble of learners %was 
can perform more accurate and robust predictions (see Figure~\ref{fig:LEAPER_SIGMETRICS/acros_board}, Figure~\ref{fig:LEAPER_SIGMETRICS/across_app}, and Figure~\ref{fig:LEAPER_SIGMETRICS/area_transfer}). 
Fourth, the correlation between applications on a single platform is lower (0.45 to 0.9) because of {the} varying application characteristics {and optimization space.}

We measure the relatedness of the performance distributions of the source ($P(\tau_{s})$) and the target applications  ($P(\tau_{t})$) because application-based environments exhibit a low linear correlation. We employ the Jensen-Shannon Divergence (JSD)~\cite{jsd} (see Table~\ref{tab:LEAPER_SIGMETRICS/jsd}) to quantify the statistical distance between $P(\tau_{s})$ and $P(\tau_{t})$. The lower the values of JSD, the more similar the target environment is to the source (i.e., if $D_{JSD}(P(\tau_{t}) || P(\tau_{s}))=0$ implies the distributions are identical, and 1 indicates unrelated distributions). This analysis confirms the trend observed from transferring application models (Figure~\ref{fig:LEAPER_SIGMETRICS/across_app}), i.e., the more closely related the source and target applications, %are 
the fewer %numbers of 
samples are required to train our nonlinear transfer learners. The measured distance between the tasks is proportional to the error of the target~task. {As can be seen from Table~\ref{tab:LEAPER_SIGMETRICS/jsd}  for many applications, transfer learning to build accurate models is feasible since their JSD is limited. } {Similar trends are observed for the resource~utilization~model.}


\input{LEAPER_SIGMETRICS/tables/jsd.tex}

\subsection{Discussion and Limitations}
 \label{subsection:LEAPER_SIGMETRICS/limit}
 \paragraph*{\textbf{Transfer to a new platform and application simultaneously.}}
In supervised learning, transferring both to a new platform and application at the same time would lead to sub-optimal results (as observed in~\cite{xapp}). This is because we would perform two-levels of the transfer. Moreover, the ML model needs to have some notion of the target environment. Therefore, we explicitly exclude this option in this chapter.

\paragraph*{\textbf{FPGA resource-constrained environments.}}
{During partial reconfiguration~\cite{beckhoff2012go} or in a multi-tenant environment~\cite{pourhabibi2020optimus}, we are often constrained by limited resources~\cite{ting2020dynamic}. In such scenarios, resource management is more efficient to be controlled by a middleware layer~\cite{vaishnav2020fos}. We do not assume such as a middleware. Therefore, our analysis targets bare-metal systems. In the future, we aim to extend our work to such scenarios as well.}
{
\paragraph*{\textbf{\namePaper~generality to other platforms.}}
\namePaper, in essence, is a framework for building and then transferring models from a small edge platform to any new, unknown FPGA-based environment. We demonstrated our approach using the cloud as our target environment because cloud systems often use expensive, high-end FPGAs, e.g., Amazon AWS~F1 cloud~\cite{aws}, Alibaba Elastic cloud with FPGAs~\cite{alibaba}, etc. Thus, we can achieve tangible gains in terms of cost, efficiency, and performance.
}

\paragraph*{\textbf{Effect of FPGA resource saturation.}}
% Our primary focus was to use a low-cost FPGA-board (available offline) for building a model using traditional ML technique and then leverage transfer-learning to reuse the same model for prediction of high-end server-grade FPGAs (e.g., in the cloud, where data collection could be expensive or even error-prone). Our approach dramatically reduces the number of costly trials on the high-end FPGA. We limit ourselves to designs that fit on the small FPGA capacity because the major contribution of this approach lies in the ability to transfer learning from low-end edge FPGA to high-end cloud FPGAs. 


An FPGA gives us the flexibility to map operations to different resources. For example, we can map a multiplication operation either to a CLB or a DSP slice. The deciding factor is the operand width (as shown in Appendix~\ref{chapter:precise_fpga}). If the operand width is smaller than the DSP slice width, the operation is mapped to a CLB else to a DSP unit. An ML-model can be trained to learn such relations. However, we avoid it in our current chapter.




==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/application.tex <==

\begin{table}[h]
  \caption{{  Evaluated applications; description including their major kernels and the input dataset. For major kernels, we mention the optimization space where $\times$ represents the optimization being applied to multiple loops or elements. see Table~\ref{tab:LEAPER_SIGMETRICS/pragma} for description of the optimization options.}}
    \label{tab:LEAPER_SIGMETRICS/app_details}
        \renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{14pt}
  \resizebox{1\linewidth}{!}{%
\begin{tabular}{l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l@{\hspace{0.9\tabcolsep}}l}
\toprule
  \textbf{Application}                  & \textbf{Domain} & \textbf{Major Kernels}     & \textbf{Dataset}    & \textbf{Optimization space}                                                                     \\ \hline
    blstm~\cite{diamantopoulos2018ectalk} &  \begin{tabular}[c]{@{}l@{}} Machine \\learning\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Hidden lay. fw\\ Hidden lay. back \\ Output layer\end{tabular} & Fraktur OCR~\cite{yousefi2015binarization} & 
    \begin{tabular}[c]{@{}l@{}}2$\times$PL, 3$\times$PR(2,4) I, 2$\times$U \\ 2$\times$PL, I, 2$\times$U  \\ PL, I, U+D, R, W, F\end{tabular}

\\\hline 
    
     cedd~\cite{gomez2017chai}             & \begin{tabular}[c]{@{}l@{}}  Image \\  proc. \end{tabular}   & \begin{tabular}[c]{@{}l@{}}
     Gaussian filter\\
     Sobel filter\\
    Suppress. filter\\
    Hysteresis filter\\
    \end{tabular}            & \begin{tabular}[c]{@{}l@{}}   Frame-354$\times$626 \\ 1000 frames               \\
    \end{tabular}  &
    \begin{tabular}[c]{@{}l@{}}  
    PL, PR(2,4), I, U\\
    PL, PR(2,4), I, U\\
    PL, PR(2,4), I, U\\
    PL, I, U+D, R, W, F\\
    
    
     \end{tabular} 
    \\
\hline 
    digit~\cite{zhou2018rosetta}             & \begin{tabular}[c]{@{}l@{}}  Machine \\learning \end{tabular}    & \begin{tabular}[c]{@{}l@{}}Hamming dist.\\
    KNN voting\end{tabular}          & \begin{tabular}[c]{@{}l@{}} MNIST\\18000 train \\
    2000 test  \end{tabular}        &       \begin{tabular}[c]{@{}l@{}}       
     2$\times$PL, 3$\times$PR(2,4), I, 4$\times$U\\
I+R,W,F\\

\end{tabular}
\\\hline 
    
 
    hist~\cite{gomez2017chai}                      &\begin{tabular}[c]{@{}l@{}}   Image\\ proc.  \end{tabular}   & Histogram avg.     &    \begin{tabular}[c]{@{}l@{}}   Input-1536$\times$1024      \\
    Bins-256\\
        \end{tabular} & \begin{tabular}[c]{@{}l@{}} PL, PR(all), I, D,\\ R, W, U, F  \end{tabular} \\
\hline 

    
   select~\cite{gomez2017chai}         & \begin{tabular}[c]{@{}l@{}}   Data-\\ base  \end{tabular}         & Selection                                                                         &     1048576 inputs        & \begin{tabular}[c]{@{}l@{}}  PL, I, D, R, W, F       \end{tabular}     
   \\\hline 
   
    sc~\cite{gomez2017chai}                & \begin{tabular}[c]{@{}l@{}}   Data\\ reorg.  \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Count\\ Compact\end{tabular}       &                  1048576 inputs    & \begin{tabular}[c]{@{}l@{}}PL, I, D, R, W, U, F       \end{tabular}          \\ \bottomrule
\end{tabular}
}
\end{table}


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/compare.tex <==
\begin{table}[t]
\centering
  \caption{Average accuracy (\%) comparison of \namePaper~ with decision tree (DT) and adaBoost (ADA) as TL for~\textit{5-shot}~transfer.}
    \label{tab:LEAPER_SIGMETRICS/compare}
    {\footnotesize
    \renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{14pt}
    \resizebox{0.65\linewidth}{!}{%
\begin{tabular}{@{}llll@{}}
\hline
\textbf{Environment}               & \textbf{DT}   & \textbf{ADA}   & \textbf{\namePaper} \\ \midrule
Across Board       & 77.7 & 83.2 & 89.8  \\
Across Application & 70.6 & 73.5 & 81.2   \\ \hline
 \vspace{-0.3cm}
\end{tabular}
}}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/hardware.tex <==
% Please add the following required packages to your document preamble:
% 

\begin{table}[t]
\centering
  \caption{System parameters and configuration.}
    \label{tab:LEAPER_SIGMETRICS/systemparameters}
    \renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{14pt}
    \resizebox{\linewidth}{!}{
\begin{tabular}{@{}lllllr@{}}
\toprule
\multicolumn{5}{l}{\textbf{Low-end base system}} & \textbf{Indicative price}                                                                                                                                                                               \\ \midrule

\textbf{Embedded Board}    & 
\multicolumn{4}{l}{ PYNQ-Z1 ZYNQ~\cite{zynq} XC7Z020-1CLG400C } & \$199\footnote{https://store.digilentinc.com/pynq-z1-python-productivity-for-zynq-7000-arm-fpga-soc/, Accessed 12 Jan. 2021} \\

&\multicolumn{4}{l}{ARM Cortex-A9 processor  @650MHz, dual-core} \\ 

\toprule
\toprule
\multicolumn{5}{l}{\textbf{{On-prem cloud} target system with OpenStack\cite{openstack} and KVM Hypervisor}}                                                                                                                                                                               \\ \midrule
\textbf{Host Configuration}    & 
\multicolumn{4}{l}{IBM\textsuperscript{\textregistered} POWER9 AC922 @2.3 GHz, 16 cores} & \$55000-\$75000\footnote{https://www.microway.com/product/ibm-power-systems-ac922/, Accessed 12 Jan. 2021} \\ 
&\multicolumn{4}{l}{4-way SMT, 32 KiB L1 cache,256 KiB L2 cache,} \\ 
&\multicolumn{4}{l}{10 MiB L3 cache, 16x32GiB RDIMM DDR4 2666 MHz \footnote{.}} \\ 

\midrule
\textbf{FPGA Description} & \multicolumn{4}{l}{}                                                                                                                                 &                             \\ 
% \textbf{FPGA Family}      & Zynq            & Virtex UltraScale\tnote{+}            & Virtex UltraScale\tnote{+}            & Kintex UltraScale\tnote{+}            & Kintex UltraScale            & Kintex UltraScale           \\
% \textbf{Board}            &                 & Semptian NSA241                   & ADM-PCIE-9V3                 & N250SP                            & ADM-PCIE-8K5                 & ADM-PCIE-KU3                \\
% \textbf{Device}           &  Z7020-2               & XCVU9P-2                          & XCVU3P-2                     & KU15P-2                           & XCKU115-2                    & XCKU060-2                   \\
% \textbf{Interface}        &                 & CAPI-2                            & CAPI-2                       & CAPI-2                            & CAPI-1                       & CAPI-1                      \\ \bottomrule

 \textbf{Board} &\textbf{FPGA Family}        &\textbf{Device}   &\textbf{Interface}   \\    
ADM-PCIE-8K5~\cite{ad8k5}   &Kintex UltraScale &XCKU115-2   & CAPI-1  & & N/A \\
ADM-PCIE-KU3~\cite{adku3}    &Kintex UltraScale &XCKU060-2  & CAPI-1  & & N/A \\
Semptian NSA241~\cite{nsa241}& Virtex UltraScale\tnote{+} &XCVU9P-2  & CAPI-2  & & N/A  \\
ADM-PCIE-9V3~\cite{ad9v3}   &Virtex UltraScale\tnote{+} & XCVU3P-2  & CAPI-2   & & N/A  \\
N250SP~\cite{250SP}&Kintex UltraScale\tnote{+} &KU15P-2  &CAPI-2  & & N/A  \\      
\bottomrule
\end{tabular}
}
\begin{flushleft}
\scriptsize \textsuperscript{6} https://store.digilentinc.com/pynq-z1-python-productivity-for-zynq-7000-arm-fpga-soc/, Accessed 12 Jan. 2021.\\
\scriptsize \textsuperscript{7} https://www.microway.com/product/ibm-power-systems-ac922/, Accessed 12 Jan. 2021.\\
N/A\footnote{.}: Not available indicative price from an online store, but in the region of \$2500-\$5000 for our purchased on-prem cards.

\end{flushleft}
\end{table}


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/jsd.tex <==
    \begin{table}[h]
\centering
  \caption{Jensen-Shannon Divergence (JSD)~\cite{jsd} between %different application's 
  performance distributions of {different applications}. JSD measures statistical distance between two probability distributions.}
    \label{tab:LEAPER_SIGMETRICS/jsd}
      {\footnotesize
    \renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{14pt}
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{@{}clllllll@{}}
\toprule   
\multirow{10}{*}{\rotatebox{90}{\textbf{Target Model}}} & \multicolumn{7}{c}{\textbf{Base Learner}}\\

                              & \multicolumn{1}{l}{}       & blstm & cedd & digit & hist & sc   & select \\ %\cmidrule(l){2-8} 
                              \cmidrule{2-8} 
                              & \multicolumn{1}{l|}{blstm}  & 0.00     & 0.24 & 0.34  & 0.25 & 0.31 & 0.30   \\
                              & \multicolumn{1}{l|}{cedd}   & 0.24  & 0.00     & 0.49  & 0.54 & 0.41 & 0.40   \\
                              & \multicolumn{1}{l|}{digit}  & 0.34  & 0.49 & 0.00      & 0.25 & 0.21 & 0.21   \\
                              & \multicolumn{1}{l|}{hist}   & 0.25  & 0.54 & 0.25  & 0.00     & 0.25 & 0.24   \\
                              & \multicolumn{1}{l|}{sc}     & 0.30  & 0.40 & 0.21  & 0.24 & 0.00     & 0.05   \\
                              & \multicolumn{1}{l|}{select} & 0.30  & 0.41 & 0.21  & 0.25 & 0.05 & 0.00       \\ \bottomrule
\end{tabular}
}}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

%\vspace{-0.1cm}

\begin{table}[h]
\centering
\caption{Main application features extracted from LLVM.}
\label{tab:LEAPER_SIGMETRICS/application_features}
\footnotesize
\begin{tabular}{p{0.24\linewidth} p{0.62\linewidth}}
\toprule
\textbf{Application Feature} & \textbf{Description} \\ 
\midrule
Instruction Mix & Fraction of instruction types (integer, floating point, memory read, memory write, etc.) \\
ILP                      & Instruction-level parallelism on an ideal machine. \\
Data/Instruction reuse distance   & For a given distance $\delta$, probability of reusing one data element/instruction (in a certain memory location) before accessing $\delta$ other unique data elements/instructions (in different memory locations). \\
Register traffic    & Average number of registers {per} instruction. \\
Memory footprint    & Total memory size used by the application. \\ 
\bottomrule

\end{tabular}
\end{table}


%For a given data distance $\sigma$, the probability that a memory \juan{location} is reused before accessing other $\sigma$ unique memory \juan{locations.} \\
%For a given instruction distance $\delta$, the probability that a memory \juan{location} is reused before accessing other $\delta$ unique memory \juan{locations.}    \\
%The percentage of operations that need to access the next level of memory hierarchy\\
%The average number of register read and write operations \\


==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/pragma_configuration.tex <==
\begin{table}[h]
\centering
  \caption{{The FPGA configuration options used to train our ML-models.}}
%   \caption{ Overview of terms related to the considered FPGA configuration options}
    \label{tab:LEAPER_SIGMETRICS/pragma}
%     \renewcommand{\arraystretch}{0.7}
% \setlength{\tabcolsep}{14pt}
\footnotesize   
        \resizebox{\linewidth}{!}{%
\begin{tabular}{p{0.25\linewidth} p{0.62\linewidth}}
\toprule
\textbf{Configuration} &  \textbf{Description}  \\ \midrule
Pipelining (PL)       &   Enabled/Disabled \\
Partitioning (PR)   &  Block/Cyclic/Complete (Factor: $2^n, 1\leq n \leq 6$)) \\

Inlining (I)        &   Enabled/Disabled function inlining \\
Dataflow (D)        &  Task level pipelining \\
Read burst (R)     &   Read data burst from the host \\
Write burst (W)    &   Write data burst from the host \\
Unrolling  (U)     &   Unrolling factor (Factor: $2^n, 1\leq n \leq 6$) \\
% Replication     &  Kernel duplication factor   \\
FPGA Frequency (F)     &  Four-different frequency levels for the FPGA logic   \\
\bottomrule
\end{tabular}
}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/timing.tex <==
\begin{table}[h]
%\HUGE
%\renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{14pt}
\caption{DoE time for gathering sampled data points for a single CPU-FPGA platform (``DoE run (hours)''), DoE execution time on the deployed platform (``Exec (ms)''), Estimated Cost on a cloud platform (``Est. Cost (\$)''), time for gathering 5 labeled samples (``5-shot (hours)''), \namePaper~time including the transfer time (``Transfer (msec)''), ``Speedup'' over building a new model from scratch using just the DoE data (still 
{more} cost-efficient than traditional ``brute-force'' training).}
\label{tab:LEAPER_SIGMETRICS/timing}
\centering
\resizebox{\linewidth}{!}{%
%\begin{tabular}{p{0.1\linewidth}|lll|lll|l}
 \begin{tabular}{l|lll|lll|l}
% \begin{tabular}{p{0.1\linewidth}|p{0.14\linewidth}p{0.12\linewidth}p{0.14\linewidth}p{0.11\linewidth}}
% \begin{tabular}{p{1.2cm}|p{1.1cm}p{1.6cm}p{1.8cm}p{1.2cm}}
\hline
\multicolumn{1}{c}{\textbf{Application}}  & \multicolumn{7}{c}{\textbf{Transfer Time}}  \\ 

Name &
 \begin{tabular}{l}    
 DoE run \\(hours)
\end{tabular}&
 \begin{tabular}{l}      
Exec \\(msec)

\end{tabular}&
 \begin{tabular}{l}    
Est.Cost$^{7}$\\(\$)

\end{tabular}&
 \begin{tabular}{l}    
5-shot \\(hours)

\end{tabular}
& \begin{tabular}{l} 
Transfer \\(msec)

\end{tabular}&
 \begin{tabular}{l}  
Est.Cost$^{7}$\\(\$)

\end{tabular}
&
 \begin{tabular}{l} 
Speedup\\

\end{tabular} \\
%Speedup\\ 
\hline
blstm   &  135  &  1245 & 168.7 & 13 & 55.6 & 16.2 & 10.4  \\

cedd    &  124  & 2217 & 155.0 & 12 & 26.5 & 15.0 & 10.3 \\

digit   & 122   & 873 & 152.5 & 12 & 58.8 & 14.9 & 10.2\\

hist    & 97  &  1104  &  121.2 & 9 & 17.1   & 11.3 & 10.8   \\

sc      & 104  & 4018 &  130.0 & 10 & 27.9 & 12.4 & 10.4 \\

select  &  106   & 3978 & 132.5 & 10 & 27.6 &  12.5 & 10.6 \\

\hline
%   \multicolumn{8}{l}{$^{7}$\large{The cost is estimated based on an enterprise online cost estimator~\cite{nimbix-calc}, using a public-cloud system with configuration  akin to  }} \\
%   \multicolumn{8}{l}{\large{our on-prem system. Specifically, we have selected an \textit{n2}~(8-core, 64GB RAM VM - 1.25\$/h) for bitstream generation (x86) and}} \\
%   \multicolumn{8}{l}{\large{an \textit{np8f1}  instance (160-thread POWER8, 1TB RAM, ADM-PCIE-KU3 with CAPI-1 - 3\$/h) for deployment.}} \\
\end{tabular}
}
%   \multicolumn{8}{l}{$^{7}$\large{The cost is estimated based on an enterprise online cost estimator~\cite{nimbix-calc}, using a public-cloud system with configuration  akin to  }} \\
%   \multicolumn{8}{l}{\large{our on-prem system. Specifically, we have selected an \textit{n2}~(8-core, 64GB RAM VM - 1.25\$/h) for bitstream generation (x86) and}} \\
%   \multicolumn{8}{l}{\large{an \textit{np8f1}  instance (160-thread POWER8, 1TB RAM, ADM-PCIE-KU3 with CAPI-1 - 3\$/h) for deployment.}} \\

\begin{flushleft}
{\tiny{$^{7}$The cost is estimated based on an enterprise online cost estimator~\cite{nimbix-calc}, using a public-cloud system with configuration  akin to  
our on-prem system. Specifically, we have selected an \textit{n2}~(8-core, 64GB RAM VM - 1.25\$/h) for bitstream generation (x86) and 
an \textit{np8f1}  instance (160-thread POWER8, 1TB RAM, ADM-PCIE-KU3 with CAPI-1 - 3\$/h) for deployment.} \\
}
\end{flushleft}

\end{table}

% blstm   &  135  &  9.1 & 13 & 10.1 & 10.4  \\

% cedd    &  124  & 2.9 & 12 & 12.0 & 10.3 \\

% digit   & 122   & 8.7 & 12& 15.3 & 10.2\\

% hist    & 97  &  0.9  &   9& 12.5   &  10.8   \\

% sc      & 104  &   2.9  &  10& 12.7 & 10.4 \\

%select    & 104  &   2.9  &  10& 12.7 & 10.4 \\

==> PhD_Thesis_Updated_arxiv (1)/LEAPER_SIGMETRICS/tables/values.tex <==
\begin{table}[h]
  \caption{{Execution time and resource utilization for low-end base configuration (PYNQ-Z1) and high-end cloud configuration, a Nimbix \textit{np8f1} instance (POWER8, ADM-PCIE-KU3 with CAPI-1).}}
 \label{tab:LEAPER_SIGMETRICS/low_high_end}
    \renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{14pt}
  \resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\textbf{Application} & \textbf{Config.} & \textbf{Exec (msec)} & \textbf{BRAM} & \textbf{DSP} & \textbf{FF} & \textbf{LUT} \\ \hline
\multirow{ 2}{*}{blstm}         &      low-end              &   4200              &    80\%       &    15\%          &     24\%           &   47\%           \\
                                &high-end  &   1245              &    62\%       &    8\%          &     12\%           &   21\%           \\

\multirow{ 2}{*}{cedd}          &    low-end                &    10254              &     83\%          &    37\%          &   95\%          &     97\%         \\
                                &   high-end &    2217             &   56\%                &      3\%          &   75\%            &              94\%         \\

\multirow{ 2}{*}{digit}         &    low-end                &   2458             &     94\%              &       33\%         &     79\%          &            85\%     \\
                                & high-end  &       873          &     84\%              &       12\%         &     24\%          &            75\%              \\

\multirow{ 2}{*}{hist}          &    low-end                &    6173              &      94\%         &     0\%         &     11\%       &         37\%     \\
                                &  high-end  &   1104              &     67\%             &    0\%           &    5\%          &             30\%           \\

\multirow{ 2}{*}{sc}            &   low-end                 &   19306              &    82\%       &    0.4\%          &     12\%           &   25\%           \\
                                &high-end  &   4018              &    91\%       &    0.1\%          &     12\%           &   23\%     \\
 
\multirow{ 2}{*}{select}        &       low-end              &   18306              &    82\%       &    0.4\%          &     12\%           &   25\%           \\
                                &high-end  &   3918              &    91\%       &    0.1\%          &     12\%           &   23\%     \\


   \bottomrule
\end{tabular}
}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/abstract.tex <==
 With the emergence of three-dimensional stacking, the decade-old concept of placing compute units close to the memory has become more viable. Essentially, processing right at the ``home" of data to eliminate unnecessary data movement is referred to as near-memory computing (NMC). 

To harness the power of these architectures, having a high-level performance model can offer fast turnaround times in early design stages. This paper proposes an NMC model that combines technology parameters and application specific characteristics to evaluate the performance of a workload. A statistical design of experiment (DoE) methodology is first employed to select a set of representative design points for simulation. These sampled points well represent the whole space of possible input configurations. Then, ensemble learning is leveraged to develop a model that can predict performance metrics for new unseen applications on these novel architectures. Further, this model can act as a classifier to predict whether or not should an application be offloaded to NMC cores.  The experimental results demonstrate that, by using DoE, we can extract more informative training data with a minimal number of experimental runs. Thus, we save a significant amount of simulation overhead with respect to a traditional exhaustive brute-force approach of random data selection. Besides minimizing the number of experiments, our inexpensive performance model can provide, on average, an additional 10$\times$ reduction in performance evaluation time with an error rate lower than 15\% compared to a computationally-intensive state-of-the-art NMC simulator.



==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/abstractDAC.tex <==
% Processing right at the "heart" of data to eliminate unnecessary data movement is referred to as near-memory computing (NMC). To harness the power of these architectures, having a high-level performance model can offer fast turnaround times in performance and energy estimation of an application. To this end, we propose an NMC model that combines technology parameters and application specific characteristics. A statistical design of experiment (DoE) methodology is first employed to select a set of representative design points for simulation which saves a significant amount of simulation overhead. Then, ensemble learning is leveraged to develop a model that can predict performance metrics and identify potential offload candidates on these novel architectures. Our NMC performance model can provide rapid exploration with an error rate lower than 15\% compared to a state-of-the-art NMC simulator.
\vspace{-0.1cm}

The cost of moving data between the memory/storage units and the compute units is a major contributor to the execution {time} and energy consumption of modern workloads in computing systems.
{A promising paradigm} to alleviate {this} \emph{data movement bottleneck} is near-memory computing (NMC), which consists of placing compute units close to the memory/storage units.
There is substantial {research} effort that proposes NMC {architectures and} identifies workloads that can benefit from NMC. System architects typically use simulation techniques to evaluate the performance and energy consumption of their designs. However, simulation is extremely slow, imposing long times for design space exploration.
In order to enable fast {early-stage} design space exploration of NMC {architectures}, {we need} high-level performance and energy models.

We present NAPEL, a high-level performance and energy estimation framework for NMC architectures. NAPEL leverages ensemble learning to develop a model that is based on microarchitectural parameters and application characteristics.
NAPEL training uses a statistical technique, called design of experiments, to collect representative training data efficiently. 
NAPEL provides early design space exploration $220\times$ faster than a state-of-the-art NMC simulator, {on average,} with error rates \juan{of} to 8.5\% and 11.6\% for performance and energy estimations, respectively, compared to {the} NMC simulator.
{NAPEL is also capable of making accurate predictions for previously-unseen applications.}

%A major trend to alleviate the \emph{data movement bottleneck} (i.e., the performance and energy cost of moving data between memory/storage and compute units) consists of placing compute units close to the memory/storage units, which is referred to as \emph{near-memory computing} (NMC). 
%In order to be able to carry out preliminary evaluations of NMC designs in a fast way, a high-level model for NMC is desirable. 
%%To harness the power of near-memory computing (NMC), having a high-level model can offer short turnaround times in performance estimation of applications. 
%%To this end, 
%In this work, we propose an NMC model that combines %hardware 
%microarchitectural parameters with application-specific characteristics to provide accurate performance and energy estimations. 
%An statistical design-of-experiment technique is used to select a set of design-points for simulation, which saves a significant simulation overhead. Then, ensemble learning is leveraged to develop a model that can identify potential offloading candidates. Our framework can provide rapid exploration with an error rate, on average, less than 8.5\% and 12\% for performance and energy estimation respectively compared to a state-of-the-art NMC simulator. 


% To harness the power of near-memory computing (NMC), having a high-level model can offer short turnaround times in performance estimation of applications. To this end, we propose an NMC application performance prediction framework using ensemble learning that combines hardware parameters and application-specific characteristics. A statistical design-of-experiment technique is used to select a set of design-points for simulation, which saves a significant simulation overhead. Our framework can identify potential offloading candidates and provide rapid exploration with an error-rate, on average, less than 8.5\% and 12\% for performance and energy estimation respectively compared to a state-of-the-art NMC simulator. 

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/analyticModel.tex <==


\begin{comment}
The near-memory processing time ($\Pi_{NMC}$) is divided into time spent in executing memory ($\Pi_{memory}$) and non memory ($\Pi_{non-memory}$) instructions.  This time corresponds to the memory model and compute-model respectively in Figure~\ref{fig:model}.
\begin{align}
\Pi_{NMC}=\Pi_{memory}+\Pi_{non-memory}\label{eq:1}
\end{align}
The performance model takes  into  account  the  time to process the instructions and latency due to memory access at  different memory  levels.
\end{comment}
% \sander{You should first explain why this model is needed. It now appears out of the blue.}
A near-memory processing system is modeled similar to a 3D stacked memory (JEDEC's High Bandwidth
Memory~\cite{6757501} or Micron's Hybrid Memory Cube~\cite{7477494}). These 3D-stacked memories are composed of a logic die upon which multiple DRAM layers are stacked. Each
memory chip consists of multiple vertical
DRAM partitions, called vaults, each with its DRAM
controller in the logic layer.
% These memories utilize a packet-based protocol by means of high-speed serializer/deserializer  (SerDes)  I/O  link. The external interface supports two or four links each with different configuration speeds depending upon bus width.
% Packets are partitioned into 16-byte elements, called flits. Supported packet sizes for data payloads range from one flit (16 B) to eight flits (128 B). Each packet also carries an eight-byte header and an eight-byte tail; therefore, each request/response has an overhead of one flit~\cite{hadidi2017demystifying}.

\begin{comment}


 We assume the number of reads and writes are evenly distributed across $n_{vaults}$ vaults. 
 \begin{align}
 n_{load}=n_r/n_{vaults}\label{eq:2}\\
 n_{store}=n_w/n_{vaults}\label{eq:3}\\
 m_{total}= n_{load}+n_{store}
 \end{align}
 
  The model estimates the memory instruction time as the ratio between the number of memory access required in order to move the block of data to and from a DRAM bank and the available I/O bandwidth inside each vault ($BW_{int}$).  We assume a close-page policy, and entire block from the row-buffer of size $b_{rb}$ is consumed by the processing element \textit{pe} in its vault. The total memory access time ($\Pi_{memory}$), when all the \textit{pe}'s $(n_{pe})$ make request to their own vault is given by
  
 \begin{align}
 \Pi_{memory}=\frac{1}{n_{pe}} \displaystyle \sum_{}^{N_{vaults}}\frac{m_{total}*b_{rb}}{BW_{int}}
  \end{align}


\jgl{In Eq. 2 and 3, you divide by the number of vaults. In Eq. 5, you add the contribution of all vaults. Because you don't have n\_r and n\_w per vault, dividing and then adding is a little bit dummy.}
\end{comment}
We embed the 3D memory with processing elements (PE) which are modeled as in-order single issue cores as in other works~\cite{7284059,7429299,DBLP:journals/corr/PicorelJF16} taking into account the limited thermal and area budget in the logic layer. We assume every vault has its own PEs and operates on the data mapped onto its vaults. 

These systems are evaluated in terms of total instructions executed per cycle, $IPC(\xi)$ . The total execution time $(\Pi_{NMC})$ is calculated from core performance as
 \begin{align}
\Pi_{NMC}=\frac{I_{Total}}{IPC(\xi).f_{core}}\label{eq:1}
 \end{align}
where $f_{core}$ is the frequency of in-order cores in the logic layer and $I_{Total}$ is the total offloaded instructions. The IPC ($\xi$) of processing elements in a near-memory processing system is obtained using the approach as described in Section \ref{subsec:machine learning}.


The host system is modeled as a traditional multi-core system with a cache hierarchy. In the host system, each core has its private L1 \& L2 cache and a shared L3 cache. 3D stacked near-memory system, with embedded compute units, is connected with a host system through a serializer/deserializer (SerDes) I/O link.

\begin{comment}

To fully utilize the high bandwidth provided, coalescing of the memory access are also taken into account. 

\section{Discussion}
Given the target computational element c an the SW memtrick vector vk, the system generates the following metrics:
\bold{(i) Number of trees voting for the suggested component}
(ii) Number of trees voting for target component c
iii Influences for each SW metric

In this work,, we are interested in verifying if the model is capable to predict efficiently accelerate a kernel k with respect to its software execution.

\subsection{Black box to white box Analysis}
\end{comment}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:napel/conclusion}
\vspace{-0.1cm}

%Data movement is a major performance and energy bottleneck in current computing systems that near-memory computing (NMC) can alleviate. 
%However, there is a lack of evaluation tools for performance and energy assessment for NMC exploration, other than time-consuming microarchitecture simulation. 
{We introduce} NAPEL, the first high-level \juan{machine learning}-based prediction framework for fast and accurate {early-stage} performance and energy-consumption estimation {on NMC architectures}.
NAPEL avoids time-consuming simulations to predict the performance and energy consumption of previously unseen applications on \juan{various} NMC architecture configurations. 
{To achieve this}, NAPEL relies on random forest, an ensemble learning technique, to build {its} prediction models. 
%First, NAPEL employs the design of experiment (DoE) methodology to select a small set of application-input configurations to gather training data using simulation. 
%Specifically, NAPEL uses a DoE variant called central composite design (CCD), which captures the interactions and non-linear effects between the application-input parameters and the application's performance and energy consumption. 
%Second, NAPEL trains the RF algorithm and tunes the algorithm's hyper-parameters to improve the prediction accuracy.

NAPEL is {$220\times$ faster} than a state-of-the-art NMC simulator, with an accuracy loss in performance (energy) prediction \juan{of only} 8.5\% (11.6\%) compared to the simulator. 
Compared to an artificial neural network, NAPEL is 1.7$\times$ (1.4$\times$) more accurate in performance (energy) prediction. 
NAPEL can accurately perform fast design-space exploration for different applications and NMC \juan{architectures}.
{We hope the NAPEL approach enables faster development of NMC systems and inspires the development of other alternatives to simulation for NMC performance and energy estimation.}
%For future work, we plan to accelerate the analyzed workloads on an IBM OpenPOWER platform, and to use NAPEL to analyze the benefits of offloading other applications to NMC. 
%For future work, we plan to use NAPEL to perform architectural design space exploration to find the best architecture configurations for different applications.


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/introduction.tex <==
\section{Introduction}
\vspace{-0.1cm}

% {Current computing systems are compute-centric: all computation takes place in the compute units while the memory/storage units are passive components.
% As a result, modern workloads (e.g., machine learning, graph processing, bioinformatics), spend a large fraction of execution time and energy on moving data between the memory/storage units and the compute units. 
% A way to alleviate this \emph{data movement bottleneck}~\cite{ghose2019, mutlu2019} is \emph{near-memory computing} (NMC), which consists of placing processing elements closer to memory.} 
% NMC is enabled by new memory integration technologies such as 3-D stacked memory~\cite{6757501,7477494,smla}, where multiple DRAM layers are stacked in the same chip with a logic layer that can embed processing elements. 
As discussed in Chapter~\ref{chapter:background}, past works~\cite{hsieh2016accelerating,Azarkhish:2016:DEP:2963802.2963805,tom, boroumand2016lazypim,googleWorkloads,kim2018grim, ahn2015pim,teserract,boroumand2019conda} show that NMC architectures can be employed {effectively} for a wide range of applications, {including graph processing, databases, neural networks, bioinformatics}. However, a common challenge all such past works {face} is how to evaluate the performance and energy consumption of the NMC {architectures} for different workloads systematically and {accurately} in a reasonable amount of time~\cite{singh2018review,mutlu2019}. In the early design stage, system architects use simulation techniques (e.g., \cite{7063219,tom, boroumand2016lazypim, Azarkhish:2016:DEP:2963802.2963805,teserract}) for architectural performance and energy evaluation.
However, this approach is extremely slow, because a single simulation for a real-world application with a representative dataset typically takes hours or even days. Specifically, the speed of a cycle-accurate simulator is in the range of a few thousand instructions per second~\cite{sanchez2013zsim}, which is {orders of magnitude} slower than native execution. 

\textbf{Our goal} is to enable fast early-stage design space exploration of NMC architectures without having to rely on time-consuming simulations. 
To this end, we propose the \textit{\underline{N}MC \underline{A}pplication performance and energy \underline{P}rediction framework using \underline{E}nsemble machine \underline{L}earning} (NAPEL). 
The key idea is to use ensemble learning to build a model that, once trained for a fraction of programs on a number of {architecture configurations}, can predict the performance and energy consumption of \emph{different} applications {on the same NMC architecture}. 
The ensemble learning mechanism we use is random forest (RF)~\cite{breiman2001random}. 
NAPEL can make performance and energy predictions for an {average} application on a specific architecture {$220\times$ faster} than using simulation.
%Such a model can then take orders of magnitude less time than actually simulating them. 
Previous ML-based approaches~\cite{6827943,calotoiu2013using,wu2011scalaextrap} {perform} extrapolations to predict, for example, the performance {of a known application} for a bigger dataset.
In contrast, NAPEL can make predictions for \emph{previously-unseen} applications, after being trained with data from applications that are different from the applications {that} we want to predict. %That is, NAPEL does not need any prior knowledge about the applications we want to evaluate on an NMC design.

NAPEL still needs to run simulations to gather training data that is required to construct {its} predictive model. 
As discussed above, running simulations is very time-consuming if we apply a brute-force approach to run all the application-input configurations needed for training data. 
To alleviate this problem, we use a technique called \emph{design of experiments} (DoE)~\cite{natrella2010nist} to extract representative data with a {small} number of experimental runs {(between 11 and 31 for the evaluated applications)}. 
Specifically, we employ a DoE variant called \emph{central composite design} (CCD), which allows us to explore the interactions and nonlinear effects between the application input parameters and the output response {(i.e., performance and energy consumption)}. 
%{Thus, by using CCD, we select representative application-input configurations to ensure a minimum number of simulations to gather training data.}

% In this paper, we make the following contributions:

% \vspace{-0.1cm}

% \begin{enumerate}
% \item We propose NAPEL, a new, {fast} high-level performance and energy estimation framework for NMC architectures. NAPEL {is the first such model to} leverage ensemble learning techniques, specifically random forest, to {quickly estimate} the performance and energy consumption of previously-unseen applications in early stages of design space exploration for NMC architectures.

% \item We {reduce} the simulation time needed to gather training data for NAPEL by employing a DoE technique~\cite{mariani2017predicting}, which selects a {small} number of application-input configurations that well represent the entire space of input configurations.

% \item {We} show that NAPEL can provide performance and energy estimates {$220\times$ faster than a state-of-the-art microarchitecture simulator} with an {average error rate of 8.5\% (performance) and 11.6\% (energy)} compared to the simulator.

% \item We show that we can use NAPEL to {accurately} determine if, {and by how much,} executing a certain workload on a specific NMC architecture can improve performance and reduce energy consumption {versus execution on a CPU}.
% \end{enumerate}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/methodology.tex <==
\section{NAPEL}
\label{sec:napel/methodology}
%Our methodology 
\vspace{-0.1cm}
NAPEL is a {performance and energy estimation} framework that targets the early stages of {NMC} system design. In this section, we describe the main components of the framework. First, we give an overview of NAPEL training and prediction (Section~\ref{sec:napel/overview}). Second, we describe the target NMC architecture we consider in this chapter (Section~\ref{sec:napel/nmcarch}). Third, we explain the code-instrumentation process for the applications used to generate training datasets and for the applications under performance and energy prediction (Section~\ref{sec:napel/code}). Fourth, we describe the two most important components of NAPEL training: the design of {experiments} methodology (Section~\ref{subsec:napel/doe}) and the ensemble machine learning (ML) technique (Section~\ref{sec:napel/rf}).
%\jgl{Don't call this section "Methodology". It can be confused with the methodology for evaluation. Call it "A Machine-learning-based Analytical Model for Near-Data Processing", or something similar.}

\vspace{-0.2cm}

\subsection{Overview}
\label{sec:napel/overview}

\vspace{-0.1cm}

NAPEL is based on ensemble learning. {Thus,} it needs to be trained before {it can} predict performance and energy consumption.
Figure~\ref{fig:napel/model} depicts the {key} components of NAPEL training and prediction.

% \vspace{-0.3cm}

\begin{figure}[h]
\centering
 \includegraphics[bb=17 0 1395 705,width=1.0\linewidth]{NAPEL/images/ModelEmbed.pdf}
% \includesvg[width=1.0\linewidth]{images/Model.svg}
\vspace{-0.8cm}
\caption{Overview of NAPEL training and prediction
\label{fig:napel/model}}
\vspace{-0.3cm}
\end{figure}

%\vspace{-0.1cm}
\noindent \textbf{Model Training.} NAPEL training consists of three phases. 
The first phase (\circled{1} {in Figure~\ref{fig:napel/model}}) is an LLVM-based~\cite{llvm} kernel {analysis} phase (Section~\ref{sec:napel/code}), which extracts architecture-independent workload characteristics. 
First, we instrument applications or parts of them that we use to gather data for model training. We consider the instrumented codes for execution on NMC compute units with a specific architecture configuration. 
%we want to study as a potential candidate to offloading to (i.e., executing on) NMC compute units with an specific architecture configuration. 
%  This initial selection can be performed by following the approach by Awan \etal~\cite{Awan:2017:IPN:3132402.3132427}. 
Second, we characterize the instrumented codes in a microarchitecture-independent manner by using a specialized plugin of the LLVM compiler framework~\cite{Anghel2016}. This type of  characterization excludes any hardware dependence and captures the inherent {characteristics} of workloads.

In the second phase~\circled{2}, microarchitectural simulations are performed to gather architectural responses for training. 
For the simulations, we use central composite design (\acrshort{ccd})~\cite{mariani2017predicting}, a technique for {the design of experiments (DoE) method}~\cite{montgomery2017design}. With CCD, we can minimize the number of simulation experiments to gather training data for NAPEL while ensuring {good} quality of the training data (Section~\ref{subsec:napel/doe}). 
The generated simulator responses along with application properties from the first phase and the {microarchitectural} parameters form the input to our ML algorithm.

In the third phase~\circled{3}, we train our ML algorithm (Section~\ref{sec:napel/rf}). During this phase, we perform additional tuning of our ML algorithm's hyper-parameters. Hyper-parameters are sets of ML algorithm variables that can be tuned to optimize the accuracy of the prediction model. 
{We validate the prediction model against performance and energy simulation results from the second phase.} 
Once trained, the framework can predict the performance and energy of a {previously-unseen} application on a specific NMC architecture.

\vspace{0.1cm}
\noindent \textbf{Model Prediction.} NAPEL prediction has only two phases. 
The first phase (\circled{A} {in Figure~\ref{fig:napel/model}}) is the same LLVM-based kernel analysis phase as in NAPEL training. {This phase extracts} architecture-independent features of the workload for which NAPEL will predict the performance and energy consumption. 
The second phase~\circled{B} {performs} the prediction by using the trained model. We feed the model with the architecture-independent workload features and {the model provides} the performance and energy estimations.

\vspace{-0.1cm}

\subsection{NMC Architecture}
\label{sec:napel/nmcarch}
\vspace{-0.1cm}

Figure~\ref{fig:napel/systemNMC} depicts the reference computing platform that we consider in this chapter. It contains a host processor and an external memory equipped with NMC compute units. %Our reference host processor is an IBM\textsuperscript{\textregistered} POWER9 system. 

\vspace{-0.3cm}

\begin{figure}[h]
\centering
\includegraphics[bb=24 168 808 467,width=0.70\linewidth]{NAPEL/images/systemNMC53.pdf}
\vspace{-0.4cm}
\caption{Overview of a system with NMC capability. On the right, an abstract view of application code with kernels {that are} offloaded to NMC
\label{fig:napel/systemNMC}}
\vspace{-0.2cm}
\end{figure}


The NMC \juan{subsystem} consists of a 3D-stacked memory~\cite{6757501,gao2015practical, teserract, lee2016smla} with processing elements (PEs) embedded in its logic layer. 
The memory is divided into several vertical DRAM partitions, called vaults, each with its own DRAM controller in the logic layer. 
In this chapter, we model NMC PEs as in-order, single-issue cores {with a private cache} as proposed in previous work~\cite{teserract,gao2015practical}, taking into account the limited thermal and area budget in the logic layer. 
NAPEL can be extended to support other types of general-purpose cores and accelerators by selecting the appropriate {architectural} features (see Table~\ref{tab:napel/application}) for training the {NAPEL model}.

\vspace{-0.2cm}

\subsection{Code Instrumentation and Analysis}
\label{sec:napel/code}
\vspace{-0.1cm}

In the first phase of NAPEL training and prediction, the programmer annotates the region of the source code, {called \emph{kernel} (\textit{k}),} \juang{which} is a candidate for offloading to NMC (i.e., execution on NMC processing elements). Then, that specific region is converted into an LLVM intermediate-representation (IR), {which} provides the basis for performing hardware-independent kernel analysis. 
{Hardware-independent} profiling enables us to generate {an} application profile \textit{p} independently of the {NMC design}. 

The {application} profile \textit{p(k, d)} is obtained by executing the instrumented application kernel \textit{k} while processing a dataset \textit{d}. \textit{p(k, d)} is a vector where each parameter is a statistic about an application feature \textit{f}. 
Table~\ref{tab:napel/application} lists the main application features {we extract} {by using the LLVM-based PISA analysis tool~\cite{Anghel2016}}. 
{We select} these features to analyze the memory access behavior of an application (data reuse distance, memory traffic, memory footprint, etc.), which is key for {assessing} the suitability of NMC for the application. 
Ultimately, the application profile \textit{p} has 395 features, which includes all the sub-features {of each metric we consider}. {Such a} large number of features enables complex relationships to be identified between the analyzed {application and its performance and energy consumption} on the underlying {NMC} architecture~\cite{mariani2017predicting}.

\vspace{-0.2cm}

\input{NAPEL/tables/metrics.tex}

\vspace{-0.1cm}

\subsection{Central Composite Design}
\label{subsec:napel/doe}
\vspace{-0.1cm}
In the second phase of NAPEL training, we use the design of experiments (DoE) {method}~\cite{montgomery2017design} as a way to minimize the number of experiments to train NAPEL without {sacrificing} the amount and quality of the information gathered by the experiments. 
DoE {is a set of} statistical techniques meant to {locate} a {small set of points in a parameter space with the goal of representing the whole parameter space}. 
The traditional brute-force approach to collecting training data is time-consuming: the sheer number of experiments renders detailed simulations intractable. Thus, the DoE strategy to gather a training dataset is a critical component of our model. 

We apply the Box--Wilson central composite design (CCD)~\cite{mariani2017predicting}, the goal of which is to minimize the uncertainty of a nonlinear polynomial model that accounts for parameter interactions. 
While applying CCD, we treat the application input dataset \textit{d} as a parameter vector (e.g., dataset size,~number of threads, etc.) and {each input} configuration as a point in {a multidimensional} parameter space. 
For example, application \textit{atax} from the PolyBench benchmark suite~\cite{pouchet2012polybench} has two significant {parameters} (\textit{dimension},~\textit{threads}) (see Table~\ref{tab:napel/results}). 
In CCD, each input parameter in the vector \textit{d} can {have} one of five levels: {\textit{minimum},~\textit{low},~\textit{central},~\textit{high},~\textit{maximum}}. 
%such that the experiments lie on the surface of a multidimensional sphere.
{First, we select these levels for each parameter.
For example, for \textit{atax}, the levels of \textit{dimension} are (500,~1250,~1500,~2000,~2300). 
Second, we place in the parameter space a point for each parameter combination (i.e., input configuration) with \textit{low} and \textit{high} levels (the corners of the solid-line square in Figure~\ref{fig:napel/doe}). 
In the case of \textit{atax}, the points (\textit{dimension}, \textit{threads}) are (1250,~8), (1250,~32), (2000,~8), (2000,~32). 
Third, we draw a multidimensional sphere (represented as a circle in Figure~\ref{fig:napel/doe}) that circumscribes the initial square. 
This sphere generalizes the DoE to capture the nonlinearity in the system. 
Fourth, we obtain additional points on the sphere by combining the \textit{central} level of each parameter with the \textit{maximum} and \textit{minimum} levels of the other parameters. For \textit{atax}, these points (\textit{dimension}, \textit{threads}) are (1500,~4), (1500,~64), (500,~16), (2300,~16). 
Fifth, we include the \textit{central} configuration, {which} is (1500,~16) for \textit{atax}.}

\vspace{-0.2cm}

% \ignore{
% \begin{figure}[h]
% \centering
% \includegraphics[width=2.8cm,trim={0.5cm 4.8cm 0.4cm 5cm},clip]{NAPEL/images/ccd.pdf}
% \vspace{-0.2cm}
% \caption{Central composite DoE for two parameters {(\textit{x},~\textit{y})}. {For example, for \emph{atax} (\textit{x},~\textit{y}) are (\textit{dimension},~\textit{threads})} 
% \label{fig:napel/doe}}
% \vspace{-0.4cm}
% \end{figure}
% }

\begin{SCfigure}[][h]
  \centering
  \caption{Central composite DoE for two parameters (\textit{x},~\textit{y}). For example, for \emph{atax} (\textit{x},~\textit{y}) are (\textit{dimension},~\textit{threads})}
  \hspace{3cm}
\includegraphics[bb=21 136 715 725,width=3.2cm,trim={0cm 0cm 0cm 0cm},clip]{NAPEL/images/ccd2.pdf}
\label{fig:napel/doe}
\vspace{-0.4cm}
\end{SCfigure}



We run these {DoE-selected application-input} configurations on different architectural configurations to collect the training dataset. {Table~\ref{tab:napel/results} lists the parameter levels for the evaluated applications. We include a \textit{test} configuration, which we use in Section~\ref{sec:napel/usecase}.}
\input{NAPEL/tables/doe.tex}

\vspace{-0.2cm}

\subsection{Ensemble Machine Learning}
\label{sec:napel/rf}
\vspace{-0.1cm}

The third phase of NAPEL training is the training of the ML algorithm. 
As we retrieve hundreds of application features from the application analysis, we make use of the random forest (\acrshort{rf})~\cite{breiman2001random} algorithm, which embeds automatic procedures to screen many input features. 
RF is an ensemble ML algorithm, {which, starting from a root node, constructs a tree and iteratively grows the tree by associating it with a splitting value for an input variable to generate two child nodes}. 
Each node is associated with a prediction of the target metric equal to the mean observed value in the training dataset for the input subspace the node represents. 
This input subspace is randomly {sampled} from the entire training dataset.

We employ RF to capture the intricacies of {new} NMC architectures by predicting instructions per cycle (\acrshort{ipc}) when {executing} an application {near} memory. Formally, we predict IPC$(p,~a)\sim$ IPC$(k,~d,~a)$, where \textit{p} is the hardware-independent application profile representation of kernel \textit{k} when processing input dataset \textit{d} on an architecture configuration \textit{a}. \juan{The input data gathered to} train our RF model \juan{has} three parts: (1) a hardware-independent application profile \textit{p(k,~d)}, (2) an architectural design configuration \textit{a}, and (3) {responses corresponding to each pair $(p,~a)$}. To gather the architectural responses, kernel \textit{k} belonging to training set T with input dataset \textit{d} is executed on an architectural simulator, simulating an architecture configuration \textit{a}. This produces IPC\textit{(k,~d,~a)} for that configuration and is used as a \textit{label} while training our RF algorithm. % This, in turn, produces...

We improve NAPEL training by tuning the algorithm's hyper-parameters~\cite{scikit-learn}. Hyper-parameter tuning can provide better performance estimates for some applications. 
{First, we perform as many iterations of the cross-validation process as hyper-parameter combinations}. %, each time using a different model setting. 
{Second, we compare all the generated models by evaluating them on the testing set, and select the best one}. 
% The best-tuned configuration is listed in Table~\ref{tab:results} for each application. %\jgl{Do we really need to show the hyper-parameters in the table?}

After training our RF algorithm, we can predict the IPC of a kernel that is \emph{not} in the training set. 
The predicted IPC can be used for performance evaluation of a kernel on an NMC system. The execution time $\Pi_{\textrm{NMC}}$ of the kernel offloaded to NMC can be calculated as $\Pi_{\textrm{NMC}}=\frac{I_{\textrm{offload}}}{IPC.f_{\textrm{core}}}$, 
%with Equation~\ref{eq:1}.
% \begin{align}
%\Pi_{\textrm{NMC}}=\frac{I_{\textrm{offload}}}{IPC.f_{\textrm{co%re}}}\label{eq:1}
% \end{align}
where $f_{\textrm{core}}$ is the frequency of the NMC processing cores and $I_{\textrm{offload}}$ is the total number of offloaded instructions. Similarly, we build another model for energy prediction where we use energy consumption as a \textit{label} when we train our RF algorithm.
%\jgl{We should open-source the code.}

\vspace{-0.3cm}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/relatedWork.tex <==
\section{Related Work}
\label{sec:napel/relatedWork}
\vspace{-0.1cm}

The lack of evaluation tools is a critical challenge \juan{to} the adoption of near-memory computing (NMC)~\cite{mutlu2019,singh2018review}.
% As the field of NMC does not have very sophisticated tools and techniques, researchers often spend a lot of time building the appropriate evaluation environment~\cite{junior2017generic}.
The importance of architecture simulators is widely acknowledged. However, simulators are generally very slow as they may take hours to simulate even \juang{a} single configuration~\cite{guo2013microarchitectural,sanchez2013zsim}.

%Several ML-based performance prediction methods have received attention in different fields. 
Recent works propose ML-based performance prediction methods for faster early-stage design space exploration of different architectures. 
Table~\ref{tab:napel/related} lists recent works (including NAPEL) that use different prediction techniques for several architectures. 

\input{NAPEL/tables/realtedWork.tex} 

Joseph~\etal~\cite{1598116} and Guo~\etal~\cite{guo2013microarchitectural} use linear regression models to predict CPU performance. Linear models cannot accurately capture nonlinearity between application and processor responses, as shown in Figure~\ref{fig:napel/results}. 
Wu~\etal~\cite{7056063} use an ANN for GPU performance prediction without applying the DoE technique. 
Unlike NAPEL, \juangg{this work uses} traditional, time-consuming brute-force techniques to collect the training dataset. 
% However, these studies {do not predict} the performance of a previously-unseen application, since their models are not trained for that, but for extrapolating application performance for datasets different {from} those used for training. 
%Some of the above prediction approaches use traditional random brute-force techniques to collect the training dataset. 
In the HPC domain, Mariani~\etal~\cite{mariani2017predicting} predict the performance of applications on cloud architectures using random forest and genetic algorithms, which are trained using DoE techniques. 
Ipek~\etal~\cite{ipek2006efficiently} use an ANN with variance-based sampling for CPU performance prediction. 
Likewise, Li~\etal~\cite{li2018processor} use an ANN with Latin hypercube sampling for design-space exploration of multicore CPUs. 
To our knowledge, NAPEL is the first performance and energy-prediction framework for NMC architectures that uses {machine-learning} models. %one that applies the random forest algorithm with the central composite design of experiment technique to systematically study the inherent relationship between input parameters and response for 
NAPEL can make accurate predictions for previously unseen applications {on NMC architectures.}






==> PhD_Thesis_Updated_arxiv (1)/NAPEL/sections/results.tex <==
\section{Experimental Results}
\label{sec:napel/results}
%\vspace{-0.1cm}

\subsection{Experimental Setup}
%\vspace{-0.1cm}

We consider different workloads from the PolyBench~\cite{pouchet2012polybench} and Rodinia~\cite{5306797} benchmark suites {that} cover a {wide} range of domains, such as image processing, machine learning, graph processing, radio astronomy.
First, we instrument the region of code that is considered for offloading to NMC processing elements. 
Second, {we apply} CCD to these workloads to select a {small} set of application input configurations that represent the space of possible input configurations. Third, we carry out the LLVM-based~\cite{llvm} microarchitecture-independent characterization to extract application metrics (Table~\ref{tab:napel/application}) by using the PISA analysis tool~\cite{Anghel2016}. 

We evaluate host performance on a real IBM POWER9 system~\cite{power9} and NMC performance on a state-of-the-art simulator, Ramulator~\cite{7063219}. We extend Ramulator with a 3D-stacked memory model to simulate the NMC processing elements~\cite{ramulator-pim-repo}.
Table~\ref{tab:napel/systemparameters} summarizes the system details used for the host system and {the NMC} system. 
We collect dynamic execution traces of the instrumented code with a Pin tool. {We feed} the acquired traces to Ramulator. 
%To maintain the coherency for NMC, we implement write-through caches. 
We {use} the simulation results {as training data for} our RF algorithm. 
Once trained, {we use NAPEL to predict the performance and energy consumption of previously-unseen applications}.

\vspace{-0.2cm}

\input{NAPEL/tables/modelParameters.tex}

%\vspace{-0.2cm}

\subsection{{Model} Training and Prediction Time}
\vspace{-0.1cm}

Table~\ref{tab:napel/timing} shows the time for performing training simulations (see ``DoE run (mins)'') {with the selected DoE configurations (``\#DoE conf.'') to gather training data. The table also includes the time for training and tuning (``Train+Tune (mins)'') and the prediction time (``Pred. (mins)'') for each application}. Once {the model is trained}, the DoE simulation time is amortized {every time we predict performance and energy consumption for a}  previously unseen application. Thus, quick exploration and {large} prediction time savings compared to simulation are possible for a previously unseen application.

\vspace{-0.2cm}

\input{NAPEL/tables/timing.tex}

%\jgl{We are working on a comparison of time needed for prediction with NAPEL and prediction with simulation. We will likely add a new plot.}
For all the evaluated applications, we compare the prediction time using trained NAPEL models with the prediction time using {Ramulator} simulations. 
{Figure~\ref{fig:napel/pred} shows NAPEL's prediction speedup over Ramulator for 256 DoE configurations for all the evaluated workloads.}
We observe that NAPEL is, on average, {$220\times$ (min.~$33\times$, max.~$1039\times$) faster than simulation.} %\jgl{Include figure?}

\vspace{-0.3cm}

\begin{SCfigure}[][h]
%\centering
\hspace{-0.3cm}
\includegraphics[bb=16 14 296 162,width=0.6\linewidth]{NAPEL/images/speedup.pdf}
\caption{NAPEL's prediction speedup (in increasing order) over Ramulator for 256 DoE configurations.}
\label{fig:napel/pred}
\vspace{-0.6cm}
\end{SCfigure}

%\vspace{-0.1cm}

\subsection{Accuracy Analysis}
\vspace{-0.1cm}

We analyze the accuracy of NAPEL for previously unseen applications by {performing} cross-validation~\cite{scikit-learn}. 
To evaluate the prediction accuracy for a particular application, our training data comprises all the collected data (using an LLVM kernel analyzer and a microarchitecture simulator) for all applications \emph{except} the application for which the prediction will be \juang{made}. 
%That one application is our testing application, for which NAPEL predicts performance and energy. 
We repeat the same process to gather test prediction results for all applications, yet every time we test for a particular application, we do \emph{not} include it in the training set. 
Therefore, when predicting performance and energy consumption of an application {on NMC}, {we do \emph{not} use any data related to that application}. 
This makes the prediction more difficult because the ML algorithm has no knowledge of {the application to be predicted}. 
Thus, the test set differs from the training set as much as applications differ from each other. 
We evaluate the accuracy of the proposed model in terms of relative error $\epsilon_i$ to indicate how close the predicted value $y_{i}^\prime$ is to the actual value $y_{i}$. 
%We compute the error $\epsilon_i$ relative to the actual value $y_{i}$ for a specific application under study. 
We calculate the mean relative error (MRE) for each application with Equation~\ref{eq:napel/2}.

\vspace{-0.3cm}

\begin{align}
 MRE= \frac{1}{N} \displaystyle \sum_{i=1}^{N} \epsilon_i=\frac{1}{N} \displaystyle \sum_{i=1}^{N}\frac{|y_{i}^\prime -y_{i}|}{y_{i}}
\label{eq:napel/2}
\end{align}

\vspace{-0.1cm}

Figure~\ref{fig:napel/results} shows {NAPEL's} MRE for the workloads in Table~\ref{tab:napel/results}. {NAPEL's average} MRE is 8.5\% for performance predictions and 11.6\%  for energy-consumption predictions. 
The highest error is for \textit{bfs}, \textit{bp}, and \textit{kmeans} because these applications exhibit quite different characteristics compared to the other {evaluated} applications. 
In Figure~\ref{fig:napel/results}, we also compare {NAPEL} with two other ML algorithms that can be used \juang{to predict} performance and energy consumption: an artificial neural network (ANN) based on Ipek~\etal~\cite{ipek2006efficiently} and a linear decision tree used by Guo~\etal~\cite{guo2013microarchitectural}. 
We make the following three observations. 
First, NAPEL is {1.7$\times$ (1.4$\times$) and 3.2$\times$ (3.5$\times$) more accurate in terms of performance (energy) prediction than the ANN and the linear decision tree, respectively}.
Second, the {linear} decision tree is very inaccurate, as {shown by its} high MRE. Decision trees are suitable {mainly} for linear regression, {so they cannot capture the nonlinearity present in NMC performance and energy}.
Third, ANN is more accurate than the decision tree, but it is {less accurate than} NAPEL for almost all workloads. 
{ANN requires a much larger training dataset to reach NAPEL's accuracy. 
When running these experiments, we also observe that the ANN takes more training time than NAPEL with hyper-parameter tuning (up to 5$\times$).} 
\vspace{-0.2cm}

\begin{figure}[h]
%\begin{SCfigure}[][h]
\centering
%\hspace{-0.3cm}
\includegraphics[bb=240 99 724 438,width=0.90\linewidth,trim={8cm 3cm 8cm 3cm},clip]{NAPEL/images/resultsDelayEnergy2_gagan.pdf}
%\hspace{-0.2cm}
\vspace{-0.45cm}
\caption{Mean relative error for performance (a) and energy (b) predictions using NAPEL vs. other methods.}
\label{fig:napel/results}
\vspace{-0.25cm}
%\end{SCfigure}
\end{figure}






% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.5\textwidth]{images/resultsDelay.eps}
% \caption{Mean relative error for performance for the applications considered here
% \label{fig:resultsDelay}}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.5\textwidth]{images/resultsEnergy.eps}
% \caption{Mean relative error for energy for the applications considered here
% \label{fig:resultsEnergy}}
% \end{figure}






% \begin{figure}[!h]
% \centering


% \includegraphics[width=0.5\textwidth]{images/speedupResults.eps}
% \caption{Performance speedup by processing close to the memory compared with processing on an IBM POWER9 system
% \label{fig:speedup}}
% \end{figure}
\vspace{-0.2cm}

\subsection{Use Case: NMC-Suitability Analysis}
\label{sec:napel/usecase}
\vspace{-0.1cm}

In this section, we use NAPEL to perform an NMC-suitability analysis, i.e., to assess the potential benefit of offloading a workload to NMC. 
This analysis compares the energy-delay product (\acrshort{edp}) of executing a workload on the NMC units, which we obtain from NAPEL's predicted NMC performance and energy consumption, to the {measured EDP} of executing the workload on a host processor.
We use \juang{EDP} as our major metric of reference in this analysis because both energy and performance are critical criteria for evaluating NMC suitability.

In order to obtain EDP results for the host system, we use a POWER9 system with 16 cores each supporting four-thread simultaneous multi-threading. 
We measure power consumption by monitoring built-in power sensors on our host system via the AMESTER\footnote{https://github.com/open-power/amester} tool. 
Figure~\ref{fig:napel/ibmPower} shows the execution time and energy consumption of each workload on the POWER9. 
For the EDP results on the NMC system, we use NAPEL with tuned hyper-parameters. 

% \vspace{-0.4cm}

\begin{figure}[h]
\centering
\includegraphics[bb=15 9 439 162,width=0.85\linewidth]{NAPEL/images/powerResults2.pdf}
\vspace{-0.5cm}
\caption{Execution time and energy on an IBM POWER9.
\label{fig:napel/ibmPower}}
\vspace{-0.3cm}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[bb=5 5 391 139,width=0.85\linewidth]{NAPEL/images/edp2.pdf}
\vspace{-0.4cm}
\caption{Estimated EDP reduction of offloading to NMC units versus \juanggg{execution} on the baseline host CPU. ``Actual'' denotes the estimation with Ramulator. ``NAPEL'' \juanggg{denotes} NAPEL's prediction results.
\label{fig:napel/edp}}
\vspace{-0.3cm}
\end{figure}
Figure~\ref{fig:napel/edp} shows estimated EDP reduction when executing each application on the NMC system compared to {executing} the same application on the host system using the \textit{test} dataset (see Table~\ref{tab:napel/results}). 
For each application, we show two bars: (1) NAPEL's estimated EDP reduction, and (2) the estimated EDP reduction obtained by simulating the application using the cycle-accurate Ramulator~\cite{7063219} (``Actual''). 
We make five observations. 
First, NAPEL {estimates the same workloads to be NMC suitable} as Ramulator does (i.e., workloads with EDP reduction greater than 1). 
Second, the MRE of NAPEL's EDP prediction is between 1.3\% and 26.3\% (14.1\% on average). 
Third, \textit{gemver}, \textit{gesummv}, \textit{lu}, \textit{mvt}, \textit{syrk}, and \textit{trmm} are not suitable for NMC, since {their} EDP reduction is less than 1. These applications have enough data locality to leverage the host cache hierarchy. 
Fourth, \textit{bfs}, \textit{bp}, \textit{cholesky}, \textit{gramschmidt}, and \textit{kmeans} are good \juang{fits} for NMC. These applications are memory intensive and have irregular memory access patterns, so the host execution suffers from expensive offchip data movement.
Fifth, \textit{atax} benefits from the host cache hierarchy when performing vector multiplication, which has high data locality. However, it also performs matrix transposition, which is memory intensive. For {\textit{atax}-like} workloads, the introduction of a small cache or scratchpad memory in the NMC compute units (larger than the 128B L1 cache in Table~\ref{tab:napel/systemparameters}) can be beneficial, such that the data locality of \juanggg{of the application} can still be exploited.

\vspace{-0.4cm}




==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/doe.tex <==

\begin{table}[h!]

% \vspace{-0.2cm}

\caption{Evaluated applications and their DoE parameters (``DoE param.''). For each DoE parameter, we show its five levels (\textit{minimum},~\textit{low},~\textit{central},~\textit{high},~\textit{maximum}) and \textit{test} input}
\label{tab:napel/results}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\vspace{-0.4cm}
\begin{center}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{p{0.8cm}p{4cm}p{1.9cm}|p{0.7cm}p{0.7cm}p{1cm}p{0.7cm}p{0.7cm}p{0.3cm}}
\toprule
\multicolumn{3}{c|}{\textbf{Application}}  & \multicolumn{6}{c}{\textbf{DoE Parameter Levels}}    \\ 

 Name& Description& DoE Param. & Min& Low& Central & High& Max& Test \\ \hline

atax    & Matrix Transpose \newline and Vector Mult.   & Dimensions    \newline Threads               &500\newline4&1250 \newline8&1500\newline16&2000\newline32&2300\newline64  &8000 \newline 32 \\

bfs      & Breadth-first \newline Search                        &  Nodes\newline Weights    \newline Threads    \newline Iterations          &400k \newline1 \newline1 \newline30 &   800k \newline2\newline9\newline40&   900k \newline4 \newline16 \newline65  &1.2m \newline25   \newline32 \newline70 &1.4m\newline49 \newline64 \newline80  &1.0m \newline 4\newline32\newline95 \\

bp    & Back-propagation                & Layer Size  \newline Seed   \newline Threads    \newline Iterations                                   &800k \newline 2 \newline 4 \newline 1&1m \newline 4 \newline 8 \newline 3&2m \newline 5 \newline 16\newline 9 &3.5m  \newline10\newline 32\newline 16 &4m \newline 12 \newline 64 \newline 25 &1.1m \newline 5\newline 32\newline 9\\

chol   & Cholesky \newline Decomposition                  & Dimensions             \newline Threads  \newline Iterations     &  64 \newline 4\newline 10&  384 \newline 8\newline 20&128 \newline 16\newline 30&320 \newline 32\newline 50&512 \newline 64\newline 80 &2000 \newline 32 \newline 60  \\

gemv &Vector Multiply \newline and Matrix\newline Addition  & Dimensions        \newline Threads      \newline Iterations             &    500  \newline4  \newline 50      &750\newline8\newline 60&1250\newline16\newline 80&2000\newline32\newline 100&2250\newline64   \newline 150 &8000 \newline 32  \newline 60  \\

gesu  & Scalar, Vector, and \newline Matrix Mult.  & Dimensions       \newline Threads     \newline Iterations              &          500  \newline4\newline10        &750\newline8\newline20&1250\newline16\newline40&2000\newline32\newline50&2250\newline64\newline60 &8000 \newline 32 \newline50  \\


gram   & Gram-Schmidt \newline Process                    & Dimension$_i$ \newline Dimension$_j$    \newline Threads                                     &  64 \newline64 \newline 4&  384 \newline384 \newline 8&128 \newline128 \newline 16&320 \newline320 \newline 32&512 \newline512 \newline 64        &2000 \newline 2000 \newline32  \\

kme     & K-Means \newline Clustering          & Data Size     \newline Clusters  \newline Threads      \newline Iterations                             & 100k \newline3\newline1\newline 10&300k \newline 5\newline9\newline 20&700k \newline 6\newline1\newline 30&    900k \newline 7\newline32\newline 40&  1.2m  \newline8\newline64\newline 50 & 819k  \newline 5\newline32\newline 30\\


lu     & LU Decomposition                          & Dimensions      \newline Threads     \newline Iterations            &196 \newline 4\newline 98 &256 \newline 8\newline 128&320 \newline 16\newline 256&420 \newline 32 \newline 420 &512 \newline 64 \newline 512  &2000 \newline 32  \newline 2000   \\


mvt     & Matrix Vector \newline Product     &Dimensions          \newline Threads     \newline Iterations        &     500  \newline4       \newline10 &750\newline8 \newline20&1250\newline16 \newline30&2000\newline32 \newline50&2250\newline64 \newline60 &2000 \newline 32   \newline40 \\

syrk     & Symmetric Rank-k \newline Operations              & Dimension$_i$     \newline Dimension$_j$ \newline  Threads                               & 64 \newline64 \newline4&128 \newline 128 \newline8&320 \newline 320 \newline16&    512 \newline 512 \newline 32&  640  \newline640  \newline 64      &2000 \newline 2000 \newline32     \\


trmm      & Triangular Matrix \newline Multiply       & Dimension$_i$\newline Dimension$_j$              \newline Threads           &196 \newline196 \newline 4 &256 \newline256 \newline 8&320 \newline320 \newline 16&420 \newline 420 \newline32 &512 \newline512 \newline 64 &2000 \newline 2000 \newline32   \\ 
\bottomrule

\end{tabular}
}
\end{center}

% \vspace{-0.4cm}

\end{table}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/doeBACKUP.tex <==
{\footnotesize
\begin{table*}[h]
\centering

\caption{Evaluated applications. We show the input datasets, random forest (RF) tuned hyper-parameters, NAPEL training time, including simulation of the selected DoE points, tuning of RF model, and NAPEL prediction time}
\label{tab:results}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\vspace{-0.3cm}
\begin{tabular}{p{1.4cm}p{2.2cm}p{1.8cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}|llll|lllll}
\hline
\multicolumn{3}{c}{\textbf{Application}}  & \multicolumn{6}{c|}{\textbf{DoE Parameter Levels}} &\multicolumn{4}{c}{\textbf{RF Hyper-Parameters}} & \multicolumn{4}{c}{\textbf{Training/Prediction Time}}  \\ 

\rot{ Name}&\rot{ Description}&\rot{ DoE Parameters}&\rot{ Min}&\rot{ Low}&\rot{ Central}&\rot{ High}&\rot{ Max}&\rot{ Test}&\rot{$n_{estimators}$}&\rot{$min_{sample  split}$}&\rot{$min_{sample leaf}$}&\rot{$max_{depth}$} &\rot{DoE simulated}&\rot{DoE run (mins)}&\rot{Tuning (mins)} &\rot{Prediction (mins)}\\ \hline




atax    & Matrix Transpose \newline and Vector \newline Multiplication   & Dimensions    \newline Threads               &500\newline4&1250 \newline8&1500\newline16&2000\newline32&2300\newline64  &8000 \newline 32&200&10&2&30 & 9& 360 &34.9 &0.49  \\

bfs      & Breadth-first \newline Search                        &  Nodes\newline Weights    \newline Threads             &400k \newline1 \newline1 &   800k \newline2\newline9&   900k \newline4 \newline16   &1.2m \newline25   \newline32  &1.4m\newline49 \newline64   &1.0m \newline 4\newline32&600&10&1&None  & 21&320 & 34.2&0.48 \\

bp    & Back-propagation                & Layer Size  \newline Seed   \newline Threads    \newline Iterations                                   &800k \newline 2 \newline 4 \newline 1&1m \newline 4 \newline 8 \newline 3&2m \newline 5 \newline 16\newline 9 &3.5m  \newline10\newline 32\newline 16 &4m \newline 12 \newline 64 \newline 25 &1.1m \newline 5\newline 32\newline 9&1800&5&4&30   & 36&420 &43.8 &0.47\\

chol   & Cholesky \newline Decomposition                  & Dimensions             \newline Threads      &  64 \newline 4&  384 \newline 8&128 \newline 16&320 \newline 32&512 \newline 64 &2000 \newline 32&  1000 &2&1&None & 15&230 &34.9&0.49   \\

gemv &Vector Multiply \newline and Matrix\newline Addition  & Dimensions        \newline Threads                  &    500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64    &8000 \newline 32&1000&2&1&None  &15&260  &24.4 & 0.51  \\

gesu  & Scalar, Vector, and \newline Matrix Multiplication  & Dimensions       \newline Threads                  &          500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64  &8000 \newline 32&1800&10&1&40&15& 310 &36.1 &0.51   \\


gram   & Gram-Schmidt \newline Process                    & Dimension$_i$ \newline Dimension$_j$    \newline Threads                                     &  64 \newline64 \newline 4&  384 \newline384 \newline 8&128 \newline128 \newline 16&320 \newline320 \newline 32&512 \newline512 \newline 64        &2000 \newline 2000 \newline32&400 &10&1&100 &21& 300  &36.5 & 0.52  \\

kme     & K-Means \newline Clustering          & Data Size     \newline Clusters  \newline Threads                                  & 100k \newline3\newline1&300k \newline 5\newline9&700k \newline 6\newline16&    900k \newline 7\newline32&  1.2m  \newline8\newline64 & 819k  \newline 5\newline32&1400&5&2&None & 21&360    &36.9&0.55\\


lu     & LU Decomposition                          & Dimensions      \newline Threads                &196 \newline 4 &256 \newline 8&320 \newline 16&420 \newline 32 &512 \newline 64  &2000 \newline 32& 200&2&4&20    &15& 360 &37.9 & 0.51  \\


mvt     & Matrix Vector \newline Product     &Dimensions          \newline Threads            &     500  \newline4        &750\newline8&1250\newline16&2000\newline32&2250\newline64 &2000 \newline 32& 1000&10&1&50& 15&520 &38.0 &0.54     \\
syrk     & Symmetric rank-k \newline operations              & Dimension$_i$     \newline Dimension$_j$ \newline  Threads                               & 64 \newline64 \newline4&128 \newline 128 \newline8&320 \newline 320 \newline16&    512 \newline 512 \newline 32&  640  \newline640  \newline 64      &2000 \newline 2000 \newline32&1000&10&1&50   & 21&480 &35.7 &0.51    \\


trmm      & Triangular matrix \newline multiply       & Dimension$_i$\newline Dimension$_j$              \newline Threads           &196 \newline196 \newline 4 &256 \newline256 \newline 8&320 \newline320 \newline 16&420 \newline 420 \newline32 &512 \newline512 \newline 64 &2000 \newline 2000 \newline32&200&2&4&20  &21& 300 &37.6 & 0.48  \\ 
\bottomrule

\end{tabular}

\vspace{-0.6cm}

\end{table*}
}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/doe_old.tex <==
\tiny{
\begin{table*}[]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{lp{2cm}p{0.7cm}p{1.1cm}llllllllllp{1cm}l}
\hline
\textbf{Name}     & \textbf{Description}   & \textbf{Variable}&\textbf{Range} & \multicolumn{5}{c}{\textbf{DoE}} &\multicolumn{4}{c}{Random Forest} & \multicolumn{2}{c}{\textbf{Simulation Cost (hours)}}  \\ 
&&&&Min&Low&Central&High&Max& n_{estimators}&min_{sample split}&min_{samples leaf}&max_{depth}& All Configuration &DoE \\ \hline

3MM      & 3 Matrix \newline Multiplication                   & NI \newline NJ \newline NK \newline NL \newline NM                 & 128-1024 \newline 128-1024 \newline 128-1024 \newline 128-1024 \newline    128-1024                             &64&128&448&768&1024    &   400+ & 26 \\
ATAX     & Matrix Transpose \newline and Vector              & NX \newline NY              &     500-4000 \newline 500-4000  &500&1250&1500&2000&2300  & 600+ & 6  \\

CHOLESKY & Cholesky \newline Decomposition                   & N                  &      128-1024 &   -                      &-&-&-& & 400+ & 3  \\
GEMM     & Matrix Multiply                          &  NI \newline NJ \newline NK                 &        128-640 \newline 128-640 \newline 128-640     &64&128&448&768&1024     & 100+ & 2   \\
GESUMMV  & Scalar, Vector, and \newline Matrix Multiplication & N                  &    500-4000              &              &-&-&-&-    & 600+ & 2     \\
GRAMSCHM & Gram-Schmidt \newline Process                     & NI \newline NJ                 & 128-512 \newline 128-512                            &  64&  384&128&320&512        & 150+ & 5    \\
LU       & LU Decomposition                         & N                & 128-1024                               &-&-&-&-&-   & 400+ & 3    \\
MVT      & Matrix Vector \newline Product and                & N                  &      500-400           &               &&-&-& & 600+ & 2.5     \\
SYR2K    & Symmetric rank -2k \newline operations            & NI \newline NJ                  &  128-1024 \newline 128-1024                               & &&&    &     &   400+ & 5    \\
SYRK     & Symmetric rank -k \newline operations             & NI \newline NJ                   &         128-1024 \newline 128-1024                      &    &&&&         & 400+ & 8     \\
TRMM     & Triangular matrix \newline multiply               & NI                  &  128-1024            &                  &-&-&-&  & 150+ & 3   \\ \hline

\end{tabular}
\caption{PolyBench workload description with parameters for DoE,possible input range, possible input configurations and configurations using DoE }
\label{tab:results}
\end{table*}
}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/doe_old2.tex <==

\begin{table*}[]
\centering

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{p{1.5cm}p{0.9cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}llllll}
\hline
\textbf{Name}      & \textbf{Variable} & \multicolumn{5}{c}{\textbf{Application Input}} &\multicolumn{4}{c}{Random Forest Parameters} & \multicolumn{2}{c}{\textbf{Simulation Cost (hours)}}  \\ 

&&\rot{Min}&\rot{Low}&\rot{Central}&\rot{High}&\rot{Max}&\rot{$n_{estimators}$}&\rot{$min_{sample  split}$}&\rot{$min_{sample leaf}$}&\rot{$max_{depth}$}&\rot{Total} &\rot{DoE} \\ \hline

3MM                        & NI \newline NJ \newline NK \newline NL \newline NM  \newline Threads                                       &64 \newline 64 \newline 64 \newline 64 \newline 64 \newline 4 &128 \newline 128 \newline 128  \newline 128 \newline 128 \newline 8  &448 \newline 448 \newline 448 \newline 448 \newline 448 \newline 16  &768 \newline 768 \newline 768 \newline 768 \newline768 \newline32 &1024 \newline 1024 \newline 1024 \newline 1024 \newline 1024 \newline 64  &1800&5&4&30   &   400+ & 26 \\


ATAX      & NX \newline NY     \newline Threads               &500\newline500\newline4&1250 \newline1250\newline8&1500\newline1500\newline16&2000\newline2000\newline32&2300\newline2300\newline64  &200&10&2&30 & 600+ & 6  \\


CHOLESKY                    & N             \newline Threads     &         -                      &-&-&-& &1000 &2&1&None&  400+ & 3  \\


GEMM                            &  NI \newline NJ \newline NK         \newline Threads                 &64\newline64\newline64\newline4&128\newline128\newline128\newline8&448\newline448\newline448\newline16&768\newline768\newline768\newline32&1024\newline1024\newline1024\newline64    &600&10&1&None &   100+ & 2   \\
GEMVER   & N         \newline Threads                  &              &-&-&-&-    &1000&2&1&None  & 600+ & 2     \\

GESUMMV   & N         \newline Threads                  &              &-&-&-&-    &1800&10&1&40  & 600+ & 2     \\


GRAMSCHM                      & NI \newline NJ     \newline Threads                                     &  64&  384&128&320&512        &400 &10&1&100&  150+ & 5    \\


LU                              & N      \newline Threads                &-&-&-&-&-  &200&2&4&20   & 400+ & 3    \\


MVT         & N           \newline Threads            &               &&-&-& & 1000&10&1&50&  600+ & 2.5     \\


SYR2K              & NI \newline NJ      \newline Threads                                    & &&&    &      &1400&5&2&None &   400+ & 5    \\


SYRK                  & NI \newline NJ    \newline Threads                                &    &&&&        &1000&10&1&50   & 400+ & 8     \\


TRMM           & NI             \newline Threads           &-&-&-& & &200&2&4&20  & 150+ & 3   \\ \hline

\end{tabular}
\caption{PolyBench workload description with parameters for DoE,possible input range, possible input configurations and configurations using DoE }
\label{tab:results}
\end{table*}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\footnotesize
%\vspace{-0.1cm}

\begin{table}[h]
\centering
\caption{Main application and architectural features}
\label{tab:napel/application}
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{p{0.4\linewidth} p{0.62\linewidth}}
\toprule
\textbf{Application Feature} & \textbf{Description} \\ 
\midrule
Instruction Mix & Fraction of instruction types (integer, floating point, memory read, memory write, etc.) \\
\acrshort{ilp}                      & Instruction-level parallelism on an ideal machine. \\
Data/Instruction reuse distance   & For a given distance $\delta$, probability of reusing one data element/instruction (in a certain memory location) before accessing $\delta$ other unique data elements/instructions (in different memory locations). \\
%Instruction reuse distance & For a given distance $\sigma$, probability of reusing one instruction (in a certain memory location) before accessing $\sigma$ other unique instructions (in different memory locations). \\
%Memory traffic                      & Percentage of memory reads/writes that need to access the second level of memory hierarchy, assuming a first level of size equal to the maximum reuse distance. \\
Memory traffic                      & Percentage of memory reads/writes that need to access the {main memory}, assuming a {cache} of size equal to the maximum reuse distance. \\
Register traffic    & Average number of registers {per} instruction. \\
Memory footprint    & Total memory size used by the application. \\ 
\bottomrule

\textbf{NMC Arch. Features }   & \textbf{Description} \\ 
\midrule
Core type & In-order\\
\#PEs & Total number of near-memory processing units\\
Core frequency & Operating frequency of the core\\
Cache line size & Total size of a cache line (bytes) \\
\#cache-lines & Number of cache lines\\
DRAM layers & Number of stacked DRAM layers\\
Size of DRAM& Total size of memory (bytes) \\
Cache access fraction & Cache hit ratio \\
DRAM access fraction & Cache miss ratio \\

\bottomrule
\end{tabular}
}
% \vspace{-0.5cm}

\end{table}
}

%For a given data distance $\sigma$, the probability that a memory \juan{location} is reused before accessing other $\sigma$ unique memory \juan{locations.} \\
%For a given instruction distance $\delta$, the probability that a memory \juan{location} is reused before accessing other $\delta$ unique memory \juan{locations.}    \\
%The percentage of operations that need to access the next level of memory hierarchy\\
%The average number of register read and write operations \\


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/modelParameters.tex <==

{\footnotesize
\begin{table}[h]
  \caption{System parameters and configuration}
    \label{tab:napel/systemparameters}
\vspace{-0.4cm}
\begin{center}
\resizebox{0.78\linewidth}{!}{%
\begin{tabular}{lp{8.6cm}}

\toprule
\textbf{Host CPU System}\\ \hline 

Configuration & IBM\textsuperscript{\textregistered} POWER9 AC922 @2.3 GHz, 16 cores (4-way SMT), 32 KiB L1 cache, 256 KiB L2 cache, 10 MiB L3 cache, 16x32GiB RDIMM DDR4 2666 MHz \\
\hline

 \textbf{NMC System} \\

\hline
Cores  &32$\times$ single issue, in-order execution @ 1.25 GHz\\
L1-I/D& 2-way, cache size = 2 cache lines, 64B per cache line \\
DRAM Module & 32 vaults, 8 stacked-layers, 256B row buffer; 4GB total size; closed-row policy \\
Off-chip Link & 16-bit full duplex high-speed serializer/deserializer (SerDes) I/O link @ 15 Gbps~\cite{7477494}\\

%NVM bandwidth & bw\textsubscript{ext} & 6 GB/s\\

\bottomrule

\end{tabular}
}
\end{center}

% \vspace{-0.4cm}
\end{table}
}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/realtedWork.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{table}[h]
\caption{Related works in different domains}
    \label{tab:napel/related}
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabularx}{\columnwidth}{p{4cm}p{4.0cm}p{2.4cm}X}
\toprule
\textbf{Name}         & \textbf{Approach}          & \textbf{Architecture} & \textbf{DoE}                                \\ \midrule
Joseph \etal~\cite{1598116} & Linear Regression & CPU          & D-optimal Design                       \\
Ipek \etal~\cite{ipek2006efficiently}         & ANN               & CPU          & Variance Based Sampling             \\

Wu \etal~\cite{7056063}     & ANN               & GPU          & None                     \\
Guo \etal~\cite{guo2013microarchitectural}   & Model Tree        & CPU          & None                     \\
%DRuiD~\cite{mariani2014druid} & Random Forest, \newline Genetic Algorithm & FPGA & None\\

Mariani \etal~\cite{mariani2017predicting} & Random Forest, \newline Genetic Algorithm & HPC & D-optimal Design, CCD\\

SemiBoost~\cite{li2018processor}    & ANN               & CPU          & Latin Hypercube Sampling               \\\bottomrule
\textbf{NAPEL}     & \textbf{Random Forest}     & \textbf{NMC}     & \textbf{CCD}    \\ \bottomrule
\end{tabularx}
}
\end{table}
}


==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/results.tex <==


\begin{table*}[!t]
\centering
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{llllp{0.15\linewidth}ll}
\hline
Name                             & Performance Estimation Error\% & Simulation Cost & Model Cost \\ \hline
2MM          &                                &           &       \\
3MM           &                                &           &       \\
ATAX          &                                &           &       \\
BICG          &                                &           &       \\
Cholesky        &                                &           &       \\
GEMM           &                                &           &       \\
GESUMMV         &                                &           &       \\
GRAMSCHM       &                                &           &       \\
LU            &                                &           &       \\
MVT           &                                &           &       \\
SYR2K         &                                &           &       \\
SYRK             &                                &           &       \\
TRMM           &                                &           &       \\ \hline
\end{tabular}
\caption{List of workloads evaluated with estimated error and  run time (cost) compared to the simulator }
\label{tab:napel/results}
\end{table*}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/results_old.tex <==


\begin{table*}[ht]
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{llllp{0.15\linewidth}ll}
\hline
Name     & Description                              & Variable Parameters & DoE Runs & Performance Estimation Error\% & Simulation Cost & Model Cost \\ \hline
2MM      & 2 Matrix Multiplication                  & 4           & 25       &                                &           &       \\
3MM      & 3 Matrix Multiplication                  & 5           & 43       &                                &           &       \\
ATAX     & Matrix Transpose and Vector              & 2           & 9        &                                &           &       \\
BICG     & BiCG Sub Kernel of Linear Solver         & 2           & 9        &                                &           &       \\
Cholesky & Cholesky Decomposition                   & 1           & 6        &                                &           &       \\
GEMM     & Matrix Multiply                          & 3           & 15       &                                &           &       \\
GESUMMV  & Scalar, Vector and Matrix Multiplication & 1           & 6        &                                &           &       \\
GRAMSCHM & Gram-Schmidt Process                     & 2           & 9        &                                &           &       \\
LU       & LU Decomposition                         & 1           & 6        &                                &           &       \\
MVT      & Matrix Vector Product and                & 1           & 6        &                                &           &       \\
SYR2K    & Symmetric rank -2k operations            & 2           & 9        &                                &           &       \\
SYRK     & Symmetric rank -k operations             & 2           & 9        &                                &           &       \\
TRMM     & Triangular matrix multiply               & 1           & 6        &                                &           &       \\ \hline
\end{tabular}
\caption{List of workloads evaluated, parameters for DoE, resulting experimental run, estimated error and  run time (cost) compared to the simulator }
\label{tab:napel/results}
\end{table*}

==> PhD_Thesis_Updated_arxiv (1)/NAPEL/tables/timing.tex <==

\begin{table}[h]


\caption{Number of DoE configurations (``\#DoE conf'') for gathering training data (``DoE run (mins)''), NAPEL training time (``Train+Tune (mins)''), including tuning, and NAPEL prediction time (``Pred. (mins)'').}
\label{tab:napel/timing}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\resizebox{0.965\linewidth}{!}{%
\begin{tabular}{p{0.1\linewidth}|llll}
% \begin{tabular}{p{0.1\linewidth}|p{0.14\linewidth}p{0.12\linewidth}p{0.14\linewidth}p{0.11\linewidth}}
%\begin{tabular}{p{1.2cm}|p{1.1cm}p{1.6cm}p{1.8cm}p{1.2cm}}
\toprule
\multicolumn{1}{c|}{\textbf{Application}}  & \multicolumn{4}{c}{\textbf{Training/Prediction Time}}  \\ 

Name &\#DoE conf.&DoE run (mins)&Train+Tune (mins) &Pred. (mins)\\ \hline




atax   & 11& 522 &34.9 &0.49  \\

bfs      &   31&1084 & 34.2&0.48 \\

bp   & 31&1073 &43.8 &0.47\\

chol  & 19&741 &34.9&0.49   \\

gemv&19&741  &24.4 & 0.51  \\

gesu  &19& 731 &36.1 &0.51   \\


gram  &19& 773  &36.5 & 0.52  \\

kme    & 31&742    &36.9&0.55\\


lu    &19& 633 &37.9 & 0.51  \\


mvt   &  19&955 &38.0 &0.54     \\

syrk    & 19&928 &35.7 &0.51    \\


trmm    &19& 898 &37.6 & 0.48  \\ 
\bottomrule

\end{tabular}
}
\vspace{-0.4cm}

\end{table}


==> PhD_Thesis_Updated_arxiv (1)/NERO/algorithms/cosmo.tex <==
\begin{algorithm}[h!]
\scriptsize
\setstretch{1}
\caption{Pseudo-code for vertical advection and horizontal diffusion {kernels}
used by the COSMO~\cite{doms1999nonhydrostatic} {weather prediction} model}
\label{algo:nero/hdiffKernel}
% \caption{Pseudo-code for vertical advection
% used by the COSMO~\cite{doms1999nonhydrostatic} atmospheric model}
% \label{algo:hdiffKernel}
 \begin{algorithmic}[1]
    \Function{verticalAdvection}
    {$float*                ccol,
                float* dcol,
                float* wcon,
                float* ustage,\newline
                \phantom{\textbf{procedure} \texttt{VISIT\_SEQUENCE\_EVAL}(}
                float* upos,
                float* utens,
                float* utensstage$}
        \For{$c\gets2$ \textbf{to} $column-2$}
            \For{$r\gets2$ \textbf{to} row-2}
                 \Function{forwardSweep}{$float* ccol,
                float* dcol,
                float* wcon,float* ustage,\newline
                \phantom{\textbf{procedure} \texttt{VISIT\_SEQUENCE\_EVAL\quad\quad\quad}(}
                float* upos,
                float* utens,
                float* utensstage$}
                
              
                \For{$d\gets1$ \textbf{to} $depth$}
                       \State{\texttt{/* forward sweep calculation */}}
                \EndFor
                \EndFunction
                       
                \Function{backwardSweep}{$float* ccol,
                float* dcol,
                float* wcon,
                float* ustage,\newline
                \phantom{\textbf{procedure} \texttt{VISIT\_SEQUENCE\_EVAL\quad\quad\quad}(}
                float* upos,
                float* utens,
                float* utensstage$}     
                 
                \For{$d\gets depth-1$ \textbf{to}$ 1$}
                \State{\texttt{/* backward sweep calculation */}}
                \EndFor
                \EndFunction
            \EndFor
        \EndFor
      \EndFunction
   
         


% \end{algorithm}


% \vspace{-1cm}
% \begin{algorithm}
% \SetAlgoLined
% \DontPrintSemicolon
% \SetNoFillComment
\hrule
% \caption{Pseudo-code for horizontal diffusion
% used by the COSMO~\cite{doms1999nonhydrostatic} atmospheric model}
% \label{algo:hdiffKernel}

  \Function{horizontalDiffusion}{$float* src, float* dst$}    
       \For{$d\gets1$ \textbf{to} $depth$}
             \For{$c\gets2$ \textbf{to} $column-2$}
                    \For{$r\gets2$ \textbf{to} row-2}
                        \State{\texttt{/* {L}aplacian calculat{ion} */}}
                        \State{$lap_{CR}=laplaceCalculate(c,r)$}
                        \State{\texttt{/* row-laplacian */}}
                        \State{$lap_{CRm}=laplaceCalculate(c,r-1)$}      
                        \State{$lap_{CRp}=laplaceCalculate(c,r+1)$}
                        \State{\texttt{{/* column-laplacian */}}}
                        \State{$lap_{CmR}=laplaceCalculate(c-1,r)$}
                        \State{$lap_{CpR}=laplaceCalculate(c+1,r)$}
                        \State{\texttt{/* column-flux calculat{ion} */}}
                        \State{$flux_{C} = lap_{CpR} - lap_{CR}$}
                        \State{$flux_{Cm} = lap_{CR} - lap_{CmR}$}
                        \State{\texttt{/* row-flux calculation */}}
                        \State{$flux_{R} = lap_{CRp} - lap_{CR}$}
                        \State{$flux_{Rm} = lap_{CR} - lap_{CmR}$}
                        \State{\texttt{/* output calculat{ion} */}}
                        \State{$dest[d][c][r] = src[d][c][r] -
                            c1 * (flux_{CR}- flux_{CmR}) + (flux_{CR}- flux_{CRm})$}
                        
            \EndFor 
             \EndFor   
   \EndFor
      \EndFunction
         

\end{algorithmic}
\end{algorithm}



==> PhD_Thesis_Updated_arxiv (1)/NERO/algorithms/scaling.tex <==
\begin{algorithm}
 \caption{AFU scaling prediction model}
 \label{algo:fpgaFamily}
\SetAlgoLined\DontPrintSemicolon
 \SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
       
\KwResult{Pareto optimal $(\omega,\mu)$ }
initialization\;
\While{$FPGA_{device}$}{
    \textbf{Step 1: Empirical characterization per AFU}\;
    \Input{ $\omega=\omega_{min},\mu=\mu_{min}$}
    \Output{$\overrightarrow{\eta_{AFU}}$, $\rho_{AFU}$}
   High-level-synthesis with Vivado HLS \&\;
   FPGA implementation with Vivado\;
    \textbf{Step 2: Performance Modeling}\;
    \Input{$\overrightarrow{\eta_{AFU}},\rho_{AFU}$}
    \Output{Pareto optimal $(\omega,\mu)$}
    \For{$\omega=\omega_{min}:\omega_{max}$}{
     \While{$\eta_{\{BRAM or DSP or FF or LUT\}}$ != $\eta_{max \{BRAM or DSP or FF or LUT\}}$  }{
        % \While{$\eta_{max,BRAM}\;\eta_{max,DSP}\;\eta_{max,FF}\;\eta_{max,LUT}\;\eta_{max,URAM}$ }{
        {\footnotesize $\hat \rho=a_{n}\times\mu^{n}(\omega)+a_{n-1}\times\mu^{n-1}(\omega)+...+a_{1}\times\mu(\omega)+a_{0}$\;} \label{line:polyEquation}
        %   $\hat \rho=a\times\mu^{2}(\omega)+b\times\mu(\omega)+c$ \; \label{line:polyEquation}
            % $\hat \rho(\omega,\mu)=a\times\rho^{2}(\omega,\mu)+b\times\rho(\omega,\mu)+c$ \; \label{line:polyEquation}
           {\footnotesize  $\mu \gets \mu + 1 $}
            }
        maximize ($ \hat\rho$)\;
    }
}
\end{algorithm}

==> PhD_Thesis_Updated_arxiv (1)/NERO/images_new/hdiff_mem_access.tex <==
\begin{figure}[h]
\centering
    \resizebox{0.5\textwidth}{!}{
    
    
    \begin{tikzpicture}[rotate=90,transform shape]

    %draws helper-grid:
%%%%%%%%%%%%%LAPLACE
    \gridThreeD{0}{8.25}{black};
    \node at (7.5,10.5)[ rotate=270] {\huge \textit{Laplace}};
      \dotesUpper{0}{8.25};
    %%%%%%%%%%%%%FLUX 
    \gridThreeDSecond{1}{4}{black};
    \node  at (7.5,5.5)[ rotate=270] {\huge \textit{Flux}};
     \lowerDots{3}{4};
     
        %%%%%%%%%%%%%OUTPUT
    \gridThreeDThird{2}{0}{black};
     \node  at (7.5,0.25) [ rotate=270] {\huge \textit{Output}};
     \lowestDot{1.6}{-0.45}
     
     
      \draw [thick,->,blue] (2.75,4.25) -- (2.7,8.4);
       \draw [thick,->,blue] (2.75,4.25) -- (2.1,8.9);
       \draw [thick,->,blue] (2.75,4.25) -- (4.1,8.9);
       \draw [thick,->,blue] (2.75,4.25) -- (3.5,9.4);
    
    
       \draw [thick,->,orange] (2.1,4.7) -- (3.5,9.4);
       \draw [thick,->,orange] (2.1,4.7) -- (1.5,9.4);
       \draw [thick,->,orange] (2.1,4.7) -- (2.1,8.9);
       \draw [thick,->,orange] (2.1,4.7) -- (2.9,9.9);
     
       \draw [thick,->,red] (4.1,4.7) -- (3.5,9.4);
       \draw [thick,->,red] (4.1,4.7) -- (5.5,9.4);
       \draw [thick,->,red] (4.1,4.7) -- (4.1,8.9);
       \draw [thick,->,red] (4.1,4.7) -- (4.9,9.9);
    
    
 
           \draw [thick,->,brown] (3.5,5.25) -- (3.5,9.4);
           \draw [thick,->,brown] (3.5,5.25) -- (2.9,9.9);
           \draw [thick,->,brown] (3.5,5.25) -- (4.9,9.9);
           \draw [thick,->,brown] (3.5,5.25) -- (4.3,10.4);
           %lowest to the middle
         \draw [thick,->,violet] (2.7,0.25) -- (3.5,5.15);
         \draw [thick,->,violet] (2.7,0.25) -- (4.1,4.65);
         \draw [thick,->,violet] (2.7,0.25) -- (2.1,4.65);
         \draw [thick,->,violet] (2.7,0.25) -- (2.75,4.15);
    
    
    
    % %draws lower graph lines and those in z-direction:
    
    % draws all graph nodes:
   
  
   
     

\end{tikzpicture}
}
    
    
% \begin{tikzpicture}

%     %draws helper-grid:

%     \gridThreeD{0}{4.25}{black};
%     \node at (7.5,5.25) {\huge \textit{Laplace}};
%     \gridThreeDSecond{1}{2}{black};
%     \node  at (7.5,2.5) {\huge \textit{Flux}};
%     \gridThreeDThird{2}{0}{black};
%      \node  at (7.5,0.25) {\huge \textit{Output}};
%       \draw [thick,->,blue] (2.75,2.25) -- (2.7,4.35);
%       \draw [thick,->,blue] (2.75,2.25) -- (2.1,4.85);
%       \draw [thick,->,blue] (2.75,2.25) -- (4.1,4.85);
%       \draw [thick,->,blue] (2.75,2.25) -- (3.5,5.35);
    
    
%       \draw [thick,->,red] (2.1,2.7) -- (3.5,5.35);
%       \draw [thick,->,red] (2.1,2.7) -- (1.5,5.35);
%       \draw [thick,->,red] (2.1,2.7) -- (2.1,4.85);
%       \draw [thick,->,red] (2.1,2.7) -- (2.9,5.85);
     
%       \draw [thick,->,orange] (4.1,2.7) -- (3.5,5.35);
%       \draw [thick,->,orange] (4.1,2.7) -- (5.5,5.35);
%       \draw [thick,->,orange] (4.1,2.7) -- (4.1,4.85);
%       \draw [thick,->,orange] (4.1,2.7) -- (4.9,5.85);
    
    
 
%           \draw [thick,->,brown] (3.5,3.25) -- (3.5,5.35);
%           \draw [thick,->,brown] (3.5,3.25) -- (2.9,5.85);
%           \draw [thick,->,brown] (3.5,3.25) -- (4.9,5.85);
%           \draw [thick,->,brown] (3.5,3.25) -- (4.3,6.35);
%           %lowest to the middle
%          \draw [thick,->,violet] (2.7,0.25) -- (3.5,3.1);
%          \draw [thick,->,violet] (2.7,0.25) -- (4.1,2.6);
%          \draw [thick,->,violet] (2.7,0.25) -- (2.1,2.6);
%          \draw [thick,->,violet] (2.7,0.25) -- (2.75,2.1);
    
    
    
%     % %draws lower graph lines and those in z-direction:
    
%     % draws all graph nodes:
   
%     \dotesUpper{0}{4.25};
%      \lowerDots{3}{2};
%      \lowestDot{1.6}{-0.45}

% \end{tikzpicture}
% }





\caption{Horizontal diffusion compound kernel composition in a two dimensional plane
\label{fig:NERO/hdiffMemory}}
\vspace{-0.3cm}
\end{figure}


==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/abstract.tex <==

% Ongoing climate change calls for {fast and accurate} %energy-efficient~
% weather and climate {modeling}. However, {when solving large-scale n{weather prediction}
% simulations,} state-of-the-art CPU and GPU implementations suffer from limited performance and high energy consumption. {These implementations are {dominated by} complex irregular memory access patterns and low arithmetic intensity {that} pose fundamental challengenn{s} to acceleration}. To overcome these challenges, we propose {and evaluate} the use of near-memory acceleration using a reconfigurable fabric with high-bandwidth memory (HBM). {We focus on} {compound stencils {that} are fundamental kernels} in weather prediction models. {By using} high-level synthesis techniques, {we} develop g{\namePaper,} an g{FPGA+HBM-based} accelerator connected through IBM CAPI2 (Coherent Accelerator Processor Interface) to an IBM POWER9\footnote{IBM and POWER9 are registered trademarks or common law marks of International Business Machines Corp., registered in many jurisdictions world-wide. Other product and service names might be trademarks of IBM or other companies.}  host system. {Our} experimental results show that g{\namePaper} outperforms a 16-core POWER9 n{system} by $4.2\times$ and $8.3\times$ when running two ggg{different} compound stencil kernels. g{\namePaper} n{reduces the energy consumption by} $22\times$ and $29\times$ ggg{for the same two kernels nn{over the POWER9 system}} n{with an energy efficiency of 1.5 GFLOPS/Watt and 17.3 GFLOPS/Watt}. {We conclude that} employing near-memory acceleration solutions for weather prediction {modeling}~{is~promising} ggg{as a means to achieve nn{both} high performance and nn{high} energy efficiency}.
        
Modern data-intensive applications demand high compute capabilities with strict power constraints. Unfortunately, such applications suffer from a significant waste of {both} execution cycles and energy in current computing systems due to the costly  
data movement between the compute units and the memory units. Weather prediction modeling is one such data-intensive application where we generate petabytes of data. Moreover, ongoing climate change calls for {fast and accurate} %energy-efficient~
weather and climate {modeling}. However, {when solving large-scale {weather prediction}
simulations,} state-of-the-art CPU and GPU implementations suffer from limited performance and high energy consumption. {These implementations are {dominated by} complex irregular memory access patterns and low arithmetic intensity {that} pose fundamental challenge{s} to acceleration}. To overcome these challenges, in this chapter, we propose {and evaluate} the use of near-memory acceleration using a reconfigurable fabric with high-bandwidth memory (HBM). %{We focus on} {compound stencils {that} are fundamental kernels} in weather prediction models. 


% {By using} high-level synthesis techniques, {we} develop g{\namePaper,} an g{FPGA+HBM-based} accelerator connected through IBM CAPI2 (Coherent Accelerator Processor Interface) to an IBM POWER9\footnote{IBM and POWER9 are registered trademarks or common law marks of International Business Machines Corp., registered in many jurisdictions world-wide. Other product and service names might be trademarks of IBM or other companies.}  host system. {Our} experimental results show that g{\namePaper} outperforms a 16-core POWER9 n{system} by $4.2\times$ and $8.3\times$ when running two ggg{different} compound stencil kernels. g{\namePaper} n{reduces the energy consumption by} $22\times$ and $29\times$ ggg{for the same two kernels nn{over the POWER9 system}} n{with an energy efficiency of 1.5 GFLOPS/Watt and 17.3 GFLOPS/Watt}. {We conclude that} employing near-memory acceleration solutions for weather prediction {modeling}~{is~promising} ggg{as a means to achieve nn{both} high performance and nn{high} energy efficiency}.
        

==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/accelerator.tex <==
\section{Design Methodology}
\label{sec:nero/design}
\subsection{NERO, A Near HBM Weather Prediction Accelerator}
The low arithmetic intensity of real-world weather {prediction} kernels limits the attainable performance on current multi-core systems. This sub-optimal performance is due to {the kernels'} complex memory {access} patterns and their inefficiency in exploiting a rigid cache hierarchy, {as quantified in {the} roofline plot in} Figure~\ref{fig:nero/roofline}. 
These kernels {cannot} fully utilize the available memory bandwidth, which leads to %a 
high %data-transfer 
{data movement overheads} in terms of latency and energy consumption. We address %this inefficiency 
{these inefficiencies} by developing an architecture {that} combines fewer off-chip data {accesses} with higher throughput for the loaded data. {To this end}, our accelerator design {takes} a data-centric approach~\cite{mutlu2019,ghose2019processing,teserract,singh2019near,NAPEL,hsieh2016accelerating,tom,ahn2015pim,googleWorkloads,kim2018grim} {that exploits} near high-bandwidth memory acceleration.

Figure~\ref{fig:nero/system} shows a high-level overview of our integrated system. An HBM-based FPGA is connected to a server system based on an IBM POWER9 processor using the Coherent Accelerator Processor Interface version 2 (CAPI2). 
The FPGA consists of two HBM stacks\footnote{We enable only a single stack based on our resource and power consumption analysis for the \texttt{vadvc} kernel.}, each with 16 \emph{pseudo-memory channels}~\cite{axi_hbm}. A channel is exposed to the FPGA as a 256-bit wide port, and in total, the FPGA has 32 such ports. The HBM IP provides 8 memory controllers (per stack) to handle the data transfer to and from the HBM memory ports. Our design consists of an \emph{accelerator functional unit} (\acrshort{afu}) that interacts with the host system through the power service layer (\acrshort{psl}), which is the CAPI endpoint on the FPGA. An AFU comprises of multiple \emph{processing elements} (\acrshort{pe}s) that perform compound stencil computation. Figure~\ref{fig:nero/complete_flow} shows the architecture overview of \namePaper. As vertical advection is the most complex kernel, we depict our architecture design flow for vertical advection. We use a similar design for the {horizontal diffusion} kernel.

\begin{figure*}[h]
\begin{subfigure}[t]{0.5\textwidth}
  \includegraphics[bb=9 17 525 278,width=1\linewidth,trim={0.5cm 0.5cm 0cm 0cm},clip]{NERO/images_new/evaluation_system_new_15_embed.pdf}
   \caption{
   \label{fig:nero/system}}
\end{subfigure}%
\begin{subfigure}[t]{0.4\textwidth}
  \includegraphics[bb=0 0 623 531,width=0.95\linewidth,trim={0cm 0cm 0cm 0cm},clip]{NERO/images_new/Execution_timeline_2_embed.pdf}
   \caption{
  \label{fig:nero/execution}}
\end{subfigure}
\caption[(a) Heterogeneous platform with an IBM POWER9 system connected to an HBM-based FPGA board via~CAPI2. (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard  FPGA  memory]{(a) Heterogeneous platform with an IBM POWER9 system connected to an HBM-based FPGA board via~CAPI2. (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard  FPGA  memory\label{fig:complete_hbm_flow}}
% \vspace{-1cm}
\end{figure*}





\begin{figure}[h]
  \centering
  \includegraphics[bb=20 21 769 347,width=\linewidth,trim={0.3cm 0.2cm 0cm 0.2cm},clip]{NERO/images_new/complete_flow_new_9_embed.pdf}
  \caption{Architecture overview of~\namePaper~with data flow sequence from the host DRAM to the on-board FPGA memory via POWER9 cachelines. We {depict a} single {processing element (PE)} fetching data from a dedicated HBM port. The number of HBM ports scales linearly with the number of {PEs}. Heterogeneous partitioning of on-chip memory blocks {reduces} read {and} write latencies across the FPGA memory hierarchy
 \label{fig:nero/complete_flow}}
 \end{figure}




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.5\linewidth,trim={0.3cm 0.2cm 0cm 0.2cm},clip]{NERO/images_new/evaluation_system_new_15_embed.pdf}
%   \caption{Heterogeneous platform with an IBM POWER9 system connected to an HBM-based FPGA board via~CAPI2.
%  \label{fig:nero/system}}
%  \end{figure}

% \begin{figure*}[t]
% \begin{subfigure}[t]{0.7\textwidth}
%   \includegraphics[width=0.95\linewidth,trim={0.5cm 0.5cm 0cm 0cm},clip]{NERO/images_new/complete_flow_new_9_embed.pdf}
%   \caption{
%   \label{fig:nero/complete_flow}}
% \end{subfigure}%
% \begin{subfigure}[t]{0.3\textwidth}
%   \includegraphics[width=0.95\linewidth,trim={0cm 0cm 0cm 0cm},clip]{NERO/images_new/Execution_timeline_2_embed.pdf}
%   \caption{
%   \label{fig:nero/execution}}
% \end{subfigure}
% \caption[(a) Architecture overview of~\namePaper~with data flow sequence from the host DRAM to the on-board FPGA memory via POWER9 cachelines. We {depict a} single {processing element (PE)} fetching data from a dedicated HBM port. The number of HBM ports scales linearly with the number of {PEs}. Heterogeneous partitioning of on-chip memory blocks {reduces} read {and} write latencies across the FPGA memory hierarchy. (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard  FPGA  memory.]{(a) Architecture overview of~\namePaper~with data flow sequence from the host DRAM to the on-board FPGA memory via POWER9 cachelines. We {depict a} single {processing element (PE)} fetching data from a dedicated HBM port. The number of HBM ports scales linearly with the number of {PEs}. Heterogeneous partitioning of on-chip memory blocks {reduces} read {and} write latencies across the FPGA memory hierarchy. (b)  Execution timeline with data flow sequence from the  host  DRAM  to the onboard  FPGA  memory.\label{fig:complete_hbm_flow}}
% % \vspace{-1cm}
% \end{figure*}


The weather data, based on the atmospheric model resolution grid, is stored in the DRAM of the host system {(\circled{1} in Figure~\ref{fig:nero/complete_flow})}.  We employ {the} double buffering technique  between the CPU and the FPGA to hide the PCIe {(Peripheral Component Interconnect Express~\cite{pcie})} {transfer} {latency}.  {By configuring a buffer of 64 cache lines, between the AXI4 interface of CAPI2/PSL and the AFU, we can reach the theoretical peak bandwidth of CAPI2/PCIe (x8 PCIe Gen4 interface with a theoretical peak bandwidth 15.75 GB/s and a transfer rate of 16 GT/s).} We create a specialized memory hierarchy from the heterogeneous FPGA memories {(i.e., URAM, BRAM, and HBM)}. By using a greedy algorithm, we determine the best-suited hierarchy for our kernel. The memory controller (shown in Figure~\ref{fig:nero/system}) handles the data placement to the appropriate memory type {based on programmer's directives}.

{On the FPGA, following the initial buffering (\circled{2}), the {transferred} grid data is mapped onto the HBM memory (\circled{3}).  As {the} FPGA ha{s} limited resources, we propose a 3D window-based grid transfer from the host DRAM to the FPGA, facilitating a smaller, less power-hungry deployment. The window size represents the portion of the grid a processing element ({PE} in Figure~\ref{fig:nero/system}) would process. {Most FPGA developers manually optimize for the right window size. However, manual optimization is tedious because of the huge design space, and {it} requires expert guidance. 
Further, selecting an inappropriate window size lead{s} to sub-optimal results. %We show by 
{Our experiments (in Section~\ref{subsection:nero/evaluation}) show that}: (1) finding the {best} window size is critical in terms of {the} area vs. performance trade-off, and (2) the {best window} size depends on the datatype precision. Hence, instead of pruning the design space manually, we formulate %finding 
{the search for} the {best} window size as a multi-objective auto-tuning problem taking into account the datatype precision. We make use of OpenTuner~\cite{opentuner}, %that 
{which} uses machine-learning techniques to guide the design-space~exploration.}}

 

% \gaganFeedback{FPGAs have limited resources while we have 32 HBM channels (For AD9H7 board). vadvc consumes a lot of resources compared to hdiff, so in case of  hdiff we can enable all 32 ports without exhausting resources. However, in vadvc we can't. So we just enable as many HBM ports as vadvc-PEs we can accommodate. Note: we are using only single stack (16 channels) in this work because atmost we were able to fit 14 vadvc-PEs so we did not enable another stack.} 

Our design consists of multiple PEs (shown in Figure~\ref{fig:nero/system}) that exploit data-level parallelism in COSMO {weather prediction} kernels. {A dedicated HBM memory port is assigned to a specific PE}; therefore, we enable as many HBM ports as the number of PEs. This allows us to use the high {HBM} bandwidth {effectively} because each PE fetches from an independent port. 
In our design, we use a switch, which provides the capability to %skip 
{bypass} the HBM, {when the} grid size {is small}, and map the data directly onto the FPGA's URAM {and BRAM}. The HBM port provides 256-bit data, {which} is half the size of {the} CAPI2 {bitwidth} (512-bit). Therefore, to match {the} CAPI2 bandwidth, we introduce a stream converter logic (\circled{4}) that converts {a} 256-bit HBM stream to {a} 512-bit stream (CAPI compatible) or vice versa.
From HBM, {a PE} reads a single stream of data that consists of all the fields\footnote{Fields represent atmospheric components like wind, pressure, velocity, etc. that are required for weather calculation.} {that} are needed for a specific COSMO kernel computation. {The PEs} use a fields stream splitter logic (\circled{5}) that splits a single HBM stream to multiple streams (512-bit each), one for each field.
  
{To optimize a PE{,} we apply various optimization strategies. First, we exploit the inherent parallelism in {a given} algorithm through hardware pipelining. {Second}, we partition on-chip memory to avoid the stalling of our pipelined design, since the on-chip BRAM/URAM has only two read/write ports. {Third}, all the tasks execute in a dataflow manner that enables task-level parallelism. \texttt{vadvc} is more { computationally complex} than \texttt{hdiff} because it involves forward and backward sweeps {with dependencies in {the} z-dimension}. While \texttt{hdiff} performs {only} {Laplacian} and flux calculations with dependencies in {the} x- and y-dimensions. 
Therefore, we demonstrate our design flow by means of {the} \texttt{vadvc} kernel (Figure~\ref{fig:nero/complete_flow}). 
Note {that} we show {only} a single port-based PE operation.  {However}, for multiple PEs, we enable multiple HBM ports.} % each {PE} having {its own} logic. as {shown} in Figure~\ref{fig:complete_flow}. }

We make use of memory reshaping techniques to  configure our memory space with multiple parallel BRAMs or URAMs~\cite{dioFPT}. {We form an intermediate memory hierarchy by decomposing (or slicing) 3D window data into a 2D grid. } This allows us to bridge the latency gap between the HBM memory and our accelerator. Moreover, it allows us to exploit the available FPGA resources efficiently. Unlike traditionally-fixed CPU memory hierarchies, which perform poorly with irregular access patterns and suffer from cache pollution effects, application-specific memory hierarchies {are} shown to improve {energy and latency} by tailoring the cache levels and cache sizes to {an} application's memory access patterns~\cite{jenga}.
  
The main computation pipeline (\circled{7}) {consists of a forward and a backward sweep logic}. The forward sweep {results} are stored in {an} intermediate buffer to allow for backward sweep calculation. {Upon} completion of {the} backward sweep, results are {placed in} an output buffer {that is followed by a degridding logic (\circled{6}). The degridding logic} converts the calculated results to a 512-bit wide output stream (\circled{8}). As there is only a single output stream (both in \texttt{vadvc} and \texttt{hdiff}), we do not need extra logic to merge the streams. The 512-bit {wide} stream goes through an HBM stream converter logic (\circled{4}) that converts the stream bitwidth to HBM port size (256-bit).  
  
{Figure~\ref{fig:nero/execution} shows the execution timeline from our host system to the FPGA board for a single PE. The host offloads the processing to an FPGA and %DMAs 
{transfers} the required data {via DMA (direct memory access)} over {the} CAPI2 interface. The SNAP framework allows for parallel execution of the host and our FPGA PEs while exchanging control signals over the AXI lite interface{~\cite{axilite}}. On task completion, the AFU notif{ies} the host system via {the} AXI lite interface and %DMA 
{transfers} back the results {via DMA}. }

\subsection{\namePaper~Application Framework}
Figure~\ref{fig:nero/snap_api} shows the \namePaper~application framework {to support our architecture}.  A software-defined COSMO API (\circledWhite{1}) handles offloading jobs to \namePaper~with an interrupt-based queuing mechanism.  This allows for minimal CPU usage (and, hence, power {usage}) during FPGA {operation}. \namePaper~employs an array of processing elements to compute COSMO kernels, such as vertical advection or horizontal diffusion. Additionally, we pipeline our PEs to exploit the available spatial parallelism. 
By accessing the host memory through %a 
{the CAPI2} cache-coherent link, \namePaper~acts as a peer to the CPU.  This is enabled {through} {the} Power-Service Layer (PSL) (\circledWhite{2}). { SNAP (\circledWhite{3}) allows for seamless {integration} of the COSMO API with our CAPI-based accelerator.} The job manager (\circledWhite{4}) dispatches jobs to streams, which are managed in the stream scheduler (\circledWhite{5}). The execution of a job is done by streams that determine which data is to be read from the host memory and sent to the PE array through DMA transfers (\circledWhite{6}). The pool of heterogeneous on-chip memory is used to store the input data from the main memory and the intermediate data generated by {each} PE.

\begin{figure}[h]
  \centering
  \includegraphics[bb=8 21 882 664,width=0.6\linewidth,trim={0cm 0cm 0.1cm 0cm},clip]{NERO/images_new/snap_accelerator_3_embed.pdf}
  \caption{%{FPGA micro-architecture support for \namePaper.  
  {\namePaper~application framework.} 
  We co-design our software and hardware using {the} SNAP framework. COSMO API allows the host to offload kernels to our FPGA platform
 \label{fig:nero/snap_api}}
 \end{figure}
% HDIFF SNAP, as depicted in Figure~\ref{fig:snap_accelerator}, allows \textit{actions} on an FPGA device to access the virtual memory space on the host in addition to resources such as the FPGA on-board DRAM memory.
% This access is achieved through the ``\textit{actions}'' wrapper, which provides the interface for the user logic to the power service layer module. Data is transferred between the POWER9 and FPGA at the granularity of cachelines of 128~bytes (\circled{2} in Figure~\ref{fig:snap_data}). 
% A CAPI link can transfer 512 bits of data per cycle, and hence we need two reads for a complete cacheline.  Assume that the total number of cachelines required to represent an entire grid domain of dimension $I \times J \times K$ is represented by $\zeta_{\text{Total}}$. 
% Let $\zeta_{\text{window}}$ represent the amount of data processed by a single window in terms of cachelines. Then the total number of sweeps required by an AFU to process the entire domain is given by $\ceil{\frac{\zeta_{\text{Total}}}{\zeta_{\text{window}}}}$. However, increasing the number of AFUs ($\mu$) decreases the number of sweeps by a factor of $\mu$. This is because each AFU is assigned its own $\zeta_{\text{window}}$. Hence, the amount of on-chip storage space required per AFU depends heavily on the 3D window dimensions and the memory hierarchy used.  The maximum available resources on an FPGA, heavily constrain the maximum number of AFUs ($\mu_{\textrm{max}}$) that can be instantiated on a chip, which is given by



% \subsection{NARMADA, a near-memory horizontal diffusion~accelerator}
% Figure~\ref{fig:system} shows a high-level overview of our integrated system. The FPGA is connected to a server system based on an IBM\textsuperscript{\textregistered} POWER9 processor using a coherent
% accelerator processor interface~2.0 (CAPI~2.0). NARMADA consists of accelerator functional unit (AFU) that interact with the host system through the power service layer (PSL), which is the CAPI endpoint
% on the FPGA. 
% Figure~\ref{fig:snap_data} shows the flow of data from the host memory to the FPGA memory (the mapping of data on different FPGA memories is shown in Figure~\ref{fig:system}). The collected weather data, which is based on the atmospheric model resolution grid, is stored in the DRAM of the host system (\circled{1} in Figure~\ref{fig:snap_data}). As FPGAs have limited resources, we propose 3D window-based grid transfer from the host DRAM to the FPGA. 
% We employ a double buffering technique (\circled{3}) between the CPU and the FPGA to hide the PCIe overhead.  {By configuring a buffer of 64 cachelines, between the AXI4 interface of CAPI2/PSL and the AFU, we can reach the theoretical peak bandwidth of CAPI2/PCIe (16 GB/s).} We create a specialized memory hierarchy from the heterogeneous FPGA memories. By using a greedy algorithm, we determine the best-suited hierarchy for our kernel. The heterogeneous memory controller (shown in Figure~\ref{fig:system}) handles the data placement to the appropriate memory type.

% On the FPGA, following the initial buffering, the 3D window-based grid data is mapped onto the FPGA DRAM (\circled{4}). The window size represents the portion of the grid an AFU will process. As the hdiff kernel has limited spatial locality, we cache only certain parts of data around the \textit{row} dimension into the register file (\circled{6}) (LUTs and FFs). To bridge the latency gap between DRAM and the register file, we introduce another memory level (\circled{5}) in between, which is made up of BRAM (B-Hierarchy). This intermediate hierarchy consists of 3D window data decomposed (or sliced) into a 2D grid. However, to exploit the available FPGA resources further, we also introduce another level of URAM-based memory between the DRAM and BRAM (U-Hierarchy). {Unlike traditionally fixed CPU memory hierarchies, that usually makes poor use of cache-hierarchies, an algorithm-specific hierarchy has been proven to improve the energy-delay product (EDP) by tailoring the cache-levels and cache-size to applications' access patterns~\cite{jenga}. In our case, we experimented with two cache setups, i.e., B-RAM and U-RAM. In every setup we place sequential data accesses, corresponding to a single hdiff step (lines 5-14 of Algorithm~\ref{algo:hdiffKernel}), in a single 2D memory space, composed of BRAMs or URAMs respectively. This 2D memory space is configured with multiple parallel BRAMs or URAMs using on-chip memory reshaping techniques that allow for bandwidth maximization~\cite{dioFPT}.}
% \begin{figure*}
  
%   %
%   \begin{subfigure}[b]{0.6\textwidth}
%     \includegraphics[width=\textwidth,trim={0.8cm 0cm 0.8cm 0.5cm},clip]{images/snap_data_updated_linux.pdf}
%     \caption{}
%     \label{fig:snap_data}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth,trim={0.2cm 0.1cm 1.2cm 0.2cm},clip]{images/snap_accelerator_updated_linux.pdf}
%     \caption{}
%     \label{fig:snap_accelerator}
%   \end{subfigure}
%   \caption[Two numerical solutions]{(a) Data flow sequence from the host DRAM in the form of a 3D window to the on-board FPGA memory via POWER9 cachelines. Heterogeneous memory partitioning of on-chip
% memory blocks enable minimal R/W
% latency across the FPGA memory hierarchy. (b) NARMADA framework: NARMADA acts as a peer to the CPU by accessing the main memory through
% a high-performance cache-coherent link, enabled by PSL. A software-defined API handles offloading jobs (``\textit{actions}'') to NARMADA  with an interrupt-based queuing
% mechanism that allows minimal CPU usage---and hence, power---during~the FPGA~use.}
% \vspace{-0.3cm}
% \end{figure*}
% Figure~\ref{fig:snap_accelerator} shows the NARMADA framework. Each~NARMADA~AFU employs an array of processing elements (PEs) to solve the horizontal diffusion computation. Additionally, to achieve a massively parallel design, we exploit the immediately available spatial parallelism by pipelining our PEs. NARMADA AFUs act as peers to the CPU by accessing the main memory through a high-performance cache-coherent link enabled by PSL. A software-defined API handles offloading jobs (``\textit{actions}'') to NARMADA with an interrupt-based queuing mechanism that allows minimal CPU usage (and hence, power) during FPGA use. The job manager dispatches jobs to streams managed in the stream scheduler. Each stream controls the execution of a job and determines which data is to be read from the host memory and sent to the PE array through DMA transfers. The pool of heterogeneous on-chip memory is used to store the input data from the main memory and the intermediate data generated by an AFU.
% HDIFF SNAP, as depicted in Figure~\ref{fig:snap_accelerator}, allows \textit{actions} on an FPGA device to access the virtual memory space on the host in addition to resources such as the FPGA on-board DRAM memory.
% This access is achieved through the ``\textit{actions}'' wrapper, which provides the interface for the user logic to the power service layer module. Data is transferred between the POWER9 and FPGA at the granularity of cachelines of 128~bytes (\circled{2} in Figure~\ref{fig:snap_data}). 
% A CAPI link can transfer 512 bits of data per cycle, and hence we need two reads for a complete cacheline.  Assume that the total number of cachelines required to represent an entire grid domain of dimension $I \times J \times K$ is represented by $\zeta_{\text{Total}}$. 
% Let $\zeta_{\text{window}}$ represent the amount of data processed by a single window in terms of cachelines. Then the total number of sweeps required by an AFU to process the entire domain is given by $\ceil{\frac{\zeta_{\text{Total}}}{\zeta_{\text{window}}}}$. However, increasing the number of AFUs ($\mu$) decreases the number of sweeps by a factor of $\mu$. This is because each AFU is assigned its own $\zeta_{\text{window}}$. Hence, the amount of on-chip storage space required per AFU depends heavily on the 3D window dimensions and the memory hierarchy used.  The maximum available resources on an FPGA, heavily constrain the maximum number of AFUs ($\mu_{\textrm{max}}$) that can be instantiated on a chip, which is given by
% \vspace{-0.1cm}
% \begin{align}
% \mu_{\textrm{max}}=\textrm{min}\floor{\frac{\overrightarrow{\eta_{{\textrm{max}}}}}{\overrightarrow{\eta_{\textrm{AFU}}}}}\label{eq:1}
% \end{align}
% \vspace{-0.1cm}
 
% where $\overrightarrow{\eta_{\textrm{max}}}$ represents a vector containing the maximum available resources on a single FPGA board, being a collection of BRAM, DSP, FF, LUT, and URAM, and where the term $\overrightarrow{\eta_{\textrm{AFU}}}$ represents a vector of FPGA resources used~by~a~single~AFU.


==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/background.tex <==
\section{Background} 
\label{sec:nero/background}
%This section 
\juang{In this section, we first provide} %gives 
an overview of the \juang{\texttt{vadvc} and \texttt{hdiff}} {compound stencils, %representing 
\juang{which represent} a large fraction of the overall computational load of the COSMO nn{weather prediction} model}. 
%and the CAPI SNAP framework that has been used 
Second, we introduce the CAPI SNAP {(Storage, Network, and Analytics Programming)} framework\footnote{https://github.com/open-power/snap} that we use to connect our \namePaper~accelerator to an IBM POWER9~system.

\subsection{{Representative} COSMO Stencils}
A stencil operation updates values in a structured multidimensional grid based on the values of a fixed local neighborhood of grid points. 
% \jgl{This sentence is related work -- it does not make sense here}. 
Vertical advection (\texttt{vadvc}) and horizontal diffusion (\texttt{hdiff}) from the COSMO model are two such compound \juang{stencil} kernels, which represent the typical code patterns found in the \emph{dycore} of COSMO.  
Algorithm~\ref{algo:nero/hdiffKernel} shows {the} pseudo-code for \texttt{vadvc} and \texttt{hdiff}  kernels. 
The horizontal diffusion kernel iterates over a 3D grid performing \textit{Laplacian} and \textit{flux} to calculate different grid points, as shown in Figure~\ref{fig:NERO/hdiffMemory}. Vertical advection has a higher degree of complexity since it uses the Thomas algorithm~\cite{thomas} to solve a tri-diagonal matrix of the velocity field along the vertical axis. Unlike the {conventional} stencil kernels, vertical advection has dependencies in the vertical direction, which leads to limited available parallelism.
\input{NERO/images_new/hdiff_mem_access}
\input{NERO/algorithms/cosmo.tex}
Such compound kernels are dominated by memory-bound operations with complex memory access patterns and low arithmetic intensity. This poses a fundamental challenge to acceleration. %An implementation on a CPU leads to limited data locality and inefficient memory usage.
{CPU implementations of these kernels~\cite{stencilOnPOWER8} suffer from limited data locality and inefficient memory usage, as our roofline analysis in Figure~\ref{fig:nero/roofline} exposes}.


\subsection{CAPI SNAP Framework}
The OpenPOWER Foundation Accelerator Workgroup~\cite{open_power} created the CAPI SNAP framework, %which is an open-source environment
{an open-source environment for FPGA programming productivity}. 
CAPI SNAP {provides two key benefits}~\cite{wenzel2018getting}: (i) it enables an improved developer productivity for FPGA acceleration and eas{es the} use of CAPI's cache-coheren{ce mechanism}, and (ii) it places %the 
{FPGA-}accelerated compute engines, %or 
{also known as} FPGA \textit{actions}, closer to {relevant} data to achieve better performance. SNAP provides a simple API to invoke an accelerated \textit{action}, and also provides programming methods to {instantiate} customized accelerated \textit{actions} on the FPGA side. These accelerated \textit{actions} can be specified in C/C++ code that is then compiled to the FPGA target using the Xilinx Vivado High-Level Synthesis (\acrshort{hls}) tool~\cite{hls}. 


% SNAP is built on top of CAPI with the goal of making the use of CAPI-enabled FPGAs as easy as possible~\cite{wenzel2018getting}. SNAP provides a simple API to call for an accelerated action, and also provides programming methods to code customized accelerated actions on the FPGA side. These accelerated actions can be specified in C/C++ code which is then compiled to the FPGA target using the Xilinx Vivado HLS tool. 
% The OpenPOWER Foundation Accelerator Workgroup,  created the CAPI SNAP (Storage, Network, and Analytics Programming) framework which is an open source enablement environment that establishes twofold technology novelties: i) enabling application programmers to embrace FPGA acceleration and CAPI’s technology benefits; ii) placing the accelerated compute engines, or FPGA ``actions'', closer to the data to provide higher performance.

% SNAP is built on top of CAPI with the goal of making the use of CAPI-enabled FPGAs as easy as possible~\cite{wenzel2018getting}. SNAP provides a simple API to call for an accelerated action, and also provides programming methods to code customized accelerated actions on the FPGA side. These accelerated actions can be specified in C/C++ code which is then compiled to the FPGA target using the Xilinx Vivado HLS tool. 

% The Coherent Accelerator Processor Interface (CAPI) allows
% for attaching co-processors or peripheral devices to a POWER9
% system in a cache coherent way. CAPI removes the
% overhead and complexity of the I/O subsystem, allowing
% accelerators to operate as an integral part of a host application
% without the need for a device driver. The accelerator operates
% on the same virtual address space as the corresponding host
% process and has full access to it. A CAPI accelerator configuration for the FPGA consists of
% the POWER Service Layer (PSL) and one or multiple Accelerator Function Units (AFUs). The PSL exposes a defined
% interface to the AFUs and provides services such as memory
% address translation and interrupt handling to the individual
% AFUs. Data movement operations between the AFU and the PSL are handled via the buffer interface and carry 64 byte (a half of a cache line)
% per transaction.

% CAPI Storage, Network, and Analytics Programming (SNAP) was developed with the goal of making the leveraging of CAPI-enabled FPGAs as easy as possible~\cite{wenzel2018getting}. On the hoste side, it aenables simple intergration of AFUs by providing infrasturcture. While on the hardware side, the framework provides libraries for accessing hardware components such as DRAM, NVMe,FPGA etc. CAPI-SNAP framework provides a powerful tool with complements the Vivado design methodology and leads to tremendous increase in productivity.


==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%We have presented 
\juang{We introduce} \namePaper, the first design and implementation on a reconfigurable fabric \juang{with \gagann{high-bandwidth memory} (HBM)} to accelerate representative weather prediction kernels, i.e., vertical advection (\texttt{vadvc}) and horizontal diffusion (\texttt{hdiff}), from a real-world weather prediction application. %on a reconfigurable fabric.
These kernels are compound stencils that are found in various weather prediction applications, including the COSMO  model. \gagannn{We show that c}ompound kernels do not perform well on conventional architectures due to their complex data access patterns and low data reusability, which \gagann{make} them memory-bounded. 
\juang{Therefore, they greatly benefit from our near-memory computing solution \gagannn{that} takes advantage of the high \gagann{data transfer} bandwidth of HBM.}

%%We used 
%\juang{We use} the IBM SNAP framework to build \namePaper, which is an HBM-based hardware accelerator with CAPI2 technology. Our experimental results %showed 
%\juang{show} that \texttt{vadvc} and \texttt{hdiff} kernels on an FPGA+HBM %%outperforms 
%\juang{outperform} a highly optimized software implementation on a 16-core POWER9 configured with SMT4 %(64-threads) 
%\juang{(i.e., 64 threads)} by $4.2\times$ and $8.3\times$, respectively. Moreover, \namePaper~improves the active energy consumption by~$22\times$ and $29\times$ with an energy efficiency of 1.5~GFLOPS/Watt and 17.3~GFLOPS/Watt for \texttt{vadvc} and \texttt{hdiff}, respectively. We %%highlighted 
%\juang{highlight} the impact of precision optimized tile-size on a Pareto-optimal accelerator design. Additionally, we %provided 
%\juang{provide} a design comparison with DDR4-based solutions. %In future, we aim to study the applicability of weather kernels with alternative number systems such as posits and fixed-point arithmetic. 

\juang{\namePaper's implementations of \texttt{vadvc} and \texttt{hdiff} outperform the optimized software implementations on a 16-core POWER9 with \gagann{4-way multithreading} by $4.2\times$ and $8.3\times$, with $22\times$ and $29\times$ less energy consumption, respectively. 
We conclude that hardware acceleration on \gagann{an} FPGA+HBM fabric is a promising solution for compound stencil\gagann{s} present in weather prediction applications. \gagann{We hope that o}ur \gagann{reconfigurable near\gagannn{-}memory} accelerator inspire\gagann{s} developers of different high-performance computing applications that suffer from \gagann{the} memory bottleneck.
}


==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/introduction.tex <==
\section{Introduction} 
{Accurate weather prediction using detailed weather models is essential to {make} weather-dependent decisions in a timely manner.}
% The global scale increase in climate temperature is indisputable. Future climatic scenarios show a continuation of a rise in atmospheric temperature. To predict these ongoing climatic changes, detailed atmospheric simulations using climate models play a fundamental role. These models are based on physical laws that describe various components of the atmosphere. 
The Consortium for Small-Scale Modeling (COSMO)~\cite{doms1999nonhydrostatic} %is 
{built} one such weather model %, which was established 
to meet the high-resolution forecasting requirements of weather services. The COSMO model is a non-hydrostatic atmospheric prediction model currently being used by a dozen nations for meteorological purposes and research applications. 

The central part of the COSMO model ({called \emph{dynamical core} or \emph{dycore}}) solves the Euler equations on a curvilinear grid and applies implicit discretization {(i.e., parameters are dependent on each other at the same time instance~\cite{bonaventura2000semi})} in the vertical dimension and %an 
explicit discretization {(i.e., %{obtains a solution using previous system state}
{a solution is dependent on the previous system state}~\cite{bonaventura2000semi})} in the horizontal dimension. The use of different discretizations leads to three computational patterns~\cite{cosmo_knl}: {1)} horizontal stencils, {2)} tridiagonal solvers in the vertical dimension, and {3)} point-wise computation. These computational kernels are compound stencil kernels that operate on a three-dimensional grid~\cite{gysi2015modesto}.  
% In the literature~\cite{sano2014multi,7582502,chi2018soda,de2018designing}, we usually come across elementary stencils. However, compound stencils consist of a collection of elementary stencils that perform a series of computations on a complete three-dimensional grid. 
\emph{Vertical advection} ({\texttt{vadvc}}) and  \emph{horizontal diffusion} ({\texttt{hdiff}})  are such compound kernels found in the \emph{dycore} of the COSMO \gagannn{weather prediction} model. {These kernels} are representative {of} the data access {patterns and algorithmic} complexity of the entire COSMO model. {They} are similar to the kernels used in other weather and climate models~\cite{kehler2016high,neale2010description,doi:10.1175/WAF-D-17-0097.1}.  Their performance is dominated by memory-bound operations with unique irregular memory access patterns %leading to a 
{and} low arithmetic intensity that often results in $<$10\% sustained floating-point performance on current CPU-based systems~\cite{chris}. 

Figure~\ref{fig:nero/roofline} shows the roofline plot{~\cite{williams2009roofline}} for {an} IBM 16-core POWER9 CPU (IC922).\footnote{IBM and POWER9 are registered trademarks or common law marks of International Business Machines Corp., registered in many jurisdictions worldwide. Other product and service names might be trademarks of IBM or other companies.} After optimizing the \texttt{vadvc} and \texttt{hdiff} kernels for the POWER architecture by following the approach in~\cite{stencilOnPOWER8}, %we were able to 
{they} achieve {29.1}~GFLOP/s and 58.5~GFLOP/s, {respectively}, {for 64 threads}. {Our roofline analysis %suggests 
{indicates} that these kernels are constrained by the host DRAM bandwidth.} %The 
{Their} low arithmetic intensity limits %the performance of these kernels 
{their performance, which is one order of magnitude smaller than the peak performance,} and results in a fundamental memory bottleneck that %cannot be overcome with 
standard CPU-based optimization techniques {cannot overcome}.

 \begin{figure}[h]
  \centering
  \includegraphics[bb=32 29 546 396,width=0.8\textwidth,trim={1cm 0.8cm 1.5cm 0.6cm},clip]{NERO/images_new/roofline_fpl20_gagan.pdf}
    \caption{Roofline~\cite{williams2009roofline} for POWER9 (1-socket) showing vertical advection {(\texttt{vadvc})} and horizontal diffusion {(\texttt{hdiff})} kernels for single-thread and 64-thread %(one socket) 
    implementations. %Also shown is 
    {The plot shows also the rooflines} %potential 
    of the FPGAs used in this chapter}
    %compiled with \textit{xlc} using the following flags: qarch=pwr9 qtune=pwr9 O3 q64  qprefetch=aggressive qsmp=omp qsimd=auto
 \label{fig:nero/roofline}
\end{figure}

% Even after optimizing the hdiff kernel for the POWER architecture by following the approach in~\cite{xu2018performance}, we were barely able to achieve {39.6}~GFLOP/s.  
% This low performance is due to inefficient bandwidth utilization because of the limited locality of the data and multiple passes of data transfers.

% The current climate simulations based on CPU and GPU that are inefficient and lead to high energy consumption.

%{We attempt to overcome this
{\textbf{Our goal} is to overcome the memory} {bottleneck {of weather {prediction} kernels} by {exploiting near-memory {computation} capability on} FPGA accelerators with high-bandwidth memory (HBM)~\cite{6757501,hbm,lee2016smla} {that are attached} {to the host CPU}. 
Figure~\ref{fig:nero/roofline} shows the roofline model{s} of the two FPGA cards {(AD9V3~{\cite{ad9v3}} and AD9H7~{\cite{ad9h7}})} used in this chapter. 
FPGAs {can} {handle} %the 
irregular memory access patterns {efficiently} and %also 
offer significantly %more 
{higher} memory bandwidth {than the host CPU with} %for 
their on-chip URAMs {(UltraRAM)}, BRAMs {(block RAM)}, and {off-chip} HBM ({high-bandwidth memory} for the AD9H7 card).} % To overcome this bottleneck, %complementing 
% {augmenting} general-purpose cores with specialized FPGA accelerators is a promising approach to enhance overall system performance ({Figure~\ref{fig:roofline} also shows the roofline potential of the FPGAs used in our work}) without a significant increase in power consumption. 
However, taking full advantage of %an 
FPGAs for accelerating a workload is not a trivial task. To compensate {for} the higher clock frequency of the {baseline} CPUs, %an 
{our} FPGAs must exploit at least one order of magnitude more parallelism in a target workload. %This can only be accomplished by optimizing the design for the FPGA micro-architecture and sufficient FPGA programming skills.
{This is challenging, as it requires sufficient FPGA programming skills to {map the workload and} optimize the design for the FPGA microarchitecture.}



As mentioned in Section~\ref{subsection:intro/data_centric}, {modern FPGA boards deploy} 
%Upcoming 
{new} cache-coherent interconnects, such as %upcoming %high-bandwidth} 
 %interconnect technologies from 
IBM Coherent Accelerator Processor Interface (CAPI)~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators
(CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{cxlwhitepaper}, {which} allow tight integration of FPGAs with CPUs at %a 
high bidirectional bandwidth {({on} the order of tens of GB/s)}. However, memory-bound applications on FPGAs are limited by {the relatively} low DDR4 bandwidth (72 GB/s %max 
{for four independent dual-rank DIMM interfaces}{~\cite{VCU}}). %To this end,
{To overcome this limitation,} FPGA vendors have started offering devices {equipped} with HBM~\cite{xilinx_utlra,hbm_specs,intel_altera,lee2016smla} %capable of offering 
{with} a theoretical peak bandwidth of 410~GB/s. %HBM-based 
{HBM-equipped} FPGAs have the potential to \gagannn{reduce} the \gagannn{memory} bandwidth bottleneck, {but} a study of their advantages for %real-life 
{real-world memory-bound} applications %compared to current DDR4-based designs 
is still~missing.\\

% In this paper, we leverage the CAPI~SNAP environment to build a near high-bandwidth memory memory accelerator
% on an FPGA for a representative kernels from a real-world COSMO weather-prediction application. 


%Our research aims 
{We aim} to answer the following {research question}: \textbf{Can FPGA-based {accelerators} with HBM {mitigate} the performance bottleneck of {memory-bound} compound weather {prediction} kernels %on %current 
%CPU-based systems 
in an energy-efficient way?} As an answer to this question{,} we present \namePaper, a \underline{ne}ar-HBM accelerator for weathe\underline{r} predicti\underline{o}n. 
{We design and implement} \namePaper~%is used to implement and 
{on an FPGA with HBM to} optimize two %representative 
kernels (vertical advection and horizontal diffusion), %on an FPGA with HBM. 
%These kernels 
{which notably} represent %a 
{the} spectrum of {computational diversity} found in the COSMO {weather prediction} application. 
{We co-design a hardware-software framework and provide an optimized API to interface efficiently with the rest of the COSMO model, which runs on the CPU}.
Our {FPGA-based} solution {for \texttt{hdiff} and \texttt{vadvc}} leads to %active energy improvement 
{performance improvements of $4.2\times$ and $8.3\times$ and}
{energy reductions} of $22\times$ and $29\times$, {respectively,} {with respect to optimized CPU implementations~\cite{stencilOnPOWER8}}. 
%In addition, we have co-designed our hardware-software framework and provide an optimized API to interface efficiently with the rest of the COSMO model, which runs on the CPU.

% {T}he major contributions of this paper are {as follows}:
% \begin{itemize}
% %\item {Our analysis reveals that weather kernels are constrained by memory bandwidth on %the 
% %current systems. 
% \item {We perform {a detailed} roofline analysis to show that representative weather {prediction} kernels are constrained by memory bandwidth on \gagannn{state-of-the-art} CPU systems.}

% \item {We propose \namePaper, {the first} near-HBM FPGA-based accelerator} for representative kernels from a real-world weather prediction application.
% %\item We propose a data-centric heterogeneous memory hierarchy~caching with precision optimized tiling.

% %\item {We propose 
% \item {We optimize \namePaper~with} a data-centric caching scheme with precision-optimized tiling for a heterogeneous memory hierarchy {(consisting of URAM, BRAM, and HBM)}.

% % \item {We present} an architecture based on IBM CAPI~2.0 on a high-end FPGA %+
% % {with} HBM, which we compare to traditional %DDR4-based 
% % FPGAs {with DDR4} and %also provide 
% % a %comparison to the 
% % state-of-the-art IBM\textsuperscript{\textregistered} POWER9\textsuperscript{\textregistered}~CPU. \jgl{I think this contribution is redundant.} \gaganFeedback{Should we remove it?}
% \item %Performance and energy evaluation with scalability analysis of our accelerator. 
% {We evaluate the performance and energy consumption of our accelerator and perform a scalability analysis.} 
% We show that an FPGA+HBM-based design %can 
% outperforms a complete 16-core POWER9 {system}~(%configured with~
% {running} 64~threads)~by~$4.2\times$ for %a 
% {the} {vertical advection} {(\texttt{vadvc})} and $8.3\times$ for %a 
% {the} {horizontal diffusion} {(\texttt{hdiff})} kernels with energy {reductions of $22\times$ and $29\times$, respectively. Our design provides an energy efficiency of 1.5 GLOPS/Watt and 17.3 GFLOPS/Watt for \texttt{vadvc} and \texttt{hdiff} kernels,} {respectively}.

% \end{itemize}


% The remainder of this article is structured as follows. Section~\ref{sec:background} provides details of the representative kernels from the COSMO model and highlights the CAPI SNAP environment employed for building \namePaper. Section~\ref{sec:design} presents the actual design of \namePaper~and our auto-tuning approach towards finding a precision optimized tile size. %Section~\ref{subsec:scaling} describes a prediction model developed for scaling NARMADA on other FPGA devices. 
% Section~\ref{sec:results} outlines the system setup and the results of our experiments, including an efficiency analysis of our accelerator compared to traditional DDR4-based FPGAs and a standalone IBM\textsuperscript{\textregistered} POWER9 CPU. Section~\ref{sec:relatedWork} lists related work and Section~\ref{sec:conclusion} concludes the paper by indicating~future~directions.
% \jgl{Remove this paragraph.}


==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/relatedWork.tex <==
\section{Related Work}
\label{sec:nero/relatedWork}
\juang{To our knowledge, this is the first thesis to evaluate the benefits of using FPGAs equipped with \gagann{high-bandwidth memory (HBM) to accelerate} stencil computation.} \gagannn{We exploit near-memory capabilities of such FPGAs to accelerate important weather prediction kernels.}

\gagannn{Modern workloads exhibit limited locality and operate on large amounts of data, which causes frequent data movement between the memory subsystem and the processing units~\cite{ghose2019processing,mutlu2019,googleWorkloads,mutlu2019enabling}. This frequent data movement has a severe impact on overall system performance and energy efficiency. 
A way to alleviate this \emph{data movement bottleneck}~\cite{singh2019near, mutlu2019, ghose2019processing,mutlu2019enabling,googleWorkloads} is \emph{near-memory computing} (NMC), which consists of placing processing units closer to memory. 
NMC is enabled by new memory technologies, such as 3D-stacked memories~\cite{7477494,6757501,6025219,hbm,lee2016smla}, and also by cache-coherent interconnects~\cite{openCAPI, benton2017ccix, cxlwhitepaper},  which allow close integration of processing units and memory units. 
Depending on the applications \gagannn{and systems} of interest (e.g.,~\cite{nai2017graphpim,7056040,lee2018application,kang2013enabling,hashemi2016continuous,akin2015data,babarinsa2015jafar,lee2015bssync,chi2016prime,kim2016neurocube,asghari2016chameleon,boroumand2016lazypim,seshadri2015gather,liu2017concurrent,gao2015practical,morad2015gp,googleWorkloads,teserract,ahn2015pim,hsieh2016accelerating,hashemi2016accelerating}), prior works propose different types of near-memory processing units, such as general-purpose CPU cores~\cite{lee2018application,alian2018application,de2017mondrian,koo2017summarizer,7927081,teserract,nair2015active,6844483,googleWorkloads,boroumand2016lazypim,boroumand2019conda}, GPU cores~\cite{zhang2014top,7756764,tom,ghose2019demystifying}, reconfigurable units~\cite{7446059, jun2015bluedbm,istvan2017caribou,singh2019narmada}, or fixed-function units~\cite{ahn2015pim,hsieh2016accelerating,gu2016biscuit,nai2017graphpim,liu2018processing,kim2018grim,hashemi2016accelerating,hashemi2016continuous}}.

FPGA accelerators are promising to enhance overall system performance \gagann{with low power consumption.}
%without a significant increase in power consumption. 
Past works~\cite{jun2015bluedbm, kara2017fpga, alser2019shouji, giefers2015accelerating,diamantopoulos2018ectalk,Lee:2017:EBG:3137765.3137776,alser2017,chai_icpe19,chang2017collaborative,jiang2020,alser2019sneakysnake} show that FPGAs can be employed {effectively} for a wide range of applications. The recent addition of HBM to \juang{FPGAs} %has sparked architectural questions on using 
\juang{presents an opportunity to exploit} 
high \juang{memory} bandwidth with \gagannn{the} low-power FPGA fabric. 
The potential of high-bandwidth memory~\cite{hbm,lee2016smla} has been explored in many-core processors~\cite{hbm_joins,ghose2019demystifying} and GPUs~\cite{hbm_gpu_data_intensive,ghose2019demystifying}. 
\juang{A recent work~\cite{wang2020} shows the potential of HBM for FPGAs with a memory benchmarking tool.}
\juang{\namePaper} is the first work to accelerate a real-world HPC weather prediction application using \juang{the} FPGA+HBM fabric. {Compared to a previous work~\cite{singh2019narmada} that \juang{optimizes only the} horizontal diffusion kernel \juang{on an FPGA with DDR4 memory}, our analysis reveals \juang{that the} vertical advection kernel has a much lower compute intensity with little to no regularity.
Therefore, this thesis \juang{accelerates} both kernels that together represent the algorithmic diversity of the entire COSMO \gagannn{weather prediction} model. Moreover, compared to %their implementation 
\cite{singh2019narmada}, \juang{\namePaper~\gagannn{improves performance by}} $1.2\times$ on a DDR4\gagannn{-}based \gagann{board} and $37\times$ on an HBM-based board for horizontal diffusion by using a dataflow implementation with auto-tuning.}

\gagan{Enabling higher performance for stencil computations has been a subject of optimizations %all
across the \juang{whole} computing stack~\cite{sano2014multi,7582502,chi2018soda,de2018designing,christen2011patus,  datta2009optimization, meng2011performance, henretty2011data, strzodka2010cache, tang2011pochoir,gonzalez1997speculative,armejach2018stencil,gysi2015modesto}}. \juang{Szustak~\etal} accelerate the MPDATA advection scheme on multi-core CPU~\cite{szustak2013using} and computational fluid dynamics kernels on FPGA~\cite{mpdata}. Bianco~\etal~\cite{bianco2013gpu} \juan{optimize the COSMO \gagannn{weather prediction} model} for GPUs while Thaler~\etal~\cite{cosmo_knl} \juan{port} COSMO to a many-core system.  Wahib~\etal~\cite{wahib2014scalable} \juang{develop} an analytical performance model for choosing an optimal GPU-based execution strategy for various scientific applications, including COSMO. 
%  Recently, Rojek~\etal~\cite{cfd_vadv} showed the applicability of using Xilinx Alveo FPGAs to solve stencils, such first-order step of the non-linear iterative upwind advection MPDATA, involved in the domain of computational fluid-dynamics.
Gysi~\etal~\cite{gysi2015modesto} \juang{provide} guidelines for optimizing stencil kernels for CPU--GPU systems.
 


% {Upcoming high-bandwidth} interconnect technologies from IBM CAPI~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators
% (CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{sharma2019compute}
% provide a tight integration of FPGAs with host-CPU system. The IBM Coherent  Accelerator  Processor  Interface (CAPI) removes significant device driver overhead, which IBM has leveraged to show the applicability of CAPI~1.0 to accelerate various algorithms such as
% arithmetic kernels~\cite{giefers2015accelerating} and graph processing~\cite{Lee:2017:EBG:3137765.3137776}. Diamantopolous~\etal~\cite{8373077} used the CAPI SNAP framework to build a trans-precise neural network co-processor. 



==> PhD_Thesis_Updated_arxiv (1)/NERO/sections/results.tex <==
\section{Results}
\label{sec:nero/results}

\subsection{System Integration}
We implemented our design on an Alpha-Data ADM-PCIE-9H7 card~\cite{ad9h7} featuring the Xilinx Virtex Ultrascale+ XCVU37P-FSVH2892-2-e~\cite{vu37p} and 8GiB HBM2 %(4GiB per stack)
{(i.e., two stacks of 4GiB each)}~\cite{hbm} with an IBM POWER9 as the host system. The POWER9 socket has 16 cores, each of which supports four-thread simultaneous multi-threading. We compare our HBM-based design to a conventional DDR4 DRAM~\cite{ad9v3} based design. %The DDR4 experiments were performed using
{We perform the experiments for the DDR4-based design on} 
an Alpha-Data ADM-PCIE-9V3 card featuring the Xilinx Virtex Ultrascale+ XCVU3P-FFVC1517-2-i~\cite{vu37p}.

Table~\ref{tab:nero/systemparameters}
provides our system parameters.
We have co-designed our hardware and software interface around the SNAP framework while using the HLS design flow.
\input{NERO/tables/system.tex}

\subsection{Evaluation}
\label{subsection:nero/evaluation}
We %ran 
{run} our experiments using a $256\times256\times64$-point domain similar to the grid domain used by the COSMO {weather prediction} model. We employ an auto-tuning technique to determine a Pareto-optimal solution (in terms of performance and resource utilization) for our 3D window dimensions.
{The auto-tuning {with OpenTuner} exhaustively searches for every tile size in the x- and y-dimensions for \texttt{vadvc}.\footnote{\texttt{vadvc} has dependencies in {the} z-dimension; therefore, it cannot be parallelized in the z-dimension.} For \texttt{hdiff}, we consider sizes in all three dimensions. We define our auto-tuning as a multi-objective optimization with the goal {of maximizing} performance with  minimal resource utilization.} Section~\ref{sec:nero/design} provides further details on our design.
Figure~\ref{fig:nero/single_afu} shows hand-tuned and auto-tuned {performance and FPGA resource utilization} results for {\texttt{vadvc}}{, as a function of the chosen tile size. From the figure, we draw two observations.} 

 \begin{figure}[h]
  \centering
  \includegraphics[width=0.98\linewidth,trim={0.4cm 0.3cm 0.35cm 0.2cm},clip]{NERO/images_new/singleAFU_vadvc_4.eps}
      \caption{Performance {and FPGA resource utilization } {of} single \texttt{vadvc} PE{, as a function of tile-size,} using hand-tuning and auto-tuning for (a) single-precision (32-bit) and (b) half-precision (16-bit). We highlight the Pareto-optimal solution that we use for our \texttt{vadvc} accelerator \gagan{(with a red circle). Note that }the Pareto-optimal solution changes with precision
  \label{fig:nero/single_afu}}
 \end{figure}

{First, by using the auto-tuning approach and our careful FPGA microarchitecture design, we can get \gagan{P}areto-optimal results with a tile size of $64\times2\times64$ for single-precision {\texttt{vadvc}}\gagan{, which} gives us a peak performance of 8.49 GFLOP/s. For half-precision, we use a tile size of $32\times16\times64$ to achieve a peak performance of 16.5 GFLOP/s. We employ a similar strategy for {\texttt{hdiff}} to attain a single-precision performance of 30.3 GFLOP/s with a tile size of $16\times64\times8$ and a \gagan{half-precision} performance of 77.8 GFLOP/s \gagan{with} a tile size of $64\times8\times64$. 

Second, in FPGA acceleration, designers usually rely on expert judgement to find the appropriate tile-size and often adapt the design to {use} homogeneous tile sizes. However, as shown in Figure~\ref{fig:nero/single_afu}\gagan{,} such hand-tuned implementations lead to sub-optimal results in terms of either resource utilization~or~performance. 

{We conclude that} the {Pareto-optimal} tile size depends on the data precision used\gagan{:} a \gagan{good} tile-size for single-precision might lead to poor results when used with half-precision.

\gagan{Figure~\ref{fig:nero/perf} shows {single-precision} performance results for the (a) vertical advection and (b) horizontal diffusion kernels. For both kernels, we implement our design %with 
{on} an HBM- and {a} DDR4-based FPGA board. To compare the performance results, we  scale the number of PEs and analyze the change in execution time. For {the} DDR4-based design, we %were able to accommodate 
{can accommodate only} 4 PEs on {the} 9V3 board, while for the HBM-based design, we %were able 
{can} fit 14 {PE}s before exhausting the on-board resources. {We draw four observations from the figure.}

 \begin{figure}[h]
  \centering
  \includegraphics[width=0.98\linewidth,trim={0.4cm 0.3cm 0.35cm 0.4cm},clip]{NERO/images_new/perf_5.eps}
   \caption{ {Single-precision} performance for (a) \texttt{vadvc} and (b) \texttt{hdiff}{, as a function of accelerator PE count on the HBM- and DDR4-based FPGA boards}. %\gagan{In the} HBM-based board, we scale the number of memory ports (upto 16 ports of 256-bit each) with {the} number of PEs. DDR4-{based board} \gagan{has only} 1x512-bit memory channel to feed \textit{n} PEs. 
   \gagan{We also show {the}} single socket (64 threads) performance of \gagan{an} IBM POWER9 host system for both \texttt{vadvc} and \texttt{hdiff}
  \label{fig:nero/perf}}
%   \vspace{-0.3cm}
 \end{figure}

First, our {full-blown} \gagan{HBM-based} {\texttt{vadvc}} and {\texttt{hdiff}} implementations} {provide} 157.1~GFLOP/s and 608.4~GFLOP/s \gagan{performance}, which are 4.2$\times$ and 8.3$\times$ higher than the performance of a complete~POWER9~socket. 
%{In case}, if we use half-precision, with 
{For half-precision, if we use} 
the same amount of {PE}s as in single precision, {our accelerator} %can 
{reaches} a performance of 247.9~GFLOP/s for \texttt{vadvc} ($2.1\times$ {the} single-precision performance) and 1.2~TFLOP/s for \texttt{hdiff} ($2.5\times$ {the} single-precision performance). \gagan{{Our} DDR4-based design achieves 34.1~GFLOP/s and 145.8~GFLOP/s {for \texttt{vadvc} and {\texttt{hdiff}, respectively, which are}} 1.2$\times$ and 2.5$\times$ {the} performance {on the POWER9 CPU}.

Second, for a single PE, which %is fetching 
{fetches} data from a single memory channel, {the} DDR4-based design provides higher performance {than the HBM-based design}. %This is because the DDR4-based FPGA has a higher bus width of 512-bit compared to the HBM port width of 256-bit {, which leads to a lower transfer rate for HBM-based port than DDR4-based port (0.8-2.1 GT/s\footnote{gigatransfers per second} vs. 2.1-4.3 GT/s).} To match DDR4 bitwidth, we would need to fetch from multiple HBM ports {in} parallel. However, using more ports lead\gagan{s} to higher power consumption ($\sim$1 Watt per HBM port). 
{This is because the DDR4-based FPGA has {a} larger bus width (512-bit) than an HBM port (256-bit). 
This {leads to} a lower transfer rate for an HBM port (0.8-2.1 GT/s\footnote{Gigatransfers per second.}) than for a DDR4 port (2.1-4.3 GT/s). 
One way to match the DDR4 bus width would be to have a single PE fetch data from multiple HBM ports in parallel. 
However, using more ports leads to higher power consumption ($\sim$1 Watt per HBM port).}

Third, as we increase the number of PEs, we observe a linear reduction in the execution time of {the} HBM-based design. 
This is because %for data-parallel applications, 
we can {evenly} divide the computation between multiple PEs{,} each \gagan{of which} %is} fed 
{fetches data} from a separate HBM port. 

Fourth, {in the DDR4-based design, the use of only a single channel to feed multiple {PE}s leads to a congestion issue that causes a non-linear run-time reduction.} {As we {increase the number of accelerator PEs}, we observe that the} {PEs}} %have to stall and wait for their turn to read from a single memory channel.}
{compete for a single memory channel, which causes frequent stalls.} {This phenomenon leads to worse performance scaling characteristics for the DDR4-based design as compared to the HBM-based design.}

% {Note that DDR4-based DRAM channel is of 512-bit, compared to a single 256-bit port of HBM, Thereotically, 2$\times$ HBM ports=1$\times$ DDR4-DRAM port. However, HBM ports are based on DDR3 standard that exhibit lower GT/s than DDR4 (0.8-2.1 vs. 2.1-4.3).}

\subsection{{Energy} Analysis}
We compare the energy consumption of our accelerator to \gagan{a} {16-core} POWER9 host system. For the POWER9 system, we use the AMESTER\footnote{https://github.com/open-power/amester} tool to measure the active power\footnote{Active power denotes the difference between the total power of a complete socket (including CPU, memory, fans, I/O, etc.) when an application is running compared to when it is idle.} consumption. % of 
{We measure}~99.2~Watt\gagan{s} for \texttt{vadvc}, and ~97.9~Watt\gagan{s} for \texttt{hdiff} by monitoring {built-in} power sensors in %our 
{the POWER9}~system. 

{By executing these kernels on an HBM-based board, we {reduce the energy consumption by} $22\times$ for {\texttt{vadvc}} and $29\times$ for {\texttt{hdiff}} compared to %executing on a 
{the} 16-core POWER9 system.} 
\gagan{Figure~\ref{fig:nero/energy_eff} shows the energy efficiency (GFLOPS per Watt) for {\texttt{vadvc}} and {\texttt{hdiff}} %with 
{on the HBM-} and DDR4-based designs.} 
We make three \gagan{major} observations from the figure. 

 \begin{figure}[h]
  \centering
  \includegraphics[width=0.98\linewidth,trim={0.4cm 0.3cm 0.35cm 0.4cm},clip]{NERO/images_new/energyEfficiency_3.eps}
     \caption{Energy efficiency for (a) \texttt{vadvc} and (b) \texttt{hdiff} on HBM- and DDR4-based FPGA boards. {We also show {the}} single socket (64 threads) energy efficiency of \gagan{an} IBM POWER9 host system for both \texttt{vadvc} and \texttt{hdiff}
     %\gagan{For the} HBM-based board we scale the number of memory ports (upto 16 ports of 256-bit each) with number of {PE}s. DDR4-system \gagan{has} only 1x512-bit memory channel to feed \textit{n} {PEs}.
  \label{fig:nero/energy_eff}}
 \end{figure}


First, with our %\gagan{highest-performing} 
{full-blown} \gagan{HBM-based} designs \gagan{(i.e., 14 PEs for \texttt{vadvc} and 16 PEs for \texttt{hdiff})}, we achieve %an 
energy efficiency {values} of 1.5~GFLOPS/Watt and 17.3~GFLOPS/Watt for {\texttt{vadvc}} and {\texttt{hdiff}}, respectively. 

Second, %as seen in the case of performance \gagan{evaluation}, 
the DDR4-based \gagan{design} is more energy efficient {than the HBM-based design} {when the number of PEs is small}. 
{This observation is inline with our discussion about performance with small PE counts in Section~\ref{subsection:nero/evaluation}.} 
However, as we increase the number of {PE}s, the HBM\gagan{-based design provides better energy efficiency} for memory-bound kernels. \gagan{This is because} more data can be fetched {and processed} in \gagan{parallel} {via} multiple ports. 

Third, kernels like {\texttt{vadvc}}, with intricate memory access patterns, \gagan{are not able to} reach the peak {computational power} of FPGAs. {The large amount of control flow in {\texttt{vadvc}} leads to large resource consumption. Therefore, {when} increasing the PE count, we observe a high increase in power consumption with low energy efficiency. } 

{We conclude that} enabling many HBM ports might not always {be} beneficial in terms of energy consumption because each HBM port {consumes} $\sim$1 Watt of power consumption. However, \gagan{data-parallel} kernels like {\texttt{hdiff}} can achieve much higher performance in an energy efficient manner} {with more PEs and HBM~ports.} 

\subsection{{FPGA Resource Utilization}}
Table~\ref{tab:nero/utilization} shows the \gagan{resource} utilization \gagan{of \texttt{vadvc}} and \texttt{hdiff} on the AD9H7 board. {We draw two observations. First, there is a high BRAM consumption compared to other FPGA resources. This is because we implement input, field, and output signals as \texttt{hls::streams}. In {high-level synthesis}, by default, streams are implemented as FIFOs that make use of BRAM. Second,  \texttt{vadvc} has a much larger resource consumption  than \texttt{hdiff} because \texttt{vadvc} has higher computational complexity and requires {a larger} number of fields to \gagan{perform} the \gagan{compound} stencil calculation. \gagan{Note that for} \texttt{hdiff}, we can \gagan{accommodate} more {PE}s, but in this thesis, we  make use of only \gagan{a} single HBM stack. Therefore\gagan{,} we \gagan{use} 16 {PE}s \gagan{because} a single \gagan{HBM} stack offers 16 memory ports.}

\input{NERO/tables/utilization}


%   \begin{figure}[h]
%     \vspace{-0.3cm}
%   \centering
%   \includegraphics[width=0.8\linewidth,trim={0.3cm 0.4cm 0.3cm 0.2cm},clip]{images_new/Utilization.pdf}
%   \vspace{-0.25cm}
%   \caption{FPGA resource utilization for AFUs with the highest performance achieved for {vadv} and {hdiff}. Also shown is the energy improvement compared to an IBM\textsuperscript{\textregistered}~POWER9~system.
%  \label{fig:Utilization}}
%  \vspace{-0.4cm}
%  \end{figure}


% ********************************************************

% As the data movement becomes more dominant rather than processing due to complex inherent memory patterns.
%   \begin{figure}[]
%   \centering
%   \includegraphics[width=\linewidth,trim={0.4cm 0.3cm 0.35cm 0.4cm},clip]{images/HDIFFscale_embed.pdf}
%  % \includegraphics[width=\linewidth,trim={9cm 6.6cm 9cm %5cm},clip]{images/HDIFFscale_embed_excel.pdf}
%   \vspace{-0.55cm}
%   \caption{Scaling the number of AFUs for B~and U-based heterogeneous memory hierarchy with different window~size. B-Hierarchy and U-hierarchy are able to achieve $2.5\times$ and $3.3\times$ performance compared to a POWER9 socket.
%  \label{fig:scaling}}
%  \vspace{-0.3cm}
%  \end{figure}
% \subsection{AFU Scaling}
% Figure~\ref{fig:scaling} shows the scaling of AFUs for both B and U-Hierarchies. Note, we only show the results that we were able to implement before the on-board resources were exhausted. In the case of $32\times32\times32$ window size, BRAM exhaustion was the reason we were not able to synthesize more accelerators for both B and H-hierarchy. Upon scaling the B-hierarchy, we were able to implement a maximum of eight AFUs, which achieved a performance gain of 2.5$\times$ compared to a complete 16-core POWER9 socket configured with SMT4 (64-threads). However, by adding an extra level of URAM, we were able to decrease the number of BRAMs per AFU, thus reaching a total of 16~AFUs with a window size of $8\times8\times8$. This design yielded a performance of 129.9~GFLOP/s, which is 3.3$\times$ better than that of a complete~POWER9~socket.  
% URAM thereby offers the resources to construct a more heterogeneous domain-specific cache hierarchy. This tailored memory hierarchy
% offers significantly more loading and eviction freedom than the hardware-managed caches in CPUs or GPUs. Moreover the U-Hierarchy scheme allows us to use the available resources more effectively, as shown in Figure~\ref{fig:Utilization}. As mentioned in Section~\ref{subsec:scaling} partitioning a bigger window size leads to a complex network of address multiplexers. As a result, we see high usage of LUTs for the implemented designs.


%   \input{tables/fpgaFamily.tex}
%   \begin{figure}[b]
%     \vspace{-0.3cm}
%   \centering
%   \includegraphics[width=\linewidth,trim={0.3cm 0.4cm 0.6cm 0.2cm},clip]{images/UtilizationScaled.pdf}
%   \vspace{-0.4cm}
%   \caption{FPGA resource utilization for AFUs with the highest performance achieved using B and U-based heterogeneous memory hierarchy. Also shown is the energy improvement and energy efficiency compared to an IBM\textsuperscript{\textregistered}~POWER9~system.
%  \label{fig:Utilization}}
%  \vspace{-0.4cm}
%  \end{figure}


% The proposed heterogeneous memory hierarchy with window cahing ensures the scalability of our accelerator design with different 3D window sizes. 



 
%   \begin{figure}[b]
%   \centering
%   \vspace{-0.5cm}
%   \includegraphics[width=\linewidth,trim={0.4cm 0.5cm 0.4cm 2.65cm},clip]{images/powerResults.pdf}
%   \caption{Active energy consumption and execution time for different B and U-based hierarchies.
%  \label{fig:hdiffPower}}
%  \vspace{-0.25cm}
%  \end{figure}


% The measured active energy improvement and performance per Watt of NARMADA are up to $13.5\times$ and 5.5~GFLOPS/Watt than that of the POWER9 processor in the case of a multi-AFU B-Hierarchy-based solution. 




==> PhD_Thesis_Updated_arxiv (1)/NERO/tables/fpgaFamily.tex <==
\begin{table*}[h]
  \caption{Prediction results for different CAPI 2.0 enabled boards across FPGA families. }
    \label{tab:nero/fpgaFamily}
   \vspace{-0.2cm}
    \begin{threeparttable}
     \begin{center}
\scalebox{1}{
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{FPGA Board} & \multirow{2}{*}{FPGA Device} & \multicolumn{5}{c|}{Utilization\%} & \multirow{2}{*}{Window} & \multirow{2}{*}{AFU} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Performance\\ (GFLOP/s)\end{tabular}} & \multirow{2}{*}{Energy Impr.}  \\ \cline{3-7}
                             &                              & BRAM  & DSP  & FF  & LUT  & URAM &                         &                      &                                                                                 &                                                                            \\ \hline
                             
ADM-PCIE-9V3\tnote{*} & XCVU3P-2 &  71 &  66 &  49&79 & 58  &$8\times8\times8$ & 16 &  120.1 &  18.1$\times$       \\ \hline

ADM-PCIE-KU3\tnote{*} & XCKU3P-2   & 70      &    33  & 61    & 96     & 70     &  $16\times16\times16$  & 4  &    48.9    &9.3$\times$      \\ \hline
Semptian NSA121B  & XCKU060    &   55    & 49     &   73  &  79    &  -    &$8\times8\times8$   & 8    & 83.5     &20.6$\times$     \\ \hline
ADM-PCIE-8K5  & XCKU115   &    59   &  58    & 81    & 77     &   -   &   $8\times8\times8$ & 16      &  162.7     &   19.2$\times$        \\ \hline


% ADM-PCIE-9V3\tnote{*} \tnote{+} & XCVU3P-2 &  71 &  66 &  49&79 & 58  &$8\times8\times8$ & 16 &  120.1 &  18.1$\times$       \\ \hline

% ADM-PCIE-KU3\tnote{*} \tnote{+} & XCKU3P-2   & 70      &    33  & 61    & 96     & 70     &  $16\times16\times16$  & 4  &    48.9    &9.3$\times$      \\ \hline
% Semptian NSA121B\tnote{$\dagger$}  & XCKU060    &   55    & 49     &   73  &  79    &  -    &$8\times8\times8$   & 8    & 83.5     &20.6$\times$     \\ \hline
% ADM-PCIE-8K5\tnote{+}  & XCKU115   &    59   &  58    & 81    & 77     &   -   &   $8\times8\times8$ & 16      &  162.7     &   19.2$\times$        \\ \hline


\end{tabular}}
\end{center}
% \begin{tablenotes}[para,flushleft]\footnotesize
%  \qquad \qquad \qquad  *URAM memory is available only in  Ultrascale\tnote{+} families \qquad  \tnote{+} Implemented and estimated  \qquad \tnote{$\dagger$} Estimated (not currently \newline \tab \tab   \qquad\qquad\qquad\qquad\qquad\qquad\qquad \qquad available at our nodes)
\begin{tablenotes}[para,flushleft]\footnotesize
 \qquad \qquad \qquad  *URAM memory is available only in  Ultrascale\tnote{+} families 
%  \qquad  \tnote{+} Implemented and estimated  \qquad \tnote{$\dagger$} Estimated (not currently \newline \tab \tab   \qquad\qquad\qquad\qquad\qquad\qquad\qquad \qquad available at our nodes)
 \end{tablenotes}
\end{threeparttable}
\vspace{-0.4cm}
\end{table*}


%KU3 belongs from US+ but has half the amount of resoursce as 9v3


==> PhD_Thesis_Updated_arxiv (1)/NERO/tables/system.tex <==


%   \vspace{0.2cm}
\begin{table}[h]
  \caption{System parameters and hardware configuration for the CPU and the FPGA board}
  \vspace{-0.4cm}
    \label{tab:nero/systemparameters}
      \begin{center}
      \footnotesize
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{|l@{\hspace{0.1\tabcolsep}}|p{7cm}|}

\hline
\textbf{Host CPU} 

 & 16-core IBM POWER9 AC922 \\&@3.2 GHz, 4\gagann{-way} SMT\\
 \hline
 \textbf{Cache-Hierarchy}&32 KiB L1-I/D, 256 KiB L2, 10 MiB L3 \\
 \hline
 \textbf{System Memory}&16x32GiB RDIMM DDR4 2666 MHz \\
\hline

 \begin{tabular}[c]{@{}l@{}}
 \textbf{HBM-based} \\\textbf{FPGA Board} \end{tabular}  &
  \begin{tabular}[c]{@{}l@{}}
 Alpha Data
ADM-PCIE-9H7\\
 Xilinx Virtex Ultrascale+ XCVU37P-2\\
  8GiB (HBM2) with PCIe Gen4 x8\\
 \end{tabular}\\
\hline
 \begin{tabular}[c]{@{}l@{}}
 \textbf{DDR4-based} \\\textbf{FPGA Board} \end{tabular}  & \begin{tabular}[c]{@{}l@{}}
 Alpha Data
ADM-PCIE-9V3\\
 Xilinx Virtex Ultrascale+ XCVU3P-2\\
 8GiB (DDR4) with PCIe Gen4 x8
  \end{tabular}\\

 
 
% \hline
% \textbf{FPGA Family}  & \\
% \hline
% \textbf{Device Memory}  & 8GiB (DDR4)\\
% \hline
% \textbf{CAPI Interface}  & PCIe Gen4 x8\\



%NVM bandwidth & bw\textsubscript{ext} & 6 GB/s\\

\hline

\end{tabular}
}
  \end{center}
 \end{table}



==> PhD_Thesis_Updated_arxiv (1)/NERO/tables/utilization.tex <==
%   \vspace{0.2cm}
\begin{table}[h]
  \caption{FPGA resource utilization {in} {our highest-performing HBM-based design{s for}} \texttt{vadvc} and \texttt{hdiff}}
  \vspace{-0.4cm}
    \label{tab:nero/utilization}
          \begin{center}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{llllllc}
\toprule
\textbf{Algorithm} & \textbf{\acrshort{bram}} & \textbf{\acrshort{dsp}} & \textbf{\acrshort{ff}} & \textbf{\acrshort{lut}} & \textbf{\acrshort{uram}} \\ \hline
\texttt{vadvc}              & 81\%            & 39\%           & 37\%          & 55\%           & 53\%                         \\ 
\texttt{hdiff}              & 58\%            & 4\%            & 6\%           & 11\%           & 8\%                           \\ \bottomrule
\end{tabular}
}
  \end{center}
\vspace{-0.2cm}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/background.tex <==
In the literature, data-centric computing has manifested with names such as \textit{processing-in memory} (PIM),  \textit{near-data processing} (NDP), \textit{near-memory processing} (NMP), or in the case of non-volatile memories as \textit{in-storage processing} (ISP). However, all these terms fall under the same umbrella of \textit{near-memory computing} (NMC), with the core principle of performing processing closer to the memory in contrast to the traditional \textit{compute-centric} approach. In this dissertation, we focus on NMC rather than \textit{in-situ} data-centric computing called \textit{computation-in-memory} that performs logical operations using memory itself  by exploiting physical properties of memory devices, such as phase-change memory. 

This chapter deals with analyzing and organizing the extensive body of literature on NMC architectures across various dimensions: starting from the memory level where this paradigm is applied to the granularity of an application that could be executed on these architectures. \fc{We provide representative architectures in each category of our NMC taxonomy.} %\fc{We provide relevant works in each category of our taxonomy.} 
The remainder of this chapter is structured as follows. Section~\ref{sec:nmc_review/background} provides background on near-memory computing. Section~\ref{sec:nmc_review/classificationmodel} outlines the evaluation and classification scheme that we use.  Section~\ref{sec:nmc_review/challenges}  highlights the present challenges with NMC-based systems, which include 
lack of evaluation tools, virtual memory, memory coherence, task scheduling, and data mapping.  Finally, Section~\ref{sec:nmc_review/concludes} concludes the chapter.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Section \ref{sec:nmc_review/analyticmodel} presents a high-level analytic approach to model NMC systems with a comparison to a traditional compute-centric approach. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Background and Related Work}
\label{sec:nmc_review/background}
The idea of processing close to the memory dates back to the 1960s~\cite{ALogicinMemoryComputer}. However, the first appearance of data-centric systems can be traced back to the early 1990s~\cite{5727436,Kogge1994,fbram1994,375174,592312,808425}. As an example, \textit{Vector IRAM} (VIRAM)~\cite{612252}, where the researchers develop a vector processor with an on-chip embedded DRAM. They use VIRAM to exploit data parallelism in multimedia applications. Although such works obtained promising results, these earlier systems did not penetrate the market, and their adoption remained limited. One of the main reasons was attributed to the technological limitations because the amount of memory we could integrate with the processor was limited due to the difference in logic and memory technology processes.



Today, after almost two decades of dormancy, research in NMC architectures is regaining attention. We can largely attribute this resurgence to the following three reasons. First, technological advancements in the stacking technology -- 3D ( e.g., hybrid memory cube (HMC)~\cite{7477494} see Figure~\ref{fig:nmc_review/HMCLayout}) and 2.5D (e.g., high-bandwidth memory (HBM)~\cite{hbm}) stacking that blends logic and memory in the same package. Second, moving the computation closer to where the data reside allows for sidestepping the performance and energy bottlenecks due to data movement by circumventing memory-package pin-count limitations. Third, \ph{the increase in data volumes produced in various} application domains, such as weather prediction modeling, radio astronomy, and bioinformatics, calls for newer architectures designed to handle the overwhelming amount of data. As a result, in recent years, researchers have proposed various NMC designs and proved their potential in enhancing performance in many application domains~\cite{teserract, ahn2015pim,nair2015active,7446059,hsieh2016accelerating,tom,ke2020recnmp,gomezluna2021upmem,cali2020genasm,fernandez2020natsa,singh2020nero}. \fc{For CIM-based architectures, prior works demonstrate that CIM can be achieved using various memory technologies such as static random-access memory (SRAM)~\cite{simon2020blade,computecache,kang2014energy,neuralcache2018}, dynamic random-access memory (DRAM)~\cite{seshadri2017ambit,chang2016low,seshadri2013rowclone}, PCM~\cite{li2016pinatubo}, and ReRAM~\cite{levy2014logic,kvatinsky2014magic,shafiee2016isaac}.}


\begin{figure}[h]
\centering
\includegraphics[bb=87 146 666 399,width=0.7\linewidth,trim={3cm 5cm 10.2cm 4.8cm},clip]{NMC_review/img/fig3journall_final.pdf}
\caption{Micron's Hybrid Memory Cube (\acrshort{hmc})~\cite{7477494} comprising of several DRAM layers stacked on top of a logic layer connected by through-silicon vias (TSVs). The memory organization is divided into vaults, with each vault consisting of multiple DRAM banks
\label{fig:nmc_review/HMCLayout}}
\end{figure}

Loh~\etal~\cite{loh2013processing}, in their position paper, present an initial taxonomy for NMC. This taxonomy is based on the computing interface with software. Siegl~\etal~\cite{siegl2016data}, in an overview paper, gave a historical evolution of NMC. Similar \dd{to the approach of this thesis}, Mutlu~\etal\cite{mutlu2020modern},  provide a thorough overview of the mechanisms and challenges in the field of near-memory computing. Unlike \dd{the survey of this thesis}, the paper~\cite{mutlu2020modern} does not focus on providing systematization to the literature. Our review characterizes near-memory computing literature in various dimensions starting from the memory level, where we apply the paradigm of near-memory computing to the type of near-memory processing unit, memory integration, and type of workloads/applications. 


==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/challenges.tex <==
\section{Challenges of Near-Memory Computing}
\label{sec:nmc_review/challenges}
In this section, we highlight five critical challenges in the domain of NMC. The challenges include evaluation tools,  virtual memory support, memory coherency, task scheduling, and data mapping. We need to address these challenges before NMC can be established as a de facto solution for modern data-intensive workloads.  %Additional challenges on design space exploration, reliable simulators, which can deal with these heterogeneous environments, will be discussed in Section~\ref{sec:nmc_review/modelingmethod}.
\subsection{Performance Evaluation Tools and Benchmarks}
\label{subsec:nmc_review/performanceevaluation}
As mentioned in Section~\ref{sec:intro/problem}, architects often use various evaluation techniques to navigate the design space of a new architecture. Based on the level of detail required, architects make use of analytic models or more detailed simulation-based techniques. 
 
\noindent\textbf{(1) Analytic modeling} abstracts low-level system details and provide quick performance estimates at the cost of accuracy. In the early design stage, system architects are faced with large design choices that range from semiconductor physics and circuit level to micro-architectural properties and cooling concerns~\cite{jongerius2017analytic}. Thus, during the first stage of design-space exploration, analytic models can provide quick estimates.

% Mirzadeh~et~al.~\cite{mirzadeh2015sort} study a join workload, on multiple HMC like 3D-stacked DRAM devices connected via SerDes links using a first-order analytic model. Zhang~et~al.~\cite{xu2015scaling} design an analytical model using machine learning techniques to estimate the final device performance. Recently, Lima~et~al.~\cite{deLima:2018:DSE:3203217.3203280} provide a theoretical design space study for enabling processing in the logic layer of HMC taking into consideration area and power limits.




\noindent \textbf{(2) Simulation-based modeling} allows us to achieve more accurate performance numbers by precisely modeling various micro-architectural mechanisms. This approach, however, can be quite slow compared to analytic techniques. There have been various academic efforts~\cite{7336224,7529923,7544479,ramulator-pim-repo} to build open-source NMC simulators. However, there is a large room for improvement for developing a cycle-accurate simulator that can allow us to explore a wide range of near-memory compute configurations. In Table~\ref{tab:nmc_review/simulator}, we mention some of the academic efforts to create NMC simulation infrastructure.

% \begin{table}[h]
% \renewcommand{\arraystretch}{1.2}
% \centering
% \renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{14pt}
% \begin{tabular}{lccc}
% \hline
% \textbf{Simulator} & \textbf{Year} & \textbf{Category} \\ \hline
% Sinuca~\cite{7336224} & 2015 & Cycle-Accurate \\
% HMC-SIM~\cite{7529923} & 2016 & Cycle-Accurate \\
% CasHMC~\cite{7544479} & 2016 & Cycle-Accurate  \\
% SMC~\cite{Azarkhish:2016:DEP:2963802.2963805} & 2016 & Cycle-Accurate \\
% CLAPPS~\cite{junior2017generic} & 2017 & Cycle-Accurate  \\ 
% Ramulator-PIM~\cite{ramulator-pim-repo}      & 2019    & Cycle-Accurate   \\

% \hline
% \end{tabular}
% \caption{Open source simulators}
% \label{tab:nmc_review/simulator}
% \end{table}
\begin{table}[ht]
\renewcommand{\arraystretch}{1.2}
\caption{Academic NMC simulators}
\label{tab:nmc_review/simulator}
\centering
{\footnotesize
\begin{tabular}{lcHc}
\toprule
\textbf{Simulator} & \textbf{Year} & \textbf{Category} & \textbf{NMC capabilities} \\ \midrule
Sinuca~\cite{7336224} & 2015 & Cycle-Accurate & Yes \\
HMC-SIM~\cite{7529923} & 2016 & Cycle-Accurate & Limited \\
CasHMC~\cite{7544479} & 2016 & Cycle-Accurate & No \\
SMC~\cite{Azarkhish:2016:DEP:2963802.2963805} & 2016 & Cycle-Accurate & Yes \\
CLAPPS~\cite{junior2017generic} & 2017 & Cycle-Accurate & Yes \\ 
Ramulator-PIM~\cite{ramulator-pim-repo}      & 2019    & Cycle-Accurate & Yes  \\
\bottomrule
\end{tabular}
}
\end{table}



As the field of NMC does not have very sophisticated tools and techniques, researchers often \dd{spend} a significant amount of time building the appropriate evaluation environment~\cite{junior2017generic,NAPEL}. Additionally, there is a critical need for near-memory specific benchmarks of workloads that could benefit from NMC~\cite{oliveira2021pimbench}. Such a benchmark suite can allow researchers to evaluate different architectural proposals and faithfully reproduce results.
%In Table~\ref{tab:simulator} we have mentioned some of the academic efforts to build open-source NMC simulator.% Hyeokjun~et~al.~\cite{DBLP:journals/corr/ChoeLPKCY16} evaluate the potential of NMC for machine learning (ML) using a full-fledged simulator of multi-channel SSD that can execute various ML algorithms on data stored on the SSD. Similarly, Jo~et~al.~\cite{jo2016data} develop the iSSD simulator based on the gem5 simulator~\cite{Binkert:2011:GS:2024716.2024718}. % Ranganathan~et~al.~\cite{chang2012limits, ranganathan2011microprocessors} for their nano-stores architecture use a bottom-up approach where they build an analytic model which breaks applications down into various phases, based on compute, network, and I/O subsystem activities. The model takes input from the low-level performance and power models regarding the performance of each phase. Then they used COTSon~\cite{cotson-osr09} for detailed micro-architectural simulation. 
% \subsection{Application Characterization}
% \label{subse:nmc_review/appchar}

% More than ever, application characterization has taken a crucial role in systems design due to the increasing number of new big data applications. Application characterization is used to extract information using specific metrics to decide for a certain application which architecture could have the best performance and energy efficiency. NMC systems have mostly proven to be effective against memory-intensive applications and are hence tailored towards such workloads. It is critical to analyze the application to quantify computational demand and memory footprint. Application characterization can be done in two way -- microarchitecture-dependent or microarchitecture-independent manner.

% \textbf{1) Microarchitecture-dependent characterization} is done using hardware performance counters. Awan \etal~\cite{awan2017identifying} use hardware performance counters to characterize the scale-out big data processing workloads into CPU-bound, memory-bound, and I/O-bound applications and propose programmable logic near DRAM and NVRAM. However, the use of hardware performance counters is limited by the impact of micro-architecture features like cache size, issue width, etc~\cite{6557175}. To overcome this problem, recently there has been a push towards following an microarchitecture independent characterization approach.

% \textbf{2) Microarchitecture-independent characterization} independent characterization consists of profiling instruction traces to collect inherent application information such as operation mix, memory behavior in a microarchitecture independent way. This approach provides more relevant workload characteristics than performance counters~\cite{4292057}, which can be easily reused for different architectures.

\subsection{Virtual Memory Support}
\label{subsec:nmc_review/virtualmemndp}
To access data inside the main memory, the CPU performs address translation from a data's virtual address to the actual physical address in the main memory. The address translation can be achieved by using the following two mechanisms: \textit{segmentation} or \textit{paging}. Segmentation~\cite{7459501,7459537} consists of a simplified approach where part of the linear virtual address space is mapped to physical memory using a direct segment. However, segmentation requires frequent swapping of segments between the main memory and the storage, leading to fragmentation. Therefore, \dd{the use of a paging mechanism is gaining wider adoption.}

Paging is a memory management mechanism that entails dividing virtual address space into blocks of addresses referred to as pages. A page table stores mapping between virtual to physical address and cache recently used mapping into a translation lookaside buffer (\acrshort{tlb}). A miss in the TLB would lead to a long-latency table walk, which can degrade the application performance. \fc{Several studies have been proposed to improve the efficiency of address translation, such as by speeding up address translation~\cite{barr2011spectlb,papadopoulou2015prediction}, increasing the TLB reach~\cite{ausavarungnirun2017mosaic,cox2017efficient}, and introducing caches to store page table address~\cite{barr2010translation,bhattacharjee2013large,bhargava2008accelerating}. }

In an NMC-based system, if an NMC accelerator requires many page table walks for the host CPU, it would substantially reduce the overall performance. Therefore, we need an effective address translation mechanism for NMC architectures. As an example, Hsieh~\etal~\cite{hsieh2016accelerating} design an NMC-side page table for their NMC accelerator, which avoids the use of CPU-side address translation. Past works adopt either a software-based~\cite{gao2015practical,Sura:2015:DAO:2742854.2742863,tom,Wei05anear-memory} or a hardware-based~\cite{Azarkhish:2016:DEP:2963802.2963805} approach to map between virtual and physical addresses.  

%\subsubsection{Paging}
% %\label{subsubsec:paging} 
% \textbf{(1) Paging} is a memory management mechanism that entails dividing virtual address space into blocks of addresses refer to as pages. A page table stores mapping between virtual to physical address and cache recently used mapping into a translation lookaside buffer (TLB). Paging can be software or hardware-managed. 

% Most NMC systems adopt a software-managed TLB to provide a mapping between virtual and physical addresses~\cite{gao2015practical,Sura:2015:DAO:2742854.2742863,tom,Wei05anear-memory}. Other works such as~\cite{Azarkhish:2016:DEP:2963802.2963805} observe that an OS managed TLB may not be the optimal solution and propose a hardware implementation where a simple controller is responsible for fetching the entry in the page table. Hsieh~\etal~\cite{hsieh2016accelerating}  notice for pointer-chasing applications, the accelerator works only on specific data structures that can be mapped onto a contiguous region of the virtual address space. 

% % As a consequence, the virtual-to-physical translation can be designed to be more compact and efficient. Picorel \etal~\cite{picorel2017near} show that restricting the associativity such that a virtual page can be mapped only with few contiguous physical pages can break the decode-and-fetch serialization. Their translation mechanism, DIPTA, allows removing the virtual-to-physical translation overhead.

% %\subsubsection{Direct Segmentation}
% \label{subsubsec:nmc_review/directsegment} 
%  \textbf{(2) Direct Segmentation}~\cite{7459501,7459537} consists of a simplified approach where part of the linear virtual address is mapped to physical memory using a direct segment rather than a page. This mechanism allows to remove TLB misses overhead and dramatically  simplifies the hardware~\cite{Basu:2013:EVM:2508148.2485943}. Segmentation requires swapping segments between main-memory and the storage, which can lead to fragmentation.


\subsection{Memory Coherency}
\label{subsec:nmc_review/cachecoherencendp}
%Although in some works the cache coherence has not been treated~\cite{7459537,6846276}, we classify the approaches proposed in literature as \textit{restricted memory region} and \textit{non-restricted region}. 
Coherency is one of the most critical challenges in the adoption of NMC. An NMC processing unit could modify the data, which the host CPU might require. Therefore, we need to maintain a coherence protocol between the shared memory. A fine-grain coherence mechanism might lead to a large number of coherence messages between the NMC cores and the host cores.  Therefore, the employed coherence mechanism can drastically affect the performance and the programming model. In NMC, researchers try to overcome this issue by following the \dd{two approaches listed below}.

%\subsubsection{Restricted Memory Regions}
%\label{subsubsec:distmemreg} 
\noindent\textbf{(1) Restricted memory region-based} techniques such as the one used by Farmahini \etal~\cite{7056040} divide the memory into two parts: one for the host processor and another for the accelerator, which is uncacheable. Ahn~\etal~\cite{teserract} use a similar approach for graph processing algorithms. 
Another strategy proposed by Ahn~\etal\cite{ahn2015pim} provides a simple hardware-based solution in which the NMC operations are restricted to only one last-level cache block, due to which they can monitor the cache block and request for invalidation or write-back if required.

%\subsubsection{Non-Restricted Memory Regions}
%\label{subsubsec:notdistmemreg} 
\noindent\textbf{(2) Non-restricted memory region-based} techniques allow NMC units to access the entire memory space.  Pattnaik~\etal\cite{7756764} propose maintaining coherence between the host GPU and near-memory compute units by flushing the L2 cache in the host GPU after kernel execution. However, this approach could evict potentially useful data from the cache. Another way is to implement a look-up table-based mechanism, as Hsieh~\etal~\cite{tom}. The NMC units record the cache line address that the offloaded block has updated, and once the offloaded block is processed, the NMC units send this address back to the host system. Subsequently, the host system gets the latest data from memory by invalidating the reported cache lines. %Liu~\etal~\cite{liu2018processing} propose a single global memory with a relaxed consistency model, shared between the NMC unit and the CPU. They implement explicit synchronization points to synchronize the accesses to shared variables across NMC unit and the CPU.
More recently, Boroumand~\etal\cite{boroumand2019conda} overcome the coherence issue with a specialized coherence protocol that batches and compresses multiple coherence requests from NMC units. As a result of this, the authors can achieve a near-ideal coherence mechanism.
 
 

\subsection{Task Scheduling}
\label{subsec:nmc_review/programmingmodel}

A critical challenge in adopting NMC is to support a heterogeneous processing environment comprising a host system and NMC processing units. It is not trivial to determine which part of an application should run on the NMC processing units. Works such as~\cite{Hadidi:2017:CCT:3154814.3155287, tom} leave this effort on the compiler, while others~\cite{ghose2018enabling, xi2015beyond, ahn2015pim} assume the programmer would manage the scheduling of tasks. Another approach~\cite{ahn2015pim, lee2018application, nai2017graphpim} uses some special set of NMC instructions, which invokes NMC processing units. This approach, however, calls for a sophisticated mechanism as it affects most of the software stack from the application down to the instruction set architecture. 

To this end, a run-time system capable of dynamically profiling applications to identify the potential offloads candidates for NMC processing units~\cite{liu2018processing, tom} can significantly help with task scheduling. Therefore, there is still a lot of research required in coming up with an efficient approach to ease the programming burden.

\begin{comment}

{\footnotesize
\begin{table*}[h]
    \centering
\begin{tabular}{l|*{2}{l}r}
\hline
\textbf{Metrics}   & \textbf{Description} \\
\hline
Reuse Distance (Temporal Locality) &The number of distinct memory accesses since the last access to a given memory address \\\hline
Data Stream Stride (Spatial Locality)&The difference in memory addresses
between two consecutive memory accesses\\\hline
Application Bandwidth &The amount of I/O bandwidth utilized by a particular application\\\hline
Instruction Mix &Provides a general overview of the application\\\hline
Parallelism &Inherent application parallelism such as instruction level parallelism, thread level parallelism, data level parallelism\\\hline
Branch Entropy&Measures the randomness of branch behavior which is essential to provide speculation support\\
\hline
\end{tabular}

    \caption{Several metrics for microarchitecture independent analysis of workloads}
    \label{tab:analysisMetrics}

\end{table*}

}

\end{comment}
\iffalse
\begin{table}[ht]
\renewcommand{\arraystretch}{1.3}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l}
\hline
\multicolumn{1}{c|}{\textbf{Metrics}} & \multicolumn{1}{c}{\textbf{Description}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Reuse Distance \\ (Temporal Locality)\end{tabular} & \begin{tabular}[c]{@{}l@{}}The number of distinct memory accesses since the \\ last access to a given memory address.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Data Stream Stride \\ (Spatial Locality)\end{tabular} & \begin{tabular}[c]{@{}l@{}}The difference in memory addresses between two \\ consecutive memory accesses.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Application \\ Bandwidth\end{tabular} & \begin{tabular}[c]{@{}l@{}}The amount of I/O bandwidth utilized by a \\ particular application.\end{tabular} \\ \hline
Instruction Mix & Provides a general overview of the application. \\ \hline
Parallelism & \begin{tabular}[c]{@{}l@{}}Inherent application parallelism such as instruction \\ level parallelism, thread level parallelism, \\ data level parallelism.\end{tabular} \\ \hline
Branch Entropy & \begin{tabular}[c]{@{}l@{}}Measures the randomness of branch behavior which \\ is essential to provide speculation support.\end{tabular} \\ \hline
\end{tabular}
}
\caption{Several metrics for microarchitecture independent analysis of workloads}
\label{tab:analysisMetrics}
\end{table}
\fi

\subsection{Data Mapping}
\label{subsec:nmc_review/datamappNDPaPIM}
\fc{The problem of data mapping and data layout have been analyzed in various contexts to improve the spatial locality of a workload~\cite{wolf1991data,mckinley1996improving,chandra1994scheduling,kelm2010waypoint}. }The absence of an adequate data mapping mechanism can severely hamper the benefits of processing close to memory. A data mapping scheme should map data in such a way that the data required by the NMC processing units is readily available in the vicinity (data and code co-location). Hence, it is crucial to look into effective data mapping schemes. Hsieh~\etal~\cite{tom} propose a hardware/software co-design method to predict which pages of the memory would be used by the offloaded code segment, following which they place those pages in the memory stack closest to the offloaded code segment. 

Yitbarek~\etal~\cite{7459537} propose a data mapping scheme to place contiguous addresses in the same vault of an HMC-based memory allowing accelerators to access data directly from their local vault. Xiao~\etal~\cite{xiao2018prometheus} propose to model an application as a two-layer graph through the \acrshort{llvm}-intermediate representation (LLVM-IR), to distinguish between memory and computation operations. On building one such graph, their framework detects groups of vertices, called \textit{community}, that have a higher probability of connection with each other. Each community is mapped to a different vault of an HMC-based memory. Thus, \dd{this technique allows multiple} NMC units to perform computation in parallel on multiple data elements.






% \section{Design Space Exploration for NMC}
% \label{sec:modelingmethod}


% As will be clear from the previous classification section, the design space of NMC is huge. To understand and evaluate this space, effective design space exploration (DSE) for NMC systems is required.
%Moreover, these architectures calls for specialized hardware software co-design strategies as shown in Figure~\ref{fig:nmc_review/methodology}.
% \begin{figure}[h]
% \centering
% \includegraphics[width=.6\linewidth]{NMC_review/img/Methodology_paper_final.png}
% \caption{Design space exploration highlighting application characteristic with performance evaluation technique
% \label{fig:nmc_review//methodology}}
% \end{figure}




\iffalse
Table~\ref{tab:metricsprevious}, highlights metrics used to decide the profitability of NMC acceleration.

\begin{table}[h]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \scalebox{0.93}{
    \begin{tabular}{l|l}
    \hline
     \textbf{Architecture or first author's name} & \textbf{Metrics}\\
     \hline
     TOP-PIM~\cite{zhang2014top} DNN-PIM~\cite{liu2018processing} & Memory Bandwidth   \\
     IMPICA~\cite{hsieh2016accelerating} & CPI \\
     \hline
     Vermij~\cite{vermij2017sorting} & Reuse distance \\
     \hline
     Cairo~\cite{Hadidi:2017:CCT:3154814.3155287} Awan~\cite{awan2017identifying,awan2017performance} & Last-level cache misses  \\
     Gokhale~\cite{gokhale2015near} PIM-enable~\cite{ahn2015pim}\\
     \hline
     TOM~\cite{tom} & Memory bandwidth  \\
     \hline
     Pattnaick~\cite{7756764} & Memory intensity \\
     & Available Parallelism  \\
     & Shared memory intensity  \\
     \hline
     PISA-NMC~\cite{corda2019scopes,corda2019DSD} & Spatial Locality \\
      & Memory Entropy \\
      & Parallelism \\
     \hline
     ProPRAM~\cite{wang2015propram} & Huge data volumes \\
     BlueDBM~\cite{Jun:2015:BAB:2872887.2750412} & High parallelism \\
     BISCUIT~\cite{gu2016biscuit} & \\
     \hline
     HMC~\cite{nair2015active} HRL~\cite{7446059} HRL~\cite{7446059} NDA~\cite{7056040} & Not Mentioned Explicitly \\
     Pugsley~\cite{6844483} AMC~\cite{nair2015active} \\
     TESSERACT~\cite{7284059} MCN~\cite{alian2018application} \\
     JAFAR~\cite{xi2015beyond} CARIBOU~\cite{istvan2017caribou} \\
     WILLOW~\cite{seshadri2014willow} XSD~\cite{cho2013xsd}
    \end{tabular}}
     \caption{Application metrics used for NMC profitability}
     \label{tab:metricsprevious}
\end{table}
\fi


% \section{An Analytic Model for NMC}
% \label{sec:nmc_review/analyticmodel}
% We make use of a first-order analytical model to demonstrate the benefits of using NMC. As mentioned in Section~\ref{sec:nmc_review/challenges}, a high-level analytic model abstract the detailed micro-architecture. Hence, this approach makes our analytical model more generic and provides quick insights. 

% To evaluate the potential of computing close to the memory and when it is useful to follow a data-centric approach, we make a comparison to a compute-centric approach consisting of a multi-core system. For multi-core system we follow the analytical approach by Nguyen~\etal~\cite{anh_model_2019}. We assume number of cores $N_{cores}$=4 each with a frequency of 3 GHz. Each core consists of a two level cache (L1 of 32-KB and L2 of 256-KB) with access latencies of one and two cycles~\cite{6175879}. The actual miss rates are depend on the target application. We assume a DRAM of size 4GB with access latency of 175 cycles~\cite{6175879} with the page fault rate of 0.1\% with a penalty of 800 cycles~\cite{}.


% Our data-centric approach has a host CPU connected NMC processing units close to a 3D stacked main-memory similar to HMC (\textit{ref.} Figure~\ref{fig:nmc_review/HMCLayout}). The host is modeled similar to that in compute-centric approach. We assume certain parts of the computation called NMC-kernels would be offloaded to the NMC processing units, and the other parts will be executed in the host CPU. %The number of vaults inside the HMC and external interconnects links are kept as varying parameters which have an impact on internal and the external bandwidth of the 3D memory respectively.  
% Table~\ref{tab:NMC_review/systemparameters} provides our system parameters. The model estimates the data transfer time as the ratio between the number of memory accesses required to move the block of data to and from a memory  and the available memory bandwidth that memory. The execution time takes into account the time to process the instructions and latency due to memory access. We make L1 and L2 miss rate are variable parameters. 






% \begin{table}[h]
% \renewcommand{\arraystretch}{1}
% \centering
% \begin{tabular}{l*{3}{c}r}
% \hline
% \textbf{Description}              & \textbf{Symbol} & \textbf{ARM} \\
% \hline
% \# Cores & N\textsubscript{cores} & 4  \\
% Host core frequency & F\textsubscript{core} & 3 GHz   \\
% NMC core frequency & F\textsubscript{core} & 1.2 GHz   \\
% L1 size           & S\textsubscript{l1} & 32 KB  \\
% L2 size     & S\textsubscript{l2} & 256 KB  \\
% DRAM size & S\textsubscript{DRAM} & 4 GB \\
% L1 cache bandwidth & BW\textsubscript{l1} & 137 GB/s\\
% L2 cache bandwidth & BW\textsubscript{l2} & 137 GB/s\\
% L1 cache hit latency & L\textsubscript{l1} & 1 cycles\\
% L2 cache hit latency & L\textsubscript{l2} & 2 cycles\\
% \hline
% \end{tabular}
% \caption{System parameters}
% \label{tab:NMC_review/systemparameters}
% \end{table}



% % \begin{comment}

% % \begin{equation}
% % \label{eq:1}
% % \begin{split}
% % n_{load}=n_r/n_{vaults}
% % \end{split}    
% % \end{equation}
% % \begin{equation}
% % \label{eq:2}
% % \begin{split}
% % n_{store}=n_w/n_{vaults}
% % \end{split}    
% % \end{equation}
% % \begin{equation}
% % \label{eq:3}
% % \begin{split}
% % m_{total}= n_{load}+n_{store}
% % \end{split}    
% % \end{equation}
% % \begin{equation}
% % \label{eq:4}
% % \begin{split}
% % \Pi_{memory}=\frac{1}{n_{pe}} \displaystyle \sum_{}^{N_{vaults}}\frac{m_{total}*b_{rb}}{BW_{int}}
% % \end{split}    
% % \end{equation}

% % \end{comment}


% % %\todo[author=Gagan, inline]{Add performance model equations here}



% \textit{Energy Calculation:} We build a power model for both CPU-centric and a near-memory system by taking into account dynamic as well as static energy. Dynamic energy is the product of the energy per memory access and the number of memory accesses at each level of the memory hierarchy.  It is assumed to scale linearly with utilization. Static energy is estimated as the product of time and static power for each component. It is scaled based on the number of cores and the cache size. 
    
% For modeling the HMC, we refer to~\cite{6242474} and~\cite{6844483}. We consider energy per bit of 3.7 pJ/b for accessing the DRAM layers and 1.5 pJ/b for the operations and data movements in the HMC logic layer. A static power of 0.96 W is assumed~\cite{6844483} to model the additional components in the logic layer.

% %\todo[author=Gagan, inline]{Add energy model equations here}


% \textit{Performance and Energy Exploration:} 
% In Figure~\ref{fig:NMC_review/results}, we show the results for delay and energy for NMC-based system and compare it to a traditional multi-core system. The x and y-axis represent the miss rate at L1 and L2, respectively. The results are normalized to NMC+host system. 
% We vary the cache miss rate, which encapsulates application characteristics, both at L1 and L2 level to see the impact it has on the performance of the entire system. In case of a near-memory system, we consider the scenario when all accesses are done to the different vaults inside the HMC memory, which can exploit the inherent parallelism offered by the 3D memory. 

% \begin{figure*}[h]
% \captionsetup[subfigure]{justification=centering}
% \centering
% \begin{subfigure}[t]{0.5\textwidth}
%   \includegraphics[width=0.95\linewidth,trim={0.5cm 0.5cm 0cm 0cm},clip]{NMC_review/img/delay3_final.png}
%   \caption{Normalized Delay
%   \label{fig:NMC_review/delay}}
% \end{subfigure}%
% \begin{subfigure}[t]{0.5\textwidth}
%   \includegraphics[width=0.95\linewidth,trim={0cm 0cm 0cm 0cm},clip]{NMC_review/img/energy3_final.png}
%   \caption{Normalized Energy
%   \label{fig:NMC_review/energy}}
% \end{subfigure}
% \caption{Delay and energy consumption comparison between a multi-core-based system and an NMC-based system with a host CPU using a high-level analytical model}
% \label{fig:NMC_review/results}
% \end{figure*}

% Based on our evaluation, we make the following three observations. First, in case of performance and energy, we can see a similar trend, i.e., if the miss rate (L1 and L2) increases the multi-core system performance degrades compared to the NMC systems. This degradation is because of the increase in data movement. The data has to be fetched from the off-chip DRAM. Second, if the CPU does not reuse the data brought into the caches, the use of caching becomes inefficient. Third, the application (or function) with low locality can take advantage of the near-memory approach, whereas the other application (or function) with high locality would benefit more from the traditional approach. We conclude that near-memory computing has the potential to overcome the data movement bottleneck for modern data-intensive applications.

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/classification.tex <==
\section{Classification and Evaluation}
\label{sec:nmc_review/classificationmodel}

Figure~\ref{fig:nmc_review/taxonomy} shows a high-level view of our classification based on the level in the memory hierarchy. We further split our classification into the type of processing unit (programmable, fixed-function, or reconfigurable). Conceptually the approach  of near-memory computing can be applied to any level or type of memory to improve the overall system performance. %Our taxonomy does not include magnetic disk-based systems as they can no longer offer timely response due to the high access latency and a high failure rate of disks~\cite{7097722}.
\dd{Our taxonomy does not include magnetic disk-based systems because nowadays, it is only used as a long-term \emph{cold data} storage medium, i.e., for long-term and rarely accessed data~\cite{fuji_tape}. }
Nevertheless, there have been various research efforts towards providing processing capabilities in the disk. However, the industry did not adopt it widely due to the marginal performance improvement that could not justify the associated cost~\cite{Keeton:1998:CID:290593.290602,Riedel:1998:ASL:645924.671345}. Instead, we include emerging non-volatile memories termed  storage class memory (\acrshort{scm})~\cite{7151782}, which are trying to fill the latency gap between DRAM and disk. %Building upon similar efforts~\cite{siegl2016data, ghose2018enabling},

\begin{figure}[h]
\centering
  \hbox{\hspace{7em} \includegraphics[width=0.7\linewidth]{NMC_review/img/NMCtaxonomy.2021_03.eps}}
\caption{Processing options in the memory hierarchy highlighting three computation paradigms: (1) Compute-centric approach where data is moved through various levels of memory to the processor for computing; (2) Near-memory computing approach where the processing elements are placed closer to memory; and (3) Computation-in memory approach that uses inherent properties of memory to perform computation
\label{fig:nmc_review/taxonomy}}
\end{figure}


This section introduces the classification and evaluation metrics (see Table~\ref{tab:nmc_review/arcLegend}) used to analyze various architectures in Appendix~\ref{sec:nmc_review/procmainmem} and Appendix~\ref{sec:nmc_review/procstorage}. We summarize different architectures in Table~\ref{tab:nmc_review/arcLegend}. 
% \linebreak

For each architecture, we evaluate and classify across five main categories:
\begin{itemize}
%  \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
 \setlength{\topsep}{-3pt}
\setlength{\itemsep}{2pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item{\textbf{Memory}} - The type of memory technology is one of the most fundamental questions on which the near-memory architecture depends.
\item{\textbf{Processing}} - The type of processing unit and the granularity of processing it performs plays a critical role in our analysis.
\item{\textbf{Tool}} - Any system's success depends heavily on the available tool support. The effectiveness of the tool infrastructure indicates the maturity of the architecture. 
\item{\textbf{Interoperability}} - \ggthesis{It is the integration of NMC processing units into the overall computer system architecture. }Interoperability deals with aspects such as virtual memory support, memory coherence,  efficient task scheduling, and data mapping. Interoperability is one of the key enablers for the adoption of any new system.
\item{\textbf{Application}} - NMC follows a data-centric principle and is usually specialized for a particular workload or a set of workloads. Therefore, in our evaluation, we include the domain of the application.  
\end{itemize}

\input{NMC_review/tables/classification}

% \input{NMC_review/tables/architectures.tex}
\subsection*{Discussion}

Based on the above classification, we highlight some of the notable architectures in the domain of near-memory computing. All solutions discussed in this section are summarized in Table~\ref{tab:nmc_review/arcClassification} and described in Appendix~\ref{chapter:appendixA}.  From Table~\ref{tab:nmc_review/arcClassification}, we make the following five observations. 
\input{NMC_review/tables/architectures.tex}
% \noindent From Table~\ref{tab:nmc_review/arcClassification}, we make the following five observations. 

First, the efficacy of architectural proposals has mostly been tested using simulators. A few works emulate~\cite{gu2016biscuit, awan2017performance, koo2017summarizer, istvan2017caribou,kang2013enabling,seshadri2014willow} their proposal on an FPGA. Recently, HBM~\cite{hbm} has been adopted by GPU and FPGA vendors. In the future, we expect more evaluation studies on these  HBM-equipped platforms and upcoming platforms with NMC capabilities, such as  FIMDRAM~\cite{fimdram2021ISCA} and UPMEM~\cite{gomezluna2021upmem}. 

Second, the majority of research papers published over the years have proposed homogeneous processing units near the main memory. However, the logic considered varies in its compute capabilities, e.g., simple in-order cores~\cite{torabzadehkashi2018compstor,lee2018application,alian2018application,de2017mondrian,koo2017summarizer,7927081,teserract,nair2015active,6844483}, graphics processing units~\cite{zhang2014top,7756764,tom,cho2013xsd}, field-programmable gate arrays~\cite{7446059, jun2015bluedbm,istvan2017caribou}, and application-specific accelerators~\cite{xi2015beyond,gokhale2015near,ahn2015pim,hsieh2016accelerating,gu2016biscuit,vermij2017sorting,nai2017graphpim,liu2018processing,fernandez2020natsa,ke2020recnmp}. 

Third, the majority of the NMC proposals are targeted towards data-intensive applications e.g., graph processing~\cite{zhang2014top,teserract,nai2017graphpim}, MapReduce~\cite{cho2013xsd,6844483,7056040}, machine learning~\cite{liu2018processing,lee2018application}, and database~\cite{kang2013enabling,xi2015beyond,gu2016biscuit,istvan2017caribou,7927081,koo2017summarizer}.  

Fourth, most of the architectures propose adding compute capabilities in the logic layer of HMC-based memory~\cite{ke2020recnmp,cali2020genasm,fernandez2020natsa,googleWorkloads,liu2018processing,lee2018application,de2017mondrian,vermij2017sorting,7756764,tom,hsieh2016accelerating,ahn2015pim,7446059,gokhale2015near,teserract,nair2015active,zhang2014top,6844483,fimdram2021ISCA}. However, memory vendors such as Micron have announced to pursue HBM instead of focusing on HMC~\cite{noHMC}. Fifth, despite the promises made by existing proposals on NMC, the support for virtual memory, memory coherence, and compiler support is fairly limited. In most of the works~\cite{torabzadehkashi2018compstor, lee2018application, nai2017graphpim, de2017mondrian, koo2017summarizer,vermij2017sorting,istvan2017caribou,gu2016biscuit}, the programmers are expected to re-write their code using specialized \acrshort{api}s in order to reap the benefits of NMC. 

Based on the above observations, we make the following three conclusions. 

\begin{enumerate}[topsep=0pt,itemsep=0ex,partopsep=1ex,parsep=1ex]
    \item HBM-equipped specialized hardware has the potential to reduce the memory bandwidth bottleneck, but a study of their advantages for a real-world data-intensive application is still missing.  

\item The idea of populating homogeneous processing units near-memory to accelerate a specific class of workloads is limited in the sense that NMC enabled servers that would be deployed in the data centers are expected to host a wide variety of workloads. Hence, these systems would need heterogeneous processing units near the memory~\cite{googleWorkloads,liu2018processing,7446059} to support the complex mix of data center workloads. 

\item For broader adoption of the NMC by the application programmers, we would require methods that enable transparent offloading to the NMC units. Transparent offloading requires the compiler or the run-time system to identify NMC-suitable code regions based on some application characteristics, such as the number of last-level cache misses~\cite{Hadidi:2017:CCT:3154814.3155287, awan2017identifying,awan2017performance, gokhale2015near, ahn2015pim} and bandwidth utilization~\cite{zhang2014top, liu2018processing, hsieh2016accelerating}. Unfortunately, integrating a profiler (such as Linux perf~\cite{perf} or Intel Pin~\cite{reddi2004pin}) in a compiler or run-time system is still a challenging task~\cite{Hadidi:2017:CCT:3154814.3155287} due to its dynamic nature. Therefore, current solutions rely on commercial profiling tools, such as Intel VTune~\cite{Vtune}, to detect the offloading kernels~\cite{awan2017performance, awan2017identifying, hsieh2016accelerating}.
\end{enumerate}

% First, the efficacy of architectural proposals have mostly been tested using simulators. Only a few works emulate~\cite{gu2016biscuit, awan2017performance, koo2017summarizer, istvan2017caribou,kang2013enabling,seshadri2014willow} their proposal on an FPGA. Recently, HBM~\cite{hbm} has been adopted by GPU and FPGA vendors. In the future, we expect more evaluation studies on these upcoming HBM-equipped platforms. UPMEM~\cite{gomezluna2021upmem} is another state-of-the-art platform with NMC capabilities. Second, the majority of research papers published over the years have proposed homogeneous processing units near the main-memory. However, the logic considered varies in its compute capabilities, e.g., simple in-order cores~\cite{torabzadehkashi2018compstor,lee2018application,alian2018application,de2017mondrian,koo2017summarizer,7927081,teserract,nair2015active,6844483}, graphics processing units~\cite{zhang2014top,7756764,tom,cho2013xsd}, field-programmable gate arrays~\cite{7446059, Jun:2015:BAB:2872887.2750412,istvan2017caribou}, and application-specific accelerators~\cite{xi2015beyond,gokhale2015near,ahn2015pim,hsieh2016accelerating,gu2016biscuit,vermij2017sorting,nai2017graphpim,liu2018processing,fernandez2020natsa,ke2020recnmp}. Third, the majority of the NMC proposals are targeted towards data-intensive applications e.g., graph processing~\cite{zhang2014top,teserract,nai2017graphpim}, MapReduce~\cite{cho2013xsd,6844483,7056040}, machine learning~\cite{liu2018processing,lee2018application}, and database~\cite{kang2013enabling,xi2015beyond,gu2016biscuit,istvan2017caribou,7927081,koo2017summarizer}.  

% Fourth, most of the architectures propose adding compute capabilities in the logic layer of HMC-based memory~\cite{ke2020recnmp,cali2020genasm,fernandez2020natsa,googleWorkloads,liu2018processing,lee2018application,de2017mondrian,vermij2017sorting,7756764,tom,hsieh2016accelerating,ahn2015pim,7446059,gokhale2015near,teserract,nair2015active,zhang2014top,6844483}. However, memory vendors such as Micron have announced to pursue HBM instead of focusing on HMC~\cite{noHMC}. Fifth, despite the promises made by existing proposals on NMC, the support for virtual memory, memory coherence, and compiler support is fairly limited. In most of the works~\cite{torabzadehkashi2018compstor, lee2018application, nai2017graphpim, de2017mondrian, koo2017summarizer,vermij2017sorting,istvan2017caribou,gu2016biscuit}, the programmers are expected to re-write their code using specialized \acrshort{api}s in order to reap the benefits of NMC. 

% Based on the above observations, we make the following three conclusions. First, HBM-equipped specialized hardware has the potential to reduce the memory bandwidth bottleneck, but a study of their advantages for a real-world data-intensive application is still missing.  Second, the idea of populating homogeneous processing units near-memory to accelerate a specific class of workloads is limited in the sense that NMC enabled servers that would be deployed in the data centers are expected to host a wide variety of workloads. Hence, these systems would need heterogeneous processing units near the memory~\cite{googleWorkloads,liu2018processing,7446059} to support the complex mix of data center workloads. 

% Third, for broader adoption of the NMC by the application programmers, we would require methods that enable transparent offloading to the NMC units. Transparent offloading requires the compiler or the run-time system to identify NMC-suitable code regions based on some application characteristics, such as number of last-level cache misses~\cite{Hadidi:2017:CCT:3154814.3155287, awan2017identifying,awan2017performance, gokhale2015near, ahn2015pim} and bandwidth utilization~\cite{zhang2014top, liu2018processing, hsieh2016accelerating}. Unfortunately, integrating profiler (such as Linux perf~\cite{perf} or Intel Pin~\cite{reddi2004pin}) in a compiler or run-time system is still a challenging task~\cite{Hadidi:2017:CCT:3154814.3155287} due to its dynamic nature. Therefore, current solutions rely on commercial profiling tools, such as Intel VTune~\cite{Vtune}, to detect the offloading kernels~\cite{awan2017performance, awan2017identifying, hsieh2016accelerating}.


==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:nmc_review/concludes}
%Modern system designers are moving away from the conventional compute-centric approach towards a more data-centric approach. 
Data-centric computing aims to reduce the data movement overhead by implementing processing capabilities close to where the data resides. With ``close'' being a relative term, there is a wide range of possibilities to bring computation closer to the data, resulting in various architectures being investigated today. Data-centric computing is attributed as one of the few real solutions to address the current scaling issues in HPC systems to realize exascale computers needed for modern and future data-intensive workloads.  There are two different approaches to enable data-centric computing. First, near-memory computing (NMC), which adds processing capabilities closer to the existing memory architectures. Second, computation-in memory (CIM), which  exploits the memory architecture and intrinsic properties of emerging technologies to perform operations using memory itself. \dd{This thesis focuses on} NMC-based architectures and techniques to overcome the data movement bottleneck.

This chapter analyzes NMC-based architectures across various dimensions and highlights that NMC is still in its infancy. We need to address multiple architectural challenges before NMC can be established as an essential component of HPC systems to accelerate data-intensive workloads. Besides designing and evaluating NMC processing capabilities for data-intensive workloads,  we stress the demand for sophisticated tools and techniques to enable the design space exploration for these novel architectures. Further, we need to solve various challenges related to the overall system integration. %Further, we need to solve challenges related to the integration of NMC units into the overall computer system architecture. 
\ou{To overcome these challenges, we should consider data as a paramount resource and
provide various mechanisms to handle and leverage the vast amount of data. In this dissertation, we tackle the above challenges in three different ways.
%First, we overcome the data movement bottleneck of memory bound real-world stencil workloads by following a data-centric computing approach.
First, we demonstrate NMC processing capabilities for a real-world data-intensive weather prediction application. Second, we provide data-driven machine learning-based solutions that allow quick and accurate performance estimation during the design-time. Third, we leverage the vast amount of available data to drive run-time system-level decisions.  }



% Besides designing and evaluating NMC processing capabilities for modern data-intensive workloads,  we stress the demand for sophisticated tools and techniques to enable the design space exploration for these novel architectures. Further, we need to solve challenges related to the integration of NMC units into the overall computer system architecture.

% The decline in performance and energy consumption for emerging big-data workloads on the conventional systems has stimulated an enormous amount of research in processing close to memory. However, to embrace this paradigm, we need to provide a complete ecosystem from hardware to software stack. We have analyzed and organized the extensive literature of placing compute units close to the memory using different synonyms (e.g., \textit{processing-in memory}, \textit{near-data processing}) under the umbrella of \textit{near-memory computing} (NMC). This organization allows us to distinguish NMC from the in-situ \textit{computation-in-memory} through novel non-volatile memories such as memristors and phase-change memory. By systematically reviewing the existing NMC systems, we have identified key challenges that we need to address for enabling the adoption of NMC-based systems. We stress the demand for sophisticated tools and techniques to enable the design space exploration for these novel architectures. %Also, we have described our approach to address a subset of those challenges.

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/future.tex <==
\section{Open Issues and Future Directions}
\label{sec:futuredirections}
Based on our analysis of many existing NMC architectures, we identify the following key
topics for future research that we regard as essential to unlock the full potential of processing close to memory:
\begin{itemize}
   
\item It is unclear which emerging memory technology best supports near-memory architectures; for example, much research is going into new 3D stacked DRAM and non-volatile memories such as PCM, ReRAM, and MRAM. The future of these new technologies relies heavily on advancements in endurance, reliability, cost, and density.

\item 3D stacking also needs unique power and thermal solutions, as traditional heat sink technology would not suffice if we want to add more computation close to the memory. Most of the proposed architectures do not take into account the strict power budget of 3D stacked memories, which limits the architecture's practicality.

\item DRAM and NVM have different memory attributes. A hybrid design can revolutionize our current systems. Huang et al.~\cite{qian2015study} evaluated a 3D heterogeneous storage structure that tightly integrates CPU, DRAM, and a flash-based NVM to meet the memory needs of big data applications, i.e., larger capacity, smaller delay, and wider bandwidth. Processing near heterogeneous memories is a new research topic with high potential (could provide the best of both worlds), and in the future, we expect much interest in this direction.

\item Most of the evaluated architectures focus on the compute aspect. Few architectures focus on providing coherency and virtual memory support. As highlighted in Section~\ref{sec:interondpcachevirtual}, lack of coherency and virtual support makes programming difficult and obstructs the adoption of this paradigm. 

\item More quantitative exploration is required for interconnect networks between the near-memory compute units and also between the host and near-memory compute system. The interplay of NMC units with the emerging interconnect standards like GenZ~\cite{genZdram}, CXL~\cite{cxlwhitepaper}, CCIX~\cite{ccixwhitepaper} and OpenCAPI~\cite{stuecheli2018ibm} could be vital in improving the performance and energy efficiency of big data workloads running on NMC enabled servers.

\item At the application level, algorithms need to provide code and data co-location for energy efficient processing. For example, in case of HMC algorithms should avoid excessive movement of data between vaults and across different memory modules. Whenever it is not possible to avoid an inter-vault data transfer, lightweight mechanisms for data migration should be provided.

\item The field requires a generic set of open-source tools and techniques for these novel systems, as often researchers have to spend a significant amount of time and effort in building the needed simulation environment. Application characterization tools should add support for static and dynamic decision support for offloading processing and data to near-memory systems. To assist in the offloading decision, new metrics are required that could assess whether an application is suitable for these architectures. These tools could provide region-of-interest (or hotspots) in an application that should be offloaded to an NMC system. Besides, a standard benchmark set is missing to gauge different architectural proposals in this domain.


\end{itemize}

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/introduction.tex <==
Over the years, memory technology has not been able to keep up with advancements in processor technology in terms of latency and energy consumption, which is referred to as the \textit{memory wall}~\cite{Wulf1995}. Earlier, system architects tried to bridge this gap by introducing memory hierarchies that mitigated some of the disadvantages of off-chip DRAMs. However, the limited number of pins on the memory package is not able to meet today's bandwidth demands of multicore processors. Furthermore, with the demise of Dennard scaling~\cite{1050511}, slowing of Moore's law, and dark silicon computer performance has reached a plateau~\cite{6175879}. 

At the same time, we are witnessing an enormous amount of data being generated across multiple areas like radio astronomy, material science, chemistry, health sciences etc~\cite{nair2015active}. In radio astronomy, for example, the first phase of the Square Kilometre Array (SKA) aims at processing over 100 terabytes of raw data samples per second, yielding of the order of 300 petabytes of SKA data products annually~\cite{6898703}. The SKA currently is in the design phase with anticipated construction in South Africa and Australia in the first half of the coming decade. These radio-astronomy applications usually exhibit massive data parallelism and low operational intensity with a limited locality. On traditional systems, these applications cause frequent data movement between the memory subsystem and the processor that has a severe impact on performance and energy efficiency. Likewise, cluster computing frameworks like Apache Spark that enable distributed in-memory processing of batch and streaming data also exhibit those mentioned above behaviour~\cite{awan2016micro,javed2015performance,awan2016node}. Therefore, a lot of current research is being focused on coming up with innovative manufacturing technologies and architectures to overcome these problems. 

Today's memory hierarchy usually consists of multiple levels of cache, the main memory, and storage. The traditional approach is to move data up to caches from the storage and then process it. In contrast, near-memory computing (NMC) aims at processing close to where the data resides. This data-centric approach couples compute units close to the data and seek to minimize the expensive data movements. Notably, three-dimensional stacking is touted as the true enabler of processing close to the memory. It allows the stacking of logic and memory together using through-silicon via's (TSVs) that helps in reducing memory access latency, power consumption and provides much higher bandwidth~\cite{6242474}. Micron's Hybrid Memory Cube (HMC)~\cite{7477494}, High Bandwidth Memory (HBM)~\cite{6757501} from AMD and Hynix, and Samsung's Wide I/O~\cite{6025219} are the competing products in the 3D memory arena. 

\begin{figure*}[t]
\centering
\includegraphics[bb=1 6 730 238,width=1\textwidth]{NMC_review/img/allsystems_final.pdf}
\caption{Classification of computing systems based on working set location, which is referred to as a working set~\cite{7092668}. Prior systems were based on a CPU-centric approach where data is moved to the core for processing (Figure 1 (a)-(c)), whereas now with near-memory processing (Figure 1 (d)) the processing cores are brought to the place where data resides. Computation-in-memory (Figure 1 (e)) further reduces data movement by using memories with compute capability (e.g. memristors, phase change memory).
\label{fig:nmc_review/allsystems}}
\end{figure*}


\begin{figure}[!hb]
\centering
\includegraphics[width=0.6\linewidth]{NMC_review/img/NMCtaxonomy_final.pdf}
\caption{Processing options in the memory hierarchy highlighting the conventional compute-centric and the modern data-centric approach
\label{fig:nmc_review/taxonomy}}
\end{figure}

Figure~\ref{fig:nmc_review/allsystems} depicts the system evolution based on the information referenced by a program during execution, which is referred to as a working set~\cite{7092668}. Prior systems were based on a CPU-centric approach where data is moved to the core for processing (Figure 1 (a)-(c)), whereas now with near-memory processing (Figure 1 (d)) the processing cores are brought to the place where data resides. Computation-in-memory (Figure 1 (e)) paradigm aims at reducing data movement completely by using memories with compute capability (e.g. memristors, phase-change memory (PCM)).

The paper aims to analyze and organize the extensive body of literature related to the novel area of near-memory computing. Figure~\ref{fig:nmc_review/taxonomy} shows a high-level view of our classification that is based on the level in the memory hierarchy and further split into the type of compute implementation (programmable, fixed-function, or reconfigurable). Conceptually the approach  of near-memory computing can be applied to any level or type of memory to improve the overall system performance. In our taxonomy, we do not include magnetic disk-based systems as they can no longer offer timely response due to the high access latency and a high failure rate of disks~\cite{7097722}. Nevertheless, there have been research efforts towards providing processing capabilities in the disk. However, it was not adopted widely by the industry due to the marginal performance improvement that could not justify the associated cost~\cite{Keeton:1998:CID:290593.290602,Riedel:1998:ASL:645924.671345}. Instead, we include emerging non-volatile memories termed as storage-class memories (SCM)~\cite{7151782} which are trying to fill the latency gap between DRAMs and disks. Building upon similar efforts~\cite{siegl2016data, ghose2018enabling}, we make the following contributions:


\begin{itemize}
    \item We analyze and organize the body of literature on near-memory computing under various dimensions.
    \item We provide guidelines for design space exploration.
    \item We present our near-memory system outlining application characterization and compiler framework. Also, we include an analytic model to illustrate the potential of near-memory computing for memory intensive application with a comparison to the current CPU-centric approach.
    \item We outline the directions for future research and highlight current challenges.
\end{itemize}

This work extends our previous work~\cite{629e227db47e4e89b539b0e072ecce08} by including our approach to near-memory computing (Section~\ref{sec:nmc_review/system}).  This outlines our application characterization and compilation framework. 
Furthermore, we evaluate more recent work in the NMC domain and provide new insights and research directions. The remainder of this article is structured as follows: Section~\ref{sec:nmc_review/background} provides a historical overview of near-memory computing and related work. Section~\ref{sec:nmc_review/classificationmodel} outlines the evaluation and classification scheme for NMC at main memory (Section~\ref{sec:nmc_review/procmainmem}) and storage class memory (Section~\ref{sec:nmc_review/procstorage}).  Section~\ref{sec:nmc_review/interondpcachevirtual} highlights the challenges with cache coherence, virtual memory, the lack of programming models, and data mapping schemes for NMC. In Section~\ref{sec:nmc_review/modelingmethod}, we look into the tools and techniques used to perform the design space exploration for these systems. This section also illustrates the importance of application characterization. Section~\ref{sec:nmc_review/system} presents our approach to near-memory computing. Additionally, we include a high-level analytic approach with a comparison to a traditional CPU-centric approach. Finally, Section~\ref{sec:nmc_review/futuredirections} highlights the lessons learned and future research directions.


\input{NMC_review/tables/classification.tex}

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/mainMemory.tex <==
\section{Processing Near-Main Memory}
\label{sec:nmc_review/procmainmem}
Processing near-main memory can allow us to reduce the data movement bottleneck by circumventing memory-package pin-count limitations.  We describe some of the notable architectures that process close to main memory. All solutions discussed in this section are summarized in Table~\ref{tab:nmc_review/arcClassification}.

\subsection{Programmable Unit}
\label{subsec:nmc_review/programmableunitmm}

\textbf{NDC (2014)} Pugsley~\etal~\cite{6844483} focus on Map-Reduce workloads, characterized by localized memory accesses and embarrassing parallelism. The architecture consists of a central multi-core processor connected in a daisy-chain configuration with multiple 3D-stacked memories. Each memory houses many ARM cores that can perform efficient memory operations without hitting the memory wall. However, they were not able to fully exploit the high internal bandwidth provided by HMC. The NMC processing units need careful redesigning to saturate the available bandwidth.

\textbf{TOP-PIM (2014)} Zhang~\etal\cite{zhang2014top} propose an architecture that consists of an accelerated processing unit (APU) coupled with 3D-stacked memory. Each APU consists of a GPU and a CPU on the same silicon die. The authors focus on providing code portability with ease-of-programmability.  The kernels analyzed span from graph processing to fluid and structural dynamics. However, the authors use traditional coherence mechanisms based on restricted memory regions that restrict data placement restriction.


\textbf{AMC (2015)} Nair~\etal\cite{nair2015active} develop an architecture called active memory cube (AMC), which is built upon the HMC-based memory. They add several processing elements to the vault of HMC, which they refer to it as \emph{lanes}. Each lane has a computational unit, a dedicated register file, and a load/store unit that performs read and write operations to a dedicated part of AMC memory. The host processor coordinates the communication between AMCs. However, such an approach requires low communication overhead to avoid performance degradation and undoing benefits of processing near-memory.

\textbf{PIM-enabled (2015)} Ahn~\etal~\cite{ahn2015pim} leverage an existing programming model so that the conventional architectures can exploit the NMC concept without changing the programming interface. They add compute-capable commands and specialized instructions to trigger the NMC computation. NMC processing units are composed of computation logic (e.g., adders) and an SRAM operand buffer. The authors place these processing units in the logic layer of an HMC-based memory. Offloading at the instruction level, however, could lead to significant overhead. In addition, the proposed solution requires substantial changes on the application side, hence reducing application readiness and can be a hurdle for wide adoption.


\textbf{TESSERACT (2015)} Ahn~\etal~\cite{teserract} focus on graph processing applications.
Their architecture consists of a host processor connected to an HMC-based memory. Each HMC vault has an out-of-order processor mapped to it. These cores can see only their local data partition, but they can communicate with each other using a message-passing protocol. The host processor has access to the entire address space of the HMC. The authors also use prefetching of data to exploit the high available memory bandwidth in their systems. However, the performance benefits largely depend upon the efficient distribution of graphs to the vaults in HMC-based memory, which the authors do not consider in this work.

\textbf{TOM (2016)} Hsieh~\etal~\cite{tom} propose an NMC architecture consisting of a host GPU interconnected to multiple 3D-stacked memories with small, light-weight GPU cores. They develop a compiler framework that automatically identifies possible offloading candidates. Code blocks are marked as beneficial to be offloaded by the compiler if the saving in memory bandwidth during the offloading execution is higher than the cost to initiate and complete the offload. A runtime system takes the final
decision as to where to execute a block. Furthermore, the framework uses a mapping scheme that ensures data and code co-location. The cost function proposed for code offloading makes use of static analysis to estimate the bandwidth saving. However, static analysis may fail on code with indirect memory accesses.

\textbf{Pattnaik\footnote{Architecture has no name, first author's name is shown.\label{noAuthor}} (2016) }Pattnaik~\etal~\cite{7756764}, similar to~\cite{tom}, develop an NMC-assisted GPU architecture. An affinity prediction model decides where to executed a kernel while a scheduling mechanism tries to minimize the application execution time. The scheduling mechanism can overrule the decision made by the affinity prediction model. The author proposes to invalidate the L2 cache of the host GPU after each kernel execution to keep memory consistency between the host GPU and the near-memory cores.  However, their affinity prediction model is trained for a specific set of applications and architecture that would have low prediction performance for a new, unknown application or architecture. 

\gcheck{
\textbf{MONDRIAN (2017)} Drumond~\etal~\cite{de2017mondrian} demonstrate that a hardware/software co-design approach is required to achieve efficiency and performance for NMC systems. In particular, they show that the current optimization of data-analytic algorithms heavily relies on random memory accesses while the NMC system prefers sequential memory accesses to saturate the huge bandwidth available. Based on this observation, the authors propose an architecture that consists of a mesh of HMC with tightly connected ARM cores in the logic layer.}

\textbf{MCN (2018)} Alian~\etal~\cite{alian2018application} use a light-weight near-memory processing unit in the buffered DRAM DIMM. The memory channel network (MCN) processor runs an OS with network software layers essential for running a distributed computing framework. The most striking feature of MCN is that the authors demonstrate unified near-data processing across various nodes using ConTutto FPGA~\cite{ConTutto_2017_MICRO} with IBM POWER8. However, supporting the entire TCP/IP stack on the near-memory accelerator requires a complex accelerator design. Current trends in the industry, however, are pushing for a simplified accelerator design shifting the complexity on the host core's side~\cite{openCAPI}).

% \gcheck{
% \textbf{SSAM (2018)} Lee~\etal~\cite{lee2018application} use Pin tool to characterize the architectural behaviors of kNN, which are at the core of similarity search applications. The instruction mix profile reveals a higher percentage of vector operations and memory reads, which confirms that vector operations are important for kNN workloads and are bound by high data movement. Based on the observation, they integrate specialized vector processing units in the logic layer of HMC and propose instruction extensions to leverage those hardware units. Similar to~\cite{ahn2015pim} they require to modify the application and the instruction-set architecture to exploit near-memory acceleration.
% }
\textbf{DNN-PIM (2018)} Liu~\etal~\cite{liu2018processing} propose heterogeneous NMC architecture
for the training of deep neural network (NN) models. The logic layer of 3D-stacked memory comprises programmable ARM cores and large fixed-function units (adders and multipliers). They extend the OpenCL programming model to accommodate the NMC heterogeneity. Both fixed-function NMC and programmable NMC appear as distinct compute devices. A runtime system dynamically maps and schedules NN
kernels on a heterogeneous NMC system based on online profiling of NN kernels.

\textbf{Boroumand\textsuperscript{\ref{noAuthor}} (2018)} Boroumand \etal\cite{googleWorkloads} evaluate NMC architectures for
Google workloads. They observe that: (1) many Google workloads spend a considerable amount of energy on data movement; (2) simple functions are responsible for a significant fraction of data movement. Based on their observations, they propose two NMC architectures, one with a general-purpose processing core and the other with a fixed-function accelerator coupled with HBM-based memory. While accelerating the Google workloads, the authors take into account the low area and power budget in consumer devices. They evaluate the benefits of the proposed NMC architectures.

\textbf{FIMDRAM (2021)} Kwon~\etal~\cite{fimdram2021ISSCC} make the following two observations. First, ML has become a driving factor in the advancement of various technologies. Second, the improvements in DRAM bandwidth could only be delivered with a significant increase in power consumption. Based on the above observations, the authors' goal is to develop an energy-efficient DRAM architecture for ML-based workloads that can deliver high bandwidth with low power consumption. To this end, the authors design an NMC architecture with 16-way floating-point16 (FP16) programmable compute units with an access granularity as the host processor, which simplifies various system-level aspects such as address mapping and interleaving. The experimental results demonstrate that FIMDRAM can provide $2\times$ performance and 70\% less energy consumption than a GPU+HBM implementation for DeepSpeech2 workload. FIMDRAM shows promising results for ML-based workloads, however, the efficacy for other data-intensive workloads such as weather prediction, genomics, and databases is still an open question.

\subsection{Fixed-Function Unit}
\label{subsec:nmc_review/ffunit}

\textbf{JAFAR (2015) }Xi~\etal\cite{xi2015beyond} embed an accelerator in a DRAM module to
implement database select operations. The key idea is to use the near-memory accelerator to scan and filter data directly in the memory while only the relevant data will be moved to the host CPU. Thus, having a significant reduction in data movement. The authors suggest using memory-mapped registers to read and write via application program interface (API) function calls to control the accelerator. Even though JAFAR shows promising potential in database applications, its evaluation is quite limited as it can handle only filtering operations. More complex operations fundamental for the database domain such as sorting, indexing and compression are not considered.


\textbf{IMPICA (2016)} Hsieh~\etal~\cite{hsieh2016accelerating} accelerate pointer chasing operations, ubiquitous in data structures. They propose adding specialized units that decouple address generation from memory accesses in the logic layer of 3D-stacked memory. These units traverse through the linked data structure in memory and return only the final node found to the host CPU. They also propose to completely decouple the page table of IMPICA from the host CPU to avoid virtual memory-related issues. The
memory coherence is assured by demarking different memory zones for the accelerators and the host CPU. This design provides a state-of-the-art technique for address translation in NMC for pointer chasing.


\textbf{Vermij\textsuperscript{\ref{noAuthor}} (2017)} Vermij~\etal~\cite{vermij2017sorting} propose a system for sorting algorithms where phases having high temporal locality are executed on the host CPU, while algorithm phases with poor temporal locality are executed on an NMC device. The architecture proposed consists of a memory technology-agnostic controller located at the host CPU side and a memory-specific controller tightly coupled with the NMC system. The NMC accelerators are placed in the memory-specific controllers and are assisted by an NMC manager. The NMC manager also supports cache coherency, virtual memory management, and communications with the host processor.

\textbf{GraphPIM (2017)} Nai~\etal~\cite{nai2017graphpim} map graph workloads in the HMC by exploiting its inherent atomic\footnote{An atomic instruction such as compare-and-set is an indivisible instruction where the CPU is not interrupted when performing such operations.} functionality. As they focus on atomics, they can offload at instruction granularity. Notably, they do not introduce new instructions for NMC and use the host instruction set to map to NMC atomics through an uncacheable memory region.  Similar to~\cite{ahn2015pim}, offloading at instruction granularity can have significant overhead. Besides, the mapping to NMC atomics instruction requires the graph framework to allocate data on particular memory regions via custom \textit{malloc}. This custom allocation requires changes on the application side, reducing the application readiness.

\textbf{GRIM-Filter (2018)} Kim~\etal~\cite{kim2018grim} develop a seed location filter for the read mapping stage of the genomics pipeline that exploits the high memory bandwidth and near-memory processing capabilities of 3D-stacked DRAM to improve the performance of DNA read mappers.  The authors demonstrate a $5.6\times-6.4\times$ lower false-negative rate with end-to-end performance improvement of $1.8\times-3.7\times$ over a state-of-the-art DNA read mapper. GRIM-Filter targets only the
short reads (i.e., segments on the order of several hundred base pairs long), while accelerating long reads is an important problem~\cite{whylongread_2018}.

\textbf{RecNMP (2020)} Ke~\etal~\cite{ke2020recnmp} overcome the memory bottleneck of personalized recommendation systems. A personalized recommendation is a fundamental part of services like a search engine, social network, etc. After characterizing production-recommendation models, the authors observe that the recommendation model's sparse embedding step leads to a memory bottleneck. To this end, the authors propose RecNMC, which
uses light-weight processing cores to accelerate embedding operations in the DIMM of existing standard DRAM. RecNMP accelerates the shows $9.8\times$ memory latency speedup and $45.9\%$ memory energy savings.

\textbf{GenASM (2020)} Cali~\etal~\cite{cali2020genasm} accelerate the \emph{approximate string matching }(ASM) step of genome analysis. ASM is a computationally-expensive step as it usually uses dynamic programming (DP)-based algorithms. The authors modify the underlying ASM algorithm to increase its parallelism and reduce its memory footprint significantly. Their accelerator design follows a systolic-array-based architecture that they place in the logic layer of HMC-based memory. The authors demonstrate the flexibility of their accelerator design in accelerating multiple steps of genome analysis.

\textbf{NATSA (2020)} Fernandez~\etal~\cite{fernandez2020natsa} design a near-memory accelerator for time series analysis. Specifically, the authors implement a matrix profile algorithm that has a low arithmetic intensity and operates on a large amount of data. As a result, this algorithm is memory-bound and performs poorly on multi-core systems. NATSA's processing element consists of floating-point arithmetic units that they place next to HBM-based 3D stacked memory.
NATSA improves performance by $9.9\times$ on average and reduces energy by $19.4\times$ on average over a multi-core implementation. However, it considers HBM as a stand-alone unit without a host-system. Such a scenario leads to practical concerns such as processing orchestration and data-mapping. 




\subsection{Reconfigurable Unit}
\label{subse:nmc_review/reconfigunit}
\textbf{Gokhale\textsuperscript{\ref{noAuthor}} (2015)} Gokhale~\etal~\cite{gokhale2015near} propose to place a data rearrangement engine (DRE) in the logic layer of the HMC to accelerate data accesses while still performing the computation on the host CPU. The authors target cache unfriendly applications with high memory latency due to irregular access patterns, e.g., sparse matrix multiplication.  Each of the DRE engines consists of a scratchpad, a simple controller processor, and a data mover. To make use of the DRE units, the
authors develop an API that supports several operations. Each operation is issued by the main application running on the host and served by a control program loaded by the OS on each DRE engine. Similar to~\cite{7756764}, the authors propose to invalidate the CPU caches after each fill and drain operation to keep memory consistency between the near-memory processors and the main CPU. This approach can introduce a significant overhead. Furthermore, the synchronization mechanism between the CPU and the near-memory processors is based on polling. Therefore, the CPU wastes clock cycles waiting for the near-memory accelerator to complete its operations. On the other hand, a light-weight synchronization mechanism based on interrupts could be a more efficient alternative.


\textbf{HRL (2015)} Gao~\etal~\cite{7446059} propose a reconfigurable logic architecture called heterogeneous reconfigurable logic (HRL) that consists of three main blocks: fine-grained configurable logic blocks (CLBs) for control unit, coarse-grained functional units (FUs) for basic arithmetic and logic operations, and output multiplexer blocks (OMBs) for branch support. Each memory module follows HMC like technology and houses multiple HRL devices in the logic layer. The central host processor is responsible for data partition and synchronization between NMC units. As in the case of~\cite{zhang2014top}, to avoid consistency issues and virtual-to-physical translation, the authors propose a memory-mapped non-cacheable memory region that puts restrictions on data placement.

\textbf{NDA (2015)} Farmahini~\etal~\cite{7056040} propose three different NMC architectures using coarse-grained reconfigurable arrays (CGRA) on commodity DRAM modules. This proposal requires minimal change to the DRAM architecture. However, programmers should identify which code would run close to memory. This dependence leads to increased programmer effort for demarking compute-intensive code for execution. Also, it does not support direct communication between NMC stacks.

% \textbf{NERO (2020)} Singh~\etal~\cite{singh2020nero} propose a \underline{ne}ar-HBM accelerator for weather prediction. 
% {We design and implement} \namePaper~%is used to implement and 
% {on an FPGA with HBM to} optimize two %representative 
% kernels (vertical advection and horizontal diffusion), %on an FPGA with HBM. 
% %These kernels 
% {which notably} represent %a 
% {the} spectrum of {computational diversity} found in the COSMO {weather prediction} application. 
% {We co-design a hardware-software framework and provide an optimized API to interface efficiently with the rest of the COSMO model, which runs on the CPU}.
% The {FPGA-based} solution for two representative compound stencil kernels leads to %active energy improvement 
% {performance improvements of $4.2\times$ and $8.3\times$ and}
% {energy reductions} of $22\times$ and $29\times$, {respectively,} {with respect to optimized CPU implementations~\cite{xu2018performance}}. 


==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/scm.tex <==
\section{Processing Near-Storage Class Memory}
\label{sec:nmc_review/procstorage}
NAND flash-based non-volatile memories (NVM) are trying to fill the latency gap between DRAMs and disks are termed as storage-class memories (SCM)~\cite{7151782}. SCM, like NVRAM, is even touted as a future replacement for DRAM~\cite{ranganathan2011microprocessors}. Moving computation in SCM has some of the similar benefits to DRAM concerning savings in bandwidth, power, latency, and energy but also because of the higher density it allows to work on much larger data-sets as compared to DRAM~\cite{quero2015self}.
%Flash and other emerging nonvolatile memories such as phase-change memory (PCM)~\cite{Qureshi:2009:SHP:1555815.1555760}, spin-transfer torque RAM (STT-RAM)~\cite{1609379}, etc., are termed as storage-class memories (SCM)~\cite{7151782}. These memories are trying to fill the latency gap between DRAMs and disks. SCM like NVRAM is even touted as a future replacement for DRAM~\cite{ranganathan2011microprocessors}. Moving computation in SCM has some of the similar benefits to DRAM concerning savings in bandwidth, power, latency, and energy but also because of the higher density it allows to work on much larger data-sets as compared to DRAM~\cite{quero2015self}.

\subsection{Programmable Unit}
\label{subsec:nmc_review/programmableunitscm}

\textbf{XSD (2013)} Cho~\etal~\cite{cho2013xsd} propose a solid-state drive (SSD)-based architecture that integrates graphics processing unit (GPU) close to the memory. They provide an API based on the MapReduce framework that allows users to express parallelism in their application and exploit the parallelism provided by the embedded GPU. They develop a performance model to tune the SSD design. The experimental results show that the proposed XSD is approximately $25\times$ faster than an SSD model incorporating a high-performance embedded CPU. However, the host CPU instruction set architecture (ISA) needs to be modified to launch the computation on the GPU embedded inside the SSD.

\textbf{WILLOW (2014)} Seshadri~\etal~\cite{seshadri2014willow} propose a system that has programmable processing units referred to as storage processor units (SPUs). Each SPU runs a small operating system (OS) that maintains and enforces security. On the host-side, the Willow driver creates and manages a set of objects that allow the OS and applications to communicate with SPUs. The programmable functionality is provided in the form of \textit{SSD Apps}. Willow enables programmers to augment and extend SSD semantics with application-specific features without compromising file system protection. The programming model based on remote procedure call (RPC) supports the concurrent execution of multiple SSD Apps and trusted code execution. However, it neither supports dynamic memory allocation nor allows users to load their tasks to run on the SSD dynamically.

\textbf{SUMMARIZER (2017)} Koo~\etal~\cite{koo2017summarizer} design APIs that can be used by the host application to offload filtering tasks to the inherent ARM-based cores inside an SSD processor. This approach reduces the amount of data transferred to the host and allows the host processor to work on the filtered result. They evaluate static and dynamic strategies for dividing the work between the host and SSD processor. However, sharing the SSD controller processor for user applications and SSD firmware can lead to performance degradation due to interference between I/O tasks and in-storage compute tasks.

\textbf{CompStor (2018) } Torabzadehkashi~\etal~\cite{torabzadehkashi2018compstor} propose an architecture that consists of NVMe over PCIe SSD and FPGA-based SSD controller coupled with in-storage processing subsystem (ISPS) based on the quad-core ARM A53 processor.  They modify the SSD controller hardware and software to provide high bandwidth and low latency data path between ISPS and the flash media interface. Fully isolated control and data paths ensure concurrent data processing and storage functionality without degradation in either one's performance. The architecture supports porting a Linux operating system. However, homogeneous processing cores in the SSD are not sufficient to meet the requirement of complex modern applications~\cite{torabzadehkashi2019catalina}.


\subsection{Fixed-Function Unit}
\label{subsec:ffunit2}

\textbf{Smart SSD (2013)} Kang~\etal~\cite{kang2013enabling} implement the Smart SSD features in the firmware of a Samsung SSD and modify the Hadoop core and MapReduce framework to use task-lets as a map or a reduce function. To evaluate the prototype, they used a micro-benchmark and log analysis application on both the device and the host. Their SmartSSD is able to outperform host-side processing drastically by utilizing internal application parallelism. Likewise, Do~\etal~\cite{park2014query} extend Microsoft SQL Server to offload database operations onto a Samsung Smart SSD. The selection and aggregation operators are compiled into the firmware of the SSD. Quero~\etal~\cite{quero2015self} modify the Flash Translation Layer (FTL) abstraction and implement an indexing algorithm based on the B++tree data structure to support sorting directly in the SSD. The approach of modifying the SSD firmware to support the processing of certain functions is fairly limited and can not support the wide variety of workloads~\cite{torabzadehkashi2019catalina}.

\textbf{ProPRAM (2015)} Wang~\etal~\cite{wang2015propram} observe that NVM is often supporting built-in logic like for data comparison, write or flip-n-write module. Therefore, the authors propose to exploit the existing resources inside NVM-based memory chips to accelerate the simple non-compute intensive functions in emerging big data applications. They expose the peripheral logic to the application stack through ISA extension. Like~\cite{kang2013enabling,park2014query,quero2015self}, this approach cannot support the diverse workload requirements.


\textbf{BISCUIT (2016)} Gu~\etal~\cite{gu2016biscuit} present a near-memory computing framework that allows programmers to write a data-intensive application to run in a distributed manner on the host and the NMC-capable storage system. The storage hardware incorporates a pattern matcher IP designed for NMC.  The authors evaluate their approach by accelerating MySQL-based application. However, the NMC system acts as a slave to the host CPU, and all data is controlled by the host CPU. Therefore, this architecture needs to manage communications messages from the host effectively.

\subsection{Reconfigurable Unit}
\label{subse:reconfigunit2}


\textbf{BlueDBM (2015) }Jun~\etal~\cite{jun2015bluedbm} present a flash-based platform, called BlueDBM, built of flash storage devices augmented with an application-specific FPGA-based in-storage processor. The data-sets are stored in the flash array and are read by the FPGA accelerators. Each accelerator implements a variety of application-specific distance comparators used in the high-dimensional nearest-neighbor search algorithms. They also use the same architecture exploration platform for graph analytics. However, the platform does not support dynamic task loading, similar to ~\cite{seshadri2014willow}, and has limited OS-level flexibility. 

\textbf{CARIBOU (2017) }Zsolt~\etal~\cite{istvan2017caribou} enable key-value store interface over TCP/IP socket to the storage node comprising of an FPGA connected to DRAM/NVRAM. They implement selection operators in the FPGA, which are parameterizable at runtime, both for structured and unstructured data, to reduce data movement and avoid the negative impact of near-data processing on the data retrieval rate. Like~\cite{jun2015bluedbm}, Caribou does not have OS-level flexibility, e.g., the file-system is not supported transparently.



==> PhD_Thesis_Updated_arxiv (1)/NMC_review/sections/system.tex <==
\section{Practicalities of Near-Memory Computing}
\label{sec:system}
In this section, we describe our approach
to solve some of the issues related to NMC. Besides the design of the near-memory computing platform itself, we are focusing on how such a hybrid system can be effectively programmed to maximize performance and minimize power consumption. Additionally, we are extensively analyzing applications to assess essential application metrics for these devices. The various components of our framework are outlined below.

\subsection{NMC Architecture}
Figure~\ref{fig:targetplatform} depicts an abstract view of our reference computing platform that we consider. We modeled a multi-core host system interconnected to an external stacked near-memory system via high speed interconnect. In this model, the near-memory compute units are modeled as low power cores (Table~\ref{tab:systemparameters}), which are placed in the logic layer of the 3D stacked DRAM. For the 3D stacked memory, we consider a 4-GB HMC like design, with 8 DRAM layers. Each DRAM layer is split into 16 dual banked partitions with four vertical partitions forming a vault. Each vault has its vault controller. 


\begin{figure}[h]
\centering
\includegraphics[width=21pc]{NMC_review/img/systemNMC53_final.pdf}
\caption{Overview of a system with NMC capability~\cite{NAPEL}. On the right, an abstract view of application code with kernels {that are} offloaded to NMC
\label{fig:targetplatform}}
\end{figure}

%}
% \subsection{Platform Agnostic Application Characterization for NMC}
% \label{subsec:platform-agnostic-NMC}

% We define the following microarchitecture independent metrics to characterize the applications from NMC perspective and identify the kernels that can potentially benefit from NMC. 

% \begin{itemize}
%     \item \textbf{Memory Entropy:} It measures the randomness of the memory accesses. Yen~et~al.~\cite{yen2008notary} devise the formula by applying Shannon's definition to the memory addresses. The higher the memory entropy, the higher the miss ratio. Hence, an application with higher entropy can benefit from NMC.  
%     \item \textbf{Spatial Locality:} It measures the probability of accessing nearby memory locations. Spatial Locality is derived from data temporal reuse, which is the number of unique addresses accessed since the last reference of the requested data. We use the formula proposed by Gu~et~al.~\cite{gu2009component} to calculate spatial locality score.     
%     \item \textbf{Data-Level Parallelism:} It measures the average possible vector length and is relevant for NMC when employing specific SIMD processing units as near-memory computation units. It is derived from instruction-level parallelism (ILP) score per opcode such as load, store, etc. This metric represents the number of instructions with the same opcode that could run in parallel, thus expressing the DLP per opcode. We compute the average value of DLP using the weighted sum over all opcodes of the DLP per code. 
%     \item \textbf{Basic-block level Parallelism:} A basic block is the smallest component in the LLVM intermediate representation (IR) that can be parallelized. If an application has high basic-block level parallelism, it can benefit from multiple processing units.

% \end{itemize}

% We extend an open-source platform-independent software analysis tool (PISA)~\cite{anghel2016instrumentation} with the above-listed metrics and use it to analyze multi-thread applications from NMC perspective. As an example, we show in Figure~\ref{fig:pisa-nmc} the analysis result of two applications from PolyBench/C 4.1~\cite{pouchet2012polybench}, which is a collection of standard kernels. Each kernel is a single file that can be tuned at compile time. In Figure~\ref{fig:pisa-nmc} we show the characterization of two applications having opposite memory behavior: \texttt{Gramschmidt} and \texttt{Jacobi-1d}.
% Figure~\ref{fig:spatial} presents the spatial locality values for different pairs of cache line sizes. For instance, 8-16B means spatial locality doubling the cache line size from 8B to 16B. In the figure, the total spatial locality is the weighted sum of all the values (see \cite{corda2019scopes}). Figure~\ref{fig:spatial} shows, for different cache size configurations, how \texttt{Gramschmidt} has significantly lower spatial locality than \texttt{Jacobi-1d}. This lower locality can be attributed to non-regular memory accesses (e.g., diagonal accesses in a matrix). Figure~\ref{fig:entropy} presents memory entropy for different address granularity. The bit reductions mean reduction in the number of bits of the addresses considered to compute the entropy. The bit reduction reflects as using bigger cache line sizes and could be used to perform further spatial locality analysis (see \cite{corda2019scopes,corda2019DSD}). Figure~\ref{fig:entropy} highlights the lower memory entropy of \texttt{Jacobi-1d} compared to \texttt{Gramschmidt} due to localized memory accesses.
% A detailed study on workload characterization from NMC perspective using above mentioned architecture-independent metrics and representative benchmarks are presented in \cite{corda2019scopes,corda2019DSD}.


% \begin{figure}[] 
%     \centering
%     \subfloat[Spatial Locality]{%
%         \includegraphics[width=8.5cm,trim={2.1cm 2cm 4.4cm 1.8cm},clip]{NMC_review/img/spat_jr_final.eps}%
%         \label{fig:spatial}%
%         }%
%     \hfill%
%     \subfloat[Memory Entropy]{%
%         \includegraphics[width=8.5cm,trim={2.1cm 2cm 4.4cm 1.8cm},clip]{NMC_review/img/entr_jr_final.eps}%
%         \label{fig:entropy}%
%         }%
%     \caption{Spatial Locality and Memory Entropy characterization for two applications from PolyBench 
%     \label{fig:pisa-nmc}}
% \end{figure}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.85\linewidth]{NMC_review/img/JournalPaper_final.pdf}
%     \caption{Proposed compilation flow for the system with NMC capabilities depicted in Figure~\ref{fig:targetplatform}. 
%     }
%     \label{fig:my_label}
% \end{figure*}

% \subsection{Compilation and Programming Model}
% The compiler support has been built on top of our previous work~\cite{zinenko:hal-01965599} and is completely integrated into a state-of-the-art loop optimizer~\cite{grosser2012polly}. Similar to previous works~\cite{akin2015data, 7856642}, we assume our near-memory accelerators expose a library of memory-bound kernels via an application programming interface (API). We provide compiler support to automatically, and transparently for the application,  detect such kernels and call the proper accelerator routine. The compilation flow (Figure~\ref{fig:my_label}) follows a classical compiler design with a front-end, a mid-level optimizer, and target-specific back-ends. We extend this design embedding a state-of-the-art pattern matching framework in the mid-level optimizer. 

% Briefly, the compilation flow is as follow: We start from an application written in C/C++; the front-end is responsible for lowering the application code to an intermediate representation. For our work, we use the LLVM compiler infrastructure and exploit its intermediate representation (LLVM-IR). At IR level, we rely on a state-of-the-art polyhedral optimizer~\cite{grosser2012polly} to extract compute kernels and obtain for each of them a mathematical description based on Presburger\cite{10.1007/978-3-642-15582-6_49} sets. On top of this mathematical model, our pattern matching framework is used to match and swap kernels with accelerator-specific run-time calls. Once the run-time calls have been introduced, we rely again on the polyhedral optimizer to lower the mathematical abstraction back to LLVM-IR. During the latest stages of compilation, the run-time accelerator specific libraries are linked with the application binary. With our approach, legacy code can exploit, in a completely transparent way for the user, near-memory acceleration without any change on the application side. 



% \subsection{Early Design Stage Modeling}
% We make use of a first-order analytic model to evaluate the benefit of using near-memory processing in our system in the early design stage. As mentioned in Section~\ref{subsec:performanceevaluation}, a high-level analytic model abstract the detailed micro-architecture. Hence, this approach makes our analytical model more generic and provides quick insights.



% Our analytic model incorporates evaluation methodology as described in Figure~\ref{fig:methodology}. To see the potential of computing close to the memory and when it is useful to follow a data-centric approach, we make a comparison of a CPU-centric approach consisting of a multi-core system and compare it to a data-centric approach which has near-memory processing units in the logic layer of HMC like 3D stacked. In the multi-core system, each core has its L1 cache and a shared L2 cache.  In the near-memory system, we assume certain parts of the computation called NMC-kernels would be offloaded to the near-memory compute units, and the other parts will be executed in the host system. The number of vaults inside the HMC and external interconnects links are kept as varying parameters which have an impact on internal and the external bandwidth of the 3D memory respectively.

% \begin{comment}

% \begin{figure*}
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.5]{img/results/delay.png}
%   \caption{Normalized Delay}
%   \label{fig:delay}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.5]{img/results/energy.png}
%   \caption{Normalized Energy}
%   \label{fig:energy}
% \end{subfigure}
% \caption{Performance and Energy Comparison between multi-core and NMC with a host system using high-level analytic model}
% \label{fig:results}
% \end{figure*}


% \end{comment}



% \begin{figure*}[h]
% \centering
% \subfloat[Normalized Delay]{\includegraphics[width=9cm]{NMC_review/img/delay3_final.png}%img/results/delay.png}
% \label{fig:delay}}
% \subfloat[Normalized Energy]{\includegraphics[width=9cm]{NMC_review/img/energy3_final.png}%img/results/energy.png}
% \label{fig:energy}}
% \caption{Performance and energy comparison between multi-core and an NMC system, which is attached to a host system, using high-level analytic model}
% \label{fig:results}
% \end{figure*}



% \textit{Performance Calculation:} The model estimates the execution time as the ratio between the number of memory accesses required to move the block of data to and from the I/O system and the available I/O bandwidth of each memory subsystem. The execution time takes into account the time to process the instructions $\Pi_{non-memory}$ and latency due to memory access $\Pi_{memory}$ (Table~\ref{tab:systemparameters}).

% \begin{comment}

% \begin{equation}
% \label{eq:1}
% \begin{split}
% n_{load}=n_r/n_{vaults}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:2}
% \begin{split}
% n_{store}=n_w/n_{vaults}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:3}
% \begin{split}
% m_{total}= n_{load}+n_{store}
% \end{split}    
% \end{equation}
% \begin{equation}
% \label{eq:4}
% \begin{split}
% \Pi_{memory}=\frac{1}{n_{pe}} \displaystyle \sum_{}^{N_{vaults}}\frac{m_{total}*b_{rb}}{BW_{int}}
% \end{split}    
% \end{equation}

% \end{comment}


% %\todo[author=Gagan, inline]{Add performance model equations here}


% \textit{Energy Calculation:} We build a power model for both CPU-centric and a near-memory system by taking into account dynamic as well as static energy. Dynamic energy is the product of the energy per memory access and the number of memory accesses at each level of the memory hierarchy.  It is assumed to scale linearly with utilization. Static energy is estimated as the product of time and static power for each component. It is scaled based on the number of cores and the cache size. 
    
% For modeling the HMC, we refer to~\cite{6242474} and~\cite{6844483}. We consider energy per bit of 3.7 pJ/b for accessing the DRAM layers and 1.5 pJ/b for the operations and data movements in the HMC logic layer. A static power of 0.96 W is assumed~\cite{6844483} to model the additional components in the logic layer.

% %\todo[author=Gagan, inline]{Add energy model equations here}


% \textit{Performance and Energy Exploration:} 
% We vary the cache miss rate, which encapsulates application characteristics, both at L1 and L2 level to see the impact it has on the performance of the entire system. In case of a near-memory system, we consider the scenario when all accesses are done to the different vaults inside the HMC memory, which can exploit the inherent parallelism offered by the 3D memory. In Figure~\ref{fig:results}, the x and y-axis represent the miss rate at L1 and L2, respectively. Results in Figure~\ref{fig:results} are normalized to NMC+host system. 

% Based on our evaluation, we make the following three observations. First, in case of performance and energy, we can see a similar trend, i.e., if the miss rate (L1 and L2) increases the multi-core system performance degrades compared to the NMC systems. This degradation is because of the increase in data movement. The data has to be fetched from the off-chip DRAM. Second, if the CPU does not reuse the data brought into the caches, the use of caching becomes inefficient. Third, the application (or function) with low locality can take advantage of the near-memory approach, whereas the other application (or function) with high locality would benefit more from the traditional approach. 
 


==> PhD_Thesis_Updated_arxiv (1)/NMC_review/tables/architectures.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.2}

\caption{Classification and evaluation of \fc{representative architectures in category of our NMC taxonomy}, refer to Table~\ref{tab:nmc_review/arcLegend} for the legend}
\label{tab:nmc_review/arcClassification}
\centering
\tabcolsep=0.22cm
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccclccllclllcl@{}|}
\hline
\multicolumn{2}{|c}{\textbf{NMC Architecture}}& \multicolumn{3}{|c|}{\textbf{Memory}}& \multicolumn{4}{c|}{\textbf{Processing}} &\textbf{Tool}&\multicolumn{3}{|c|}{\textbf{Interoperability}}& \multicolumn{1}{|c|}{\textbf{App. Domain}} \\ \hline
\multicolumn{1}{|l}{\rotatebox[origin=c]{90}{\textbf{Architecture}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Year}}}&
\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Hierarchy}}}   & \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Type}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Integration}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{NMC Unit}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Implementation}}} &
\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Granularity}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Host Unit}}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Evaluation}}} & 
%\multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Programming Interface} }} &
\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Programming Model} }} &
\multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Cache Coherence}}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{90}{\textbf{Virtual Memory}}} &
\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Workload}}}\\ 

\multicolumn{1}{|c}{}& %architecture
\multicolumn{1}{c|}{}& %year
\multicolumn{1}{c|}{}& %Hierarchy
\multicolumn{1}{c|}{}&  %Kind of memory
\multicolumn{1}{l|}{}& %Stacked
\multicolumn{1}{c|}{}& %NMC unit
\multicolumn{1}{l|}{}& %implementation
\multicolumn{1}{l|}{}& %granularity
\multicolumn{1}{l|}{}& %host unit
\multicolumn{1}{l|}{}& %evaluation 
%\multicolumn{1}{l|}{}& %programming interface
\multicolumn{1}{l|}{}&%programming model
\multicolumn{1}{l|}{}&  %cache coherence
\multicolumn{1}{l|}{}&  % virtual memory
\multicolumn{1}{l|}{}\\ \hline % application 

\multicolumn{1}{|l}{XSD~\cite{cho2013xsd}}&
\multicolumn{1}{c|}{2013} &
\multicolumn{1}{c|}{SCM} &
\multicolumn{1}{c|}{SSD} & 
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{GPU}&
\multicolumn{1}{l|}{P} &
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{MapReduce}&
\multicolumn{1}{l|}{-}& 
\multicolumn{1}{l|}{-} & 
\multicolumn{1}{l|}{MapReduce}\\ \hline

\multicolumn{1}{|l}{SmartSSD~\cite{kang2013enabling}}& %architecture
\multicolumn{1}{c|}{2013} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{MapReduce}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{N} &  % virtual memory
\multicolumn{1}{l|}{Database}\\ \hline %application

\multicolumn{1}{|l}{WILLOW~\cite{seshadri2014willow}}& %architecture
\multicolumn{1}{c|}{2014} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y}& %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-}&  % virtual memory
\multicolumn{1}{l|}{Generic}\\ \hline %application


\multicolumn{1}{|l}{NDC~\cite{6844483}}&
\multicolumn{1}{c|}{2014} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & 
\multicolumn{1}{l|}{S}  & 
\multicolumn{1}{c|}{CPU}&
\multicolumn{1}{l|}{P} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{N} &
\multicolumn{1}{l|}{MapReduce}&
\multicolumn{1}{l|}{R} & 
\multicolumn{1}{l|}{N}& 
\multicolumn{1}{l|}{MapReduce}\\ \hline


\multicolumn{1}{|l}{TOP-PIM~\cite{zhang2014top}}& %architecture
\multicolumn{1}{c|}{2014} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{GPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{N} & %programming interface
\multicolumn{1}{l|}{OpenCL}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Graph and HPC}\\ \hline %application


\multicolumn{1}{|l}{AMC~\cite{nair2015active}}&
\multicolumn{1}{c|}{2015} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & 
\multicolumn{1}{l|}{S}  & 
\multicolumn{1}{c|}{CPU}&
\multicolumn{1}{l|}{P} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{OpenMP}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Y} & 
\multicolumn{1}{l|}{HPC}\\ \hline

\multicolumn{1}{|l}{JAFAR~\cite{xi2015beyond}}&
\multicolumn{1}{c|}{2015} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{DRAM} & 
\multicolumn{1}{l|}{US}  & 
\multicolumn{1}{c|}{ACC}&
\multicolumn{1}{l|}{F} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}& 
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Database}\\ \hline

\multicolumn{1}{|l}{TESSERACT~\cite{teserract}}& %architecture
\multicolumn{1}{c|}{2015} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation     in house
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{N} &  % virtual memory
\multicolumn{1}{l|}{Graph processing}\\ \hline %application

\multicolumn{1}{|l}{Gokhale~\cite{gokhale2015near}}&
\multicolumn{1}{c|}{2015} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & 
\multicolumn{1}{l|}{S}  & 
\multicolumn{1}{c|}{ACC}&
\multicolumn{1}{l|}{F} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Y} & 
\multicolumn{1}{l|}{Generic}\\ \hline

\multicolumn{1}{|l}{HRL~\cite{7446059}}&
\multicolumn{1}{c|}{2015} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & %kind of memory
\multicolumn{1}{l|}{S}  & %stacked
\multicolumn{1}{c|}{CGRA+FPGA}& %NMC unit
\multicolumn{1}{l|}{R} & % implementation
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} &%host unit
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{N}& %programming interface
\multicolumn{1}{l|}{MapReduce}& %\ahsan[check for inconsistency]
\multicolumn{1}{l|}{Y}& %cache coherence
\multicolumn{1}{l|}{N} & %virtual memory
\multicolumn{1}{l|}{Data analytics}\\ \hline

\multicolumn{1}{|l}{ProPRAM~\cite{wang2015propram}}& %architecture
\multicolumn{1}{c|}{2015} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{PCM} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{I} & %granularity
\multicolumn{1}{l|}{-} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{ISA Extension}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Data analytics}\\ \hline %application

\multicolumn{1}{|l}{BlueDBM~\cite{jun2015bluedbm}}& %architecture
\multicolumn{1}{c|}{2015} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{FPGA}& %NMC unit
\multicolumn{1}{l|}{R} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{-} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Data analytics} \\ \hline %application

%\multicolumn{1}{|l}{Huang~\cite{qian2015study}}& %architecture
%\multicolumn{1}{c|}{2015} & %year
%\multicolumn{1}{c|}{HM} & %Hierarchy
%\multicolumn{1}{c|}{SSD + DRAM} &  %Kind of memory
%\multicolumn{1}{l|}{S}  & %Stacked
%\multicolumn{1}{c|}{CPU}& %NMC unit
%\multicolumn{1}{l|}{P} & %implementation
%\multicolumn{1}{l|}{A} & %granularity
%\multicolumn{1}{l|}{-} & %host unit
%\multicolumn{1}{c|}{S}& %evaluation  DrAmSim2 7 Flash Sim; benchmark: CloudRank-D v1.0
%\multicolumn{1}{l|}{N} & %programming interface
%\multicolumn{1}{l|}{Y}&  %cache coherence
%\multicolumn{1}{l|}{N} &  % virtual memory
%\multicolumn{1}{l|}{Data Analytics} \\ \hline %application

\multicolumn{1}{|l}{NDA~\cite{7056040}}& %architecture
\multicolumn{1}{c|}{2015} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{DRAM} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{CGRA}& %NMC unit
\multicolumn{1}{l|}{R} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{OpenCL}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{MapReduce}\\ \hline %application

\multicolumn{1}{|l}{PIM-enabled~\cite{ahn2015pim}}& %architecture
\multicolumn{1}{c|}{2015} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{I} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation inhouse/cycle accurate---CACTI 6.5
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{ISA extension}&
\multicolumn{1}{l|}{Y}&  %cache coherence non cacheable
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{Generic}\\ \hline %application

%\multicolumn{1}{|l}{BSSync}& %architecture
%\multicolumn{1}{c|}{2015} & %year
%\multicolumn{1}{c|}{MM} & %Hierarchy
%\multicolumn{1}{c|}{C3D} &  %Kind of memory
%\multicolumn{1}{l|}{S}  & %Stacked
%\multicolumn{1}{c|}{ACC}& %NMC unit
%\multicolumn{1}{l|}{F} & %implementation
%\multicolumn{1}{l|}{I} & %granularity
%\multicolumn{1}{l|}{CPU} & %host unit
%\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
%\multicolumn{1}{l|}{NC}&  %cache coherence
%\multicolumn{1}{l|}{N} &  % virtual memory
%\multicolumn{1}{l|}{Machine Learning} \\ \hline %application

\multicolumn{1}{|l}{IMPICA~\cite{hsieh2016accelerating}}& %architecture
\multicolumn{1}{c|}{2016} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}&  %cache coherence *************CHECK****
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{Pointer chasing}\\ \hline %application

\multicolumn{1}{|l}{TOM~\cite{tom}}&
\multicolumn{1}{c|}{2016} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & 
\multicolumn{1}{l|}{S}  & 
\multicolumn{1}{c|}{GPU}&
\multicolumn{1}{l|}{P} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{GPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{N} &
\multicolumn{1}{l|}{CUDA}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Y} & 
\multicolumn{1}{l|}{Generic}\\ \hline


%\multicolumn{1}{|l}{CHAMELEON~\cite{7783753}}& %architecture
%\multicolumn{1}{c|}{2016} & %year
%\multicolumn{1}{c|}{MM} & %Hierarchy
%\multicolumn{1}{c|}{LRDIMM} &  %Kind of memory
%\multicolumn{1}{l|}{US}  & %Stacked
%\multicolumn{1}{c|}{CGRA}& %NMC unit
%\multicolumn{1}{l|}{R} & %implementation
%\multicolumn{1}{l|}{K} & %granularity
%\multicolumn{1}{l|}{CPU} & %host unit
%\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface adapt to openCL
%\multicolumn{1}{l|}{Y}&  %cache coherence
%\multicolumn{1}{l|}{Y} &  % virtual memory
%\multicolumn{1}{l|}{Generic} \\ \hline %application

\multicolumn{1}{|l}{BISCUIT~\cite{gu2016biscuit}}& %architecture
\multicolumn{1}{c|}{2016} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Database}\\ \hline %application

\multicolumn{1}{|l}{Pattnaik~\cite{7756764}}& %architecture
\multicolumn{1}{c|}{2016} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Simulation 
\multicolumn{1}{c|}{GPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{GPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{-} & %programming interface
\multicolumn{1}{l|}{CUDA}&
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Generic}\\ \hline %application

\multicolumn{1}{|l}{CARIBOU~\cite{istvan2017caribou}}& %architecture
\multicolumn{1}{c|}{2017} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{DRAM} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{FPGA}& %NMC unit
\multicolumn{1}{l|}{R} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{-} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Database}\\ \hline %application


\multicolumn{1}{|l}{Vermij~\cite{vermij2017sorting}}&
\multicolumn{1}{c|}{2017} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{C3D} & 
\multicolumn{1}{l|}{S}  & 
\multicolumn{1}{c|}{ACC}&
\multicolumn{1}{l|}{F} &
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Y} & 
\multicolumn{1}{l|}{Sorting}\\ \hline

\multicolumn{1}{|l}{SUMMARIZER~\cite{koo2017summarizer}}& %architecture
\multicolumn{1}{c|}{2017} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Database}\\ \hline %application

\multicolumn{1}{|l}{MONDRIAN~\cite{de2017mondrian}}& %architecture
\multicolumn{1}{c|}{2017} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{A+S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{Data analytics}\\ \hline %application

\multicolumn{1}{|l}{GraphPIM~\cite{nai2017graphpim}}&
\multicolumn{1}{c|}{2017} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{DRAM} & 
\multicolumn{1}{l|}{US}  & 
\multicolumn{1}{c|}{ACC}&
\multicolumn{1}{l|}{F} &
\multicolumn{1}{l|}{I} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{S}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{API}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{N} & 
\multicolumn{1}{l|}{Graph}\\ \hline

\multicolumn{1}{|l}{MCN~\cite{alian2018application}}&
\multicolumn{1}{c|}{2018} &
\multicolumn{1}{c|}{MM} &
\multicolumn{1}{c|}{DRAM} & 
\multicolumn{1}{l|}{US}  & 
\multicolumn{1}{c|}{CPU}&
\multicolumn{1}{l|}{P} &
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} &
\multicolumn{1}{c|}{P}&
%\multicolumn{1}{l|}{Y} &
\multicolumn{1}{l|}{TCP/IP}&
\multicolumn{1}{l|}{Y}& 
\multicolumn{1}{l|}{Y} & 
\multicolumn{1}{l|}{Generic}\\ \hline

% \multicolumn{1}{|l}{SSAM~\cite{lee2018application}}&
% \multicolumn{1}{c|}{2018} &
% \multicolumn{1}{c|}{MM} &
% \multicolumn{1}{c|}{C3D} & 
% \multicolumn{1}{l|}{S}  & 
% \multicolumn{1}{c|}{CPU}&
% \multicolumn{1}{l|}{P} &
% \multicolumn{1}{l|}{K} & %granularity
% \multicolumn{1}{l|}{CPU} &
% \multicolumn{1}{c|}{P}&
% %\multicolumn{1}{l|}{Y} &
% \multicolumn{1}{l|}{API}&% programming model
% \multicolumn{1}{l|}{N}& 
% \multicolumn{1}{l|}{N} & 
% \multicolumn{1}{l|}{Similarity search}\\ \hline 

\multicolumn{1}{|l}{DNN-PIM~\cite{liu2018processing}}&
\multicolumn{1}{c|}{2018} &
\multicolumn{1}{c|}{MM} & %hierarcy
\multicolumn{1}{c|}{C3D} & %type
\multicolumn{1}{l|}{S}  & %integration
\multicolumn{1}{c|}{CPU + ACC}& % MCN Unit
\multicolumn{1}{l|}{P+F} & % Implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %Host Unit
\multicolumn{1}{c|}{P+S}& %Evauation
%\multicolumn{1}{l|}{Y} & %Programming Interface
\multicolumn{1}{l|}{OpenCL}& % programming model
\multicolumn{1}{l|}{Y}&  %cache coherence support
\multicolumn{1}{l|}{N} & %virtual memory 
\multicolumn{1}{l|}{DNN training}\\ \hline %workload

\multicolumn{1}{|l}{Boroumand~\cite{googleWorkloads}}& %architecture
\multicolumn{1}{c|}{2018} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{CPU+ACC}& %NMC unit
\multicolumn{1}{l|}{P+F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y}& %programming interface
\multicolumn{1}{l|}{-}& % programming model
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-}&  % virtual memory
\multicolumn{1}{l|}{Google workloads}\\ \hline%application

\multicolumn{1}{|l}{GRIM-Filter~\cite{kim2018grim}}& %architecture
\multicolumn{1}{c|}{2018} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y}& %programming interface
\multicolumn{1}{l|}{-}& % programming model
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-}&  % virtual memory
\multicolumn{1}{l|}{Read mapping}\\ \hline%application

\multicolumn{1}{|l}{CompStor~\cite{torabzadehkashi2018compstor}}& %architecture
\multicolumn{1}{c|}{2018} & %year
\multicolumn{1}{c|}{SCM} & %Hierarchy
\multicolumn{1}{c|}{SSD} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{CPU}& %NMC unit
\multicolumn{1}{l|}{P} & %implementation
\multicolumn{1}{l|}{A} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{P}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&% programming model
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{Text search}\\ \hline% application

\multicolumn{1}{|l}{RecNMP~\cite{ke2020recnmp}}& %architecture
\multicolumn{1}{c|}{2020} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{DRAM} &  %Kind of memory
\multicolumn{1}{l|}{US}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&% programming model /////HIDDEN
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{Y} &  % virtual memory
\multicolumn{1}{l|}{Recommendation system}\\ \hline% application


\multicolumn{1}{|l}{GenASM~\cite{cali2020genasm}}& %architecture
\multicolumn{1}{c|}{2020} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{CPU} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&% programming model /////HIDDEN
\multicolumn{1}{l|}{Y}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{String matching}\\ \hline% application



\multicolumn{1}{|l}{NATSA~\cite{fernandez2020natsa}}& %architecture
\multicolumn{1}{c|}{2020} & %year
\multicolumn{1}{c|}{MM} & %Hierarchy
\multicolumn{1}{c|}{C3D} &  %Kind of memory
\multicolumn{1}{l|}{S}  & %Stacked
\multicolumn{1}{c|}{ACC}& %NMC unit
\multicolumn{1}{l|}{F} & %implementation
\multicolumn{1}{l|}{K} & %granularity
\multicolumn{1}{l|}{-} & %host unit
\multicolumn{1}{c|}{S}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{API}&% programming model /////HIDDEN
\multicolumn{1}{l|}{-}&  %cache coherence
\multicolumn{1}{l|}{-} &  % virtual memory
\multicolumn{1}{l|}{Time series analysis}\\ \hline% application


\multicolumn{1}{|l}{{NERO}~\cite{singh2020nero}}& %architecture
\multicolumn{1}{c|}{{2020}} & %year
\multicolumn{1}{c|}{{MM}} & %Hierarchy
\multicolumn{1}{c|}{{C3D}} &  %Kind of memory
\multicolumn{1}{l|}{{S}}  & %Stacked
\multicolumn{1}{c|}{{ACC}}& %NMC unit
\multicolumn{1}{l|}{{R}} & %implementation
\multicolumn{1}{l|}{{K}} & %granularity
\multicolumn{1}{l|}{{CPU}} & %host unit
\multicolumn{1}{c|}{{P}}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{{API}}&% programming model /////HIDDEN
\multicolumn{1}{l|}{{Y}}&  %cache coherence
\multicolumn{1}{l|}{{Y}} &  % virtual memory
\multicolumn{1}{l|}{{Weather prediction modeling}}\\ \hline% application


\multicolumn{1}{|l}{{FIMDRAM}~\cite{fimdram2021ISSCC}}& %architecture
\multicolumn{1}{c|}{{2021}} & %year
\multicolumn{1}{c|}{{MM}} & %Hierarchy
\multicolumn{1}{c|}{{C3D}} &  %Kind of memory
\multicolumn{1}{l|}{{S}}  & %Stacked
\multicolumn{1}{c|}{{ACC}}& %NMC unit
\multicolumn{1}{l|}{{P}} & %implementation
\multicolumn{1}{l|}{{I}} & %granularity
\multicolumn{1}{l|}{{-}} & %host unit
\multicolumn{1}{c|}{{P}}& %evaluation 
%\multicolumn{1}{l|}{Y} & %programming interface
\multicolumn{1}{l|}{{API}}&% programming model /////HIDDEN
\multicolumn{1}{l|}{{Y}}&  %cache coherence
\multicolumn{1}{l|}{{Y}} &  % virtual memory
\multicolumn{1}{l|}{{Machine learning}}\\ \bottomrule% application
\end{tabular}
}
\end{table*}

     

==> PhD_Thesis_Updated_arxiv (1)/NMC_review/tables/classification.tex <==

\begin{comment}


\begin{table*}[h]
\centering


\begin{tabular}{|l|l|l|l|}
\hline
                                  & \textbf{Property}                              & \textbf{Abbrev}  & \textbf{Description}                        \\ \hline
\multirow{10}{*}{\textbf{Memory}}         & \multirow{3}{*}{Hierarchy}            & MM    & Main memory                        \\
                                  &                                       & SCM   & Storage class memory               \\
                                  &                                       & HM    & Heterogeneous memory               \\
                             \rule{0pt}{25pt}     \cline{2-4} 
                                  &  \multirow{6}{*}{Type}                 & C3D   & Commercial 3D memory                \\
                                %   &                                       & DIMM    &  Dual in-line memory module                      \\
                                  &                                       & PCM   & Phase change memory                \\
                                  &                                       & DRAM    & Dynamic random-access memory                      \\
                                  &                                       & SSD     & Flash SSD memory                           \\
                                %   &                                       & LRDIMM & Load-reduce DIMM                   \\ 
                                  \cline{2-4} 
                                  &  \multirow{2}{*}{Integration}                               & US   & Conventional unstacked                         \\&& S   & Stacked using 2.5D or 3D                        \\ \hline
\multirow{10}{*}{\textbf{Processing}}
                                  & \multirow{5}{*}{NMC/Host Unit}       & CPU     & Central processing unit                  \\
                                  &                                       & GPU   & Graphics processing unit                \\
                                  &                                       & FPGA     & Field programmable gate array  \\
                                  &                                       & CGRA     & Coarse-grained reconfigurable architecture  \\                                  &                                       & ACC     & Application specific accelerator  \\
                                  
                                  \cline{2-4} 
                                  & \multirow{3}{*}{Implementation}       & P     & Programmable unit                  \\
                                  &                                       & F     & Fixed function unit                \\
                                  &                                       & R     & Reconfigurable unit                \\ \cline{2-4} 
                                  & \multirow{3}{*}{Granularity}          & I     & Instruction                        \\
                                  &                                       & K     & Kernel                           \\
                                  &                                       & A     & Application                        \\ \cline{2-4} 
                                  & Host Unit                             &      & Type of host unit                  \\ \hline
\multirow{4}{*}{\textbf{Tool}}             & \multirow{3}{*}{Evaluation Technique}&                                        A     & Analytic                           \\& & S     & Simulation                         \\
                                  &                                       & P     & Prototype/Hardware                          \\
                                   \hline
\multirow{3}{*}{\textbf{Interoperability}} & Programming Interface                 & Y/N   & Programming interface support \\ \cline{2-4} 
                                  & \multirow{1}{*}{Cache Coherence}      & Y/N & Mechanism for cache coherence              \\ \cline{2-4} 
                                  & Virtual Memory                        & Y/N   & Virtual memory support             \\ \hline
                                  
\multirow{2}{*}{\textbf{App. Domain}} & Workload                 &  -  & Target application domain for the architecture \\ \cline{2-4} 
                                  & \multirow{1}{*}{Programming model}      & - & Programming model used for the accelerator 
                                     \\ \hline
                               
%{\textbf{App. Domain}}                    & Workload                                && Target application domain for the architecture
%                        \\ \hline

\end{tabular}

\caption{Classification table, and legend for table~\ref{tab:arcClassification}}
\label{tab:arcLegend}
\end{table*}

\end{comment}



\begin{table}[h]
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{10pt}
\caption{Classification metrics that we use to analyze some notable NMC architectures (see Table~\ref{tab:nmc_review/arcClassification}).}
\label{tab:nmc_review/arcLegend}
\centering
\footnotesize
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{l|l|c|l}
\toprule
\textbf{} & \textbf{Property} & \textbf{Abbreviation} & \textbf{Description} \\ \hline
\multirow{11}{*}{\textbf{Memory}} & \multirow{3}{*}{Hierarchy} & MM & Main memory \\
 &  & SCM & Storage class memory \\
 &  & HM & Heterogenous memory \\ \cline{2-4} 
 & \multirow{6}{*}{Type} & C3D & Commercial 3D memory \\
%  &  & DIMM & Dual in-line memory module \\
 &  & PCM & Phase change memory \\
 &  & DRAM & Dynamic random-access memory \\
 &  & \acrshort{ssd} & Solid-state drive \\
%  &  & LRDIMM & Load-reduce DIMM \\ 
 \cline{2-4} 
 & \multirow{2}{*}{Integration} & US & Conventional unstacked \\
 &  & S & Stacked using 2.5D or 3D \\ \hline
\multirow{12}{*}{\textbf{Processing}} & \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}NMC/Host\\ Unit\end{tabular}} & CPU & Central processing unit \\
 &  & GPU & Graphics processing unit \\
 &  & FPGA & Field programmable gate array \\
 &  & \acrshort{cgra} & \begin{tabular}[c]{@{}l@{}}Coarse-grained reconfigurable \\ architecture\end{tabular} \\
 &  & ACC & Application-specific accelerator \\ \cline{2-4} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Implemen-\\ tation\end{tabular}} & P & Programmable unit \\
 &  & F & Fixed-function unit \\
 &  & R & Reconfigurable unit \\ \cline{2-4} 
 & \multirow{3}{*}{Granularity} & I & Instruction \\
 &  & K & Kernel \\
 &  & A & Application \\ \cline{2-4} 
 & Host Unit &  & Type of the host unit \\ \hline
\multirow{3}{*}{\textbf{Tool}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Evaluation \\ Technique\end{tabular}} & A & Analytic \\
 &  & S & Simulation \\
 &  & P & Prototype/Hardware \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Interop-\\ erability\end{tabular}}} & \begin{tabular}[c]{@{}l@{}}Programming \\ Model\end{tabular} & - & \begin{tabular}[c]{@{}l@{}}Programming model for \\ NMC unit \end{tabular} \\
 & \begin{tabular}[c]{@{}l@{}}Memory Coherence\end{tabular} & Y/N & Mechanism for memory coherence \\
 & \begin{tabular}[c]{@{}l@{}}Virtual Memory\end{tabular} & Y/N & Virtual memory support \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Application \\ Domain\end{tabular}} & Workload & - & \begin{tabular}[c]{@{}l@{}}Target application domain \\ for the architecture\end{tabular} \\ \bottomrule
\end{tabular}
}

\end{table}

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/Conclusion.tex <==
\section{Conclusion}
% In this work we proposed a resource utilization predictor for ML application. We used HLS synthesis report for 2 possible precisions and were able to predict the resource predictions for bitwidth less than 32. Our model was able to predict the resource utilization in FPGA for 9 CNN model with average accuracy of 86\%. We also observed 98\% reduction in runtime after implementing our approach compared to the traditional FPGA design cycle. Our model was also able to provide Pareto-Optimal solution for bitwidth with respect to Power and Accuracy. In conclusion, our method is able to reduce significant design exploration time by providing Optimal bitwidth prediction for fixed point data type. 

In this appendix, we propose \namePaper, a resource and power prediction framework for the exploration of  fixed-point representation on an FPGA.  \linebreak \namePaper~uses high-level synthesis results for only two fixed-point configurations to predict the post-implementation power and resource utilization for all possible fixed-point configurations. While predicting the post-implementation results, \linebreak\namePaper~takes into account the effect of resource saturation and provides a Pareto-optimal configuration in terms of power consumption and error.  We show that  \namePaper can provide accurate estimates of resource utilization and power consumption with up to three orders of magnitude reduction in design space exploration time. In the future, we aim to extend \namePaper to quantize the activations of a neural network and further examine our approach for other application domains.


% We show by experiment that our approach reduces the design-space exploration time, on average, by $674\times$ compared to an exhaustive search for 8 neural-network architectures. \namePaper  leads to, on average, a prediction error of $4.40\%, 4.30\%, 4.04\%,$ and $4.21\%$ for FF, LUT, BRAM, and DSP, respectively with a power consumption prediction error of less than 4\% for all the considered models.



==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/Motivation.tex <==
\vspace{-0.15 cm}
\section{Motivation}\label{preciseFPGA/motivation}

In fixed-point representation (see Section~\ref{sec:low_precision/methodology}), % for a \bitwidth of size N, with only one bit dedicated to the fractional values, the number of possible configurations are $(N-1)$. 
the feasible fixed-point configuration  $<x,y>$ for bit-width $\leq N$ can be represented by Equation~\ref{preciseFPGA/eq1}, where $x$ is the total \bitwidth including $y$ integer bits.  In general, the total number of fixed-point configurations can be given by Equation~\ref{preciseFPGA/eq2}. 

\begin{equation}\label{preciseFPGA/eq1}
x \leq N \quad \forall x \in [2, N] \quad \forall y \in [1, x-1] 
\end{equation}
\vspace{-0.5 cm}
\begin{equation}\label{preciseFPGA/eq2}
 S = \frac{N(N-1)}{2}
\end{equation}
% \vspace{-0.2 cm}

 As we are interested in reduced precision fixed-point configurations, we restrict the maximum \bitwidth to the default \bitwidth of our baseline single-precision floating-point representation, i.e., 32-bit. An exhaustive search to obtain an optimal fixed-point configuration requires post-implementation resource and power estimates for all possible configurations. Therefore, with a \bitwidth of 32, we would need 496 FPGA downstream mapping runs (using Equation~\ref{preciseFPGA/eq2}) to complete an exhaustive search. We have discussed different number systems, which include fixed-point, floating-point, and posit, in Chapter~\ref{chapter:low_precision_stencil}.


To motivate the need for \namePaper, we perform three experiments to study the behavior of an NN model with different fixed-point precision configurations.

\subsection{Effect on Power Consumption}
{Figure~\ref{preciseFPGA/fig_power}} shows the power consumption of the LeNet-5~\cite{lecun2015lenet, lenet_code} convolutional  neural network (CNN) model using different \bitwidth. We analyze the impact on the post-implementation power consumption using all possible fixed-point configurations (\tikzcircle[fill=navyblue]{3pt}). We use Equation~\ref{preciseFPGA/eq1} to enumerate all possible fixed-point configuration options. We draw two conclusions from Figure~\ref{preciseFPGA/fig_power}. First, the power consumption increases with increasing \bitwidth. Second, the maximum power consumption is given by floating-point (\crule[red]{0.2cm}{0.2cm})  with a \bitwidth of 32.
% We used widely used LeNet-5\cite{lecun2015lenet} model architecture in our experiment. We used the Xilinx HLS implementation of Lenet-5 architecture from\ToDo{add link of the github code}. We customized the data type to fixed-point for the NN weights. We ran the entire design cycle for 496 configurations starting from $<2,1>$ to $<32,31>$. We also implemented C-Simulation for these 496 configurations to obtain the accuracy metrics. 

%  \vspace{-0.8 cm}
\begin{figure}[h!]
  \centering
\includegraphics[width=0.8\linewidth,trim={0cm 0cm 0cm 0.7cm},clip]{PreciseNN/sections/figures/motivation/motivationpowergagan.pdf}
\caption{Power consumption with change in \bitwidth for LeNet-5~\cite{lecun2015lenet, lenet_code}.}\label{preciseFPGA/fig_power}
 \end{figure}
 
\subsection{Effect on Inference Accuracy}\label{preciseFPGA/motivation_inference_accuracy_loss}
We also studied the impact of different fixed-point configurations on inference accuracy compared to our baseline 32-bit floating-point by following the approach in Section~\ref{sec:low_precision/methodology}. We use the percentage accuracy drop of a fixed-point configuration with respect to floating-point implementation as an error metric. We calculated the error for all possible 496 fixed-point configurations using the C-simulation results.  We plot the maximum ($\mathbin{\color{red}\blacklozenge}$) and the minimum  ($\tikzcircle[fill=forestgreen]{3pt}$) error (\%) of the fixed-point configurations with respect to \bitwidth in Figure~\ref{preciseFPGA/fig_error}.
We draw two conclusions from Figure~\ref{preciseFPGA/fig_error}. First, increasing the \bitwidth only does not reduce the error. To find the right \bitwidth, we need to find both the appropriate \integer and the \fractional part. Second, increasing the \bitwidth beyond a certain point does not significantly improve accuracy but drastically increases the power consumption. For LeNet-5, we found the optimum \bitwidth, in terms of power consumption and accuracy, at $<14,2>$. 
% \end{enumerate}
% \vspace{-0.8 cm}
 \begin{figure}[h!]
  \centering
\includegraphics[width=0.8\linewidth,trim={0cm 0cm 0cm 0.6cm},clip]{PreciseNN/sections/figures/motivation/motivationerrorgagan.pdf}
\caption{Error in the inference accuracy of LeNet-5~\cite{lecun2015lenet, lenet_code}. To find the optimum \bitwidth that minimizes the error without a drastic increase in power consumption, we need to determine both the \integer and the \fractional part of a fixed-point configuration.}\label{preciseFPGA/fig_error}
 \end{figure}

\subsection{Design Space Exploration Time}
While designing an efficient FPGA-based implementation, our goal is to find a Pareto-optimal configuration with respect to power and accuracy. The Pareto-Optimal configuration can vary according to the power budgets and accuracy requirements of a model.  In Figure~\ref{preciseFPGA/fig_power}, we observe that the optimal configuration is obtained at $<14,2>$ ($\mathbin{\color{forestgreen}\blacklozenge}$), and using a \bitwidth beyond 14 does not add much to the accuracy (see Figure~\ref{preciseFPGA/fig_error}) but increases the power consumption linearly. This Pareto-optimal point enables $\sim$55\% savings in terms of power with only a 4\% loss in accuracy compared to a full-precision floating-point implementation. 

However, to achieve this Pareto-optimal design point, we have to perform an exhaustive search for all design options. In the case of LeNet-5 architecture, it took us nearly five days to get the post-implementation results for all possible 496 configurations. This runtime is impractical, and it prohibits us from an effective design-space exploration. Therefore, we require a fast and accurate framework to explore the optimum fixed-point configuration that does not require post-implementation results for all possible configurations. This motivated us to create \namePaper, which can predict the post-implementation resource and power consumption for fixed-point configurations using only C-Synthesis results of two fixed-point configurations.  %Experimental results demonstrate that \namePaper~delivers,  on  average,  95\%  accuracy in predicting the post-implementation results  and  reduces  the design-space exploration time by ${500\times}$ compared to an exhaustive search.



==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/Related_Works.tex <==
\vspace{-0.15 cm}
\section{Related Work}
In this section, we discuss related work that makes use of prediction and analytic-based techniques to overcome the productivity issue with FPGAs. 

\noindent\textbf{ML-based.} HLSPredict~\cite{o2018hlspredict} estimates pre-implementation resource utilization using program-counters (PC) available in off-the-shelf CPU-based processors. As the PC of a processor is used, arbitrary precision cannot be evaluated using this method. Additionally, pre-implementation resource estimation deviates dramatically compared to post-implementation results~\cite{dai2018fast}. Works such as
% Y.Lecun \textit{et al.}~
~\cite{dai2018fast}, Pyramid\cite{Pyramid}, and Minerva~\cite{Minerva} predict post-implementation resource utilization using an ML framework. However, these frameworks require C-Synthesis~\cite{xilinx_hls} run results for all possible fixed-point configurations, which is a time-consuming process. 

\noindent\textbf{Analytic-based.} Frameworks such as Lin-Analyzer~\cite{linAnalyzer} and HLSCope+~\cite{hls_scope} predict performance metrics for applications using an analytic-based approach. These works do not take into the effect of different fixed-point precision configurations. FINN~\cite{FINN} targets quantized NNs to generate dataflow style architectures for the network. However, these frameworks do not predict post-implementation resource utilization or power prediction for all possible fixed-point configurations. 

ApproxFPGAs~\cite{approxfpgas} is an ML framework that analyzes ASIC-based approximate circuits (ACs) to determine a set of Pareto-optimal FPGA-based designs with respect to power and performance. This framework is specialized only for ASIC-based ACs. Hence, it cannot be generalized for other applications. Additionally, this framework does not predict post-implementation DSP, BRAM, LUT, and FF utilization.

Compared to \namePaper, none of the above frameworks incorporates the resource bound of a particular FPGA device. For example, if BRAM or DSP is exhausted,  how can it  be mapped to the slice logic is a question not answered by those frameworks. Hence, to our knowledge, \namePaper~is the only framework that: (1) predicts post-implementation power and resource utilization for all fixed-point configurations with only two C-Synthesis~\cite{xilinx_hls} run results, and (2) \namePaper~takes into account the heterogeneity of FPGA by mapping the logic to other possible components when any of the components is exhausted.

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/Results.tex <==
\vspace{-0.1 cm}
\section{Evaluation}

We evaluate our proposed method with LeNet-5~\cite{lecun2015lenet, lenet_code}-based CNN architecture. A CNN model consists of a combination of convolution layers, activation layers, fully-connected layers, and pooling layers~\cite{CNN}.   We vary the number of layers and dimensions of each layer of a CNN model to obtain 8 different NN architectures that have an impact on all the FPGA resource types, i.e., FF, LUT, BRAM, and DSP. Table-\ref{table_results} shows the number of parameters of each CNN model used in our evaluation. We use the Xilinx Vivado HLS 2019.1~\cite{xilinx_hls_Design_hub} tool to implement CNN designs targeted for the Zynq-7z020~\cite{xilinx_zynq} edge FPGA-based device. To predict the post-implementation resources and power utilization of a particular model, we use that specific model as the test set and exclude that model from the training and validation set. From the remaining set of 7 models, we randomly choose 6 models for training and 1 model for validation.

% \vspace{-0.15 cm}
% \subsection{ML Training}\label{ML_training}
% To predict the post-implementation resources and power utilization of a particular model, we use that specific model as the test set and exclude that model from the training and validation set. From the remaining set of 7 models, we randomly choose 6 models for training and 1 model for validation. We use \bitwidth, \integer and HLS~\cite{xilinx_hls_Design_hub} estimate features to train SVR~\cite{xyz} model for FF and LUT. For power predictor, we use FF, LUT, BRAM and DSP count as the features to train the SVR~\cite{xyz} model.

% \vspace{-0.15 cm}
% \vspace{-0.3 cm}
\subsection{Resource and Power Prediction}\label{results_pred}
%$<17,8>$ and $<16,10>$
For each model, we obtain C-Synthesis results for only two fixed-point configurations. We feed these results to our \namePaper~framework and obtain power prediction results for all the possible configurations of a model.

In Table~\ref{table_results}, we mention the total runtime and error results. The time taken to predict power and resource utilization for all possible fixed-point configurations using \namePaper~and Xilinx HLS~\cite{xilinx_hls_Design_hub} are mentioned under the columns \textit{Total Runtime (\namePaper)} and \textit{Total Runtime (HLS)}, respectively. Total time taken by \namePaper~consists of the prediction time of making predictions for all possible fixed-point configurations (496 configurations) and runtime for C-Synthesis~\cite{xilinx_hls} for two distinct precision configurations.  We calculate the \textit{speedup} in time obtained using \namePaper~ instead of the exhaustive search (using the HLS tool) in the column \textit{Total Runtime (Speedup)}. We also mention the average prediction error for resources (FF, BRAM, LUT, and DSP) and power estimates. We calculate the prediction error by averaging the relative error with respect to HLS post-implementation estimates.  

We achieve an average prediction error of $4.40\%, 4.30\%, 4.04\%,$ and $4.21\%$ for FF, LUT, BRAM, and DSP, respectively. We observe \namePaper is, on average, $674\times$ faster than an exhaustive search using HLS. For power prediction, we achieve an error of less than 4\% for all the considered models.

\input{PreciseNN/sections/tables/results}

\subsection{Pareto Curve Generation}
We use the MNIST~\cite{mnist} dataset to obtain the error in a CNN model's inference task under test while using 32-bit floating-point baseline and 496 possible fixed-point configurations. Figure~\ref{plot_pareto} shows the plot for the predicted power using \namePaper and the relative error for each model.  For the prediction error, we calculate the change in relative accuracy of fixed-point implementation compared to the baseline floating-point implementation. The power consumption estimated by \namePaper~ and HLS tool is shown as \textit{Predicted} and \textit{Actual}, respectively. We also show the performance of baseline 32-bit floating-point (\textit{Float}) as well as 16-bit floating point (\textit{Half}) in the plot. The figure also highlights the entire search space (496 configurations) using the points labeled as \textit{All}. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{PreciseNN/sections/figures/paretohalfgagan.pdf}
  \vspace{-0.4 cm}
  \caption{Pareto-Optimal plot of power vs relative error for 8 different architectures of LeNeT-5-based~\cite{lecun2015lenet, lenet_code} CNN model.}
  \label{plot_pareto}
\end{figure}


From the Pareto curve, we make three observations. First, the {\textit{Predicted} Power} faithfully follows the trend of the {\textit{Actual} Power}. Second, after attaining optimal configuration, in terms of power consumption and error, an increase in \bitwidth does not improve the error but drastically increases the power consumption. Third, the optimal configuration enables greater saving in power consumption than the floating-point implementation and higher \bitwidth fixed-point configurations. 


==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/abstract.tex <==

\begin{abstract}

% Edge-devices have hard power, bandwidth, memory, and performance constraints because of which resource-efficient accelerator design is critical to deploy  Machine  Learning solutions on the edge.  Lower precision fixed-point-implementations on FPGAs can provide tremendous resource savings by leveraging the arbitrary-precision capability of an  FPGA. However,   optimal-precision-search in a resource-constrained device is a challenging task because of the huge design-space and the time-consuming FPGA design-cycle. To this end, we propose PreciseNN,  a  novel solution to the optimal-precision-calculation for resource-constrained edge-FPGA devices.  Experimental results show that  PreciseNN delivers,  on average,  95\%  accuracy and reduces the design-space exploration time by $\sim\mathbf{500\times}$ over exhaustive search.
% \jgl{By only reading the abstract it is impossible to understand what this work is about.}
% \jgl{Use this flow: 1. NNs can use fixed-point arithmetic. Reduced precision can be enough. 2. Using reduced fixed-point precisions can be beneficial in edge devices with FPGAs, since they are resource constrained. 3. However, determining the optimal precision is challenging (define what optimal precision means). It requires time-consuming design space exploration. 4. Our key idea is to use an ML-based prediction framework to find what is the optimal precision. 5. We present PreciseNN... 6. Explain results.}
% \arpan{this is not entirely ML based framework. Modified accordingly.}

% \jgl{I've tried to propose a better organization. Use the same flow in the introduction.}

% \arpan{Does this look better?
% Neural  Networks  (NN)  can use lower \gagan{precision} fixed-point \gagan{representation} to perform inference with acceptable accuracy.   Reduced fixed-point precision, compared to floating-point can provide savings in resource and power consumption which can be beneficial to deploy NN models on resource-constrained edge-FPGA-devices. However, finding optimal precision w.r.t. accuracy and power is a  challenging task because of the huge design-space and the time-consuming FPGA design-cycle. Our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle. To this end, we propose PreciseNN, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that PreciseNN delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search.
% }

\gagan{Low precision formats for neural network inference offer a resource-efficient alternative to single-precision floating point implementation. %A reduced precision implementation provides savings in resource and power consumption with minimal accuracy loss. Such implementations can allow for easy deployment of accelerators on resource-constrained FPGA-based edge devices. 
However, determining the optimal precision in terms of accuracy and power is challenging because of the following two reasons: (1) the design space of choices makes it infeasible to perform an exhaustive manual-tuning; and (2) FPGAs have a slow downstream implementation process.  To this end, we propose \namePaper, a novel solution for the optimal-precision-evaluation for edge-FPGA-devices. Our key idea is to use a prediction-based framework to obtain optimal-precision with a reduced design-cycle time to overcome these issues. Experimental results show that \namePaper~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\mathbf{500\times}$ over exhaustive search.  }
% \gagan{Neural  Network  (NN) parameter can be used with reduced \gagan{precision} to perform inference with an acceptable accuracy. A reduced precision implementation provides savings in terms of resource and power consumption. Such implementations can allow for easy deployment of accelerators on edge devices with FPGAs, which  are often constrained by the available computational resources. However, determining the optimal precision in terms of accuracy and power is challenging because of the following two reasons: (1) the design space of choices is infeasible to perform exhaustive manual-tuning; and (2) FPGAs have a slow downstream implementation process. To overcome these issues, our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle time. To this end, we propose \namePaper, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that \namePaper~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search.  }

% \gagan{Fixed point arithmetic for neural network (NN) implementation provides a trade-off
% between  accuracy and  computational complexity. NNs can tolerate lower precision computation that allows for  easy deployment these accelerators in edge devices with FPGAs. These devices are often constrained by the available computational resources. However, determining the optimal precision in terms of accuracy and power is challenging because of following two reasons. First, the design space of choices is infeasible to perform manual-tuning. Second, FPGAs have long downstream implementation process. To overcome these issues, our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle. To this end, we propose PreciseNN, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that PreciseNN delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search. }
\end{abstract}

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/background.tex <==
% \vspace{-0.1 cm}
\section{Background}\label{background}
% \begin{Background}
% \gagan{Deep Neural Networks are used to solve a range of tasks including image processing, speech recognition, and natural language processing. However, these networks require a vast amount of computing resources that limits its applicability. To overcome this issue,  we quantize\cite{fixed-point-compression, quant_han2016deep,quant_zhou2017incremental, fixed-point-hw} these networks to reduced precision, taking advantage of inherent error resilience of deep neural networks. To quantize these networks, we make use of reduced precision fixed-point representation that reduces the resource overhead for these networks. 


% \vspace{-0.1 cm}
% \subsection{Fixed-Point Arithmetic}

% In current computing system, IEEE-754 floating-point representation is used as the \textit{de-facto} standard for real numbers representation~\cite{singh2019low}. The floating-point number consists of mantissa, exponent, and an additional bit for the sign. Floating numbers provide a big dynamic range %that enables its application \todo{change} 
% that enables single data to undergo a long sequence of calculations. 
% On the other hand, the fixed-point number has dedicated a number of bits to represent integer part and fraction part. A commonly used fixed-point configuration is denoted by $<x,y>$ where $x$ represents the \bitwidth and $y$ represents the number of dedicated bits used to represent integer part. Even though floating-point operations are better in providing a better dynamic range compared to fixed-point, many applications do not need this dynamic range. Prior works\cite{cnn_approx, dnn_approx, xilinx_wp_int4, xilinx_wp_int8,singh2019low} have shown that applications such as Convolutional Neural Network (CNN) can work well with 8 bit or lower precision with acceptable error.
% \vspace{-0.1 cm}
% \subsection{Fixed-Point Implementation on FPGA}
% FPGAs are being widely used because of their capability to provide massive parallelism and reconfigurability. FPGAs have limited resources where the application performance is also a function of resource utilization. The number of computational units that can be mapped onto an accelerator is key to exploiting maximum parallelism possible from these FPGA devices. In FPGAs the use of lower precision fixed-point data type can be beneficial in terms of power and resource consumption\cite{xilinx_wp_float_to_fixed}. Compared to floating-point precision, reduced fixed-point has two main advantages. First, fixed-point arithmetic requires lower operand width thus fewer logic units, such as DSP (digital signal processing) units\cite{xilinx_dsp}. Second, reduced precision fixed-point requires smaller \bitwidth thus requiring less memory footprint\cite{guptaetal}\cite{fixed-point-hw}\cite{fixed-point-ternary}. Thus, replacing floating-point by reduced precision fixed-point leads to the reduction in area, power and cost\cite{8bit_approx}. In turn allows us to put more compute units within the same device. %Additionally, floating-point to fixed-point conversion support offered for FPGAs by High-Level Synthesis Tools makes this conversion effortless. \jgl{And these tools can be used in FPGA design?\addressed{yes}}


% Even though reduced fixed-point arithmetic has many advantages over floating-point arithmetic, the inference accuracy of a NN model depends largely on the fixed-point configuration\footnote{An optimal fixed-point configuration for an application is defined as the fixed-point configuration for which the application uses minimum power while keeping the application inference accuracy in acceptable range.}.  On one hand, reducing the \bitwidth can provide significant saving in resources and power but it can have detrimental effect on the inference accuracy (ref. Section~\ref{motivation}). So its critical to obtain the fixed-point configuration that can enable an application to operate at an acceptable error while adhering to memory, power, and resource budgets. 
\vspace{-0.1 cm}
\subsection{FPGA design-cycle}
FPGA design cycle consists of three main stages: (1) C-Synthesis\cite{xilinx_hls}\cite{xilinx_hls_tutorial}; (2) RTL Synthesis\cite{xilinx_synth}; and (3) Implementation\cite{xilinx_impl}. After implementation stage, a bitstream (executable) is generated that can be deployed on an FPGA. At every stage of the design-cycle design report ( Section~\ref{hls_report} ), containing the resource utilization and latency estimates, is generated. 



The most accurate estimates are generated after the final implementation stage, thus are the most reliable results. However, the complete downstream process can take several hours for a single design point. To find the optimal fixed-point configuration for an application we need to exhaustively search over all possible fixed-point configurations. This approach quickly becomes intractable and infeasible in case of FPGAs. For example, to obtain optimal fixed-point configuration compared to baseline floating-point ($bitwidth=32$) we require the post-implementation run results for $bitwidth\leq 32$ and $1\leq integer < 32$, for a total of 496 configurations for a single model. An exhaustive search for all configurations  can  easily take from hours to days to even weeks. Due to this high runtime incurred in the FPGA design cycle, it is not practical to run the entire FPGA design cycle exhaustively to find a Pareto-optimal solution. 

 



 
 %%%%%%%%%%%%%%%%%%%%
%  This requires design exploration in the order of $O(n^2)$ for $bitwidth\leq n$. For an example, in order to obtain optimal configuration for $bitwidth\leq 32$ and $1\leq integer < 32$ we require 496 ( \ref{motivation} )\jgl{Refer to section, not equation\addressed{}}  implementation runs which can take hours to even days. 
 
 
%  In FPGA finding optimal fixed-point configuration for an application requires an exhaustive search through all the possible fixed-point configuration. To search the optimal fixed-point configuration compared to baseline floating point requires exhaustive search over 496 configurations. Thus, in FPGA the search space requires to run 496 implementation runs in total, to obtain the resource utilization and power utilization numbers. Implementation runs in FPGA for these 496 configurations can take significant time which can vary from hours to days to even weeks. Thus, its not practical to perform the exhaustive search to obtain the optimal fixed-point configuration. 



% The logic required to implement a given floating-point operation is more compared to fixed-point arithmetic. \gagan{This causes the floating-point implementation to be costly on hardware resources and from both latency and power aspects. }


% \jgl{Start this section with NNs. Then, talk about floating-point. Then, talk about fixed-point and its benefits. Then, introduce FPGAs and why they can be useful on the edge. Then, say that good FPGA resource exploitation needs fixed-point and finding the optimal precision (define what optimal precision means in the context of FPGA and NNs.\addressed{}}




% \jgl{Any particular example from previous works about these benefits?\arpan{addressed}}




% \end{Background}


==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/introduction.tex <==
\vspace{-0.2 cm}

In Chapter~\ref{chapter:low_precision_stencil}, we demonstrate the benefits of using lower precision datatypes on an FPGA. However, determining the optimal fixed-point precision in terms of accuracy and power on an FPGA is challenging because of the following two reasons: (1) the design space of choices makes it infeasible to perform an exhaustive manual-tuning; and (2) FPGAs have a slow downstream mapping process.  To this end, this appendix presents {\namePaper}, our preliminary work on building an automated solution for fixed-point precision evaluation for FPGA-based devices, which overcomes the aforementioned issues. %Experimental results show that \namePaper~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\mathbf{500\times}$ over exhaustive search.  

\section{Introduction}

%FPGAs offer an attractive platform for fixed-point implementation. 
Fixed-point data types have been used for energy-efficient computing in various applications~\cite{guptaetal,cnn_approx,8bit_approx}. For a fixed-point configuration, the impact on accuracy, throughput, power, and resource utilization depends largely on its chosen configuration. A random selection of a fixed-point configuration can have a detrimental effect on the accuracy without significant gains in terms of area and power. Therefore, application-aware fixed-point configuration selection is critical to obtain an optimal solution in terms of resource/power consumption without compromising the accuracy.

An FPGA allows us to implement any arbitrary precision fixed-point configuration. However, the number of precision options leads to a very large design space that is infeasible to explore exhaustively on an FPGA because of its time-consuming design cycle. Recently, FPGA designers have started to adopt high-level synthesis (HLS)~\cite{xilinx_hls_Design_hub} to increase productivity with reduced time-to-market. HLS converts a C/C++ program into register-transfer logic (RTL) that is further synthesized and mapped to a target FPGA. This complete downstream process can take several hours for a single design point~\cite{dai2018fast}. Hence, it is impossible to enumerate all possible fixed-point precision choices and exhaustively search for the optimal design that offers low resource consumption while considering the hardware mapping constraints. 


\textbf{Our key idea} is to develop an automated framework to obtain an application-aware optimal fixed-point configuration without exhaustively searching the entire design space while taking into account the mapping constraints of an FPGA. To this end, we propose \namePaper~- a resource and power estimation framework for arbitrary fixed-point data precision. 
%\addressed{}As we are considering the reduced precision, we have kept the search space for $bitwidth \leq  32$(default floating-point bitwidth). \addressed{}PreciseNN uses FPGA resource architecture aware heuristic (\ref{overview}) method to predict the resource utilization. As FPGA design cycle includes optimizations in each design step, the resource utilization estimates obtained from the heuristic method deviates from the post-implementation resource estimates. In order to accommodate the deviation in the resource estimates caused by these FPGA design steps, PreciseNN uses Machine learning method namely Support Vector Regression(SVR) to predict the resource utilization for post-implementation phase using the utilization results obtained from the heuristic method. 
\namePaper~requires HLS C-Synthesis results from {only two} fixed-point configurations (see Section~\ref{subsec:preciseFPGA/func_detec}) to provide a Pareto-optimal post-implementation solution with respect to power and error. \namePaper~uses these two C-Synthesis utilization reports to obtain the relation between the operation-width of FPGA components and the fixed-point configuration. 
% \addressed{We are using floating point data as a standard, thus, we are evaluating the fixed-point configurations with $bitwidth \leq 32$ }. 
The extracted relation is extrapolated to obtain operation-width for all possible configurations. Compared to previous works~\cite{o2018hlspredict,Pyramid,linAnalyzer,hls_scope,kao2020confuciux}, \namePaper~provides the following key capability. \namePaper is aware of the effect of FPGA-resource saturation, e.g., in case if we saturate digital signal processing (\acrshort{dsp}) units then our framework would map operands to a lookup table (\acrshort{lut}), which makes our approach more practical. We demonstrate our approach by quantizing weights of a neural network (\acrshort{nn})-based accelerator.
%Note: our approach is equally applicable to other application where the control flow remains constant with change in fixed-point configuration (\textit{ref.} Section~\ref{preciseFPGA/overview}); however, in this chapter, we demonstrate our approach with neural networks.



% Recent years have seen a dramatic increase in the use of neural networks to solve various challenging tasks.\cite{near_human_1,near_human_2,near_human_3,near_human1,near_human2}. While we strive to build more accurate \gagan{and robust} NN models, these models are becoming more computationally expensive\cite{yang2017designing}. This limits their deployment on resource constrained  devices such as edge platforms that have strict resource limits. Previous works \cite{guptaetal,power_reduction,int8} have shown that in deep learning inference, floating-point representation is not necessary to obtain an acceptable level of accuracy. Replacing floating-point with a fixed-point representation and further computing at a lower precision could bring large performance gains with minimal loss in accuracy\cite{int8,xilinx_wp_int4}. Fixed-point implementation requires a lower number of bits to perform the same amount of computation as floating-point implementation that helps reducing the resource requirements. 
% % \jgl{Briefly mention the advantages of fixed-point wrt edge FPGA design.}

% Although fixed-point data types have proven to be successful in many applications\cite{guptaetal,cnn_approx,8bit_approx}, their impact on accuracy, throughput, power, and resource utilization depends largely on its used configuration.  Random selection of a fixed-point configuration can have a detrimental effect on the accuracy without significant gains in terms of area and power. Therefore, application-aware fixed-point configuration selection is critical to obtain an optimal solution in terms of resource consumption without compromising on accuracy.

% FPGAs offer an attractive platform for fixed-point implementation. An FPGA allows us to implement arbitrary precision fixed-point implementations. However, the amount of arbitrary precision choices leads to a huge design exploration space that is infeasible to explore on an FPGA because of its time-consuming design cycle. The FPGA design cycle starts with a high-level synthesis (HLS\cite{xilinx_hls_Design_hub}) program that is synthesized and implemented to generate a bitstream for a target FPGA. This complete process can take several hours for a single design point~\cite{dai2018fast}. Therefore, to enumerate for all possible fixed-point precision choices and exhaustively search for the optimal design that offers low resource consumption while satisfying hardware constraints is impossible. 


% Our key idea is to use machine learning (ML) to obtain an application-aware optimal fixed-point configuration that is able to meet the strict resource constraints without exhaustively searching the entire design space. In this paper, we propose \namePaper~- a resource and power prediction framework for arbitrary \gagan{data} precision. 
 
% \namePaper~requires HLS\cite{xilinx_hls_Design_hub} C-Synthesis\cite{xilinx_hls} results from \gagan{only two randomly-selected} fixed-point configurations to provide a Pareto-optimal solution with respect to power and error. \namePaper~uses two C-Synthesis\cite{xilinx_hls} utilization report to obtain the relation between the operation-width and the used fixed-point configuration. 
% % \addressed{We are using floating point data as a standard, thus, we are evaluating the fixed-point configurations with $bitwidth \leq 32$ }. 
% The extracted relation is extrapolated to obtain operation-width for all the possible configurations. Compared to previous works\cite{hls_predict}\cite{Pyramid}\cite{lin_analyzer}\cite{hls_scope}\cite{kao2020confuciux}, \namePaper~provides two key capabilities: (1) the ability to find the Pareto-optimal solution for resource-constrained edge devices; and (2) it is aware of the effect of FPGA-resource saturation.



% In this paper, we make the following contributions:
% % \setlist{nolistsep}
% \begin{enumerate}
% \setlength{\itemsep}{0pt}
% \setlength{\parskip}{3pt}
% \setlength{\parsep}{0pt}
% \item We propose \namePaper, a new resource prediction framework for resource-constrained FPGA-based edge devices taking into account the effect of FPGA-resource saturation for neural network (NN) inference.

% % delivering, \gagan{on average}, resource prediction accuracy of 95\% and reduction in design cycle by .

% \item \namePaper~allows us to predict post-implementation FPGA power and resource utilization for NNs with an average accuracy of 96\% and 95\%, respectively.
% \item We show \namePaper~can provide highly accurate Pareto-Optimal implementation by using only C-Synthesis\cite{xilinx_hls} results of two \random~ fixed point configurations. \namePaper~reduces design-space exploration time by ${500\times}$ compared to an exhaustive search.

% \end{enumerate}
% \vspace{-0.1cm}



==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/methods.tex <==
\vspace{-0.1 cm}
\section{\namePaper}\label{preciseFPGA/overview}
% \begin{PreciseNN}
% \arpan{
\namePaper~is a resource and power estimation framework for fixed-point precision arithmetic targeting Xilinx HLS~\cite{xilinx_hls_Design_hub} designs. \namePaper~uses two realistic assumptions. First, the change in precision does not affect the control path, which means the number of operations in the application is not varied with the change in precision. Second, the operand-width associated with the precision arithmetic changes linearly with the change in the fixed-point configuration. In this section, we describe the main components of \namePaper. First, we give an overview (Section~\ref{subsection:preciseFPGA/overview}) of our framework. Second, we mention the HLS-based features that vary with change in fixed-point configuration (Section~\ref{preciseFPGA/hls_report}). Third, we describe the two most important blocks of \namePaper: (1) function detector and feature predictor (Section~\ref{subsec:preciseFPGA/func_detec}) and (2) resource and power predictor (Section~\ref{subsec:preciseFPGA/resource_predic}). 
\vspace{-0.2 cm}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.9\textwidth]{PreciseNN/sections/figures/Untitledpresentation1.pdf}
    \caption{Overiew of \namePaper.}
    \label{preciseFPGA/block_diagram}
\end{figure}
\vspace{-0.7 cm}
\subsection{Overview}
\label{subsection:preciseFPGA/overview}
% \jgl{Start the overview enumerating what are the main components, and briefly what is their goal and how they are connected.}
% \arpan{
The C-Synthesis results of a C++ application obtained for two fixed-point precision configurations (\circled{1} in Figure \ref{preciseFPGA/block_diagram}) are fed through a \emph{feature extractor} block (\circled{2} in Figure \ref{preciseFPGA/block_diagram}). We extract all resource and timing-based features from the synthesis and the implementation reports. % The {Feature-Extractor} block arranges the instances reported in the HLS~\cite{xilinx_hls_Design_hub} C-Synthesis~\cite{xilinx_hls} report and  extracts the features of these instances with the help of the RTL sourcecode and the C-Synthesis~\cite{xilinx_hls}report.
The \emph{function detector} (\circled{3} in Figure \ref{preciseFPGA/block_diagram}) uses the features extracted from the {feature extractor} to calculate offsets $\mathbf{\hat{x}}$, $\mathbf{\hat{y}}$, and $\mathbf{\hat{x}-\hat{y}}$ of each instance~\footnote{Instance refers to the functions or operators in a design.} for each of the two fixed-point configurations. We compare the calculated offsets of the two configurations to find a common offset function. This common function represents the relation of \bitwidth with an instance.


The \emph{feature predictor} block (\circled{4} in Figure~\ref{preciseFPGA/block_diagram}) uses the identified common functions to generate the feature values for all instances of all possible fixed-point configurations $<x_i,y_i>$. The {resource predictor} block (\circled{5} in Figure \ref{preciseFPGA/block_diagram}) uses the features generated from the {feature predictor} to predict the post-implementation resource utilization for all possible fixed-point configurations. The \emph{power predictor} block (\circled{6} in Figure \ref{preciseFPGA/block_diagram}) uses the resource estimates obtained from the resource predictor to obtain the post-implementation power prediction using a regression model called the Support Vector Regression (SVR)\cite{xyz}. The {power predictor} output along with the C-Simulation (\circled{7} in Figure \ref{preciseFPGA/block_diagram}) is used to obtain a Pareto-optimal fixed-point configuration (\circled{8} in Figure \ref{preciseFPGA/block_diagram}) with respect to power and error in an inference task. We further explain the above steps in the following sections.



% \subsubsection{HLS-based features} \label{hls_report}
% Xilinx HLS tool transforms a C specification into a register transfer level (RTL) implementation using C-Synthesis step. In our framework, we use the reports and the RTL sourcecode generated as the output of the C-Synthesis step of the FPGA design cycle to predict the post-implementation resource and power consumption. We have captured the important components(Comp.) of the HLS report in the first four columns of the Table-\ref{table_hls_report}. 
% \input{sections/tables/hls_report}
% C-Synthesis report captures the variables mapped to FPGA resources under five main categories Comp. (components) listed in Table~\ref{table_hls_report}. First, \textbf{DSP}-Multiply-and-Accumulate (MAC) and Multiplication (MUL) operation instances above a certain operand-width is mapped to the DSP slices is reported under DSP components. The operand-width of a DSP instance is extracted from the respective RTL sourcecode generated from the C-Synthesis. Second, \textbf{Memory}-Memory instances mapped to BRAM components or slice logic is reported along with its attributes namely Bits or width, Words or depth, Number of banks properties. Third, \textbf{Expressions(Expr)}-The variables responsible for logical and arithmetic operation are listed with their operand widths and operation type.  Fourth, \textbf{Multiplexer (MUX)}-This section includes the selector instances with the number of inputs and input bit width. Fifth, \textbf{Register (Reg)} - The variables mapped to storage excluding the memory instances are listed under this section.

% \subsubsection{Features}
% Xilinx HLS C-Synthesis utilization reports the components listed in Table-\ref{table_hls_report}. 
% The features expected to change with change in precision type is marked with \cmark and others with \xmark in the Status column. Each component listed affects the utilization count of the resources listed is marked with \cmark and the ones unaffected is marked with \xmark. Taking an example, Memory can be defined by height, width as well as number of banks. These are reported under Features 1,2 and 3 respectively. Changing precision will affect the memory width only as height depends on array size and banks depends on the access type. Thus, the Status has \xmark for depth and bank and \cmark for width. In an FPGA Memory can be mapped to BRAM or LUT and FF. Thus these components have a \cmark and DSP is marked with \xmark as its count is not affected by modifying memory features.
\vspace{-0.1 cm}
 
\subsection{HLS-based Features} \label{preciseFPGA/hls_report}
The Xilinx HLS tool transforms a C/C++ specification into a register transfer level (RTL) implementation using a C-Synthesis step. Our framework uses the reports and the RTL source code (generated in the C-Synthesis step of the FPGA design cycle) to predict the post-implementation resource and power consumption. 

We mention the important components of the HLS report in Table-\ref{preciseFPGA/table_hls_report}. A C-Synthesis report captures the variables mapped to FPGA resources under five main categories (``Comp''). First, \textbf{Memory} represents instances mapped to block RAM (BRAM) or slice logic (i.e., FF and LUT) and is reported along with its three features, i.e., depth or words, width or bits, and banks. \gthesis{The bank depends on the memory ports.}  Second, 
\textbf{Expression (Expr)} represents the variables responsible for logical and arithmetic operations and lists their operand widths and operation type.  Third, \textbf{Multiplexer (MUX)} includes the selector instances with the number of inputs and input \bitwidth. Fourth, \textbf{DSP} describes multiply-accumulate (MAC) and multiplication (MUL) operation instances above a certain operand-width that are mapped to DSP slices. The operand-width of a DSP instance is extracted from the respective RTL source code generated from the C-Synthesis step. Fifth, \textbf{Register (Reg)} is implemented using flip-flop and stores the results of a look-up table.
\input{PreciseNN/sections/tables/hls_report}
\textbf{Precision dependent features:} 
The features expected to change with change in precision type are marked with \cmark~and others with \xmark~in the \emph{Status} column of Table-\ref{preciseFPGA/table_hls_report}. % Each component listed affects the utilization count of the resources listed is marked with \cmark~and the ones unaffected is marked with \xmark~. 
For example, as mentioned above, for the {Memory} component, HLS reports define memory in terms of depth, width, and banks. %These are reported under Features 1, 2 and 3 respectively. 
A change in the fixed-point precision would affect the memory width only because the depth depends on the array size and banks depend on the access type (i.e., a single-port or a double-port). Thus, the \emph{Status} has \xmark~for depth and bank, and \cmark~for width. In FPGA, we can use \acrshort{bram} or LUT and FF to implement the memory component. Thus, these components have a \cmark~ while DSP is marked with \xmark~as we cannot use DSP to implement a memory.

\vspace{-0.15 cm}
\subsection{Function Detector and Feature Predictor}
\label{subsec:preciseFPGA/func_detec}
% \arpan{
%   
We require C-Synthesis reports of only two  fixed-point configurations (for example $<x_1,y_1>$ and $<x_2,y_2>$) to determine if a feature is fixed or varies with a change in precision. As mentioned before, an instance that is a part of the control-flow, such as loop count, is expected to remain constant, whereas an instance involving fixed-point operands would change with a change in data width precision. 

The features extracted for an application with precision configurations $<x_1,y_1>$ and $<x_2,y_2>$ are given as an input to the {function detector} block (\circled{3} in Figure \ref{preciseFPGA/block_diagram}). The function detector uses two steps. In the first step, the offset between the feature \emph{value}\footnote{Value refers to HLS reported output of an instance's feature, which belongs to a specific component (see Table~\ref{preciseFPGA/table_hls_report}) i.e, memory, expression, multiplexer, DSP, or register. } and \texttt{bitwidth}, \texttt{integer}, and \texttt{fraction} part of a fixed-point representation for both  $<x_1,y_1>$ and  $<x_2,y_2>$ configurations is calculated separately.  This offset captures the relation between feature value and different components of the number representation, i.e., \texttt{bitwidth}, \texttt{integer}, and \texttt{fraction}. The calculated offsets are mentioned under columns $\mathbf{\hat{x}, \hat{y}}$, and $\mathbf{\hat{x}-\hat{y}}$ for each of the two configurations. We obtain these offsets by subtracting \texttt{bitwidth}, \texttt{integer}, and \texttt{fraction} part of a fixed-point representation  from the obtained \emph{Value} of an instance's feature, respectively.   

To understand the relationship between an instance of an application and the \texttt{bitwidth, integer}, and \texttt{fraction} part of a fixed-point representation, we need to ensure that the two chosen fixed-point configurations follow the conditions given by Equation~\ref{preciseFPGA/unique}
\vspace{-0.2 cm}
\begin{equation}\label{preciseFPGA/unique}
    x_{1}\not=x_{2} \quad \text{and} \quad y_{1}\not=y_{2} \quad \text{and} \quad (x_{1}-y_{1})\not=(x_{2}-y_{2})
\end{equation}
\vspace{-0.7 cm}


In the second step, the offsets obtained in the first step for two different fixed-point precision configurations are compared to find a common matching offset function, which we refer to it as \emph{function detected}. In the case of a match, the \emph{function detected} is replaced by the common offset function plus the offset's calculated value. In case there is no match, the \emph{function detected} is replaced with 1, which implies that an instance's feature is independent of the chosen data-width and, therefore, remains constant for all the fixed-point configurations.

\textbf{Example:} In Table~\ref{preciseFPGA/table_func_generate_new} we explain the above step using the instances captured from the HLS C-Synthesis report for $<17,8>$ and $<16,10>$ fixed-point configurations for LeNet-5. We report the values achieved by HLS for different features under the \emph{Value} column for each precision. In the case of the \emph{Expression} component with instance name $out\_V\_d0$, we have two features, op1-width and op2-width. First, we calculate the offsets for each feature of the \emph{Expression} component. For each fixed-point precision configuration, we mention the calculated offsets under $\mathbf{\hat{x},  \hat{y}}$, and $\mathbf{\hat{x}-\hat{y}}$. Second, we compare the offsets obtained for the two fixed-point precision configurations to find a common function. In the case of \emph{op1-width}, the offsets obtained for $<x_1,y_1>$ are different than the offsets obtained for $<x_2,y_2>$. However, for op2-width, $\mathbf{\hat{x}}$  with a value of -1 is common between the offsets of the two precision configurations. Thus, the function detected for op1-width and op2-width features are 1 and $\mathbf{\hat{x}-1}$, respectively.

% \input{PreciseNN/sections/tables/PreciseNN}
\input{PreciseNN/sections/tables/preciseNN_new_gagan}
% \input{PreciseNN/sections/tables/preciseNN_new_gagan}
% Let us denote as $\alpha_{cifj}$ feature value of feature f of instance i of component c with fixed-point configuration j is given by . In the first step, this block maps the feature value ($\alpha_{cifj}$) as a function of $<x_j,y_j>$ according to the Equation-\ref{function}. Thus, for each, $\alpha_{cifj}$ we obtain three functions $f(\alpha_{cifj},x_{j}),f(\alpha_{cifj},y_{j})$ and $f(\alpha_{cifj},(x_{j}-y_{j}))$ for each feature $\alpha_{cifj}$ of a component instance for single fixed-point configuration $<x_j,y_j>$. 
% \vspace{-0.05 cm}
% \begin{equation}\label{function}
%     f(\alpha_{cifj},p_{j})=p_{j}+(\alpha_{cifj}-p_{j}) \quad \forall p_{j} \in [x_j,y_j,(x_j-y_j)] 
% \end{equation}
% Using Equation-\ref{function}, the list of functions extracted by the Function Detector for a fixed-point configuration $<x_1,y_1>$ is given by $f(\alpha_{cif1},x_{1}),f(\alpha_{cif1},y_{1}),f(\alpha_{cif1},(x_{1}-y_{1}))$. Similarly, for the fixed-point configuration $<x_2,y_2>$ the extracted functions are $f(\alpha_{cif2},x_{2}),f(\alpha_{cif2},y_{2}),f(\alpha_{cif2},(x_{2}-y_{2}))$ respectively.
% In the second step, the Function Detector identifies the unique function which maps the feature $\alpha_{cifj}$ to the fixed-point configuration $<x_j,y_j>$ from the list of three functions obtained.

% We have performed C-Synthesis for an application for fixed-point configuration $<17,8>$ and  $<16,10>$ and reported few instances of the components from the C-Synthesis report with their value and feature value in Table-\ref{table_func_generate}. Let us use an instance \texttt{out\_V\_d0} of Component Expression to understand the working of the Function Detector. The instance \texttt{out\_V\_d0} has two features namely op1-width and op2-width. The value for feature op1-width obtained from the C-Synthesis report for configurations $<17,8>$ and $<16,10>$ are 1 and 1 respectively. For each fixed-point configuration the $\alpha_{cifj}-x_{j}$, $\alpha_{cifj}-y_{j}$, $\alpha_{cifj}-(x_{j}-y_{j})$ are reported under columns $\mathbf{x}$, $\mathbf{y}$ and $\mathbf{x-y}$ respectively. As the numbers reported for the columns of $\mathbf{x}$, $\mathbf{y}$ and $\mathbf{x-y}$ for $<17,8>$ and $<16,10>$ are different, we conclude that the feature value does not change in accordance to different configurations. Thus, the function detected by the function detector reported in Function Detected column is 1 (same value as under $<17,8>$ or $<16,10>$).
% Similarly, for feature op2-width of the \texttt{out\_V\_d0}, we perform the steps discussed for the op1-width.  We found that $\mathbf{x}$ column for $<17,8>$ and $<16,10>$ has the same value. Thus, the Function Detected obtained for op2-width of \texttt{out\_V\_d0} is $\mathbf{x-1}$ by using Equation-\ref{function}. 


In the \emph{feature prediction} phase, we use the \emph{function detected} to find the value of an instance's feature for all possible fixed-point precision configurations. In Table~\ref{preciseFPGA/table_func_generate_new}, we demonstrate the feature prediction for six different fixed-point configurations (<2,1>, <3,1>, <3,2>, <4,1>, <4,2>, and <4,3>). For each of these configurations, to obtain the feature value of an instance, we replace <x,y> values of a configuration into the \emph{function detected}.

\subsection{Resource and Power Predictor}
\label{subsec:preciseFPGA/resource_predic}
% \arpan{
The {resource predictor} step uses the feature values generated from the {feature predictor} (\circled{4} in Figure \ref{preciseFPGA/block_diagram}) to predict the post-implementation DSP, BRAM, FF, and LUT resource utilization for all possible fixed-point configurations. For each FPGA resource type, we employ a different estimation technique \gthesis{based on the feature complexity}. %In this section we will go through the prediction model used for each resource in detail.

\noindent\textbf{BRAM:} %This uses an architecture-aware heuristic method to obtain the BRAM  consumption for a given memory width, depth, and banks. 
Our target Xilinx FPGA board~\cite{xilinx_zynq} has block RAM resources that store up to 36-Kbits of data and can be configured as either two independent 18-Kbits RAM or one 36-Kbit RAM. Each 18-Kb block RAM can be configured as a 16K x 1, 8K x2 , 4K x 4, 2K x 9, 1K x 18 or 512 x 36 in dual-port mode. For a given  memory instance with width, depth, and banks, our BRAM resource predictor finds the possible BRAM utilization for all possible combinations of the configuration. The BRAM configuration requiring the lowest cascade depth and the lowest BRAM utilization is selected. This process is repeated for all the BRAM instances for the particular fixed-point configuration. Total BRAM count is obtained as the sum over all the BRAM instances. 

\noindent\textbf{FF and LUT}:  FF and LUT estimates vary non-linearly with the feature values. Therefore, for the prediction of the FF and LUT, we use SVR (Support Vector Machine)~\cite{xyz}, which is a simple non-linear machine learning algorithm, to map HLS estimates to post-implementation FF and LUT count. We use the calculated FF, and LUT estimates from the feature predictor step as features to train our SVM model.


\noindent\textbf{DSP:}\label{preciseFPGA/resource_prediction_dsp}
% As we are interested in the reduced-precision, the operand-widths for threse configurations is expected to be small and the size to be limited.
As discussed in Section~\ref{preciseFPGA/hls_report}, MAC and MUL operations above a certain threshold are mapped to the dedicated DSP slices on an FPGA. This threshold value is extracted from the RTL generated in the C-Synthesis step of the HLS design cycle.  There is a linear mapping between the number DSP slices a particular MAC, or MUL operation requires and the operand-width. Therefore, we use operand-width to estimate post-implementation DSP utilization. %We extract this mapping information from t We perform an exhaustive set of operand-width from 1-64 for MAC and MUL operation and their DSP utilization in the post-implementation phase. 

% We performed the entire FPGA design cycle for the MAC and MUL operations for operand width 1 to 64 and stored the DSP utilization obtained in the post-implementation in a lookup-table. The lookup-table maps the operand-width to the DSP utilization for each operation. For each fixed-point configuration, we obtain multiple MAC and MUL instances. We use the op1-width and op2-width generated from the Feature Predictor for each MAC and MUL instance to predict the DSP utilization using the lookup-table for that particular instance. We calculate the total DSP used for a fixed-point configuration as the sum of the DSP utilization obtained for all the MAC and MUL operations. 

 

% \noindent\textbf{FF and LUT}: The prediction for the FF and LUT uses two step approach. In the first step, the features obtained from the feature feature predictor block is mapped to the C-Synthesis~\cite{xilinx_hls} estimates. Lookup table is used to calculate the HLS~\cite{xilinx_hls_Design_hub} C-Synthesis~\cite{xilinx_hls} estimates from the features obtained from the feature predictor. In the second step the predictor uses a ML method SVR~\cite{xyz} to map HLS~\cite{xilinx_hls_Design_hub} estimate to post-implementation FF and LUT count.

% \textbf{Step-1}- In the first step, the features obtained from the feature predictor block is used to obtain the total C-Synthesis HLS prediction for FF and LUT. \textbf{FF}-FF count is affected by three components(Table-\ref{table_hls_report}). First, the  memory resources with lower size and the register components are mapped to the register. In our framework memory instances requiring less than a threshold ($th_{mem}$) bits are mapped to the registers. We obtained this threshold $th_{mem}=1024$ after exhaustive search for memory configurations for width,depth and banks. The limited number of memory resources are mapped to a lookup table to obtain the HLS predicted FF and LUT count for a particular memory configuration. Total FF ($FF_{mem}$) and LUT ($LUT_{mem}$) count for a fixed-point configuration used for memory instances is obtained by summing the FF and LUT requirement over all the instances. Second, the instances reported under registers are mapped to FFs. For each register instance, the FF used is calculated as $(bits - const bits)$. The FFs required for all the instances are added to obtained the FF required for register instances ($FF_{reg}$). Third, for some particular operand width MAC and MUL operation uses FF and LUT. Similar to DSP prediction (\ref{resource_prediction_dsp}), it uses a lookup table to predict the FF and LUT estimate for HLS using the operand width as the input. Total number of FFs and LUT used for these MAC and MUL operation are denoted by $FF_{dsp}$ and $LUT_{dsp}$ respectively, is obtained by summing over all the MAC and MUL operations. Total HLS estimated FF ($FF_{hls}$) for a fixed-point configuration is obtained as $FF_{hls}=FF_{mem}+FF_{reg}+FF_{dsp}$.  \textbf{LUT}- LUT count is affected by four components. First two components are Memory and DSP utilizing LUTs denoted by $LUT_{mem}$ and $LUT_{dsp}$ respectively. Third and fourth component are Multiplexer and Expressions instances. The LUT count for MUX and Expr instances denoted by $LUT_{MUX}$ and $LUT_{Expr}$ also calculated from a lookup table using the features obtained from the Feature Predictor. Total LUT predicted from the HLS viewpoint is $LUT_{hls}=LUT_{mem}+LUT_{dsp}+LUT_{MUX}+LUT_{Expr}.$

% \textbf{Step-2}- In the second step, we use a ML based SVR model to predict the post-implementation FF and LUT utilization using the C-Synthesis HLS prediction result obtained in the first step. We use a set of eight CNN models and obtain the HLS C-Synthesis and post-implementation resource FF and LUT utilization for each 496 configuration. We use randomly 6 models out of 8 to train the SVR model using input features as C-Synthesis resource estimate,\texttt{bitwidth},\texttt{integer} and the output as the post-implementation resource estimate. We use one model as the test data and one model as the validation data. 
% }

\textbf{Power Prediction:} The power prediction step (\circled{6} in Figure \ref{preciseFPGA/block_diagram}) uses the resource estimates obtained from the resource predictor to obtain the post-implementation power prediction for a certain fixed-point configuration. We again use a simple SVM~\cite{xyz} model for power prediction because of the non-linearity between the resource utilization and power consumption. We train a separate SVM-based model for each FPGA resource type, i.e., BRAM, FF, LUT, and DSP.
% \emph{BRAM}-
% Xilinx FPGA BRAM\cite{xilinx_memory_reources} blocks supports some fixed configurations to used as memory. We calculate the number of possible BRAM utilization using the features predicted by the Feature Predictor for every configurations. Then we use a heuristic method to optimize the number of BRAMs using cascade depth. We add the number of BRAMs for all the Instances under memory to obtain the post-implentation BRAM utilization for the respective BRAM utilization.

% \emph{FF and LUT}-
% FF count is contributed by Registers and Memory as listed in Table-\ref{table_hls_report}. Similarly LUT count is affected by the expressions and Multiplexer. The final FF as well as LUT count differs from the value listed in the HLS report due to optimizations in synthesis as well as implementation. We use Support Vector Regression(SVR) to predict the FF and LUT utilization. The SVR model is trained using HLS predicted resource utilization, x and y value as features and post-implementation resource utilization as the output.


% \subsection{Power Predictor}
% Power predictor is also a SVR model which maps the post-implementation resource utilization to Power consumption. The Resource utilization obtained from the Resource Predictor is used as input to Power predictor to obtain the power figures.



==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/tables/PreciseNN.tex <==

% \end{PreciseNN}


 \begin{table*} 
 \HUGE
 \renewcommand{\arraystretch}{0.65}
\setlength{\tabcolsep}{6pt}
 \resizebox{1\linewidth}{!}{%
 \centering
 \begin{tabular}{!{\vrule width 4pt}c!{\vrule width 1pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 4pt}}

  \specialrule{.1em}{.05em}{.05em} 
 \multicolumn{1}{!{\vrule width 4pt}c!{\vrule width 2pt}}{\textbf{Component}}&\multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Instance}} &\textbf{Feature} &\multicolumn{4}{c!{\vrule width 2pt}}{\textbf{\textit{$<$x=17,y=8$>$}}}
& \multicolumn{4}{c!{\vrule width 2pt}}{\textbf{\textit{$<$x=16,y=10$>$}}} &\textbf{Function} &\multicolumn{6}{c!{\vrule width 4pt}}{\textbf{Feature Predicted}}  \\
\cline{4-9}

 \multicolumn{1}{!{\vrule width 4pt}c!{\vrule width 2pt}}{\textbf{Name}} &\multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Name}} & \textbf{Name}  &\textbf{Value}&{$\mathbf{x}$} &\textbf{$\mathbf{y}$} &\textbf{$\mathbf{x-y}$} &\textbf{Value}&\textbf{$\mathbf{x}$} &\textbf{$\mathbf{y}$} &\textbf{$\mathbf{x-y}$} &\textbf{Detected}&\textbf{$\mathbf{<2,1>}$} &\textbf{$\mathbf{<3,1>}$} &\textbf{$\mathbf{<3,2>}$} &\textbf{$\mathbf{<4,1>}$} &\textbf{$\mathbf{<4,2>}$} &\textbf{$\mathbf{<4,3>}$} \\
 \specialrule{.1em}{.05em}{.05em} 
 \multirow{1}{*}{Memory} &C2\_weights\_V\_0\_U  &width &9 &$\mathbf{-8}$ &$\mathbf{+1}$ &$\textbf{0}$ &6 &$\mathbf{-10}$ &$\mathbf{-4}$ &$\mathbf{0}$ &$\mathbf{x-y}$ &1&2&1&3&2&1 \\ 
 \specialrule{.1em}{.05em}{.05em} 
 %%%%%%%%%%%%Expressions%%%%%%%%%%%%%%%%%%%%%
 \multirow{2}{*}{Expression}
 &\multirow{2}{*}{out\_V\_d0}  &op1 width &1 &$\mathbf{-16}$ &$\mathbf{-7}$ &$\mathbf{-8}$ &1 &$\mathbf{-15}$ &$\mathbf{-9}$ &$\mathbf{-5}$ &1 &1 &1 &1 &1 &1 &1 \\
\cline{3-18}
 &&op2 width &16 &$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$&1 &2 &2 &3 &3 &3\\
 \specialrule{.1em}{.05em}{.05em} 
%%-----------------MUX---------------------------
 \multirow{1}{*}{Multiplexer} &p\_Val2\_40\_0\_reg\_412 &Bits &17 &$\mathbf{0}$ &$\mathbf{+9}$ &$\mathbf{+8}$ &16 &$\mathbf{0}$ &$\mathbf{+6}$ &$\mathbf{+10}$ &$\mathbf{x}$&2 &3 &3 &4 &4 &4\\
 \specialrule{.1em}{.05em}{.05em} 
 %%----------------------------DSP------------------------- 
 \multirow{2}{*}{DSP}&\multirow{2}{*}{nnet\_mac\_muladd\_sc4}  &op1 width &16 &$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$ &1 &2 &2 &3 &3 &3 \\
\cline{3-18}
&&op2 width &10&$\mathbf{-7}$ &$\mathbf{+2}$ &$\mathbf{+1}$ &7 &$\mathbf{-9}$ &$\mathbf{-3}$ &$\mathbf{+1}$ &$\mathbf{x-y+1}$&2 &3 &2 &4 &3 &2\\
 % \hline
 \specialrule{.1em}{.05em}{.05em} 
 \multirow{1}{*}{Register}& C2\_weights\_V\_0\_load\_reg\_1181 &Bits &9&$\mathbf{-8}$ &$\mathbf{+1}$ &$\mathbf{0}$&6 &$\mathbf{-10}$ &$\mathbf{-4}$ &$\mathbf{0}$ &$\mathbf{x-y}$&1 &2 &1 &3 &2 &1\\
% \arrayrulecolor{gray}\cline{2-18}
% & in\_V\_load\_reg\_1186 &Bits &16&$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$&1 &2 &2 &3 &3 &3\\
 \specialrule{.1em}{.05em}{.05em} 
 \end{tabular}
 }
\caption{Brief overview of the HLS C-Synthesis report with Function-Detector and Feature-Predictor output}
 \label{preciseFPGA/table_func_generate}
\end{table*}
% \vspace{0.5 cm}

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/tables/hls_report.tex <==
\begin{table}[!htp] 
% \Huge
 \caption{Components and their features extracted from the C-Synthesis report.}
           \label{preciseFPGA/table_hls_report}
\centering
 \resizebox{1\linewidth}{!}{%
\begin{tabular}{ c | c | c | c | c | c |c |c|c}
%  \specialrule{.1em}{.05em}{.05em} 
\toprule
            \multicolumn{1}{c|}{\textbf{Comp}} & {\textbf{Feature1}} & {\textbf{Feature2}} &{\textbf{Feature3}} &{\textbf{Status}} &{\textbf{FF}}&{\textbf{LUT}}&{\textbf{BRAM}}&{\textbf{DSP}}\\ \hline
            % \endhead
            Memory & depth & width & bank  &\xmark, \cmark, \xmark &\cmark &\cmark &\cmark &\xmark \\ \hline
            Expr & op1 width & op2 width & op type  &\cmark, \cmark, \xmark &\xmark &\cmark &\xmark &\cmark\\ \hline
            MUX & ip size & bits & total bits  &\xmark, \cmark, \cmark &\xmark &\cmark &\xmark &\xmark \\ \hline
            DSP & op1 width & op2 width & op3 width  &\cmark, \cmark, \cmark &\cmark &\cmark &\xmark &\cmark \\ \hline
            Reg & variable bits & const bits & N/A  &\cmark, \xmark, \xmark &\cmark &\xmark &\xmark &\xmark \\ \bottomrule
            % \specialrule{.1em}{.05em}{.05em} 
           \end{tabular}
           }
        \end{table}
        

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/tables/preciseNN_new_gagan.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\HUGE
 \renewcommand{\arraystretch}{0.95}
  \caption{Example of an HLS C-Synthesis report with outputs from function-detector and feature-predictor.}
   \centering
 \label{preciseFPGA/table_func_generate_new}
\setlength{\tabcolsep}{6pt}
 \resizebox{1\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Comp\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Instance\\ Name\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Feature\\ Name\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\textless{}x=17, y=8\textgreater{}}} & \multicolumn{4}{c|}{\textbf{\textless{}x=16, y=10\textgreater{}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Function \\ Detected\end{tabular}}} & \multicolumn{6}{c|}{\textbf{Feature Predicted}}                                                                                                                  \\ \cline{4-11} \cline{13-18} 
&                                                                                   &                                                                                  & \textbf{Value}    & \textbf{$\hat{x}$}   & \textbf{$\hat{y}$}   & \textbf{$\hat{x}-\hat{y}$}   & \textbf{Value}    & \textbf{$\hat{x}$}    & \textbf{$\hat{y}$}   & \textbf{$\hat{x} - \hat{y}$}   &                                                                                        & \textbf{\textless{}2,1\textgreater{}} & \textbf{\textless{}3,1\textgreater{}} & \textbf{\textless{}3,2\textgreater{}} & \textbf{\textless{}4,1\textgreater{}} & \textbf{\textless{}4,2\textgreater{}} & \textbf{\textless{}4,3\textgreater{}} \\ \hline
Memory & C2\_weights\_V\_0\_U & width   & 9       & -8   & +1   & 0   & 6   & -10      & -4     & 0       & $\hat{x} - \hat{y}$         & 1         & 2     & 1     & 3        & 2          & 1       \\ \hline
\multirow{2}{*}{Exr}      & \multirow{2}{*}{out\_V\_d0}                                 & op1 width                                                           & 1                 & -16          & -7           & -8             & 1                 & -15           & -9           & -5             & 1                                      & 1                                     & 1                         & 1                & 1      & 1         & 1                          \\ \cline{3-18} 
             &                           & op2 width                           & 16                & -1           & +8           & +7             & 15                & -1            & +5           & +9             & $\hat{x}$-1                                                                                    & 1                                     & 2                                     & 2                                     & 3                                     & 3                                     & 3                                     \\ \hline
MUX                                                                        & p\_Val2\_40\_reg                                                                  & bits                                                                             & 17                & 0            & +9           & +8             & 16                & 0             & +6           & +10            & $\hat{x}$                                                                                      & 2                                     & 3                                     & 3                                     & 4                                     & 4                                     & 4                                     \\ \hline
\multirow{2}{*}{DSP}                                                               & \multirow{2}{*}{nnet\_mac\_muladd}                                                & op1 width                                                                        & 16                & -1           & +8           & +7             & 15                & -1            & +5           & +9             & $\hat{x}$-1                                                                                    & 1                                     & 2                                     & 2                                     & 3                                     & 3                                     & 3                                     \\ \cline{3-18} 
                                                                                   &                                                                                   & op2 width                                                                        & 10                & -7           & +2           & +1             & 7                 & -9            & -3           & +1             & $\hat{x}-\hat{y}$ +1                                                                                  & 2                                     & 3                                     & 2                                     & 4                                     & 3                                     & 2                                     \\ \hline
Reg                                                                           & C2\_weights\_V\_0\_reg                                                            & bits                                                                             & 9                 & -8           & +1           & 0              & 6                 & -10           & -4           & 0              & $\hat{x}-\hat{y}$                                                                                    & 1                                     & 2                                     & 1                                     & 3                                     & 2                                     & 1                                     \\ \bottomrule
\end{tabular}
}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/tables/result_1.tex <==
\begin{table}[h]
\Huge
 \centering
 \resizebox{1\linewidth}{!}{%
 \begin{tabular}{!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c|c|c!{\vrule width 2pt}c|c|c|c|c!{\vrule width 2pt}c!{\vrule width 2pt}}
\specialrule{.1em}{.05em}{.05em} 
\rowcolor{Lightgray}
 \multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{}& & \multicolumn{3}{c!{\vrule width 2pt}}{\textbf{Total Runtime(hrs)}} &  \multicolumn{5}{c!{\vrule width 2pt}}{\textbf{Average Relative Prediction Error(in \%)}}\\
 \cline{3-10}
\rowcolor{Lightgray}
 \multirow{-2}{*}{\textbf{Model}}  &\multirow{-2}{*}{\textbf{\#(Parameters)}}&\textbf{Tool}&\textbf{PreciseNN} &\textbf{Gain(in\%)}&\textbf{FF}&\textbf{LUT}&\textbf{BRAM}&\textbf{DSP} &\textbf{Power}\\
 \specialrule{.1em}{.05em}{.05em} 
1 & 16278 & 223 & 0.205 & 1087 & 3.93 & 4.93 & 3.18 & 4.73 &2.71
\\
\hline
2 & 42704 & 107 & 0.220 & 486 & 4.26 & 3.96 & 2.83 & 4.99 &3.07	
\\
\hline
3 & 14758 & 103 & 0.21 & 490 & 4.65 & 4.24 & 5.44 & 2.89 &2.63\\
\hline
4 & 14822 & 115 & 0.219 & 525 & 4.42 & 3.80 & 5.91 & 3.25 &	2.42	 \\
\hline
5 & 9222 & 111 & 0.223 & 498 & 3.54 & 4.19 & 6.53 & 3.43 &2.64 \\
\hline
6 & 36004 & 132 & 0.227 & 581 & 4.04 & 4.19 & 2.84 & 4.95 &	3.41	\\
\hline
7 & 24114 & 119 & 0.232 & 512 & 6.07 & 4.14 & 2.75 & 4.52 &3.68 \\
\hline
8 & 16498 & 239 & 0.203 & 1177 & 4.24 & 4.92 & 2.89 & 4.92 &	3.72 \\
\specialrule{.1em}{.05em}{.05em} 
\multicolumn{4}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Average}} &\textbf{99.83} &\textbf{4.40} &\textbf{4.30}		&\textbf{4.04}		&\textbf{4.21} &\textbf{3.03
}\\
\specialrule{.1em}{.05em}{.05em} 

 \end{tabular}%
 }
\caption{Model Runtime and Resource Prediction metrics}
 \label{preciseFPGA/table_results}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/PreciseNN/sections/tables/results.tex <==
% \begin{table}[h]
% \Huge
%  \centering
%  \resizebox{1\linewidth}{!}{%
%  \begin{tabular}{!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c|c|c!{\vrule width 2pt}c|c|c|c|c!{\vrule width 2pt}c!{\vrule width 2pt}}
% \specialrule{.1em}{.05em}{.05em} 
% \rowcolor{Lightgray}
%  \multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{}& & \multicolumn{3}{c!{\vrule width 2pt}}{\textbf{Total Runtime(hrs)}} &  \multicolumn{5}{c!{\vrule width 2pt}}{\textbf{Average Relative Prediction Error(in \%)}}\\
%  \cline{3-10}
% \rowcolor{Lightgray}
%  \multirow{-2}{*}{\textbf{Model}}  &\multirow{-2}{*}{\textbf{\#(Parameters)}}&\textbf{Tool}&\textbf{PreciseNN} &\textbf{Gain(in\%)}&\textbf{FF}&\textbf{LUT}&\textbf{BRAM}&\textbf{DSP} &\textbf{Power}\\
%  \specialrule{.1em}{.05em}{.05em} 
% 1 & 16278 & 223 & 0.205 & 99.91 & 3.93 & 4.93 & 3.18 & 4.73 &2.71
% \\
% \hline
% 2 & 42704 & 107 & 0.220 & 99.79 & 4.26 & 3.96 & 2.83 & 4.99 &3.07	
% \\
% \hline
% 3 & 14758 & 103 & 0.21 & 99.79 & 4.65 & 4.24 & 5.44 & 2.89 &2.63\\
% \hline
% 4 & 14822 & 115 & 0.219 & 99.81 & 4.42 & 3.80 & 5.91 & 3.25 &	2.42	 \\
% \hline
% 5 & 9222 & 111 & 0.223 & 99.80 & 3.54 & 4.19 & 6.53 & 3.43 &2.64 \\
% \hline
% 6 & 36004 & 132 & 0.227 & 99.83 & 4.04 & 4.19 & 2.84 & 4.95 &	3.41	\\
% \hline
% 7 & 24114 & 119 & 0.232 & 99.80 & 6.07 & 4.14 & 2.75 & 4.52 &3.68 \\
% \hline
% 8 & 16498 & 239 & 0.203 & 99.91 & 4.24 & 4.92 & 2.89 & 4.92 &	3.72 \\
% \specialrule{.1em}{.05em}{.05em} 
% \multicolumn{4}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Average}} &\textbf{99.83} &\textbf{4.40} &\textbf{4.30}		&\textbf{4.04}		&\textbf{4.21} &\textbf{3.03
% }\\
% \specialrule{.1em}{.05em}{.05em} 

%  \end{tabular}%
%  }
% \caption{Model Runtime and Resource Prediction metrics}
%  \label{table_results}
% \end{table}

\begin{table}[h]
\Huge
 \centering
 \caption{Model runtime and resource prediction results.}
 \label{table_results}
 \resizebox{1\linewidth}{!}{%
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
 \multicolumn{1}{|c|}{}& & \multicolumn{3}{c|}{\textbf{Total Runtime (hrs)}} &  \multicolumn{5}{c|}{\textbf{Average Relative Prediction Error (\%)}}\\
 \cline{3-10}
 \multirow{-2}{*}{\textbf{Model}}  &\multirow{-2}{*}{\textbf{\# Parameters}}&{HLS}&{\namePaper} &{Speedup}&{FF}&{LUT}&{BRAM}&{DSP} &{Power}\\
\hline
1 & 16278 & 223 & 0.205 & 1087 & 3.93 & 4.93 & 3.18 & 4.73 &2.71
\\
\hline
2 & 42704 & 107 & 0.213 & 502 & 4.26 & 3.96 & 2.83 & 4.99 &3.07	
\\
\hline
3 & 14758 & 103 & 0.204 & 505 & 4.65 & 4.24 & 5.44 & 2.89 &2.63\\
\hline
4 & 14822 & 115 & 0.219 & 525 & 4.42 & 3.80 & 5.91 & 3.25 &	2.42	 \\
\hline
5 & 9222 & 111 & 0.221 & 502 & 3.54 & 4.19 & 6.53 & 3.43 &2.64 \\
\hline
6 & 36004 & 132 & 0.227 & 581 & 4.04 & 4.19 & 2.84 & 4.95 &	3.41	\\
\hline
7 & 24114 & 119 & 0.232 & 512 & 6.07 & 4.14 & 2.75 & 4.52 &3.68 \\
\hline
8 & 16498 & 239 & 0.203 & 1177 & 4.24 & 4.92 & 2.89 & 4.92 &	3.72 \\
\hline
\multicolumn{4}{|c|}{\textbf{Average}} &\textbf{673.8} &\textbf{4.40} &\textbf{4.30}		&\textbf{4.04}		&\textbf{4.21} &\textbf{3.03
}
\\
% \specialrule{.1em}{.05em}{.05em} 
\bottomrule
 \end{tabular}%
 }
\end{table}




==> PhD_Thesis_Updated_arxiv (1)/Sibyl/algorithm/rl_algo.tex <==
% \begin{figure*}[b]
%   \centering
% \begin{minipage}{\linewidth}
% \centering
% {\fontsize{4}{10}\selectfont
%  \vspace{-0.3cm}
\setlength{\textfloatsep}{0.1cm}
\setlength{\floatsep}{0.00cm}
% \begin{minipage}{\linewidth}
\begin{algorithm}[h]
\scriptsize
\setstretch{1}
 \caption{\namePaper's \gont{reinforcement learning-based} data placement \gon{algorithm}}
 \label{algo:rl_algo}
 \begin{algorithmic}[1]
 \State \textbf{Intialize:} \texttt{the experience buffer \textit{EB} to capacity \textit{$e_{EB}$}\label{algo:intial_eb}}
 \State \textbf{Intialize:}  \texttt{{the} {{training} network}  with random weights $\theta$\label{algo:intial_exp}}
 \State \textbf{Intialize:}  \texttt{{the} {inference} {network}  with random weights \textit{$\hat{\theta}$}\label{algo:intial_inf}}
 \State \textbf{Intialize:} \texttt{the observation vector $O_t$=$O(s_1)$ with storage request $s_1$=\{$req_{t}$\}, and host and  storage features\label{algo:intial_req}}

%  \Require  \texttt{\gca{exploration network} policy action-value function \textit{Q} with random weights $\theta$}
%  \Require  \texttt{\gca{inference}  network action-value function \textit{$\hat{Q}$} with weights \textit{$\hat{\theta}$}}
% \textbf{Outputs:} \texttt{Learned \namePaper~data-placement policy}

    % \For{\texttt{$ Iterations \gets 1$ to $T$}  }
        \ForAll{\texttt{storage requests}     }
            \If{\texttt{(rand() $<\epsilon$)}} \Comment{\comm{with probability $\epsilon$, perform exploration}\label{algo:exploration1}}
                \State    \texttt{ random action $a_t$} \label{algo:exploration2}
                %\Comment{\comm{{fast or slow device}}}
                % \Comment{\comm{ }}  
            \Else \Comment{\comm{{with probability 1-$\epsilon$}{,} perform exploitation}} \label{algo:exploitation1}
                \State  \texttt{ $a_t=argmax_a Q_t(a)$}  \label{algo:exploitation2}
                \Comment{\comm{select action with the highest $Q_t$ value {from inference network}}}
            \EndIf
           \State \texttt{execute  $a_t$} \label{algo:act}
             \Comment{\comm{{place} the requested page {to}  fast or  slow storage}}
        %   \State \texttt{$r_t \gets$ observe\_reward()\label{algo:reward}} 
           \If{ no eviction}\label{algo:reward_if} 
                \State \texttt{$r_t \gets$  $\frac{1}{L_t}$\label{algo:reward_no_evict}} 
                \Comment{\comm{{reward, given} no eviction of a page from fast to slow storage}}
            \Else
              \State \texttt{$r_t \gets$ max(0,$\frac{1}{L_t}$-\textit{$R_p$})\label{algo:reward_evict}} 
              \Comment{\comm{{reward with} an eviction penalty in case of an eviction}}
              \EndIf
        %   \Comment{\comm{collect immediate reward associated with current data placement}}
        %   \State \texttt{next storage request $req_{t+1}$ and $O_{t+1}$=$O(s_{t+1})$}
           \State \texttt{store {experience} $(O_t,a_t,r_t,O(t+1))$ in \textit{EB} \label{algo:store_exp}}
            \If{{\texttt{({num} requests \gonx{in \textit{EB}}==$e_{EB}$)}}\label{algo:eb_full}}   \Comment{\comm{train  {training} network when EB is full}}
               \State \texttt{sample random batch{es} of  experiences  from \textit{EB}, which are in format $(O_j,a_j,r_j,O(j+1))$} \label{algo:line:sample_experiences}\;
               \Comment{\comm{where $O_j$ represents an observation  at a time instant j from \textit{EB}}}
                % \State \texttt{$\hat{T}_{z_j}:= r + \gamma z_j \vspace{-0.05cm}  $}
            %   \Comment{ \comm{perform Bellman update using the retrieved Q-value distribution for each \emph{atom} $z_j$  \label{algo:line:bellman_update} }}
            \State \texttt{Perform stochastic gradient descent}
               \Comment{ \comm{update the {training} network weights \label{algo:line:bellman_update} }}
                  \State \texttt{$\hat{\theta} \gets \theta$ \label{algo:weight_trans}} \Comment{ \comm{{copy} the {training} network weights to the inference network }}
            %   \State \texttt{$D_{KL} (\oplus\hat{T}Z_{\hat{\theta}}(x,a)||Z_{\theta}(x,a))$ } 
            %   \Comment{ \comm{calculate cross entropy loss $\mathcal{L}_{x,a}(\theta)$ (KL divergence) to update \namePaper's~policy\vspace{-0.05cm} \label{algo:line:kl}}}
              \EndIf 
            % \[ (\oplus\hat{T}Z_{\theta}(x,a))_i= \sum_{j=0}^{N-1} \left[ 1-\frac{\big|\left[ \hat{T}z_j \right]^{V_{max}}_{V_{min}} - z_i\big|}{\Delta z}  \right]^{1}_{0}p_j(x',\pi(x'))   \]
        %   \State \texttt{$Z(x,a)=r(x,a)+\gamma Z(x',a'))$}
        % \texttt{where Z=return for a distribution, r=reward, and (x',a')=next state-action. }
        %   \texttt{where $\hat{T}$ is the Bellman operator.}
          
           
                % \State where $\hat{T}_{z_j}$ is the Bellman update for atom $z_j$ using:\vspace{-0.05cm}\label{algo:line:atoms}
        \EndFor
    % \EndFor
\end{algorithmic}
   \end{algorithm}
       
        %   \begin{algorithmic}[1]
        %   \STATE this is code \Comment{\comm{iterate over each edit distance}}
        % \end{algorithmic}
    % }
    
    % \end{minipage}
    % \end{figure*}
    % \setlength{\textfloatsep}{0.1cm}
    % \setlength{\floatsep}{0.1cm}
        % \vspace{-0.3cm}
        
        
        
%  \setlength{\textfloatsep}{0.05cm}
%     \setlength{\floatsep}{0.05cm}
%     % \begin{minipage}{\linewidth}
%     \begin{algorithm}[h]
%     \ssmall
%      \caption{\namePaper data-placement algorithm.}
%      \label{algo:rl_algo}
%     \DontPrintSemicolon
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%       \KwIn{ Initialize experience buffer \textit{B} to capacity \textit{1000}\\ 
%       Initialize action-value function \textit{Q} with random weights $\theta$\\ 
%       Initialize target action-value function \textit{$\hat{Q}$} with weights \textit{$\hat{\theta}$}}
%       \KwOut{Trained RL-based data placement policy for hybrid storage systems}
%       \For{$ Iterations \gets 1$ to $T$}    
%       {  
%         Initialize storage request $s_1$=\{$req_{t}$\} as Observation $O_t=O(s_1)$\tcp*[l]{first storage request}
  
%             \ForAll{Storage requests}     
%             {
%               \If{(rand() $<\epsilon$)}{     random action $a_t$=\{fast or slow device\}\tcp*[l]{With probability $\epsilon$ select a random action to perform exploration}    }
%                 {     otherwise select $a_t=argmax_a Q_t(a)$\tcp*[l]{perform exploitation}
%                 }
%                 Execute chosen data placement $a_t$ and observe reward $r_t$ and next storage request $req_{t+1}$\;
%                 Set $s_{t+1}=s_t,a_t,req_{t+1}$ and $O_{t+1}$=$O(s_{t+1})$\;
%                 Store transition $(O_t,a_t,r_t,O(t+1))$ in the \textit{experience buffer}\;
%                 Sample random batch of transitions ($(\phi_j,a_j,r_j,\phi(j+1))$) from \textit{B} \label{algo:line:sample_experiences}\; \tcp*[l]{where $\phi$ represents an observation from the replay buffer}
%                 Perform Bellman update using the retrieved Q-value distribution\cite{C51} \label{algo:line:bellman_update}  \vspace{-0.2cm}
%             \[ (\oplus\hat{T}Z_{\theta}(x,a))_i= \sum_{j=0}^{N-1} \left[ 1-\frac{\big|\left[ \hat{T}z_j \right]^{V_{max}}_{V_{min}} - z_i\big|}{\Delta z}  \right]^{1}_{0}p_j(x',\pi(x'))   \]
%             \\where $\hat{T}_{z_j}$ is the Bellman update for atom $z_j$ using:\vspace{-0.05cm}\label{algo:line:atoms}
%             \[ \hat{T}_{z_j}:= r + \gamma z_j \vspace{-0.05cm}  \]
%           \\ Calculate cross entropy loss (KL divergence) to update \namePaper~data-placement policy:\vspace{-0.05cm} \label{algo:line:kl}
%             \[D_{KL} (\oplus\hat{T}Z_{\theta}(x,a)||Z_{\theta}(x,a)) \]  
%              }
%         } 
%       \end{algorithm}

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/abstract_v2.tex <==
\go{Hybrid storage systems (HSS) use multiple different storage devices to \gonn{provide} high and scalable storage capacity at high performance. Data placement across different devices is critical to maximize the benefits \gonn{of} such a hybrid system. Recent research proposes various techniques that aim to accurately identify performance-critical data to \gca{place} it in a ``best-fit'' storage device. Unfortunately, most of these techniques are 
%largely ad-hoc
\rakeshisca{rigid}, which (1) limits their \gon{adaptivity} to perform well \gon{for} a wide range of \gon{workloads} and storage device configurations, and (2) makes it difficult for designers to extend these techniques \gon{to} different storage system configuration\gon{s} (e.g., \gon{with \gonn{a} different number \gonn{or different types} of} storage devices) than the configuration \rbc{they are} designed for.  }
% Hybrid storage %system is 
% \juangg{systems are} a potential solution to cater to %a wide range of  
% performance-capacity tradeoffs required in modern computing systems. In recent years, researchers have proposed multiple data placement techniques for hybrid storage systems that try to accurately identify performance-critical data to put it in a ``best-fit" storage device. However, most of these techniques are largely ad-hoc and heuristics-based, which (1) limits their adaptability to perform well in a wide range of applications and storage device configurations, and (2) puts a significant burden on the human designers to extend these techniques for a different storage system configuration than the configuration it is designed for (e.g., increasing the number of storage device types in a hybrid storage system).
\go{Our goal} is to design a new data placement technique for hybrid storage \gon{systems} that \gon{overcomes these issues and provides: (1) \emph{adaptivity}\gonn{,} by}  %dynamically %derive} a data-placement policy by 
\emph{continuously learn\gon{ing}} from and \go{adapt\gon{ing} to} the \gon{workload} and the storage device characteristics, and (2) \emph{easy \gon{extensibility}} to  a wide range of \go{\gon{workloads} and} HSS configurations.


We introduce \emph{\namePaper}, \gon{the first technique that uses} 
%\gca{a data-placement technique that formulates}  %which formulates \jgll{"Sibyl formulates...", but what is it? "We introduce Sibyl, a data placement techniques that formulates..."} 
%the data-placement problem in hybrid storage systems using 
reinforcement learning \gca{for data placement in hybrid storage systems}. \namePaper observes different features \gon{of} the \gon{running workload}  \gon{as well as the}  storage devices to make system-aware data placement decisions. For every decision \gon{it makes}, \namePaper receives a reward from the system that it uses to evaluate the long-term \gon{performance} impact of its decision and continuously optimizes its data placement policy online. 

We implement \namePaper on  \emph{real} \gonn{systems with various} \go{HSS configurations, including dual- and tri-hybrid storage systems}, and extensively compare it against \gon{four previously proposed data placement techniques (both heuristic- and machine learning-based) } over a wide range of \go{\gon{workloads}}.
%heuristics-based and supervised machine learning-based methods.}
Our results show that  %performance-optimized %\jgll{"performance-oriented"? It may not be "optimized", even though the used SSDs are fast. We "optimize" it with Sibyl.} 
 \namePaper~\gon{ provides \gonzz{21.6\%/19.9\%} performance improvement in a performance-oriented\gonn{/cost-oriented} HSS configuration %and 23.2\% performance improvement in cost-oriented HSS configuration 
 compared to the best previous data placement technique.} %19.9\%-36.1\% performance improvement compared to the prior data-placement techniques. \gca{While in} a \gca{cost-oriented} %cost-optimized \jgll{"low-cost"?} 
% HSS configuration, \namePaper improves performance by 23.2\%-68.8\%. 
%Our tri-hybrid system evaluation results show that \namePaper provides extensibility and reduces system architect's burden in designing sophisticated data-placement mechanisms to provide, on average, 43.5\% performance improvement over a heuristic-based policy. 
Our evaluation using an HSS configuration with three different storage devices shows that \namePaper outperforms \gonn{the state-of-the-art} \gonzz{data placement} %heuristic-based 
policy by 23.9\%-48.2\%\gonn{,} while significantly reducing the system architect's burden %\jgll{Sounds weird: do we measure this burden in any way?} %\gaganF{it's in terms of effort to device a new policy; for RL we just need to add a new action but for heuristic-based policy we would need to code all the new scenarios and for ML-based we need to collect new dataset.} 
in designing a data placement mechanism that can simultaneously incorporate three storage devices.
% \gon{ We demonstrate that \namePaper outperforms a state-of-the-art supervised-learning-based hybrid storage data placement policy (\arc), by 36.1\% and 68.8\% on high-end and middle-end hybrid storage configuration and on high-end and low-end hybrid storage configuration, respectively. Compared to a recurrent neural network-based (\kleio) data placement technique, \namePaper improves performance by 21.6\% and 34.1\%, respectively. While comparing to  two state-of-the-art heuristic-based policies (\cde and \hps), \namePaper provides 28.1\% and 23.2\% performance improvements on high-end and middle-end hybrid storage configuration, 19.9\% and 45.\% on high-end and low-end hybrid storage configuration, respectively. }
% We demonstrate that \namePaper~outperforms the state-of-the-art supervised learning-based data placement policy by 27.9\% on average and two heuristics-based techniques
%under two different hybrid-storage configurations
% by 24.1\% and 34.7\% on average, respectively. 
We show that \namePaper  achieves 80\% of the performance of an {oracle} policy that has \gon{complete} knowledge~of~future access patterns while incurring \gon{a \gonn{very modest} storage}  overhead of only \gonzz{124.4} KiB. %\jgll{Where? In the host CPU?}. %\gca{We open-source \namePaper~to aid future research in hybrid storage systems: \MYhref[black]{https://github.com/CMU-SAFARI/Sibyl}{https://github.com/CMU-SAFARI/Sibyl}}.


==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/background.tex <==
\section{Background\label{sec:Sibyl/background}}
% remove during ISCA'22 revision
% We provide a background on hybrid storage systems and reinforcement learning. % necessary to understand the rest of the paper.
% remove during ISCA'22 revision
\vspace{-0.1cm}
\subsection{Hybrid Storage Systems (HSSs)\label{subsec:Sibyl/bg_hybrid}}

\fig{\ref{fig:Sibyl/hybrid}} depicts a typical HSS \gca{consisting} of a fast-yet-small \gon{storage} device \rcam{(e.g., \cite{inteloptane,samsung2017znand})} and a large-yet-slow \gon{storage} device \rcam{(e.g., \cite{intels4510, intelqlc, seagate, adatasu630})}. \gon{Traditional hybrid storage systems~\cite{heuristics_hyrbid_hystor_sc_2011,feng2014hdstore,micheloni2018hybrid} were designed with a smaller NAND flash-based SSD and a larger HDD. 
Nowadays, hybrid storage systems come with emerging {NVM} devices \rcam{(e.g.,~\cite{kim2014evaluating, tsuchida201064mb, kawahara20128, choi201220nm})} coupled with slower {high-density} NAND flash devices~\cite{matsui2017design, oh2013hybrid, lee2010high, okamoto2015application}. } The storage management layer can be implemented either as system software running on the host system or as \gca{the} firmware of a hybrid storage device (e.g., flash translation layer (FTL) in flash-based SSDs \rcam{\cite{cai2017error,gal2005algorithms}}), depending on the configuration of the HSS. In this chapter, we \gon{demonstrate and implement our ideas in \gonzz{the} storage management layer \gonzz{of} the operating system (OS)\gonzz{,} but they can be easily implemented in firmware as well.} The storage management layer {in the OS} orchestrates host I/O requests across heterogeneous {devices}, which are connected via an NVM Express (NVMe)~\cite{nvme} or SATA~\cite{sata} interface. {The storage management layer} provides the operating system with a unified logical \rcam{address} space (like the multiple device driver (md) kernel module in Linux~\cite{linux}).\rcam{~As illustrated in \fig{\ref{fig:Sibyl/hybrid}}, the unified logical address space is divided into a number of logical pages (e.g., 4 KiB pages). The pages in the logical address space are assigned to an application. The storage management layer translates \rcamfix{a} read/write performed on \rcamfix{a} logical page into a read/write operation on a target storage device based on the data placement policy. In addition, the storage management layer manages data migration between the storage devices in an HSS. When data currently stored in the slow storage device is moved to the fast storage device, it is called \emph{promotion}. Promotion is usually performed when \rcamfix{a page} in the slow storage device is accessed frequently. Data is moved from the fast storage device to the slow storage device during an \emph{eviction}. Eviction typically occurs when the data in the fast storage device is infrequently accessed or when the fast storage device becomes full.}

  \begin{figure}[h]
  \centering
%   \vspace{-0.04cm}
   %\includegraphics[width=0.65\linewidth]{images/Hybrid_Storage_System_15.pdf}
   \includegraphics[width=0.6\linewidth]{Sibyl/images/isca'22/Hybrid_Storage_System_25.pdf}
  \caption{Overview of a hybrid storage system} %\jgl{Make font bigger (text inside boxes, etc.).}}
  \label{fig:Sibyl/hybrid}
  \end{figure}
% \todo{enrich this figure with all the different processes}


%######################################################REMOVED for hpca#####
\gon{The performance of {a} hybrid storage system highly depend{s} on the ability of the storage management layer (\fig{\ref{fig:Sibyl/hybrid}}) {to \gonn{effectively} manage diverse devices and}
%the nature of the application and its 
workloads~\cite{matsui2017design, ren2019archivist}.
%\jgl{cite}
This \gonn{diversity} presents a {challenge} %an opportunity 
for system {architects} %designers 
\gonn{when they} design an intelligent data placement policy. %\gonn{An ideal data-placement technique should 
%: (1)} {{serve} as many requests to performance-critical data as possible using the fast storage device} to adapt to the \gon{workload}'s needs over time while being aware of devices and their characteristics. 
{A desirable policy has} to effectively utilize the low latency characteristics of the fast device {while making} optimal use of its small capacity %~\cite{sun2013high, matsui2017design, cheng2019optimizing, ren2019archivist, shetti2019machine}
and \gon{should provide easy extensibility to a wide range of workloads and HSS configurations. }}


==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/conclusion.tex <==
\section{Conclusion}

We introduce \namePaper, the first reinforcement learning-based mechanism for  data placement in hybrid storage systems.
Our extensive \gagan{real-system} {evaluation} demonstrate\rcamfix{s} that \namePaper~\gon{provides adaptivity and extensibility by} continuously learning from and autonomously adapting to the workload characteristics\rcamfix{, storage configuration and device characteristics,} and system-level feedback to maximize the overall long-term performance of a hybrid storage system. {We interpret \gca{\namePaper}'s policy through our explainability analysis} and {conclude that \namePaper provides an \rcamfix{effective} and robust approach \gonx{to} data placement in current and future hybrid storage systems.} 
\rcamfix{We hope that \namePaper and our open-sourced implementation of it~\cite{sibylLink} inspire future work and ideas in self-optimizing storage and memory systems.}
%We hope \namePaper~will  inspire system architects to replace rigid system policies with self-adaptable techniques. }
%{\namePaper continuously and automatically adapts its data-placement policy to place data in the best-fit storage device.} %Hybrid storage consists of multiple storage devices tiered together to provide both large storage capacity and fast access speed at a minimal cost.
%Correct data placement in the faster storage is critical in terms of latency because accessing the data directly from the faster storage \gagan{can be} orders of magnitude faster than retrieving the data from slower storage in a hybrid storage tier.   



==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/design.tex <==
 
\section{\namePaper: Design}
% \subsection{Overview}
\label{sec:Sibyl/mechanism}
 \begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth,trim={0cm 1.4cm 0cm 0.2cm},clip]{Sibyl/images/isca'22/Sibyl-19_embed.pdf}
   \vspace{-1.7cm}
   \caption{Overview of \namePaper 
  \label{fig:Sibyl/curator}}
% \vspace{-0.5cm}
\end{figure*}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth,trim={0cm 1.4cm 0cm 0.2cm},clip]{Sibyl/images/isca'22/network_6_embed.pdf}
   \vspace{-0.5cm}
   \caption{\gon{\gonz{Training}} network design using as input the \gonx{state} features from Table~\ref{tab:Sibyl/state}. \gon{The inference network \gonz{is identical except it is used only for inference}}
  \label{fig:Sibyl/model}}
\end{figure}

 \rbc{We implement \namePaper in \gon{the storage management layer of the host system's \gonz{operating system}}}. %\namePaper updates its decision-making policy \emph{online}.
 Figure~\ref{fig:Sibyl/curator} shows a high-level overview of \namePaper. \gonz{Sibyl} is \rbc{composed of} two parts, \gonz{each implemented as a separate thread},  that run in parallel %\jgll{To me, "phase" has a temporal meaning, so I cannot understand two phases running in parallel. You can consider "parts", "tasks", "functions", "operations", or other words.}. 
{\rbc{(1)} the \emph{RL decision thread}, \gont{where Sibyl decides the data placement \gonx{\circled{4}} of the current storage request  while collecting  \gonz{information \circled{7} about its decisions \gonx{\circled{4}} and their effects} \gonx{\circled{6}} in an \emph{experience buffer} \circled{5}, and} % where \gon{a collection policy is used to explore the} HSS \emph{environment} \gonff{while we \emph{deploy} the \namePaper policy to take data-placement decision, and} %that explores the environment 
\rbc{(2)} the \emph{RL training thread}}, \gonff{where} \namePaper uses the collected \textit{experiences}\footnote{Experience is a representation of a transition from one time step to another, in terms of $\langle State, Action, Reward, Next State \rangle$.} \gonx{\circled{8}}  to \gca{ update its decision-making policy online \gonx{\circled{9}}.} \gont{Sibyl continuously learns from its past decisions \gonz{and their impact}. Our two-threaded implementation avoids that the learning (i.e., training) interrupts \gonz{or delays} data placement decisions for incoming requests. To enable the parallel execution of the two threads, we duplicate the neural network \gonz{that is} used to \gonz{make} data placement \gonz{decisions}. While one network \gonz{(called the \emph{inference network} \circled{2})} is deployed \gonx{(i.e., makes decisions)} the second network \gonz{(called the} \gonz{training} network \circled{9}), is  trained in the background. \gonx{The} inference network is used \emph{only} for inference, while \gonx{the}
training network is used \emph{only} for training.} \gonz{Therefore, \gonx{\namePaper does} \textit{not} perform a separate training step for the inference network and} \gonx{instead} periodically cop\gonx{ies} the  \gonz{\gonz{training}} network weights to the \gonz{inference} network \circleds{10}.

\gont{For every new storage request to the HSS, Sibyl uses the state information \circled{1} to \gonz{make} a data placement decision \gonx{\circled{4}}. %vector from the attributes of the incoming request and the current system state (e.g., access frequency, remaining capacity in the fast storage, etc.) 
The inference network  predicts the Q-value for each available action given the state information. Sibyl policy \circled{3} selects the action with the maximum Q-value \gonx{or, with a low probability, a random action for exploration} and performs the data placement. % Sibyl uses the exploration policy \circled{2} to explore the HSS environment and update its policy. 
}




\vspace{-0.2cm}
 \subsection{\namePaper Data Placement Algorithm}
\label{subsec:Sibyl/mechanism_rl_algo}

Algorithm~\ref{algo:rl_algo} describes \gon{how} \namePaper~\gon{performs} {data placement}  \grakesh{for} an HSS. \gon{Initially, the experience buffer is allocated to hold $e_{EB}$ entries \gonz{(line~\ref{algo:intial_eb})}, and the \gonz{training} and the inference network weights are initialized to \gonz{random values } \gonz{(lines~\ref{algo:intial_exp} and \ref{algo:intial_inf})}.} \gon{When a storage request is received \gonz{(line~\ref{algo:intial_req})}}, Sibyl policy (\circled{3}  Figure~\ref{fig:Sibyl/curator}) either (1) randomly selects an action  with $\epsilon$ probability (lines~\ref{algo:exploration1}-\ref{algo:exploration2}) to perform exploration in an HSS environment,  or \gon{(2) selects \gonx{the action that maximizes the Q-value, based on information stored in the inference network}} %exploitation of its \gca{current} policy 
(lines~\ref{algo:exploitation1}-\ref{algo:exploitation2}). After performing the \gon{selected} action \gont{(line~\ref{algo:act})}, \namePaper collects its reward\gonx{, whose value depends on whether an eviction is needed from fast storage} (lines~\ref{algo:reward_if}-\ref{algo:reward_evict}). The \gont{generated experience \gonx{is} stored} in the experience buffer (line~\ref{algo:store_exp}). \gonz{Once the experience buffer has $e_{EB}$ entries (line~\ref{algo:eb_full}), \gonx{\namePaper} trains the training network.} \gont{During training,} the training network samples a batch of experiences  from the \gor{ experience buffer} (line~\ref{algo:line:sample_experiences}) and updates its weights using stochastic gradient descent (SGD)~\cite{bottou2003stochastic} (line~\ref{algo:line:bellman_update}). \gonx{\namePaper} does \textit{not} perform a separate training step for the inference network.  \gon{Instead}, the training network weights are copied to the inference network (line~\ref{algo:weight_trans}), which removes the training
of the inference network from the critical path \gonx{of decision-making}.  %Sibyl policy uses the inference network to select the action with the maximum Q-value to perform the placement of the current storage request. %Thus, ensuring that the training delay does not affect the inference time for a data-placement decision. %In line~\ref{algo:line:bellman_update}, we use the Bellman equation~\cite{bellman1952theory}  to update Q-value of a state-action pair associated with the current storage request.
 \input{Sibyl/algorithm/rl_algo}% ,  experiences are fed to calculate the Q-value of a storage request $s_t$  . %, and 2) the target network to estimate the Q-value of the a state storage request  $s_{t+1}$.} 
%In line~\ref{algo:line:bellman_update}, we use the Bellman~\cite{bellman1952theory} update equation to update Q-value of a state-action pair associated with the current storage request over a number of \emph{atoms}\footnote{Atoms is the number of  points in our probability distribution estimates. %\jgll{Too many fancy terms. This does not help understand.}}.
%The Bellman update equation is extended for probability distribution in the C51 algorithm (line~\ref{algo:line:bellman_update}). The equation updates the Q-value of a  state-action pair associated with the current storage request. 
%The Bellman update is projected to a set of \textit{atoms} or \textit{quantiles} representing the number of points in the probability distribution of the Q-values~\cite{C51}. 
% The distribution represents a probability of returns from our action space (e.g., fast and slow storage). Our policy network is trained using Kullback-Leibler (KL)~\cite{filippi2010optimism} divergence (line~\ref{algo:line:kl}) between the resulting probability distribution of our policy model and the inference network. 
%\jgll{Algorithms need to be explained line by line. Noone reads algorithms unless they are very much interested. If you explain it line by line, they will understand them, and they won't feel uncomfortable because of an algorithm looking at them :D}
%the target probability distribution of the target network.   %\gaganRemove{{As discussed in Section~\ref{sec:mechanism}}, there are two main phases in \namePaper~algorithm that run in parallel: (1) \textbf{the collection phase} that samples the environment to collect \textit{experiences};  and (2) \textbf{the learning phase} that randomly select data from \textit{experience} collected in the collection phase, to learn a data-placement policy.}% using stochastic gradient descent. 
% {As discussed in Section~\ref{subsec:mechanism_rl_agent}}, deep Q-network-based (DQN) algorithms use a neural network-based policy network instead of a table~\cite{qlearning_ML_1992} to estimate the Q-value of a state-action pair. %As discussed earlier (Section~\ref{subsec:mechanism_rl_agent}), .
% However, to train this policy network, DQN does not use the conventional  supervised learning approach %as used by most neural network-based algorithms 
% because of the lack of \emph{labeled} output data. Instead, DQN uses a \emph{target network} that is used to calculate the Q-values for the next state.  
% After each action, the agent stores tuple of $\langle State, Action, Reward, Next State \rangle$  into a replay buffer. This buffer is used to improve the quality of training and sample efficiency by breaking the temporal correlations~\cite{dqn}. 

 %The  training phase aims to improve the policy network by using value-iteration based reinforcement learning called C51~\cite{C51}. 



\subsection{\gont{Detailed Design of \namePaper}}
%  \subsection{\namePaper Architecture}
\label{subsec:Sibyl/detail_design}




 \subsubsection{RL Decision Thread} In this thread, \namePaper~\gonx{makes} data placement decisions while storing \textit{experiences} in an experience buffer. %These experiences are used during the training \circled{8} of the \textit{\gonz{training} network} \circled{9} in the RL training thread.
 Sibyl extracts the observation vector \circled{1} from the attributes of the incoming request and the current system state (e.g., access \gonz{count}, remaining capacity in the fast storage) and uses \gonx{the} inference network \circled{2} to predict the Q-values for each \gonx{possible} action with %\gonx{globally} 
 the given state vector.
 \gonz{While making data placement decisions, Sibyl balances the \gonx{random} \textit{exploration} of the environment (to \gonx{find a better} policy \gonzz{without getting stuck at a suboptimal one}) with the \textit{exploitation} of its current  policy (to \gonx{maximize its reward based on the current inference network weights}).} %an \textit{\gont{exploration} policy}  (\circled{3} \gonff{in}  Figure~\ref{fig:Sibyl/qrator}(a)) explores an HSS \textit{environment}. This policy generates \textit{experiences}\footnote{Experience is a representation of a transition from one time step to another, in terms of $\langle State, Action, Reward, Next State \rangle$.} that are stored % that the \textit{observer} stores 
 %into a {software-managed} \textit{experience buffer} \circled{4} in host DRAM. These experiences are used during the training \circled{5} of the \textit{\gonz{training} network} \circled{6} in the RL training thread to update Sibyl's data-placement policy. %\gup{The observer acts as a resting station while the experience buffer feeds training data to update \namePaper's policy.  The observer  ensures that data collection can occur in parallel \rbc{with the} training \rbc{of} the exploration network in the RL training \rbc{thread}.} 
 %{Each} experience is stored as a tuple of \gont{experiences} in the experience~buffer, 
%  These experiences are used during the training of the \textit{exploration network }in the RL training thread.
 %\jgll{I don't know why Driver and Observer are two separate entities. Maybe it is that the difference between them is not clear.} \jgll{The driver is the agent? I see an action arrow coming out of the driver...}
%  \begin{figure*}[h]
%   \centering
%   \includegraphics[width=0.5\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/QRator_2.pdf}
%      \vspace{-0.1cm}
%   \caption{Overview of \namePaper}
% \label{fig:Sibyl/curator}
%  \end{figure*}

% \head{RL components} 
\head{Sibyl policy} For every storage request, %Sibyl policy \circled{3} takes the data-placement decision \circled{4}.  
Sibyl policy selects the action that leads to \gonx{the highest long-term} reward \circled{6}.
% % \jgll{Recall to mention in the intro what the NN is for. The reader cannot wait until this page to understand why there is an NN in this RL story.}
 \iffalse
 Recently, in the domain of computer architecture, several different RL-based algorithms have been used to solve various tasks~\cite{rl_prefetching_2015_ISCA,rl_NOC_AIDArc_2018,rl_GC_TECS,ipek2008self,multi_scheduler_HPCA_2012,rl_opti_TACO_2017}.
 \fi
 We use \rbc{a} Categorical Deep Q-Network (also known as C51)~\cite{C51} to update  $Q(s,a)$.
%  As our state-action space is discrete, we use Deep Q-Network-based algorithms (DQN)~\cite{dqn}. We use Categorical Deep Q-Network (C51)~\cite{C51}. 
C51's objective is to learn the distribution of Q-values, %\jgll{No idea what a Q-value is and what its distribution means.}, 
whereas other variants of Deep Q-Networks~\cite{sutton1999policy,baird1995residual,liang2016deep,mnih2013playing,silver2016mastering,silver2017mastering} aim to approximate \gonx{a single value for $Q(s,a)$}. This distribution helps \rbc{Sibyl} to capture more information from the environment %, such as the variance of the distribution, 
to make \gonz{better} \gont{data placement} decisions~\cite{harrold2022data}.  

\gont{For \gonx{tracking} the state, we divide each feature into a small number of bins to reduce the state space \gonx{(see Section \ref{sec:Sibyl/rl_formulation})}, which directly affects the implementation overhead of \namePaper.} We \gonx{select the number of bins (Table~\ref{tab:Sibyl/state}) based on empirical} sensitivity analysis. % on different binning choices  (ref. Table~\ref{tab:state}). % with the aim to reduce the state size without a loss of information. 
Our state representation uses a more relaxed encoding of 40 bits \gont{(than using only 20 bits for the \gonx{observation vector})} 
to allow for future extensions (e.g., features with more bins). %, where 8 bits are size of the requested page, 4 bits for type of the requested page,  
%We use} 8 and 4 bits to represent the size and type of the current request, respectively, while to compute access interval and access \gonz{count}, we \gont{use} a separate 8-bit counter each. We use 8 bits for the remaining capacity in the fast storage and 4 bits for the current placement of the requested page. %\gor{We use a more relaxed encoding of 40 bits (8+4+8+8+8+4) \gont{than using 20 bits} for our observation vector to allow for future extensions (e.g., features with more bins). 
Similarly,  we use a relaxed 4\gonzz{-bit} encoding for the action to allow extensibility to a different number of storage devices. \gont{For the reward structure, we use a half-precision floating-point (16-bit) representation. }% \jgll{The distribution helps to capture the variance of the distribution? Sorry, I'm lost.}} 

\head{Experience buffer}  %It is important to notice that deep Q-networks-based algorithms do not use supervised learning as used by most neural network-based algorithms. The reason for that is the lack of labels (or golden output). This golden output is not provided to the learning agent beforehand, i.e., the learning agent has to figure it out on its own while exploring an environment. 
 \gonx{\namePaper} stores \emph{experiences} \gonx{it} collect\gonx{s} while interacting with the HSS in an  \emph{experience buffer}~\cite{dqn}. The experience buffer is allocated in  the host \gonz{main memory (DRAM)}. % and holds samples of past experiences. % added by \rbc{the} \emph{observer}. 
To minimize \gonx{its} design overhead, we %use a hashed replay buffer memory \jgll{"Hash replay buffer memory" sounds very cool. No idea what it means though.} that 
deduplicate data in the stored experiences. %trajectories along the last axis of the observations. 
  To improve the training quality, we \gonx{perform batch training where each batch consists of randomly sampled experiences}. \gonzz{This technique of randomly sampling experiences from the experience buffer} is called  \textit{experience replay}~\cite{dqn}. %{We copy the weights from the policy network to the \emph{target network} (see Section~\ref{subsec:mechanism_rl_algo}), } which predicts the Q-value of the next state-action pair. 
%  \namePaper aims to find a policy $\pi$ that leads to maximum cumulative reward  through the RL training thread.  

Figure~\ref{fig:Sibyl/training_f} shows the effect \rbc{of} different \rbc{experience} buffer sizes \gonx{on \namePaper's performance} in the \hmssd configuration. %, which is a hyper-parameter for \namePaper training. 
We observe that \namePaper's performance saturates \gonx{at 1000 entries, which we select as \gonzz{the experience buffer} size}. %  \jgll{Actually the jump from 10 to 100 looks bigger.}. 
%Therefore, we use a buffer \rbc{size that can store} 1000 experiences. 
{Since the size of our state representation is 40 bits, to store a single experience tuple, %$\langle State, Action, Reward, Next State \rangle$, 
we  need 40-bit+\gonzz{4}-bit+16-bit+40-bit, i.e., 100 bits. %  \jgll{Why only 4? Only 1 observation vector is a tuple of 6 elements.}, 
\gont{In total, for 1000 experiences, the \gor{experience buffer} requires 100 KiB in the host DRAM.}}

  \begin{figure}[h]
\centering
  \includegraphics[width=0.5\linewidth,trim={0cm 0.1cm 0cm 0cm},clip]{Sibyl/images/isca'22/buffer_micro_3.pdf}
  \vspace{-0.1cm}
\caption[Two numerical solutions]{Effect \gonx{of different experience buffer sizes on} the \gont{average request} latency (normalized to \fast) \label{fig:Sibyl/training_f}}
% \vspace{-0.1cm}
\end{figure}

\iffalse
  \begin{figure}[!h]
\centering
\begin{subfigure}[t]{.6\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Sibyl/images/hpca/buffer_micro_2.pdf}
   \vspace{-3cm}
  \caption{
  \label{fig:Sibyl/buffer_cap}}
\end{subfigure}%
\begin{subfigure}[t]{.4\linewidth}
  \centering
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{Sibyl/images/real_system/batch_loss_micro.pdf}
     \vspace{-3cm}
    \caption{
  \label{fig:Sibyl/batch_size}}
\end{subfigure}
  \vspace{-0.5cm}
\caption[Two numerical solutions]{ For \namePaper: (a) effect on the performance \gh{for different} buffer sizes. (b) effect on training loss with  batch size. \label{fig:Sibyl/training_f}}
% \vspace{-0.1cm}
\end{figure}
\gf{
 We sample a batch of tuples from the experience buffer to train our policy network. The experience replay serves the following two purposes. First, a naive Q-learning algorithm that learns from each experience tuple in a sequential order runs the risk of getting swayed by high correlation effects. Therefore, using an experience buffer of past experiences and randomly sampling data instead of using the latest experience helps break this correlation. Second, experience replay allows \namePaper to learn more from past experiences. 
 
 \gaganF{REMOVE?: Figure~\ref{fig:Sibyl/training_f}(b) shows the effect of different batch sizes. We make two observations. First, with a smaller batch \grakesh{size} ($<$128), the training loss reduces quickly. However, the loss fluctuates and is not able to converge well. Second, while \grakesh{with}  a bigger batch size ($>=$128), it takes more iterations for the loss to decrease. However, the agent can converge well. Based on these observations, we make use of 128 as our batch size.}} \jgll{Is this the batch size for NN training? Have we mentioned this before?}
 
 \fi


 
\head{Exploration vs. exploitation}  An \gonx{RL} agent needs to \emph{explore} the environment to improve its policy %for future decisions 
%in order to obtain a higher reward for future decisions. 
\rbc{to maximize \gonx{its} long-term reward beyond  local maxima~\cite{sutton_2018}}.
At the same time, the agent \gonx{needs} to \emph{exploit} what it has already \emph{experienced} \gonx{so that it can take advantage of its learning so far}.   
\rbc{To balance exploration and exploitation,}
%To overcome this dilemma, 
we use the $\epsilon$-greedy policy~\cite{tokic2011value}: the best-known action based on the agent's experience is selected with (1-$\epsilon$) probability, and \rbc{otherwise}, i.e., with $\epsilon$ probability, \rbc{another} action is chosen randomly. \gonx{Exploration allows \namePaper to experience states it may not otherwise get into~\cite{sutton_2018} and thus avoid missing higher long-term rewards.} %\gont{During the execution of a workload, \namePaper experiences the outcome of some of the states (via reward), while for %other it rely %\textit{trial-and-error} approach \juancr{others, it relies} on the exploration of its environment. 
To perform exploration, \namePaper randomly chooses to \gonx{place data} \gonx{to} the fast or the slow storage \juancr{device}, \gonx{so that it can} get more information about the HSS and the workload. Based on the received reward, \namePaper updates its \gonx{training network}. %current data placement policy to gain better rewards in the long run. 
  \gonx{Such exploration} helps \namePaper to avoid making suboptimal data placement decisions \gonx{in the long run.}%while exploiting its data-placement policy in the future.  % {However, we} observe that rather than using a fixed $\epsilon$ value, we achieve better performance if we decrease the \grakesh{epsilon} monotonically. Therefore, we start with a high epsilon value of 0.99 that allows our agent to explore more initially. As we progress through an \textit{iteration}, we decrease the epsilon to 0.0001 because the agent has done enough exploration and is ready for exploitation.

\subsubsection{RL Training {Thread}}  %The 
 \gont{This thread uses a} batch \rbc{of collected experiences} \circled{8} from the experience buffer \gonx{to train the training} network \circled{9}. %The training process results in updated weights for the training network while the inference network weights are fixed.  %The \gca{exploration} network is used to predict an action-value \textit{Q(s, a)} of a state-action pair \gca{that is}  used to update  \gca{\namePaper's data-placement} \textit{policy} $\pi$ \circled{5}. 
 %\gup{Note that there are two networks in \namePaper: (1) the inference and (2) the exploration network (see Figure~\ref{fig:Sibyl/qrator}). \gup{ The exploration network \gca{uses} the information of %\gca{the most} recent 1000  I/O requests \gca{present in} the experience buffer \gca{for retraining} the exploration network. 
The updated weights \gonx{of the training network} are transferred to the inference network after every 1000 requests \circleds{10}. %The inference network predicts $Q(s,a)$ values for the current storage request, which guides the {\namePaper policy.} %\gca{The training process} results in updated weights for the exploration network while the inference network weights are fixed  
 
% removed for ISCA'22 revision
% \gont{\namePaper uses two separate neural networks \gonff{for} (1) exploration and (2) inference.} \gup{ The exploration network \gca{uses} the information of %\gca{the most} recent 1000 
%  the past I/O requests \gonff{to} \gca{retrain} \gonff{itself}. }\gca{This retraining} results in updated weights for the exploration network. % while the inference network weights are fixed. 
%  After the training process, the weights of the exploration network are transferred to the inference network. \gonff{The inference network is used to predict $Q(s,a)$ values for the current storage request, which guides the \namePaper policy.}  \gup{The two \gonff{networks} run asynchronously, ensuring that the \gonff{exploration network training} would not affect \rbc{\namePaper's latency to take a} data-placement decision.} 
 
 
 %We use a deep RL-based approach that combines supervised-learning methods with an RL approach~\cite{sutton1999policy,baird1995residual,liang2016deep,mnih2013playing,silver2016mastering,silver2017mastering}}
%The first phase, {which explores the environment}, is called %as 
%the \emph{collection phase}, %that explores the environment 
%while the second phase, {called the \emph{RL learning phase}}, learns and updates the \namePaper~policy. 

% \jgll{The next two paragraphs are not easy to understand. I assume that the collection happens during the normal agent activity, but this is not said.}
% \begin{figure}[h]
% \centering
%   \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0.4cm},clip]{images/hpca/sibyl_4.pdf}
% \caption{Overview of \namePaper. }
% \label{fig:Sibyl/qrator}
% \vspace{-0.2cm}
% \end{figure}

 


 
\head{\gonz{Training} and inference \rbc{networks}} %\gonz{Training} network weights are trained using the past \textit{experiences} periodically updates inference network weights. 
The training an\gonzz{d} inference network allows \gonzz{the} parallel execution of \gonx{decision} and training threads.
% \gonz{Training} network weights are trained using the past \textit{experiences}, which  periodically updates inference network weights.   e used to calculate the \textit{Q}-values of state-action pairs. %A {deeper} neural network  would provide better results for a complex environment that consists of many state-action pairs at the expense.
We use an identical neural network structure for the training and inference networks.
\gup{A \rbc{deep neural network can be} prohibitive due to the long time \gonx{it requires for} train\gonx{ing} and converge\gonx{nce}, preventing \namePaper to  adapt to new state-action pairs \gonx{in a timely manner}. Based on experiments, we find that a simple feed-forward network~\cite{bebis1994feed} with only two hidden layers~\cite{de1993backpropagation} \gonx{provides} good \gonzz{performance} %approximation \gonx{of Q-values} 
for \gonx{\namePaper's} data placement task.} Figure~\ref{fig:Sibyl/model} shows the structure of our \rbc{\gonz{training}} network.\footnote{\rbc{The inference network is identical in shape to the \gonz{training} network.}} The network takes the observation vector $O_t$ as \gonx{its} input and produces a probability distribution of \rbc{Q-values} as \gonx{its} output. Before feeding the data to the network, we preprocess the data by normalizing and casting the data to low precision data types, which allows us to reduce memory in the experience buffer. 
Next, we apply two fully-connected \juangg{hidden} layers of 20 and 30 neurons, respectively. 
{We select these neurons based on our extensive design space exploration with different numbers of hidden layers and neurons per layer.} After the two hidden layers, we have an output layer of 2 neurons, one for each action. \gonx{Sibyl policy \circled{3} selects the action with the maximum Q-value.} All fully-connected layers use the swish {activation} function~\cite{ramachandran2017searching},  a non-monotonic function that
 %provides better performance
 outperforms ReLU~\cite{agarap2018relu}. 
 
 \gca{During the training of the \gonz{training} network, \gonzz{the} inference network's weights are fixed.}  \gont{ After every 1000 requests, \gonzz{the} weights of the \gonz{training} network are copied to the inference network, %\jgll{If the target network is updated, why do you say above that it is fixed?}
which removes the training of the inference network from the critical path. We set the number of requests to 1000 based on our empirical evaluation of the experience buffer size \gonx{(Figure~\ref{fig:Sibyl/training_f})}. Each training step is composed of \gont{8 batches of experiences from an experience buffer of 1000 experiences with a batch size of 128}. We perform the training on the host CPU rather than on \gonx{a dedicated hardware accelerator} because (1) the network size is small and the weights perfectly fit in on-chip caches of the CPU in our evaluated system, \gonzz{and}  (2) to avoid continuous weight transfer overhead between the host CPU and the \gonx{accelerator} over the external interface. }
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/network.pdf}
%      \vspace{-0.1cm}
%   \caption{Policy Model}
% \label{fig:Sibyl/model}
%  \end{figure}



 

 
 

% \subsection{Implementation and Optimization}
% \subsection{Hyper-Parameter Tuning}
\sloppy\head{Hyper-parameter tuning}
\label{subsec:Sibyl/lhs}
%It would be imprudent to exhaustively run for all the available optimization options, which is often done in research to collect training data. 
\gont{We improve \namePaper's accuracy by tuning its hyper-parameters.  Hyper-parameters are sets of RL algorithm variables that can be tuned to optimize the accuracy of the RL agent~\cite{paine2020hyperparameter,NAPEL}.} 
% \gont{We improve \namePaper's training by tuning its hyper-parameters. We perform additional tuning of our RL algorithm’s hyper-parameters. Hyper-parameters are sets of RL algorithm variables that can be tuned to optimize the accuracy of the RL agent.} 
{For hyper-parameter tuning, we perform % the
cross-validation~\cite{arlot2010survey} % process while
using different hyper-parameter values. During cross-validation, we randomly select one workload for hyper-parameter tuning and  \gonx{use the} other \gont{thirteen} workloads for validation. On the selected workload, we use different hyper-parameter configurations that we choose using \gonzz{the} \mbox{\textit{design of experiments}} (DoE)~\cite{montgomery2017design}. }DoE allows us  to minimize the number of experiments needed%to train
{ to find the \gonx{best} hyper-parameter \grakesh{values}} without sacrificing the quality of the information gathered by the experiments. \gont{Unlike traditional supervised learning methods, we do \emph{not} train Sibyl \emph{offline} using a training dataset before deploying it for data placement. \gonx{All training happens online in \namePaper.} For every evaluated workload, Sibyl starts with no prior knowledge and gradually learns to make data placement decisions online by interacting with the hybrid storage system.  \namePaper  needs only one-time \gonx{offline} hyper-parameter tuning.}

Table~\ref{tab:Sibyl/hyperparameter} shows the hyper-parameters considered \gonx{in} \namePaper's design \gonx{as well as their chosen values after the tuning process.  %space. \gont{We also mention the chosen values for each hyper-parameter. 
The discount  factor ($\gamma$) \gonx{determines the balance between} the immediate and future rewards. \gonx{At $\gamma$=0 ($\gamma$=1), \namePaper gives importance only to the immediate (long-term) reward.} The learning rate ($\alpha$) determines the rate at which neural network weights are updated. \gonzz{A lower $\alpha$ makes small updates to the neural network weights, which could take more training iterations to converge to an optimal policy. While a higher $\alpha$ results in large updates to the neural network weights, which could cause the model to converge too quickly to a suboptimal solution.} %\gon{A higher $\alpha$ gives more importance to the {recently} calculated Q-values for the weight update.} 
The exploration rate ($\epsilon$) balances exploration and exploitation for \gonx{\namePaper}. We also explore different batch sizes \gonx{(i.e., the number of samples processed in each training iteration)} and experience buffer sizes to train our \gonz{training} network.} 
% DoE is a set of statistical techniques meant to locate a small set of points in  parameter space to represent the entire parameter space. Running experiments for all available hyper-parameter options can be an extremely time-consuming process. 
\input{Sibyl/tables/hyperparameter}
\iffalse
This ``brute-force'' approach to training is too time-consuming; the sheer number of experiments renders detailed implementation intractable.
\fi

%The traditional brute-force approach to collecting training data is {too} time-consuming: the sheer number of experiments renders detailed simulations intractable. 
%Thus, the DoE strategy to gather a training dataset is a critical component of our model. 
% {In particular, we make use of \textit{Latin hypercube sampling} (LHS)~\cite{li2018processor} because it allows each of the critical parameters to be represented in a fully stratified manner, which provides better coverage~\cite{fang2002centered}.} LHS divides each parameter range into \textit{k} intervals and takes only one sample from each interval with equal probability, which  is more efficient compared to a random or ``brute-force'' approach.
\iffalse
To apply %Latin Hypercube sampling, one must
{LHS, we} %first 
choose \textit{m} sample points, which we refer to as \textit{c$_{lhs}$}, each from a specific interval. %; hence 
{Thus,} LHS guarantees effective space-filling~\cite{li2018processor}. 
\fi

  

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/discuss.tex <==
\section{Discussion}
\label{sec:Sibyl/discussion}


\gsa{\head{Cost of generality} %\todo[size=\small,color=orange!80]{\textbf{Q1. Generality claim}} \todo[size=\small,color=orange!20]{\textit{A1. rewrite + added about black-box policies}} 
\gon{We identify two main limitations of using RL for data placement. First, currently, RL is largely a \emph{black-box policy}.  Our explainability analysis (Section \ref{sec:Sibyl/explanability}) tries to provide intuition into Sibyl’s internal mechanism. However, providing rigorous explainability to reinforcement learning-based mechanisms is an active field of research~\cite{verma2018programmatically,liu2018toward,juozapaitis2019explainable,madumal2020explainable,sequeira2020interestingness,puiutta2020explainable}, a problem that is beyond the scope of this paper. Perfectly finding worst-case workloads against an RL policy is, therefore, very difficult, in fact, impossible, given the state-of-the-art in reinforcement learning. There are many dynamic decisions that the agent performs, which cannot be easily explained or modeled in human-understandable terms.}   % RL lacks a thorough explanation for its policies and actions. Our explainability analysis (\cref{sec:explanability}) tries to provide intuition into \namePaper’s actions. 
Second, \gonff{\namePaper} requires \emph{engineering effort} to (1) \gonff{thoroughly} tune the RL hyper-parameters, and (2) implement and integrate \namePaper components into the host OS's storage management layer. %As discussed in \cref{sec:overhead_analysis}, \namePaper requires an overhead of 119.1 KiB. 
This second limitation is not specific to Sibyl and applies to any ML-based storage management technique. \gonff{As quantified in  Section \ref{sec:Sibyl/overhead_analysis}, \namePaper's storage and latency overheads are small. }   }

\head{\namePaper's implications} \gor{\gont{\namePaper} (1) provides performance improvements on a wide variety of workloads and system configurations (our evaluations \gonff{in} Section \ref{sec:Sibyl/results} show that \namePaper outperforms all evaluated state-of-the-art data placement policies \gonff{under all system configurations}),  (2) provides extensibility by {reducing} the designer burden when extending data placement policies to multiple devices \gonff{and different storage configurations}, and (3) \gonff{enables reducing } the fast storage {device} \gonff{size} by taking \gonff{better} advantage of \rcamfix{the} fast-yet-small storage device and large-yet-slow storage device to deliver high storage capacity at low latency.}

\head{Adding more features and optimization objectives}
\gsa{An RL-based approach simplifies adding new features (such as bandwidth utilization) \gont{in} \gonzz{the} RL state and optimization objectives (such as endurance) using \gonzz{the} RL reward function. This flexibility allows an RL-based mechanism to self-optimize and adapt its decision-making policy to achieve an objective without \gont{the designer} explicitly defining \emph{how} to achieve it. We demonstrate and evaluate example implementations of Sibyl using a reward scheme that is a function of  request latency and eviction latency. We \gont{find} that \gonx{request} latency in the reward structure best encapsulates system conditions since latency could vary for each \gon{storage} request \gont{based on complex system conditions}. To optimize for a different device-level objective, one needs to define a new reward function with appropriate state features, e.g., to optimize for endurance, one might use the number of writes to an endurance-critical device in the reward function. Another interesting research direction would be to perform multi-objective optimization, \gont{e.g., optimizing for \gonx{both}} performance and energy. We leave \gont{the study of different objectives and features to} future \gont{work}.
}

\head{Necessity of the reward} \gsa{RL training is highly dependent upon the quality of the reward function and state features. Using an incorrect reward or improper state features could lead to severe performance degradation. }Creating the right reward is a human-driven effort that could benefit from design insights. We tried two other reward structures to achieve our objective to \grakesh{\rcamfix{improve}  \gonff{system} performance}:
\begin{itemize}[leftmargin=*, noitemsep, topsep=0pt]
\item \textbf{Hit rate of the fast storage device:} Maximizing the hit rate of \ghpca{the} fast \gon{storage} device is another \gonff{potentially plausible objective}. However,  
%we observe that while using the 
\rcamfix{if we use} \gonff{the} hit rate as \gonzz{a} reward, \namePaper (1) tries to aggressively place data in \gonzz{the} fast storage \rcamfix{device}, \gon{which leads to unnecessary evictions}, \gonzz{and} (2)  cannot capture the asymmetry in the latencies  present in \gonx{modern} storage devices \gonff{(e.g., due to  \mbox{read/write} latencies, latency of garbage collection, queuing delays, error handling latencies, \gonzz{and} write buffer state)}.

\item \textbf{High negative reward for eviction:} We also tried a negative reward for eviction and \gonz{a} zero \rcamfix{reward} in other cases. We observe that such a reward structure \gon{provides suboptimal performance because \gonff{\namePaper places more pages in the slow device to avoid evictions. Thus, \gonx{with such a reward structure,} \namePaper is not able to effectively utilize the fast storage.}} % it makes}~\namePaper believe that it cannot control dynamic changes in the system state. \gont{In behavioral psychology, this is referred to as \emph{learned helplessness}~\cite{carlson1997psychology}. Therefore, we provide a positive reward, which motivates \namePaper to explore. } %Therefore, we need the penalty at the correct scale so that it is large enough to penalize the agent and small enough not to deviate the learned policy too much on a wrong decision. %, \js{leading to a sub-optimal data-placement policy. %\js{which eventually makes the agent stop trying leading to a sub-optimal data-placement policy. 



\end{itemize}
  \noindent We conclude that our chosen  reward structure works well for a wide variety of workloads \gonff{Section \ref{sec:Sibyl/results}}, as \gonff{\gonx{reinforced} by} our generality studies using unseen workloads in \mbox{Section \ref{subsection:Sibyl/perf_unseen}}.   

\head{Managing hybrid main memory using RL} \gca{The key idea of \namePaper can be adapted for managing hybrid main memory architectures. However, managing data placement at different levels of the memory hierarchy
%, such as the main memory, 
has its own set of challenges~\cite{li2017utility_HMM,agarwal2015page_HMM,agarwal2017thermostat_HMM,goglin2016exposing,ham2013disintegrated_HMM,lin2016memif,malladi2016dramscale,pavlovic2013data,pena2014toward,qureshi2009scalable,yoon2012row,meza2013case, meza2012enabling, ren2015thynvm} that \namePaper would need to adapt \rcamfix{to}, such as the low latency decision-making \gonff{and control} requirements in  main memory. %and limited space for metadata), 
% We believe managing hybrid storage systems is equally important as managing hybrid main memory.
Even with the \gonx{use} of hybrid main memories, many systems \rcamfix{continue to} benefit from using hybrid storage devices \gonff{due to much lower cost\gonx{-}per\gonx{-}bit of storage, which accommodates increasingly larger datasets.} %, especially in the cloud and \gont{high performance computing (HPC) systems}, where efficient data placement techniques can reduce the total cost of ownership. %storage \gont{leads to a lower total cost of ownership.} %provides a much lower cost per bit. 
 Therefore,  we focus on hybrid storage systems and leave it \rcamfix{to} future \rcamfix{work} to \rcamfix{\gonff{study} RL to manage} hybrid main memories. 
}





==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/evaluation.tex <==

\section{Evaluation Methodology} \label{sec:Sibyl/evaluation}
% \subsection{{Methodology}} \label{subsec:method}
\head{Evaluation setup}
{
We evaluate  \namePaper~\gon{using}  real \gonf{systems with various HSS}   configurations.
%,} consisting of a fast storage {device} and a slow storage {device}. Both %
The \gonf{HSS devices} \gon{appear} as a single flat {block device \rcamfix{that exposes} one contiguous logical block address space \gon{to the OS}, as depicted in \fig{\ref{fig:Sibyl/hybrid}}}. { We implement a lightweight custom block driver interface that manages the I/O requests to storage devices.  \tab{\ref{tab:Sibyl/devices}} {provides our system details, including the characteristics of the \gon{three}  storage devices \gon{we use}.}  %The use of direct IO data transfers provides three key benefits: 1) keeps the implementation overhead minimal, (2) reduces the CPU interrupt overhead, (3) eliminates the memory allocation and copy operations that are inherent in buffered I/Os. 
}  {To analyze the {sensitivity of our approach to} different device characteristics, we evaluate two different hybrid storage configurations (1) \em{performance-oriented HSS}: high-end device (\textsf{H})~\cite{inteloptane} and middle-end device (\textsf{M})~\cite{intels4510}, and (2) \em{cost-oriented HSS}: high-end device  (\textsf{H})~\cite{inteloptane} and low-end device (\textsf{L}) ~\cite{seagate}. %as they are part of one continuous \js{logical block address} space. 
\gca{We also evaluate two tri-hybrid \gon{HSS} configurations \gon{consisting of (1)}  \thold~and  \gon{(2)} \thnew~ devices.  }
{We \gon{run the} Linux Mint 20.1  operating system~\cite{linuxmint} with the  Ext3
file system~\cite{tweedie1998journaling}}. We use \gon{the} TF-Agents API~\cite{TFagents} to develop \namePaper. \gon{We evaluate \namePaper using two different metrics: \mbox{(1) \emph{average}} \emph{request latency}\rcamfix{, i.e.,} average \rcamfix{of the latencies of all storage \mbox{read/write} requests in a workload}, \gonzz{and} (2) \emph{request throughput (IOPS)}\rcamfix{, i.e., throughput of all storage requests in a workload in terms of completed I/O operations per second}. %We include the number of evictions performed with different data placement techniques in the throughput calculation. 
} %and %TensorFlow-based~\cite{abadi2016tensorflow} wrappers to 
%connect the hybrid storage-based \emph{environment} to our agent.  %To facilitate further research in this area, w
% We plan to open-source our RL environment for the hybrid storage systems to aid % RL-based research in hybrid storage systems. 
% {future research on RL-based data placement for storage systems.}
}}
% \input{tables/devices_updated}
\input{Sibyl/tables/devices_real}

{{\head{Baselines}} \label{subsec:Sibyl/eval:baselines} {We compare \namePaper against \rcamfix{two } state-of-the-art heuristic-based \gon{HSS} data placement techniques, (1) cold data eviction (\cde) \cite{matsui2017design} and (2) history-based \gon{page selection} (\hps)~\cite{meswani2015heterogeneous}, \gon{(3)} a state-of-the-art supervised learning-based technique (\arcc)~\cite{ren2019archivist}, \gon{and (4)} a recurrent neural network (RNN)-based data placement technique (\kleio), adapted from \rakeshisca{Kleio~\cite{doudali2019kleio}, a data placement technique for hybrid memory systems}. \gup{\kleio %is designed for hybrid memory systems but we faithfully adapt it for hybrid storage systems because it 
provides a state-of-the-art ML-based data placement \gon{baseline}.} %Note that, for conservative comparison, our performance evaluation does not take into account the computation overheads of \kleio while considering that of \namePaper.
We compare the above policies with three extreme \gon{baselines}:
(1) \slow{}, {where all data resides in \gon{the} slow \gon{storage (i.e., there is no fast storage)}}, (2) \fast, {where all data resides in \gon{the}  fast \gon{storage}}, {and (3) \textsf{Oracle}}
%, similar} to the B\'el\'ady's cache-replacement algorithm~\cite{belady1966study}
\cite{meswani2015heterogeneous}, which exploits \gon{complete} {knowledge of} future I/O-access patterns  %\gaganRemove{(which is impossible to obtain \juang{in a real scenario})}
{to perform data placement and to }\js{select victim data blocks for eviction from} the fast device. 

 

{\head{Workloads}} 
We use fourteen different \js{block-I/O traces} from {the} MSRC benchmark suite~\cite{MSR} that are collected from real enterprise server workloads. 
{We carefully select the fourteen traces to have {distinct} I/O-access patterns, as shown in \tab{\ref{tab:Sibyl/workload}}, in order to study a diverse set of workloads with different \rcamfix{randomness} and  \rcamfix{hotness} \gon{properties} (see Figure~\ref{fig:Sibyl/apps}). %\gonf{We mention the percentage write and read requests in a workload.} 
We quantify a workload’s randomness using the average request size of the workload; the higher (lower) the average request size, the more sequential (random) the workload. \gon{The average access \rcamfix{\gonz{count}} provides the average \rcamfix{of the access counts of all pages in a workload;}
%access count of each page in a workload; 
the higher (lower) the average access \rcamfix{\gonz{count}}, the hotter (colder) the workload.  
%We also mention 
\rcamfix{\tab{\ref{tab:Sibyl/workload}} also  shows}  \rcamfix{the number of} unique requests in a workload.} To demonstrate {\namePaper}'s ability to generalize and provide performance gains across \gon{\emph{unseen traces}}, \gon{i.e., traces} that are \emph{not} used to tune the \gon{hyper-parameters of} \namePaper, we evaluate {\namePaper} using \gon{four} additional workloads from FileBench~\cite{tarasov2016filebench}.} 

\input{Sibyl/tables/workload}

%We randomly select 50\% of workloads out of the MSRC traces %(which are \emph{not} part of the testing set) 
% to update {\namePaper}'s data placement policy. %We do not include {\kleio} because {\kleio} is designed for a single workload (training and inference is performed per time \textit{epoch} in a workload), instead we include \textsf{Archivist}\cite{ren2019archivist}.
% % \todo[size=\small,color=orange!80]{\textbf{Q1. Generality claim}} \todo[size=\small,color=orange!20]{\textit{A1. rewrite}}
% \gsa{In this step, Sibyl tunes its data-placement policy  to  adapt  to dynamically changing workloads. The tuned data-placement policy is then used to perform data placement for the four \gon{workloads} from the FileBench suite, which Sibyl  has not seen before. We use the same approach for  \mbox{\arcc} and \mbox{\kleio}, where we first train these algorithms using the MSRC workloads and then use the completely different FileBench workloads for testing. } %with %varying amount of access patterns 
%\nh{various amount of data hotness and memory access randomness} (ref. Figure~\ref{fig:Sibyl/apps} and Table~\ref{tab:workload}). 
%Table~\ref{tab:devices} summarizes the technology parameters of the simulated storage devices.




 \begin{figure*}[t]
%  \vspace{-1em}
\centering
\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0cm 0.2cm},clip]{Sibyl/images/isca'22/speedup_latency1_real_6.pdf}
  \vspace{-0.6cm}
   \caption{\textsf{H\&M} \gon{HSS} configuration\label{fig:Sibyl/perf_1}}
%  \caption{High-end and middle-end (\textsf{H\&M}) \gon{HSS}.\label{fig:Sibyl/perf_1}}
\end{subfigure}%


\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0.2cm 0.2cm},clip]{Sibyl/images/isca'22/speedup_latency2_real2_6.pdf}
    \vspace{-0.6cm}
   \caption{\textsf{H\&L} \gon{HSS} configuration \label{fig:Sibyl/perf_2}}
%   \caption{High-end and low-end (\textsf{H\&L}) \gon{HSS}. \label{fig:Sibyl/perf_2}}
\end{subfigure}
\caption[Two numerical solutions]{\gon{Average request latency} under two different hybrid storage configurations (normalized to \fast
%ideal case where we can serve all the requests from the faster storage and avoid the eviction latency
)
\label{fig:Sibyl/perf}}
%  \vspace{-0.1cm}
\end{figure*}
 
\begin{figure*}[h]
% \vspace{-1em}
\centering
\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0cm 0.2cm},clip]{Sibyl/images/isca'22/throughput_hm_6.pdf}
%   \caption{High-end and middle-end (\textsf{H\&M}).
  \vspace{-0.6cm}
\caption{\textsf{H\&M} \gon{HSS} configuration 
  \label{fig:Sibyl/iops_1}}
\end{subfigure}%

\begin{subfigure}[h]{.85\textwidth}
  \centering
  \vspace{-0.04cm}
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0.2cm 0.2cm}, clip]{Sibyl/images/isca'22/throughput_hl_6.pdf}
%   \caption{High-end and low-end (\textsf{H\&L}).
  \vspace{-0.6cm}
  \caption{\textsf{H\&L} \gon{HSS} configuration 
  \label{fig:Sibyl/iops_2}}
\end{subfigure}
\caption{\gon{Request throughput (IOPS)} under two different hybrid storage configurations (normalized to \fast
%ideal case where we can serve all the requests from the faster storage and avoid the eviction latency
)
\label{fig:Sibyl/iops}}
% \vspace{-0.5cm}
\end{figure*}

% \com{explanation for the policies is in the motivation as well}\\
% \vspace{-0.1cm}
\section{Results}
\label{sec:Sibyl/results}
 \subsection{Performance Analysis}
 \label{subsection:Sibyl/Evaluation_perf}
%We evaluated our approach with two different baseline policies  and an oracle approach that knows the future accesses under two device settings. We use a wide range of workloads with varying access patterns. 
Figure~\ref{fig:Sibyl/perf} compares the average \gon{request} latency of \namePaper against the baseline policies \gon{for \hmssd (Figure~\ref{fig:Sibyl/perf}(a)) and \hlssd (Figure~\ref{fig:Sibyl/perf}(b)) HSS configurations}. \js{All values are} normalized to \js{\fast}. % an ideal scenario where we can serve all the requests from the faster storage without having capacity constraints. 
We make \rcamfix{five major} observations. 
First, \namePaper consistently outperforms all the baselines for all the workloads in \hlssd and all but two workloads in \hmssd. \gon{In the} \js{\textsf{H\&M}} \gon{HSS} configuration (Figure~\ref{fig:Sibyl/perf}(a)), {where the latency difference between  two  devices  is  relatively  smaller than \textsf{H\&L},} \namePaper improves \gon{average} performance by {28.1\%, 23.2\%, 36.1\%, and 21.6\%} %44.9\%, 26.9\%, and 10.6\%
\gonzz{over} \cde, \hps, \arcc, and \kleio, respectively. In \gon{the} \js{\textsf{H\&L}} \gon{HSS} configuration (Figure~\ref{fig:Sibyl/perf}(b)), where there is a large difference between the latencies of the two {storage devices}, \namePaper~improves performance by 19.9\%, 45.9\%, 68.8\%, and 34.1\% %14.9\%, 71.5\%, and 75.6\% 
\gonzz{over} \cde, \hps, \arcc and \kleio, respectively.  } 
\gor{
%Through 
%\gon{Figure~\ref{fig:Sibyl/perf}(a), we observe that the} 
\rcamfix{We observe that the} larger the latency gap between HSS devices, the higher the expected benefits {of avoiding} the eviction penalty by placing only performance-critical pages in the fast storage.
Second, in \rcamfix{the} \textsf{H\&M} HSS configuration, \gon{\cde and \hps are ineffective for certain workloads (\textsf{hm\_1}, \textsf{prn\_1}, \textsf{proj\_2}, \textsf{proj\_3}, and \textsf{src1\_0}) even when compared to \slow.} % \slow~\gon{provides higher performance for} \textsf{hm\_1}, \textsf{prn\_1}, \textsf{proj\_2}, \textsf{proj\_3}, and \textsf{src1\_0}} \gca{than}  \cde~and \hps~\nh{as it does not perform evictions.%, thereby eliminating the eviction} penalty.
\rcamfix{In contrast,} ~\namePaper~\gon{consistently \rcamfix{and significantly} outperforms \slow for all workloads because it} can learn the small latency difference between \js{the two storage devices in \textsf{H\&M}} and dynamically \gonzz{adapts its} data placement decisions, which is \rcamfix{difficult} \js{for \cde and \hps due to their inability to holistically take into account the underlying device characteristics.} \gsa{Third, \namePaper provides slightly lower performance than \gon{other} baselines in only two workloads: \slow, \hps, \arcc, and \kleio for \hmone and \cde and \hps for \proxy in the \hmssd HSS configuration. We observe that such workloads are write-intensive and have many random requests (in terms of \gon{both access pattern}  and request size). Therefore,  such  workload\gon{s} would benefit from  more frequent retraining of Sibyl’s \gonzz{training} network. We experimentally  show in Section \ref{subsection:Sibyl/mixed_workload} that using a lower learning rate \gonzz{during} the training of the \gonzz{training} network helps to improve \rcamfix{\namePaper's} performance for such workloads. \gon{ Fourth, \namePaper achieves, on average, 80\% of the performance of the \oracle, \rcamfix{which} has complete knowledge of future access patterns, \gont{across \hmssd and \hlssd}. Fifth, \kleio provides higher performance than heuristic-based policies (2.1\% and 8.9\% than \cde and \hps, respectively, in \hmssd and 9.8\% than \hps in \hlssd), \rcamfix{but \namePaper outperforms it by \gonz{27.9\%}}.
%it shows an average performance gap of 27.85\%  than \namePaper
Unlike \namePaper, \rcamfix{the two machine learning-based policies,} \arcc and \kleio, do \emph{not} consider any system-level feedback, which leads to \rcamfix{their} suboptimal performance. }}

Figure~\ref{fig:Sibyl/iops} \gon{compares the request throughput (IOPS)} of {\namePaper} against other {baseline} policies. We make two observations. 
%First,  \gon{in the} \textsf{H\&M} \gon{HSS} configuration (Figure~\ref{fig:Sibyl/iops}(a)), {\namePaper} improves throughput by 32.6\%, 21.9\%, 54.2\%, and 22.7\% than {\cde}, {\hps}, {\arcc}, and {\kleio}, respectively. While, in \gon{the} {\textsf{H\&L}} \gon{HSS} configuration (Figure~\ref{fig:Sibyl/iops}(b)), {\namePaper}~improves throughput by 22.8\%, 49.1\%, 86.9\%, and 41.9\% %14.9\%, 71.5\%, and 75.6\% 
%than {\cde}, {\hps}, \arcc, and {\kleio}, respectively.
\rcamfix{First, in the \textsf{H\&M} ({\textsf{H\&L}}) HSS configuration (Figure~\ref{fig:Sibyl/iops}), {\namePaper} improves throughput by $32.6\%$ ($22.8\%$), $21.9\%$ ($49.1\%$), $54.2\%$ ($86.9\%$), and $22.7\%$ ($41.9\%$) \gonzz{over} {\cde}, {\hps}, {\arcc}, and {\kleio}, respectively.}
Second, \namePaper provides slightly lower performance than \slow, \cde, \hps, \arcc, and \kleio for \rcamfix{only} \hmone in \hmssd HSS configuration. We draw similar observations \rcamfix{for throughput results} as \rcamfix{we did for latency results} (Figure~\ref{fig:Sibyl/perf}) because as \rcamfix{\namePaper} consider\rcamfix{s} the request size in state features and \gonz{request} latency in the reward, \rcamfix{it} {also} indirectly captures throughput (size/latency).


\gon{ We conclude that \namePaper 
%through our state features and reward function, 
consistently provides higher performance than \rcamfix{all five} baselines and \rcamfix{significantly} improves both average request latency and request throughput.}}

\subsection{{Performance on Unseen Workloads}}
\label{subsection:Sibyl/perf_unseen}
To demonstrate {\namePaper}'s ability to generalize and provide performance gains across \textit{unseen} \rcamfix{workloads} that are \textit{not} used to tune the \rcamfix{hyper-parameters of the} data placement policy of \namePaper, we evaluate {\namePaper} using \gonzz{four} additional  workloads from FileBench~\cite{tarasov2016filebench}. \gon{No data placement policy \rcamfix{we evaluate}, including \namePaper, \rcamfix{is} tuned on these workloads. } Figure~\ref{fig:Sibyl/unseen} shows the performance of \rcamfix{these} unseen \rcamfix{workloads}. 
We observe the following observations. First, in \textsf{H\&M} (\textsf{H\&L}) \gon{HSS} configuration, {\namePaper}~outperforms {\kleio} and {\arcc}  by $46.1\%$ ($54.6\%$) and $8.5\%$ ($44.1\%$), respectively. Second, \mbox{\namePaper} may misplace some pages during the \rcamfix{online} adaptation period, but it provides significant performance benefit\rcamfix{s} over existing ML-based data placement techniques.} %Whereas \textsf{Archivist}, provides $85.2\%$ ($67.5\%$) lower performance than {\namePaper} in \textsf{H\&M} (\textsf{H\&L}) configuration. 
We conclude that {\namePaper} \gon{
%tuned on a set of workloads 
provides high performance benefits on unseen \rcamfix{workloads} for which it has not been tuned.} 


\begin{figure}[h]
    \centering
 \includegraphics[width=0.9\linewidth]{Sibyl/images/isca'22/unseen_traces_6.pdf}
    \caption{{\gon{Average request} latency on unseen workloads (normalized to \fast) under two HSS configurations}}
    % \vspace{-0.2cm}
    \label{fig:Sibyl/unseen}
\end{figure} 



\subsection{Performance on Mixed Workloads}
\label{subsection:Sibyl/mixed_workload}
% \todo[color=blue!40]{\textbf{Q2. Experiments with dynamic workloads}} \todo[color=blue!20]{\textit{A2. New experiment}}
We evaluate mixing  two or more workloads at the same time while \rcamfix{randomly varying} their relative start times.  Table~\ref{tab:Sibyl/mixed_workloads} describes the characteristics of these mixed workloads. These workloads are truly independent of each other, potentially creating more evictions from the fast storage device than a single workload.  Such a scenario \mbox{(1) leads} to unpredictable execution where requests arrive at different, unpredictable timesteps, (2) mimics distributed workloads, and (3) further tests the \gon{ability} of Sibyl to dynamically adapt its decision-making policy.

Figure~\ref{fig:Sibyl/mixedWorkloads} shows \gonzz{average request latency} for mixed workloads. We use two different settings for \namePaper: (a) \sibyldef, where we use our default hyper-parameters (Section \ref{subsec:Sibyl/lhs}), and (b) \sibylopt, where we optimize the hyper-parameters \rcamfix{for} these mixed workloads and use a lower learning rate ($\alpha$) of $1e^{-5}$. A lower learning rate performs small\rcamfix{er} updates to the \gonz{training}  network’s weights in each training \rncam{iteration}, thus requiring more training to converge to an optim\gon{al} solution.
\input{Sibyl/tables/mixed_workloads}

\begin{figure}[h]
    \centering
    % \fcolorbox{red}{white}{
 \includegraphics[width=1\linewidth]{Sibyl/images/isca'22/shepherd_dynamic_3.pdf}    
%  }
% \vspace{-0.4cm} 
 \caption{{\gon{Average request} latency on mixed workloads (normalized to \fast) \rcamfix{and two HSS configurations}}}
    %  \vspace{-0.2cm}
  
    \label{fig:Sibyl/mixedWorkloads}
\end{figure} 


We make two observations.   First, \sibyldef consistently outperforms \cde, \hps, \arcc, and \kleio~ \gon{by} 27.9\%, 12.2\%, 12.1\%, and 12.9\%,  %44.9\%, 26.9\%, and 10.6\%
 respectively, in \rcamfix{the} \textsf{H\&M} HSS \gon{configuration} and 9.4\%, 21.3\%, 19.4\%, and 17.1\%, respectively, in \textsf{H\&L} HSS \gon{configuration}. Second,  with a lower learning rate \rcamfix{and optimized hyper-parameters}, \sibylopt provides  5.2\% (9.3\%) higher average performance for \textsf{H\&M} (\textsf{H\&L}) \gon{HSS} configuration than \sibyldef.
  %Note that \mixfive, on average, has an equal number of reads and writes, and hence has a different execution behavior than \mix.   
 \gon{Third}, for \mix,  \hps provides comparable performance to \sibyldef in \textsf{H\&M},
 %\gon{HSS configuration},
 and \cde provides slightly  better performance  in \textsf{H\&L}.
 %\gon{HSS configuration}.
 As discussed in Section \ref{subsection:Sibyl/Evaluation_perf}, \proxy  is write-intensive and has  random requests (with an average request size of 7.2) \gon{within} every 1000 requests, which is the experience buffer size to train the \gonz{training}  network. Such a workload requires more frequent retraining of Sibyl’s \gonz{training}  network to achieve higher performance. \gon{We conclude that \namePaper ~\gonz{can} \rcamfix{effectively} adapt its \rcamfix{data placement} policy \rcamfix{online} to highly dynamic workloads.}

% \todo[color=green!40]{\textbf{Q3. Worse-case workload}} \todo[color=green!20]{\textit{A3. Observation drawn from new experiment}}








\gon{
\subsection{Performance with Different Features}
{Figure~\ref{fig:Sibyl/ablation} compares the use of some of the most \rcamfix{useful} features for the \emph{state} of \namePaper in our \textsf{H\&L} \gon{HSS} configuration.  \textsf{All} represents using all the six features \gca{in Table~\ref{tab:Sibyl/state}}. \namePaper~\gca{autonomously} decides which features are important to maximize the performance of \gon{the running} workload. %\jgll{Why don't we show all combinations? Why some features ($c_t, x_t$) are only considered as part of All?}


\begin{figure}[h]
  \centering
    \includegraphics[width=1\linewidth,trim={0cm 0.35cm 0cm 0cm},clip]{Sibyl/images/isca'22/ablation_hl_hpca_5.pdf}
  \caption{\rcamfix{Average request latency when using} different features (see Table~\ref{tab:Sibyl/state}) for the state space of \namePaper in the \textsf{H\&L} \gon{HSS configuration}  (normalized to \fast) }
\label{fig:Sibyl/ablation}
 \end{figure}

We make two {key} observations from Figure~\ref{fig:Sibyl/ablation}. First, \namePaper consistently achieves the lowest latency \gup{(up to 43.6\% lower)} by using all the features {mentioned in Table~\ref{tab:Sibyl/state}} (\textsf{All} in {Figure~\ref{fig:Sibyl/ablation}}). Second, by using the same features as in \rcamfix{baseline} heuristic-based polic\gonz{ies}, \namePaper is able to perform better data placement decisions. For example, \rcamfix{\textsf{$r_t$} and \textsf{$f_t$}  configurations of} \namePaper \rcamfix{~(in Figure~\ref{fig:Sibyl/ablation})} use \rcamfix{only one} feature, \rcamfix{just like} {\cde and \hps} do. 
%\namePaper  uses these features to find the best data placement policy autonomously and outperforms {\cde and \hps}  policies by 4.9\% and 5.5\%, respectively (\textit{ref.} {Figure~\ref{fig:Sibyl/perf_2}(b)}). 
\rcamfix{These two \namePaper configurations outperform {\cde and \hps}  policies by 4.9\% and 5.5\%, respectively (\textit{ref.} {Figure~\ref{fig:Sibyl/perf}(b)}). Using the same features as a heuristic-based policy, Sibyl autonomously finds a \rncam{higher-performance} dynamic policy that can maximize the reward function, which heuristic-based policies cannot possibly do.}
%This performance improvement is because \namePaper with its \textit{reward} structure \gup{brings the underlying device characteristics into the \namePaper's decision-making process.} %  that are not explicit in the state representation.
We conclude that {\namePaper}~uses a richer set of features %\jgll{Now the set is rich. I thought it was better to use only a few features to simplify the implementation.} 
that can capture multiple aspects of a storage request to \gon{\gonz{m}ake \gonz{better}}  {data} placement decisions than a heuristic-based policy. \gup{RL reduces %system architects' burden in designing burden 
\juangg{the design burden on system architects,} as \namePaper autonomously learns to use \gon{the provide\rcamfix{d}} features to achieve the highest cumulative reward.} In contrast, traditional heuristic-based policies use \rcamfix{features to make rigid data placement decisions without any system-level feedback,} \gonz{and thus they underperform \rncam{compared to \namePaper}.}
%\gca{features, such as} recency, frequency, and/or size, in isolation or combination to %take 
%\gon{take} 
%\jgll{This section is about justifying the state features, not about comparing to the heuristics. We have already explained in the motivation that the heuristics are bad. 
%Anyway, the comparison based on $r_t$ and $f_t$ is interesting, but I would think about having it somewhere else (Evaluation section?).}
%, in addition to the application characteristics via the state representation. 
 %\jgl{What is the reason for only a few features?}.  
} 
% Based on the above \js{six} features and storage device  characteristics, the agent %would 
% {will} decide to  serve %a 
% requests from a device that optimizes the overall long-term system performance rather than the short-term performance. 
}


\subsection{Performance with Different Hyper-Parameters}

Figures~\ref{fig:Sibyl/hyper_senstivity}(a), \ref{fig:Sibyl/hyper_senstivity}(b), and \ref{fig:Sibyl/hyper_senstivity}(c) show the effect \gon{of}  three critical hyper-parameters (discount factor, learning rate, and exploration rate) \rcamfix{on \namePaper's throughput in \hmssd HSS configuration}. 
%First, from 
Figure~\ref{fig:Sibyl/hyper_senstivity}(a) \rcamfix{shows} that \namePaper's \rcamfix{throughput} drops sharply at $\gamma=0$.
%This performance drop is because, a
At $\gamma=0$, \namePaper gives importance \gonz{only} to the immediate reward \gonz{and not} \rncam{at all to} the long-term reward, \gca{leading to} lower performance. We use $\gamma=0.9$, where \namePaper ~\rcamfix{is more forward-looking, giving enough weight to} long-term rewards.
%balances the short-term and 
%Second, the learning rate ($\alpha$) \gon{determines the rate at which exploration network wights are updated} (Figure~\ref{fig:Sibyl/learning_rate}).
\rcamfix{Figure~\ref{fig:Sibyl/hyper_senstivity}(b) shows} that at \rcamfix{a learning rate of} $\alpha=1e^{-4}$, \namePaper~\gon{provides} the best performance. \rcamfix{The learning rate determines the rate at which \gonz{training} network w\gonz{e}ights are updated.} \gonz{Both too slow and too fast} updates are detrimental \gonz{for}  adaptive learning and \gonz{stable \rncam{exploitation} of a learned policy}, \rncam{respectively}.
%, on average, across all the workloads. 
Third, Figure~\ref{fig:Sibyl/hyper_senstivity}(c)  shows  that the performance of \mbox{\namePaper} drops sharply if it performs exploration \rncam{too frequently} \rcamfix{(i.e., $\epsilon=1e^{-1}$)} and \rcamfix{thus} does not \gonz{sufficiently} exploit its learned policy. \namePaper achieves \rcamfix{the highest} performance improvement\rcamfix{s} for \rcamfix{$ 1e^{-5}\leq ~\epsilon \leq 1e^{-2}$}. 
%Figure~\ref{fig:Sibyl/LHS} illustrates LHS with two parameters, where the input space is divided into equal intervals.  % \gaganFPGA{To select the amount of samples to perform and effective hyper-parameter tuning we follow the approach from Valov~\etal~\cite{valov2015empirical}.}   %We use T\textit{$\times\mathbb{CO}$} samples, where T=5 allows to build highly accurate prediction models.

% \input{images/LHS.tex}




%   \begin{figure}[h]
% \centering
%   \includegraphics[width=0.5\linewidth,trim={0cm 0.8cm 0cm 0cm},clip]{images/hpca/buffer_micro_2.pdf}
%   \vspace{-0.1cm}
% \caption[Two numerical solutions]{ Effect on the latency \gh{for different} buffer sizes. \label{fig:Sibyl/training_f}}
% % \vspace{-0.1cm}
% \end{figure}

\begin{figure}[h]
%  {\renewcommand\fbox{\fcolorbox{ddgreen}{white}}
%  \fboxrule=1pt\fbox{
% \parbox[c]{\linewidth}{
% \begin{subfigure}[t]{.45\linewidth}
%   \includegraphics[width=\linewidth,trim={0cm 0.8cm 0cm 0cm},clip]{images/hpca/buffer_micro_2.pdf}
%   \vspace{-1.8cm}
%   \caption{\hspace{-2cm}
%   \label{fig:Sibyl/training_f}}
% \end{subfigure}%
\begin{subfigure}[t]{.45\linewidth}
% \vspace{-6pt}
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{Sibyl/images/isca'22/discount_factor_hpca_5.pdf}
   \vspace{-3.8cm}
  \caption{ \hspace{-2cm}
  \label{fig:Sibyl/discount}}
\end{subfigure}%
\begin{subfigure}[t]{.45\linewidth}
% \hspace{2cm}
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{Sibyl/images/isca'22/learning_hpca_5.pdf}
  \vspace{-3.9cm}
   \caption{\hspace{-2cm}
  \label{fig:Sibyl/learning_rate}}
\end{subfigure}
\begin{subfigure}[t]{.45\linewidth}
\hspace{4cm}
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{Sibyl/images/isca'22/epislon_4.pdf} 
  \vspace{-3.9cm} 
   \caption{\hspace{-8cm}
  \label{fig:Sibyl/epsilon}}
\end{subfigure}
% }}}
% \vspace{-0.1cm}
\caption{Sensitivity of \namePaper~\rcamfix{throughput} to: (a) the discount factor ($\gamma$), (b) the learning rate ($\alpha$), (c) the exploration rate ($\epsilon$), \rcamfix{averaged across 14 workloads (normalized to Fast-Only)} \label{fig:Sibyl/hyper_senstivity}}
\end{figure}




{\subsection{{Sensitivity to Fast Storage Capacity}}
%Figure~\ref{fig:Sibyl/sensitivity} shows the sensitivity of policies with percentage available capacity in the faster storage. \gaganF{How %do restict the size??} 
%\gon{The fast memory size allows to place more pages in the fast storage device, thereby likely offering great system performance. Therefore, we evaluate how each mechanism performs across a range of fast storage sizes by restricting the number of pages of a workload that can fit in the fast storage.}
{Figure~\ref{fig:Sibyl/sensitivity} shows the \gon{average request latency} of \namePaper and baseline policies \gon{as we vary}  the available capacity in the fast  \gon{storage}. \gonzz{The} \rcamfix{\rncam{x}-axis denotes a range of fast storage device sizes available for data placement and represented in terms of percentages of the entire fast storage device capacity, \gonz{where 100\% represents \rncam{the size where} all pages of a workload can fit in the fast storage}}. %In this study, we vary the fast storage capacity that the data-placement policies can utilize at a logical level.
%In this study, we configure the hybrid storage system at the logical level to limit the available capacity of the faster storage device.
%In this study, we limit the capacity of the faster storage available to the policies at a logical level.
%In this study, we configure the policies to access a limited address space of the faster storage.
%In this study, the policies are logically configured to access a limited address space of the faster storage for data placement.
\begin{figure}[h]
    \centering
%     {\renewcommand\fbox{\fcolorbox{ddgreen}{white}}
%  \fboxrule=1pt\fbox{
% \parbox[c]{\linewidth}{
 \includegraphics[width=1\linewidth]{Sibyl/images/isca'22/sensitivity_with_slow_7.pdf}
%  }}}
% \vspace{-0.5cm}
    % \caption{Latency normalized to \fast~policy with restricting the amount of data that can fit in the faster storage.}
    \caption{\gon{Average request latency for various fast storage \gonz{device} sizes (normalized to \fast)}}
    \label{fig:Sibyl/sensitivity}
\end{figure} 
}

%We limit the logical address space of the fast storage available to the policies for data placement.} We make two observations. 
\gonzz{We make two observations.} First, \rcamfix{for all fast storage sizes}, \namePaper performs better than  the baseline heuristic- % as we vary the amount of available capacity, a dynamically adaptable data-placement policy is required. In
and supervised learning-based policies for both \textsf{H\&M} and \textsf{H\&L} HSS configurations. 
%\gon{Even for 1\% of available fast storage capacity, which offers less opportunity for optimization, 
\rcamfix{Even when the fast storage size is as small as 1\%,}~\namePaper outperforms \cde, \hps, \arcc, \kleio by 47.2\% (11.5\%), 17.3\% (58.9\%), 12.3\% (110.1\%), 21.7\% (50.2\%), respectively, in \hmssd (\hlssd)
%and 11.5\%, 58.9\%, 110.1\%, and 50.2\%, respectively, in \hlssd. 
}. Second, at a larger %(higher) 
({smaller}) \rcamfix{fast storage device size}, the 
%decision-making policy becomes equal to 
\rcamfix{performance approaches that of} \gca{the} \fast (\slow) policy, \gf{ except \rcamfix{for} \arcc. \arcc classifies pages \gca{as} hot or cold \gca{at} the beginning of an epoch and does not change its placement decision throughout the execution of that epoch. It does not perform any promotion or eviction of data. We observe that \arcc often mispredicts the target device for a request and classifies the same number of requests for the fast and slow storage device under different fast storage sizes. 


As we vary the \gonz{size} of \gonz{the} \rcamfix{fast storage device}, a dynamically adaptable data placement policy is required, which considers features from both the running workload and the underlying storage system. \gon{ We conclude that \namePaper can provide scalability by dynamically \rcamfix{and effectively} adapting \rcamfix{its policy} to the available storage size to achieve high performance. %and greatly shrink the fast storage size. 
}} %All new requests are going to fast SSD. }



% \vspace{-0.2cm}
\subsection{{Tri-Hybrid Storage Systems}}
\label{subsec:Sibyl/trihybrid}
We evaluate two \gca{different} tri-HSS configurations, \thold~and \thnew ~(Table \ref{tab:Sibyl/devices}), implemented as a single flat block device. The \thnew \ configuration has a low-end SSD (L$_{SSD}$), %ADATA SU630~\cite{adatasu630} with a capacity of 960GB and performance (Max R/W: 520/450 MB/s) 
\gon{whose} performance \gon{is} lower than \rcamfix{the} \textsf{H} and \textsf{M} devices but higher than \rcamfix{the} \textsf{L} device. We restrict the available capacity of \textsf{H} and \textsf{M} %storage device to \gor{(1) 5\% and 5\%, respectively, and (2) 5\% and 10\%, respectively,} 
\rcamfix{to 5\% and 10\%, respectively,}
of the working set size of \gon{a given workload}. This ensures data eviction from \textsf{H} and \textsf{M} devices once \gon{they are} full. We compare the performance of \namePaper on a tri-hybrid system with a \gon{state-of-the-art} heuristic-based policy~\cite{matsui2017design, matsui2017tri} that divides data into \emph{hot}, \emph{cold}, and \emph{frozen} and places \gon{them} \rcamfix{respectively} into \textsf{H}, \textsf{M}, and \textsf{L} devices.\footnote{\gon{\cde, \hps, \arcc, and \kleio do \textit{not} consider more than two devices and \gonz{are not easily adaptable to a tri-hybrid HSS}.}} Figure~\ref{fig:Sibyl/triybrid} shows the performance \gon{of the} heuristic-based and \namePaper data placement policies. 
%Due to space reasons, we do not show results for \textsf{H} and \textsf{L} with capacity restricted to 5\% and 5\%, respectively.

 \begin{figure}[h]
%  \vspace{-1em}
\centering
\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0cm 0.2cm},clip]{Sibyl/images/isca'22/trihybrid1_new_4.pdf}
  \vspace{-2em}
   \caption{\thold~configuration\label{fig:Sibyl/triybrid1}}
%  \caption{High-end and middle-end (\textsf{H\&M}) \gon{HSS}.\label{fig:Sibyl/perf_1}}
\end{subfigure}%

\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth,trim={0.2cm 0.2cm 0.2cm 0.2cm},clip]{Sibyl/images/isca'22/trihybrid2_new_4.pdf}
    \vspace{-2em}
   \caption{\thnew ~configuration \label{fig:Sibyl/triybrid2}}
%   \caption{High-end and low-end (\textsf{H\&L}) \gon{HSS}. \label{fig:Sibyl/perf_2}}
\end{subfigure}
  \caption{\gor{\gon{Average request} latency for \rcamfix{the tri-hybrid HSS} (normalized to \fast) }}%, with available capacity of the middle device restricted to 5\% and 10\% of the working set size.}   }
\label{fig:Sibyl/triybrid}
%  \vspace{-0.1cm}
\end{figure}

We observe that  \namePaper outperforms the heuristic-based policy by, on average, \gor{43.5\% (48.2\%) and 23.9\% (25.2\%) for \mbox{\thold} (\mbox{\thnew})}. \rcamfix{This is because Sibyl is much more dynamic and adaptive to  \gonz{the storage} system configuration \gonz{due to its RL-based \rncam{decision-making}} than the baseline heuristic-based policy, which is rigid in its decision-making.}
%\namePaper autonomously adapts its data-placement policy using the system-level feedback, \gca{in terms of the reward and state}, to devise a new data-placement policy. 
To extend \namePaper for three storage devices, we had to only (1) add a new action in \namePaper's action space, and (2) add the remaining capacity in the \textsf{M} device as a state feature. \gon{We conclude that \namePaper provides \gca{ease of extensibility} \rcamfix{to new storage \gonz{system} configurations, which} reduces the system architect's burden in designing sophisticated data placement mechanisms.}  %\gor{Third, \mbox{\namePaper} provides a higher benefit-cost ratio in devices with a larger latency gap by avoiding the eviction penalty. Therefore, \mbox{\namePaper} can efficiently use hybrid storage devices to reduce the total cost of ownership. }  



==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/explainability.tex <==
 
\section{Explainability Analysis}
% \subsection{Explainability Analysis: Demystifying \namePaper}
 \label{sec:Sibyl/explanability}
%In this section, we provide intuition into \namePaper's internal mechanism. 
We perform an explainability analysis to understand our results further and explain Sibyl’s decisions. %\footnote{\juancr{Providing rigorous explainability to reinforcement learning-based mechanisms is an active field of research~\cite{verma2018programmatically,liu2018toward,juozapaitis2019explainable,madumal2020explainable,sequeira2020interestingness,puiutta2020explainable}, a problem that is beyond the scope of this paper.}}. 
We extract \namePaper's actions for different workloads under \hmssd and \hlssd~ \gon{HSS configurations and analyze the page placements for each workload}. 
%under different HSS configurations}. %However, providing rigorous explainability to reinforcement learning-based mechanisms is an active field of research~\cite{verma2018programmatically,liu2018toward,juozapaitis2019explainable,madumal2020explainable,sequeira2020interestingness,puiutta2020explainable}, a problem that is beyond the scope of this paper. } 
Figure~\ref{fig:Sibyl/explain} shows \gon{\namePaper's preference for \rcamfix{the} fast storage \rcamfix{device} over \rcamfix{the} slow storage \rcamfix{device}, measured as the} ratio of the  number of fast storage placements to the \gont{sum of the number of placements in \rcamfix{both} fast and slow storage devices} \gon{(i.e., $\text{Preference=}\frac{\# \text{fast placements}}{\# \text{fast}+\# \text{slow placements}}$)}.

% \renewcommand{\thefigure}{14}
\begin{figure}[h]
% \vspace{-0.3cm}
  \centering
    \includegraphics[width=1\linewidth,trim={0.2cm 0.2cm 0.2cm 0.2cm},clip]{Sibyl/images/isca'22/rl_action_update_6.pdf}
  \caption{\namePaper's preference for the fast {storage device} under different \gon{HSS} configurations}
\label{fig:Sibyl/explain}
\vspace{-0.1cm}
 \end{figure}


% \renewcommand{\thefigure}{15}
  \begin{figure*}[h]
    %   \vspace{-1em}
\centering
\begin{subfigure}[h]{.85\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Sibyl/images/isca'22/evicts1_new_4.pdf}
   \vspace{-0.8cm}
  \caption{\textsf{H\&M} \gon{HSS configuration}
  \label{fig:Sibyl/evict_1}}
\end{subfigure}%

\begin{subfigure}[h]{.85\textwidth}
  \centering
%   \vspace{-0.2cm}
  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{Sibyl/images/isca'22/evicts2_new_4.pdf}
   \vspace{-0.8cm}
   \caption{\textsf{H\&L}  \gon{HSS configuration}
  \label{fig:Sibyl/evict_2}}
\end{subfigure}
%   \vspace{-0.1cm}
\caption[Two numerical solutions]{Comparison of evictions from the fast storage \gon{to the slow storage} (normalized to the total number of \gon{storage requests}) \label{fig:Sibyl/evict}}
% \vspace{-0.7cm}
\end{figure*}

We make the following four observations. 
First, in the \js{\textsf{H\&L}} configuration, where the latency difference is large {between the two storage devices}, \namePaper~ \gon{prefers} to place \gon{more} data in the fast \gon{storage} device. \namePaper learns that despite the eviction penalty, the benefit of serving more requests from the fast \gon{storage} device is significant. On the other hand, in the \js{\textsf{H\&M}} device configuration, where the latency difference between two devices is smaller compared to \rakesh{\textsf{H\&L}}, \namePaper places only performance-critical pages in the faster \rcamfix{storage device} to avoid the eviction penalty.  


Second, \rcamfix{in the} {\textsf{H\&M}} configuration, \namePaper~shows less preference to place pages from  \texttt{mds\_0}, \texttt{prn\_1}, \texttt{proj\_2}, \texttt{proj\_3}, \texttt{src1\_0}, \texttt{stg\_1}, and \texttt{web\_1}  in \juan{the} fast storage \gon{device}. These workloads \gonz{are} cold and sequential (Table~\ref{tab:Sibyl/workload}) \gonz{and thus} \gon{are less suitable for} the fast storage \gon{device}. Therefore, \gon{for such workloads}, \namePaper shows more preference for  \gon{the} slow storage \gon{device}. \rcamfix{In contrast,} for hot and random workloads (\texttt{prxy\_0} and \texttt{prxy\_1}), \namePaper shows \rcamfix{more} preference to place \rcamfix{pages} in the fast \gon{storage} device.

% Third, \gor{\namePaper} leverages asymmetry in R/W latencies to make data-placement decisions to place pages of workloads with low \rcamfix{number of} unique requests {\texttt{hm\_1}}, {\texttt{proj\_0}}, and {\texttt{prxy\_0}} in the fast storage.

Third, for \texttt{rsrch\_0}, \texttt{wdev\_2}, and \texttt{web\_1}, \namePaper~ \gonzz{places} \gonff{$\le$40\%} \gon{of pages} in the fast storage \gon{device}. Such requests have random access patterns, while pages with cold and sequential accesses are \gonzz{placed in the} slow storage. 
%: (1) {\namePaper} places {\texttt{proj\_0}} in the fast storage as it has only a few unique write requests with high write update frequency (Table~\ref{tab:workload}), and (2) {\texttt{hm\_1}} is a read-intensive workload with a low average write access frequency.  However, this workload has a small number of unique pages. A heuristic-based approach (such as {\cde} and {\hps}) would serve all the pages from the high-capacity device (i.e., slow \gon{storage} device) because of the low average access frequency. In contrast, {\namePaper} performs dynamic decisions and serves more requests from the fast \gon{storage} device.  } 

\gont{Fourth},  in the \js{\textsf{H\&L}} setting, \namePaper shows more preference to \gonzz{place} requests in the fast \gon{storage} device, except for \texttt{proj\_2} and \texttt{src1\_0}  workloads. {We observe that these two workloads \gonff{are} \gon{highly random with} a low average access \gonz{count} (Table~\ref{tab:Sibyl/workload}). Therefore,  aggressive placement in \gonzz{the}  fast storage is not beneficial for  long-term performance.  }
%We observe that these two workloads have a significantly higher number of unique random write requests (\textit{ref.} Table~\ref{tab:workload}). Therefore, an aggressive placement of data in the faster storage, even though these two workloads are cold and sequential, is not beneficial for long-term performance.   }




%\js{without high dependence on workload and device characteristics, as shown in Figure~\ref{fig:Sibyl/perf}.} % and maximize the overall long-term performance.

%\noindent\textbf{\nh{Number} of evictions:} 
%In Figure~\ref{fig:Sibyl/evict} we show the \nh{number} of evicts that occur while using \namePaper~and other baseline policies. We make following two observations. 
\js{We also measure} the number of evictions \gonff{(as a \gonz{fraction} of all storage requests)} that occur while using \namePaper~and other baseline policies, as shown in  Figure~\ref{fig:Sibyl/evict}. 
We make two observations. First, \gon{in \gonff{the} \hmssd HSS configuration, \namePaper~\gonff{leads to} 68.4\%, 43.2\%, 19.7\%, and 29.3\% \gonff{fewer} evictions from the fast storage than \cde, \hps, \arc, and \kleio, respectively. }
Second, \cde places more data in the fast \gon{storage}, which leads to a \js{large} number of evictions in both \gon{HSS} configurations. However, if the latency difference between the two devices is large (e.g., \js{\textsf{H\&L}} configuration), \gon{\cde} provides higher performance than other baseline policies (see Figure~\ref{fig:Sibyl/perf}(b)). 
Therefore, in the \js{\textsf{H\&L} HSS configuration}, we observe \gonzz{that}~\namePaper follows a similar policy, leading to more evictions compared to other baselines. 
% Second, in the \js{\textsf{H\&M} configuration}, where the device latency difference is small, \namePaper provides better performance (Figure~\ref{fig:Sibyl/perf} and Figure~\ref{fig:Sibyl/iops}) while performing \js{fewer} evictions on average.


% \gon{From our explainability analysis, we conclude that \namePaper provides (1) adaptivity by continuously learning from and adapting to the workload and the storage device characteristics, and (2) easy extensibility
% to a wide range of workloads and HSS configurations. Thus, \namePaper provides better performance \nh{than prior data-placement techniques.}} %, as shown in Figures~\ref{fig:Sibyl/perf} and \ref{fig:Sibyl/iops}.} %dynamic{ally adapt} \gon{its} {data-placement} \gon{policy} {taking into account} \emph{both} the {underlying} device  and the workload characteristics. Thus, \namePaper provides better performance \nh{than prior data-placement techniques}. %, as shown in Figures~\ref{fig:Sibyl/perf} and \ref{fig:Sibyl/iops}.



%This can be easily stored in the internal DRAM of an SSD.
%If we would like \namePaper~to learn continuously from an environment we would have additional cost of an experience buffer to maintain a table of 1k entries. Total area overhead of online \namePaper~would be 2.5 MB.

\section{Overhead Analysis}
\label{sec:Sibyl/overhead_analysis}
% \gon{We analyze the \gont{inference and training latencies} and area overhead of \namePaper. }
%\noindent\textbf{Computational Overhead:}
% \hg{TensorFlow-GPU is used to deploy QRator. As mentioned in Section \ref{}, the mechanism is divided into collection phase and learning phase. Once, deployed the neural network retraining is triggered after every 500 sec and takes 100 msec per iteration. When triggered this training, happens in parallel with  which we found empirically. work in parallel. Therefore, the }
% \vspace{0.05cm}

\subsection{Inference and Training Latencies} 
The input layer \gon{of the} \gonz{training}  and inference network\gont{s} consists of \js{six} neurons, \gont{equal} to the number of features \js{listed} in Table~\ref{tab:Sibyl/state}. \gont{Each feature is} normalized to transform the \gont{value} range of different features to a common scale. { The size of one state entry is 40 bits (32 bits for state features and 8 bits for the counter used for tracking \gonzz{the remaining capacity in the} fast storage device).  We make use of two hidden layers with 20 and 30 neurons each. The final output layer has neurons equivalent to our action space, \gca{ i.e., two for \gont{dual-HSS} configurations and three for \gont{the} tri-HSS configurations}. 

\head{Inference \gonff{latency}} Our inference network has 52 \gont{inference} neurons (20+30+2)  with 780 \gon{weights} (6$\times$20+20$\times$30+30$\times$2). %1460 synapses ($40\times20+20\times30+30\times2$). 
{As a result, {\namePaper} requires 780 MAC operations per inference (1$\times$6$\times$20+1$\times$20$\times$30 +1$\times$30$\times$2). On our evaluated \gont{CPU}, we can perform these operations in $\sim$10ns, which is several orders of magnitude smaller than the I/O read latency of even a high-end SSD ($\sim$10us)~\cite{inteloptane, samsung2017znand}.} %On our evaluated system,  we observe an average increase of 3.2\% and  2.6\%  in the overall latency while using onboard CPU and GPU, respectively.
\gca{\gont{\namePaper's inference} computation can also be performed in the SSD controller.}
% \gca{The CPU can also perform this computation in an SSD management unit.} 

\gor{{\noindent{\head{Training \gonff{latency}}}  For each training step, \mbox{\namePaper} needs to compute 1,597,440 MAC operations, where each batch requires 128$\times$6$\times$20+ 128$\times$20$\times$30+128$\times$30$\times$2 MAC operations. % (each training step is composed of \gca{8 batches for an experience buffer of 1000 experiences with a batch size of 128}). 
This computation takes $\sim$2us on our evaluated \gont{CPU}. %(AMD Ryzen 3 CPU with 942 GFLOPS of compute throughput). 
\gonff{This} training latency does not affect the \gonff{benefits} of \mbox{\namePaper}
%due to \gca{the following} two reasons. 
\rcamfix{because (1)}
%First, the 
training occurs asynchronously \rcamfix{with} inference, \gonzz{and}
%Second, the 
\rcamfix{(2)} training latency is \gonff{$\sim$5$\times$} smaller than the I/O read latency of even a high-end SSD.  }}

% Therefore, our optimized implementation does not throttle the overall system performance.
\noindent\gonff{We conclude that Sibyl's performance benefits come at small latency overheads that are easily realizable in existing CPUs.}
% \gon{We conclude that \namePaper’s performance benefits come at a negligible cost in performance overheads.}

% As discussed in Section~\ref{sec:mechanism}, training of the exploration network occurs asynchronous to the inference performed by the inference network. Therefore, training is not in the critical path. % {Therefore, we use TensorFlow-GPU to deploy \namePaper.  }  }

\vspace{-0.35cm}
\subsection{Area Overhead} 

\noindent{\head{Storage cost}} We use a half-precision floating-point format for the weights \gon{of the \gonz{training} and the inference network\rcamfix{s}}. With 780 16-bit weights, \rcamfix{each} neural network requires 12.2 KiB of memory. %\gca{For the inference network, we require 12.2 KiB ($16\times780$)}. 
Since we use 
%a similar 
\rcamfix{the same} network architecture for the \gonz{two} networks, we need 24.4 KiB of memory. In total, with an experience buffer of 100 KiB (Section \ref{subsec:Sibyl/detail_design}), \namePaper require\rcamfix{s} \gonzz{124.4} KiB of \gont{DRAM} overhead, \js{which is negligible compared to {the} memory size of modern computing systems}.  } %As mentioned in Section~\ref{sec:mechanism}, the mechanism is divided into the collection and learning phases, which run in parallel. 




\noindent{\head{Metadata cost}} HSSs need to maintain the address mapping information for the underlying storage devices~\cite{tsukada2021metadata}.  {\namePaper} \gonff{requires} 40 bits to store  \gont{state information} (\gonff{i.e., the per-page state features;} see Table~\ref{tab:Sibyl/state}). This overhead is $\sim$0.1\% of the total storage capacity when using a 4-KiB data placement granularity (5-byte per 4-KiB data). % Note that, as explained in Section~\ref{sec:mechanism}, our replay buffer requires access to 1,000 entries of the most recent page requests, so  {\namePaper} training requires only 16-KiB of data.



\noindent\gon{We conclude that \namePaper~\gon{has \gonzz{a} very} modest cost in \gon{terms of} \gon{storage capacity} overhead \gon{in \gonz{main memory (DRAM)}}.}



==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/introduction.tex <==
\section{Introduction}
\label{sec:Sibyl/introduction}
%Architecting 
%Hybrid storage systems (HSS)~\cite{qureshi2009scalable,bailey2013exploring,smullen2010accelerating,lu2012pram,tarihi2015hybrid,xiao2016hs,wang2017larger,lu2016design,luo2015design,srinivasan2010flashcache,reinsel2013breaking,lee2014mining,felter2011reliability,bu2012optimization,canim2010ssd,bisson2007reducing,saxena2012flashtier,krish2016efficient,zhao2016towards,lin2011hot,chen2015duplication,niu2018hybrid} use multiple different storage devices to achieve high and scalable storage capacity at high performance. 
Hybrid storage systems (HSS) take advantage of both \gon{fast-yet-small} storage devices and large-yet-slow storage devices to deliver high storage capacity at low latency~\cite{meza2013case,bailey2013exploring,smullen2010accelerating,lu2012pram,tarihi2015hybrid,xiao2016hs,wang2017larger,lu2016design,luo2015design,srinivasan2010flashcache,reinsel2013breaking,lee2014mining,felter2011reliability,bu2012optimization,canim2010ssd,bisson2007reducing,saxena2012flashtier,krish2016efficient,zhao2016towards,lin2011hot,chen2015duplication,niu2018hybrid, oh2015enabling,liu2013molar,tai2015sla,huang2016improving,kgil2006flashcache,kgil2008improving,oh2012caching,yang2013hec,ou2014edm,appuswamy2013cache,cheng2015amc,chai2015wec,dai2015etd,ye2015regional,chang2015profit,saxena2014design,li2014enabling,zong2014faststor,do2011turbocharging,lee2015effective,baek2016fully,liu2010raf,liang2016elastic,yadgar2011management,zhang2012multi,klonatos2011azor}. The key challenge in designing a high-performance and cost-effective hybrid storage system is to accurately identify the performance-critical\gon{ity} of  application \gon{data} and place \gon{data} in the ``best-fit'' storage device~\cite{niu2018hybrid}. 

%Data placement across different devices is critical to maximize the benefits in such a hybrid system.
%\go{A hybrid storage system (HSS)  aims to combine the benefits of different storage devices in a cost-effective manner. }%(i.e., {using} multiple {heterogeneous} storage {devices}) %is 
%\juangg{are} a \gf{potential} %\jgll{Still promising? Not already a good existing solution?} 
%HSS provide high performance \gf{of modern computing systems} at low cost. 
%\gup{Such systems take} advantage of both small-yet-fast storage devices and large-yet-slow storage devices. 
%Hybrid storage systems make the data allocation significantly more challenging \gf{due to two key reasons: (1) where to} allocate the data, and (2) when to migrate data between the devices. 
%In order to successfully deliver high storage capacity at low latency, HSSs  must make intelligent data placement decisions. A desired data-placement technique should be able to accurately \emph{predict} the future I/O-access pattern in order to store 
%frequently-accessed
%performance-critical
%data in the fast storage device while avoiding unnecessary data migration between different storage devices.

{Past works~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,doudali2019kleio,ren2019archivist,cheng2019optimizing,raghavan2014tiera,salkhordeh2015operating,hui2012hash,xue2014storage,zhang2010automated,zhao2010fdtm,shi2013optimal,wu2012data,ma2014providing,iliadis2015exaplan,wu2009managing,wu2010exploiting,park2011hot}  propose many different data placement techniques to improve the performance of an HSS. We identify \gon{two major} shortcomings \gon{of} prior proposals that significantly limit their performance: \gonn{lack of (1) adaptivity \gonzz{to workload changes and the storage device characteristics,} and (2) extensibility.}


\head{(\gon{1a}) Lack of adaptivity \gca{to workload changes}} \gon{To guide data placement, past techniques consider only a limited number of \gon{workload} characteristics} ~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,lv2013hotness,montgomery2014extent}.
%largely ad-hoc and
%Designers statically tune the \gon{parameter} values of all  considered \gon{workloads} at design time based on
Designers statically tune the {parameters values} for all considered \gon{workloads} at design time based on
%their prior 
\rcam{empirical analysis and designer} experience, and expect those {statically-fixed values} to be equally effective \rnlast{for} a wide range of \rcam{dynamic }\gon{workload \rcam{demands}} and system configurations seen in the real world. As a result, such data placement techniques \gon{cannot easily} adapt 
%to cater 
\rakeshisca{to} a wide range of \gonn{dynamic} \gon{workload} demands and significant\gon{ly} \gon{underperform}  when compared to an oracle technique that has \gon{complete} knowledge of future \gon{storage} access patterns (up to $41.1\%$ lower performance, \gonn{ref.} Section \ref{sec:Sibyl/motivation_limitations}).%\rakeshisca{~Few sophisticated supervised-learning data-placement techniques~\cite{doudali2019kleio,ren2019archivist} lose their accuracy when the workload characteristics change and these techniques need frequent retraining of the supervised learning models.}

% \head{(1) Lack of adaptability} \rakeshisca{Many} prior data-placement techniques are %largely ad-hoc and 
% heuristic-driven~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014}. Designers statically tune the values of all of the heuristics at design time based on their prior experience and expect those statically-fixed heuristics values to be equally effective in a wide range of applications and system configurations seen in real world. As a result, such data-placement techniques lose adaptability to cater \rakeshisca{to} a wide range of application demands and leave a significant performance headroom when compared to an oracle technique that has the knowledge of future access patterns  (up to $41.1\%$ lower performance as we show in Section~\ref{sec:motivation_limitations}).%\rakeshisca{~Few sophisticated supervised-learning data-placement techniques~\cite{doudali2019kleio,ren2019archivist} lose their accuracy when the workload characteristics change and these techniques need frequent retraining of the supervised learning models.}

\head{(\gon{1b}) \gon{Lack of adaptivity to changes in device types and configurations}} Most prior \gon{HSS} data placement techniques \gonn{(e.g.,~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,doudali2019kleio,ren2019archivist})}
%are purely agnostic to
\rakeshisca{do not adapt well to changes in the}
underlying storage device characteristics (e.g., \gonn{changes in the level of} asymmetry in the \mbox{read/write} latenc\gonzz{ies},  \gon{or the number and types of storage devices}%\gca{ change in latencies on replacing hybrid storage devices}
). As a result, \rcam{existing techniques} cannot effectively take  into account the cost of data \gca{movement} between  storage devices while making data placement decisions. This lack of %awareness
\rcam{adaptivity} leads to highly inefficient data placement policies, especially in HSSs with significantly-different device access latencies \gon{than what prior techniques were designed for} (as show\rcam{n} in Section \ref{sec:Sibyl/motivation_limitations}). %\jgll{This is about device characteristics and also HSS characteristics. It is surprising that past works do not consider the cost of data movement. Btw, this seems to be a different issue than the asymmetry of read/write, which is a single device characteristic.} %gaganF{updated a bit}

\head{(2) Lack of extensibility} A large number of prior \gon{data placement} techniques \rcam{(e.g., ~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014})} are typically designed for an HSS that consists of only two storage devices. As modern HSSs \gon{already} incorporat\gon{e} more than two types of storage devices\rakeshisca{~\cite{ren2019archivist, matsui2017tri, matsui2017design}}, system architects need to put significant effort into extending prior techniques to accommodate more than two devices. We observe that a \rcam{state-of-the-art} heuristic-based data placement technique optimized for an HSS with two storage devices~\cite{matsui2017tri} often leads to \gf{suboptimal} performance in an HSS with three storage devices (up to \gonzz{48.2}\% lower performance, \gonn{ref.} Section \ref{subsec:Sibyl/trihybrid}).  

\textbf{Our goal} is to develop a new, efficient, and high-performance data placement mechanism for hybrid storage systems that \gonn{provides} (1) \gon{\emph{adaptivity}}\gonn{,}  %\go{dynamically} %autonomously learn to  derive a data-placement strategy 
by \emph{continuously learning} from and {adapting to} the \gon{workload and  storage device characteristics,} and  (2) \emph{\gon{easy extensibility}} to a wide range of \gon{\gon{workloads} and HSS} configurations.
}


\textbf{Key ideas.} To this end, we propose \namePaper, %\footnote{In Greek mythology, Sibyl is an oracle who prophesied with divine inspiration.}, 
a reinforcement \linebreak learning-based data placement technique for hybrid storage systems.\footnote{In Greek mythology, \namePaper is an oracle who makes accurate prophecies\rcam{~\cite{wiki:Sibyl}}.} Reinforcement learning (RL)~\cite{sutton_2018} is a goal-oriented decision-making process in which an autonomous agent learns to \gon{take} optimal actions that maximize a reward function by interacting with an environment.    {The key idea of \namePaper is to design the data placement module in hybrid storage systems as a reinforcement learning agent that \emph{autonomously learns} and adapts to the best-fit data placement policy for the \gon{running} \gon{workload} and \gon{the current} hybrid storage \gonn{system} configuration.} %\jgll{No need to motivate RL? Is RL the only way of achieving the goal?}
%\textbf{The key idea} of \namePaper{} is to enhance the hybrid storage system with a \emph{data-placement module} that automatically \emph{learns} the best-fit data placement (i.e., which data should be stored in the fast/slow {device}), to achieve high performance while minimizing the migration overhead, by taking into account the workload and the hybrid storage characteristics. To do so, we design the data-placement module as an RL agent that utilizes its past experience to  perform future data-placement decisions.   
For every storage \gon{page} access,  \namePaper observes
different features from the running \gon{workload} and the underlying storage system (e.g., access \gonz{count} of the current request, \gon{remaining capacity in the fast storage, etc.}). \rbc{It uses the features as  \textbf{\emph{state}} information to \gon{take} a data placement \textbf{\emph{action}} (i.e., which device to place the page into). \gont{For every action,} \namePaper receives 
%a system level feedback,
a \gon{delayed} \textbf{\emph{reward}}} from the system in terms of per-\gup{request} latency. %\jgll{"latency per request"?}.
\gca{This} reward encapsulates the internal device characteristics  of \juanggg{an} HSS (such as read/write latenc\rcamfix{ies}, latency of garbage collection, \rcamfix{queuing delays,} \gont{error handling latencies,} and write buffer state). \namePaper uses this reward to estimate
the long-term impact of its \gon{action (i.e., data placement} decision\gon{)} on the overall application performance \gup{and continuously optimizes its data placement policy online} \gon{to maximize the long-term benefit \gonn{(i.e., reward)} of its actions}.
%to improve performance}.  
\iffalse
While \namePaper can incorporate any system level information in its decision making process \jgll{Would there be any benefit from doing so? This gives the impression that there may be better information to use.}, to minimize the implementation overhead, we demonstrate \namePaper using: (1) the most correlated \jgll{Meaning?} application features as the state information, and (2) the reward to provide information on the internal state of the hybrid storage system \jgll{Not clear. Request latency is the only possible reward providing information on the internal state?}.
\fi
% \subsection{Challenges of Using RL for Data Placement}

\rbc{\textbf{Benefits.}} %An RL-based design 
\rbc{Formulating the data placement module as an RL agent} \rbc{enables a human designer} to specify only \emph{what} performance objective \rbc{the} data placement module should target, rather than designing and implementing a new data placement \gon{policy} that requires \gca{explicit specification of} \emph{how}  to achieve the performance objective. The use of RL not only \gon{enables} the data placement module to \emph{autonomously} learn the ``best-fit'' data placement strategy for a wide range of \gon{workloads} and hybrid storage \gon{system} configurations but also significantly reduces the burden of a human designer \gon{in finding a good data placement policy}. %\jgll{And RL is the only way of doing this?}
%The RL agent works autonomously using the provided features and system level feedback to reach the objective without any human intervention. 

\rbc{\textbf{Challenges.}} While RL provides a promising alternative to existing data placement techniques, we identify two main  challenges in applying RL to data placement in an HSS. 


\head{(1) Problem formulation}  The RL agent's effectiveness depends on how the data placement problem is cast as a reinforcement learning-based task. Two key issues arise  \gonn{when} formulating \gon{HSS} data placement as an RL problem\rnlast{:}  (1) \gonn{taking into account} the \gonn{latency} asymmetry \gonn{within and across} storage devices, and (2) deciding which actions to reward and penalize (\gca{also known as the} \emph{credit assignment problem}~\gca{\cite{minsky1961steps}}). %\jgll{Meaning?}. 
First, we need to make the agent aware of the asymmetry in read and write latencies of \gon{each} storage \gon{device} and \gonx{the} differences in latencies across \gon{multiple} storage devices. Real-world storage devices could have \gon{dynamic} latency variations due to their complex hardware and software components (e.g., internal  caching, garbage collection, \gon{error handling, multi-level cell reading,} etc.)~\cite{cai2015data,grupp2009characterizing, jung2012nandflashsim, cai2014neighbor, cai2017error, cui2017dlv, Cai2018, park2021reducing}. %\jgll{Any reference that shows those high latency variations?}} 
Second, \gonn{if the fast storage is running \gonzz{out} of free space, there might be evictions \gup{in the background} \gon{from} the fast storage to the slow storage.%while the agent performs data placement decisions.

%,  \gon{device, if it} is running out of free space. % \jgll{Isn't the agent aware of the evictions? Why aren't they handled by the agent too?} %Therefore, the agent will perform a multitude of decisions. 
\gon{As a result, when} we reward the agent, \gon{not only there is a \gon{variable} \gonn{and delayed} reward,% comes with a variable delay, 
~but} it is \gon{also} hard to properly \gon{assign} \emph{credit} or \emph{blame} \gon{to} different decisions.

\head{(2) Implementation overhead} A \gon{workload} could have \gon{hundreds of} thousands \rcam{ of} pages \gon{of \gonn{storage} data}, making it challenging to efficiently handle the large data footprint with a low design overhead \gon{for the learning agent.} %\jgll{Why? Can you give an intuition of how the data footprint impact the implementation overhead?}

 
 
%To address the above challenges, we make use of five techniques. 
To address the first challenge, we use two \gon{main} techniques. First, we design a \textit{reward} structure in terms of \emph{request latency}, \gon{which} allows \namePaper~to learn the \gon{workload and storage} device characteristics %while being aware of the changes in an application
\nh{when} \gonn{continuously and frequently} interacting with a hybrid storage system. We  \gca{add} a negative penalty \gca{to the reward structure} in case of eviction, \gonn{which helps  \gca{with handling} the credit assignment problem and \gont{encourages the} agent \gont{to} place only performance-critical pages in the fast storage.} {Second, we perform thorough hyper-parameter tuning \gon{to find parameter values that work well for a wide variety of workloads.}} %\jgll{Sounds like giving contradicting hints (if there is an eviction after a data placement decision that would be good if no eviction). Do we evaluate the agent under circumstances with frequent evictions?} 
To address the second challenge, we use two main techniques. First, we divide states into a small number of bins that reduce \gon{the} state space, which directly \gon{affects}  the implementation overhead. {Second, instead of adopting a traditional table-based RL approach  (e.g., \cite{ipek2008self}) to store \gonn{the} agent's state-action information (collected by interacting with \gon{an HSS})\gonn{, which} can \gonn{easily} introduce significant performance overhead\gonn{s in the presence of}  a large \gont{state/action} space}, we use a {simple} feed-forward neural network~\cite{zell1994simulation} with only two hidden layers of 20 and 30 nodes, respectively. % \jgll{Using the NN is a novelty of us or can we cite something here?}. %\jgll{What is the table for and what is the NN for?} 
% For the third challenge \jgll{Third challenge? We only mention 2 challenges above.} we implement a light-weight custom block driver that receives the placement decision from \namePaper and performs direct IO to the target device. The use of direct IO data transfers provides three key benefits: 1) keeps the implementation overhead minimal, (2) reduces the CPU interrupt overhead, (3) eliminates the memory allocation and copy operations that are inherent in buffered IOs.

% \subsection{Key Results and Contributions}

\textbf{Key results.}} \gup{We  evaluate \namePaper~\gf{using \gon{two different dual-HSS} configurations and two different tri-HSS configurations.} We use fourteen diverse \gon{storage} traces from \rakeshisca{Microsoft Research Cambridge (MSRC)} \cite{MSR} collected on real enterprise servers. \gon{We  evaluate \namePaper on workloads from  FileBench~\cite{tarasov2016filebench} on which it has never been trained}. \gon{We compare \namePaper to four state-of-the-art data placement techniques.} We demonstrate four key results. \gon{ First, \namePaper~\gonn{ provides \gonzz{21.6\%/19.9\%} performance improvement in a performance-oriented\gonn{/ cost-oriented} HSS configuration %and 23.2\% performance improvement in cost-oriented HSS configuration 
 compared to the best previous data placement technique.}} % \namePaper~\gon{ provides 19.9\% performance improvement in a performance-oriented HSS configuration and 23.2\% performance improvement in cost-oriented HSS configuration compared to the best previous data-placement technique.}}
%First, \gca{in} a performance-oriented HSS \gca{configuration}, \namePaper provides 19.9\%-36.1\% performance improvements compared to prior data-placement techniques. While using a cost-oriented HSS \gca{configuration}, \namePaper improves performance by 23.2\%-68.8\%. %\jgll{Never talked about this technique until now. All motivation is about human-designed heuristics. Anyway, calling Kleio the SotA is not accurate, since it is for a different problem. It would have been much better to say that we also explore an RNN-based policy (which has used for memory but not for storage). It would be one more contribution of this work, and would get away the criticism about comparing to Kleio.}. 
Second,  \namePaper outperforms the best-performing supervised learning-based technique  \gon{ on workloads it has never been trained on} by 46.1\% and 54.6\%, on average, } \gon{in} performance-oriented and cost-oriented HSS \gca{configurations, respectively}. %Compared to a learning-based policy, \namePaper provides 76.7\% higher performance. 
%Current learning-based policies are designed for specific applications and/or system scenarios that lead to many mispredictions when used in a different scenario.
Third,  \namePaper provides 23.9\%-48.2\% higher performance in tri-hybrid storage systems than a \gonn{state-of-the-art} heuristic-based \gon{data placement} technique \gonn{demonstrating that} \namePaper \gon{~is} \gonn{easily} extensible and alleviates the designer's burden in \gon{finding} sophisticated data placement mechanisms \gon{for new and complex HSS configurations}. Fourth, \namePaper's performance benefits come with a low \gagan{storage} implementation overhead of only \gonzz{124.4} KiB. %\go{, which is able to satisfy} \rbc{ latency requirement of a data placement module for an HSS}.} %\jgll{What is the "latency requirement of a data placement module"? Is this that we are evaluating QoS and SLA?}

\vspace{0.2em}
\noindent This work makes the following  \textbf{major contributions}:
%\vspace{-0.1cm}
\begin{itemize}[leftmargin=*, noitemsep, topsep=0pt]
 \item  We show on real \gonn{hybrid storage systems (HSSs)}  that prior state-of-the-art \gont{HSS data placement mechanisms} fall 
 %short significantly than the oracle
  short of the oracle placement due to: lack of  \gon{(1) adapt\gonn{i}vity to workload changes and \gonn{storage device characteristics}, and (2) extensibility. } %(1) strict policies that take into account only a certain aspect of the application or the system, (2) no system-level feedback, and (3)  lack of extensibility.
  \item We propose \namePaper%\footnote{We plan to open-source \namePaper upon paper acceptance.}
  , a new self-\gon{optimizing}  mechanism %for %effective data placement in hybrid storage systems 
  \gon{that uses} reinforcement learning \gon{to make data placement decisions in hybrid storage systems}. \namePaper{} %\juang{data-placement module} 
  \go{dynamically}
  \emph{learns}\gont{,} \gonn{ using both multiple workload features and system-level feedback information\gont{, how} to continuously adapt its policy to improve \rnlast{its} long-term performance \rnlast{for} a workload.}
    
    \item We conduct an in-depth evaluation of \namePaper on \gon{real \gonn{systems with various} HSS configurations\gont{,}} showing that it outperforms \gonn{four} state-of-the-art %heuristic- and learning-based 
    techniques over a wide variety of applications with a low implementation overhead.
    \item We provide an \rbc{in-depth} explanation of \namePaper's actions that show that \namePaper performs dynamic data placement decisions by learning \gonn{ changes in the level of asymmetry in the read/write latenc\gonzz{ies} and the number and types of storage devices.} % the asymmetry in the read/write latencies present in \rbc{modern} hybrid storage devices. % while taking into account the inherent application characteristics.
    \item \gca{ We \gon{freely} open-source \namePaper to aid % RL-based research in hybrid storage systems. 
 {future research \gon{in} data placement for storage systems~\cite{sibylLink}}.} %\MYhref[black]{https://github.com/CMU-SAFARI/Sibyl}{https://github.com/CMU-SAFARI/Sibyl}}} \jgll{You can better have this link as a citation. You can cite it from other parts of the paper too.}
    
    \end{itemize}
 

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/motivation.tex <==
\section{Motivation}\label{sec:Sibyl/motivation_limitations}
% We first motivate our \namePaper{} \gagan{approach} with an empirical study to assess the effectiveness of existing data-placement techniques for hybrid storage systems {with diverse} workloads.
% We then {argue} why RL is a promising {approach }to overcome the limitations of existing techniques.
% \gup{We motivate our RL-based approach for \acrshort{hss}s.} % 

 



% \head{(1) Rigid techniques without system awareness}

To assess the effectiveness of existing \gon{HSS} data placement techniques under diverse workloads and hybrid storage configurations, we evaluate {state-of-the-art } heuristic-based (\emph{\cde}~\cite{matsui2017design} and \emph{\hps}~\cite{meswani2015heterogeneous}) and supervised learning-based  (\emph{\arcc}~\cite{ren2019archivist}) techniques. We also implement an RNN-based data placement technique (\kleio), adapted from hybrid main memory~\cite{doudali2019kleio}. To evaluate the effect of underlying storage device technologies, we use {three  different storage devices}: high-end {(\textsf{H})}~\cite{inteloptane}, middle-end {(\textsf{M})}~\cite{intels4510}, and low-end {(\textsf{L})}~\cite{seagate}, configured into two different hybrid storage configurations: a performance-oriented HSS (\hmssd) and a cost-oriented HSS (\hlssd).  %{We use a real} {system with two different hybrid storage {configurations},\footnote{Section~\ref{sec:evaluation} describes our evaluation methodology.}  as shown in
Table~\ref{tab:Sibyl/devices} provides details of our system and devices. We restrict the fast storage capacity to 10\% of the working set size of a workload, which ensures eviction of data from  fast storage to slow storage when  fast storage capacity is full.
% in Figure~\ref{fig:motivation_iops}.}} %trace-driven simulator that faithfully models a hybrid storage system consisting of two different storage devices.}
%an Intel 3D XPoint-based SSD~\cite{} and an Intel 3D TLC NAND flash-based SSD~\cite{}.}
%We implemented two most widely used algorithms for data placement. 




% {The first technique, called \emph{cold data eviction (CDE)}~\cite{matsui2017design}},
% %The first algorithm is cold data eviction  (CDE)~\cite{matsui2017design,sun2013high} that 
% separates write-hot or random data from cold and sequential data in a hybrid storage system. 
%In this algorithm, hot or random write requests are written to the faster storage. 
{\cde}~\cite{matsui2017design} \gon{allocates} hot or random write requests in the faster storage, {whereas} cold and sequential write requests are evicted to the slower device. 
\hps~\cite{meswani2015heterogeneous} uses the access \gonz{count} \gca{of pages} to periodically migrate cold pages to the slower storage device. %in a scheduling \emph{epoch}. 
\arcc~\cite{ren2019archivist} uses a neural network classifier to predict the target device for data placement. %performs data placement based on the prediction of target storage device for each request by a supervised neural network classifier.
\emph{\kleio}, adapted from~\cite{doudali2019kleio}, is a supervised learning-based mechanism {that} exploits recurrent neural networks (RNN) to \gca{predict the hotness of a page} \gon{and place hot pages in fast storage}.
We compare the above policies with three extreme \gon{baselines}:
(1) \slow{}, {where all data reside\rcamfix{s in} \gon{the} slow \gon{storage \rcamfix{device} (i.e., there is no fast storage \rcamfix{device})}}, (2) \fast, {where all data resides in \gon{the}  fast \gon{storage} \rcamfix{device}}, {and (3) \textsf{Oracle}}
%, similar} to the B\'el\'ady's cache-replacement algorithm~\cite{belady1966study}
\cite{meswani2015heterogeneous}, which exploits \gon{complete} {knowledge of} future I/O-access patterns  %\gaganRemove{(which is impossible to obtain \juang{in a real scenario})}
{to perform data placement and to }\js{select victim data blocks for eviction from} the fast device. %\jgll{So the oracle handles evictions but Sybil doesn't? Is that a fair oracle?}. 


We identify \gon{two major}  shortcomings \gon{of the \gonn{state-of-the-art} baseline data placement techniques}: \gonzz{lack of (1) adaptivity to workload changes and the storage device characteristics, and (2) extensibility.}

\head{(1a) Lack of adaptivity \gca{to workload changes}} %From \fig{\ref{fig:motivation_iops}}, 
\fig{\ref{fig:Sibyl/motivation_iops}} shows \gonzz{the} \gon{average request} latency of \gon{all} policies, \gon{normalized to \fast,} under two different hybrid storage configurations. \gon{We make the following \gonn{three} observations.}
First, \gon{all the baseline}  techniques are only effective under specific workloads, showing significantly \gonn{lower} performance \gonn{than} \textsf{Oracle} in most workloads.  \cde, \hps, \arcc, and \kleio~achieve comparable performance to \textsf{Oracle} {for specific workloads} \gagan{(e.g.,  \textsf{hm\_1} for \hps~in \textsf{H\&M},  \textsf{usr\_0} for \cde~in \textsf{H\&L}, \gon{\textsf{hm\_1} for \arcc~in \textsf{H\&M}, and \kleio in \textsf{proj\_2} for \cde~in \textsf{H\&L} }). Second, the baselines show a {large} \gon{average} performance \gon{loss} of 41.1\% (32.6\%), 37.2\% (55.5\%), \gonn{39.7\% (66.7\%), and 34.4\% (47.6\%)} \gon{compared} to \textsf{Oracle}'s performance, under the \textsf{H\&M} (\textsf{H\&L}) hybrid {storage} configuration, respectively.} %\gonn{Third, due to unnecessary evictions, baseline techniques can even lead to a worse performance than \slow (e.g., \textsf{hm\_1} and \textsf{proj\_2} for \cde/\hps/\arcc in \hmssd and \hlssd, respectively, and \textsf{hm\_1} for \kleio in \hmssd). 
\gonn{Third, in \hmssd, the baseline techniques provide a performance improvement of only 1.4\%, 7.4\%, 3.5\%, and 11.3\% compared to \slow.  }

\begin{figure}[h]
% \vspace{-0.03cm}
    \centering
 \includegraphics[width=1\linewidth,trim={0.2cm 0cm 0.2cm 0cm},clip]{Sibyl/images/isca'22/latency_motivation_without_qrator_7.pdf}
 \vspace{-0.55cm}
    \caption{Average request latency normalized to \fast~policy} %\jgll{What is "Archivist"?} \jgll{The reference of Fast-only is completely lost in the right plot. A plot that breaks the bar would help here.}}
    \vspace{-0.1cm}
    \label{fig:Sibyl/motivation_iops}
\end{figure} 
{


\gonn{We conclude that \gon{all four baselines} consider only a limited number of \gon{workload} characteristics to construct a data placement technique, which leads to a significant performance gap compared to the \oracle policy. Thus, there is no single  policy that} %would work 
\juangg{works} well for all \gon{the workloads}. 

\gon{To further analyze the characteristics  of our evaluated workloads, %different workloads from MSR Cambridge Traces~\cite{MSR} that are collected from real enterprise servers,
we} plot the \gca{average} hotness (y-axis) and randomness (x-axis) in \fig{\ref{fig:Sibyl/apps}}. %\gsa{These workloads encapsulate the compute time in the form of inter-request intervals.} 
\gagan{We provide details on these workloads in Table~\ref{tab:Sibyl/workload}.} \gonn{  In these workload traces,} each \gon{storage} request is labeled with a timestamp that indicates the time \gonzz{when} the request was issued from the processor core. Therefore, the time interval between two consecutive I/O requests represents the time the core has spent computing.  {We quantify a workload’s hotness (or coldness) using the average access 
%ratio
\rcamfix{count}, \gca{which is} the average \rcamfix{of the access counts of all pages} in a workload; the higher (lower) the average access \rcamfix{count}, the hotter (colder) the workload. We quantify a workload’s randomness using the average request size in the workload; the higher (lower) the average request size, the more sequential (random) the workload. } %\jgll{The relation between request size and randomness is not obvious to me.}
\gon{From \fig{\ref{fig:Sibyl/apps}}\rcamfix{,} we make \rcamfix{the}  following two observations. First, }the average hotness and randomness {vary widely between \gon{workloads}}. \gon{Second, we observe that each of our evaluated \gon{workload}\rcamfix{s}  exhibits highly dynamic behavior throughout its execution. For example, in Figure~\mbox{\ref{fig:Sibyl/dynamic}}, we show the execution \gonn{timeline} of \texttt{rsrch\_0}, \gonn{which \gonx{depicts} the accessed address\gonx{es} and request sizes.} %measured by storage access and request size. 
\gon{We conclude that} an efficient policy needs to incorporate continuous adaptation to highly dynamic changes in workload behavior.}}  %This performance gap is because these approaches {do not} utilize the experience from {past} data-placement decisions for future decisions.


% \begin{figure}[h]
% %   \vspace{-.7em}
%       \centering
%   \includegraphics[width=.8\linewidth]{images/workload_analysis.pdf}
%   %\includegraphics[width=0.6\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/Apps_4.pdf}
%      %\vspace{-0.1cm}
%   %\caption{{Applications categorized by hot versus cold (based on recency and frequency of use), and sequential versus random (based on the size of request}).}
%   \vspace{-.3em}
%   \caption{Workload characteristic of real-world MSRC traces~\cite{MSR}.} %\jgll{The hot/cold workload distinction is pretty weird: I thought a workload has hot and cold pages (in each epoch), not that a workload itself is hot or cold... Something like "Amount of hot pages per epoch" would be more clear. Or maybe it is just a matter of explaining better what a hot/cold workload is.}} %Table~\ref{tab:workload} lists various characteristics of these workloads.}
% \label{fig:apps}
% \end{figure}

\begin{SCfigure}[][h]
  \centering
%  - \hspace{0.5cm}
 \includegraphics[width=0.7\linewidth,trim={0cm 0.02cm 0.2cm 0cm},clip]{Sibyl/images/isca'22/workload_analysis_new.pdf}
 \vspace{-75pt}
 \caption{\gonx{Randomness and hotness} characteristics of real-world MSRC \gonx{workloads}~\cite{MSR}}
\label{fig:Sibyl/apps}
\vspace{1.2cm}
\end{SCfigure}

% {
% \floatsetup{style=BOXED,capposition=beside,capbesideposition={top,right},frameset={\fboxrule2pt\fboxsep1pt},colorframeset=yellowplate,framestyle=colorbox,framefit=yes,heightadjust=object,valign=c}
% \floatsetup{style=plain,framestyle=colorbox,capposition=beside,capbesideposition={top,right},
% framearound=row,colorframeset=white,frameset={\fboxrule0pt},
% framestyle=colorbox,framefit=yes,heightadjust=object,valign=c}
% \begin{figure}[h]
%  \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/isca21/dynamic_rsrch_0.pdf}
%   \caption{Storage access to a logical address and request size during execution of \texttt{rsrch\_0} workload.}
% \label{fig:dynamic}
% \end{figure}
% }

{
\begin{SCfigure}[][h]
  \centering
  \hspace{0.2cm}
 \includegraphics[width=0.6\linewidth,trim={0cm 0cm 0.2cm 0cm},clip]{Sibyl/images/isca'22/dynamic_rsrch_0_3.pdf}
%  \vspace{}
\vspace{-45pt}
  \caption{\gor{\gonz{Timeline of} accessed logical addresses and request sizes during \gont{the} execution of \texttt{rsrch\_0} workload}}
\label{fig:Sibyl/dynamic}
\vspace{0.6cm} 
\end{SCfigure}
}
%   \begin{figure}[h]
%     %   \vspace{-1em}
% \centering
% \begin{subfigure}[h]{.55\textwidth}
%   \centering
%  \includegraphics[width=0.6\linewidth]{images/workload_analysis.pdf}
%   \vspace{-0.8cm}
%   \caption{ \label{fig:apps}}
% \end{subfigure}%

% \begin{subfigure}[h]{.55\textwidth}
%   \centering
%   \includegraphics[width=0.6\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/isca21/dynamic_rsrch_0.pdf}
%   \hspace{1cm}\vspace{-0.8cm}
%   \caption{\label{fig:dynmc_rsrch}}
% \end{subfigure}
%   \vspace{-0.1cm}
% \caption{(a) Workload characteristic of real-world MSRC traces~\cite{MSR}. (b) Storage access and request size during execution of }
% % \vspace{-0.5cm}
% \end{figure}
\vspace{0.1cm}
\head{\gon{(1b) Lack of adaptivity to changes in device types and configurations}} %The NVM technologies used significantly influence the effectiveness of the hybrid storage system.
\juangg{\gon{There are a wide variety and number of storage devices 
%\gaganF{CITE More}
~\cite{samsung2017znand, seagate, inteloptane, cheong2018flash,micron3dxpoint, hady2017platform, intelp4610, intelqlc, intels4510, adatasu630, kim2014evaluating, tsuchida201064mb, kawahara20128, choi201220nm, matsui2017design, oh2013hybrid, lee2010high, okamoto2015application} that can be used  to configure \gca{an HSS}.} The \gca{underlying storage} technology used in \gca{an HSS}  significantly influences \gca{the} effectiveness \gca{of a data placement policy}.} \gon{We demonstrate this with an example  observation from \fig{\ref{fig:Sibyl/motivation_iops}}}. In the \textsf{H\&M} configuration (\fig{\ref{fig:Sibyl/motivation_iops}(a)}), we \gon{observe} that  for certain workloads (\textsf{hm\_1} and \textsf{prn\_1}), both \cde  and \hps provide rather %lower 
\juangg{low} performance even compared to \slow. Similarly, \arcc and  \kleio provide lower performance for \textsf{hm\_1} and \textsf{proj\_2} in \hmssd compared to \slow.   %, and (2) \hps~generally outperforms \cde.
While in the \textsf{H\&L} configuration (\fig{\ref{fig:Sibyl/motivation_iops}(b)}), we  observe that \cde, \hps, \arcc, and \kleio~%have 
\juangg{result in} lower latency than \slow for the respective workloads. %and (2) \cde~is more effective than \hps~in most workloads. 
% \gon{Second, }
% % {{\kleio}, similar to {\hps}, performs data placement based on the access frequency of a page without considering %a 
% % \juangg{any} system-level feedback. %\jgll{Does "system-level feedback" mean the same as "device awareness"?}. 
% \kleio shows comparable performance to \textsf{Oracle} for hm\_1 in \textsf{H\&M} configuration, however in \textsf{H\&L}, it leads to sub-optimal performance.
% Therefore, \kleio shows, on average, a performance gap of 34.4\% (47.6\%)  to \textsf{Oracle}'s performance for \textsf{H\&M} (\textsf{H\&L}).   %, each of which exhibits different latency and density characteristics.} %{
\gonn{Thus, we conclude that both heuristic-based and learning-based data placement policies lead to poor performance due to their inability to holistically take into account the device characteristics. The high diversity in \gagan{device} characteristics makes it very difficult for a system architect to design a generic  data-placement technique that is suitable for all \acrshort{hss} configurations. }
%\gonn{We conclude that} the high diversity in \gagan{device} characteristics makes it very difficult for a system architect to design a generic  data-placement technique that is suitable for all \acrshort{hss} configurations. 
%\jgll{The previous subsection (1) is already about workload variability. Here we only need to talk about device diversity.}
%\jgll{Btw, this point (2) is not difficult to believe and understand, but you could do much better work if you talk about specific workloads for a mechanism and compare across device configurations. For example, RNN does pretty well compared to Oracle for hm\_1 on H\&M vs. H\&L. Or usr\_0. There is where we can see that RNN does not adapt well to different device configurations.}
%\textbf{The existing heuristic-based approaches are far from the optimal performance.}


\head{(2) Lack of extensibility} \gon{As} modern \gon{HSSs already incorporate more than two types of storage  devices~\cite{ren2019archivist, matsui2017tri, matsui2017design, meza2013case}, system architects need  to put significant effort into extending prior \gonn{data placement} techniques to
accommodate more than two devices.} \rakeshisca{In Section \ref{subsec:Sibyl/trihybrid}, we evaluate the effectiveness of a state-of-the-art heuristic-based policy~\cite{matsui2017tri} \gon{for different tri-HSS configurations, \gonn{comprising} of three different storage devices.} This policy is based on the \cde~\cite{matsui2017design} policy that divides pages into hot, cold, and frozen data and allocates these pages to \textsf{H}, \textsf{M}, and \textsf{L} devices, respectively. \gon{ A system architect needs to statically define the hotness values and explicitly handle the eviction and promotion between the three devices during  design-time.} %The hotness values are set statically during the design-time and are not adapted during the run-time.} 
Through  our evaluation in Section \ref{subsec:Sibyl/trihybrid}, we conclude that such a heuristic-based policy (1) lacks extensibility, \rcam{thereby increasing}  
%that increases 
 the system architect's effort, and (2) leads to lower performance when compared to an RL-based solution (up to 48.2\% lower).} %\namePaper easily extends its best-fit data placement policy to multiple storage devices in the system and continuously adapts to the complexities of a tri-hybrid storage system.} 
% \jgll{I feel this point (3) a little bit out of place. Section III.A is motivation from the results in Fig. 3. However, point (3) has nothing to do with Fig. 3. CDE, HPS and RNN can simply not do 3 devices because their authors didn't use 3 devices.}
% \jgll{Btw, are we the first ones to do hot/cold data placement techniques on 3 storage devices?}

%Figure~\ref{fig:motivation:tri_hybrid} shows performance of a heuristic-based policy~\cite{matsui2017design, matsui2017tri} on a tri-hybrid system that divides data into hot, cold, and frozen and places it into \textsf{H}, \textsf{M}, and \textsf{L} devices, respectively.

%¬\begin{figure}[h]
%%   \vspace{-.7em}
%      \centering
%  \includegraphics[width=.75\linewidth]{images/hpca/trihybrid_mot.pdf}
%  %\includegraphics[width=0.6\linewidth,trim={0cm 0cm 0cm 0cm},clip]{images/Apps_4.pdf}
%     %\vspace{-0.1cm}
%  %\caption{{Applications categorized by hot versus cold (based on recency and frequency of %use), and sequential versus random (based on the size of request}).}
%  \vspace{-.3em}
%  \caption{Performance normalized to \fast policy for tri-hybrid setting.} %%Table~\ref{tab:workload} lists various characteristics of these workloads.}
%\label{fig:motivation:tri_hybrid}
%\end{figure}
% \gon{
% \head{(3) Implementation overhead} \kleio is  inspired by the state-of-the-art data-placement technique in hybrid main-memory~\cite{doudali2019kleio}. It uses sophisticated recurrent neural networks (RNNs) for data-placement.  \kleio shows promising results. However, it has the following limitations: \juangg{it} (1) trains  an RNN for each page, which significantly increases computation and resource overheads as well as training time, and (2) requires offline application profiling. This makes such an approach impractical or very difficult to implement.}
%On the other hand, through our real system evaluation, we show the implementability of our RL-based approach with much higher performance at a lower implementation overhead.


 \gon{Our} empirical study  shows \js{that \textbf{the \gonn{state-of-the-art} {heuristic- and learning-based} data placement techniques are rigid and far from %the 
optimal,}} which strongly motivates us to develop a new data placement technique \gonn{to achieve significantly higher performance than existing policies}.
The new technique should provide \mbox{(1) \emph{adaptivity}} to better capture the features \gonn{and dynamic changes} in I/O-access patterns and storage device characteristics, %\gca{while dynamically adapting its data placement policy}, 
and \mbox{(2) \emph{easy}} \emph{extensibility} to a wide range of \gon{workloads} and HSS configurations. \gonn{Our goal is to develop such a technique using reinforcement learning.}  % \gon{at a low implementation overhead}. %under varying workloads and device configurations.    


% \emph{ \gon{Our} empirical study  shows \js{that \textbf{the existing {heuristic- and learning-based} data-placement techniques are rigid and far from %the 
% optimal,}} which strongly motivates us to develop a new data-placement technique.
% The new technique should  be able to better capture the features in diverse I/O-access patterns and storage device characteristics \gca{while dynamically adapting its data placement policy} to achieve significantly higher performance under varying workloads and device configurations.    
% }

%In Figure~\ref{fig:motivation_speed} we show the effect of using these baseline policies for difference workload in a hybrid storage system (\textit{ref.} Table~\ref{tab:devices} setting 1). We compare these policies with two naive policies: only slow where we serve all the incoming requests from slower storage; and only fast where we assume an infinite fast device capacity and serve all requests from the faster storage. There are no migrations or evictions in either policy. We observe in this setting the most naive policy of placing everything in the slow memory, on average, is better than the state-of-the-art policies. This is because state-of-the-art policies follow a strict heuristic favoring certain workload characteristics over the other. Such bias eventually leads to frequent eviction penalty and in turn performance degradation. 

%We also compared these baseline policies with an oracle policy. The oracle policy has the knowledge of future page accesses and places data with high reuse in the faster storage. We observe in various workloads the baseline policies poorly than an oracle policy and, on average, we observe a performance gap of 57\% and 27\% for CDE and history-based policy, respectively.


% Two other policies against which we compare \namePaper~are Only-Fast and Only-Slow. The Only Fast policy assumes an infinite fast device capacity and serves all requests from that device. The Only Slow policy serves all requests from the slower device. There are no migrations or evictions in either policy. These two policies serve as additional benchmarks for performance comparison. 
% Multiple algorithm designs for data placement in hybrid storage architectures are proposed in~\cite{matsui2017design}. In round-robin frozen data
% collection algorithm (RR-FDCA) designed for multiple-level cell (MLC) and triple-level cell (TLC) NAND flash memory combination, hot data resides in MLC NAND flash, and static and frozen data are placed in TLC NAND flash. In this policy, all write requests are written to MLC NAND flash. Frozen data blocks are chosen in a round robin manner based on their access recency and periodically evicted to TLC NAND flash during garbage collection (GC). Reads are performed directly from the device in which the data resides.

% To separate write-hot or random data from cold and sequential data in Storage class memory (SCM) and MLC NAND flash memory hybrid architecture, Cold Data Eviction (CDE) algorithm~\cite{matsui2017design,sun2013high} maintains a size-fixed table that records the most recently accessed data in a FIFO manner. Data that is stored in the MRU table are considered write-hot. In this algorithm, hot or random write requests are written to the SCM, and cold and sequential write requests are evicted to the MLC NAND flash memory when the SCM is filled to a certain threshold. Host reads are performed from the device in which the data currently resides. The CDE policy attempts to reduce fragmentation in the MLC NAND flash memory and minimize the write amplification. 

% A state-of-the-art data placement policy for die-stacked and off-package heterogeneous DRAM or DRAM/NVM hybrid design is the History page scheduler~\cite{meswani2015heterogeneous,doudali2019kleio}. The history page scheduler classifies pages as hot and cold based on their access frequencies in the current scheduling epoch. The pages are migrated across memories at the end of every epoch to ensure that hot pages are placed in the faster memory and cold pages are placed in the slower memory. This scheduler assumes that access patterns are preserved across epochs. However, it cannot dynamically adapt to changes in workload behavior. 

% Oracular data placement policies use a-priori knowledge of data access patterns to perform data placement. Although oracular policies are infeasible to implement in a real-world scenario, they can be useful in analyzing the extent of performance improvement of our work when compared to the state-of-the-art data placement policies. The Oracle page scheduler~\cite{doudali2019kleio}, similar to the History page scheduler described above, uses access frequencies in the upcoming epoch to place the data in DRAM/NVM hybrid architecture. It periodically migrates pages such that the hottest data (pages with highest access counts in the upcoming epoch) resides in the DRAM.

% Another oracular policy for cache replacement is Belady's optimal policy~\cite{belady1966study}. This policy looks at future reuse distances to determine the pages that must be evicted from cache. Belady's policy can be adapted for a hybrid storage architecture by looking at future reuse distances for incoming requests as well. Pages which will not be accessed in the near-term future will be placed in or evicted to the slower storage device, while those pages that will be accessed soon are placed in the faster storage device.

% Two other policies against which we compare \namePaper~are Only-Fast and Only-Slow. The Only Fast policy assumes an infinite fast device capacity and serves all requests from that device. The Only Slow policy serves all requests from the slower device. There are no migrations or evictions in either policy. These two policies serve as additional benchmarks for performance comparison. 

% We have simulated these approaches to serve as benchmarks to evaluate \namePaper.


 
%\subsection{Inefficiency of Prediction-based approaches}

\iffalse
Many prior works have proposed various data placement techniques for hybrid memory/storage systems~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,doudali2019kleio,ren2019archivist,cheng2019optimizing}.
\fi



%the high diversity of I/O workloads.
%We analyze the I/O characteristics of 14 different workloads from Microsoft Research Cambridge (MSRC) Traces~\cite{} that are collected from real enterprise servers for various applications.
%We use two metrics to represent the I/O characteristics of each workload: (1) \emph{hotness} determined by the average access count of each data block within entire execution of the workload (the higher the access count, the hotter the workload) and (2) \emph{randomness} determined by the average request size of the workload (the smaller the request size, the more random the workload). 
%As shown in \fig{\ref{fig:apps}}, the hotness and randomness significantly vary across different workloads.
%Note that these workloads also exhibit different read/write ratio (see \tab{\ref{}} for more detail) that can significantly affect the effectiveness of a data-placement technique.

%Figure~\ref{fig:apps} shows different workloads that have been categorized into four different group.  The amount of reuse in a workload is used to categorize it as hot or cold. If there is a high (low) reuse of logical addresses then the workload described as hot (cold). The amount of randomness is defined based on the request size compared to the page size of the storage. Further, if a workload has more write requests than write requests, then the workload is classified as write intensive.

%Most heuristic-based approaches[] are designed to favour certain characteristics over the based that are tightly tied to the device characterises. Once, we change the underneath devices these algorithms would not be able provide acceptable amount of performance.

%\subsection{Inefficiency of current heuristics-based data placement policies approaches}
%\label{subsec:CurrentApproaches}

%Prior works~\cite{} have proposed various data-placement techniques} for hybrid storage systems.  
%Various data placement algorithms have been proposed for hybrid storage systems [].
% \head{(2) Heterogeneity in workloads and devices}  Second, 

 
% Second, there exist various storage technologies with different characteristics, which significantly increases the diversity of hybrid storage systems. %As shown in \tab{\ref{tab:nvm_devices}}, 


% Second, there exist various storage technologies with different characteristics, which significantly increases the diversity of hybrid storage systems. %As shown in \tab{\ref{tab:nvm_devices}}, 
% There are a number of technologies~\cite{samsung2017znand, cheong2018flash,micron3dxpoint, hady2017platform} \gagan{that we can use} to configure a hybrid storage system, each of which exhibits different latency and density characteristics.

% \input{tables/NVM_Technologies}


\iffalse
\subsection{Practical Limitation}
In addition to the above discussed functional limitations, we identify that most of the prior techniques have not been evaluated on a real system.

\head{(1) Missing real system analysis} {Although {other} works~\cite{matsui2017design,sun2013high,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,doudali2019kleio,ren2019archivist,cheng2019optimizing, sun2016design} have proposed several data placement techniques for different hybrid storage configurations, we observe their effectiveness has not been evaluated on a real system under {real-world} conditions. Simulation-based approaches use deterministic latencies, which model the data placement mechanism in isolation {from the  rest of the system processes}. However, there are variable read and write latencies on a real system with non-deterministic behavior due to noise caused by background processes. Such complex, realistic behavior makes the task of {devising} and deploying an effective data placement solution even more challenging.}
\jgll{First, I don't know if we really need this. Simulation is used in most architecture works. I would not doubt about it. Second, we are using MSRC traces, not real programs running on a server. So we are also not perfect...}

% \com{Can we add more? some challenges of real system?}

{
\head{(4) No learning from past experiences} We observe that existing techniques have two inherent issues. First, these approaches {do not} utilize the experience from {past} data placement decisions for future decisions. Supervised learning-based data placement techniques~\cite{doudali2019kleio,ren2019archivist} have been proposed to overcome these issues. However, such  machine learning models are trained for specific applications or hybrid storage settings and, thus, lack adaptavity to automatically update {their} decision making policies for new devices or \gon{workloads}. Second, most existing techniques largely rely on manually-engineered heuristics to capture common I/O-access patterns and use them for future I/O prediction~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient}.
Unfortunately, I/O-access patterns significantly vary across different workloads, and even a single workload often exhibits complex I/O-access patterns in which random and sequential accesses are intermixed.} 

\fi


% \com{Can we add more?}\\\
%\js{This means that the efficacy of} models trained using non-RL methods \js{highly depends on} 
%are as good as 
%the data provided during the training phase. 


% \begin{enumerate} [leftmargin=*,nosep]
% \item An RL agent aims to optimize a particular objective. This agent works autonomously to reach that objective without any direct human intervention. 
% \item In case of a change in the environment (i.e., different workload or device), the RL agent has the capability to self-optimize its decision making policy to reach its defined objective. 
% \item Other learning techniques require \emph{labeled} data on optimal decisions while training these algorithms. Whereas an RL agent does not require labeled data. An  agent updates its policy by interacting with the \textit{environment} through \textit{actions} and \textit{rewards}.%\js{This means that the efficacy of} models trained using non-RL methods \js{highly depends on} 
% %are as good as 
% %the data provided during the training phase. 
%  \end{enumerate}
%  For these reasons, we choose RL to design a new data-placement technique for hybrid storage systems that can easily adapt to dynamic changes of workload and device characteristics. 
%  {Many} prior works~\cite{rl_GC_TECS,ipek2008self,rl_NOC_AIDArc_2018,rl_opti_TACO_2017,rl_prefetching_2015_ISCA,rl_voltage_scaling_TC_2018} %to 
% propose promising RL-based approaches for various system optimizations including cache~\cite{liu2020imitation} and memory management~\cite{ipek2008self}.
%The 
% \juan{Prior} works demonstrate that a variety of ML algorithms (e.g., reinforcement learning (RL)~\cite{wanglearning}, convolutional neural networks (CNNs)~\cite{}, recurrent neural networks (RNNs)~\cite{doudali2019kleio}, and multi-level perceptron (MLP) networks~\cite{ren2019archivist}) can outperform state-of-the-art heuristics in predicting future access patterns. \jgl{Only access patterns? Are all these works about memory?}



 



% \js{
% Such an RL-based approach has two advantages over other ML-based approaches in designing an effective data-placement technique.
% First, ...
% }
%\noindent\textbf{Time-varying workload demands:} The intensity of application workloads changes over time of an application i.e., application runs in phases. As a result, the demand for individual memory changes over time. Most heuristic-based approaches allocate memory for peak demands, thus wasting memory and lead to poor performance during the execution phases of an application. Therefore, a \rl~based approach is highly suited for such kind of dynamics.


%\subsection{Formulation of RL-Based Hybrid storage data placement}
%\label{subsec:motivation_formulation}
% To leverage reinforcement learning (RL) for hybrid storage data placement we need to specify set of \textit{states} that can be observed to perform specific \textit{actions} and formulate a \textit{reward} structure to provide feedback to our agent. We term the whole execution of a workload as an RL \textit{episode} or an \textit{iteration}. We treat each request to the storage as a different {time-step}. At each time step, our agent receives the current state $O(s_t)$  of the environment based on which the agent performs an action (i.e., from which storage device the incoming request should be served). In figure~\ref{fig:rl_formulation}, we show a conceptual diagram of how a hybrid data placement fits within the RL-framework.



==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/related.tex <==
\section{Related Work}
% \gaganF{add RL related work}


%To our knowledge, this is the first work that uses reinforcement learning for data placement in hybrid storage systems.
% \gca{In this section, we look at prior work in the area of data placement in hybrid memory/storage systems including some of the policies that served as benchmarks for the evaluation of \namePaper. }
\gagan{To our knowledge, this is the first work to propose \rcamfix{a reinforcement learning}-based data placement technique for hybrid storage systems. \rcamfix{\namePaper can} continuously learn from and adapt to the \rcamfix{running} application and \rcamfix{the} storage \rcamfix{configuration and} device characteristics. }\gca{We \rcamfix{briefly} discuss closely-related prior works that propose data management techniques for hybrid memory/storage systems and RL-based system optimizations.} 


\head{Heuristic-based data placement}
Many prior works~\cite{matsui2017design,sun2013high,heuristics_hyrbid_hystor_sc_2011,vasilakis2020hybrid2,lv2013probabilistic,li2014greendm,guerra2011cost,elnably2012efficient,heuristics_usenix_2014,li2017utility_HMM,agarwal2015page_HMM,agarwal2017thermostat_HMM,ham2013disintegrated_HMM, bu2012optimization, krish2016efficient, lin2011hot, tai2015sla, zhang2010automated, wu2012data, iliadis2015exaplan, lv2013hotness, matsui2017tri, feng2014hdstore,salkhordeh2015operating, pavlovic2013data, meza2013case, yang2017autotiering, chiachenchou2015batman, kim2011hybridstore, wang2019panthera, ramos2011page, liu2019hierarchical,luo2020optimal,doudali2021cori} propose heuristic-based techniques to perform data placement. % in a hybrid storage system.
These techniques rely on statically-chosen design features that \rcamfix{usually} favor certain workload\gonzz{s} and/or device characteristics, \rcamfix{leading to \gonx{relatively} rigid policies}.
%over the other.
In Section \ref{sec:Sibyl/motivation_limitations} and Section \ref{sec:Sibyl/results}, we  show \gca{that} \namePaper outperforms two \rcamfix{state-of-the-art} works, CDE~\cite{matsui2017design} and HPS~\cite{meswani2015heterogeneous}.
% \gaganRemove{We show that \namePaper outperforms the two heuristics-based techniques, achieving much closer I/O performance to an \gagan{oracle} policy.}
% \gaganRemove{While CDE and HPS efficiently perform only for specific workloads and/or hybrid-storage configurations, \namePaper better adapts to the environmental changes with performance improvement in most workloads and all evaluated storage configurations. Therefore, this heuristics-based rigid design approach performs far lower than an optimal policy.}
 

%Multiple heuristics-based algorithm designs for data placement in hybrid storage architectures are proposed in~\cite{matsui2017design}. In round-robin frozen data collection algorithm (RR-FDCA), hot data resides in faster storage (MLC NAND flash), and static and frozen data are placed in slower storage (TLC NAND flash). Frozen data blocks are chosen from faster storage in a round robin manner based on their access recency and periodically evicted to slower storage during garbage collection (GC). Cold Data Eviction (CDE), described in section~\ref{subsec:CurrentApproaches}, maintains an MRU table to keep track of the recently accessed data and identify write-hot pages. To make space for new requests in the faster storage (SCM), cold and sequential pages are evicted to the slower storage device (MLC NAND flash). The CDE policy attempts to reduce fragmentation in the MLC NAND flash and minimize write amplification. 

%The other heuristic approach used as a benchmark for comparison against \namePaper~is the History Page scheduler~\cite{meswani2015heterogeneous,doudali2019kleio} (See section~\ref{subsec:CurrentApproaches}). The history page scheduler is a state-of-the-art data placement policy for die-stacked and off-package heterogeneous DRAM or DRAM/NVM hybrid design. This epoch-based scheduler migrates pages across fast and slow memories based on their past access frequencies. The scheduler cannot quickly adapt to change in workload behaviour due to the underlying assumption that access patterns are preserved across epochs.

%\namePaper~outperforms the heuristic data placement approaches due to its ability to dynamically adapt to changes in environment and workload patterns.
%Oracular data placement policies use a-priori knowledge of data access patterns to perform data placement. Although oracular policies are infeasible to implement in a real-world scenario, they can be useful in analyzing the extent of performance improvement of our work when compared to the state-of-the-art data placement policies.
%The Oracle page scheduler~\cite{doudali2019kleio}, similar to the History page scheduler described above, uses access frequencies in the upcoming epoch to place the data in DRAM/NVM hybrid architecture. It periodically migrates pages such that the hottest data (pages with highest access counts in the upcoming epoch) resides in the DRAM.

\head{ML-based data placement}
%Prior works
%\rcamfix{Several works}, such as  %\cite{maas2020taxonomy,zhou2019multi,mendis2019compiler,delimitrou2014quasar,mendis2019ithemal,alam2019zero,maas2020learning,hashemi2018learning,berger2018towards,such2017deep, mutlu2021intelligent_DATE} have proposed ML-based techniques for system optimizations, including data-placement techniques for hybrid memory/storage systems \cite{doudali2019kleio,ren2019archivist,cheng2019optimizing,shetti2019machine}.
% \gaganRemove{Recently, for DRAM-NVM-based hybrid memory systems, Doudali~\etal~propose Kleio~\cite{doudali2019kleio}, a page scheduler using RNNs. }%\gaganRemove{ Like HPS~\cite{meswani2015heterogeneous}, Kleio also performs data migration between the fast and slow devices at the end of every epoch, but it exploits RNNs to determine performance-critical pages to move into the fast device.} 
%Application pages that are critical for system performance are placed using the RNN-based page scheduler, that creates a separate neural network for each such page. 
%The rest of the pages are placed using the history page scheduler~\cite{meswani2015heterogeneous}. 
%Kleio requires \gmicro{offline application profiling and trains}  an RNN for each page that significantly increases computation and resource overheads as well as training time.
\rcamfix{Several works~\cite{doudali2019kleio,ren2019archivist,cheng2019optimizing,shetti2019machine,sen2019machine} propose ML-based techniques for data placement in hybrid memory/storage systems. These  works 1) are based on supervised learning techniques that require frequent \rcamfix{and very costly} retraining to adapt to changing workload and device characteristics, and 2) have not been evaluated on a real system.} \gonn{\rcamfix{We evaluate} \kleio, which is  inspired by the state-of-the-art data placement technique in hybrid main memory~\cite{doudali2019kleio}. It uses sophisticated recurrent neural networks (RNNs) for data placement \rcamfix{and} shows promising results \rcamfix{compared to heuristic-based techniques}. However, it has \gonx{two major} limitations \gonx{that make it impractical or difficult to implement}: \juangg{it} (1) trains  an RNN for each page, which \rcamfix{leads to large} computation\gonx{, storage, and training time \gonzz{overheads}}, and (2) requires offline application profiling.}
\gagan{Our evaluation (ref. Section \ref{subsection:Sibyl/Evaluation_perf}) shows that \namePaper outperforms \rcamfix{two state-of-the-art ML-based data placement techniques}, \kleio~\cite{doudali2019kleio} and \arcc~\cite{ren2019archivist}, \rcamfix{across a wide variety of workloads.}}
%on average, by 27.9\%  and 52.5\%, respectively.}
%to minimize the number of neural networks that need to be trained, the training time per page is still very long and requires significant computation and memory resources. Additionally, training an RNN for each page separately may ignore dependencies among different pages. This hybrid page scheduler reduces the performance gap between history page scheduler and oracular page scheduler by 80\% on average. Since \namePaper~uses a single reinforcement learning agent, the training time and the computational resources required are less.
%Although Kleio attempts to minimize the number of neural networks that need to be trained, the training time per page is still very long and requires significant computation and memory resources. Additionally, training an RNN for each page separately may ignore dependencies among different pages. This hybrid page scheduler reduces the performance gap between history page scheduler and oracular page scheduler by 80\% on average. Since \namePaper~uses a single reinforcement learning agent, the training time and the computational resources required are less.
% Archivist~\cite{ren2019archivist} uses a neural network-based offline classifier that predicts file access patterns to take data-placement decisions. {We observe that Archivist leads to 68.9\% (28.15\%) lower performance compared to \kleio for {\hlssd (\hmssd)} configuration.} 
%Archivist assumes an unlimited capacity for all the devices in the hybrid storage systems, thereby ignoring the long-term performance effect of eviction/migration.
%Cheng~\etal~\cite{cheng2019optimizing} propose data placement using regression trees for hierarchical storage %systems. %They  focus on data replacement in which the dimensional space is significantly narrower than in data placement. 
 %\ghpca{Note that none of the above works in data placement evaluate their approach on a real system.}
%\gaganRemove{Unlike \namePaper, these approaches make use of supervised learning that lacks adaptability.}
\iffalse
Compared to our approach, supervised learning has the following two issues. First, supervised learning lacks the ability to self-optimize in case of a change in workload and/or hardware environment. In case of a change, the model would need to be retrained. Second, supervised learning techniques require labeled data on optimal placement choices while training. Therefore, the models trained using supervised learning are as good as the data provided during the training phase.
\fi

%CHOPT~\cite{zhang2020optimal} is an offline data placement algorithm for caching that is oracular in nature. In this work, memory hierarchy placement decisions in a DRAM/NVM hybrid memory environment are represented as network flows and translated into a Minimum Cost Maximum Flow (MCMF) problem. CHOPT shows significant latency improvements over other offline algorithms, but with many underlying assumptions.
% {Many} prior works~\cite{rl_GC_TECS,ipek2008self,rl_NOC_AIDArc_2018,rl_opti_TACO_2017,rl_prefetching_2015_ISCA,rl_voltage_scaling_TC_2018} %to 
% propose promising RL-based approaches for various system optimizations including cache~\cite{liu2020imitation} and memory management~\cite{ipek2008self}.

%\head{{Novelty compared to prior works}}
\head{{\rcamfix{RL-based techniques in storage systems}}}
Recent works \gon{(e.g., \cite{liu2019learning,yoo2020reinforcement,wang2020reinforcement,rl_GC_TECS, kang2018dynamic})} propose the use of RL-based approaches for managing different aspects of storage systems. These works cater to use cases and objectives that are \gonx{very} different \rcamfix{from} \namePaper's.
%, which leads to completely different goals and implications. 
Specifically, {Liu}~\etal~\cite{liu2019learning} (1) \rcamfix{propose} data placement in cloud systems and \emph{not} \gf{hybrid storage \rcamfix{systems}, (2) consider devices with unlimited capacity, sidestepping the capacity limitations, (3) \emph{emulate} a data center network rather than \gon{use} a real system \gon{for design and evaluation}, and (4) focus only on data-analytics workloads. }%. The %performance and
%effectiveness of their approach on other sets of workloads or even other system configurations are unknown \jgll{But would it be applicable to our scenario in some way? Does this work deal with hybrid storage? It is not a good idea to say "unknown". Why didn't we test it? It would be better to explain that it is not applicable to our case}. Moreover, rather than using a real system, the authors \emph{emulate} a data center network \jgll{The simulation/emulation vs. real system is not such a strong argument}.
{Yoo}~\etal~\cite{yoo2020reinforcement} do \emph{not} focus on data placement; they instead deal with dynamic storage resizing %\jgll{What is "changing memory size"? Not clear what this work solves.} 
based on workload characteristics using a trace-based simulator.  Wang~\etal~\cite{wang2020reinforcement} (1) focus on cloud \gon{systems} to predict the data storage consumption, and %to adapt the data storage cost to the actual \gca{system} needs, and }% \jgll{Their goal is to predict the data storage consumption to adapt the data storage cost to the actual current needs? Be more clear}. 
(2) do \emph{not} consider hybrid storage systems. 
%hybrid storage with different device characteristics. 
%Therefore, these RL approaches: (1) do not evaluate their mechanism on a real system \jgll{Not super strong argument. Put it third}, (2) aim for different, and not necessarily compatible \jgll{Do we need to say this? The end goals are different. That is enough. Whether what they do is orthogonal or not, or compatible or not, with our work is better to not discuss (unless we can say it's orthogonal).}, end goals, and (3) are not plug-and-play in other system configurations or workloads \jgll{First time we say plug-and-play. Does this relate to the adaptability? If so, make the connection clear.}. 
\namePaper is the first RL-based mechanism \gon{for data placement in hybrid storage systems.} 
 
%\namePaper provides: (1) \emph{adaptivity} by %dynamically %derive} a data-placement policy by 
%\emph{continuously learn\gon{ing}} from and {adapt\gon{ing} to} the \gon{workload} and the storage device %characteristics, and (2) \emph{easy extensibility} to  a wide range of {applications and} HSS configurations.}

\head{RL-based system optimizations}
Past works~\ghpca{\cite{lin2020deepNOC,ipek2008self,liu2020imitation,rl_NOC_AIDArc_2018,rl_voltage_scaling_TC_2018,mirhoseini2021chip,mutlu2021intelligent_DATE, pythia, peled2015semantic, martinez2009dynamic, multi_scheduler_HPCA_2012, jain2016machine,zheng2020agile, pd2015q}} propose RL-based methods for various system optimizations, such as memory scheduling~\cite{ipek2008self, multi_scheduler_HPCA_2012}, data prefetching~\cite{pythia,peled2015semantic}, cache replacement~\cite{liu2020imitation}, and network-on-chip arbitration~\cite{rl_NOC_AIDArc_2018,lin2020deepNOC}. \gca{Along with \namePaper\rcamfix{, designed} for efficient data placement in hybrid storage systems, \rcamfix{this body of work} demonstrate\rcamfix{s} that RL is a promising approach to designing high-performance\rcamfix{, and highly-adaptive} self-optimizing computing systems. }



%A combined neural network and reinforcement learning based approach, DataBot+, has been proposed by Liu~\etal~\cite{liu2019learning} for data placement across multiple compute nodes in a data center network. DataBot+ trains the neural network using Q-learning for prediction of near-future latency. To reduce training time overhead, DataBot+ decouples the online decision-making and offline training components.
%Reinforcement learning algorithms have also been used to optimize other areas of memory systems such as DRAM command scheduling~\cite{ipek2008self}, data prefetching~\cite{yoon2018design} and caching policies~\cite{liu2020imitation}. 





==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/rl_formulation.tex <==
\section{\namePaper: RL Formulation}
\label{sec:Sibyl/rl_formulation}

% \subsection{High-level Overview}
%Traditional techniques for data placement make use of heuristics that rely on immediately observed behavior to make decisions for future data placement.   Prior works [] have shown such approaches lead to severe performance degradation, thus failing to fully leverage the hybrid memory resources. This performance penalty because of frequent data movement is forcing the industry to look for new ways for efficient data handling []. 
%The feature space for data placement is high dimensional since each feature can have any possible value. Therefore, using a simple lookup table-based approach is not possible for data placement. Although
\fig{\ref{fig:rl_formulation}} shows our formulation of  data placement as an RL problem. We design \namePaper as an RL agent that learns to perform accurate and system-aware data placement decisions by interacting with the hybrid storage system. With every storage request, \namePaper observes \gup{multiple \gon{workload}} \gont{and system-level} features \gca{as \gonzz{a} \emph{state}} to make a data placement decision. After every \emph{action}, \namePaper receives a \emph{reward} \gca{in terms of \gont{the served} request latency} that takes into account the data placement decision and internal storage system state. \namePaper's goal is to find an optimal data placement policy that %would increase 
\gont{maximizes} overall performance for \gon{the running} workload and \rcam{the current} system configuration.
\gon{To reach its performance goal, \namePaper needs to minimize the \gont{average request} latency \gon{of the running workload} \gont{by maximizing} the use of the fast storage device while avoiding the eviction penalty \gont{due to non-performance critical pages}. }


 \begin{figure}[h]
  \centering
 \includegraphics[width=0.85\linewidth,trim={1.12cm 3.5cm 1.8cm 5.5cm},clip]{Sibyl/images/isca'22/Sibyl_intro_bw_2_embed.pdf}
  \caption{Formulating data placement as an RL problem}
\label{fig:rl_formulation}
 \end{figure}
% \gaganF{add high-level figure here}

% \jgll{I do not think we need two subsections in this section. The previous paragraph is ok as a reminder of Fig. 2 and to introduce the next subsections about state, action, and reward.}

% \subsection{RL Components}
% \label{subsec:mechanism_components}
\head{Reward} 
\gon{After every data placement decision} at time-step\footnote{\gor{In HSS, a time-step is defined as a new storage request.
}}  $t$, {\namePaper gets a reward %\jgll{Do we need this definition? Do we use the term "return" in this paper?}} 
from the environment} at time-step $t+1$ that acts as a feedback to \namePaper's previous action. %This total sum represents the quality of the data placement.
{To achieve \namePaper's performance goal, we craft \gon{the} reward \gon{function} \textit{R} as follows:
\begin{equation}
R =\begin{cases}
       {\scalemath{1}{ \frac{1}{L_t} }}& 
        \begin{gathered}
            \textit{if no eviction \gon{of a page from the}} \\[-\jot]
            \textit{\gon{fast storage to the slow storage}}
        \end{gathered}\\
        % \text{{if no eviction \gon{of a page from the}}}\\ 
        % &\text{{\gon{fast storage to the slow storage}}}\\
        max(0,\frac{1}{L_t}-\textit{$R_p$}) & \text{\textit{in case of eviction} }
    \end{cases}
\end{equation}
{where $L_t$ and \textit{$R_p$} represent \rcamfix{the} \gonff{last} \gont{served} \gca{request latency}  and eviction penalty, respectively. \gont{If the fast storage is running \gonff{out} of free space, there might be evictions in the background from the fast
storage to the slow storage. Therefore, we add an eviction penalty (\textit{$R_p$}) to  guide \namePaper to  place only performance\gonzz{-}critical pages in the fast storage. %, and (2) leads to a faster convergence of \namePaper towards an optimal policy.
} 
\gon{We empirically select \gont{\textit{$R_p$} to be equal to} 0.001$\times$$L_e$ ($L_e$ is the time spent in evicting pages from the fast storage to the slow storage)}\rcamfix{, which}  prevents the agent from aggressively \gonff{placing} all requests \gonff{into} the fast storage device.}}
% \jgll{Equation 2 is not clear. Is it a piece-wise function? If so, when R is equal to the inverse of the latency and when it is equal to max()? Also, why do you have the explanation "where..." at the right of the equation. That is normally placed after the equation.}
% \jgll{In the first line, you have to say "$L_t$, if no eviction." In the second line, "max(), if an eviction happens." -- or similar wording. Then, you explain the meaning of $L_t$ and $R_p$ below.}
% \jgll{Btw, what is the penalty of an eviction? Is it a penalty value you come up with or is it an actual latency penalty (due to the needed data movement)?}

% {The above reward structure} guides the agent to explore the \textit{environment} to achieve a higher reward.
\gont{$L_t$} \gonff{(request latency)}  is the time taken to service \gont{the last} read or write  I/O request \gont{from the OS}. Request latency can faithfully capture the status of the hybrid storage system, as it significantly varies depending on the request type, device type, and the internal state \gont{and \gonz{characteristics}} of the device (e.g., such as read/write latenc\rcamfix{ies}, \gonzz{the} latency of garbage collection, \rcamfix{queuing delays, \gonz{and error handling latencies})}.
\rcamfix{Intuitively, if} \gont{$L_t$} is low (high), i.e., if the agent serves a storage request from the fast (slow) device, the agent receives a high (low) reward. However, \gonff{if there is an eviction,} we \rcam{penalize} the agent \gonff{so as} \gup{ to \rcamfix{encourage} the agent \rcamfix{to} place only performance-critical pages in the fast storage device.} % \jgll{Not clear if this is the penalty of the eviction or it is a penalty for the migration needed if the page is, e.g., in the slow device but the action is "place in fast device".}. 
   We need the \rcamfix{eviction} penalty \gonff{to be} %at the correct scale so that it is 
   large enough to \rcamfix{discourage} the agent \rcamfix{from evicting} and small enough not to deviate the learned policy too much on a \gonff{placement} decision \gonz{that leads} to higher latency.  %After enough exploration, the agent learns to place only performance-critical data in the faster device and the rest of the data in the slower device. 

\head{State}
% The state represents features or attributes of 
% %the system, 
% {both the host and the hybrid storage subsystem, {and workload characteristics} based on which our agent} %takes
% {makes} a {data-placement} decision. %We select 6 dimensional observation vector $O(s_t)$ that characterizes requests to the hybrid storage system. 
At each time-step $t$, the state features for a particular \mbox{read/write} request  are collected in an \emph{observation} vector. %\jgll{So at each time step we only consider one request, right? It would be good to say.}. %{Following the approach in~\cite{NAPEL}, we can obtain 395 features for our state vector.
  % Note that we could use any number of features in the observation vector; however, 
  \gon{We  perform feature selection~\cite{kira1992featureselection} to determine the best state features to include in \namePaper's \gont{observation} vector.} %select only the most correlated features to data placement decisions. %\jgll{Do we explain why these 6 particular features? Why are they the most correlated to data placement decisions?}


We use a limited number of features due to two reasons. First, a limited feature set allows us to reduce the implementation overhead of our mechanism \gont{(\gonff{see} \ref{sec:Sibyl/overhead_analysis})}. Second, we empirically observe that our RL agent is more sensitive to the reward structure than to the \gca{number} of features in the \gonff{observation vector}.  Specifically, using the request latency as a reward provides indirect feedback on the internal timing \rcam{characteristics} \emph{and} the current state \gon{(e.g., queu\rcamfix{e}ing delays, buffer dependencies, effects of garbage collection, read/write latenc\gonzz{ies},  write buffer state, \gonzz{and} \rcamfix{error handling latencies})} of the hybrid storage system. Our observation aligns with a recent study~\cite{silver2021reward} that argues that the reward is the most critical component \gca{in RL to find an optimal decision-making policy}. 


 

In our implementation of \namePaper{}, the observation vector is a 6-dimensional tuple:
\vspace{-0.1cm}
\begin{equation}
% \vspace{-0.05cm}
% O_t = (m_t, x_t, r_t, f_t, c_t, p_t).
\gonx{
O_t = (size_t, type_t, intr_t, cnt_t, cap_t, curr_t).}
% \vspace{-0.05cm}
\end{equation}

 %that 
\noindent
Table~\ref{tab:Sibyl/state} %shows 
{lists our \js{six}} selected features. \gon{We \rcamfix{quantize the representation of each state} into a small number of bins \gonff{to} reduce \gonff{the} \gont{storage overhead of state representation}.} These features can be captured in the block layer of the storage system \gup{and stored in a separate metadata table (\ref{sec:Sibyl/overhead_analysis})}.  %, including request size, I/O timestamp, write/read, and offset.}
%At each time-step the observation vector is as follows
%\[\Scale[0.8]{O_j = (S_j(t), T_j(t), R_j(t),F_j(t), C_j(t), A_j(t-1))}\]
$size_t$ represents the size \gon{of the current request} in terms of the number of pages associated with \gon{it}. It {indicates whether the incoming request} is sequential or random. % \jgll{I don't get yet why the size is related to sequential/random.}. 
%As storage devices have asymmetric read and write latencies, we use $T_j$ to differentiate between read and write requests. 
{$type_t$ \gon{(request type)} differentiates between read and write requests, \gon{important} for data placement decisions since storage devices have asymmetric read and write latencies.} 
$intr_t$ (access interval)  and $cnt_t$ (access \gonz{count}) represent the temporal and spatial reuse \gon{characteristics} of \gont{the currently requested page}\gca{, respectively}.  \gup{Access interval  
%\gon{checks} 
\rcamfix{is defined as} the number of page accesses between two  references to the same page. %\jgll{I hope this definition is widely accepted by the SSD community. Othewise, it will cause confusion, because it is very similar to what we usually call "reuse distance" or "temporal locality" (check DAMOV, for example). That is, "temporal" not "spatial".}. 
\gf{ Access \gonz{count} 
%\gon{checks the} 
\rcamfix{is defined as} \gonff{the} total \gon{number of} accesses to \gon{the page}.} \gonz{These metrics} provide
insight into \gonzz{the} \gonz{dynamic} \gon{behavior of the currently requested page.}%some 
% insights into a program's behavior \gca{by measuring} the probability of reuse.
\footnote{We did not use the reuse distance as a locality metric due to its high computation overhead during online profiling~\cite{zhong2009program}.}%\jgll{Now I'm completely confused lol}. 
%\jgll{You don't define "access frequency"?}
} %{{For spatial distance, we keep an 8-bit counter to track number of memory accesses in between two memory references to the same  location,} while for access frequency, we use a separate 8-bit counter to measure total accesses to a specific memory location. } 
%The goal of our agent is to maximize the use of limited capacity of the faster storage. Therefore, we provide the space utilized in the fast storage ($C_j$) as one of the features. 
$cap_t$ is a global counter \gonz{that tracks} the remaining capacity in the fast storage \gon{device, which }is an important feature since our agent's goal is to maximize the use of the limited fast storage capacity \gca{while avoiding evictions} \gon{from the fast storage device}.  \gup{By including this feature, the agent can learn}
% To effectively use %the 
% {this} limited capacity, we make our agent learn 
to \gonff{avoid the eviction penalty (i.e., learn to } restrain {itself} from \gonff{placing in fast storage} non-performance critical pages that would lead to evictions). % {(incurring an eviction penalty)}. 
 \gon{$curr_t$ \gont{is the} current placement of the requested page. Since every data placement decision affects the decision for future requests, $curr_t$ guides \namePaper to perform past-aware decisions.}% by proactively placing a hot (cold) page on the fast (slow) device. } 
%Every 
%{Since every} data placement decision affects the decision for future requests, %. Therefore, 
%we \gca{include} the current placement of the page $p_t$ \gca{in our state information}. %as a part of $O(s_t)$ so that 
%This way, the agent can perform past-aware decisions to proactively place a page on the faster or slower device. For the number of bins, 

%\input{tables/features}

\input{Sibyl/tables/features}

 
\head{Action} 
{At each time-step $t$, in a given state, \namePaper selects an action \gup{($a_t$ in Figure~\ref{fig:rl_formulation})} from \gon{all} possible actions. \gca{In a hybrid storage system with two devices,  possible actions are: } placing data in \gon{(1) the fast storage device}} %(represented as 1 \jgll{Is this 1 or 0 important?}), 
or (2) the slow storage device. \gont{This is easily extensible to $N$ storage devices, where $N\ge3$.} %(represented as 0). 
% {The agent's goal is to learn and adapt a \gor{policy that autonomously} chooses actions that maximize the overall reward.} }




 
%  the agent performs an action $a_t$ (faster or slower device) from the action space ${A}$ of the agent. ${A}$  is represented as $\{0,1\} \forall  O_t$, where 0 corresponds to slower device and 1 to fast device. Note: we can design much more fine-grained actions as well, such as which page, however, such fine-grained action space is directly proportional to the computational complexity and the design overhead. The agent {tries to achieve a} policy which chooses actions that  maximizes the overall return~\cite{sutton_2018}.


% Our goal is to design a data-placement module (i.e., \namePaper{})
% that operates as an RL \emph{agent} over the target hybrid storage system, which acts as an RL \emph{environment}.
% We term the complete execution of a workload as an RL %\emph{episode} or an 
% \emph{iteration} while treating each I/O request to the hybrid storage system as a different \emph{time step}. {For every storage access, the RL agent observes different features of the storage system and the application. Based on the observation, the agent performs a data-placement action that leads to a new state. For every action, the agent receives a reward in terms of latency. The agent's goal is to make the data placement decisions to minimize the overall application latency.}

% At each time step $t$, the RL agent monitors an observation of the current state $O(s_{t})$ from the storage system and receives a \emph{reward} $r_{t+1}$, based on a previous data placement \emph{action} $a_{t}$ %(e.g., from which storage device the incoming request should be served) 
% that the agent performed. 

%\namePaper~is an RL-based mechanism for data placement in hybrid storage systems. 
% 
% \gaganRemove{In this section, we describe the main components of \namePaper. First, we give an overview of \namePaper  (Section~\ref{subsec:mechanism_overview}). Second, %in Section~\ref{subsec:mechanism_components}  
% we define the necessary components needed for the RL mechanism -- \textit{state}, \textit{reward}, and \textit{action} (Section~\ref{subsec:mechanism_components}). Third, we discuss \namePaper's architecture (Section~\ref{subsec:mechanism_rl_agent}). Fourth, we describe %the 
% how our agent learns and makes data placement decisions (Section~\ref{subsec:mechanism_rl_algo}). Fifth, we explain {the} \textit{design of experiments} methodology   {for} hyper-parameter tuning to improve our agent's performance(Section~\ref{subsec:lhs}).}

%   \begin{figure*}[h]
% \centering
% \begin{subfigure}[t]{.53\linewidth}
%   \centering
%   \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0.4cm},clip]{images/hpca/sibyl_4.pdf}
%   \vspace{-0.7cm}
%   \caption{
%   \label{fig:curator}}
% \end{subfigure}%
% \hspace{0.3cm}
% \begin{subfigure}[t]{.23\linewidth}
%   \centering
%   \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0.2cm},clip]{images/hpca/network_3.pdf}
%   \vspace{-0.6cm}
%   \caption{
%   \label{fig:model}}
% \end{subfigure}
%   \vspace{-0.215cm}
% \caption[Two numerical solutions]{(a) Overview of \namePaper. (b) Neural network design using \hy{the input  features} from Table~\ref{tab:state}. }
% \label{fig:qrator}
% \vspace{-0.5cm}
% \end{figure*}



==> PhD_Thesis_Updated_arxiv (1)/Sibyl/sections/rlmotivation.tex <==
\section{{Reinforcement Learning}}
\vspace{-0.1cm}
\subsection{{Background}}
\label{background:rl}
Reinforcement learning (RL)~\cite{sutton_2018} is a class of machine learning (ML) algorithms that involve an \emph{agent} learning to achieve an objective by interacting with its \emph{environment}{, as shown in \fig{\ref{fig:rl_basic}}}. The agent starts from an initial representation of its environment in the form of an initial state\footnote{{State is a representation of an environment using different features.} } $s_0$ $\in$ $S$, where $S$ is the set of all  possible states. 
Then, at each \emph{time step} $t$, the agent performs an \emph{action} $a_t$ $\in$ $A$ in state $s_t$ ($A$ represents the set of possible actions) and moves to the next state $s_{t+1}$. The agent receives a numerical reward $r_{t+1}$ $\in$ $R$, \gon{which could be \textit{immediate} or \textit{delayed} in time},  for action $a_t$ that \gca{changes} the environment state from $s_t$ to $s_{t+1}$. The sequence of states and actions starting from an initial state to the final state is called an \emph{episode}. % or an \emph{iteration}.
The agent \gca{\gonx{makes} decisions and receives corresponding rewards} %until the end of an {episode} 
while trying to maximize the \textit{accumulated} reward, \gont{\rcamfix{as opposed to} \gonz{maximizing} the reward for \gonz{only} \emph{each} action}. In this way, the agent can optimize for the long-term impact of its decisions. 

 \begin{figure}[h]
  \centering
%   \vspace{-0.1cm}
    \includegraphics[width=0.7\linewidth,trim={2.2cm 7.6cm 3cm 1.4cm},clip]{Sibyl/images/isca'22/Sibyl_intro_bw_2_embed.pdf}
  \caption{Main components of \gon{general} RL}
\label{fig:rl_basic}
 \end{figure}
%The agent receives a numerical reward $r($$s_t$, $a_t$, $s_{t+1}$$)$ $\in$ $R$ for moving  from the state $s_t$ to $s_{t+1}$ through action at.
\gon{
The policy $\pi$ governs an agent's action in a state.  The agent’s goal is to find the optimal policy that maximizes the cumulative reward\footnote{The total cumulative reward is also known as the \emph{return}~\cite{sutton_2018}.} collected from the environment
over time.  %An agent's decision to make an action in a given state is governed by its policy $\pi$.} 
The agent finds an optimal policy $\pi^{*}$ by calculating the optimal action-value function \gont{($Q^{*}$), also known as the \textbf{Q-value}} of the state-action pair, where $Q(S,A)$ represents the expected cumulative reward by taking an action A in a given state S.  

\gonz{Traditional RL methods (\rbc{e.g.,}~\cite{watkins1989learning,qlearning_ML_1992,rummery1994line,ipek2008self,pythia}) use a tabular approach with a lookup table to store the \rbc{Q-values associated with each} state-action pair. %Such an approach \rbc{is} inefficient for data placement in HSS due to a large number of possible states leading to high memory and computation requirements.  
These approaches can lead to high storage and computation overhead for environments with a large number of states and actions. % because the memory and computation requirements to store the values of all possible state-action pairs can be huge. %Therefore, these methods lack the capability to generalize and be effectively used in real-world scenarios. 
 To overcome this issue, \rbc{\emph{value function approximation} was proposed.~\cite{silver2016mastering,silver2017mastering,mnih2013playing,liang2016deep}}. Value function approximation replaces \gonzz{the} lookup table with \gonzz{a} supervised-learning model~\cite{sutton1999policy,baird1995residual,liang2016deep,mnih2013playing,silver2016mastering,silver2017mastering}, which provides the capability to generalize over a large number of state-action pairs with a low storage and computation overhead. } }

\vspace{0.1cm}
\iffalse
Each sequence of states and actions from an initial state to the final state is called an \emph{episode} or an \emph{iteration}.
\fi



 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.8\linewidth,trim={0cm 4cm 0cm 0cm},clip]{images/rl_abstract.pdf}
%      %\vspace{-0.1cm}
%   \caption{Conceptual diagram of reinforcement learning.}
% \label{fig:intro}
%  \end{figure}

 
%  \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{images/Hybrid_Storage_System.pdf}
%      \vspace{-0.1cm}
%   \caption{Overview of a hybrid storage system}
% \label{fig:hybrid}
%  \end{figure}
%The way an agent chooses actions to perform in a particular state becomes the agent's policy $\pi$. 





\iffalse
\gonff{
Traditional RL methods (\rbc{e.g.,}~\cite{watkins1989learning,qlearning_ML_1992,rummery1994line,ipek2008self,pythia}) use a tabular approach with a lookup table to store the \rbc{Q-values associated with each} state-action pair. Such an approach \rbc{is} inefficient for data placement in HSS due to a large number of possible states leading to high memory and computation requirements.  %These approaches cannot scale in real-world scenarios that have a high number of states and actions because the memory and computation requirements to store the values of all possible state-action pairs can be huge. Therefore, these methods lack the capability to generalize and be effectively used in real-world scenarios. 
To overcome this issue, we use \rbc{\emph{value function approximation}~\cite{silver2016mastering,silver2017mastering,mnih2013playing,liang2016deep}} that combines supervised-learning methods with an RL approach~\cite{sutton1999policy,baird1995residual,liang2016deep,mnih2013playing,silver2016mastering,silver2017mastering}. 
We use a deep RL-based approach that combines supervised-learning methods with an RL approach \cite{sutton1999policy,baird1995residual,liang2016deep,mnih2013playing,silver2016mastering,silver2017mastering}}
\fi
\vspace{-0.2cm}
\subsection{Why Is RL  a Good Fit for Data Placement in Hybrid Storage Systems?}


We choose RL \gon{for data placement in HSS} due to the following advantages
% There exist other machine learning (ML) approaches that can be used for system optimizations, we choose RL due to its following three advantages
% There exist other machine learning (ML) approaches that can be used for system optimizations, we choose RL due to its following three advantages
%\gagan{Reinforcement learning is a machine learning technique that involves an autonomous agent \js{learning} to perform optimal decisions to maximize its reward in an environment. 
compared to heuristic-based (e.g.,~\cite{matsui2017design,
meswani2015heterogeneous}) and supervised learning-based (e.g.,~\cite{ren2019archivist}) techniques.
%RL has three unique characteristics. 
% First, an RL agent aims to optimize a \grahul{performance} objective. This agent works autonomously to reach that objective without any direct human intervention. 



\head{(1) \gon{Adaptivity}} As discussed in Section \ref{sec:Sibyl/introduction} and Section \ref{sec:Sibyl/motivation_limitations}, a data placement technique should have the ability to adapt to changing workload demands and underlying device characteristics. This \gon{adaptivity}  requirement of data placement makes RL a good fit \gca{to model} data placement. %RL-based design does not require explicitly designing and implementing a new data-placement algorithm that requires us to spend time on specifying \emph{how} and \emph{which} features should be exploited to achieve the performance goal. 
The RL agent works autonomously \gon{in an HSS} using the provided \gca{state} features and reward to \gon{\gonx{make} data placement decisions} without any human intervention.

\head{(2) Online learning} Unlike an \emph{offline} learning-based approach, an RL agent uses an \emph{online} learning approach. Online learning allows an RL agent to  continuously adapt  its decision-making policy using  system-level feedback and specialize to \juangg{the} current workload and system configuration. %to changing workload demands \grakesh{and underlying device characteristics} while providing long term performance improvements.}
% Second, in case of a change in the environment (i.e., different workload or device), unlike a heuristics-based policy, the RL agent has the capability to self-optimize its decision-making policy to reach its defined objective. 
% Second, other learning techniques require \emph{labeled} data on optimal decisions while training these algorithms. \grahul{ It is virtually impossible to determine, let alone label, every possible system state with its optimal action. Thus, supervised learning techniques fall short. } In comparison, an RL agent does not require labeled data. An  agent updates its policy by interacting with the host and the storage system through \textit{actions} and \textit{rewards}.  

% \gca{As shown} in \cref{sec:evaluation}, our RL-based approach provides higher performance at lower implementation overhead \gca{than an RNN-based mechanism}.
\gont{
\head{(3) Extensibility} RL provides the ability to easily extend a mechanism with \gonzz{a} \gonff{small} effort required to implement the extension. As shown in Section \ref{subsec:Sibyl/trihybrid}, unlike heuristic-based mechanisms,  RL can be easily extended to different \gonff{types and} number of storage devices\gonff{. Such extensibility} reduces the system architect's burden in designing sophisticated data placement mechanisms.} 

\gonff{\head{(4) Design Ease} \gonz{With RL, the designer of the HSS} does not need to specify \gonz{a data placement} policy. They need to specify \emph{what} to optimize (via reward function) but not \emph{how} to optimize it. }

\gon{
\head{(5) Implementa\gont{tion Ease}} RL provides ease of implementation \gonff{that requires a} \gonz{small}  computation overhead. %Kleio~\cite{doudali2019kleio}, the state-of-the-art technique in hybrid main memory,   proposed sophisticated learning-based data-placement techniques using recurrent neural networks (RNNs).  
{As shown} in Section \ref{sec:Sibyl/results}, \textit{function approximation}-based~RL~techniques can generalize over all the possible state-action pairs by using a simple feed-forward neural network to provide high performance at low implementation overhead {\gont{(compared to} sophisticated RNN-based mechanisms}).}


\iffalse
    \hy{ The action-value function uses Bellman equation~\cite{sutton_2018} to represent how good it is for an agent to pick an action \textit{a} while being in state \textit{s} and following a certain policy $\pi$. }
    \vspace{-0.4cm}
    \begin{equation}
      \label{q-value}
    \Scale[0.74]{{Q^{\pi}(s_t,a_t) = \mathbb{E}\left[r_{t+1} + \gamma r_{t+2} + \gamma^{2} r_{t+3}.... \right]\left[ s_t, a_t\right]}} 
    \end{equation}
    \noindent \hy{ where $\mathbb{E}$ is the mathematical expectation for discount cumulative reward.}
    %when we provide the environment as a Markov decision process (MDP)~\cite{sutton_2018}. 
    For a certain state-action pair $(s, a)$, $Q^{\pi}(s, a)$ represents an estimate of expected future reward ($r_{t+1}$) while following a policy $\pi$.    The agent's goal is to find an optimal $\pi^{*}$ that maximizes the total reward over the agent's lifetime. The agent updates action-value function {$Q^{*}(s, a)$} 
    %by solving the following Bellman update~\cite{bellman1966dynamic} equation~\eqref{q-def}:
    by solving the Bellman update equation~\cite{bellman1966dynamic} \js{described as follows}:
    \vspace{-0.1cm}
    \begin{equation}
      \label{q-def}
    \Scale[0.74]{Q^{new}(s,a) \leftarrow Q(s,a)+ \alpha\left[r_{t+1} + \gamma \max_{a_{t+1}}~Q(S_{t+1},a_{t+1}) -Q(S_{t},a_{t})  \right]} 
    \end{equation}
    
    % \[ 
    % \Scale[0.8]{Q(s,a)=Q(s,a)+ \alpha\left[R_{t+1} + \gamma \max_{a'}~Q(S_{t+1},a_{t+1}) -Q(S_{t},a_{t})  \right]} \label{eqn:bellman}  \\
    % \]
    %where $0<\alpha, \gamma<1$ are learning rate and discount factor, respectively. 
    \noindent where $\alpha$, and $\gamma$ represent  learning rate, and discount factor, respectively, \js{in a range of $(0, 1)$}.
     The policy $\pi^{*}$ can be computed from $Q^{*}(s,a)$ by the following equation:
    \vspace{-0.1cm}
    \begin{equation}
    \pi^*=\argmaxH_a  Q^*(s,a).
    % \pi^*=\operatorname*{arg\,max}_{a} Q^*(s,a).
    \vspace{-0.0cm}
    \end{equation}
\fi
% There are two ways of calculating an agent's policy: (1) value iteration~\cite{bellman1957markovian} and (2) policy iteration~\cite{howard1960dynamic}. Value iteration{-based algorithms} iteratively update \q~until they converge to optimal values. Policy iteration{-based} algorithms aim to estimate the policy $\pi$  instead of improving the action-value function. In \js{this} work, we choose a value iteration{-based algorithm} rather than a policy iteration {-based algorithm} because value iteration \js{is} more sample-efficient\footnote{
% Sample efficiency measures the number of data samples required for an RL agent to converge to an optimal policy.} and less computationally expensive~\cite{nachum2017bridging}.
%A value function \texttt{V$^{\pi}$(s)} represent how good is a state for an agent to be in while state-action value 






==> PhD_Thesis_Updated_arxiv (1)/Sibyl/tables/devices_real.tex <==
\begin{table}[h]
% \vspace{-0.3cm}
\begin{center}
\small
\setstretch{0.9}
\vspace{5pt}
\caption{{Host system and \gca{storage devices used in} hybrid storage configurations }}
 \label{tab:Sibyl/devices}
  \renewcommand{\arraystretch}{1} %spacing between rows
\setlength{\tabcolsep}{2pt} %spacing between columns
 \resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{lll}
\hline
\multicolumn{1}{l|}{\textbf{Host System}}                  & 
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}AMD Ryzen 7 2700G~\gon{\cite{amdryzen}}, 8-core\gon{s}@3.5 GHz, \\ 8$\times$64/32 KiB L1-I/D, 4 MiB L2, 8 MiB L3,  \\16 GiB RDIMM DDR4 2666 MHz
\end{tabular}}  
\\ \hline
\multicolumn{1}{l|}{\textbf{Storage \rcamfix{Devices}}}                  & \multicolumn{2}{l}{\textbf{Characteristics}}                                                                                                                                        \\ \hline
\multicolumn{1}{l|}{\textsf{H}: Intel Optane SSD P4800X~\cite{inteloptane}}     & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}375 GB, PCIe 3.0 NVMe, SLC, R/W: 2.4/2 GB/s,\\ random R/W: 550000/500000 IOPS\end{tabular}} \\ \hline

\multicolumn{1}{l|}{\textsf{M}: Intel SSD D3-S4510~\cite{intels4510}} & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}1.92 TB, SATA TLC (3D), R/W: 550/510 MB/s, \\ random R/W: 895000/21000 IOPS\end{tabular}}           \\ \hline
\multicolumn{1}{l|}{\textsf{L}: Seagate \ghpca{HDD} ST1000DM010~\cite{seagate} } & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}1 TB, SATA 6Gb/s 7200 RPM \\ \rakesh{Max. Sustained Transfer Rate: 210 MB/s}\end{tabular}}   \\      \hline
\multicolumn{1}{l|}{\textsf{L$_{SSD}$}: ADATA SU630 SSD ~\cite{adatasu630} } & \multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}960 GB, SATA 6 Gb/s, TLC,   \\ Max R/W: 520/450 MB/s\end{tabular}}      
\\ \hline                          \multicolumn{1}{l|}{\textbf{HSS \gon{Configurations}}}              & \multicolumn{1}{l|}{\textbf{Fast \ghpca{Device}}  }                                                            & \textbf{Slow \ghpca{Device}}                                                             \\ \hline
\multicolumn{1}{l|}{\textsf{H\&M} (Performance-oriented) }                       & \multicolumn{1}{l|}{high-end (\textsf{H})}                                                                   & middle-end (\textsf{M})                                                                \\
\multicolumn{1}{l|}{\textsf{H\&L} (Cost-oriented) }                          & \multicolumn{1}{l|}{high-end (\textsf{H})}                                                                   & low-end (\textsf{L})                                                                   \\ \hline                                           
\end{tabular}
}
\end{center}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/tables/features.tex <==

{
% \floatsetup{style=BOXED,capposition=beside,capbesideposition={top,right},frameset={\fboxrule2pt\fboxsep1pt},colorframeset=yellowplate,framestyle=colorbox,framefit=yes,heightadjust=object,valign=c}
\begin{table}[h]
 \caption{State features \gon{used by} \namePaper}
    \label{tab:Sibyl/state}
\centering
% \resizebox{\linewidth}{!}{%
\small
 \renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{2pt}
  \resizebox{1\linewidth}{!}{%
\begin{tabular}{l||l|c|c}
\hline
\textbf{Feature}             & \textbf{Description} & \textbf{\# of bins} & 
\textbf{Encoding (bits)}\\ 
% & & &\textbf{Encoding (bits)}\\
\hline
% $a_j$                      &  address of incoming request    \\
\gonx{$size_t$}                      &  Size of the \gont{requested page (in pages)} &  8  & 8 \\
\gonx{$type_t$}                      &  Type of the \gont{current request (read/write) }  &2 & 4  \\
\gonx{$intr_t$}                      &  \gh{Access} interval \gon{of the requested page}&64 & 8 \\ 
\gonx{$cnt_t$}                      & Access \gonz{count} of the \gon{requested} page &64 &8   \\
\gonx{$cap_t$}   %(global counter)
&  Remaining capacity in the fast storage device  &8&8    \\
% $f_j/s_j$                      &  frequency to size of the incoming request   \\
% $d_j$                      &  difference in address of incoming and previous page   \\
\gonx{$curr_t$}                      &   Current {placement} \gon{of the requested page} \gonff{(fast/slow)} &2 & 4\\
\hline
\end{tabular}
% 
}
\end{table}

}

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/tables/hyperparameter.tex <==
\begin{table}[h]
\small
\begin{center}
 \caption{Hyper-parameters considered \gon{for} tuning }
    \label{tab:Sibyl/hyperparameter}
     \renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{10pt}
  \resizebox{1\linewidth}{!}{%
\begin{tabular}{l||l|l}
\hline
\textbf{Hyper-parameter}             & \textbf{Design Space} & \textbf{Chosen Value} \\  \hline

Discount factor   ($\gamma$)                           & 0-1  &0.9   \\
Learning rate     ($\alpha$)                  & $1e^{-5}-1e^{0}$ & $1e^{-4}$     \\
Exploration rate  ($\epsilon$)                           & 0-1  &0.001   \\
Batch size                          & 64-256   & 128     \\
\gonx{Experience buffer size ($e_{EB}$)}                         & 10-10000 & 1000      \\
\hline
\end{tabular}
}
\end{center}
\end{table}
 

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/tables/mixed_workloads.tex <==
\gsa{{
\begin{table}[h]
 \caption{Characteristics of mixed workloads}
    \label{tab:Sibyl/mixed_workloads}
\centering
% \resizebox{\linewidth}{!}{%
\normalsize
 \setstretch{0.8}
   \renewcommand{\arraystretch}{0.8} %spacing between rows
\setlength{\tabcolsep}{2pt}
  \resizebox{0.8\linewidth}{!}{%
\begin{tabular}{c||c|l}
\hline
\textbf{\rcamfix{Mix}}             & \textbf{\rcamfix{Workloads}} & \textbf{Description} \\ 
% \textbf{Setting}   & &\\
\hline
\hline
\textbf{mix1}                     &  $prxy\_0$~\cite{MSR} and $ntrx\_rw$~\cite{tarasov2016filebench} & \begin{tabular}{l}    
 Both $prxy\_0$ and \\ $ntrx\_rw$ are write-intensive
\end{tabular}
    \\
\hline
\textbf{mix2}                      &  $rsrch\_0$~\cite{MSR} and $oltp\_rw$~\cite{tarasov2016filebench}  &
\begin{tabular}{l} 
$rsrch\_0$ is  write-intensive and \\ $oltp\_rw$ is read-intensive
\end{tabular}
\\
\hline
\textbf{mix3}                      &  $proj\_3$~\cite{MSR} and $YCSB\_C$~\cite{cooper2010benchmarking}& 
\begin{tabular}{l}
Both $proj\_3$ and \\ $YCSB\_C$ are read-intensive
\end{tabular}
\\
\hline
\textbf{mix4}                      & $src1\_0$~\cite{MSR} and fileserver~\cite{tarasov2016filebench} &
\begin{tabular}{l}
Both $src1\_0$ and \\ fileserver have nearly equal \\ numbers of reads and writes
\end{tabular} \\
\hline
\textbf{mix5}                     & 
\begin{tabular}{l}
$prxy\_0$~\cite{MSR}, $oltp\_rw$~\cite{tarasov2016filebench} and \\ fileserver~\cite{tarasov2016filebench}
\end{tabular}
&
\begin{tabular}{l}
$prxy\_0$ is write-intensive, \\ $oltp\_rw$ is read-intensive, and \\fileserver has nearly equal \\numbers of reads and writes
\end{tabular}
\\
\hline
\textbf{mix6}                     &   
\begin{tabular}{l}
$src1\_0$~\cite{MSR}, $YCSB\_C$~\cite{cooper2010benchmarking} and \\ fileserver~\cite{tarasov2016filebench}  
\end{tabular}
&
\begin{tabular}{l}
$src1\_0$ and fileserver have\\nearly equal numbers \\of reads and writes while \\$YCSB\_C$ is read-intensive
\end{tabular}
\\
\hline
\end{tabular}
}
\end{table}
}
}

==> PhD_Thesis_Updated_arxiv (1)/Sibyl/tables/workload.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
% 
\caption{Characteristics of 14 evaluated workloads}
 \label{tab:Sibyl/workload}
 \centering
 \tiny
 \setstretch{0.85}
   \renewcommand{\arraystretch}{0.85} %spacing between rows
\setlength{\tabcolsep}{2pt} %spacing between columns
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{@{}lrrrrr@{}}
\hline
 \textbf{Workload}        & \multicolumn{1}{l}{\textbf{Write}} & \multicolumn{1}{l}{\textbf{Read}} & \multicolumn{1}{r}{\textbf{Avg. request}} & \multicolumn{1}{r}{\textbf{Avg. access}} & \textbf{No. of unique}  \\ 
                &         \%                  &    \%                      & \multicolumn{1}{r}{\textbf{size}}          & \multicolumn{1}{r}{\textbf{\gonz{count}}} & \textbf{requests} \\ 
         
         \hline
$hm\_1$    & 4.7\%                     & 95.3\%                   & 15.2                                  & 44.5                                  & 6265                     \\


$mds\_0$    & 88.1\%                     & 11.9\%                   & 9.6                                  & 3.5                                  &        31933              \\
$prn\_1$   & 24.7\%                    & 75.3\%                   & 20.0                                  & 2.6                                  & 6891                     \\
$proj\_0$  & 87.5\%                    & 12.5\%                   & 38.0                                  & 48.3                                 & 1381                     \\
$proj\_2$  & 12.4\%                    & 87.6\%                   & 42.4                                 & 2.9                                  & 27967                    \\
$proj\_3$  & 5.2\%                     & 94.8\%                   & 9.6                                  & 3.6                                  & 19397                    \\
$prxy\_0$  & 96.9\%                    & 3.1\%                    & 7.2                                  & 95.7                                 & 525                      \\
$prxy\_1$  & 34.5\%                    & 65.5\%                   & 12.8                                  & 150.1                                 & 6845                     \\
$rsrch\_0$ & 90.7\%                    & 9.3\%                    & 9.2                                 & 34.7                               & 5504                     \\
$src1\_0$  & 43.6\%                    & 56.4\%                   & 43.2                                 & 12.7                                  & 13640                    \\
$stg\_1$   & 36.3\%                    & 63.7\%                   & 40.8                                 & 1.1                                  & 3787                     \\
$usr\_0$   & 59.6\%                    & 40.4\%                   & 22.8                                  & 19.7                                  & 2138                     \\
$wdev\_2$  & 99.9\%                    & 0.1\%                    & 8.0                                  & 17.7                                 & 4270                     \\
$web\_1$   & 45.9\%                    & 54.1\%                   & 29.6                                  & 1.2                                  & 6095                     \\ \hline
\end{tabular}
}
\end{table}


==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/abstract.tex <==
Modern scientific workloads have demonstrated the inefficiency of using high-precision formats. Moving to a lower bit format or even to a different number system can provide tremendous gains in terms of performance and energy efficiency. This chapter explores the applicability of different number formats and searches for the appropriate bit-width for three-dimensional stencil kernels, which are among the most widely used scientific workloads. Further, we demonstrate the achievable performance of these kernels on state-of-the-art hardware that includes a host CPU connected to an FPGA. An FPGA provides us with the capability to implement arbitrary fixed-point precision. Thus, this chapter fills the gap between current hardware capabilities and future systems for stencil-based scientific applications.

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/background.tex <==
% \subsection{POWER9 Processor}
% The IBM POWER9 is the latest addition to the IBM's POWER processor family. POWER9 cores have been optimized for stronger thread performance and efficiency. It has been designed to handle a wide range of workloads, from deep learning (DL) and artificial intelligence (AI) to data-analytics and high-performance computing (HPC). IBM POWER9 processors can offer up to 22 cores at up to 2.80 GHz (3.10 GHz turbo) performance with up to 2 TB of memory~\cite{caldeira2018ibm}. It comes with fourth-generation PCIe 4.0, NVIDIA NVLink 2.0 technology, IBM Coherent Accelerator Processor Interface (CAPI) 2.0, and the new IBM OpenCAPI 3.0 interface. Moreover, this new processor design gives the capability of attaching up to six  NVIDIA Tesla V100 GPUs, based on the NVIDIA SXM2 form factor connectors. POWER9 processor enables deeper out-of-order execution, better branch prediction, larger cache spaces, and wider bandwidth

\section{Background}
% \spaceSectionHeading
\label{sec:low_precision/background}
This section provides details on the stencil kernels used and discusses the relevance of the precision analysis.
\vspace{-0.2cm}
\subsection{Stencil Benchmark}
% \spaceSubSectionHeading
Stencil computation updates a multi-dimensional grid based on a specific computation pattern. A stencil kernel's performance on the current multicore system depends heavily on the data mapping of the grid. For instance, suppose a 3D grid in (\textit{row}, \textit{column}, \textit{depth}). When the grid is stored by \textit{row}, accessing data elements in the other dimensions typically results in cache eviction. This issue is because, for real-world applications, the problem size is too large to fit in the processor cache.
\input{Stencil_Precise/hdiff.tex}
This chapter focuses on both a \sevpoint and \tfivepoint 3D elementary stencil and a compound horizontal diffusion (\hdiff) stencil, shown in Figure~\ref{fig:low_precision/kernels}. These kernels access a three-dimensional grid and have complex access patterns.  The 3D \sevpoint and \tfivepoint (see Figure~\ref{fig:low_precision/stencil7&25}) stencils commonly arise
from the finite difference method for solving partial differential equations~\cite{stencilOnPOWER8}. 
 The \sevpoint stencil performs
eight FLOPS per grid point, while the \tfivepoint stencil performs twenty-seven FLOPS per grid point (without any common subexpression elimination). Thus, the arithmetic intensity,
the ratio of FLOPS performed for each byte of memory traffic, is much higher
for the \tfivepoint stencil than the \sevpoint stencil.  

As discussed in Chapter~\ref{chapter:nero}, stencil patterns in a real-world weather prediction application consist of a collection of stencils that performs a sequence of element-wise computations. Horizontal diffusion kernel is an example of one such kernel that executes each
stencil using a separate loop nest. It iterates over a 3D grid that performs \textit{laplacian} and \textit{flux}, as depicted in Figure~\ref{fig:low_precision/stencilHdiff}, as well as calculations for different grid points. Such compound kernels have intricate memory access patterns because they apply a series of elementary stencil operations. Although such implementations may be straightforward to write, they are not efficient in terms of data
locality, memory usage, or parallelism. 


% \begin{algorithm}
% \caption{Demonstration of 7 points 3D stencil}
% \label{3dStencil}
% \begin{algorithmic}[1]
% % \Procedure{void stencilComputation}{double depth, double column, double row}
% \State{void stencilComputation}{(double depth, double column, double row)}

 
%     \For {$d\gets 1$ to depth+$ 1$}
%         \For {$c\gets 1$ to column+$ 1$}
%         \For {$r\gets 1$ to row+$ 1$}
%             \State Calculate 7 point stencil
%  \EndFor
%  \EndFor
%  \EndFor

% % \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \caption{Demonstration of 25 points 3D stencil}
% \label{3dStencil}
% \begin{algorithmic}[1]
% % \Procedure{void stencilComputation}{double depth, double column, double row}
% \State{void stencilComputation}{(double depth, double column, double row)}

 
%     \For {$x\gets 2$ to depth-$ 2$}
%         \For {$y\gets 2$ to column-$ 2$}
%         \For {$z\gets 2$ to row-$ 2$}
%              \State dest[x][y][z] =24 * src[x][y][z] - (src[x-2][y][z] + src[x-1][y][z] +
%             \State src[x+1][y][z] + src[x+2][y][z] + src[x][y-2][z] + 
%     \State src[x][y-1][z] + src[x][y+1][z] + src[x][y+2][z] + 
%     \State src[x][y][z-2] + src[x][y][z-1] + src[x][y][z+1] + 
%     \State src[x][y][z+2] + src[x-1][y-1][z] + src[x+1][y-1][z] +    \State src[x-1][y+1][z] + src[x+1][y+1][z] + src[x-1][y][z-1] + 
%     \State src[x+1][y][z-1] + src[x-1][y][z+1] + src[x+1][y][z+1] +
%     \State src[x][y-1][z-1] + src[x][y+1][z-1] + src[x][y-1][z+1] +
%     \State src[x][y+1][z+1]);
%  \EndFor
%  \EndFor
%  \EndFor

% % \EndProcedure
% \end{algorithmic}
% \end{algorithm}
\vspace{-0.2cm}
\subsection{Precision Optimization}
% \spaceSubSectionHeading
IEEE-754 floating-point representation has become the universal standard in modern computing systems. Floating-point numbers have a mantissa and exponent component with an additional bit to represent the sign of a number. In terms of computing resources, this floating-point arithmetic requires complex circuitry leading to high latency and power consumption~\cite{finnerty2017reduce}. 

The use of low-precision arithmetic with a minimal loss in the accuracy has been proposed as a promising alternative to the commonly used floating-point arithmetic for emerging workloads, e.g.,
machine learning and graph processing. From the system perspective, there are two main benefits of moving to a
lower precision. First, the hardware resources
for a given silicon area may enable higher operations per second
(OPS) at a lower precision as these operations require less hardware
area, and thus power. Note, this also necessitates efficient memory traffic management. Secondly, many operations are memory bandwidth bound~\cite{singh2019near,NAPEL}, and reducing precision would allow for better cache usage and reduction of bandwidth bottlenecks.
Thus, data can be moved faster through the memory hierarchy to maximize the utilization of computing resources.
% \spaceSectionEnd

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/conclusion.tex <==
\section{Conclusion}
\label{sec:low_precision/conclusion}
Stencils are one of the most widely used computational kernels across various real-world applications. This chapter analyzed the precision tolerance for different 3D stencil kernels using fixed-point, floating-point, and posit number systems. We demonstrated by exhaustive precision exploration that these kernels have a margin to move to a lower bit-width with minimal loss of accuracy using different number formats.

Further, in a case study, we measured the performance of these kernels on a state-of-the-art multi-core platform and designed lower bit-width-based accelerators for all considered 3D stencil kernels on an FPGA platform. FPGA is the only device that gives us the capability to implement arbitrary fixed-point precision data types. Hence, we leveraged this capability to show the advantages of accelerating these kernels with lower precision compared to the ubiquitous IEEE floating-point format.  In the future, we can use this analysis technique in an integrated design-flow to build efficient systems for stencil-based applications. Another future direction would be to study the effects of low precision processing not only for streaming applications, e.g., stencil and convolution, where computation is done locally but also for iterative applications where errors accumulate.
%Moreover, we will work on extending this analysis to other kernels in different domains.


==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/evaluation.tex <==
\section{Evaluation}
% \spaceSectionHeading
\label{sec:low_precision/evaluation}
We use IBM\textsuperscript{\textregistered} POWER9 as the host system comprising of 16 cores, each of which supports four-thread simultaneous multi-threading. Table~\ref{tab:low_precision/systemparameters}
provides complete details of our system parameters. To provide a full-scale analysis of stencil optimization techniques, we set the grid size of all stencil kernels as $1280\times1080\times960$, much larger than the on-chip cache capacity of POWER9, with input data distribution as a Gaussian function. The problem size dictates which input dataset would reside in the cache; hence is an important parameter while measuring the system performance.  Note: in Chapter~\ref{chapter:nero}, we use a grid domain used by the COSMO weather
prediction model. 
\input{Stencil_Precise/system_gagan}
For precision tuning of the fixed-point number system, we use the Xilinx fixed-point library from the Vivado 2018.2 tool~\cite{xilinx_hls}. We use the C++ template-based \emph{FloatX} (Float eXtended) library~\footnote{https://github.com/oprecomp/FloatX} to explore arbitrary precision for floating-point arithmetic. Software-based posit implementation is available as part of the ongoing efforts to develop an ecosystem for posit evaluation\footnote{https://github.com/stillwater-sc/universal}. All three libraries are provided as a C++ header format, which allows us to replace the data types in the source code of the application and study the effect of low precision using the same software toolchain as that of the application itself.
We develop a highly optimized FPGA accelerator for all the kernels to make a performance comparison between floating-point and fixed-point number systems. We implement these designs on an Alpha-Data ADM-PCIE-9V3~\cite{ad9v3} card featuring the Xilinx Virtex Ultrascale+ XCVU3P-FFVC1517-2-i device.
%  \vspace{-0.8cm}
% \input{Stencil_Precise/system.tex}

% \vspace{-0.75cm}
%  \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{perfromance.png}
% \caption{\tfivepoint stencil performance
% \label{fig:perf}}
% \end{figure}
\subsection{Emulated Precision Tuning}
% \spaceSubSectionHeading
The tuning process analyzes multiple configurations for each of the arithmetic types considered. The tuner re-executes the program for each
configuration and computes the error on its output values to
provide a measure of the resultant accuracy.
Figure~\ref{fig:low_precision/precisionResults} shows the precision results for the considered workloads for three different number systems. The accuracy is compared to the most ubiquitously used IEEE single-precision floating number system. 

For all the kernels, we can achieve full accuracy with much lower bits. Moreover, as the error tolerance increases, we could use a lower number of total bits. Based on this, we make three observations. First, in the case of a \sevpoint and \tfivepoint stencil, we could reduce bits by more than $50\%$ for the considered three data types, with a precision loss of only $1\%$. Second, elementary 3D stencil kernels (\sevpoint and \tfivepoint) could not exploit the high dynamic range offered by posit. Therefore, with a lower bit-width floating-point arithmetic, we could achieve better results. Third, the weather compound kernel comparatively needs a higher dynamic range; therefore, with $0.1\%$ tolerance in the accuracy, we could cut the number of bits to half compared to the IEEE floating-point and move to a posit of (16,2). This observation motivates the use of posit number format can be useful in the domain of weather prediction modeling.

\begin{figure}[h]
 \centering
 \includegraphics[bb=10 12 725 264,width=\linewidth]{Stencil_Precise/bitAccuracy.pdf}
%  \vspace{-0.5cm}
 \caption{Total bits vs accuracy (percentage) for (a) \sevpoint, (b) \tfivepoint, and (c) horizontal diffusion compared to single-precision IEEE floating-point representation. Notation fixed (\textit{w},\textit{i}) defines a fixed number with total \textit{w} bits including \textit{i} integer bits. With floatx, \textit{e} refers to the exponent bits and \textit{m} defines the mantissa. In the case of the posit number system, \textit{n} is the total number of bits with \textit{es} bits for the exponent part
 \label{fig:low_precision/precisionResults}}
%  \vspace{-0.7cm}
 \end{figure}
 
 \subsection{Case Study for Current Multi-Core Systems and Arbitrary Precision Supported Hardware}
% \spaceSubSectionHeading
We perform a case study to measure the capabilities of current state-of-the-art hardware platforms.
 We tune the considered stencil kernels both for IBM POWER9 CPU and for a high-end FPGA platform. Our FPGA is coherently attached to our host CPU through the CAPI2 link. For the FPGA and the POWER9 node, we use the AMESTER\footnote{https://github.com/open-power/amester} tool to measure the active power consumption.
 
 Our current FPGA devices only support floating-point and arbitrary fixed-point arithmetic. Therefore, we compared hardware implementations across the stencil benchmarks for floating-point single and half precision with fixed-point datatype for the bit width that gave similar accuracy to the floating-point. Note, as current state-of-the-art hardware devices do not support the posit data type, we did not include it in our hardware comparison because the emulation of posit data type would be expensive in an FPGA and would lead to unfair comparisons with other data types. In Appendix~\ref{chapter:precise_fpga}, we develop PreciseFPGA, an automated framework to obtain an application-aware optimal fixed-point configuration without exhaustively searching the entire design space. 



 In Figure~\ref{fig:low_precision/system}, we show a high-level overview of our integrated system. The FPGA is connected to a server system, based on the IBM\textsuperscript{\textregistered} POWER9 processor, using IBM\textsuperscript{\textregistered} coherent accelerator processor interface 2.0 (CAPI~2.0). The FPGA implementation consists of accelerator function units (AFU) that interact with the power service layer (PSL), which is the CAPI endpoint on the FPGA. The co-designed execution flow is shown in Figure~\ref{fig:low_precision/execution}. We provide the experimental results of tuning stencil kernels for current CPU and FPGA-based systems. 
 
  \begin{figure}[h]
\centering
\begin{subfigure}[h]{.6\textwidth}
  \centering
  \includegraphics[bb=1 7 847 346,width=\linewidth]{Stencil_Precise/System.pdf}
  \caption{
  \label{fig:low_precision/system}}
\end{subfigure}%
\begin{subfigure}[h]{.4\textwidth}
  \centering
  \includegraphics[bb=5 4 339 192,width=\linewidth]{Stencil_Precise/Execution.pdf}
    \caption{
  \label{fig:low_precision/execution}}
\end{subfigure}
 \vspace{-0.1cm}
\caption{(a) CAPI 2-based accelerator platform with IBM\textsuperscript{\textregistered} POWER9 (b) FPGA is acting as a peer to the  CPU by accessing the main memory through a high-performance CAPI2 link, enabled by PSL. Data flow sequence from the  Host  DRAM  to the onboard  FPGA  memory. A software-defined API handles offloading jobs to accelerators with an interrupt-based queuing mechanism that allows minimal CPU usage (thus, power) during FPGA use}
% \vspace{-1cm}
\end{figure}

 Figure~\ref{fig:low_precision/roofline} shows the roofline of the three stencil kernels  (\sevpoint, \tfivepoint, and \hdiff)  that we use in this study. By mapping both, arithmetic intensity of all examined stencils and peak attainable GFLOP/sec (GOP/sec for fixed-point) on the roofline of our heterogeneous system (CPU+FPGA), we make the following three observations. First, we observe that compiler and tiling optimizations~\cite{stencilOnPOWER8} lead to 125.2$\times$ 119.4$\times$ and 90.4$\times$ speedup compared to non-optimized CPU implementations for \sevpoint, \tfivepoint, and \hdiff, respectively. The memory bandwidth constrains the performance of elementary stencils (\sevpoint, \tfivepoint) since the stencil data for the 3D grid cannot be mapped to contiguous memory location leading to limited cache locality. Although \hdiff has a higher arithmetic intensity, its access patterns are more complex because it applies a series of elementary stencil operations with different stencil patterns. 
 
  \begin{figure}[h]
 \centering
 \includegraphics[width=1.1\linewidth,trim={1.2cm 0.6cm 0.4cm 0.4cm},clip]{Stencil_Precise/roofline_samos19.eps}
%  \caption{Attainable performance for the examined stencils, in CPU and FPGA testbeds, with different precision data types.
 \caption{Roofline~\cite{williams2009roofline} for POWER9 (1-socket) showing elementary stencil (\sevpoint and \tfivepoint) and horizontal diffusion (\texttt{hdiff}) kernels for single-thread baseline and 64-thread fully-optimized %(one socket) 
    implementations. %Also shown is 
    The plot shows also the roofline %potential 
    of the FPGA with attained performance of our examined stencils using different precision data types
 \label{fig:low_precision/roofline}}
%  \vspace{-0.65cm}
 \end{figure}
 
Second, we observe that the floating-point FPGA implementations increase the additional speedup to 2.5$\times$, 3.3$\times$, and 4.1$\times$ compared to the CPU-optimized implementation for \sevpoint, \tfivepoint, and \hdiff, respectively. By effectively using the FPGA's on-chip memory, the FPGA-based implementations are not constrained by the DRAM memory bandwidth. However, the CAPI2/PCIe4 link offers an order of magnitude less bandwidth than that of the host CPU's DRAM. Since our platform offers memory-coherent access of FPGA to the system memory, we build a pipelined execution, where communication time for transferring data from host to FPGA memory is masked with the actual FPGA processing~\cite{diamantopoulos2018ectalk}. This technique allows us to exploit FPGA processing capabilities completely. 

Third, we have measured additional gains by replacing a single-precision floating-point data type with a lower precision data type.  Specifically, in the roofline of Figure~\ref{fig:low_precision/roofline}, we plot the performance of three stencils using half and fixed-point data types. The specific bit-width for the integer and fractional part of the fixed point was selected at 99\% accuracy, i.e., Q14.7 for \tfivepoint, Q16.4 for \sevpoint, and Q11.5 for \hdiff. Arithmetic intensity is improved for both half and fixed data types since the bytes fetched from memory are half that of the single-precision floating-point (i.e., 2 bytes instead of 4 bytes). Since fixed-point implementations use fewer resources on an FPGA than float and half, we were able to add more accelerators on the same FPGA device, allowing us to measure 468.1, 527.9, and 659.1 GOPs/sec for \sevpoint, \tfivepoint, and \hdiff, respectively. These numbers are very close to the theoretical peak performance of   0.97 TOPs/s offered by our FPGA device %when the device is configured with the stencil micro-architecture of \sevpoint, \tfivepoint and \hdiff
\footnote{While the three stencils comprise different access patterns and acceleration kernels, the primary operations, i.e., vectorized multiply-accumulate computation (MAC), which define the FPGA micro-architecture, remain the same. Using vectorized 
MAC, we have calculate 0.97 TOPs/s theoretical top performance for stencils for our AD9V3 FPGA.}.

% We make use of XLC compiler with appropriate flags targeting IBM POWER9 CPU. While optimize our code and also explore different SMT (simultaneous multi-threading modes) and report the best performing configuration. Effective multi-threading on POWER9 with combination of SMT levels can provide different results. Stencil algorithms are usually memory bounded hence benefits by using SMT can be lower than its overhead. 
% % As can be seen, by using OpenMP SMT2 generates better results compared to SMT4. Thus by reducing maximum SMT, can save the space for more cores if the processors This was the similar scenario on earlier POWER machine~\ref[STENCIL PAPER].

%  POWER9 has large amount of cache capacity and by tiling we were able to achieve the highest gains. We decompose the entire grid into chunk blocks based on the size of last level cache (LLC). Due to which DRAM access are reduced and hence we are able to reduce the memory contention. Furthermore, this reduction in contention provides us with linear performance gains with increase in SMT. Even after fully optimizing these kernels we are not able to reach the peak CPU performance. Large amount of time is spent in data movement rather than the computing. Based on this observation we investigate the tolerance of these 3D stencils to a lower precision and implement that design in FPGA.  Figure~\ref{fig:7-pointRes} shows the totals bits and accuracy obtained for \sevpoint and \tfivepoint stencil respectively. 
 

 
Table~\ref{tab:low_precision/fpgaResources} shows the resource utilization for our examined stencil kernels on an FPGA using different precision data types. In all the scenarios, going from single to half-precision increases the performance with a corresponding reduction in the number of resources. Further, moving to fixed-point arithmetic representation increases the performance due to a decrease in the number of bytes loaded at the cost of LUT utilization. However, the utilization of other FPGA resources is reduced. Figure~\ref{fig:low_precision/energyEff} shows the achieved energy efficiency with different precision data types. As the number of bits reduces, we see an increase in energy efficiency for all considered kernels. Designs implemented in fixed-point will always be more efficient than their equivalent in floating-point alternative because fixed-point implementations consume fewer resources and less power (see Table~\ref{tab:low_precision/fpgaResources}). As these stencil kernels do not require the high dynamic range achievable with
floating-point, moving to fixed-point implementations could provide better energy efficiency. In the case of \hdiff, we see a huge increase in energy efficiency on moving to a lower precision. This increase is because \hdiff is a compound kernel; therefore, each elementary stencil's energy improvement with lower precision leads to much higher cumulative gains.
% \vspace{-0.8cm}
\input{Stencil_Precise/fpga.tex}

   \begin{figure}[h]
 \centering
 \includegraphics[bb=14 12 509 191,width=\linewidth]{Stencil_Precise/energyEfficiency.pdf}
 \vspace{-0.8cm}
 \caption{Evaluated design points for different stencil kernels. The plot shows energy efficiency (GFLOPS/Watt) with different precision implementations on an Alpha-Data ADM-PCIE-9V3~\cite{ad9v3} card featuring the Xilinx Virtex Ultrascale+ XCVU3P-FFVC1517
 \label{fig:low_precision/energyEff}}
%  \vspace{-0.3cm}
 \end{figure}
 
%  \spaceSectionEnd
% \vspace{-0.4cm}



==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/fpga.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\renewcommand{\arraystretch}{0.95}
\setlength{\tabcolsep}{8pt}
\centering
   \caption{FPGA resource utilization and performance for the examined stencil kernels on FPGA testbeds, with different precisions}
    \label{tab:low_precision/fpgaResources}
\resizebox{\textwidth}{!}{% use resizebox with textwidth
\begin{tabular}{p{1.6cm}Hp{2cm}ccccccc}
\toprule
\multirow{2}{*}{\textbf{Kernel}} & \multirow{2}{*}{Data Size} & \multirow{2}{*}{\textbf{Precision}}&\multirow{2}{*}{\textbf{Accuracy} \textbf{(\%)}}  & \multicolumn{4}{c}{\textbf{Utilization} (\%)} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Performance}\\ \textbf{(GLOP/s)}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Energy} \\ \textbf{(mJ)}\end{tabular}} \\ \cline{5-8}
&                            &                          &  & {BRAM}    & {DSP}   & {FF}   & {LUT}    &                                                                                 &                                                    \\ \hline
\sevpoint                  & $1280\times1080\times960  $              & float         &100             & 38      & 35     & 18   & 29     & 228.4                                                                           & 4617.2                                                                     \\
\sevpoint                  & $1280\times1080\times960    $           & half &99.95                      & 25      & 24     & 15   & 28     & 319.5                                                                           & 2887.6                                                                     \\
\sevpoint                  &$1280\times1080\times960$                 & fixed (20,4)    &100           & 16      & 12     & 49   & 95    & 467.6                                                                           & 1832.3                                                                     \\
\sevpoint                  & $1280\times1080\times960 $               & fixed (16,4)      &99.96         & 12      & 12     & 47   & 92.5   & 468.1                                                                          & 1689.4                                                                     \\
%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\tfivepoint                 & $1280\times1080\times960$              & float    &100                  & 42      & 62    & 36   & 44     & 327.7                                                                           & 1608.7                                                                     \\
\tfivepoint                 & $1280\times1080\times960$            & half     & 99.06                  & 32      & 43   & 32   & 43     & 342.1                                                                         & 1541.5                                                                     \\
\tfivepoint                 & $1280\times1080\times960$              & fixed (22,7)      & 100         & 29       & 21    & 56   & 95    & 527.9                                                                         & 1510.3                                                                     \\
\tfivepoint                 & $1280\times1080\times960 $               & fixed (14,7)       &99.05        & 19       & 21    & 55   & 91     & 528.9                                                                         & 1497.9                                                                     \\
%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\hdiff                   & $1280\times1080\times960$                & float    &100                  & 52      & 89    & 65   & 61     & 350.3                                                                       & 3010.5                                                                      \\
\hdiff                   &$1280\times1080\times960  $                 & half  &98.02                     & 44      & 84    & 35   & 57     & 421.8                                                                         & 2031.1                                                                      \\
\hdiff                   &$1280\times1080\times960   $                & fixed (21,5)    &100           & 24      & 45     & 77  & 76     & 653.9                                                                        & 1007.9                                                                       \\
\hdiff                   & $1280\times1080\times960   $                   & fixed (11,5)   &97.92            & 14       & 35     & 69   & 71     & 659.1                                                                   & 997.9                        \\\bottomrule                                                     
\end{tabular}}
\vspace{-0.4cm}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/hdiff.tex <==
\begin{figure}[htp]

\begin{subfigure}[t]{0.5\textwidth}
\centering
\includegraphics[bb=54 138 703 460,width=\linewidth,trim={0.8cm 4.9cm 0.4cm 2cm},clip]{Stencil_Precise/stencil.pdf}
 \caption{
\label{fig:low_precision/stencil7&25}}
\end{subfigure}
  %
  \begin{subfigure}[t]{0.5\linewidth}
\centering
\resizebox{0.8\textwidth}{!}{
    \begin{tikzpicture}[rotate=90,transform shape]

    %draws helper-grid:
%%%%%%%%%%%%%LAPLACE
    \gridThreeD{0}{8.25}{black};
    \node at (7.5,10.25)[ rotate=270] {\huge \textit{Laplace}};
      \dotesUpper{0}{8.25};
    %%%%%%%%%%%%%FLUX 
    \gridThreeDSecond{1}{4}{black};
    \node  at (7.5,5.5)[ rotate=270] {\huge \textit{Flux}};
     \lowerDots{3}{4};
     
        %%%%%%%%%%%%%OUTPUT
    \gridThreeDThird{2}{0}{black};
     \node  at (7.5,0.25) [ rotate=270] {\huge \textit{Output}};
     \lowestDot{1.6}{-0.45}
     
     
      \draw [thick,->,blue] (2.75,4.25) -- (2.7,8.4);
       \draw [thick,->,blue] (2.75,4.25) -- (2.1,8.9);
       \draw [thick,->,blue] (2.75,4.25) -- (4.1,8.9);
       \draw [thick,->,blue] (2.75,4.25) -- (3.5,9.4);
    
    
       \draw [thick,->,orange] (2.1,4.7) -- (3.5,9.4);
       \draw [thick,->,orange] (2.1,4.7) -- (1.5,9.4);
       \draw [thick,->,orange] (2.1,4.7) -- (2.1,8.9);
       \draw [thick,->,orange] (2.1,4.7) -- (2.9,9.9);
     
       \draw [thick,->,red] (4.1,4.7) -- (3.5,9.4);
       \draw [thick,->,red] (4.1,4.7) -- (5.5,9.4);
       \draw [thick,->,red] (4.1,4.7) -- (4.1,8.9);
       \draw [thick,->,red] (4.1,4.7) -- (4.9,9.9);
    
    
 
           \draw [thick,->,brown] (3.5,5.25) -- (3.5,9.4);
           \draw [thick,->,brown] (3.5,5.25) -- (2.9,9.9);
           \draw [thick,->,brown] (3.5,5.25) -- (4.9,9.9);
           \draw [thick,->,brown] (3.5,5.25) -- (4.3,10.4);
           %lowest to the middle
         \draw [thick,->,violet] (2.7,0.25) -- (3.5,5.15);
         \draw [thick,->,violet] (2.7,0.25) -- (4.1,4.65);
         \draw [thick,->,violet] (2.7,0.25) -- (2.1,4.65);
         \draw [thick,->,violet] (2.7,0.25) -- (2.75,4.15);
    
    
    
    % %draws lower graph lines and those in z-direction:
    
    % draws all graph nodes:
   
  
   
\end{tikzpicture}
}
 \caption{
 \label{fig:low_precision/stencilHdiff}}
\end{subfigure}
\vspace{-0.1cm}
\caption{(a) 7-point stencil and 25-point elementary stencils (b) Compound horizontal diffusion stencil that is used by the COSMO weather prediction model 
\label{fig:low_precision/kernels}}
\vspace{-0.25cm}
\end{figure}

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/introduction.tex <==
\section{Introduction}
Stencil computation is essential for numerical simulations of finite difference methods~(FDM)~\cite{ozicsik2017finite} and is applied in iterative solvers of linear equation systems. We use stencil computation in a wide range of applications, including computational fluid dynamics~\cite{huynh2014high}, image processing~\cite{hermosilla2008non}, weather prediction modeling~\cite{doms1999nonhydrostatic}, etc. A stencil operation~\cite{gysi2015modesto} defines a computation sequence where elements in a multidimensional grid are updated using data values from a subset of its neighbors based on a fixed pattern.

Stencil computation is applied to data structures that are generally much larger than the available system's cache capacity~\cite{datta2008stencil}. Stencils are cache-unfriendly because the amount of data reuse within a stencil iteration is limited to the number of points in a stencil. Due to the cache-unfriendly, complex data
access patterns, and low operational intensity~\cite{stencilOnPOWER8,singh2020nero}, stencil compute kernels do not perform well on traditional CPU or GPU-based systems. 

High-performance implementations of stencils on modern processors operate using a single-precision or a double-precision floating-point data type. The floating-point format is the most widely supported datatypes by our current hardware devices. Using this data type in real-world applications, which use large grid sizes, puts enormous stress on the memory subsystem.  Therefore, storing data in the memory using a smaller number of bits can decrease the memory footprint and provide reductions in latency and energy consumption. The industry trend~\cite{finnerty2017reduce} shows a clear shift away from using floating-point representation. For example, applications like
neural networks can use an 8-bit fixed-point format or lower precision without significant loss in accuracy~\cite{iwata1989artificial}. Hence, in this chapter, we examine the use of different number systems -- fixed-point, posits, floating-point -- and analyze the precision tolerance of three-dimensional stencil kernels, one of the most widely used kernels in real-world applications.

% To summarize, the major contributions of this paper are:
% \begin{itemize}

% \item We perform a systematic precision exploration of 3D stencil kernels for future mixed-precision systems using a wide range of number systems including fixed-point, floating-point, and posit.
 
% \item Based on an exhaustive exploration of a broad range of number systems -- fixed-point, floating-point, and posit, we provide optimum precision and the corresponding accuracy deviation.

% \item We tune these kernels on current state-of-the-art IBM\textsuperscript{\textregistered} POWER9\footnote{IBM and POWER9 are registered trademarks or common law marks of International Business Machines Corp., registered in many jurisdictions world-wide. Other product and service names might be trademarks of IBM or other companies.} CPU and further evaluate them on an FPGA supporting arbitrary precision, which is coherently attached to the host memory. Thus, this work fills the gap between the current hardware capabilities and future hardware design.
% \end{itemize}


% The remainder of this chapter is structured as follows. Section~\ref{sec:low_precision/background} provides details on the various 3D stencil kernels and the benefits of lower precision. In Section~\ref{sec:methodology} we describe the methodology and different number systems explored. Section~\ref{sec:evaluation} mentions the system setup and provides the results of our experiments, including a case study of implementing and optimizing these kernels on current state-of-the-art hardware devices. We list the related work in Section~\ref{sec:relatedWork} and Section~\ref{sec:conclusion} concludes with future directions.
% % \spaceSectionEnd

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/methodology.tex <==
\section{Methodology}
% \spaceSectionHeading
\label{sec:low_precision/methodology}
The following section provides detail on our methodology to explore precision for different number systems, as depicted in Figure~\ref{fig:low_precision/methodology}. In the first phase (\circled{1}), we analyze and instrument a part of an application for which the precision exploration needs to be performed. In the next phase (\circled{2}), we execute an exhaustive search to find the appropriate precision based on the number system used. In this chapter, we make use of fixed-point, floating-point, and posit number systems. During the exhaustive design space exploration, continuous error tracking (\circled{3}) is performed to measure the extent of accuracy deviation compared to the IEEE floating-point arithmetic format.

 \begin{figure}
\centering
\includegraphics[bb=2 21 848 194,width=\linewidth,trim={0cm 0.7cm 0cm 0cm},clip]{Stencil_Precise/Tuning_camera.pdf}
\vspace{-0.3cm}
\caption{Overview of application precision exploration. The designer inputs the code with an appropriate precision template. Exhaustive precision exploration is performed for different number systems that include fixed-point arithmetic, floating-point arithmetic, and posit arithmetic. While exploring, error tracking is performed using the 2-norm matrix approach
\label{fig:low_precision/methodology}}
\end{figure}
\vspace{-0.5cm}

 \paragraph{Accuracy:} In our experiments, for precision tuning, we consider the induced 2-norm of a matrix~\cite{normError} as our measure of the accuracy. A matrix norm is a vector norm in a vector space. The induced 2-norm of an \textit{m}$\times$\textit{n}  matrix \textit{A} is the supremum of the ratio between the 2-norm of a vector \textit{Ax} and the 2-norm of \textit{x}, where \textit{x} is an  \textit{n}-dimensional vector. We calculate the relative norm or mean relative error (MRE)  $\epsilon_i$ to indicate how close the predicted value $A_{i}^\prime$ is to the actual value $A_{i}$. MRE provides an unbiased estimate of the error variance between two matrices.
\vspace{-0.3cm}
\begin{align}
 \epsilon_i= \frac{||A_{i}^\prime -A_{i}||_{2}}{||A_{i}||_{2}}
\label{eq:low_precision/2}
\end{align}

\subsection{Evaluated Arbitrary Precision}
% \spaceSubSectionHeading
As an alternative to the currently used IEEE single and double-precision floating-point representation, we explore the precision tolerance of 3D stencil kernels using the following number formats (see Figure~\ref{fig:low_precision/arithemacticTypes}):

1) Fixed-Point Arithmetic: A fixed-point consists of an integer and a fraction part where total width could be any multiple of 2, based on the bit-width of the data path. Compared to the floating-point format, fixed-point numbers simplify the logic by fixing the radix point. 

In an FPGA, the fixed-point format offers a more resource-efficient alternative to the floating-point implementation. This efficiency is because floating-point support often uses more than 100$\times$ as many gates compared to fixed-point support~\cite{finnerty2017reduce}.

2) Dynamic Floating-Point Arithmetic: By lowering the precision of a floating-point format, we could retain the advantages of floating-point arithmetic (e.g., higher dynamic range) with a lower bit-width. Dynamic floating-point arithmetic uses an arbitrary number of bits for the exponent and significand (or mantissa) parts of a floating-point number. 


3) Posit Arithmetic: Posit\cite{gustafson2017beating} borrows most of the components from the IEEE 754 floating-point scheme, such as the exponent and fraction (or mantissa) fields. However, posit has an additional \textit{regime} bit introduced to create a tapered accuracy, which lets small exponents have more accuracy. One
could choose to either represent a large number by assigning more bits to the exponent
field or opt for more decimal precision by having more fraction bits. 

Figure~\ref{fig:low_precision/arithemacticTypes} shows the different datatypes explored in this chapter. While analyzing these types, there are several things to take into account. Firstly, posit can provide the highest dynamic range compared to the other number systems, and fixed-point offers the lowest~\cite{carmichael2018deep}. Additionally, floating-point numbers are susceptible to rounding errors and could lead to an overflow or underflow~\cite{gustafson2017beating}. We determine the precision bit-width through bit accurate simulations for different bit-width configurations. While changing bitwidth, we analyze the trend of the relative error.
\vspace{-0.2cm}
 \begin{figure}
\centering
\includegraphics[bb=1 3 707 241,width=\linewidth]{Stencil_Precise/arithemacticTypes1_camera.pdf}
\caption{Arithmetic types used with widths indicated above each field. IEEE single precision floating-point number is 32-bit where a positive sign bit is represented by a 0 and a negative by 1.  Fixed-point has fixed integer and fraction bits where w (total bits) could be any multiple of 2, based on the bitwidth of the data path. Dynamic floating-point arithmetic uses arbitrary exponent and mantissa bits. A posit number~\cite{gustafson2017beating} is similar to floating-point with additional bits for the regime part. It has $e_s$ exponent bits, but depending upon the data this could be omitted (same is valid for mantissa bits)
\label{fig:low_precision/arithemacticTypes}}
\end{figure}



==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/ref.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{normError}
Anderson, E., et~al.: LAPACK Users' guide, vol.~9. Siam (1999)

\bibitem{carmichael2018deep}
Carmichael, Z., et~al.: {D}eep {P}ositron: A deep neural network using the
  posit number system. arXiv preprint arXiv:1812.01762  (2018)

\bibitem{chi2018soda}
Chi, Y., Cong, J., Wei, P., Zhou, P.: Soda: stencil with optimized dataflow
  architecture. In: 2018 IEEE/ACM International Conference on Computer-Aided
  Design (ICCAD). pp.~1--8. IEEE (2018)

\bibitem{datta2008stencil}
Datta, K., et~al.: Stencil computation optimization and auto-tuning on
  state-of-the-art multicore architectures. In: Proceedings of the 2008
  ACM/IEEE conference on Supercomputing. p.~4. IEEE Press (2008)

\bibitem{diamantopoulos2018ectalk}
Diamantopoulos, D., Giefers, H., Hagleitner, C.: ec{TALK}: Energy efficient
  coherent transprecision accelerators—the bidirectional long short-term
  memory neural network case. In: 2018 IEEE Symposium in Low-Power and
  High-Speed Chips (COOL CHIPS). pp.~1--3. IEEE (2018)

\bibitem{doms1999nonhydrostatic}
Doms, G., Sch{\"a}ttler, U.: The nonhydrostatic limited-area model {LM}
  (lokal-model) of the {DWD. P}art {I: S}cientific documentation. DWD, GB
  Forschung und Entwicklung  (1999)

\bibitem{de2018designing}
de~Fine~Licht, J., Blott, M., Hoefler, T.: Designing scalable FPGA
  architectures using high-level synthesis. ACM SIGPLAN Notices
  \textbf{53}(1),  403--404 (2018)

\bibitem{finnerty2017reduce}
Finnerty, A., Ratigner, H.: Reduce power and cost by converting from floating
  point to fixed point. In: WP491 (v1. 0) (2017)

\bibitem{gustafson2017beating}
Gustafson, J.L., Yonemoto, I.T.: Beating floating point at its own game: Posit
  arithmetic. Supercomputing Frontiers and Innovations  \textbf{4}(2),  71--86
  (2017)

\bibitem{gysi2015modesto}
Gysi, T., Grosser, T., Hoefler, T.: Modesto: Data-centric analytic optimization
  of complex stencil programs on heterogeneous architectures. In: Proceedings
  of the 29th ACM on International Conference on Supercomputing. pp. 177--186.
  ACM (2015)

\bibitem{iwata1989artificial}
Iwata, A., et~al.: An artificial neural network accelerator using general
  purpose 24 bits floating point digital signal processors. In: IJCNN-89.
  vol.~2, pp. l71--175 (1989)

\bibitem{klower2019posits}
Kl{\"o}wer, M., D{\"u}ben, P.D., Palmer, T.N.: {P}osits as an alternative to
  floats for weather and climate models  (2019)

\bibitem{langroudi2018deep}
Langroudi, S.H.F., Pandit, T., Kudithipudi, D.: Deep learning inference on
  embedded devices: Fixed-point vs posit. In: 2018 1st Workshop on Energy
  Efficient Machine Learning and Cognitive Computing for Embedded Applications
  (EMC2). pp. 19--23. IEEE (2018)

\bibitem{nguyen20103}
Nguyen, A., et~al.: 3.5-{D} blocking optimization for stencil computations on
  modern {CPU}s and {GPU}s. In: Proceedings of the 2010 ACM/IEEE International
  Conference for High Performance Computing, Networking, Storage and Analysis.
  pp. 1--13. IEEE Computer Society (2010)

\bibitem{parker2014understanding}
Parker, M.: {U}nderstanding peak floating-point performance claims. Technical
  White Paper WP-012220-1.0  (2014)

\bibitem{sano2014multi}
Sano, K., Hatsuda, Y., Yamamoto, S.: Multi-FPGA accelerator for scalable
  stencil computation with constant memory bandwidth. IEEE Transactions on
  Parallel and Distributed Systems  \textbf{25}(3),  695--705 (2014)

\bibitem{singhReview}
Singh, G., et~al.: A review of near-memory computing architectures:
  {O}pportunities and challenges. In: 2018 21st Euromicro Conference on Digital
  System Design (DSD). pp. 608--617. IEEE (2018)
  
\bibitem{NAPEL}
Singh, G., et~al.: {NAPEL}: Near-Memory Computing Application Performance Prediction via Ensemble Learning. In {\em Proceedings of the 56th Annual Design Automation Conference
  2019}, DAC '19, pages 27:1--27:6, New York, NY, USA, 2019. ACM.

\bibitem{7582502}
{Waidyasooriya}, H.M., et~al.: {O}pen{CL-B}ased {FPGA-P}latform for {S}tencil
  {C}omputation and {I}ts {O}ptimization {M}ethodology. IEEE Transactions on
  Parallel and Distributed Systems  \textbf{28}(5),  1390--1402 (May 2017)

\bibitem{stencilOnPOWER8}
Xu, J., et~al.: {P}erformance {T}uning and {A}nalysis for {S}tencil-{B}ased
  {A}pplications on {POWER}8 {P}rocessor. ACM Transactions on Architecture and
  Code Optimization (TACO)  \textbf{15}(4), ~41 (2018)

\end{thebibliography}

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/relatedWork.tex <==
\section{Related Work}
\label{sec:low_precision/relatedWork}
Floating-point representation is the most widely supported data type by current hardware devices. Recently, in many application domains, there has been a significant amount of research to explore error resilience across the complete stack of computer architecture from application to device physics. \fc{A large body of literature~\cite{iwata1989artificial,menard2002methodology,de2017understanding,higham2019simulating,esmaeilzadeh2012neural,menard2002automatic,ha2021precision} has analyzed the benefits of using lower precision fixed-point computation compared to floating-point for different application domains.} With the emergence of the posit number system~\cite{gustafson2017beating}, research into lower precision with these alternate number systems is regaining attention. In neural-networks, Langroudi~\etal~\cite{langroudi2018deep} demonstrate a minimum accuracy degradation by using a 7-bit posit format. In another study,  Kl{\"o}wer~\etal~\cite{klower2019posits} show the applicability of posit in weather modeling. However, they used a different weather prediction model than COSMO, which uses different numerical solvers for predicting weather.

High-performance implementations of stencils on modern processors usually use the IEEE single-precision or double-precision floating-point data types. There have been various efforts to improve these kernels for different architectures using various software-based optimization techniques. Datta~\etal~\cite{datta2008stencil} optimized the 2D and 3D stencil for multicore architectures using several hardware adherent optimizations. Similarly, Nguyen~\etal~\cite{nguyen20103} worked on algorithm optimization for CPU and GPU-based systems. Gysi~\etal~\cite{gysi2015modesto} provided guidelines for optimizing complex kernels for CPU--GPU systems using analytic models. \ou{ Gan~\etal~\cite{gan2013accelerating} use a mixed-precision approach for 13-point shallow water equation (SWE) stencils. The authors use fixed-point representation for variables that require a lower precision, while floating point precision for other variables.}  However, to the best of our knowledge, this thesis is the first to study the precision tolerance for scientific 3D stencil kernels, including a compound weather prediction stencil kernel, for a wide range of number systems, i.e., fixed-point arithmetic, floating-point arithmetic, and posit arithmetic.

% \spaceSectionEnd

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/system.tex <==
\begin{table}
    \caption{System configuration for the host CPU system.}
    \label{tab:low_precision/systemparameters}
    \centering
    \resizebox{\textwidth}{!}{% use resizebox with textwidth
    \begin{tabular}{c|c|c|c|c}
    \toprule
     \textbf{Architecture} & \textbf{Physical Cores} &\textbf{Frequency}& \textbf{On-chip Memory (Per Core)} & \textbf{Off-chip Memory}\\
     \hline
     IBM Power9& 16-cores/socket; (SMT4)  & Min: 2.3GHz & L1-cache: 32KiB & DDR4: \\
      & &Max: 3.8GHz & L2-cache: 256KiB & 16x32GiB RDIMM\\
      &  & & L3-cache: 10MiB  & 2666MHz\\
     
     \bottomrule
    
    \end{tabular}}
\end{table}

==> PhD_Thesis_Updated_arxiv (1)/Stencil_Precise/system_gagan.tex <==


  \vspace{0.2cm}
\begin{table}[h]
  \caption{System parameters and hardware configuration for the CPU and the FPGA board}
  \vspace{-0.4cm}
    \label{tab:low_precision/systemparameters}
   
      \begin{center}
      \footnotesize
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{|l@{\hspace{0.1\tabcolsep}}|p{7cm}|}

\hline
\textbf{Host CPU} 

 & 16-core IBM POWER9 AC922 \\&@3.2 GHz, 4\gagann{-way} SMT\\
 \hline
 \textbf{Cache-Hierarchy}&32 KiB L1-I/D, 256 KiB L2, 10 MiB L3 \\
 \hline
 \textbf{System Memory}&16x32GiB RDIMM DDR4 2666 MHz \\
\hline
 \begin{tabular}[c]{@{}l@{}}
 \textbf{DDR4-based} \\\textbf{FPGA Board} \end{tabular}  & \begin{tabular}[c]{@{}l@{}}
 Alpha Data
ADM-PCIE-9V3\\
 Xilinx Virtex Ultrascale+ XCVU3P-2\\
 8GiB (DDR4) with PCIe Gen4 x8
  \end{tabular}\\

 
 
% \hline
% \textbf{FPGA Family}  & \\
% \hline
% \textbf{Device Memory}  & 8GiB (DDR4)\\
% \hline
% \textbf{CAPI Interface}  & PCIe Gen4 x8\\



%NVM bandwidth & bw\textsubscript{ext} & 6 GB/s\\

\hline

\end{tabular}
}
  \end{center}
 \end{table}



==> PhD_Thesis_Updated_arxiv (1)/abstract.tex <==
% \section*{Designing, modeling, and optimizing \\data-intensive computing systems} 
% \subsection*{Abstract}
\section*{Abstract}
% Characterization of real DRAM devices has enabled findings in DRAM device properties, which has led to proposals that significantly improve overall system performance by reducing DRAM access latency and power consumption. In addition to improving system performance, a deeper understanding of DRAM technology via characterization can also improve device reliability and security. These can be seen with the recent discoveries of 1) DRAM-based true random number generators (TRNGs), a method for generating true random numbers using DRAM devices which can be used in many applications, 2) DRAM-based physical unclonable functions (PUFs), a method for generating unique device-dependent keys for identification and authentication, and 3) the RowHammer vulnerability, a phenomenon where repeatedly accessing a DRAM row can cause failures in unaccessed neighboring DRAM rows. 
 
% To advance DRAM-based discoveries and mechanisms, this dissertation rigorously characterizes many modern commodity DRAM devices and shows that by exploiting DRAM access timing margins within manufacturer-recommended DRAM timing specifications, we can significantly improve system performance, reduce power consumption, and improve device reliability and security. First, we characterize DRAM timing parameter margins and find that certain regions of DRAM can be accessed faster than other regions due to DRAM cell process manufacturing variation. We exploit this by enabling variable access times depending on the DRAM cells being accessed, which not only improves overall system performance, but also decreases power consumption. Second, we find that we can uniquely identify DRAM devices by the locations of failures that result when we access DRAM with timing parameters reduced below specification values. Because we induce these failures with DRAM accesses, we can generate these unique identifiers significantly more quickly than prior work. Third, we propose a random number generator that is based on our observation that timing failures in certain DRAM cells are randomly induced and can thus be repeatedly polled to very quickly generate true random values. Finally, we characterize the RowHammer security vulnerability on a wide range of modern DRAM chips while violating the DRAM refresh requirement in order to directly characterize the underlying DRAM technology without the interference of refresh commands. We demonstrate with our characterization of real chips, that existing RowHammer mitigation mechanisms \jky{either} are not scalable or suffer from prohibitively large performance overheads in projected future devices and it is critical to research more effective solutions to RowHammer. Overall, our studies build a new understanding of modern DRAM devices to improve computing system performance, reliability and security all at the same time. 

% Current computing systems are compute-centric where all computation takes place in the compute units while the memory units are
% passive components. As a result, modern workloads spend a large fraction of execution time and energy on moving data between the memory units and the compute units. Since the application demand for memory continues to grow, the traditional compute-centric approach of moving stored data to the CPU for computation has become a major system bottleneck. Moreover, the end of Dennard scaling and increasing influence of \textit{dark silicon} has made current systems inadequate at providing optimum performance. This calls for new intelligent architectures that can effectively handle data. Therefore, while designing modern systems we need to follow two key guidelines: (1) \textit{data-centric}: improve performance by minimizing the data movement overhead through hardware specialization;  and (2) \textit{data-driven}: take advantage of the vast amount of data to make decisions, which are based on inherent data characteristics.

% %%%%%%%%%%%%%%%%%VERSION WITH DATACENTRIC+DATA DRIVEN#######################3
% %We are witnessing an enormous amount of data being generated across multiple application domains. %such as weather forecasting, radio astronomy, bioinformatics, and material science. 
% The cost of moving data between the memory units and the compute units is a major contributor to the execution time and energy consumption of modern workloads in computing systems. At the same time, we are witnessing an enormous amount of data being generated across multiple application domains. 
% % Currently, to process these workloads, we follow a compute-centric approach where the data is moved from the memory system to the compute units for processing.  As a result, applications spend a large fraction of execution time and energy on data movement. 
% Moreover, the end of Dennard scaling and increasing influence of \textit{dark silicon} has made our current systems inadequate at providing optimum performance. This inefficiency calls for a redesign of our current architectures to effectively handle this enormous amount of data. These trends suggest opportunities for a paradigm shift to more effectively handle the data.  %while simultaneously exploiting the inherent characteristics of the available data. 
% Therefore, we need to follow two fundamental principles: (1) \textit{data-centric}: improve performance by minimizing the data movement overhead through hardware specialization;  and (2) \textit{data-driven}: take advantage of the vast amount of data by exploiting inherent data characteristics. As a step towards modern architectures, this dissertation contributes to both data-centric and data-driven-based mechanisms.

% First, we design NERO, a data-centric accelerator for a real-world weather prediction application. NERO overcomes the memory bottleneck of weather prediction stencil kernels by exploiting near-memory computation capability on specialized field-programmable gate array (FPGA) accelerators with high-bandwidth memory (HBM) that are attached to the host CPU. Second, we explore the applicability of different number formats and exhaustively search for the appropriate bit-width for complex stencil kernels to improve performance and energy-efficiency with minimal loss in accuracy. Stencils are one of the most widely used kernels in real-world applications. Based on an exhaustive exploration of a range of number systems, including fixed-point, floating-point, and posit. We provide optimum precision and the corresponding accuracy deviation. Third, we develop a machine learning-based framework to obtain an application-aware optimal fixed-point configuration that can meet the strict resource constraints of an FPGA without exhaustively searching the entire design space. 

%  Fourth, we propose NAPEL, a machine learning-based application performance and energy prediction framework for data-centric architectures. NAPEL uses ensemble learning to build a model that, once trained for a fraction of programs on a number of architecture configurations, can predict the performance and energy consumption of {different} applications. Fifth, we present the first use of {few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications. These machine learning-based mechanisms follow {data-driven} techniques by leveraging inherent characteristics in the data to make fast and accurate performance prediction results.

% Sixth, we propose Sibyl, a  reinforcement learning (RL)-based data-placement technique for hybrid storage systems.  Sibyl is a data-driven technique, which uses RL to develop a data-placement policy agent that decides which data should be stored in what storage device to achieve the best performance while minimizing the migration overhead taking into account the device and the workload characteristics. Our evaluation results show that Sibyl significantly improves a hybrid storage subsystem's performance compared to state-of-the-art data placement techniques. Furthermore, we provide explainability to our agent's decision. 

% % Overall, this dissertation contributes to designing, modeling, and optimizing architectures that handle data well by following both \textit{data-centric} and \textit{data-driven} principles.
% Overall, this thesis provides two key conclusions: (1) hardware acceleration on FPGA+HBM fabric is a promising solution to overcome data movement bottleneck on current multi-core systems; (2) machine-learning assisted techniques can leverage the enormous amount of data to perform efficient decisions or predictions in various aspects of computer architecture. Thus, we conclude that the mechanisms proposed by this dissertation provide promising solutions to handle data well by following both \textit{data-centric} and \textit{data-driven} principles. 
% We hope that the proposed architectural techniques and detailed experimental data presented in this dissertation will enable the development of other new mechanisms to improve the performance and energy efficiency of future computing systems. 

% % One such immediate implication is a paradigm shift from compute-centric to a data-centric approach. Processing right at the “home” of data to completely diminish data movement is referred to as \textit{Near-Memory Computing} (NMC). Thus, NMC architectures can save valuable bandwidth on the memory channel as well as reduce system energy consumption.
% % \\
% % \\\noindent For mainstream adoption of NMC a lot of research needs to be done in exploring the huge architectural design space for which the lack of evaluation methodologies needs to be addressed. This proposal aims to address this need by means of performance models and tools that abstract away low-level details of the workings of computing systems, but still provide reasonable performance estimates on modern near memory compute systems. Furthermore, explore the principle of near memory computing in heterogeneous memories and obtain a heterogeneous NMC solution which would be evaluated and implemented.


%%%%%%%%%%%%%%%%%VERSION WITH DATACENTRIC AND SUBSET DATA DRIVEN#######################3
%We are witnessing an enormous amount of data being generated across multiple application domains. %such as weather forecasting, radio astronomy, bioinformatics, and material science. 
The cost of moving data between the memory units and the compute units is a major contributor to the execution time and energy consumption of modern workloads in computing systems. At the same time, we are witnessing an enormous amount of data being generated across multiple application domains.  %The technological gap between the memory and the logic scaling has become a significant performance and energy bottleneck.   
Moreover, the end of Dennard scaling, the slowing of Moore's law, and the emergence of dark silicon limit the attainable performance on current computing systems. 
% Currently, to process these workloads, we follow a compute-centric approach where the data is moved from the memory system to the compute units for processing.  As a result, applications spend a large fraction of execution time and energy on data movement. 
% This inefficiency calls for a redesign of our current architectures to effectively handle this enormous amount of data. 
These trends suggest a need for a paradigm shift towards a \emph{data-centric} approach where computation is performed close to where the data resides. This approach allows us to overcome our current systems' performance and energy limitations by minimizing the \emph{data movement overhead} \ggthesis{by ensuring that data does not overwhelm system components.} Further, a {data-centric} approach can enable a \emph{data-driven} view where we take advantage of vast amounts of available data to improve architectural decisions. Our current systems are designed to follow rigid and simple policies that lack adaptability. Therefore, current system policies fail to %do not optimize or adapt themselves with the change in data. Due to the lack of adaptability, a rigidly-design approach fails to 
provide robust improvement across varying workloads and system conditions.
%Therefore, we need to follow two fundamental principles: (1) \textit{data-centric}: improve performance by minimizing the data movement overhead through hardware specialization;  and (2) \textit{data-driven}: take advantage of the vast amount of data by exploiting inherent data characteristics. 

As a step towards modern computing architectures, this dissertation contributes to various aspects of the \emph{data-centric} approach and further proposes several \emph{data-driven} mechanisms.
% As a step towards modern architectures, this dissertation contributes to various aspects of the \textit{data-centric} approach and provides a \textit{data-driven} mechanism that shows the importance of leveraging the inherent data semantics to improve architectural decisions.

First, we design NERO, a data-centric accelerator for a real-world weather prediction application. NERO overcomes the memory bottleneck of weather prediction stencil kernels by exploiting near-memory computation capability on specialized field-programmable gate array (FPGA) accelerators with high-bandwidth memory (HBM) that are attached  through a cache-coherent interconnect to a host CPU system. Second, we explore the applicability of different number formats, including fixed-point, floating-point, and posit, for memory-bound stencil kernels. %Stencils are one of the most widely used kernels in real-world applications. 
We search for the appropriate bit-width that reduces the memory footprint and improves the performance and energy efficiency with minimal loss in the accuracy. %We provide the optimum precision and the corresponding accuracy deviation for these workloads based on an exhaustive exploration of a range of number systems, including fixed-point, floating-point, and posit. 
%=============================================
% Third, we develop PreciseFPGA, an automated framework to obtain an application-aware Pareto-optimal fixed-point configuration without exhaustively searching the entire design space. Our framework comprehends the resource mapping constraints of an FPGA. 
%=============================================

Third, we propose NAPEL, an ML-based application performance and energy prediction framework for data-centric architectures. NAPEL uses ensemble learning to build a model that, once trained for a fraction of programs, %on a number of architecture configurations, 
 can predict the performance and energy consumption of {different} applications. Fourth, we present LEAPER, the first use of {few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications. LEAPER provides the ability to reuse a prediction model  built on an {{inexpensive}} low-end local system to a new, unknown, high-end FPGA-based system. %These machine learning-based mechanisms follow {data-driven} techniques by leveraging inherent characteristics in the data to make fast and accurate performance prediction results.

Fifth, we propose Sibyl, the first reinforcement learning-based mechanism for data placement in hybrid storage systems.  Sibyl is a data-driven mechanism. It observes different features of the running workload as well as the storage devices to make system-aware data placement decisions. For every decision it makes, Sibyl receives a reward from the system that it uses to evaluate the long-term performance impact of its decision and continuously optimizes its data placement policy online. Our extensive real-system evaluation demonstrates that Sibyl provides adaptivity and extensibility by continuously learning from and autonomously adapting to the workload characteristics, storage configuration and device characteristics, and system-level feedback to maximize the overall long-term performance of a hybrid storage system. We interpret Sibyl's policy through our explainability analysis and conclude that Sibyl provides an effective and robust approach to data placement in current and future hybrid storage systems. 



% , which uses RL to develop a data-placement policy agent. The data-placement agent decides which data should be stored in what storage device to achieve the best performance while minimizing the migration overhead taking into account the device and the workload characteristics. Our evaluation results show that Sibyl significantly improves a hybrid storage subsystem's performance compared to state-of-the-art data placement techniques. We also provide explainability to our agent's decision. 

% Overall, this dissertation contributes to designing, modeling, and optimizing architectures that handle data well by following both \textit{data-centric} and \textit{data-driven} principles.
Overall, this thesis provides two key conclusions: (1) hardware acceleration on an FPGA+HBM fabric is a promising solution to overcome the data movement bottleneck of our current computing systems; (2) data should drive system and design decisions by leveraging inherent data characteristics to make our computing systems more efficient. %self-optimizing mechanisms can leverage the enormous amount of data to perform efficient architectural decisions or predictions in various aspects of computer architecture. 
Thus, we conclude that the mechanisms proposed by this dissertation provide promising solutions to handle data well by following a \emph{data-centric} approach and further demonstrates the importance of leveraging data to devise \emph{data-driven} policies.

We hope that the proposed architectural techniques and detailed experimental results presented in this dissertation will enable the development of energy-efficient data-intensive computing systems and drive the exploration of new mechanisms to improve the performance and energy efficiency of future computing systems. 

% One such immediate implication is a paradigm shift from compute-centric to a data-centric approach. Processing right at the “home” of data to completely diminish data movement is referred to as \textit{Near-Memory Computing} (NMC). Thus, NMC architectures can save valuable bandwidth on the memory channel as well as reduce system energy consumption.
% \\
% \\\noindent For mainstream adoption of NMC a lot of research needs to be done in exploring the huge architectural design space for which the lack of evaluation methodologies needs to be addressed. This proposal aims to address this need by means of performance models and tools that abstract away low-level details of the workings of computing systems, but still provide reasonable performance estimates on modern near memory compute systems. Furthermore, explore the principle of near memory computing in heterogeneous memories and obtain a heterogeneous NMC solution which would be evaluated and implemented.

==> PhD_Thesis_Updated_arxiv (1)/ack.tex <==
\section*{Acknowledgements}
% \lenka{I really love the way you introduced it, id just suggest different formulation - e.g. "than delivering thesis" or "than just a thesis" but in any, the first paragraph is badass, it is so beautiful, you are the best <3 } 
At the end of this journey, I believe Ph.D. is more than just a thesis. It is who you have become. I would like to reflect on the many people who have supported and helped me to become who I am today. Certainly, I would not have gotten this far without the support of many excellent people around me.

First and foremost, I express my gratitude to my promotor, Dr. Henk Corporaal, for giving me the opportunity and for his unwavering support and guidance throughout my Ph.D. Henk has been more than a supervisor and always guided me on any matter I needed his help. Despite his busy schedule, he always made time to discuss and brainstorm about any idea and always provided rigorous feedback. I would like to thank my co-promotor, Dr. Sander Stuijk, for his supervision and guidance. Sander was instrumental in my Ph.D. as he always believed in my skills and helped me to set ambitious but realistic goals.  Moreover, a special mention for helping with incessant administrative issues.  

My time at ETH with the SAFARI research group took my research career to the next level. I am deeply indebted to Dr. Onur Mutlu for his invaluable scientific discussions, feedback, and support. His passion for Computer Architecture intrigued me to pursue  research in this domain. I am grateful to have experienced the rigor, thought, and care Onur puts into every scientific task. \gthesis{Further, he always makes sure that extraneous issues do not constraint us in any way, so we can focus on high-impact research and realize our true potential.} I cannot begin without expressing my gratitude to Dr. Juan G{\'o}mez-Luna, who provided me with the encouragement and patience throughout my Ph.D. He always believed in my abilities and motivated me to keep going. %I am immensely grateful to have found many great friends in the SAFARI research group. 
I also thank Jisung Park, Nastaran Hajinazar, and Rakesh Nadig for their discussions, feedback, collaboration, and support. I would like to recognize the help I received from Kaan Kara,  Geraldo Oliviera, Jeremie Kim, Damla Senol Cali, Mohammed Alser, Rahul Bera, Konstantinos Kanellopoulas, Abdullah Giray Ya\u{g}l{\i}k\c{c}{\i}, Can Firtina, Taha Shahroodi, Tracy Ewen, and Christian Rossi.

During my secondment at IBM Research, I had invaluable experiences that have shaped me both personally and professionally.  I am incredibly grateful to Dionysios Diamantopoulos. I spent more time in his office than in mine discussing and brainstorming while using his coffee machine.  I would like to extend my sincere thanks to Christoph Hagleitner for the guidance and for providing access to the IBM systems.  I always enjoyed our interactions, both technical and lunch-time. Special thanks to Ronald Luijten for our numerous discussions on weather forecasting and personal guidance. One of the greatest joys of working at IBM is the presence of many talented individuals who I called upon numerous times for their expertise during my research, and thus I would like to express my appreciation to Robert Haas,  Giovanni Mariani, Andreea Anghel, Abu Sebastian, Florian Auernhammer, Gero Dittmann,  Raphael Polig, Jan van Lunteren,  Teodoro Laino, Miguel Prada, Martino Dazzi, Irem Boybat, Iason Giannopoulos, Mitra Purandare, Francois Abel, Beat Weiss, Pier Andrea Francese, Celestine D\"unner, Burkhard Ringlein, Judith Blanc, Lilli-Marie Pavka, and numerous other IBMers and interns for many interesting discussions and assistance with my work. I also had the great pleasure of working with Lorenzo Chelini, Ahsan Jawed Awan (Ericsson Research), and Stefano Corda.

I would like to thank the members of the doctoral committee for agreeing to participate in my defense during such difficult times, as well as for taking the time to read my drafts and provide constructive feedback, which helped improve the quality of this thesis.

I am deeply indebted to my family, who has done everything in their power to support me in both my academic and personal life. My father, Harinder Singh's steadfastness and humbleness, my mother Ravinder Kaur's kindness and encouragement, and my sister Jasmeet Kaur's unique perspective and guidance have helped me focus on what is important. Their support underlies everything that I do, and I am grateful to have such a wonderful family.

  I am grateful to Jan and Evelyn for making my time in the Netherlands memorable. Last but not least, I cannot begin to express my gratitude to Lenka, Ilde,  Mladen,  Savvas, Victor, Luc, Mark, Barry, Amr, Marja,  Kanishkan, Sajid, Alessandro, Sayandip, Paul, Hamideh, Mojtaba, Kamlesh, Umar, Roel, and other friends and colleagues from Eindhoven who always invited me to every event and never made me feel that I am away from them. I appreciate their continued  motivation and support throughout my stay away from home in the Netherlands and Switzerland.\\

 \begin{flushright}
\noindent \textbf{Gagandeep Singh}\\
 \textit{Z\"urich, Switzerland}\\
\textit{March 12, 2021}
\end{flushright}
% I have many people to thank for their support during my PhD journey. First and
% foremost, I am extremely grateful to my advisor, Onur Mutlu, who has generously
% mentored and guided me since my sophomore year of college. His passion for
% Computer Architecture and his research initially caught my interest during a
% seminar course lecture, and his exemplary feedback, encouragement, and ongoing
% support helped me to adopt his passion into my own work as well. I am grateful
% to have experienced, first-hand, the thought and care Onur puts into both his
% teaching and his research, and I have learned greatly through many iterations
% of paper submissions, conference talks, course exams, and lectures with him.
% Onur has also provided countless opportunities for collaboration within the
% SAFARI research group and industrial collaborators, which provided me with many
% new experiences during my exciting and unique PhD experience, as well as made
% this thesis possible. 

% I am grateful to the members of my PhD committee, James Hoe, Derek Chiou, and
% Saugata Ghose, for their valuable feedback and stimulating discussions. 

% I am immensely grateful to have found many great friends in the SAFARI research
% group. I could not have done it without Minesh Patel, a great friend that truly
% made my PhD experience enjoyable. He brought an immense wealth of knowledge,
% enforced high research standards, and fostered my enjoyment of hard liquors.  I
% am very thankful for Can Firtina, an endless source of entertainment,
% unforgettable experiences, and shelter. I am grateful for Hasan Hassan who on
% many occasions kept me company in the office late into the night. I am thankful
% for Damla Senol Cali, my first friend in SAFARI with whom I had to navigate the
% new field of bioinformatics and learn Onur's research process. I also want to
% thank Giray Yaglikci for his friendship and company on hikes around the world. 

% I would like to acknowledge all past and current members of our research group
% for being both great friends and colleagues. I want to especially thank Yoongu
% Kim, Hongyi Xin, Donghyuk Lee, Rachata Ausavarungnirun, Yixin Luo, Saugata
% Ghose, Vivek Seshadri, and Kevin Chang, for their mentorshop during my
% formative years in SAFARI. I thank Can Firtina, Giray Yaglikci, Nastaran
% Hajinazar, Geraldo De Oliveira, and Ivan Fernandez-Vega for gracefully
% welcoming my invasion of their office space and providing a fun working
% environment. I also thank all others for their discussions, feedback,
% collaboration, and support: Arash Tavakkol, Jawad Haj-Yahya, Mohammed Alser,
% Roknoddin Azizibarzoki, Nika Mansourighiasi, Lois Orosa, Juan Gomez Luna,
% Amirali Boroumand, Jisung Park, Nandita Vijaykumar, Ivan Puddu, Ataberk Olgun,
% Nisa Bostanci, Rahul Bera, Konstantinos Kanellopoulos, and Taha Shahroodi. 

% I am especially grateful to have met and worked with Tyler Huberty, Stephan
% Meier, Jared Zerbe, Jung-Sik Kim, Heonjae Ha, Seung Lee, Gihong Kim, Taehyun
% Kim, Augustin Hong, Can Alkan, and countless others during my PhD journey. They
% have all provided great insight, mentorship, and support.  

% I would also like to thank my internship mentors, Stefan Saroiu and Alec
% Wolman, during my time at Microsoft Research, who provided me with a
% stimulating environment and an industrial perspective on system security. I
% sincerely thank Microsoft for this opportunity.

% I would like to thank the National Science Foundation (grants 1212962 and
% 1320531), the National Institutes of Health (grant HG006004) and SAFARI
% Research Group's industrial partners for respectively the financial support and
% the gift funding they have provided that have contributed to works during my
% PhD.

% To my many friends and family, your support and encouragement throughout my
% journey were worth more than I can express on paper. I want to particularly
% thank Jimmy Lee, Ho-Gyun Choi, Noelle Jung, Stephanie Chen, Justine Kim, and
% Matt Yin for always being there. 

% Finally, I want to thank my parents Hyong and Anita for their unwavering
% support, encouragement, and love.  




==> PhD_Thesis_Updated_arxiv (1)/biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
% \begin{singlespace}
% \small
% \bibliography{refs}
% \bibliographystyle{plain}
% %% Get rid of 'no \citation' error in certain compilers. Alin Tomescu (2015).
% %\nocite{*} %% 
% \end{singlespace}


==> PhD_Thesis_Updated_arxiv (1)/ch-Backg.tex <==
\chapter{Near-Memory Computing}
\label{chapter:background}
\chapternote{The content of this chapter was published as \emph{``Near-Memory Computing: Past, Present, and Future''} in MICPRO 2019.}

% The conventional approach of moving data to the CPU for computation has become a significant performance bottleneck for emerging scale-out data-intensive applications due to their limited data reuse. At the same time, the advancement in 3D integration technologies has made the decade-old concept of coupling compute units close to the memory --- called near-memory computing (NMC) --- more viable. Processing right at the ``home'' of data can significantly diminish the data movement problem of data-intensive applications.

% In this paper, we survey the prior art on NMC across various dimensions (architecture, applications, tools, etc.) and identify the key challenges and open issues with future research directions. We also provide a glimpse of our approach to near-memory computing that includes i) NMC specific microarchitecture independent application characterization ii) a compiler framework to offload the NMC kernels on our target NMC platform and iii) an analytical model to evaluate the potential of NMC. 


% \input{NMC_review/sections/introduction.tex}

\input{NMC_review/sections/background.tex}


\input{NMC_review/sections/classification.tex}






\input{NMC_review/sections/challenges.tex}


% \input{NMC_review/sections/system.tex}


% \input{NMC_review/sections/future.tex}

\input{NMC_review/sections/conclusion.tex}


==> PhD_Thesis_Updated_arxiv (1)/ch-Conclusion.tex <==
\chapter{Conclusions and Future Directions}
\label{chapter:conclusion}


In this dissertation, the goal was twofold. First, overcome the data movement bottleneck by following a data-centric approach of bringing processing close to the memory  and ensure that system components are not overwhelmed by data; thus, enabling high-performance in an energy-efficient way. Second, leverage the enormous amount of data to devise computer architecture mechanisms that can assist us in architectural decisions or optimizations. To this end, \dd{the dissertation} presented five contributions to effectively handle and leverage the vast amount of data for future computing systems. Table~\ref{tab:intro/methods_end} shows nine architectural methods that we use across our five contributions. 

\input{table_methods_end}

\noindent \textbf{A data-centric architecture:} In \textbf{Chapter~\ref{chapter:nero}}, we designed NERO, a data-centric accelerator for a real-world weather prediction application. NERO overcomes the memory bottleneck {of weather {prediction} stencil kernels} by {exploiting near-memory {computation} capability on} specialized field-programmable gate array (FPGA) accelerators with high-bandwidth memory (HBM) {that are attached} {to the host CPU}. {Our} experimental results showed that {\nameNERO} outperforms a 16 core POWER9 {system} by $4.2\times$ and $8.3\times$ when running two {different} compound stencil kernels. {\nameNERO} {reduces the energy consumption by} $22\times$ and $29\times$ {for the same two kernels {over the POWER9 system}} {with an energy efficiency of 1.5 GFLOPS/Watt and 17.3 GFLOPS/Watt}. {We concluded that} employing near-memory acceleration solutions for weather prediction {modeling}~{is~promising} {as a means to achieve {both} high performance and {high} energy efficiency}.

\noindent \textbf{Precision tolerance and alternate number system:} In \textbf{Chapter~\ref{chapter:low_precision_stencil}}, we  explored the applicability of different number formats and searched for the appropriate bit-width for complex stencil kernels, which are one of the most widely used scientific kernels. Further, we leveraged the arbitrary fixed-point precision capabilities of an FPGA to demonstrate these kernels' achievable performance on state-of-the-art hardware that includes IBM POWER9 CPU with an FPGA board connected via CAPI interface. Thus, this chapter filled the gap between current hardware capabilities and future systems for stencil-based scientific applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent \textbf{Pareto-optimal low-precision exploration framework:} In \textbf{Appendix~\ref{chapter:precise_fpga}} , we develop an automated framework to obtain an application-aware optimal fixed-point configuration without exhaustively searching the entire design space. Experimental results show that \namePreciseFPGA~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by ${674\times}$ over exhaustive search.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Data-driven alternative to system simulation:} In \textbf{Chapter~\ref{chapter:napel}},  we proposed NAPEL, a machine learning-based application performance and energy prediction framework for data-centric architectures. NAPEL uses ensemble learning to build a model that, once trained for a fraction of programs on a number of architecture configurations, can predict the performance and energy consumption of {different} applications. Our inexpensive performance model can provide, on average, an additional 10$\times$ reduction in performance evaluation time with an error rate lower than 15\% compared to a computationally-intensive state-of-the-art NMC simulator.


\noindent   \textbf{Data-driven modeling of FPGA-based systems:} In \textbf{Chapter~\ref{chapter:leaper}}, we presented LEAPER, the first use of \textit{few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications. Experimental results showed that our approach delivers, on average, 85\% accuracy  {when we use our transferred model for prediction in a cloud environment} with \textit{5-shot learning} and reduces {design-space exploration} time by 10$\times$, from days to {only} a few hours. These machine learning-based mechanisms follow \textit{data-driven} techniques by using the vast amount of data to provide fast and accurate performance prediction results.

\noindent \textbf{Data-driven mechanism for data-placement in hybrid storage systems}: In \textbf{Chapter~\ref{chapter:sibyl}}, we proposed Sibyl, a  reinforcement learning (RL)-based data-placement technique for a hybrid storage system (HSS). Sibyl observes different features \gon{of} the \gon{running workload}  \gon{as well as the}  storage devices to make system-aware data placement decisions. For every decision \gon{it makes}, Sibyl receives a reward from the system that it uses to evaluate the long-term \gon{performance} impact of its decision and continuously optimizes its data placement policy online. Our real system evaluation results show that  %performance-optimized %\jgll{"performance-oriented"? It may not be "optimized", even though the used SSDs are fast. We "optimize" it with Sibyl.} 
 Sibyl \gon{ provides \gonzz{21.6\%/19.9\%} performance improvement in a performance-oriented\gonn{/cost-oriented} HSS configuration %and 23.2\% performance improvement in cost-oriented HSS configuration 
 compared to the best previous data placement technique.} 
Our evaluation using an HSS configuration with three different storage devices shows that Sibyl outperforms \gonn{the state-of-the-art} \gonzz{data placement} %heuristic-based 
policy by 23.9\%-48.2\%\gonn{,} while significantly reducing the system architect's burden in designing a data placement mechanism that can simultaneously incorporate three storage devices. We show that Sibyl  achieves 80\% of the performance of an {oracle} policy that has \gon{complete} knowledge~of~future access patterns while incurring \gon{a \gonn{very modest} storage}  overhead of only \gonzz{124.4} KiB. 
%In \textbf{Chapter~\ref{chapter:sibyl}}, we proposed Sibyl, a  reinforcement learning (RL)-based data-placement technique for hybrid storage systems.  QRator is a {data-driven} technique, which uses RL to develop a data-placement policy agent that decides which data should be stored in what storage device to achieve the best performance while minimizing the migration overhead taking into account the device and the workload characteristics. We demonstrated our approach on two different hybrid storage configurations. \nameQRator~improved performance, on average, by 29.9\%, 49.2\%, and 43.1\% compared to three state-of-the-art data-placement policies, respectively. Furthermore, we provided explainability to our agent’s decision.

We conclude that the mechanisms proposed by this dissertation provide promising solutions to handle data well by following a \textit{data-centric} approach and further demonstrates the importance of leveraging data to devise \textit{data-driven} policies.

% We hope that the proposed architectural techniques and detailed experimental data presented in this dissertation will enable the development of energy-efficient data-intensive computing systems, and drive the exploration of new mechanisms to improve
% the performance and energy efficiency of future computing systems.

\section{Outlook and Future Directions}

Throughout this dissertation, we considered data as a paramount resource and provided various mechanisms to effectively handle and leverage the vast amount of data. We identify topics for future research both in data-centric computing and data-driven optimization techniques.
% Based on our analysis of many existing NMC architectures, we identify the following key
% topics for future research that we regard as essential to unlock the full potential of processing close to memory:

\subsection{Data-Centric Computing}
In data-centric computing, we ensure that our computing systems are not overwhelmed by data. There are two different approaches to enable data-centric computing. First, near-memory computing (\acrshort{nmc})~\cite{nair2015active,teserract,7446059,ahn2015pim,hsieh2016accelerating,tom,ke2020recnmp,gomezluna2021upmem,cali2020genasm,fernandez2020natsa,singh2020nero} adds processing capabilities close to the existing memory architectures. Second, computation-in memory (\acrshort{cim})~\cite{seshadri2013rowclone,chang2016low,rezaei2020nom,gao2019computedram,seshadri2019dram,seshadri2017ambit,li2016pinatubo,computecache,li2017drisa} exploits the memory architecture and intrinsic properties of emerging technologies to perform operations using memory itself. We identify the following key topics for future research that
we regard as essential to unlock the full potential of data-centric computing.

\noindent\textbf{Architecture:} It is unclear which emerging memory technology best supports data-centric computing; for example, much research is going into new 3D stacked DRAM and non-volatile memories such as PCM and ReRAM. The future of these new technologies relies heavily on advancements in endurance, reliability, cost, and density. Moreover, these memories have different memory attributes, such as latency, bandwidth, cost, and energy consumption. We believe a hybrid approach of complementing two different technologies, as we show in Chapter~\ref{chapter:sibyl}, can revolutionize our current systems. Huang~\etal~\cite{qian2015study} evaluate one such architecture that tightly integrates CPU, DRAM, and a flash-based NVM to meet the memory needs of big data applications, i.e., larger capacity, smaller delay, and wider bandwidth. Processing near-heterogeneous memories is a new research topic with high potential (could provide the best of both worlds), and in the future, we expect much interest in this direction. \gthesis{Further, we see a trend towards processing near caches~\cite{computecache,neuralcache2018}, and we expect more works in this direction. The right level of cache where to place the processing unit would be an interesting future direction. }

The interplay of NMC units with the emerging interconnects standards like CXL~\cite{cxlwhitepaper}, CCIX~\cite{ccixwhitepaper}, and CAPI~\cite{openCAPI} could be vital in improving the performance and energy efficiency of big data workloads running on NMC enabled servers. More quantitative exploration is required for interconnecting networks between the near-memory compute units and between the host and near-memory compute systems.  Besides the design of the near-memory computing device itself, the integration of such architectures into the overall computing system and how multiple near-memory computing devices can work together to scale to larger data volumes are critical challenges to solve.

% \begin{itemize}
   
% \item It is unclear which emerging memory technology best supports near-memory architectures; for example, much research is going into new 3D stacked DRAM and non-volatile memories such as PCM, ReRAM, and MRAM. The future of these new technologies relies heavily on advancements in endurance, reliability, cost, and density.

% % \item 3D stacking also needs unique power and thermal solutions, as traditional heat sink technology would not suffice if we want to add more computation close to the memory. Most of the proposed architectures do not take into account the strict power budget of 3D stacked memories, which limits the architecture's practicality.

% \item DRAM and NVM have different memory attributes. A hybrid design can revolutionize our current systems. Huang et al.~\cite{qian2015study} evaluated a 3D heterogeneous storage structure that tightly integrates CPU, DRAM, and a flash-based NVM to meet the memory needs of big data applications, i.e., larger capacity, smaller delay, and wider bandwidth. Processing near heterogeneous memories is a new research topic with high potential (could provide the best of both worlds), and in the future, we expect much interest in this direction.

% \item More quantitative exploration is required for interconnect networks between the near-memory compute units and also between the host and near-memory compute system. The interplay of NMC units with the emerging interconnect standards like GenZ~\cite{genZdram}, CXL~\cite{cxlwhitepaper}, CCIX~\cite{ccixwhitepaper} and OpenCAPI~\cite{stuecheli2018ibm} could be vital in improving the performance and energy efficiency of big data workloads running on NMC enabled servers.
% \end{itemize}

\noindent\textbf{Software:} Most of the evaluated architectures focus on the compute aspect. Few architectures focus on providing coherency and virtual memory support. As highlighted in Section~\ref{sec:nmc_review/challenges}, lack of coherency and virtual memory support makes programming difficult and obstructs the adoption of the NMC paradigm. 
 At the application level, algorithms need to provide code and data co-location for efficient processing. For example, in NMC, algorithms should prevent excessive movement of data between vaults (as in 3D stacked memory, see Figure~\ref{fig:nmc_review/HMCLayout}) and across different memory modules. Whenever it is not possible to avoid an inter-vault data transfer, we should provide light-weight data migration mechanisms. 
 
% \begin{itemize}
% \item Most of the evaluated architectures focus on the compute aspect. Few architectures focus on providing coherency and virtual memory support. As highlighted in Section~\ref{sec:interondpcachevirtual}, lack of coherency and virtual support makes programming difficult and obstructs the adoption of this paradigm. 

% \item At the application level, algorithms need to provide code and data co-location for energy efficient processing. For example, in case of HMC algorithms should avoid excessive movement of data between vaults and across different memory modules. Whenever it is not possible to avoid an inter-vault data transfer, lightweight mechanisms for data migration should be provided.
% \end{itemize}

\noindent\textbf{Tool support and benchmarks:} The field requires a generic set of open-source tools and techniques for these novel systems. Often researchers have to spend a significant amount of time and effort in building the needed simulation environment. Application characterization tools should add support for static and dynamic decision support for offloading processing and data to near-memory systems. NMC-specific metrics are required to assist in the offloading decision to assess whether an application is suitable for these architectures. These tools could provide region-of-interest (or hotspots) in an application that should be offloaded to an NMC system. Besides, a standard benchmark set is missing to gauge different architectural proposals in this domain.

% 
 
\subsection{Data-Driven System Optimization}

We are seeing an enormous amount of data being generated in different applications domains. Rather than discarding the available data, our machines should leverage this data to understand inherent characteristics or patterns to make better architectural decisions or predictions. To this end, machine learning-based approaches provide an attractive tool that can assist our computer architecture in various aspects. In this dissertation, we use this tool for performance and energy prediction to reduce the time for simulation overhead (Chapter~\ref{chapter:napel}), resource and application performance prediction to overcome the disadvantages of the slow FPGA downstream mapping process (Chapter~\ref{chapter:leaper}), effective data-placement (Chapter~\ref{chapter:sibyl}), and perform design space exploration for the fixed-point precision (Appendix~\ref{chapter:precise_fpga}). These mechanisms are likely just the beginning of a paradigm shift in computer architecture design and use.  Below we highlight some aspects of computer architecture where data-driven mechanisms can greatly assist us.

\noindent \textbf{Architecture:} Past works have demonstrated the applicability of using supervised learning-based techniques in hardware such as prefetching~\cite{liao2009machine}, branch prediction~\cite{jimenez2001dynamic}, and cache replacement~\cite{shi2019applying}. However, hardware feasibility is one of the fundamental challenges in the adoption of these techniques. In the future, we need to make these approaches hardware friendly with low cost and area overhead by using techniques such as pruning, quantization, model compression, etc. 

\noindent \textbf{Software:} The operating system is a ripe place to use ML-based approaches as  software-based mechanisms can tolerate higher latency and implementation overhead than latency-critical aspects of computer architecture such as prefetching and cache-replacement. We can apply modern ML techniques, such as deep reinforcement learning and natural language processing, on problems like software caching, task scheduling, power management, virtual memory management, etc. 

\noindent \textbf{Explainability:} Explainability is providing an explanation of the internal mechanisms of a machine learning model that led the model to a certain prediction or decision. The machine learning community has started to look into the explainability to understand these models' inner workings. However, we still use these tools as mere black-box models in the computer architecture community without making them as white-box models. Explainability can lead to certain insights that have been unknown to our current community, and learn from it to develop better human-driven policies. Since implementing ML algorithms in the hardware can be costly, leveraging insights from ML algorithms can help us better optimize our computing systems.\\


We hope that the ideas, analyses, methods, and techniques presented in this dissertation will enable the development of energy-efficient data-intensive computing systems and drive the exploration of new mechanisms to improve the performance and energy efficiency of future computing systems.



% % bibunit to list our publications
% {\bf \large First author}
% \begin{bibunit}[plain]

% \renewcommand\bibname{List of Publications}
% % \makeatletter
% % \renewcommand\@biblabel[1]{}
% % \makeatother
% \def\bibfont{\small}

% %list all the references in the publications bibtex file
% \nocite{*}

% \putbib[mypublication]
% {\bf \large First author}
% \end{bibunit}



% {\bf \large First author}
% \bibliography{mypublication}
% \nocite{*}
% \begin{thebibliography}{100} % 100 is a random guess of the total number of
% %references
% \bibitem{Boney96} Boney, L., Tewfik, A.H., and Hamdy, K.N., ``Digital
% Watermarks for Audio Signals," \emph{Proceedings of the Third IEEE
% International Conference on Multimedia}, pp. 473-480, June 1996.
% \bibitem{MG} Goossens, M., Mittelbach, F., Samarin, \emph{A LaTeX
% Companion}, Addison-Wesley, Reading, MA, 1994.
% \bibitem{HK} Kopka, H., Daly P.W., \emph{A Guide to LaTeX},
% Addison-Wesley, Reading, MA, 1999.
% \bibitem{Pan} Pan, D., ``A Tutorial on MPEG/Audio Compression," \emph{IEEE
% Multimedia}, Vol.2, pp.60-74, Summer 1998.
% \end{thebibliography}
\renewcommand\bibname{Bibliography}
%%%%%%%%%%%%% end %%%%%%%

==> PhD_Thesis_Updated_arxiv (1)/ch-Intro.tex <==
\chapter{Introduction}
\label{chapter:intro}

% The conventional approach of moving data to the CPU for computation has become a significant performance bottleneck for emerging scale-out data-intensive applications due to their limited data reuse. At the same time, the advancement in 3D integration technologies has made the decade-old concept of coupling compute units close to the memory --- called near-memory computing (NMC) --- more viable. Processing right at the ``home'' of data can significantly diminish the data movement problem of data-intensive applications.
A wide range of application domains have emerged with the ubiquity of computing platforms in every aspect of our daily lives. These modern workloads (e.g., machine
learning, graph processing, and bioinformatics) demand high compute capabilities within strict power constraints~\cite{ghose2019processing}. However, today's computing systems are getting constrained by current technological capabilities, making them incapable of delivering the required performance. We highlight three major trends that call for a paradigm shift in the computing system landscape.

\noindent\textbf{(1) The Memory Wall:} Over the years, the improvements in memory access latency have not been able to keep up with the improvements in processor latency, which is referred to as the \emph{memory wall}~\cite{Wulf1995}.
%Over the years, memory technology has not been able to keep up with advancements in processor technology in terms of latency and energy consumption, which is referred to as the \emph{memory wall}~\cite{Wulf1995}. 
Earlier, system architects tried to bridge this gap by introducing multiple levels of the memory hierarchy that can cache data to avoid unnecessary off-chip data movement. Yet, the system remained \emph{compute-centric}, where the data has to move a long distance from the memory subsystem over the power-hungry off-chip data bus through multiple levels of memory hierarchy to the compute units for processing. This compute-centric nature has lead to a fundamental \emph{data movement bottleneck}, which incurs a significant amount of energy and latency overhead in our current computing systems~\cite{mutlu2020modern}. \fc{In addition, for a given application,  there can be a strong mismatch between the nature of the data access patterns and the layout of the data in memory.  %type of memory in which they are stored. 
Such a mismatch leads to limited spatial locality, which causes frequent data movement between the memory subsystem and the processing units.} %However, the limited number of pins on the memory package is not able to meet today's bandwidth demands of multicore processors.

% \noindent\textbf{(2) The Slowdown of Moore's Law:} \gthesis{In 1974, Dennard~\cite{1050511} postulated that the total chip power for a given chip area stayed constant from one process generation to another.} This allowed CPU vendors to raise clock frequencies. However, with the demise of Dennard scaling~\cite{1050511}, we witness  that with every process generation total chip power  does not remain constant due to the leakage effects. This increase in power consumption led to the onset of dark silicon~\cite{6175879}, whereby a large portion of transistors on a chip have to be switched off or run at a lower frequency to avoid the effects of high leakage~\cite{martin2014postdennard}. Therefore, in the Post-Dennard scaling era, the single-core CPU performance has stagnated because of its inability to operate within the given power budget. 

% The continuation of Moore's law allowed more transistors per chip for each transistor node technology generation. This transistor scaling enabled us to have CPUs with multi-core with multiple levels of caches. Over the years, advancements in manufacturing technology have been slowing due to device physics limitations in transistor node scaling. However, the demand for more performance with high energy-efficiency has continued to grow. In the \acrlong{hpc} (\acrshort{hpc}) domain, current scaling issues are limiting HPC systems to realize exascale computers that are needed for modern and future data-intensive workloads~\cite{nair2015active}.


\noindent\textbf{(2) The Slowdown of Moore's Law:} \gthesis{The continuation of Moore's law allowed more transistors per chip for each transistor node technology generation. This transistor scaling enabled us to have CPUs composed of a multi-core architecture with multiple levels of caches. In 1974, Dennard~\cite{1050511} postulated that the total chip power for a given chip area stayed constant from one process generation to another.} This trend allowed CPU vendors to have higher clock frequencies without drastically impacting the overall system power consumption. However, with the demise of Dennard scaling~\cite{1050511}, we witness  that with every process generation, total chip power  does not remain constant due to the leakage effects. \ph{The leakage effects limit the shrinking of gate oxide in a transistor that forces higher voltage than required for Dennard scaling, which in turn increases the power density.} \fc{As a result,  the system-level performance gains are not enough to motivate a further increase in the single-core clock frequency compared to the significant increase in energy consumption.} This increase in power consumption has led to the onset of dark silicon~\cite{6175879} \fc{in servers}, whereby a large portion of transistors on a chip has to be switched off or run at a lower frequency to avoid the effects of high leakage~\cite{martin2014postdennard}. \fc{While in system-on-a-chip (\acrshort{soc})-based designs, specialized heterogeneous cores have emerged to overcome the disadvantages of dark silicon and slowdown of Moore's law~\cite{hardavellas2012rise}, where each core is optimized for a specific task.}   Therefore, in the Post-Dennard scaling era, the single-core CPU performance has stagnated because of its inability to operate within the given power budget. 

Over the years, advancements in manufacturing technology have been slowing due to device physics limitations in transistor node scaling. \fc{On the other hand, the memory scaling is becoming even more challenging~\cite{mutlu2017rowhammer,ghose2018your,frigo2020trrespass}}. However, the demand for performance with high energy-efficiency has continued to grow. In the high-performance computing (\acrshort{hpc}) domain, current scaling issues \fc{and high communication overheads} limit HPC systems to realize exascale computers needed for modern and future data-intensive workloads~\cite{nair2015active}.

Therefore, future architectural innovations are expected to come from optimizations across the entire hardware/software computing stack~\cite{mutlu2020intelligent,mutlu2021intelligent_DATE}.

% \subsection{Data Avalanche and Inefficient Systems}
\noindent\textbf{(3) The Data Avalanche:} At the same time, we are witnessing an enormous amount of data being generated across multiple application domains~\cite{nair2015active} like weather prediction modeling, radio astronomy, bioinformatics, material science, chemistry, health sciences, etc.  In the domain of climate and weather modeling, for example, there is a data avalanche due to large atmospheric simulations~\cite{schar2020kilometer}. Major efforts are currently underway towards refining the resolution grid of climate models that would generate \emph{zettabytes} of data~\cite{schar2020kilometer}. These high-resolution simulations are useful to predict and address events like severe storms. However, the sheer amount of generated data is one of the biggest challenges to overcome. 

The \acrlong{cosmo} (\acrshort{cosmo})~\cite{doms1999nonhydrostatic} %is 
\juang{built} one such weather model %, which was established 
to meet the high-resolution forecasting requirements of weather services. \gthesis{We use COSMO as a major case-study in this thesis.}   The main computational pipeline of COSMO consists of compound stencil kernels that operate on a three-dimensional grid~\cite{gysi2015modesto}. 
The performance of these compound stencil kernels is dominated by memory-bound operations with irregular memory access patterns and low arithmetic intensity that often results in $<$10\% sustained floating-point performance on current CPU-based systems~\cite{chris} that standard CPU-based optimization techniques cannot overcome (see Chapter~\ref{chapter:nero}). 

We find another relevant example in radio astronomy. The first phase of the Square Kilometre Array (SKA) aims to process over 100 terabytes of raw data samples per second, yielding of the order of 300 petabytes of SKA data produced annually~\cite{6898703}. \fc{ Recent biological disciplines such as genomics have also emerged as one of the most data-intensive workloads across all different sciences wherein just a single human genome sequence produces hundreds of gigabytes of raw data. With the rapid advancement in sequencing technology, the data volume in genomics is projected to surpass the data volume in all other application domains~\cite{navarro2019genomics}.}  \\ %The SKA currently is in the design phase with anticipated construction in South Africa and Australia in the first half of the coming decade. 

\emph{{\gthesis{The above trends suggest that} computer architects and system designers need to\linebreak develop novel architectural solutions to overcome the aforementioned major technological challenges and effectively handle the overwhelming amount of data. }}\\

% \todo{write about data driven techniques in modeling and controlling systems}
% \todo{what do I solve in thesis: high level overview (think concentric)}
% \todo{Maybe a section overview}

% \subsection{Slow Evaluation Techniques}


%To quickly access the benefits and shortcoming of these architecture we need new modeling and evaluation techniques. 

% \subsection{Human-driven Rigid Policies}
% While evaluating new architectures, computer architects often run a number of workloads on a multitude of hardware configurations. This leads to huge amounts of data which researchers often study in a limited fashion on ad hoc
% basis.  we might be able to see the
% true potential of that data and its ability to help us discover new findings.}

% Further, while evaluating new architectures, computer architects often run a number of workloads on a multitude of hardware configurations. This leads to huge amounts of data which researchers often study in a limited fashion on ad hoc
% basis.  we might be able to see the
% true potential of that data and its ability to help us discover new findings.
% These radio-astronomy applications usually exhibit massive data parallelism and low operational intensity with a limited locality. On traditional systems, these applications cause frequent data movement between the memory subsystem and the processor that has a severe impact on performance and energy efficiency. 


% \begin{figure}[!hb]
% \centering
% \includegraphics[width=0.6\linewidth]{NMC_review/img/NMCtaxonomy_final.pdf}
% \caption{Processing options in the memory hierarchy highlighting the conventional compute-centric and the modern data-centric approach
% \label{fig:taxonomy}}
% \end{figure}


% Figure~\ref{fig:taxonomy} shows a high-level view of our classification that is based on the level in the memory hierarchy and further split into the type of compute implementation (programmable, fixed-function, or reconfigurable). Conceptually the approach  of near-memory computing can be applied to any level or type of memory to improve the overall system performance. In our taxonomy, we do not include magnetic disk-based systems as they can no longer offer timely response due to the high access latency and a high failure rate of disks~\cite{7097722}. Nevertheless, there have been research efforts towards providing processing capabilities in the disk. However, it was not adopted widely by the industry due to the marginal performance improvement that could not justify the associated cost~\cite{Keeton:1998:CID:290593.290602,Riedel:1998:ASL:645924.671345}. Instead, we include emerging non-volatile memories termed as storage-class memories (SCM)~\cite{7151782} which are trying to fill the latency gap between DRAMs and disks. Building upon similar efforts~\cite{siegl2016data, ghose2018enabling}, we make the following contributions:

% \input{NMC_review/sections/introduction}
This chapter serves as an introduction to this dissertation. The chapter is structured as follows. Section~\ref{sec:intro/problem} highlights the two guiding principles that we follow in this dissertation to  overcome our current system challenges. Based on these guiding principles, we provide the thesis statement. Section~\ref{sec:intro/overview} describes our approach to solve the thesis statement, while Section~\ref{sec:intro/contributions} lists the contributions of this dissertation. Finally, Section~\ref{sec:intro/outline} provides the dissertation outline.

\section{Problem and Thesis Statement}
\label{sec:intro/problem}

\gthesis{Future architectural innovations are expected to come from optimizations across the entire hardware/software computing stack~\cite{mutlu2020intelligent}. We highlight two guiding principles that can be applied in \dd{complementary} aspects of computer architecture to overcome the current system challenges and improve the overall performance: (1) \emph{data-centric \dd{computing}},  where we bring processing closer to the memory and use different techniques to reduce the data movement bottleneck (such as hardware specialization, data quantization, and  domain specific-memory hierarchies); (2) \emph{data-driven \dd{system optimization}}, where we exploit the available data to perform architectural decisions or predictions. }%In Section~\ref{sec:nmc_review/challenges}, we highlight a challenges that NMC architectures needs to address before it can be established as a de facto solution for modern data-intensive workloads.}
\subsection{Data-Centric \dd{Computing}}
% \subsection{Data-Centric Hardware Specialization}
\label{subsection:intro/data_centric}
Today's memory hierarchy usually consists of multiple levels of cache, the main memory, and the storage. The traditional approach is to move data up to caches from the storage and then process it. Figure~\ref{fig:nmc_review_allsystems} depicts the system evolution based on the information referenced by a program during execution, which is referred to as a working set~\cite{7092668}. Prior systems were based on a \emph{compute-centric} approach where data is moved to the core for processing (Figure 1 (a)-(c)). In contrast, the \emph{data-centric} approach aims at processing close to where the data resides. This approach couples compute units close to the data and seek to minimize the expensive data movement. The system ensures that data does not overwhelm its components. 

As shown in Figure 1 (d-e), near-memory computing (\acrshort{nmc})~\cite{nair2015active,teserract,7446059,ahn2015pim,hsieh2016accelerating,tom,ke2020recnmp,gomezluna2021upmem,cali2020genasm,fernandez2020natsa,singh2020nero} and computation-in memory (\acrshort{cim})~\cite{seshadri2013rowclone,chang2016low,simon2020blade,rezaei2020nom,gao2019computedram,seshadri2019dram,seshadri2017ambit,li2016pinatubo,computecache,li2017drisa} are two data-centric paradigms.  In near-memory computing (Figure 1 (d)), we place the processing cores closer to the memory units. On the other hand, the computation-in-memory (Figure 1 (e)) paradigm is more disruptive as it aims at reducing data movement completely by using memories with \ggthesis{built-in} compute capability (e.g., resistive random-access memory (ReRAM) and  phase-change memory (PCM)). Processing right at the ``home'' of data can significantly diminish the data movement problem of data-intensive applications. \gthesis{Thus, data-centric architectures have the potential to overcome our current data movement bottleneck.} 

\begin{figure*}[h]
\centering
\includegraphics[width=1\textwidth]{NMC_review/img/allsystems_final_update.pdf}
\caption[Classification of computing systems based on working set location~\cite{7092668}.]{Classification of computing systems based on working set location~\cite{7092668}. Prior systems were based on a compute-centric approach where data is moved to the core for processing (Figure 1-1 (a)-(c)), whereas now, with near-memory computing (Figure 1-1 (d)), the processing cores are brought closer to the place where data resides. Therefore, in a data-centric approach, the data resides much closer to the processing units than in a compute-centric approach. Computation-in-memory (Figure 1-1 (e)) further reduces data movement by using memories with built-in compute capability (e.g., phase-change memory (PCM)~\cite{li2016pinatubo})
\label{fig:nmc_review_allsystems}}
\end{figure*}


\fc{
\textbf{Heterogeneous computing} has emerged as an answer to continue to improve performance beyond the limits imposed by the slow down in Moore’s Law and the end of Dennard scaling~\cite{sundararajan2010hpcwithfpga}. Heterogeneous computing entails complementing processing elements with different compute capabilities, each to perform the tasks to which it is best suited. In the HPC domain, coupling specialized compute units with general-purpose cores while following a data-centric approach can meet the high-performance computing demands and provides the ability to realize exascale systems  needed to process data-intensive workloads~\cite{nair2015active}. }

% \textbf{Hardware specialization} has emerged as an answer to continue to improve performance beyond the limits imposed by the slow down in Moore’s Law and the end of Dennard scaling~\cite{sundararajan2010hpcwithfpga}. Hardware specialization entails using available chip area to accelerate a specific application or a part of the application rather than implementing a general-purpose processor for a larger set of applications. In the HPC domain, coupling these specialized units with general-purpose cores while following a data-centric approach can meet the high performance computing demands and provides the ability to realize exascale systems  needed to process data-intensive workloads~\cite{nair2015active}. 
%There is a wide variety of hardware acceleration platform which tradeoff betw between the CPUs, GPUs, ASICs, FPGAs, and even SoCs have various advantages and design trade-offs.

The graphics processing unit (\acrshort{gpu}) is one of the most popular acceleration platforms. GPUs have been used to accelerate workloads like computer graphics and linear algebra~\cite{volkov2008benchmarking} because of their many-core architecture. However, GPUs are power-hungry due to high transistor density and, depending on the power constraints, may not always be the ideal platform for implementation. Recently, the use of field-programmable gate array (\acrshort{fpga}) in accelerating machine learning workloads with high energy-efficiency has inspired researchers to explore the use of FPGAs instead of GPUs for various high-performance computing applications~\cite{caulfield2016cloud,duarte2018fast}.  

FPGAs provide a unique combination of flexibility and performance without the cost, complexity, and risk of developing custom application-specific integrated circuits (\acrshort{asic}s). 
The researchers at CERN, for example, are using FPGAs to accelerate physics workload in CERN's \dd{exploration} for dark matter~\cite{duarte2018fast}. Microsoft's Project Catapult~\cite{caulfield2016cloud} is another example of how FPGAs can be used in the data center infrastructure. \dd{Driven by Catapult's promising research results, Microsoft further deployed the architecture on the Azure cloud marketplace~\cite{FPGA_in_azure}. } Such integration \fc{for certain workloads} can even offer more energy efficiency than CPU or GPU-based systems. However, taking full advantage of %an 
FPGAs for accelerating a workload is not a trivial task. Compared to CPUs or GPUs, {an} FPGA must exploit an order of magnitude more parallelism in a target workload to compensate for the lower clock frequency. 

The above trend raises a question: \textbf{how can we accelerate other scientific applications in an energy-efficient way on specialized hardware?}\\


% {Heterogeneous computing} has emerged as an answer to continue to improve performance beyond the limits imposed by the slow down in Moore’s Law~\cite{sundararajan2010hpcwithfpga}. Heterogeneous computing entails the use of accelerators such as graphics processing units (GPU) and/or field-programmable gate arrays (FPGAs), with a general-purpose CPU to accelerate a specific application or a part of application. Thus, improving the overall system performance and/or energy efficiency. 

% Traditionally, \acrshort{gpu}s have been  used to accelerate workloads such as computer graphics and mathematical computation algebra~\cite{volkov2008benchmarking} because of their many-core architecture. However, GPUs are power-hungry due to high transistor density and depending on the power constraints, may not always be the ideal platform for an implementation. Recently, the use of \acrshort{fpga} in accelerating machine learning workloads with high energy-efficiency has inspired researchers to explore the use of FPGAs instead of GPUs for various high-performance computing applications~\cite{cosmo_knl}.  FPGAs provide a unique combination of flexibility and performance without the cost, complexity, and risk of developing custom application-specific integrated circuits (ASICs). 
% The researchers at CERN, for example, are using FPGAs to accelerate physics workload in CERN's search for dark matter~\cite{duarte2018fast}. Microsoft's Project Catapult~\cite{caulfield2016cloud} is another example of how FPGAs can be used in the datacenter infrastructure that can offer more energy efficiency than CPU or GPU-based systems. However, taking full advantage of %an 
% FPGAs for accelerating a workload is not a trivial task. Compared to CPUs or GPUs, {an} FPGA must exploit an order of magnitude more parallelism in a target workload to compensate for the lower clock frequency. 

% The above trend raises a question: \textbf{how can we accelerate other scientific applications in an energy-efficient way on an FPGA-based heterogeneous computing platform?}


\noindent Modern FPGAs show four key trends. 
\begin{itemize} [leftmargin=*,topsep=0pt,itemsep=1ex,partopsep=1ex,parsep=1ex] %[leftmargin=*, itemsep=1ex, topsep=0pt]
    \item The integration of high-bandwidth memory (\acrshort{hbm})~\cite{hbm} on the same package as an FPGA allows us to implement our accelerator logic much closer to the memory with an order of magnitude more bandwidth than the traditional DDR4-based FPGA boards. Thus, these modern FPGAs \gthesis{adopt} a \emph{data-centric} approach. 
    \item The introduction of UltraRAM (URAM)~\cite{uram} along with the BlockRAM (BRAM) that offers massive \emph{scratchpad}-based on-chip memory next to the logic. 
    \item New cache-coherent interconnects, such as IBM Coherent Accelerator Processor Interface (\acrshort{capi})~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators (CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{cxlwhitepaper},  allow tight integration of FPGAs with CPUs at high bidirectional bandwidth {({on} the order of tens of GB/s)}. This integration \ggthesis{reduces programming effort and} enables us to coherently access the host system's memory through a pointer rather than having multiple copies of the data.   
    \item FPGAs are being manufactured with an advanced technology node of 7-14nm FinFET technology~\cite{gaide2019xilinx} that offers higher performance. \\
\end{itemize}
% First, the integration of high-bandwidth memory (\acrshort{hbm}) on the same package as an FPGA allows us to implement our accelerator logic much closer to the memory with an order of magnitude more bandwidth than the traditional DDR4-based FPGA boards. Thus these modern FPGAs \gthesis{adopt} a \emph{data-centric} approach. Second, FPGA manufactures have introduced UltraRAM (URAM) along with the BlockRAM (BRAM) that offer massive \emph{scratchpad}-based on-chip memory next to the logic. 

% Third, new cache-coherent interconnects, such as IBM Coherent Accelerator Processor Interface (\acrshort{capi})~\cite{openCAPI}, Cache Coherent Interconnect for Accelerators (CCIX)~\cite{benton2017ccix}, and Compute Express Link (CXL)~\cite{cxlwhitepaper},  allow tight integration of FPGAs with CPUs at %a 
% high bidirectional bandwidth \juang{({on} the order of tens of GB/s)}. This integration \ggthesis{reduces programming effort and} allows us to coherently access the host system's memory through a pointer rather than having multiple copies of the data.  Fourth,  FPGAs are being manufactured with an advanced technology node of 14nm FinFET technology that offers higher performance. 

\noindent These four trends suggest that \textbf{modern FPGA architectures deliver \linebreak unprecedented levels of integration and compute capability due to new technological advances, which \fc{further} provides an opportunity to overcome {the} \emph{memory bottleneck} of real-world data-intensive applications.}

% The above trends highlight that, apart from evaluating other important scientific domains, \textbf{there is a need to evaluate the performance potential of these new technological changes that bring processing close to the data and how it can impact the proliferation of FPGAs in future.}


\subsection{Data-Driven System Optimization}
\label{subsection:intro/data_driven}
On a computing system, we generally run a diverse set of workloads that generate a large amount of data.  However, our present systems do not take advantage of vast amounts of data available to them~\cite{mutlu2020modern, mutlu2020intelligent,mutlu2021intelligent_DATE}.  %Big data provides us with notably 3V's~\cite{bigdataV}: (1) Volume: the size of data; (2) Variety: data from different sources; and (3) Velocity: the speed of data generated and processed.  
Current systems are built around rigid design rules that follow fixed heuristic-driven policies or perform an exhaustive exploration with a change in system scenario rather than leveraging previous knowledge.  Moreover, these heuristic-driven approaches cannot fully capture complex relations present in various aspects of the computer architecture, such as data placement, memory management, and task scheduling. These approaches favor certain workloads and/or system configurations over others without considering an application's inherent behavior or the underlying device characteristics. For example, the storage subsystem keeps executing the same data placement policy during the entire lifetime of a system regardless of the impact of the resulting decisions on the system. A storage subsystem sees a vast amount of data, yet it cannot learn from that data and adapt its policy because the policy is rigid and hard-coded by a human. 

To overcome the inefficiency of our current computing system, we need to devise \emph{data-driven} mechanisms that take advantage of the vast amount of available data by exploiting inherent data characteristics~\cite{ipek2008self,jimenez2001dynamic,jimenez2003fast,teran2016perceptron,jimenez2005piecewise,jimenez2011optimized,bhatia2019perceptron,peled2019neural,peled2015semantic,rl_GC_TECS,rl_NOC_AIDArc_2018}. To this end, a data-driven approach can enable machine learning (\acrshort{ml}) techniques in different aspects of computer architecture design and use. ML models are trained to make predictions or decisions without explicit programming by discovering inherent patterns or relationships in the data. % Compared to commonly used heuristics, these ML-based approaches provide much more rigorous
Traditionally, computer architects have \ph{focused more} on accelerating ML algorithms. %In contrast, there has been relatively limited work on using ML to assist in architectural optimizations~\cite{MLsurvey2019}. 
In contrast, \fc{only in the past few years have we seen a growth in works using ML for architecture design and use~\cite{MLsurvey2019}. }

% Therefore, there is \textbf{an opportunity to develop novel mechanisms that allow computers to learn from experiences and reuse those experiences to make future decisions, in turn, closing a loop where computer architects enable ML, and ML improves computer architectures. Moreover, we need to assess if these machine learning-driven approaches can outperform our current human-driven approaches.}

Therefore, there is \textbf{an opportunity to develop novel mechanisms that allow computers to learn from experiences and reuse those experiences to make future decisions. In turn, closing a loop where computer architects enable ML and ML improves computer architectures. Moreover, we need to assess if these machine learning-driven approaches can outperform our current human-driven approaches.}

\gthesis{Data-driven techniques using ML can assist us in many aspects of computer architecture, including  architectural evaluation and design space exploration (\acrshort{dse}).} In the early design stage, architects often use various evaluation techniques to navigate the design space of new architectures, avoiding the cost of chip fabrication.  Usually, we employ analytic models or simulation techniques to provide performance and energy consumption estimates while using different workloads or architectural configurations. Analytic models are typically based on simple mathematical equations that provide fast estimates but at the cost of accuracy. Therefore, we often resort to simulation-based techniques that can model architectural interactions more accurately. However, simulation techniques \gthesis{can be} extremely slow because a single simulation for a real-world application with a representative dataset can take hours or even days (see Chapter~\ref{chapter:napel}). This slow speed cannot meet the modern design productivity demands, despite the efforts of accelerating simulations with both hardware~\cite{pellauer2011hasim} and software-based~\cite{sanchez2013zsim} techniques. 

In the later phase of the design cycle, architects often use FPGAs to prototype their design to get the accurate performance and power estimates. An FPGA is highly configurable and allows us to reconfigure its circuitry to implement any algorithm. However, an FPGA's large configuration space and the complex interactions among configuration options lead many developers to explore individual optimization options in an ad hoc manner. Moreover, FPGAs have infamously low productivity due to the time-consuming FPGA \fc{mapping} process~\cite{o2018predictive}. 

Therefore, a common challenge that past works {have also faced} is \textbf{how to evaluate the performance of an application or a new architecture in a reasonable amount~of~time~\cite{o2018hlspredict} \gthesis{such that a large design space can be covered}? 
}



% % \subsection{Human-Driven Heuristics}
% Our present computing systems do not take advantage of vast amounts of data available to them~\cite{mutlu2020modern}.  %Big data provides us with notably 3V's~\cite{bigdataV}: (1) Volume: the size of data; (2) Variety: data from different sources; and (3) Velocity: the speed of data generated and processed.  
% Current systems are built around rigid design rules that follow heuristic-driven policies or perform an exhaustive exploration with a change in system scenario rather than leveraging previous knowledge. We generally run a diverse set of workloads from different domains, which generate a large amount of amount.  These heuristics favor certain workload and/or system configurations over another. Moreover, human-driven approaches cannot fully capture complex relations present in various aspects of computer architecture, such as task scheduling, data-placement, and memory scheduling.  Therefore, we need to devise \emph{data-driven} mechanisms that take advantage of the vast amount of data by exploiting inherent data characteristics such as instruction/data reuse distance, memory footprint, and instruction/data level  parallelism. \gthesis{}~\cite{mutlu2020intelligent}. To this end, data-driven approach can enable machine learning (ML) techniques in different aspects of the computer architecture. ML models are trained to make predictions or decisions without explicit programming, by discovering inherent patterns or relationships in the data. Traditionally, computer architects have paid more focus on developing specialized architectures for ML algorithms. In contrast, there has been relatively limited work on applying ML to assist in architectural design~\cite{MLsurvey2019}. Therefore, there is \textbf{an opportunity to develop novel mechanisms that allow computers to learn from experiences and reuse those experiences to make future decisions, in turn, closing the loop where architects enable ML, and ML improves computer architecture. Moreover, we need to access if these machine learning-driven approaches can outperform our current human-driven approaches.}
%Notably, three-dimensional stacking is touted as the true enabler of processing close to the memory. It allows the stacking of logic and memory together using through-silicon via's (TSVs) that helps in reducing memory access latency, power consumption and provides much higher bandwidth~\cite{6242474}. Micron's Hybrid Memory Cube (HMC)~\cite{7477494}, High Bandwidth Memory (HBM)~\cite{6757501} from AMD and Hynix, and Samsung's Wide I/O~\cite{6025219} are the competing products in the 3D memory arena. 
\subsection*{Thesis Statement}
\gthesis{Based on the above-discussed aspects,} the thesis problem statement is as follows: \emph{Design system architectures to effectively handle data by: (1) overcoming the data movement bottleneck in data-intensive applications through a data-centric approach of bringing processing close to the memory and ensuring that data does not overwhelm system components; thus, enabling high performance in an energy-efficient way; and (2) further leverage the enormous amount of data to model and optimize computing systems by exploiting the inherent data characteristics to perform data-driven decisions. }

% The problem thesis statement is as follows: \emph{Design system architectures to overcome the data movement bottleneck in data-intensive application, by following a data-centric approach of bringing processing close to the memory, thus enabling high-performance in an energy-efficient way, and further leverage the enormous amount of data to model and optimize computing systems by exploiting the inherent characteristics in the data. }

\section{Overview of Our Approach}
\label{sec:intro/overview}
% \todo{add figure on contributions}\\
In line with the thesis statement, this dissertation provides five contributions based on nine methods (concepts) to handle and leverage data effectively.  In Table~\ref{tab:intro/methods}, we discuss nine different methods that we use in this dissertation.  Methods are architectural concepts that we use in our contribution to reach a specific goal. \ggthesis{ We use six data-centric (DC) methods that put data and its processing at the center of the design. These methods minimize data movement and maximize efficiency while processing, accessing, and storing data. We also adopt three data-driven (DD) methods that take advantage of the vast amount of data that flow through the system.  We briefly discuss these nine methods.
 %Architectural concepts such as \textit{specialization} and \textit{dataflow} optimize the processing of an application while concepts such as \textit{domain-specific memory hierarchy} and \textit{near-memory computing} provide low latency access to data. By \textit{reducing the memory footprint}, we can better utilize the memory space and efficiently access and process data. Moreover, the redundant amount of \textit{data copies between the host and the specialized hardware} could lead to high overhead and potentially undo the hardware acceleration benefits.
  \input{table_methods}
  \begin{enumerate} [leftmargin=*,topsep=0pt,itemsep=0.3ex] %[leftmargin=*, itemsep=1ex, topsep=0pt]
%  \begin{enumerate} [leftmargin=*,nosep]
     \item \textbf{Specialization  (DC):} Using specialized hardware platforms such as an FPGA to accelerate an application in an energy-efficient way.
     \item \textbf{Revisit memory hierarchy  (DC):} Design memory hierarchies to provide low latency access to data.
     \item \textbf{Reducing copies between host and accelerator (DC):} Minimize the redundant amount of data copies between the host and the specialized hardware.
     \item\textbf{Near-memory computing (DC):} Process data closer to the main memory to reduce the data movement overhead. 
     \item\textbf{Dataflow architecture (DC):} Enable task-level parallelism \fc{while exploiting data-level parallelism} to maximize the utilization of compute resources.
     \item \textbf{Reducing the memory footprint (DC):} Reduce an application's required memory space to efficiently access and process data.
     \item \textbf{Static machine learning  (DD):} Leveraging ML during the design phase of architecture.
     \item \textbf{Speedup design space exploration  (DD):} Quick and accurate architectural evaluation and exploration.
     \item \textbf{Dynamic machine learning  (DD):} Leveraging reinforcement learning (\acrshort{rl}) during the run-time of a system to continuously adapt system policies.\\
 \end{enumerate}

%  We also adopt three data-driven methods that take advantage of the vast amount of data that flow through the system. We leverage\textit{ static machine learning} in the design phase of an architecture, where we train ML-based models offline to speedup architectural evaluation and \textit{design space exploration}. During the run-time of a system, we use \textit{dynamic machine learning} that continuously optimizes system policies based on current system conditions. Below we highlight our approach and techniques to overcome the current inefficiencies in the computing systems.  
 }

\noindent We demonstrate these above nine methods across the following five mechanisms.\\ \linebreak
First,  we design NERO, a data-centric accelerator for a real-world weather prediction application. As mentioned above, the sheer amount of atmospheric simulation data generated is one of the biggest challenges in the domain of weather prediction.  We use a heterogeneous system comprising of IBM\textsuperscript{\textregistered} POWER9 CPU with field-programmable gate array (FPGA) as our target platform. An FPGA can provide both flexibility and energy efficiency, and moreover, is a cost-effective \gthesis{alternative} to an application-specific integrated circuit (ASIC). We create a heterogeneous domain-specific memory hierarchy using on-chip \acrshort{uram}s and  \acrshort{bram}s on an FPGA. Unlike traditionally fixed CPU memory hierarchies, which perform poorly with irregular access patterns and suffer from cache pollution effects, application-specific memory hierarchies are shown to improve energy and latency by tailoring the cache levels and cache sizes to an application's memory access patterns~\cite{jenga}.  
% \todo{ stencil, coherent accelerators, power servers, quantization, different number systems, machine learning: transfer learning, supervised, reinforcement learning, design of experiments, hybrid memory system} 
NERO overcomes the memory bottleneck {of weather {prediction} stencil kernels} by {exploiting near-memory {computation} capabilities on} specialized FPGA accelerators with high-bandwidth memory (HBM), {which are attached} {to the host CPU}. 

Second, we explore the applicability of different number formats and exhaustively search for the appropriate bit-width for memory-bound stencil kernels to improve performance and energy-efficiency with minimal loss in the accuracy.  Stencils are one of the most widely used kernels in real-world applications. Based on an exhaustive exploration of a broad range of number systems -- fixed-point, floating-point, and posit~\cite{gustafson2017beating} -- we provide the precision and the corresponding accuracy deviation. \gthesis{Each number representation offers a different dynamic range, the usability of which depends upon the target workload.} %Third, we develop PreciseFPGA, an automated framework to obtain an application-aware optimal fixed-point configuration without exhaustively searching the entire design space. 
%======================
% Third, we develop PreciseFPGA, a machine learning-based framework to obtain an application-aware optimal fixed-point configuration that can meet the strict resource constraints without exhaustively searching the entire design space.  
%======================

Third, we propose NAPEL, a machine learning-based application performance and energy prediction framework for data-centric architectures. NAPEL uses ensemble learning to build a model that, once trained for a fraction of programs on a number of architecture configurations, can predict the performance and energy consumption of {different} applications. 

Fourth, we present LEAPER, the first use of \emph{few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications. \gthesis{Machine learning (ML)-based modeling has emerged as an alternative to traditional, slow simulation (or evaluation) techniques~\cite{o2018hlspredict}. ML modeling provides the capability to both quickly evaluate various architectural design choices and perform suitability analysis for many workloads. Thus, quick exploration and large prediction time savings compared to simulation are possible. To this end, we develop NAPEL and LEAPER, which are ML-based model solutions. 

However, ML needs a large amount of data to train models, which requires running time-consuming simulations. To alleviate this problem, we use a technique called the \emph{design of experiments} (\acrshort{doe})~\cite{montgomery2017design} to extract representative data with a small number of experimental runs.  DoE is a set of statistical techniques meant to locate a small set of points in a parameter space with the goal of representing the whole parameter space. The traditional brute-force approach to collecting training data is time-consuming: the sheer number of experiments renders detailed simulations intractable.  } 

Fifth, we propose Sibyl, the first technique that uses  reinforcement learning (\acrshort{rl}) \gca{for data placement in hybrid storage systems}. Sibyl observes different features \gon{of} the \gon{running workload}  \gon{as well as the}  storage devices to make system-aware data placement decisions. For every decision \gon{it makes}, Sibyl receives a reward from the system that it uses to evaluate the long-term \gon{performance} impact of its decision and continuously optimizes its data placement policy online.  \gthesis{Compared to supervised learning, reinforcement learning provides the following three benefits. \ggthesis{First, supervised learning requires large amounts of labeled data. In some scenarios, collecting labeled data can be difficult or even infeasible.} Second, unlike supervised learning, which is purely driven by prediction accuracy, an RL-agent is objective-driven, making RL a great fit for objective-driven policies. Third, RL does not require separate training and testing phases. Instead, RL continuously learns and adapts based on the changes in the environment.} We implement Sibyl on  \emph{real} \gonn{systems with various} \go{HSS configurations, including dual- and tri-hybrid storage systems}. Our in-depth evaluation of Sibyl shows that it outperforms \gonn{four} state-of-the-art %heuristic- and learning-based 
    techniques over a wide variety of applications with a low implementation overhead. 



% Overall, this dissertation contributes to designing, modeling, and optimizing architectures that handle data well by following both \emph{data-centric} and \emph{data-driven} principles.


% Computer architects often run a number of benchmarks/workloads on a multitude of hardware
% configurations (and generate multiple statistics) when studying new or existing ideas. This
% leads to huge amounts of data which researchers often study in a limited fashion on ad hoc
% basis. In contrast, if ML based analysis is performed on this data, we might be able to see the
% true potential of that data and its ability to help us discover new findings.

% ML techniques can potentially be used to build customizable computer systems which will
% learn to change their behavior at different granularities. Take an example of an ’A’ cache
% eviction policy which works better for workload type ’X’ and another policy ’B’ which works
% better for workload type ’Y’. Since, ML makes learning easier, same processor can learn to
% adapt to using policy ’A’ or ’B’ depending on the workloads run on it.
% Therefore,
% ML techniques can come to rescue and enable building simulation tools of the future as
% traditional cycle level modeling might be too slow for cross-stack studies. Not only that ML
% techniques can enable building new tools, they can help in improving the accuracy of current
% simulation tools (or performance/power models) which are the primary enabler of computer
% architecture research at the moment
\section{Contributions}
\label{sec:intro/contributions}
\noindent This dissertation makes the following \textbf{key contributions}:
% \begin{enumerate}[leftmargin=*,nosep]

\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=1.3ex]
\renewcommand{\namePaper}{NERO\xspace} %TITLE
% ,topsep=0pt
\item In \textbf{Chapter~\ref{chapter:nero}}, we propose \namePaper, {the first} near-HBM FPGA-based accelerator for representative kernels from a real-world weather prediction application.  Weather prediction is one such high-performance computing application that generates a large amount of data. It consists of   compound stencil kernels that operate on a three-dimensional grid. Such compound kernels are dominated by memory-bound operations with complex memory access patterns and low arithmetic intensity. This poses a fundamental challenge to acceleration.
 \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item We perform a detailed roofline analysis to show that representative weather prediction kernels are constrained by memory bandwidth on state-of-the-art CPU systems.
    \item We optimize \namePaper~with a data-centric caching scheme with precision-optimized tiling for a heterogeneous memory hierarchy (consisting of URAM, BRAM, and HBM).
    \item We evaluate the performance and energy consumption of our accelerator and perform a scalability analysis. We show that an FPGA+HBM-based design 
    outperforms a complete 16-core POWER9 system~(running 64~threads)~by~$4.2\times$ for the vertical advection (\texttt{vadvc}) and $8.3\times$ for %a 
    the horizontal diffusion (\texttt{hdiff}) kernels with energy reductions of $22\times$ and $29\times$, respectively. 
    %Our design provides an energy efficiency of 1.5 GLOPS/Watt and 17.3 GFLOPS/Watt for \texttt{vadvc} and \texttt{hdiff} kernels, respectively.
    \end{enumerate}
\item In \textbf{Chapter~\ref{chapter:low_precision_stencil}}, we perform a precision exploration of the three-dimensional stencil kernels for future mixed-precision systems using a wide range of number systems, including fixed-point, floating-point, and posit.
       \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item  We provide the precision and the corresponding accuracy deviation for a broad range of number systems -- fixed-point, floating-point, and posit.
    \item We tune stencil-based kernels on a state-of-the-art IBM POWER9 CPU and further evaluate them on an FPGA, which is coherently attached to the host memory. Thus, this chapter fills the gap between the current hardware capabilities and future hardware design.
    \item As an extension of this chapter, in Appendix~\ref{chapter:precise_fpga}, we demonstrate our approach to automate the exploration for fixed-point configurations. We show our results for tuning the precision of weights for a neural network.
    \end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
% \renewcommand{\namePaper}{PreciseFPGA\xspace} %TITLE
%  \item In \textbf{Appendix~\ref{chapter:precise_fpga}}, we propose \namePaper, a new resource prediction framework  for fixed-point computation taking into account the effect of FPGA-resource saturation. \ggthesis{This work demonstrates our approach to automate fixed-point configuration exploration.}
%     \begin{enumerate}
%     \setlength{\itemsep}{0pt}
%     \setlength{\parskip}{3pt}
%     \setlength{\parsep}{0pt}
%     \item \namePaper~allows us to predict post-implementation FPGA power and resource utilization with an average accuracy of 96\% and 95\%, respectively.
%     \item We show \namePaper~can provide highly accurate Pareto-Optimal implementation using only C-Synthesis~\cite{hls} results of only two fixed-point configurations. \namePaper~reduces design-space exploration time by ${674\times}$ compared to an exhaustive search.
%     \end{enumerate}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%       
\item In \textbf{Chapter~\ref{chapter:napel}}, we propose NAPEL, a new, {fast} high-level performance and energy estimation framework for NMC architectures. NAPEL {is the first such model to} leverage ensemble learning techniques, specifically random forest, to {quickly estimate} the performance and energy consumption of previously-unseen applications in the early stages of design space exploration for NMC architectures.

     \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item We {reduce} the simulation time needed to gather training data for NAPEL by employing a DoE technique~\cite{mariani2017predicting}, which selects a {small} number of application input configurations that well represent the entire space of input configurations.
    \item {We} show that NAPEL can provide performance and energy estimates {$220\times$ faster than a state-of-the-art microarchitecture simulator} with an {average error rate of 8.5\% (performance) and 11.6\% (energy)} compared to the simulator.
    \item We show that we can use NAPEL to {accurately} determine if, {and by how much,} executing a certain workload on a specific NMC architecture can improve performance and reduce energy consumption {versus execution on a CPU}.
    \end{enumerate}

\item In \textbf{Chapter~\ref{chapter:leaper}}, we present LEAPER, the first use of \emph{few-shot learning} to transfer FPGA-based computing models across different hardware platforms and applications. This approach dramatically reduces (up to $10\times$) the training overhead by adapting a \emph{base model} trained on a low-end {edge} {FPGA} platform to a {new}, unknown high-end environment ({a cloud environment in our case}) rather than building a new model from scratch).
  \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item We create an {ensemble of transfer learning models} to accurately transfer learning from multiple base learners to avoid a negative transfer, i.e.,  severe degradation of the predictive power of the transferred model. % The use of {multiple} base learners lets us avoid severe degradation of the \textit{transferred} model's predictive power, i.e., avoid a \textit{negative transfer} \jgl{What is a negative transfer? If you want to include this term, then flip the sentence: "...to avoid a negative transfer, i.e., a severe degradation of the predictive power of the transferred model.}.  
    \item We demonstrate our approach across \textit{five} {state-of-the-art,} high-end, {on-premise cloud} FPGA-based platforms with \textit{three} different {interconnect} technologies, between host CPU and FPGA, on \textit{six} real-world applications. %{The kernels are specified in C/C++ and compiled to the FPGA target using Vivado HLS for the target and Xilinx SDSoC for the base model.}
    For \textit{5-shot} learning, we achieve an average performance and area prediction accuracy of 80--90\%. 
    \end{enumerate}

    
 \renewcommand{\namePaper}{Sibyl\xspace} %TITLE  
 \item In \textbf{Chapter~\ref{chapter:sibyl}}, we propose \namePaper%\footnote{We plan to open-source \namePaper upon paper acceptance.}
  , a new self-\gon{optimizing}  mechanism %for %effective data placement in hybrid storage systems 
  \gon{that uses} reinforcement learning \gon{to make data placement decisions in hybrid storage systems}. \namePaper{} %\juang{data-placement module} 
  \go{dynamically}
  \emph{learns}\gont{,} \gonn{ using both multiple workload features and system-level feedback information\gont{, how} to continuously adapt its policy to improve \rnlast{its} long-term performance \rnlast{for} a workload.}
    \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item  We show on real \gonn{hybrid storage systems (HSSs)}  that prior state-of-the-art \gont{HSS data placement mechanisms} fall 
 %short significantly than the oracle
  short of the oracle placement due to: lack of  \gon{(1) adapt\gonn{i}vity to workload changes and \gonn{storage device characteristics}, and (2) extensibility. } %(1) strict policies that take into account only a certain aspect of the application or the system, (2) no system-level feedback, and (3)  lack of extensibility.
 
    
    \item We conduct an in-depth evaluation of \namePaper on \gon{real \gonn{systems with various} HSS configurations\gont{,}} showing that it outperforms \gonn{four} state-of-the-art %heuristic- and learning-based 
    techniques over a wide variety of applications with a low implementation overhead.
    \item We provide an \rbc{in-depth} explanation of \namePaper's actions that show that \namePaper performs dynamic data placement decisions by learning \gonn{ changes in the level of asymmetry in the read/write latenc\gonzz{ies} and the number and types of storage devices.} % the asymmetry in the read/write latencies present in \rbc{modern} hybrid storage devices. % while taking into account the inherent application characteristics.
    \item \gca{ We \gon{freely} open-source \namePaper to aid % RL-based research in hybrid storage systems. 
 {future research \gon{in} data placement for storage systems~\cite{sibylLink}}.} %\MYhref[black]{https://github.com/CMU-SAFARI/Sibyl}{https://github.com/CMU-SAFARI/Sibyl}}} \jgll{You can better have this link as a citation. You can cite it from other parts of the paper too.}
    \end{enumerate}
\item In addition to the above contributions, in \textbf{Chapter~\ref{chapter:background}}, we analyze and organize the extensive body of literature on near-memory computing  architectures across various dimensions: starting from the memory level where this paradigm is applied to the granularity of an application that could be executed on these architectures. 
    \begin{enumerate}[leftmargin=*, noitemsep, topsep=-1pt]
    \item A survey of existing near-memory computing architectures. We review more than 30 architectures in detail and identify the strengths and weaknesses of the existing architectures in Appendix~\ref{chapter:appendixA}.
    \item We highlight the opportunities and the challenges in the domain of near-memory computing. % The challenges include evaluation tools, virtual memory support, memory coherency, task scheduling, and data mapping. 
    %Our design provides an energy efficiency of 1.5 GLOPS/Watt and 17.3 GFLOPS/Watt for \texttt{vadvc} and \texttt{hdiff} kernels, respectively.
    \end{enumerate}
    
\end{enumerate}
% \pagebreak
\subsection*{Thesis Conclusion}
\noindent Overall, we make the following two conclusions for this thesis. 
 \begin{enumerate} 
\item \emph{Hardware acceleration on an FPGA+HBM fabric is a promising solution to reduce the data movement bottleneck of our current computing systems in an energy-efficient way. }

\item \emph{Data should drive system and design decisions by exploiting the inherent \linebreak characteristics of data to perform efficient architectural decisions or predictions in various design aspects of the computer architecture.} 
  \end{enumerate}
Therefore, we conclude that the mechanisms proposed by this dissertation provide \linebreak promising solutions to handle data well by following a \emph{data-centric} approach and further demonstrate the importance of leveraging data to devise \emph{data-driven} policies. 

\section{Dissertation Structure}
\label{sec:intro/outline}
This thesis is organized into \gcheck{eight} chapters. Chapter~\ref{chapter:background} provides background into near-memory computing, where we classify and evaluate various state-of-the-art \emph{data-centric} architectures. In Appendix~\ref{chapter:appendixA}, we describe in detail all the evaluated architectures. Additionally,  Chapter~\ref{chapter:background} also highlights various challenges that need to be addressed. Chapter~\ref{chapter:nero} presents NERO, a \emph{data-centric} architecture of weather prediction application. Chapter~\ref{chapter:low_precision_stencil} explores the applicability of different number systems \ou{for stencil kernels}. As an extension to Chapter~\ref{chapter:low_precision_stencil}, Appendix~\ref{chapter:precise_fpga} presents PreciseFPGA. It provides an automated exploration framework for fixed-point representation. Chapter~\ref{chapter:napel} introduces NAPEL, a fast high-level performance, and energy estimation framework. Chapter~\ref{chapter:leaper} presents LEAPER, our approach to quickly model different FPGA-based hardware platforms and applications. Chapter~\ref{chapter:sibyl} introduces Sibyl, the first RL-based \emph{data-driven} mechanism for data placement in a hybrid storage system. Chapter~\ref{chapter:conclusion} concludes this dissertation and provides future directions that are enabled by \ggthesis{its results} -- both in the domain of \emph{data-centric computing}  and \emph{data-driven optimization}  that can help us overcome present computing system challenges. In addition to the works presented in this thesis, Appendix~\ref{chapter:appendixB} highlights several other contributions of the author.
 
% \section{Dissertation Outline}

% \input{NMC_review/sections/mainMemory.tex}


% \input{NMC_review/sections/scm.tex}


% \input{NMC_review/sections/challenges.tex}


% \input{NMC_review/sections/system.tex}


% \input{NMC_review/sections/future.tex}

% \input{NMC_review/sections/conclusion.tex}


==> PhD_Thesis_Updated_arxiv (1)/ch2-NERO.tex <==
% \chapter[NERO: A Near-High Bandwidth Memory Stencil Accelerator]{NERO: A Near-High Bandwidth Memory Stencil Accelerator for Weather Prediction Modeling }
\chapter[\texorpdfstring{NERO: A Near-High Bandwidth Memory Stencil Accelerator for Weather Prediction Modeling}{NERO: A Near-High Bandwidth Memory Stencil Accelerator for Weather Prediction Modeling}
]{\chaptermark{header} NERO: A Near-High Bandwidth Memory Stencil Accelerator for Weather Prediction Modeling}
\chaptermark{NERO}
\label{chapter:nero}
\chapternote{The content of this chapter was published as \emph{``NERO: A Near High-Bandwidth Memory Stencil Accelerator for Weather Prediction Modeling''} in FPL 2020. (\emph{Nominated for the Stamatis Vassiliadis Memorial Best Paper Award})\\
Our earlier work was published as \emph{``{NARMADA}: {N}ear-Memory Horizontal Diffusion Accelerator for Scalable Stencil Computations''} in FPL 2019 where we accelerate only horizontal diffussion kernel from the COSMO (Consortium for Small-Scale Modeling) model. }
\renewcommand{\namePaper}{NERO\xspace} %TITLE
\input{NERO/sections/abstract.tex}
\input{NERO/sections/introduction.tex}
\input{NERO/sections/background}
\input{NERO/sections/accelerator.tex}
\input{NERO/sections/results.tex}
 \input{NERO/sections/relatedWork.tex}
 \input{NERO/sections/conclusion.tex}

==> PhD_Thesis_Updated_arxiv (1)/ch3-precision.tex <==
\chapter{Low Precision Processing for High Order Stencil Computations}
\chapternote{The content of this chapter was published as \emph{``Low Precision  Processing  for  High Order  Stencil Computations''} in Springer LNCS 2019.}
\label{chapter:low_precision_stencil}
\input{Stencil_Precise/abstract.tex}

%\keywords{First keyword  \and Second keyword \and Another keyword.}

%
%
% \showthe\textwidth  % <-- this tells you the textwidth
\vspace{-0.7cm}

\input{Stencil_Precise/introduction.tex}
\input{Stencil_Precise/background.tex}
\input{Stencil_Precise/methodology.tex}
\input{Stencil_Precise/evaluation.tex}
\input{Stencil_Precise/relatedWork.tex}
\input{Stencil_Precise/conclusion.tex}

==> PhD_Thesis_Updated_arxiv (1)/ch4-SIBYL.tex <==
\renewcommand{\namePaper}{Sibyl\xspace} %TITLE
% \chapter{\namePaper: Reinforcement Learning-{B}ased Data Placement for Hybrid Storage Systems} 
\chapter[\texorpdfstring{\namePaper: Adaptive and Extensible  Data Placement in Hybrid Storage Systems Using Online Reinforcement Learning}{\namePaper: Adaptive and Extensible  Data Placement in Hybrid Storage Systems Using Online Reinforcement Learning}
]{\chaptermark{header} \namePaper: Adaptive and Extensible  Data Placement in Hybrid Storage Systems Using Online Reinforcement Learning}
\chaptermark{\namePaper}
% \chapternote{The content of this chapter is under submission as \emph{``\namePaper: Reinforcement Learning-{B}ased Data Placement for Hybrid Storage Systems''}.}
\label{chapter:sibyl}
% \input{QRATOR/sections/abstract}
% \input{QRATOR/sections/introduction}
% \input{QRATOR/sections/background}
% \input{QRATOR/sections/motivation}
% \input{QRATOR/sections/mechanism}
% \input{QRATOR/sections/evaluation}
% \input{QRATOR/sections/related}
% \input{QRATOR/sections/conclusion}


\input{Sibyl/sections/abstract_v2}
\input{Sibyl/sections/introduction}
\input{Sibyl/sections/background}
% \vspace{-0.5cm} 
\input{Sibyl/sections/motivation}
\vspace{-0.2cm}
\input{Sibyl/sections/rlmotivation}
% \vspace{-0.1cm}
\input{Sibyl/sections/rl_formulation}
% \vspace{-0.2cm}
\input{Sibyl/sections/design}
% \vspace{-0.2cm}
\input{Sibyl/sections/evaluation}
% \vspace{-0.1cm}
\input{Sibyl/sections/explainability}
% \vspace{0.9cm}
\input{Sibyl/sections/discuss}
% \vspace{-0.1cm}
\input{Sibyl/sections/related}
% \vspace{-0.1cm}
\input{Sibyl/sections/conclusion}



==> PhD_Thesis_Updated_arxiv (1)/ch5-NAPEL.tex <==
% \chapter{NAPEL: Near-Memory Computing Application Performance Prediction via Ensemble Learning}

\chapter[\texorpdfstring{NAPEL: Near-Memory Computing Application Performance Prediction via Ensemble Learning}{NAPEL: Near-Memory Computing Application Performance Prediction via Ensemble Learning}
]{\chaptermark{header} NAPEL: Near-Memory Computing Application Performance Prediction via Ensemble Learning}
\chaptermark{NAPEL}
\label{chapter:napel}
\renewcommand{\namePaper}{NAPEL\xspace} %TITLE

\chapternote{The content of this chapter was published as \emph{``NAPEL: Near-Memory Computing Application Performance Prediction via Ensemble Learning''} in DAC 2019.}
%  With the emergence of three-dimensional stacking, the decade-old concept of placing compute units close to the memory has become more viable. Essentially, processing right at the ``home" of data to eliminate unnecessary data movement is referred to as near-memory computing (NMC). 

To harness the power of near-memory computing architectures, having a high-level performance model can offer fast turnaround times in early design stages. This chapter proposes an NMC model that combines technology parameters and application specific characteristics to evaluate the performance of a workload. A statistical design of experiment (DoE) methodology is first employed to select a set of representative design points for simulation. These sampled points well represent the whole space of possible input configurations. Then, ensemble learning is leveraged to develop a model that can predict performance metrics for new unseen applications on these novel architectures. Further, this model can act as a classifier to predict whether or not should an application be offloaded to NMC cores.  %The experimental results demonstrate that, by using DoE, we can extract more informative training data with a minimal number of experimental runs. Thus, we save a significant amount of simulation overhead with respect to a traditional exhaustive brute-force approach of random data selection. Besides minimizing the number of experiments, our inexpensive performance model can provide, on average, an additional 10$\times$ reduction in performance evaluation time with an error rate lower than 15\% compared to a computationally-intensive state-of-the-art NMC simulator.


\input{NAPEL/sections/introduction.tex}
\input{NAPEL/sections/methodology}
\input{NAPEL/sections/results.tex}
\input{NAPEL/sections/relatedWork.tex}
\input{NAPEL/sections/conclusion.tex}

==> PhD_Thesis_Updated_arxiv (1)/ch6-LEAPER.tex <==
\renewcommand{\namePaper}{LEAPER\xspace} %TITLE
% \chapter{\namePaper: Modeling Cloud FPGA-based Systems via Few-Shot Learning}
\chapter[\texorpdfstring{\namePaper: Modeling FPGA-Based Systems via Few-Shot Learning}{\namePaper: Modeling Cloud FPGA-based Systems via Few-Shot Learning}
]{\chaptermark{header} \namePaper: Modeling FPGA-Based Systems via Few-Shot Learning}
\chaptermark{\namePaper}
\label{chapter:leaper}

\chapternote{A part of this chapter is published as \emph{``Modeling FPGA-Based Systems via Few-Shot Learning''} in FPGA 2021.
% \\A detailed version of this chapter is under submission as \emph{``LEAPER: Modeling Cloud FPGA-Based Systems via Few-Shot Learning''}.\\
}

% \input{LEAPER/sections/abstract.tex}
% \input{LEAPER/sections/introduction.tex}


% \input{LEAPER/sections/methodology.tex}


% \input{LEAPER/sections/results.tex}
% \input{LEAPER/sections/relatedWork.tex}
% \input{LEAPER/sections/conclusion.tex}


\input{LEAPER_SIGMETRICS/sections/abstract.tex}
\input{LEAPER_SIGMETRICS/sections/introduction.tex}
\input{LEAPER_SIGMETRICS/sections/methodology.tex}
\input{LEAPER_SIGMETRICS/sections/results.tex}
\input{LEAPER_SIGMETRICS/sections/relatedWork.tex}
\input{LEAPER_SIGMETRICS/sections/conclusion.tex}

==> PhD_Thesis_Updated_arxiv (1)/ch7-PreciseFPGA.tex <==
\renewcommand{\namePaper}{PreciseFPGA\xspace} %TITLE
% \chapter{\namePaper: Constrained Neural Network Accelerator Search for FPGA}
% \chapter{\namePaper: Low Precision Accelerator Search for FPGA}
\chapter[\texorpdfstring{\namePaper: Low Precision Accelerator Search for FPGA}{\namePaper: Low Precision Accelerator Search for FPGA}
]{\chaptermark{header} \namePaper: Low Precision Accelerator Search for FPGA}
\chaptermark{\namePaper}
% \chapternote{The content of this appendix is under submission as \emph{``\namePaper: Low Precision Accelerator Search for FPGA''}.}
\label{chapter:precise_fpga}
\input{PreciseNN/sections/introduction}
% \input{PreciseNN/sections/background}
\input{PreciseNN/sections/Motivation}
\input{PreciseNN/sections/methods}
\input{PreciseNN/sections/Results}
\input{PreciseNN/sections/Related_Works}
\input{PreciseNN/sections/Conclusion}

==> PhD_Thesis_Updated_arxiv (1)/contents.tex <==
  % -*- Mode:TeX -*-
%% This file simply contains the commands that actually generate the table of
%% contents and lists of figures and tables.  You can omit any or all of
%% these files by simply taking out the appropriate command.  For more
%% information on these files, see appendix C.3.3 of the LaTeX manual. 

\begingroup
\setstretch{1.05}
\setlength\bibitemsep{0.1pt}
\pdfbookmark{\contentsname}{toc}
\tableofcontents
\endgroup

\newpage
%%%%%%%%%%%%%%%%%%%%%%add list of figures to content page%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cleardoublepage
% % \phantomsection
\pagenumbering{roman}

%%%%%%%%%%%%%%%%%%%%%%add list of figures to content page%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begingroup
\setstretch{1}
\setlength\bibitemsep{0.1pt}
\listoffigures
\addcontentsline{toc}{chapter}{\listfigurename}
\endgroup

% \newpage


\begingroup
\setstretch{1}
\setlength\bibitemsep{0.1pt}
\listoftables
\addcontentsline{toc}{chapter}{\listtablename}
\endgroup


\begingroup
\setstretch{0.95}
\setlength\bibitemsep{0.1pt}
        % \addcontentsline{toc}{chapter}{List of terms}
\glsfindwidesttoplevelname
\printglossary[title=List of Acronyms, toctitle=List of Acronyms, type=\acronymtype]
\endgroup
% \listoffigures
% \listoftables

==> PhD_Thesis_Updated_arxiv (1)/cover.tex <==
% -*-latex-*-
% 
% For questions, comments, concerns or complaints:
% thesis@mit.edu
% 
%
% $Log: cover.tex,v $
% Revision 1.8.1 2015/08/14 8:58:00  alinush
% Citations in .tex files now point to dummy entries in main.bib
% Font smoothness issues solved. Created an easy to use Makefile.
%
% Revision 1.8  2008/05/13 15:02:15  jdreed
% Degree month is June, not May.  Added note about prevdegrees.
% Arthur Smith's title updated
%
% Revision 1.7  2001/02/08 18:53:16  boojum
% changed some \newpages to \cleardoublepages
%
% Revision 1.6  1999/10/21 14:49:31  boojum
% changed comment referring to documentstyle
%
% Revision 1.5  1999/10/21 14:39:04  boojum
% *** empty log message ***
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.3  93/05/17  17:06:29  starflt
% Added acknowledgements section (suggested by tompalka)
% 
% Revision 1.2  92/04/22  13:13:13  epeisach
% Fixes for 1991 course 6 requirements
% Phrase "and to grant others the right to do so" has been added to 
% permission clause
% Second copy of abstract is not counted as separate pages so numbering works
% out
% 
% Revision 1.1  92/04/22  13:08:20  epeisach

% NOTE:
% These templates make an effort to conform to the MIT Thesis specifications,
% however the specifications can change.  We recommend that you verify the
% layout of your title page with your thesis advisor and/or the MIT 
% Libraries before printing your final copy.

% If you wish to list your previous degrees on the cover page, use the 
% previous degrees command:
%       \prevdegrees{A.A., Harvard University (1985)}
% You can use the \\ command to list multiple previous degrees
%       \prevdegrees{B.S., University of California (1978) \\
%                    S.M., Massachusetts Institute of Technology (1981)}


% Make the titlepage based on the above information.  If you need
% something special and can't use the standard form, you can specify
% the exact text of the titlepage yourself.  Put it in a titlepage
% environment and leave blank lines where you want vertical space.
% The spaces will be adjusted to fill the entire page.  The dotted
% lines for the signatures are made with the \signature command.


% The abstractpage environment sets up everything on the page except
% the text itself.  The title and other header material are put at the
% top of the page, and the supervisors are listed at the bottom.  A
% new page is begun both before and after.  Of course, an abstract may
% be more than one page itself.  If you need more control over the
% format of the page, you can use the abstract environment, which puts
% the word "Abstract" at the beginning and single spaces its text.

%% You can either \input (*not* \include) your abstract file, or you can put
%% the text of the abstract directly between the \begin{abstractpage} and
%% \end{abstractpage} commands.

%\null\vfill
%\noindent
%Copyright 2010 -- Example Cooperation\\
%Some text ...

% Uncomment the next line if you do NOT want a page number on your
% abstract and acknowledgments pages.
% \pagestyle{empty}
% \setcounter{savepage}{\thepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

% Additional copy: start a new page, and reset the page number.  This way,
% the second copy of the abstract is not counted as separate pages.
% Uncomment the next 6 lines if you need two copies of the abstract
% page.
% \setcounter{page}{\thesavepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

% \cleardoublepage

% \input{ack}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-


==> PhD_Thesis_Updated_arxiv (1)/cover_tue.tex <==
\title{Near-Data Computing and \\ Data-Driven Architectures} 
\title{Performance modeling and enhancement for data-centric systems} 
\title{Designing, modeling, and optimizing \\data-centric architectures} 
\covertitle{Designing, modeling, and optimizing \\data-centric architectures} 
\title{Designing, Modeling, and Optimizing \\Data-Intensive Computing Systems}
\covertitle{Designing, Modeling, and Optimizing Data-Intensive Computing Systems}
\author{Gagandeep Singh} 
\birthplace{Chandigarh, India}
\defencedate{maandag 29  maart 2021 om 16:00 uur}
% \defencedate{dinsdag 1 december 2015 om 14.00 uur} % ofwel iets als {maandag 1 januari 2015 om 16.00 uur}
\backoffront{\noindent Dit proefschrift is goedgekeurd door de promotoren en de samenstelling van de \linebreak promotiecommissie is als volgt:\\[2em]

\noindent\begin{tabular}{ll}
voorzitter:     & prof.dr.ir.\ A. B.\ Smolders \\
1$^e$ promotor: & prof.dr.\ H.\ Corporaal\\
2$^e$ promotor:  & prof.dr.\ O.\ Mutlu    (ETH Z\"urich)\\
copromotor:     & dr.ir.\ S.\ Stuijk \\
 leden: & prof.dr.\ H.P.\ Hofstee    (IBM Research Austin/TU Delft)\\
                  & prof.dr.\ F.\ Catthoor (IMEC/KU Leuven)\\
                  & prof.dr.ir.\ C.H.\ van Berkel\\
% leden:          & prof.dr.Tech.\ J.H.\ Takala MSc (Tampere University of Technology) \\
%                 & prof.dr.\ K.L.M.\ Bertels (Technische Universiteit Delft) \\
% 				& prof.dr.ir.\ P.H.N. de With \\
 adviseurs:   & dr.\ O.\ Unsal (BSC-CNS) \\
 
 & dr.\ D.\ Diamantopoulos (IBM Research Europe) \\
 				
\end{tabular}

\vfill
\noindent Het onderzoek dat in dit proefschrift wordt beschreven is uitgevoerd in overeenstemming met de TU/e Gedragscode Wetenschapsbeoefening.
}

\backofcover{\noindent Doctorate committee:\\

\noindent\begin{tabular}{ll}
prof.dr.\ H.\ Corporaal         & Eindhoven University of Technology, 1$^{st}$  promotor\\
prof.dr.\ O.\ Mutlu    & ETH Z\"urich, 2$^{nd}$ promotor \\
dr.ir.\ S.\ Stuijk        & Eindhoven University of Technology, copromotor\\
prof.dr.ir.\ A.B.\ Smolders  & Eindhoven University of Technology, chairman \\
prof.dr.\ H.P.\ Hofstee  & IBM Research Austin/TU Delft\\
 prof.dr.\ F.\ Catthoor & IMEC/KU Leuven\\
 prof.dr.ir.\ C.H.\ van Berkel & Eindhoven University of Technology\\
dr.\ O.\ Unsal & BSC-CNS\\
dr.\ D.\ Diamantopoulos &IBM Research Europe \\

% prof.dr.ir.\ A.C.P.M.\ Backx    & Eindhoven University of Technology, chairman\\
% prof.dr.Tech.\ J.H.\ Takala MSc & Tampere University of Technology\\
% prof.dr.\ K.L.M.\ Bertels       & Delft University of Technology\\
% prof.dr.ir.\ P.H.N.\ de With    & Eindhoven University of Technology\\
% dr.ir.\ J.A.J.\ Leijten         & Intel Benelux\\
% dr.ir.\ B.\ Mesman              & Eindhoven University of Technology\\
 \end{tabular}
\vfill \small

\noindent This work is supported in part by the European Commission under Marie Sklodowska-Curie Innovative Training Networks European Industrial Doctorate (Project ID: 676240).
\vspace{1em}
% was performed in the framework of the Horizon 2020 program for the project ``Near-Memory Computing (NeMeCo)''. It is funded by the European Commission under Marie Sklodowska-Curie Innovative Training Networks European Industrial Doctorate (Project ID: 676240).

\noindent \textcopyright{} Copyright 2021, Gagandeep Singh\\All rights reserved.  Reproduction in whole or in part is prohibited without the written consent of the copyright owner.
\vspace{1em}

\noindent Cover design by Harpreet Kaur
\vspace{1em}

\noindent Printed by ProefschriftMaken || www.proefschriftmaken.nl %CPI-Koninklijke W\"ohrmann -- The Netherlands
\vspace{1em}

\noindent A catalogue record is available from the Eindhoven University of Technology Library.\\
ISBN: 978-90-386-5227-6
 }

==> PhD_Thesis_Updated_arxiv (1)/list-acronym.tex <==
\usepackage[toc,nopostdot,style=alttree,nogroupskip,acronym,nonumberlist]{glossaries}

% \setlength{\glslistdottedwidth}{0.6\textwidth} % adjust distance betwen acronym short and acronym long columns

% \newglossarystyle{mydottedstyle}{%
%  \glossarystyle{list}%
%  \renewcommand*{\glossaryentryfield}[5]{%
%     \item[]\makebox[\glslistdottedwidth][l]{%
%       \glsentryitem{##1}\glstarget{##1}{##3 (##2)}%
%       \unskip\leaders\hbox to 2.9mm{\hss.}\hfill\strut}##5}%
% }

% \glossarystyle{mydottedstyle}

\makeglossaries

\newglossaryentry{latex}
{
        name=latex,
        description={Is a mark up language specially suited for 
scientific documents}
}

\newglossaryentry{maths}
{
        name=mathematics,
        description={Mathematics is what mathematicians do}
}

\newglossaryentry{formula}
{
        name=formula,
        description={A mathematical expression}
}

\newacronym{nmc}{NMC}{Near-Memory Computing}
\newacronym{scm}{SCM}{Storage Class Memory}
\newacronym{soc}{SoC}{System-on-a-Chip}
\newacronym{ssd}{SSD}{Solid-State Drive}
\newacronym{llvm}{LLVM}{Low Level Virtual Machine}
\newacronym{tco}{TCO}{Total Cost of Ownership}
\newacronym{asic}{ASIC}{Application-Specific Integrated Circuits}
\newacronym{cgra}{CGRA}{Coarse-Grained Reconfigurable Architecture}
\newacronym{cim}{CIM}{Computation-In Memory}
\newacronym{hpc}{HPC}{High-Performance Computing}
\newacronym{cosmo}{COSMO}{Consortium for Small-Scale Modeling}
\newacronym{fpga}{FPGA}{Field-Programmable Gate Array}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{pe}{PE}{Processing Element}
\newacronym{hbm}{HBM}{High-Bandwidth Memory}
\newacronym{hmc}{HMC}{Hybrid Memory Cube}
\newacronym{doe}{DoE}{Design of Experiments}
\newacronym{lhs}{LHS}{Latin Hypercube Sampling}
\newacronym{uram}{URAM}{UltraRAM}
\newacronym{bram}{BRAM}{Block RAM}
\newacronym{dse}{DSE}{Design Space Exploration}
\newacronym{lut}{LUT}{Lookup Table}
\newacronym{ff}{FF}{Flip Flop}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{dsp}{DSP}{Digital Signal Processor}
\newacronym{clb}{CLB}{Configurable Logic Block}
\newacronym{api}{API}{Application Programming Interface }
\newacronym{hls}{HLS}{High-Level Synthesis}
\newacronym{capi}{CAPI}{Coherent Accelerator Processor Interface}
\newacronym{psl}{PSL}{Power-Service Layer}
\newacronym{ilp}{ILP}{Instruction Level Parallelism}
\newacronym{afu}{AFU}{Accelerator Functional Unit}
\newacronym{ccd}{CCD}{Central Composite Design}
\newacronym{nn}{NN}{Neural Network}
\newacronym{rf}{RF}{Random Forest}
\newacronym{ipc}{IPC}{Instructions Per Cycle}
\newacronym{edp}{EDP}{Energy-Delay Product}
\newacronym{nvm}{NVM}{Non-volatile Memory}
\newacronym{slc}{SLC}{Single-level Cell}
\newacronym{mlc}{MLC}{Multi-level Cell}
\newacronym{tlc}{TLC}{Triple-level Cell}
\newacronym{tlb}{TLB}{Translation Lookaside Buffer}
\newacronym{hss}{HSS}{Hybrid Storage System}

==> PhD_Thesis_Updated_arxiv (1)/mypublication.tex <==
% \renewcommand\bibname{List of Publications}
\begin{refsection}
% If you print a bibliography within this section, only citations within this refsection will be printed.
% Option 1: Make nocite for all of your papers.
% Options 2 would be a seperate file which contains all of your papers.
\nocite{singh2020nero_own}
\nocite{singh2019narmada_own}
\nocite{singh2019napel_own}
\nocite{singh2019near_own}
\nocite{singh2019low_own}
\nocite{singh2018review_own}

\defbibnote{myPrenote}{
 {\bf First Author:}
}
% \defbibnote{myPostnote}{
%     {\bf Co-Author:}
% }
% \newrefcontext[sorting=ynt]

\begin{refcontext}[sorting=ydndt]
\printbibliography[heading=bibintoc,  title={List of Publications},
    prenote=myPrenote
  ]
\end{refcontext}
\end{refsection}

\begin{refsection}
\nocite{diamantopoulos2020agile}
\nocite{vadivel2020tdo}
\nocite{corda2019platform}
\nocite{corda2019memory}
\nocite{chris2019DATE}

\defbibnote{myPrenote}{
 {\bf Co-Author:}
}
% \defbibnote{myPostnote}{
%     {\bf Co-Author:}
% }
\begin{refcontext}[sorting=ydndt]
\printbibliography[
   heading=none, 
    prenote=myPrenote
  ]
\end{refcontext}
\end{refsection}


        % \begin{refsection}
        % % If you print a bibliography within this section, only citations within this refsection will be printed.
        % % Option 1: Make nocite for all of your papers.
        % % Options 2 would be a seperate file which contains all of your papers.
        % \nocite{undersub-singh2021micro}
        % \nocite{undersub-singh2021leaper}
        % \nocite{undersub-singh2021qrator}
        % \nocite{undersub-arpan2021preciseNN}
        % \nocite{undersub-keerthana2021weather}
        % \nocite{undersub-alain2021stencil}
        
        % \defbibnote{myPrenote}{
        %  {\bf Under Submission:}
        % }
        % % \defbibnote{myPostnote}{
        % %     {\bf Co-Author:}
        % % }
        % \begin{refcontext}[sorting=ydndt]
        % \printbibliography[
        %   heading=none, 
        %     prenote=myPrenote
        %   ]
        % \end{refcontext}
        % \end{refsection}



\begin{refsection}
% If you print a bibliography within this section, only citations within this refsection will be printed.
% Option 1: Make nocite for all of your papers.
% Options 2 would be a seperate file which contains all of your papers.
\nocite{poster-singh2021leaper}
\nocite{poster-singh2021ISC}
\defbibnote{myPrenote}{
 {\bf Poster:}
}
% \defbibnote{myPostnote}{
%     {\bf Co-Author:}
% }

\printbibliography[sorting=none,
   heading=none, 
    prenote=myPrenote
  ]

\end{refsection}


    \begin{refsection}
    
        \nocite{patent}
        
        \defbibnote{myPrenote}{
         {\bf Patent:}
        }
        \printbibliography[sorting=none,
           heading=none, 
            prenote=myPrenote
          ]
    
    \end{refsection}


==> PhD_Thesis_Updated_arxiv (1)/package.tex <==
\usepackage{lgrind}
%% These have been added at the request of the MIT Libraries, because
%% some PDF conversions mess up the ligatures.  -LB, 1/22/2014
\usepackage{cmap}
\usepackage[T1]{fontenc}
\pagestyle{plain}
% \pagenumbering{roman}
\pagenumbering{roman}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{lmodern}
\usepackage[babel=true]{microtype}
\usepackage{graphicx}
\usepackage{bm} 
\usepackage{array} 
\usepackage{xspace}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{url} 
\usepackage{hhline}

\usepackage[normalem]{ulem}
\usepackage{booktabs}
\usepackage{makecell} 
\usepackage{titlesec} 
\usepackage{indentfirst} 
\usepackage{float} 
\usepackage{dblfloatfix} 
\usepackage{changepage} 
% \usepackage[algoruled,resetcount,linesnumbered,algpseudocode ]{algorithm2e}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\newcommand{\incircle}[1]{\raisebox{0.5pt}{\protect \textcircled{\raisebox{-0.8pt}{#1}}}}


\newcommand{\delete}[1]{{\color{red}\sout{}}}

\usepackage{multirow}
\usepackage{comment}

% \newcommand{\etal}{\textit{et al.}}



%\newcommand{\minesh}[1]{{\color{amber}#1}}
%\newcommand{\jk}[1]{{\color{blue}#1}}
%\newcommand{\jk}[1]{{\color{dollarbill}#1}}


%\newcommand{\jk}[1]{{\color{black}#1}}
%\newcommand{\jktwo}[1]{{\color{black}#1}}
%\newcommand{\minesh}[1]{{\color{black}#1}}
%\newcommand{\mptwo}[1]{{\color{black}#1}}
%\newcommand{\mpthree}[1]{{\color{black}#1}}
%\newcommand{\hasan}[1]{{\color{black}#1}}


\newcommand{\squeezeme}{ \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} }


\usepackage[nolessnomore, italic]{mathastext}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}

\usepackage{textcomp}

\usepackage{fancyhdr}
% \usepackage[hyphens]{url}
% \usepackage[utf8x]{inputenc} 
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\usepackage{upgreek} %for non-italic Greek alphabet
\usepackage{hhline}
% \usepackage[
%   paperwidth=17cm,
%   paperheight=24cm
%   % other options
% ]{geometry}
% \usepackage{colortbl}
% % Ensure letter paper
% \pdfpagewidth=8.5in
% \pdfpageheight=11in
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{enumitem}
% For editing
\newcommand{\js}[1]{{\color{black}{#1}}}
\newcommand{\nh}[1]{{\color{black}{#1}}}
\newcommand{\juan}[1]{{\color{black}{#1}}}
\newcommand{\todo}[1]{\textbf{\fcolorbox{black}{red}{\color{white}{TODO}}} \underline{$\overline{\hbox{\textcolor{red}{\emph{#1}}}}$}}
% \newcommand{\js}[1]{{\color{purple}{#1}}}
% \newcommand{\nh}[1]{{\color{green}{#1}}}
% \newcommand{\juan}[1]{{\color{blue}{#1}}}
% \newcommand{\todo}[1]{{\textcolor{red}{#1}}}

%sections, figures, tables
\newcommand{\sects}[1]{{Sections~#1}\xspace} % for referencing multiple sections
\newcommand{\sect}[1]{{Section~#1}\xspace} % for referencing a section
\newcommand{\figs}[1]{{Figures~#1}\xspace} % for referencing multiple figures
\newcommand{\fig}[1]{{Figure~#1}\xspace} % for referencing a figure
\newcommand{\tab}[1]{{Table~#1}\xspace} % for referencing a table
\newcommand{\head}[1]{{\noindent\textbf{#1.}\xspace}} % for heading of a paragraph


\usepackage{listings}
\usepackage[font=small,labelfont=bf,textfont={bf}]{caption}
% will apply to all subcaptions
\usepackage[labelfont=bf,textfont=normalfont,singlelinecheck=off,justification=centering]{subcaption}

% \usepackage[algoruled,resetcount,linesnumbered ]{algorithm2e}
 \usepackage{amsmath,amssymb,amsfonts}
 \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
% % \usepackage{textcomp}
% % \usepackage{xcolor}
% \usepackage{sidecap}
% \usepackage{enumitem}
% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%             \node[shape=circle,draw,inner sep=0pt,fill=black, text=white] (char) {#1};}}


\usepackage{booktabs} % For formal tables
\usepackage{textcomp}

\usepackage{balance}
\usepackage[rightcaption]{sidecap} % Caption on a side of figure
% Version header
\usepackage{fancyhdr}
\usepackage[us,12hr]{datetime}

% For page numbers:
%\pagestyle{plain}

\newcommand{\ignore}[1]{}

% Circles
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0pt,fill=black, text=white] (char) {#1};}}
\newcommand*\circledWhite[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0pt,fill=white, text=black] (char) {#1};}}

% \usepackage{array,graphicx}
\usepackage{grffile}
\usepackage{float}
\usepackage{svg}
\usepackage{pifont}
\usepackage{threeparttable}
\usepackage{graphics}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{verbatim}
\usepackage{booktabs}

\usepackage{dblfloatfix}
% Copyright
%\setcopyright{none}
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}



%commands by gagan
% \usepackage{soul,xcolor}
\usepackage{adjustbox}
\usepackage{diagbox}
% \usepackage[table,xcdraw]{xcolor}
% \usepackage{color, colortbl}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}

\newcommand{\gaganRemove}[1] {\st{#1}}
\definecolor{dred}{rgb}{255.00, 0.00, 0.00}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}%
\pagenumbering{gobble} % Remove page numbers
\definecolor{dred}{rgb}{0.75, 0.00, 0.00}

\definecolor{dgreen}{rgb}{0.00, 0.75, 0.00}
\definecolor{dpink}{rgb}{0.75, 0.0, 0.75}
\definecolor{dblack}{rgb}{0.00, 0.00, 0.00}
\definecolor{dblue}{rgb}{0.00, 0.00, 0.75}
\definecolor{gyell}{rgb}{0.5, 0.5, 0.0}
\definecolor{dbleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{navyblue}{rgb}{0.0, 0.0, 0.5}
\definecolor{forestgreen}{rgb}{0.13, 0.55, 0.13}

% \newcommand{\gaganF}[1]{{\color{dblue}TODO:#1}}
% \newcommand{\rakesh}[1]{{\color{dbleudefrance}#1}}
% \newcommand{\jgl}[1]{{\color{blue}JGL:#1}}

\newcommand{\gthesis}[1]{{\color{dblack}#1}}
\newcommand{\ggthesis}[1]{{\color{dblack}#1}}
\newcommand{\fc}[1]{{\color{dblack}#1}}
\newcommand{\ph}[1]{{\color{dblack}#1}}
\newcommand{\dd}[1]{{\color{dblack}#1}}
\newcommand{\ou}[1]{{\color{dblack}#1}}

\newcommand{\gcheck}[1]{{\color{dblack}#1}}
\newcommand{\gagan}[1]{{\color{dblack}#1}}
\newcommand{\gagann}[1]{{\color{black}#1}}
\newcommand{\gagannn}[1]{{\color{black}#1}}
\newcommand{\gaganH}[1]{{\color{black}#1}}
\newcommand{\rakesh}[1]{{\color{black}#1}}
\newcommand{\juang}[1]{{\color{black}#1}}
\newcommand{\juangg}[1]{{\color{black}#1}}
\newcommand{\juanggg}[1]{{\color{black}#1}}
\newcommand{\jgl}[1]{}
\usepackage{notoccite}
\newcommand{\hps}{\textsf{HPS}\xspace}
\newcommand{\cde}{\textsf{CDE}\xspace}
\newcommand{\slow}{\textsf{Slow-Only}\xspace}
\newcommand{\fast}{\textsf{Fast-Only}\xspace}
\newcommand{\oracle}{\textsf{Oracle}\xspace}

\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\q}{$Q(s,a)$}
\renewcommand\fbox{\fcolorbox{yellow}{white}}

% \usepackage{hyperref}
% Circles

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\include{pythonlisting}
\newcommand{\namePaper}{NERO\xspace} %TITLE
\newcommand{\nameQRator}{Sibyl\xspace} %TITLE
\newcommand{\nameNAPEL}{NAPEL\xspace} %TITLE
\newcommand{\nameLEAPER}{LEAPER\xspace} %TITLE
\newcommand{\nameNERO}{NERO\xspace} %TITLE
\newcommand{\namePreciseFPGA}{PreciseFPGA\xspace} %TITLE

\newcommand{\rl}{reinforcement learning\xspace} %rl
  %The following commands are the most basic for specifying a coordinate.
%\pgfpoint{<x coordinate>}{<y coordinate>}

% \pgftransformcm{<a>}{<b>}{<c>}{<d>}{<point>}
% Applies the transformation matrix given by a, b, c, and d and the shift <point> to coordinates (in addition to any previous transformations already in force).

\newcommand{\myGlobalTransformation}[2]
{
    \pgftransformcm{1}{0}{0.4}{0.5}{\pgfpoint{#1cm}{#2cm}}
}

% draw a 4x4 helper grid in 3D
% Input: point of origins x and y coordinate and additional drawing-parameters
\newcommand{\gridThreeD}[3]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
        \draw [#3] grid (5,5);
    \end{scope}
}
\newcommand\crule[3][black]{\textcolor{#1}{\rule{#2}{#3}}}


\newcommand{\gridThreeDSecond}[3]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
        \draw [#3] grid (3,3);
    \end{scope}
}

\newcommand{\gridThreeDThird}[3]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
        \draw [#3] grid (1,1);
    \end{scope}
}

\tikzstyle myBG=[line width=3pt,opacity=1.0]

% draws lines with white background to show which lines are closer to the
% viewer (Hint: draw from bottom up and from back to front)
%Input: start and end point
\newcommand{\drawLinewithBG}[2]
{
    \draw[white,myBG]  (#1) -- (#2);
    \draw[black,very thick] (#1) -- (#2);
}



%draws nodes of the grid
%Input: point of origins x and y coordinate


\newcommand{\dotesUpper}[2]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
   
     \node at (2.5,0.5) [circle,fill=black] {};
     \node at (1.5,1.5) [circle,fill=black] {};
    % \node at (2.5,1.5) [circle,fill=black] {}; %new
    \node at (3.5,1.5) [circle,fill=black] {};

     \node at (0.5,2.5) [circle,fill=black] {};
     % \node at (1.5,2.5) [circle,fill=black] {}; %new
      \node at (2.5,2.5) [circle,fill=black] {};
     % \node at (3.5,2.5) [circle,fill=black] {}; %new
      \node at (4.5,2.5) [circle,fill=black] {};
      \node at (1.5,3.5) [circle,fill=black] {};
     % \node at (2.5,3.5) [circle,fill=black] {};%new
         \node at (3.5,3.5) [circle,fill=black] {};
           \node at (2.5,4.5) [circle,fill=black] {};
                
                
                %this way circle of nodes will not be transformed
            
        
    \end{scope}
}


\newcommand{\lowerDots}[2]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
 
     \node at (0.5,1.5) [circle,fill=black] {};
      % \node at (-0.5,1.5) [circle,fill=black] {}; %new
       \node at (-1.5,1.5) [circle,fill=black] {};
          \node at (-0.5,0.5) [circle,fill=black] {};
           \node at (-0.5,2.5) [circle,fill=black] {};
             
                
                %this way circle of nodes will not be transformed
            
        
    \end{scope}
}

\newcommand{\lowestDot}[2]
{
    \begin{scope}
        \myGlobalTransformation{#1}{#2};
 
    \node at (0.5,1.5) [circle,fill=black] {};
      
             
                
                %this way circle of nodes will not be transformed
            
        
    \end{scope}
}
\usepackage[backend=biber,maxbibnames=99,style=ieee,citestyle=numeric,autocite=plain, giveninits,maxcitenames=99,sortfirstinits= true,sorting=nyt,dashed=false,sortcites=true]{biblatex} % load the package
%\AtBeginBibliography{\small} % setting font size of bibliography
\DeclareNameAlias{sortname}{family-given}
\DeclareNameAlias{author}{last-first} % last name first of bibliography
\bibliography{ref}
% \addbibresource{ref.bib} % add a bib-reference file
% \renewbibmacro{in:}{} % remove in from bibliography

\newcommand{\SubItem}[1]{
    {\setlength\itemindent{15pt} \item[-] #1}
}
\newcommand\like[1]{\begin{picture}(1,1)
\ifnum0=#1\put(.5,.35){\circle{1}}\else
\ifnum10=#1\put(.5,.35){\circle*{1}}\else
\put(.5,.35){\circle{1}}\put(.5,.35){\circle*{.#1}}
\fi\fi\end{picture}}

\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%




\newcommand{\hdiff}{\texttt{hdiff}\xspace}
\newcommand{\sevpoint}{\texttt{7-point}\xspace}
\newcommand{\tfivepoint}{\texttt{25-point}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%ADDED FROM PRECISENN%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bitwidth}{{bitwidth}\xspace }
\newcommand{\integer}{\texttt{integer}\xspace } %TITLE
\newcommand{\fractional}{\texttt{fractional}\xspace } %TITLE
\newcommand{\cmark}{\ding{51}\xspace}%
\newcommand{\xmark}{\ding{55}\xspace}%

% \usepackage[nottoc,numbib]{tocbibind}
\usepackage[nottoc,notlot,notlof]{tocbibind}
%USE H to hide a column
\usepackage{array}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\newlength\mylen
\newcommand\myinput[1]{%
  \settowidth\mylen{\KwIn{}}%
  \setlength\hangindent{\mylen}%
  \hspace*{\mylen}#1\\}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%below is to add footer in chapter without mark
\newcommand{\chapternote}[1]{{%
  \let\thempfn\relax% Remove footnote number printing mechanism
  \footnotetext[0]{{#1}}% Print footnote text
}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%addjust the spacing in list of tables
% \usepackage{hyperref}
% \hypersetup{pdftex,colorlinks=true,allcolors=blue}
% \usepackage{hypcap}

\usepackage[]{hyperref}
\hypersetup{
    pdftitle={Designing, Modeling, and Optimizing Data-Intensive Computing Systems},
    pdfauthor={Gagandeep Singh},
    % pdfsubject={Your subject here},
    % pdfkeywords={keyword1, keyword2},
    bookmarksnumbered=true,     
    % bookmarksopen=true,         
    % bookmarksopenlevel=1,       
    % colorlinks=true,            
    pdfstartview=Fit,           
    pdfpagemode=UseOutlines    % this is the option you were lookin for
    % pdfpagelayout=TwoPageRight
}

\usepackage{nicematrix}


 \aboverulesep=0ex
 \belowrulesep=0ex
%  \let\savehline\hline
% \def\hline{\noalign{\vskip3pt}\savehline\noalign{\vskip3pt}}

%%%%%%%%%%%%%%%%%%%%%%%remove discontinuous row and column lines
\usepackage{bigstrut}
    \setlength\bigstrutjot{3pt}
    
    
\makeatletter
\newlength\mylena
\newlength\mylenb
\newcommand\mystrut[1][2]{%
    \setlength\mylena{#1\ht\@arstrutbox}%
    \setlength\mylenb{#1\dp\@arstrutbox}%
    \rule[\mylenb]{0pt}{\mylena}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%sort based on first name
% \DeclareSortingNamekeyScheme{
%   \keypart{
%     \namepart{given}
%   }
%   \keypart{
%     \namepart{prefix}
%   }
%   \keypart{
%     \namepart{family}
%   }
%   \keypart{
%     \namepart{suffix}
%   }
% }


% \DeclareNameAlias{sortname}{default}
% \renewcommand{\bibopenparen}{\addcomma\addspace}
% \renewcommand{\bibcloseparen}{.\addspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%sort descending order based on year
\DeclareSortingTemplate{ydndt}{
  \sort{
    \field{presort}
  }
  \sort[final]{
    \field{sortkey}
  }
  \sort[direction=descending]{
    \field{sortyear}
    \field{year}
    \literal{9999}
  }
  \sort[direction=descending]{
    \field{sortname}
    \field{author}
    \field{editor}
    \field{translator}
    \field{sorttitle}
    \field{title}
  }
  \sort{
    \field{sorttitle}
    \field{title}
  }
}

% \usepackage{nicematrix}
% \usepackage{xcolor}
% \usepackage{amssymb}
% \usepackage{geometry}

% \usepackage{tikz}
% \usetikzlibrary{matrix}

% \usepackage{xcolor}
% \definecolor{mygray}{HTML}{C0C0C0}
% \definecolor{mylightgray}{HTML}{EFEFEF}
% \definecolor{myred}{HTML}{FD6864}
% \definecolor{mylightred}{HTML}{FFCCC9}
% \definecolor{myyellow}{HTML}{F6DB53}
% \definecolor{mylightyellow}{HTML}{FDF0AD}
% \definecolor{mygreen}{HTML}{77CA5C}
% \definecolor{mylightgreen}{HTML}{CFEAC6}
% \definecolor{mypurple}{HTML}{CDA7F6}
% \definecolor{mylightpurple}{HTML}{F2E7FD}
\usepackage{color, colortbl}
\definecolor{Gray}{gray}{0.9}
\usepackage[first=0,last=9]{lcg}
\newcommand{\ra}{\rand0.\arabic{rand}}

\newcommand{\gh}[1]{{\color{black}#1}}
\newcommand{\go}[1]{{\color{black}#1}}
\newcommand{\goo}[1]{{\color{black}#1}}
\newcommand{\gup}[1]{{\color{black}#1}}
\newcommand{\gca}[1]{{\color{black}#1}}
\newcommand{\rakeshisca}[1]{{\color{black}#1}}
\crefformat{section}{\S#2#1#3} % see manual of cleveref, section 8.2.1

\newcommand{\gsa}[1]{{\color{black}#1}}
\newcommand{\gor}[1]{{\color{black}#1}}
%first round
\newcommand{\gf}[1]{{\color{black}#1}}

\newcommand{\gon}[1]{{\color{black}#1}}
\newcommand{\gonn}[1]{{\color{black}#1}}
%second round
\newcommand{\gont}[1]{{\color{black}#1}}
%third round
\newcommand{\gonff}[1]{{\color{black}#1}}
\newcommand{\gonz}[1]{{\color{black}#1}}
\newcommand{\gonx}[1]{{\color{black}#1}}
\newcommand{\gaganF}[1]{[{\color{magenta}GAGAN:#1}]}

\newcommand{\gaganup}[1]{{\color{black}#1}}
\newcommand{\ghpca}[1]{{\color{black}#1}}
\newcommand{\grev}[1]{{\color{black}#1}}
\newcommand{\grahul}[1]{{\color{black}#1}}
\newcommand{\grakesh}[1]{{\color{black}#1}}

\newcommand{\gonf}[1]{{\color{black}#1}}
\newcommand{\rcam}[1]{{\color{black}#1}}
\newcommand{\rcamfix}[1]{{\color{black}#1}}
\newcommand{\rncam}[1]{{\color{black}#1}}
\newcommand{\rnlast}[1]{{\color{black}#1}}
\newcommand{\rbc}[1]{{\color{black}#1}}
\newcommand{\rakeshhpca}[1]{{\color{black}#1}}

\newcommand{\gonzz}[1]{{\color{black}#1}}
\newcommand{\jgll}[1]{{\color{ddgreen}\textbf{\textit{JGL: #1}}}}

\newcommand{\juancr}[1]{{\color{black}{#1}}}

\newcommand{\hlssd}{\textsf{$H\&L$}\xspace}
\newcommand{\hmssd}{\textsf{$H\&M$}\xspace}
\definecolor{NavyBlue}{rgb}{0.19, 0.55, 0.91}
\newcommand{\comm}[1]{{\color{NavyBlue}#1}}
\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill\fontsize{5.8}{6}\selectfont$\triangleright$ {\textcolor{blue}{#1}}\egroup}
\newcommand{\arcc}{\textsf{Archivist}\xspace}
\newcommand{\kleio}{\textsf{RNN-HSS}\xspace}
\newcommand{\sibyldef}{\textsf{Sibyl$_{Def}$}\xspace}
\newcommand{\sibylopt}{\textsf{Sibyl$_{Opt}$}\xspace}
\newcommand{\thhdd}{\textsf{H$_{SSD}$\&M$_{SSD}$\&L$_{HDD}$}}
\newcommand{\thssd}{\textsf{H$_{SSD}$\&M$_{SSD}$\&L$_{SSD}$}}
\newcommand{\thold}{\textsf{$H\&M\&L$}}
\newcommand{\thnew}{\textsf{$H\&M\&L_{SSD}$}}
\newcommand{\accessinterval}{\textsf{r$_{t}$}}
\newcommand{\accessfrequency}{\textsf{f$_{t}$}}
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
\newcommand*\circleds[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=-0.5pt,fill=black, text=white] (char) {#1};}}
\newcommand\mixfive{\textsf{$mix\_5$}\xspace}
\newcommand\mix{\textsf{$mix\_1$}\xspace}
\newcommand\hmone{\textsf{$hm\_1$}\xspace}
\newcommand\stg{\textsf{$stg\_0$}\xspace}
\newcommand\proxy{\textsf{$prxy\_0$}\xspace}
\newcommand\prn{\textsf{$prn\_1$}\xspace}
\newcommand\proj{\textsf{$proj\_1$}\xspace}
\newcommand\mds{\textsf{$mds\_1$}\xspace}
\newcommand\usr{\textsf{$usr\_1$}\xspace}
\newcommand\yc[1]{\textsf{YCSB-#1}\xspace}


==> PhD_Thesis_Updated_arxiv (1)/table_methods.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
% \renewcommand{\arraystretch}{0.9}
% 
\caption[List of contributions and methods used to achieve the thesis statement]{We highlight across five contributions nine different methods (concepts) used in this dissertation to achieve the thesis statement of handling data well. We make use of two guiding principles: (1) \textit{data-centric} (DC) is bringing processing closer to where data resides and ensuring that data does not overwhelm system components; (2) \textit{data-driven} (DD) is leveraging data to perform architectural decisions or predictions
\label{tab:intro/methods}}
\centering
\HUGE
\renewcommand{\arraystretch}{0.8}
\setlength{\arrayrulewidth}{2pt}
\setlength{\tabcolsep}{10pt}
% \setlength{\arrayrulewidth}{1mm}
% \arrayrulecolor[HTML]{black}
\resizebox{1\linewidth}{!}{
% \begin{NiceTabular}{lllllll}
\begin{tabular}{l|l|l|Hl|l|l}
\toprule 
% \textbf{\diagbox[width=9em]{Methods}{Contribution}}    
% \rule{0pt}{32pt} & \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
\rule{0pt}{32pt}& \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
\textbf{METHODS} & \textbf{NERO~\cite{singh2020nero}}                                                                                                   & \textbf{Low Precision~\cite{singh2019low}}                                                                                        & \textbf{PreciseFPGA~\cite{not_published_arpan2021preciseNN}}                                                                                      & \textbf{NAPEL~\cite{NAPEL}}                                                                                       & \textbf{LEAPER~\cite{singh2021leaper_fpga}}                                                                                                                 & \textbf{Sibyl~\cite{not_published_singh2021qrator}}                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\textbf{Specialization} (DC)                                                                          &  \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}    &                                             \begin{tabular}[c]{@{}l@{}}Implementation on\\an FPGA for fixed-\\point and floating-\\point representation\end{tabular}                                                                                                                 & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                         &                                                                                                      & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                                               &                                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Revisit memory}\\\textbf{hierarchy} (DC)       \end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}Scratchpad-based\\ hybrid memory\end{tabular}                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Tiered hybrid\\storage system\end{tabular}                             \\ \hline 
\rowcolor[HTML]{DCDCDC}
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Reducing copies}\\\textbf{between host and}\\\textbf{accelerator} (DC)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Shared memory \\space    \end{tabular}                                                                                             & Quantize data                                                                                                 & Quantize data                                                                                             &                                                                                                      &                                                                                                                                 &                                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut   
\begin{tabular}[c]{@{}l@{}}\textbf{Dataflow} \\ \textbf{architecture} (DC)     \end{tabular}                                                                                   & Task pipelining                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 &                                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Near-memory}\\\textbf{computing} (DC)    \end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}}{Processing near-}\\{high-bandwidth} \\{memory}   \end{tabular}                                                                                            &                                                                                                               &                                                                                                           & \begin{tabular}[c]{@{}l@{}}Processing near-\\3D stacked memory \end{tabular}                           &                                                                                                                                 &                                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut   
\begin{tabular}[c]{@{}l@{}}\textbf{Reducing memory}\\ \textbf{footprint} (DC)     \end{tabular}                                                          &                                                                                                          \begin{tabular}[c]{@{}l@{}}Single and half\\floating-point\\precision \end{tabular}        & \begin{tabular}[c]{@{}l@{}}Different number \\ representations--\\ posit, fixed-point,\\and floating-point\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Automatic\\ quantization of \\ fixed-point\\ representation\end{tabular} &                                                                                                      &                                                                                                                                 &                                                                                                   \\ \hline 
\rowcolor{gray!45} 
\mystrut  
\textbf{Static ML} (DD)                                                                 &                                                                                                                 &                                                                                                               &                                             \begin{tabular}[c]{@{}l@{}}Learns resource\\ and power\\utilization\end{tabular}                                                                &\begin{tabular}[c]{@{}l@{}}Learns application\\ performance and\\ energy consumption\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Learns resource\\ utilization and\\ performance\\ models\end{tabular}                                    &         
\\\hline 
\rowcolor{gray!45} 
\mystrut  
%\\\specialrule{.05em}{.05em}{.05em} 
\begin{tabular}[c]{@{}l@{}}\textbf{Speed up design} \\ \textbf{space exploration}\\  (DD)\end{tabular}         &    \begin{tabular}[c]{@{}l@{}}Auto-tuning\\for data transfer\\window size\end{tabular}                                                                                                                      &                                                                                                               & Supervised ML                                                                                                  & \begin{tabular}[c]{@{}l@{}}Supervised ML,\\Design of \\ experiment\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Few-shot\\learning\end{tabular}                                                                                                           &                           \begin{tabular}[c]{@{}l@{}}Design of\\experiment\end{tabular}                                                                            \\\hline 
\rowcolor{gray!45}
\mystrut  
\textbf{Dynamic ML} (DD)                                                          &                                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Reinforcement\\ Learning\end{tabular}                                                                             \\ \hline 
\mystrut  
\textbf{Goal}                                                                                & {\begin{tabular}[c]{@{}l@{}}Overcome memory\\bottleneck of\\weather prediction\\ application\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Investigate\\ computationally\\ cheaper number\\ representations\end{tabular}} &   {\begin{tabular}[c]{@{}l@{}}Automate DSE\\ for fixed-point\\ representation\end{tabular}}                                                                                  & {\begin{tabular}[c]{@{}l@{}}Quick performance\\ and energy\\ estimates of new \\ applications\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Quick area and\\ performance\\ estimates on\\ new high-end \\FPGA-based \\platforms\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Efficient and \\ high performance\\data placement \\mechanism\end{tabular}} \\ \bottomrule
% \specialrule{.05em}{.05em}{.05em} 
\end{tabular}
%\end{NiceTabular}
}
\end{table}


% \begin{table}
% \centering
% \begin{NiceTabular}{wl{2.2cm}CCC}[hvlines,code-before = \cellcolor{lightgray}{2-4,3-3,4-2,4-4}]
% \rule[-3mm]{0pt}{9mm}
% \diagbox{Enhed}{Interface} & ED    & DDG   & \textit{Server}  \\
%   ED                       & \checkmark    & \checkmark     &  \\
%  DDG                       & \checkmark    &                & \checkmark \\
%  \textit{Server}           &               & \checkmark     & \\
% \end{NiceTabular}
% \caption{Oversigt over interfaces mellem enhederne.}
% \label{tab:interfacesMellemEnheder}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcolumntype{g}{>{\columncolor{Gray}}c}
% \begin{table}[ht]
% \centering
% \HUGE
% \renewcommand{\arraystretch}{0.8}
% \setlength{\arrayrulewidth}{2pt}
% \setlength{\tabcolsep}{10pt}
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{g|g|g|g|g|g|g}
% \hline
% \rowcolor{white}
% % \textbf{\diagbox[width=9em]{Methods}{Contribution}}    
% % \rule{0pt}{32pt} & \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
% \rule{0pt}{32pt}& \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
% \rowcolor{white}
% \textbf{METHODS} & \textbf{NERO~\cite{singh2020nero}}                                                                                                   & \textbf{Low Precision~\cite{singh2019low}}                                                                                        & \textbf{PreciseFPGA~\cite{not_published_arpan2021preciseNN}}                                                                                      & \textbf{NAPEL~\cite{NAPEL}}                                                                                       & \textbf{LEAPER~\cite{singh2021leaper_fpga}}                                                                                                                 & \textbf{QRator~\cite{not_published_singh2021qrator}}                                                                                   \\ \hline 
% \mystrut  
% \rowcolor[HTML]{DCDCDC} 
% \textbf{Specialization} (DC)                                                                          &  \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}    &                                             \begin{tabular}[c]{@{}l@{}}Implementation on\\an FPGA for fixed-\\point and floating-\\point representation\end{tabular}                                                                                                                 & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                         &                                                                                                      & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                                               &                                                                                                   \\\hline 
% \mystrut  
% \rowcolor[HTML]{DCDCDC} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Revisit memory}\\\textbf{hierarchy} (DC)       \end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}Scratchpad-based\\ hybrid memory\end{tabular}                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Tiered\\ hybrid storage\end{tabular}                             \\\hline 
% \mystrut  
% \rowcolor[HTML]{DCDCDC} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Reducing copies}\\\textbf{between host and}\\\textbf{accelerator} (DC)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Shared memory \\space    \end{tabular}                                                                                             & Quantize data                                                                                                 & Quantize data                                                                                             &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
% \mystrut   
% \rowcolor[HTML]{DCDCDC} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Dataflow} \\ \textbf{architecture} (DC)     \end{tabular}                                                                                   & Task pipelining                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
% \mystrut  
% \rowcolor[HTML]{DCDCDC} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Near-memory}\\\textbf{computing} (DC)    \end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}}{Processing near-}\\{high-bandwidth} \\{memory}   \end{tabular}                                                                                            &                                                                                                               &                                                                                                           & \begin{tabular}[c]{@{}l@{}}Processing near-\\3D stacked memory \end{tabular}                           &                                                                                                                                 &                                                                                                   \\\hline 
% \rowcolor[HTML]{DCDCDC} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Reducing memory}\\ \textbf{footprint} (DC)     \end{tabular}                                                          &                                                                                                          \begin{tabular}[c]{@{}l@{}}Single and half\\floating-point\\precision \end{tabular}        & \begin{tabular}[c]{@{}l@{}}Different number \\ representations--\\ posit, fixed-point,\\and floating-point\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Automatic\\ quantization of \\ fixed-point\\ representation\end{tabular} &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
% \rowcolor{gray!45} 
% \textbf{Static ML} (DD)                                                                 &                                                                                                                 &                                                                                                               &                                             \begin{tabular}[c]{@{}l@{}}Learns resource\\ and power\\utilization\end{tabular}                                                                &\begin{tabular}[c]{@{}l@{}}Learns application\\ performance and\\ energy consumption\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Learns resource\\ utilization and\\ performance\\ models\end{tabular}                                    &         
% \\\hline 
% %\\\specialrule{.05em}{.05em}{.05em} 
% \rowcolor{gray!45} 
% \begin{tabular}[c]{@{}l@{}}\textbf{Speed up design} \\ \textbf{space exploration}\\  (DD)\end{tabular}         &    \begin{tabular}[c]{@{}l@{}}Auto-tuning\\for data transfer\\window size\end{tabular}                                                                                                                      &                                                                                                               & Supervised ML                                                                                                  & \begin{tabular}[c]{@{}l@{}}Supervised ML,\\Design of \\ experiment\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Few-shot\\learning\end{tabular}                                                                                                           &                           \begin{tabular}[c]{@{}l@{}}Design of\\experiment\end{tabular}                                                                            \\\hline 
% \rowcolor{gray!45}
% \textbf{Dynamic ML} (DD)                                                          &                                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Reinforcement\\ Learning\end{tabular}                                                                             \\ \hline 
% \rowcolor{white}
% \textbf{Goal}                                                                                & {\begin{tabular}[c]{@{}l@{}}Overcome memory\\bottleneck of\\weather prediction\\ application\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Investigate\\ computationally\\ cheaper number\\ representations\end{tabular}} &   {\begin{tabular}[c]{@{}l@{}}Automate DSE\\ for fixed-point\\ representation\end{tabular}}                                                                                  & {\begin{tabular}[c]{@{}l@{}}Quick performance\\ and energy\\ estimates of new \\ applications\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Quick area and\\ performance\\ estimates on\\ new high-end \\FPGA-based \\platforms\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Low cost\\ but high\\ performance\\storage sub-\\system\end{tabular}} \\ \specialrule{.05em}{.05em}{.05em} 
% \end{tabular}
% }
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> PhD_Thesis_Updated_arxiv (1)/table_methods_end.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
% \renewcommand{\arraystretch}{0.9}
% 
\caption[List of contributions and methods used to achieve the thesis statement]{We highlight across five contributions nine different methods (concepts) used in this dissertation to achieve the thesis statement of handling data well. We make use of two guiding principles: (1) \textit{data-centric} (DC) is bringing processing closer to where data resides and ensuring that data does not overwhelm system components; (2) \textit{data-driven} (DD) is leveraging data to perform architectural decisions or predictions.
\label{tab:intro/methods_end}}
\centering
\HUGE
\renewcommand{\arraystretch}{0.8}
\setlength{\arrayrulewidth}{2pt}
\setlength{\tabcolsep}{10pt}
% \setlength{\arrayrulewidth}{1mm}
% \arrayrulecolor[HTML]{black}
\resizebox{1\linewidth}{!}{
% \begin{NiceTabular}{lllllll}
\begin{tabular}{l|l|l|Hl|l|l}
\toprule 
% \textbf{\diagbox[width=9em]{Methods}{Contribution}}    
% \rule{0pt}{32pt} & \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
\rule{0pt}{32pt}& \multicolumn{5}{c}{\textbf{CONTRIBUTIONS}} \\ \cmidrule{2-7} 
\textbf{METHODS} & \textbf{NERO~\cite{singh2020nero}}                                                                                                   & \textbf{Low Precision~\cite{singh2019low}}                                                                                        & \textbf{PreciseFPGA~\cite{not_published_arpan2021preciseNN}}                                                                                      & \textbf{NAPEL~\cite{NAPEL}}                                                                                       & \textbf{LEAPER~\cite{singh2021leaper_fpga}}                                                                                                                 & \textbf{Sibyl~\cite{not_published_singh2021qrator}}                                                                                   \\ \hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\textbf{Specialization} (DC)                                                                          &  \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}    &                                             \begin{tabular}[c]{@{}l@{}}Implementation on\\an FPGA for fixed-\\point and floating-\\point representation\end{tabular}                                                                                                                 & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                         &                                                                                                      & \begin{tabular}[c]{@{}l@{}}FPGA-based \\ accelerator\end{tabular}                                                               &                                                                                                   \\\hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Revisit memory}\\\textbf{hierarchy} (DC)       \end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}Scratchpad-based\\ hybrid memory\end{tabular}                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Tiered hybrid\\storage system\end{tabular}                             \\\hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Reducing copies}\\\textbf{between host and}\\\textbf{accelerator} (DC)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Shared memory \\space    \end{tabular}                                                                                             & Quantize data                                                                                                 & Quantize data                                                                                             &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut   
\begin{tabular}[c]{@{}l@{}}\textbf{Dataflow} \\ \textbf{architecture} (DC)     \end{tabular}                                                                                   & Task pipelining                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut  
\begin{tabular}[c]{@{}l@{}}\textbf{Near-memory}\\\textbf{computing} (DC)    \end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}}{Processing near-}\\{high-bandwidth} \\{memory}   \end{tabular}                                                                                            &                                                                                                               &                                                                                                           & \begin{tabular}[c]{@{}l@{}}Processing near-\\3D stacked memory \end{tabular}                           &                                                                                                                                 &                                                                                                   \\\hline 
\rowcolor[HTML]{DCDCDC} 
\mystrut   
\begin{tabular}[c]{@{}l@{}}\textbf{Reducing memory}\\ \textbf{footprint} (DC)     \end{tabular}                                                          &                                                                                                          \begin{tabular}[c]{@{}l@{}}Single and half\\floating-point\\precision \end{tabular}        & \begin{tabular}[c]{@{}l@{}}Different number \\ representations--\\ posit, fixed-point,\\and floating-point\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Automatic\\ quantization of \\ fixed-point\\ representation\end{tabular} &                                                                                                      &                                                                                                                                 &                                                                                                   \\\hline 
\rowcolor{gray!45} 
\mystrut  
\textbf{Static ML} (DD)                                                                 &                                                                                                                 &                                                                                                               &                                             \begin{tabular}[c]{@{}l@{}}Learns resource\\ and power\\utilization\end{tabular}                                                                &\begin{tabular}[c]{@{}l@{}}Learns application\\ performance and\\ energy consumption\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}Learns resource\\ utilization and\\ performance\\ models\end{tabular}                                    &         
\\\hline 
\rowcolor{gray!45} 
\mystrut  
%\\\specialrule{.05em}{.05em}{.05em} 
\begin{tabular}[c]{@{}l@{}}\textbf{Speed up design} \\ \textbf{space exploration}\\  (DD)\end{tabular}         &    \begin{tabular}[c]{@{}l@{}}Auto-tuning\\for data transfer\\window size\end{tabular}                                                                                                                      &                                                                                                               & Supervised ML                                                                                                  & \begin{tabular}[c]{@{}l@{}}Supervised ML,\\Design of \\ experiment\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Few-shot\\learning\end{tabular}                                                                                                           &                           \begin{tabular}[c]{@{}l@{}}Design of\\experiment\end{tabular}                                                                            \\\hline 
\rowcolor{gray!45}
\mystrut  
\textbf{Dynamic ML} (DD)                                                          &                                                                                                                 &                                                                                                               &                                                                                                           &                                                                                                      &                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Reinforcement\\ Learning\end{tabular}                                                                             \\ \hline 
\mystrut  
\textbf{Goal}                                                                                & {\begin{tabular}[c]{@{}l@{}}Overcome memory\\bottleneck of\\weather prediction\\ application\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Investigate\\ computationally\\ cheaper number\\ representations\end{tabular}} &   {\begin{tabular}[c]{@{}l@{}}Automate DSE\\ for fixed-point\\ representation\end{tabular}}                                                                                  & {\begin{tabular}[c]{@{}l@{}}Quick performance\\ and energy\\ estimates of new \\ applications\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Quick area and\\ performance\\ estimates on\\ new high-end \\FPGA-based \\platforms\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}Efficient and \\ high performance\\data placement \\mechanism\end{tabular}} \\ \bottomrule
\end{tabular}
%\end{NiceTabular}
}
\end{table}

==> PreciseNN/sections/abstract.tex <==

\begin{abstract}

% Edge-devices have hard power, bandwidth, memory, and performance constraints because of which resource-efficient accelerator design is critical to deploy  Machine  Learning solutions on the edge.  Lower precision fixed-point-implementations on FPGAs can provide tremendous resource savings by leveraging the arbitrary-precision capability of an  FPGA. However,   optimal-precision-search in a resource-constrained device is a challenging task because of the huge design-space and the time-consuming FPGA design-cycle. To this end, we propose PreciseNN,  a  novel solution to the optimal-precision-calculation for resource-constrained edge-FPGA devices.  Experimental results show that  PreciseNN delivers,  on average,  95\%  accuracy and reduces the design-space exploration time by $\sim\mathbf{500\times}$ over exhaustive search.
% \jgl{By only reading the abstract it is impossible to understand what this work is about.}
% \jgl{Use this flow: 1. NNs can use fixed-point arithmetic. Reduced precision can be enough. 2. Using reduced fixed-point precisions can be beneficial in edge devices with FPGAs, since they are resource constrained. 3. However, determining the optimal precision is challenging (define what optimal precision means). It requires time-consuming design space exploration. 4. Our key idea is to use an ML-based prediction framework to find what is the optimal precision. 5. We present PreciseNN... 6. Explain results.}
% \arpan{this is not entirely ML based framework. Modified accordingly.}

% \jgl{I've tried to propose a better organization. Use the same flow in the introduction.}

% \arpan{Does this look better?
% Neural  Networks  (NN)  can use lower \gagan{precision} fixed-point \gagan{representation} to perform inference with acceptable accuracy.   Reduced fixed-point precision, compared to floating-point can provide savings in resource and power consumption which can be beneficial to deploy NN models on resource-constrained edge-FPGA-devices. However, finding optimal precision w.r.t. accuracy and power is a  challenging task because of the huge design-space and the time-consuming FPGA design-cycle. Our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle. To this end, we propose PreciseNN, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that PreciseNN delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search.
% }

\gagan{Low precision formats for neural network inference offer a resource-efficient alternative to single-precision floating point implementation. %A reduced precision implementation provides savings in resource and power consumption with minimal accuracy loss. Such implementations can allow for easy deployment of accelerators on resource-constrained FPGA-based edge devices. 
However, determining the optimal precision in terms of accuracy and power is challenging because of the following two reasons: (1) the design space of choices makes it infeasible to perform an exhaustive manual-tuning; and (2) FPGAs have a slow downstream implementation process.  To this end, we propose \namePaper, a novel solution for the optimal-precision-evaluation for edge-FPGA-devices. Our key idea is to use a prediction-based framework to obtain optimal-precision with a reduced design-cycle time to overcome these issues. Experimental results show that \namePaper~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\mathbf{500\times}$ over exhaustive search.  }
% \gagan{Neural  Network  (NN) parameter can be used with reduced \gagan{precision} to perform inference with an acceptable accuracy. A reduced precision implementation provides savings in terms of resource and power consumption. Such implementations can allow for easy deployment of accelerators on edge devices with FPGAs, which  are often constrained by the available computational resources. However, determining the optimal precision in terms of accuracy and power is challenging because of the following two reasons: (1) the design space of choices is infeasible to perform exhaustive manual-tuning; and (2) FPGAs have a slow downstream implementation process. To overcome these issues, our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle time. To this end, we propose \namePaper, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that \namePaper~delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search.  }

% \gagan{Fixed point arithmetic for neural network (NN) implementation provides a trade-off
% between  accuracy and  computational complexity. NNs can tolerate lower precision computation that allows for  easy deployment these accelerators in edge devices with FPGAs. These devices are often constrained by the available computational resources. However, determining the optimal precision in terms of accuracy and power is challenging because of following two reasons. First, the design space of choices is infeasible to perform manual-tuning. Second, FPGAs have long downstream implementation process. To overcome these issues, our key idea is to use a prediction framework to obtain optimal-precision with a reduced design-cycle. To this end, we propose PreciseNN, a novel solution to the optimal-precision-calculation for edge-FPGA-devices. Experimental results show that PreciseNN delivers,  on average,  95\%  prediction-accuracy and reduces the design-space exploration-time by $\sim\mathbf{500\times}$ over exhaustive search. }
\end{abstract}

==> PreciseNN/sections/background.tex <==
% \vspace{-0.1 cm}
\section{Background}\label{background}
% \begin{Background}
% \gagan{Deep Neural Networks are used to solve a range of tasks including image processing, speech recognition, and natural language processing. However, these networks require a vast amount of computing resources that limits its applicability. To overcome this issue,  we quantize\cite{fixed-point-compression, quant_han2016deep,quant_zhou2017incremental, fixed-point-hw} these networks to reduced precision, taking advantage of inherent error resilience of deep neural networks. To quantize these networks, we make use of reduced precision fixed-point representation that reduces the resource overhead for these networks. 


% \vspace{-0.1 cm}
% \subsection{Fixed-Point Arithmetic}

% In current computing system, IEEE-754 floating-point representation is used as the \textit{de-facto} standard for real numbers representation~\cite{singh2019low}. The floating-point number consists of mantissa, exponent, and an additional bit for the sign. Floating numbers provide a big dynamic range %that enables its application \todo{change} 
% that enables single data to undergo a long sequence of calculations. 
% On the other hand, the fixed-point number has dedicated a number of bits to represent integer part and fraction part. A commonly used fixed-point configuration is denoted by $<x,y>$ where $x$ represents the \bitwidth and $y$ represents the number of dedicated bits used to represent integer part. Even though floating-point operations are better in providing a better dynamic range compared to fixed-point, many applications do not need this dynamic range. Prior works\cite{cnn_approx, dnn_approx, xilinx_wp_int4, xilinx_wp_int8,singh2019low} have shown that applications such as Convolutional Neural Network (CNN) can work well with 8 bit or lower precision with acceptable error.
% \vspace{-0.1 cm}
% \subsection{Fixed-Point Implementation on FPGA}
% FPGAs are being widely used because of their capability to provide massive parallelism and reconfigurability. FPGAs have limited resources where the application performance is also a function of resource utilization. The number of computational units that can be mapped onto an accelerator is key to exploiting maximum parallelism possible from these FPGA devices. In FPGAs the use of lower precision fixed-point data type can be beneficial in terms of power and resource consumption\cite{xilinx_wp_float_to_fixed}. Compared to floating-point precision, reduced fixed-point has two main advantages. First, fixed-point arithmetic requires lower operand width thus fewer logic units, such as DSP (digital signal processing) units\cite{xilinx_dsp}. Second, reduced precision fixed-point requires smaller \bitwidth thus requiring less memory footprint\cite{guptaetal}\cite{fixed-point-hw}\cite{fixed-point-ternary}. Thus, replacing floating-point by reduced precision fixed-point leads to the reduction in area, power and cost\cite{8bit_approx}. In turn allows us to put more compute units within the same device. %Additionally, floating-point to fixed-point conversion support offered for FPGAs by High-Level Synthesis Tools makes this conversion effortless. \jgl{And these tools can be used in FPGA design?\addressed{yes}}


% Even though reduced fixed-point arithmetic has many advantages over floating-point arithmetic, the inference accuracy of a NN model depends largely on the fixed-point configuration\footnote{An optimal fixed-point configuration for an application is defined as the fixed-point configuration for which the application uses minimum power while keeping the application inference accuracy in acceptable range.}.  On one hand, reducing the \bitwidth can provide significant saving in resources and power but it can have detrimental effect on the inference accuracy (ref. Section~\ref{motivation}). So its critical to obtain the fixed-point configuration that can enable an application to operate at an acceptable error while adhering to memory, power, and resource budgets. 
\vspace{-0.1 cm}
\subsection{FPGA design-cycle}
FPGA design cycle consists of three main stages: (1) C-Synthesis\cite{xilinx_hls}\cite{xilinx_hls_tutorial}; (2) RTL Synthesis\cite{xilinx_synth}; and (3) Implementation\cite{xilinx_impl}. After implementation stage, a bitstream (executable) is generated that can be deployed on an FPGA. At every stage of the design-cycle design report ( Section~\ref{hls_report} ), containing the resource utilization and latency estimates, is generated. 



The most accurate estimates are generated after the final implementation stage, thus are the most reliable results. However, the complete downstream process can take several hours for a single design point. To find the optimal fixed-point configuration for an application we need to exhaustively search over all possible fixed-point configurations. This approach quickly becomes intractable and infeasible in case of FPGAs. For example, to obtain optimal fixed-point configuration compared to baseline floating-point ($bitwidth=32$) we require the post-implementation run results for $bitwidth\leq 32$ and $1\leq integer < 32$, for a total of 496 configurations for a single model. An exhaustive search for all configurations  can  easily take from hours to days to even weeks. Due to this high runtime incurred in the FPGA design cycle, it is not practical to run the entire FPGA design cycle exhaustively to find a Pareto-optimal solution. 

 



 
 %%%%%%%%%%%%%%%%%%%%
%  This requires design exploration in the order of $O(n^2)$ for $bitwidth\leq n$. For an example, in order to obtain optimal configuration for $bitwidth\leq 32$ and $1\leq integer < 32$ we require 496 ( \ref{motivation} )\jgl{Refer to section, not equation\addressed{}}  implementation runs which can take hours to even days. 
 
 
%  In FPGA finding optimal fixed-point configuration for an application requires an exhaustive search through all the possible fixed-point configuration. To search the optimal fixed-point configuration compared to baseline floating point requires exhaustive search over 496 configurations. Thus, in FPGA the search space requires to run 496 implementation runs in total, to obtain the resource utilization and power utilization numbers. Implementation runs in FPGA for these 496 configurations can take significant time which can vary from hours to days to even weeks. Thus, its not practical to perform the exhaustive search to obtain the optimal fixed-point configuration. 



% The logic required to implement a given floating-point operation is more compared to fixed-point arithmetic. \gagan{This causes the floating-point implementation to be costly on hardware resources and from both latency and power aspects. }


% \jgl{Start this section with NNs. Then, talk about floating-point. Then, talk about fixed-point and its benefits. Then, introduce FPGAs and why they can be useful on the edge. Then, say that good FPGA resource exploitation needs fixed-point and finding the optimal precision (define what optimal precision means in the context of FPGA and NNs.\addressed{}}




% \jgl{Any particular example from previous works about these benefits?\arpan{addressed}}




% \end{Background}


==> PreciseNN/sections/tables/PreciseNN.tex <==

% \end{PreciseNN}


 \begin{table*} 
 \HUGE
 \renewcommand{\arraystretch}{0.65}
\setlength{\tabcolsep}{6pt}
 \resizebox{1\linewidth}{!}{%
 \centering
 \begin{tabular}{!{\vrule width 4pt}c!{\vrule width 1pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 4pt}}

  \specialrule{.1em}{.05em}{.05em} 
 \multicolumn{1}{!{\vrule width 4pt}c!{\vrule width 2pt}}{\textbf{Component}}&\multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Instance}} &\textbf{Feature} &\multicolumn{4}{c!{\vrule width 2pt}}{\textbf{\textit{$<$x=17,y=8$>$}}}
& \multicolumn{4}{c!{\vrule width 2pt}}{\textbf{\textit{$<$x=16,y=10$>$}}} &\textbf{Function} &\multicolumn{6}{c!{\vrule width 4pt}}{\textbf{Feature Predicted}}  \\
\cline{4-9}

 \multicolumn{1}{!{\vrule width 4pt}c!{\vrule width 2pt}}{\textbf{Name}} &\multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Name}} & \textbf{Name}  &\textbf{Value}&{$\mathbf{x}$} &\textbf{$\mathbf{y}$} &\textbf{$\mathbf{x-y}$} &\textbf{Value}&\textbf{$\mathbf{x}$} &\textbf{$\mathbf{y}$} &\textbf{$\mathbf{x-y}$} &\textbf{Detected}&\textbf{$\mathbf{<2,1>}$} &\textbf{$\mathbf{<3,1>}$} &\textbf{$\mathbf{<3,2>}$} &\textbf{$\mathbf{<4,1>}$} &\textbf{$\mathbf{<4,2>}$} &\textbf{$\mathbf{<4,3>}$} \\
 \specialrule{.1em}{.05em}{.05em} 
 \multirow{1}{*}{Memory} &C2\_weights\_V\_0\_U  &width &9 &$\mathbf{-8}$ &$\mathbf{+1}$ &$\textbf{0}$ &6 &$\mathbf{-10}$ &$\mathbf{-4}$ &$\mathbf{0}$ &$\mathbf{x-y}$ &1&2&1&3&2&1 \\ 
 \specialrule{.1em}{.05em}{.05em} 
 %%%%%%%%%%%%Expressions%%%%%%%%%%%%%%%%%%%%%
 \multirow{2}{*}{Expression}
 &\multirow{2}{*}{out\_V\_d0}  &op1 width &1 &$\mathbf{-16}$ &$\mathbf{-7}$ &$\mathbf{-8}$ &1 &$\mathbf{-15}$ &$\mathbf{-9}$ &$\mathbf{-5}$ &1 &1 &1 &1 &1 &1 &1 \\
\cline{3-18}
 &&op2 width &16 &$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$&1 &2 &2 &3 &3 &3\\
 \specialrule{.1em}{.05em}{.05em} 
%%-----------------MUX---------------------------
 \multirow{1}{*}{Multiplexer} &p\_Val2\_40\_0\_reg\_412 &Bits &17 &$\mathbf{0}$ &$\mathbf{+9}$ &$\mathbf{+8}$ &16 &$\mathbf{0}$ &$\mathbf{+6}$ &$\mathbf{+10}$ &$\mathbf{x}$&2 &3 &3 &4 &4 &4\\
 \specialrule{.1em}{.05em}{.05em} 
 %%----------------------------DSP------------------------- 
 \multirow{2}{*}{DSP}&\multirow{2}{*}{nnet\_mac\_muladd\_sc4}  &op1 width &16 &$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$ &1 &2 &2 &3 &3 &3 \\
\cline{3-18}
&&op2 width &10&$\mathbf{-7}$ &$\mathbf{+2}$ &$\mathbf{+1}$ &7 &$\mathbf{-9}$ &$\mathbf{-3}$ &$\mathbf{+1}$ &$\mathbf{x-y+1}$&2 &3 &2 &4 &3 &2\\
 % \hline
 \specialrule{.1em}{.05em}{.05em} 
 \multirow{1}{*}{Register}& C2\_weights\_V\_0\_load\_reg\_1181 &Bits &9&$\mathbf{-8}$ &$\mathbf{+1}$ &$\mathbf{0}$&6 &$\mathbf{-10}$ &$\mathbf{-4}$ &$\mathbf{0}$ &$\mathbf{x-y}$&1 &2 &1 &3 &2 &1\\
% \arrayrulecolor{gray}\cline{2-18}
% & in\_V\_load\_reg\_1186 &Bits &16&$\mathbf{-1}$ &$\mathbf{+8}$ &$\mathbf{+7}$ &15 &$\mathbf{-1}$ &$\mathbf{+5}$ &$\mathbf{+9}$ &$\mathbf{x-1}$&1 &2 &2 &3 &3 &3\\
 \specialrule{.1em}{.05em}{.05em} 
 \end{tabular}
 }
\caption{Brief overview of the HLS C-Synthesis report with Function-Detector and Feature-Predictor output}
 \label{preciseFPGA/table_func_generate}
\end{table*}
% \vspace{0.5 cm}

==> PreciseNN/sections/tables/result_1.tex <==
\begin{table}[h]
\Huge
 \centering
 \resizebox{1\linewidth}{!}{%
 \begin{tabular}{!{\vrule width 2pt}c!{\vrule width 2pt}c!{\vrule width 2pt}c|c|c!{\vrule width 2pt}c|c|c|c|c!{\vrule width 2pt}c!{\vrule width 2pt}}
\specialrule{.1em}{.05em}{.05em} 
\rowcolor{Lightgray}
 \multicolumn{1}{!{\vrule width 2pt}c!{\vrule width 2pt}}{}& & \multicolumn{3}{c!{\vrule width 2pt}}{\textbf{Total Runtime(hrs)}} &  \multicolumn{5}{c!{\vrule width 2pt}}{\textbf{Average Relative Prediction Error(in \%)}}\\
 \cline{3-10}
\rowcolor{Lightgray}
 \multirow{-2}{*}{\textbf{Model}}  &\multirow{-2}{*}{\textbf{\#(Parameters)}}&\textbf{Tool}&\textbf{PreciseNN} &\textbf{Gain(in\%)}&\textbf{FF}&\textbf{LUT}&\textbf{BRAM}&\textbf{DSP} &\textbf{Power}\\
 \specialrule{.1em}{.05em}{.05em} 
1 & 16278 & 223 & 0.205 & 1087 & 3.93 & 4.93 & 3.18 & 4.73 &2.71
\\
\hline
2 & 42704 & 107 & 0.220 & 486 & 4.26 & 3.96 & 2.83 & 4.99 &3.07	
\\
\hline
3 & 14758 & 103 & 0.21 & 490 & 4.65 & 4.24 & 5.44 & 2.89 &2.63\\
\hline
4 & 14822 & 115 & 0.219 & 525 & 4.42 & 3.80 & 5.91 & 3.25 &	2.42	 \\
\hline
5 & 9222 & 111 & 0.223 & 498 & 3.54 & 4.19 & 6.53 & 3.43 &2.64 \\
\hline
6 & 36004 & 132 & 0.227 & 581 & 4.04 & 4.19 & 2.84 & 4.95 &	3.41	\\
\hline
7 & 24114 & 119 & 0.232 & 512 & 6.07 & 4.14 & 2.75 & 4.52 &3.68 \\
\hline
8 & 16498 & 239 & 0.203 & 1177 & 4.24 & 4.92 & 2.89 & 4.92 &	3.72 \\
\specialrule{.1em}{.05em}{.05em} 
\multicolumn{4}{!{\vrule width 2pt}c!{\vrule width 2pt}}{\textbf{Average}} &\textbf{99.83} &\textbf{4.40} &\textbf{4.30}		&\textbf{4.04}		&\textbf{4.21} &\textbf{3.03
}\\
\specialrule{.1em}{.05em}{.05em} 

 \end{tabular}%
 }
\caption{Model Runtime and Resource Prediction metrics}
 \label{preciseFPGA/table_results}
\end{table}

==> Stencil_Precise/ref.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{normError}
Anderson, E., et~al.: LAPACK Users' guide, vol.~9. Siam (1999)

\bibitem{carmichael2018deep}
Carmichael, Z., et~al.: {D}eep {P}ositron: A deep neural network using the
  posit number system. arXiv preprint arXiv:1812.01762  (2018)

\bibitem{chi2018soda}
Chi, Y., Cong, J., Wei, P., Zhou, P.: Soda: stencil with optimized dataflow
  architecture. In: 2018 IEEE/ACM International Conference on Computer-Aided
  Design (ICCAD). pp.~1--8. IEEE (2018)

\bibitem{datta2008stencil}
Datta, K., et~al.: Stencil computation optimization and auto-tuning on
  state-of-the-art multicore architectures. In: Proceedings of the 2008
  ACM/IEEE conference on Supercomputing. p.~4. IEEE Press (2008)

\bibitem{diamantopoulos2018ectalk}
Diamantopoulos, D., Giefers, H., Hagleitner, C.: ec{TALK}: Energy efficient
  coherent transprecision accelerators—the bidirectional long short-term
  memory neural network case. In: 2018 IEEE Symposium in Low-Power and
  High-Speed Chips (COOL CHIPS). pp.~1--3. IEEE (2018)

\bibitem{doms1999nonhydrostatic}
Doms, G., Sch{\"a}ttler, U.: The nonhydrostatic limited-area model {LM}
  (lokal-model) of the {DWD. P}art {I: S}cientific documentation. DWD, GB
  Forschung und Entwicklung  (1999)

\bibitem{de2018designing}
de~Fine~Licht, J., Blott, M., Hoefler, T.: Designing scalable FPGA
  architectures using high-level synthesis. ACM SIGPLAN Notices
  \textbf{53}(1),  403--404 (2018)

\bibitem{finnerty2017reduce}
Finnerty, A., Ratigner, H.: Reduce power and cost by converting from floating
  point to fixed point. In: WP491 (v1. 0) (2017)

\bibitem{gustafson2017beating}
Gustafson, J.L., Yonemoto, I.T.: Beating floating point at its own game: Posit
  arithmetic. Supercomputing Frontiers and Innovations  \textbf{4}(2),  71--86
  (2017)

\bibitem{gysi2015modesto}
Gysi, T., Grosser, T., Hoefler, T.: Modesto: Data-centric analytic optimization
  of complex stencil programs on heterogeneous architectures. In: Proceedings
  of the 29th ACM on International Conference on Supercomputing. pp. 177--186.
  ACM (2015)

\bibitem{iwata1989artificial}
Iwata, A., et~al.: An artificial neural network accelerator using general
  purpose 24 bits floating point digital signal processors. In: IJCNN-89.
  vol.~2, pp. l71--175 (1989)

\bibitem{klower2019posits}
Kl{\"o}wer, M., D{\"u}ben, P.D., Palmer, T.N.: {P}osits as an alternative to
  floats for weather and climate models  (2019)

\bibitem{langroudi2018deep}
Langroudi, S.H.F., Pandit, T., Kudithipudi, D.: Deep learning inference on
  embedded devices: Fixed-point vs posit. In: 2018 1st Workshop on Energy
  Efficient Machine Learning and Cognitive Computing for Embedded Applications
  (EMC2). pp. 19--23. IEEE (2018)

\bibitem{nguyen20103}
Nguyen, A., et~al.: 3.5-{D} blocking optimization for stencil computations on
  modern {CPU}s and {GPU}s. In: Proceedings of the 2010 ACM/IEEE International
  Conference for High Performance Computing, Networking, Storage and Analysis.
  pp. 1--13. IEEE Computer Society (2010)

\bibitem{parker2014understanding}
Parker, M.: {U}nderstanding peak floating-point performance claims. Technical
  White Paper WP-012220-1.0  (2014)

\bibitem{sano2014multi}
Sano, K., Hatsuda, Y., Yamamoto, S.: Multi-FPGA accelerator for scalable
  stencil computation with constant memory bandwidth. IEEE Transactions on
  Parallel and Distributed Systems  \textbf{25}(3),  695--705 (2014)

\bibitem{singhReview}
Singh, G., et~al.: A review of near-memory computing architectures:
  {O}pportunities and challenges. In: 2018 21st Euromicro Conference on Digital
  System Design (DSD). pp. 608--617. IEEE (2018)
  
\bibitem{NAPEL}
Singh, G., et~al.: {NAPEL}: Near-Memory Computing Application Performance Prediction via Ensemble Learning. In {\em Proceedings of the 56th Annual Design Automation Conference
  2019}, DAC '19, pages 27:1--27:6, New York, NY, USA, 2019. ACM.

\bibitem{7582502}
{Waidyasooriya}, H.M., et~al.: {O}pen{CL-B}ased {FPGA-P}latform for {S}tencil
  {C}omputation and {I}ts {O}ptimization {M}ethodology. IEEE Transactions on
  Parallel and Distributed Systems  \textbf{28}(5),  1390--1402 (May 2017)

\bibitem{stencilOnPOWER8}
Xu, J., et~al.: {P}erformance {T}uning and {A}nalysis for {S}tencil-{B}ased
  {A}pplications on {POWER}8 {P}rocessor. ACM Transactions on Architecture and
  Code Optimization (TACO)  \textbf{15}(4), ~41 (2018)

\end{thebibliography}

==> Stencil_Precise/system.tex <==
\begin{table}
    \caption{System configuration for the host CPU system.}
    \label{tab:low_precision/systemparameters}
    \centering
    \resizebox{\textwidth}{!}{% use resizebox with textwidth
    \begin{tabular}{c|c|c|c|c}
    \toprule
     \textbf{Architecture} & \textbf{Physical Cores} &\textbf{Frequency}& \textbf{On-chip Memory (Per Core)} & \textbf{Off-chip Memory}\\
     \hline
     IBM Power9& 16-cores/socket; (SMT4)  & Min: 2.3GHz & L1-cache: 32KiB & DDR4: \\
      & &Max: 3.8GHz & L2-cache: 256KiB & 16x32GiB RDIMM\\
      &  & & L3-cache: 10MiB  & 2666MHz\\
     
     \bottomrule
    
    \end{tabular}}
\end{table}

==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
% \begin{singlespace}
% \small
% \bibliography{refs}
% \bibliographystyle{plain}
% %% Get rid of 'no \citation' error in certain compilers. Alin Tomescu (2015).
% %\nocite{*} %% 
% \end{singlespace}


==> cover.tex <==
% -*-latex-*-
% 
% For questions, comments, concerns or complaints:
% thesis@mit.edu
% 
%
% $Log: cover.tex,v $
% Revision 1.8.1 2015/08/14 8:58:00  alinush
% Citations in .tex files now point to dummy entries in main.bib
% Font smoothness issues solved. Created an easy to use Makefile.
%
% Revision 1.8  2008/05/13 15:02:15  jdreed
% Degree month is June, not May.  Added note about prevdegrees.
% Arthur Smith's title updated
%
% Revision 1.7  2001/02/08 18:53:16  boojum
% changed some \newpages to \cleardoublepages
%
% Revision 1.6  1999/10/21 14:49:31  boojum
% changed comment referring to documentstyle
%
% Revision 1.5  1999/10/21 14:39:04  boojum
% *** empty log message ***
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.3  93/05/17  17:06:29  starflt
% Added acknowledgements section (suggested by tompalka)
% 
% Revision 1.2  92/04/22  13:13:13  epeisach
% Fixes for 1991 course 6 requirements
% Phrase "and to grant others the right to do so" has been added to 
% permission clause
% Second copy of abstract is not counted as separate pages so numbering works
% out
% 
% Revision 1.1  92/04/22  13:08:20  epeisach

% NOTE:
% These templates make an effort to conform to the MIT Thesis specifications,
% however the specifications can change.  We recommend that you verify the
% layout of your title page with your thesis advisor and/or the MIT 
% Libraries before printing your final copy.

% If you wish to list your previous degrees on the cover page, use the 
% previous degrees command:
%       \prevdegrees{A.A., Harvard University (1985)}
% You can use the \\ command to list multiple previous degrees
%       \prevdegrees{B.S., University of California (1978) \\
%                    S.M., Massachusetts Institute of Technology (1981)}


% Make the titlepage based on the above information.  If you need
% something special and can't use the standard form, you can specify
% the exact text of the titlepage yourself.  Put it in a titlepage
% environment and leave blank lines where you want vertical space.
% The spaces will be adjusted to fill the entire page.  The dotted
% lines for the signatures are made with the \signature command.


% The abstractpage environment sets up everything on the page except
% the text itself.  The title and other header material are put at the
% top of the page, and the supervisors are listed at the bottom.  A
% new page is begun both before and after.  Of course, an abstract may
% be more than one page itself.  If you need more control over the
% format of the page, you can use the abstract environment, which puts
% the word "Abstract" at the beginning and single spaces its text.

%% You can either \input (*not* \include) your abstract file, or you can put
%% the text of the abstract directly between the \begin{abstractpage} and
%% \end{abstractpage} commands.

%\null\vfill
%\noindent
%Copyright 2010 -- Example Cooperation\\
%Some text ...

% Uncomment the next line if you do NOT want a page number on your
% abstract and acknowledgments pages.
% \pagestyle{empty}
% \setcounter{savepage}{\thepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

% Additional copy: start a new page, and reset the page number.  This way,
% the second copy of the abstract is not counted as separate pages.
% Uncomment the next 6 lines if you need two copies of the abstract
% page.
% \setcounter{page}{\thesavepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

% \cleardoublepage

% \input{ack}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-

